Introduction into Calculus over Division Ring

Based on twin representations of division ring in an Abelian group I consider $D$\Hyph vector spaces over division ring. Morphism of $D$\Hyph vector spaces is linear map of $D$\Hyph vector spaces. I consider derivative of function $f$ of continuous division ring as linear map the most close to function $f$. I explore expansion of map into Taylor series and method to find solution of differential equation. The norm in $D$\Hyph vector space allows considering of continuous mapping of $D$\Hyph vector spaces. Differential of mapping $f$ of $D$\Hyph vector spaces is defined as linear mapping the most close to map $f$.

==> 0812.4763.tex <==
%auto-ignore
\def\PrintBook{}
\input{Commands}
\def\BookNumber{0812.4763}
\xRefDef{0701.238}

\makeatletter
\def\@part[#1]#2{%
  \ifnum \c@secnumdepth >-2\relax \refstepcounter{part}%
    %\addcontentsline{toc}{part}{\partname\ \thepart.
    %    \protect\enspace\protect\noindent#1}%
	\addcontentsline{toc}{part}{\partname\ \thepart. \ #1}%
  \else
    \addcontentsline{toc}{part}{#1}\fi
  \begingroup\centering
  \ifnum \c@secnumdepth >-2\relax
       {\fontsize{\@xviipt}{22}\bfseries
         \partname\ \thepart} \vskip 20\p@ \fi
  \fontsize{\@xxpt}{25}\bfseries
      #1\vfil\vfil\endgroup \newpage\thispagestyle{empty}}

\def\@spart#1{
  %\addcontentsline{toc}{part}{\protect\noindent#1}%
  \addcontentsline{toc}{part}{\partname\ \thepart. \ #1}%
  \begingroup\centering
  \fontsize{\@xxpt}{25}\bfseries
     #1\vfil\vfil\endgroup \newpage\thispagestyle{empty}}
\makeatother

\DefEq
{
\maketitle
\tableofcontents
\Input{Preface.\BookNumber}
\Input{Convention}
\PartA
\label{part: Linear Algebra over Division Ring}
\Input{Linear.Map}
\Input{Ring.Linear.Map}
\Input{Vector.Linear.Map}
\PartB
\label{part: Calculus over Division Ring}
\Input{Differential}
\Input{Differential.Vector}
\Input{Quaternion}
\Input{Second.Differential}
\Input{Second.Differential.Vector}
\Input{Biblio}
\Input{Index}
\Input{Symbol}
}
{contents}

\def\texTitle{ Introduction into Calculus over Division Ring }
\def\texAuthors{ Aleks Kleyn }
\def\texComments
{
English text - 97 pages; Russian text - 103 pages.
Version 3: Considered definition of Taylor series and integral.
}
%\def\texSubjClass{ Differential Geometry, General Relativity }
\def\texAbstract
{
Based on twin representations of division ring in
an Abelian group I consider $D$\Hyph vector spaces over division ring.
Morphism of $D$\Hyph vector spaces is linear map of $D$\Hyph vector spaces.

I consider derivative of function $f$ of continuous division ring
as linear map the most close to
function $f$.
I explore expansion of map into
Taylor series and method
to find solution of differential equation.

The norm in $D$\Hyph vector space allows considering of
continuous map of $D$\Hyph vector spaces.
Differential of map $f$ of $D$\Hyph vector spaces
is defined as linear map the most close to
map $f$.
}

\def\JRef{
Clifford Analysis, Clifford Algebras and their applications,
Issue 4, Vol 7, pages 291 - 355, 2012
}



==> Algebra.Quaternion.Eq.tex <==
%auto-ignore

\DefEquation
{
\begin{array}{|c|r|r|r|r|}
\hline
&\Vector e_{\giA}&\Vector e_{\gi 2}&\Vector e_{\gi 3}
\\
\hline
\Vector e_{\giA}&-\Vector e_{\gi 0}&\Vector e_{\gi 3}&-\Vector e_{\gi 2}
\\
\hline
\Vector e_{\gi 2}&-\Vector e_{\gi 3}&-\Vector e_{\gi 0}&\Vector e_{\giA}
\\
\hline
\Vector e_{\gi 3}&\Vector e_{\gi 2}&-\Vector e_{\giA}&-\Vector e_{\gi 0}
\\
\hline
\end{array}
}
{product in quaternion, table}

\DefEq
{
\[
\begin{array}{r@{\ }rr@{\ }rr@{\ }rr@{\ }r}
C_{\gi{00}}^{\gi 0}=&1&
C_{\gi{01}}^{\giA}=&1&
C_{\gi{02}}^{\gi 2}=&1&
C_{\gi{03}}^{\gi 3}=&1
\\
\VirtVar
C_{\gi{10}}^{\giA}=&1&
C_{\gi{11}}^{\gi 0}=&-1&
C_{\gi{12}}^{\gi 3}=&1&
C_{\gi{13}}^{\gi 2}=&-1
\\
\VirtVar
C_{\gi{20}}^{\gi 2}=&1&
C_{\gi{21}}^{\gi 3}=&-1&
C_{\gi{22}}^{\gi 0}=&-1&
C_{\gi{23}}^{\giA}=&1
\\
\VirtVar
C_{\gi{30}}^{\gi 3}=&1&
C_{\gi{31}}^{\gi 2}=&1&
C_{\gi{32}}^{\giA}=&-1&
C_{\gi{33}}^{\gi 0}=&-1
\end{array}
\]
}
{structural constants, quaternion}

\DefEq
{
\begin{equation}
\begin{array}{r@{}l}
\FM 00&=\FC krC_{\gi{k0}}^{\gi p}C_{\gi{pr}}^{\gi 0}
\\&\VirtVar
=\FC 00C_{\gi{00}}^{\gi 0}C_{\gi{00}}^{\gi 0}%1 1
+\FC 11C_{\gi{10}}^{\giA}C_{\gi{11}}^{\gi 0}%1 -1
+\FC 22C_{\gi{20}}^{\gi 2}C_{\gi{22}}^{\gi 0}%1 -1
+\FC 33C_{\gi{30}}^{\gi 3}C_{\gi{33}}^{\gi 0}%1 -1
\\&\VirtVar
=\FC 00
-\FC 11
-\FC 22
-\FC 33
\end{array}
\EqLabel{Standard components of linear function, 1, 0, 0, quaternion}
\end{equation}
\begin{equation}
\begin{array}{r@{}l}
\FM 10&=\FC krC_{\gi{k0}}^{\gi p}C_{\gi{pr}}^{\giA}
\\&\VirtVar
=\FC 01C_{\gi{00}}^{\gi 0}C_{\gi{01}}^{\giA}%1 1
+\FC 10C_{\gi{10}}^{\giA}C_{\gi{10}}^{\giA}%1 1
+\FC 23C_{\gi{20}}^{\gi 2}C_{\gi{23}}^{\giA}%1 1
+\FC 32C_{\gi{30}}^{\gi 3}C_{\gi{32}}^{\giA}%1 -1
\\&\VirtVar
=\FC 01
+\FC 10
+\FC 23
-\FC 32
\end{array}
\EqLabel{Standard components of linear function, 1, 0, 1, quaternion}
\end{equation}
\begin{equation}
\begin{array}{r@{}l}
\FM 20&=\FC krC_{\gi{k0}}^{\gi p}C_{\gi{pr}}^{\gi 2}
\\&\VirtVar
=\FC 02C_{\gi{00}}^{\gi 0}C_{\gi{02}}^{\gi 2}%1 1
+\FC 13C_{\gi{10}}^{\giA}C_{\gi{13}}^{\gi 2}%1 -1
+\FC 20C_{\gi{20}}^{\gi 2}C_{\gi{20}}^{\gi 2}%1 1
+\FC 31C_{\gi{30}}^{\gi 3}C_{\gi{31}}^{\gi 2}%1 1
\\&\VirtVar
=\FC 02
-\FC 13
+\FC 20
+\FC 31
\end{array}
\EqLabel{Standard components of linear function, 1, 0, 2, quaternion}
\end{equation}
\begin{equation}
\begin{array}{r@{}l}
\FM 30&=\FC krC_{\gi{k0}}^{\gi p}C_{\gi{pr}}^{\gi 3}
\\&\VirtVar
=\FC 03C_{\gi{00}}^{\gi 0}C_{\gi{03}}^{\gi 3}%1 1
+\FC 12C_{\gi{10}}^{\giA}C_{\gi{12}}^{\gi 3}%1 1
+\FC 21C_{\gi{20}}^{\gi 2}C_{\gi{21}}^{\gi 3}%1 -1
+\FC 30C_{\gi{30}}^{\gi 3}C_{\gi{30}}^{\gi 3}%1 1
\\&\VirtVar
=\FC 03
+\FC 12
-\FC 21
+\FC 30
\end{array}
\EqLabel{Standard components of linear function, 1, 0, 3, quaternion}
\end{equation}
\begin{equation}
\begin{array}{r@{}l}
\FM 01&=\FC krC_{\gi{k1}}^{\gi p}C_{\gi{pr}}^{\gi 0}
\\&\VirtVar
=\FC 01C_{\gi{01}}^{\giA}C_{\gi{11}}^{\gi 0}%1 -1
+\FC 10C_{\gi{11}}^{\gi 0}C_{\gi{00}}^{\gi 0}%-1 1
+\FC 23C_{\gi{21}}^{\gi 3}C_{\gi{33}}^{\gi 0}%-1 -1
+\FC 32C_{\gi{31}}^{\gi 2}C_{\gi{22}}^{\gi 0}%1 -1
\\&\VirtVar
=-\FC 01
-\FC 10
+\FC 23
-\FC 32
\end{array}
\EqLabel{Standard components of linear function, 1, 1, 0, quaternion}
\end{equation}
\begin{equation}
\begin{array}{r@{}l}
\FM 11&=\FC krC_{\gi{k1}}^{\gi p}C_{\gi{pr}}^{\giA}
\\&\VirtVar
=\FC 00C_{\gi{01}}^{\giA}C_{\gi{10}}^{\giA}%1 1
+\FC 11C_{\gi{11}}^{\gi 0}C_{\gi{01}}^{\giA}%-1 1
+\FC 22C_{\gi{21}}^{\gi 3}C_{\gi{32}}^{\giA}%-1 -1
+\FC 33C_{\gi{31}}^{\gi 2}C_{\gi{23}}^{\giA}%1 1
\\&\VirtVar
=\FC 00
-\FC 11
+\FC 22
+\FC 33
\end{array}
\EqLabel{Standard components of linear function, 1, 1, 1, quaternion}
\end{equation}
\begin{equation}
\begin{array}{r@{}l}
\FM 21&=\FC krC_{\gi{k1}}^{\gi p}C_{\gi{pr}}^{\gi 2}
\\&\VirtVar
=\FC 03C_{\gi{01}}^{\giA}C_{\gi{13}}^{\gi 2}%1 -1
+\FC 12C_{\gi{11}}^{\gi 0}C_{\gi{02}}^{\gi 2}%-1 1
+\FC 21C_{\gi{21}}^{\gi 3}C_{\gi{31}}^{\gi 2}%-1 1
+\FC 30C_{\gi{31}}^{\gi 2}C_{\gi{20}}^{\gi 2}%1 1
\\&\VirtVar
=-\FC 03
-\FC 12
-\FC 21
+\FC 30
\end{array}
\EqLabel{Standard components of linear function, 1, 1, 2, quaternion}
\end{equation}
\begin{equation}
\begin{array}{r@{}l}
\FM 31&=\FC krC_{\gi{k1}}^{\gi p}C_{\gi{pr}}^{\gi 3}
\\&\VirtVar
=\FC 02C_{\gi{01}}^{\giA}C_{\gi{12}}^{\gi 3}%1 1
+\FC 13C_{\gi{11}}^{\gi 0}C_{\gi{03}}^{\gi 3}%-1 1
+\FC 20C_{\gi{21}}^{\gi 3}C_{\gi{30}}^{\gi 3}%-1 1
+\FC 31C_{\gi{31}}^{\gi 2}C_{\gi{21}}^{\gi 3}%1 -1
\\&\VirtVar
=\FC 02
-\FC 13
-\FC 20
-\FC 31
\end{array}
\EqLabel{Standard components of linear function, 1, 1, 3, quaternion}
\end{equation}
\begin{equation}
\begin{array}{r@{}l}
\FM 02&=\FC krC_{\gi{k2}}^{\gi p}C_{\gi{pr}}^{\gi 0}
\\&\VirtVar
=\FC 02C_{\gi{02}}^{\gi 2}C_{\gi{22}}^{\gi 0}%1 -1
+\FC 13C_{\gi{12}}^{\gi 3}C_{\gi{33}}^{\gi 0}%1 -1
+\FC 20C_{\gi{22}}^{\gi 0}C_{\gi{00}}^{\gi 0}%-1 1
+\FC 31C_{\gi{32}}^{\giA}C_{\gi{11}}^{\gi 0}%-1 -1
\\&\VirtVar
=-\FC 02
-\FC 13
-\FC 20
+\FC 31
\end{array}
\EqLabel{Standard components of linear function, 1, 2, 0, quaternion}
\end{equation}
\begin{equation}
\begin{array}{r@{}l}
\FM 12&=\FC krC_{\gi{k2}}^{\gi p}C_{\gi{pr}}^{\giA}
\\&\VirtVar
=\FC 03C_{\gi{02}}^{\gi 2}C_{\gi{23}}^{\giA}%1 1
+\FC 12C_{\gi{12}}^{\gi 3}C_{\gi{32}}^{\giA}%1 -1
+\FC 21C_{\gi{22}}^{\gi 0}C_{\gi{01}}^{\giA}%-1 1
+\FC 30C_{\gi{32}}^{\giA}C_{\gi{10}}^{\giA}%-1 1
\\&\VirtVar
=\FC 03
-\FC 12
-\FC 21
-\FC 30
\end{array}
\EqLabel{Standard components of linear function, 1, 2, 1, quaternion}
\end{equation}
\begin{equation}
\begin{array}{r@{}l}
\FM 22&=\FC krC_{\gi{k2}}^{\gi p}C_{\gi{pr}}^{\gi 2}
\\&\VirtVar
=\FC 00C_{\gi{02}}^{\gi 2}C_{\gi{20}}^{\gi 2}%1 1
+\FC 11C_{\gi{12}}^{\gi 3}C_{\gi{31}}^{\gi 2}%1 1
+\FC 22C_{\gi{22}}^{\gi 0}C_{\gi{02}}^{\gi 2}%-1 1
+\FC 33C_{\gi{32}}^{\giA}C_{\gi{13}}^{\gi 2}%-1 -1
\\&\VirtVar
=\FC 00
+\FC 11
-\FC 22
+\FC 33
\end{array}
\EqLabel{Standard components of linear function, 1, 2, 2, quaternion}
\end{equation}
\begin{equation}
\begin{array}{r@{}l}
\FM 32&=\FC krC_{\gi{k2}}^{\gi p}C_{\gi{pr}}^{\gi 3}
\\&\VirtVar
=\FC 01C_{\gi{02}}^{\gi 2}C_{\gi{21}}^{\gi 3}%1 -1
+\FC 10C_{\gi{12}}^{\gi 3}C_{\gi{30}}^{\gi 3}%1 1
+\FC 23C_{\gi{22}}^{\gi 0}C_{\gi{03}}^{\gi 3}%-1 1
+\FC 32C_{\gi{32}}^{\giA}C_{\gi{12}}^{\gi 3}%-1 1
\\&\VirtVar
=-\FC 01
+\FC 10
-\FC 23
-\FC 32
\end{array}
\EqLabel{Standard components of linear function, 1, 2, 3, quaternion}
\end{equation}
\begin{equation}
\begin{array}{r@{}l}
\FM 03&=\FC krC_{\gi{k3}}^{\gi p}C_{\gi{pr}}^{\gi 0}
\\&\VirtVar
=\FC 03C_{\gi{03}}^{\gi 3}C_{\gi{33}}^{\gi 0}%1 -1
+\FC 12C_{\gi{13}}^{\gi 2}C_{\gi{22}}^{\gi 0}%-1 -1
+\FC 21C_{\gi{23}}^{\giA}C_{\gi{11}}^{\gi 0}%1 -1
+\FC 30C_{\gi{33}}^{\gi 0}C_{\gi{00}}^{\gi 0}%-1 1
\\&\VirtVar
=-\FC 03
+\FC 12
-\FC 21
-\FC 30
\end{array}
\EqLabel{Standard components of linear function, 1, 3, 0, quaternion}
\end{equation}
\begin{equation}
\begin{array}{r@{}l}
\FM 13&=\FC krC_{\gi{k3}}^{\gi p}C_{\gi{pr}}^{\giA}
\\&\VirtVar
=\FC 02C_{\gi{03}}^{\gi 3}C_{\gi{32}}^{\giA}%1 -1
+\FC 13C_{\gi{13}}^{\gi 2}C_{\gi{23}}^{\giA}%-1 1
+\FC 20C_{\gi{23}}^{\giA}C_{\gi{10}}^{\giA}%1 1
+\FC 31C_{\gi{33}}^{\gi 0}C_{\gi{01}}^{\giA}%-1 1
\\&\VirtVar
=-\FC 02
-\FC 13
+\FC 20
-\FC 31
\end{array}
\EqLabel{Standard components of linear function, 1, 3, 1, quaternion}
\end{equation}
\begin{equation}
\begin{array}{r@{}l}
\FM 23&=\FC krC_{\gi{k3}}^{\gi p}C_{\gi{pr}}^{\gi 2}
\\&\VirtVar
=\FC 01C_{\gi{03}}^{\gi 3}C_{\gi{31}}^{\gi 2}%1 1
+\FC 10C_{\gi{13}}^{\gi 2}C_{\gi{20}}^{\gi 2}%-1 1
+\FC 23C_{\gi{23}}^{\giA}C_{\gi{13}}^{\gi 2}%1 -1
+\FC 32C_{\gi{33}}^{\gi 0}C_{\gi{02}}^{\gi 2}%-1 1
\\&\VirtVar
=\FC 01
-\FC 10
-\FC 23
-\FC 32
\end{array}
\EqLabel{Standard components of linear function, 1, 3, 2, quaternion}
\end{equation}
\begin{equation}
\begin{array}{r@{}l}
\FM 33&=\FC krC_{\gi{k3}}^{\gi p}C_{\gi{pr}}^{\gi 3}
\\&\VirtVar
=\FC 00C_{\gi{03}}^{\gi 3}C_{\gi{30}}^{\gi 3}%1 1
+\FC 11C_{\gi{13}}^{\gi 2}C_{\gi{21}}^{\gi 3}%-1 -1
+\FC 22C_{\gi{23}}^{\giA}C_{\gi{12}}^{\gi 3}%1 1
+\FC 33C_{\gi{33}}^{\gi 0}C_{\gi{03}}^{\gi 3}%-1 1
\\&\VirtVar
=\FC 00
+\FC 11
+\FC 22
-\FC 33
\end{array}
\EqLabel{Standard components of linear function, 1, 3, 3, quaternion}
\end{equation}
}
{Standard components of linear function, 1, quaternion}

\DefEq
{
\begin{equation}
\EqLabel{quaternion linear system, 1, 0}
\left\{
\begin{array}{r@{}r}
\FM 00=&
\FC 00
-\FC 11
-\FC 22
-\FC 33
\\
\VirtVar
\FM 11=&
\FC 00
-\FC 11
+\FC 22
+\FC 33
\\
\VirtVar
\FM 22=&
\FC 00
+\FC 11
-\FC 22
+\FC 33
\\
\VirtVar
\FM 33=&
\FC 00
+\FC 11
+\FC 22
-\FC 33
\end{array}
\right.
\end{equation}
\begin{equation}
\EqLabel{quaternion linear system, 1, 1}
\left\{
\begin{array}{r@{}r}
\FM 10=&
\FC 01
+\FC 10
+\FC 23
-\FC 32
\\
\VirtVar
\FM 01=&
-\FC 01
-\FC 10
+\FC 23
-\FC 32
\\
\VirtVar
\FM 32=&
-\FC 01
+\FC 10
-\FC 23
-\FC 32
\\
\VirtVar
\FM 23=&
\FC 01
-\FC 10
-\FC 23
-\FC 32
\end{array}
\right.
\end{equation}
\begin{equation}
\EqLabel{quaternion linear system, 1, 2}
\left\{
\begin{array}{r@{}r}
\FM 20=&
\FC 02
-\FC 13
+\FC 20
+\FC 31
\\
\VirtVar
\FM 31=&
\FC 02
-\FC 13
-\FC 20
-\FC 31
\\
\VirtVar
\FM 02=&
-\FC 02
-\FC 13
-\FC 20
+\FC 31
\\
\VirtVar
\FM 13=&
-\FC 02
-\FC 13
+\FC 20
-\FC 31
\end{array}
\right.
\end{equation}
\begin{equation}
\EqLabel{quaternion linear system, 1, 3}
\left\{
\begin{array}{r@{}r}
\FM 30=&
\FC 03
+\FC 12
-\FC 21
+\FC 30
\\
\VirtVar
\FM 21=&
-\FC 03
-\FC 12
-\FC 21
+\FC 30
\\
\VirtVar
\FM 12=&
\FC 03
-\FC 12
-\FC 21
-\FC 30
\\
\VirtVar
\FM 03=&
-\FC 03
+\FC 12
-\FC 21
-\FC 30
\end{array}
\right.
\end{equation}
}
{quaternion linear system, 1}

\DefEq
{
\eqref{eq: Standard components of linear function, 1, 0, 0, quaternion},
\eqref{eq: Standard components of linear function, 1, 1, 1, quaternion},
\eqref{eq: Standard components of linear function, 1, 2, 2, quaternion},
\eqref{eq: Standard components of linear function, 1, 3, 3, quaternion}
}
{quaternion linear system ref, 0}


\DefEq
{
\eqref{eq: Standard components of linear function, 1, 0, 1, quaternion},
\eqref{eq: Standard components of linear function, 1, 1, 0, quaternion},
\eqref{eq: Standard components of linear function, 1, 2, 3, quaternion},
\eqref{eq: Standard components of linear function, 1, 3, 2, quaternion}
}
{quaternion linear system ref, 1}


\DefEq
{
\eqref{eq: Standard components of linear function, 1, 0, 2, quaternion},
\eqref{eq: Standard components of linear function, 1, 1, 3, quaternion},
\eqref{eq: Standard components of linear function, 1, 2, 0, quaternion},
\eqref{eq: Standard components of linear function, 1, 3, 1, quaternion}
}
{quaternion linear system ref, 2}


\DefEq
{
\eqref{eq: Standard components of linear function, 1, 0, 3, quaternion},
\eqref{eq: Standard components of linear function, 1, 1, 2, quaternion},
\eqref{eq: Standard components of linear function, 1, 2, 1, quaternion},
\eqref{eq: Standard components of linear function, 1, 3, 0, quaternion}
}
{quaternion linear system ref, 3}

\DefEquation
{
\left(
\begin{array}{r}
\FM 00
\\
\FM 11
\\
\FM 22
\\
\FM 33
\end{array}
\right)
=
\left(
\begin{array}{rrrr}
1&-1&-1&-1
\\
1&-1&1&1
\\
1&1&-1&1
\\
1&1&1&-1
\end{array}
\right)
\left(
\begin{array}{r}
\FC 00
\\
\FC 11
\\
\FC 22
\\
\FC 33
\end{array}
\right)
}
{quaternion matrix 0}

\DefEquation
{
\left(
\begin{array}{r}
\FM 10
\\
\FM 01
\\
\FM 32
\\
\FM 23
\end{array}
\right)
=
\left(
\begin{array}{rrrr}
1&1&1&-1
\\
-1&-1&1&-1
\\
-1&1&-1&-1
\\
1&-1&-1&-1
\end{array}
\right)
\left(
\begin{array}{r}
\FC 01
\\
\FC 10
\\
\FC 23
\\
\FC 32
\end{array}
\right)
}
{quaternion matrix 1}

\DefEquation
{
\left(
\begin{array}{r}
\FM 20
\\
\FM 31
\\
\FM 02
\\
\FM 13
\end{array}
\right)
=
\left(
\begin{array}{rrrr}
1&-1&1&1
\\
1&-1&-1&-1
\\
-1&-1&-1&1
\\
-1&-1&1&-1
\end{array}
\right)
\left(
\begin{array}{r}
\FC 02
\\
\FC 13
\\
\FC 20
\\
\FC 31
\end{array}
\right)
}
{quaternion matrix 2}

\DefEquation
{
\left(
\begin{array}{r}
\FM 30
\\
\FM 21
\\
\FM 12
\\
\FM 03
\end{array}
\right)
=
\left(
\begin{array}{rrrr}
1&1&-1&1
\\
-1&-1&-1&1
\\
1&-1&-1&-1
\\
-1&1&-1&-1
\end{array}
\right)
\left(
\begin{array}{r}
\FC 03
\\
\FC 12
\\
\FC 21
\\
\FC 30
\end{array}
\right)
}
{quaternion matrix 3}



==> Biblio.English.tex <==
%auto-ignore
\OpenBiblio

%22. A.G. Kurosh, Lectures on General Algebra, Chelsea, New York, 1963

\BiblioItem{Einstein: Electrodynamics of Moving Bodies}
{
Albert Einstein,
On the Electrodynamics of Moving Bodies, 1905,
\\
The Principle of Relativity: A Collection of Original
Memoirs on the Special and General Theory of Relativity , 37 - 65,
\\
Courier Dover Publications, 1952; ISBN-13: 978-0486600819
\\
Zur Elektrodynamik der bewegter K\"orper. Ann. Phys., 1905, 17, 891-921. 
}%

\BiblioItem{Einstein: On the Relativity Principle}
{
Albert Einstein,
On the Relativity Principle and the Conclusions Drawn from It, 1907,
\\
The Collected Papers of Albert Einstein, Volume 2:
The Swiss Years: Writings, 1900-1909. English translation. 252 - 311.
\\
Anna Beck, translator; Peter Havas, consultant.
Princeton University Press, 1989; ISBN-13: 9780691085494
\\
\"Uber das Relativit\"atsprinzip und die aus demselben gezogenen Folgerungen. 
Jahrb. d. Radioaktivit\"at u. Elektronik, 1907, 4, 411-462. 
}%

\BiblioItem{Einstein: Foundations of general relativity}
{
Albert Einstein,
Die Grundlage der allgemeinen Relativit\"atstheorie,
Ann. Phys., 1916, {\bf 49}, 769 - 822,\\
Einstein's Annalen Papers: The Complete Collection 1901-1922,
edited by J\"urgen Renn, 517 - 571,\\
Wiley-VCH Verlag GmbH \& Co. KGaA, 2005
}%

\BiblioItem{Einstein: Geometry and Experience}
{
Albert Einstein, Geometry and Experience, (1921)\\
Albert Einstein, Sidelights on Relativity, 25 - 56,\\
Courier Dover Publications, 1983
}%

\BiblioItem{Einstein: Main problems of general relativity}
{
Albert Einstein,
Grundgedanken und Probleme der Relativit\"atstheorie, (1923),\\
Nobelstiftelsen, Les Prix Nobel en 1921 - 1922,
Imprimerie Royale, Stockholm, 1923
}%

\BiblioItem{Einstein: Noneuclidean Geometry and Physics}
{
Albert Einstein,
Nichtenklidische Geometrie in der Physik Neue Rundschan, (1925)
Berlin, S. 16 - 20
}%

\BiblioItem{Einstein: Isaak Newton}
{
Albert Einstein,
Isaak Newton, 1927,
Out of My Later Years, 
Citadel Press, 1995, 219 - 223
}%

\BiblioItem{Einstein: On Science}
{
Albert Einstein,
On Science, 
Cosmic Religion, with Other Opinions and Aphorisms,142 - 146,
New York, 1931, 97 - 103
}%

\BiblioItem{Einstein: Autobiographical Notes}
{
Albert Einstein,
Autobiographical Notes, 1949,\\
Paul A. Schilpp, editor, Albert Einstein: Philosopher-Scientist,
Evanston, 
Illinois, The Library of Living Philosophers, 1949, 1 - 95
}%

\BiblioItem{Feynman 1}
{
Richard Phillips Feynman, Robert B. Leighton, Matthew Linzee Sands.
The Feynman lectures on physics: Volume 1.
Mainly Mechanics, Radiation, and Heat.
Addison\Hyph Wesley, 1965.
}%

\BiblioItem{0538731877}
{
James Shipman, Jerry D. Wilson and Aaron Todd.
Introduction to Physical Science.
Cengage Learning, 2009; ISBN 0538731877.
}%

\BiblioItem{Cite: 104}
{
Cite 104, Source unknown
}%

\BiblioItem{Ghez}
{
Ghez et al.,
The First Measurement of Spectral Lines in a Short-Period Star Bound to the Galaxy's Central Black Hole: A Paradox of Youth,
\href{http://www.journals.uchicago.edu/ApJ/journal/issues/ApJL/v586n2/16990/brief/16990.abstract.html}{ApJL, 586, L127} (2003),
eprint \href{http://arxiv.org/abs/astro-ph/0302299}{arXiv:astro-ph/0302299} (2003)
}%

\BiblioItem{Schodel}
{
R. Sch\"odel et al.,
A star in a 15.2-year orbit around the supermassive black hole at the centre of the Milky Way,
\href{http://www.nature.com/cgi-taf/DynaPage.taf?file=/nature/journal/v419/n6908/abs/nature01121_fs.html}{Nature 419, 694} (2002)
}%

\BiblioItem{Mielke}
{
Eckehard W. Mielke, Affine generalization of the Komar complex of general relativity,
\href{http://prola.aps.org/searchabstract/PRD/v63/i4/e044018}{Phys. Rev. D 63, 044018} (2001)
}%

\BiblioItem{Obukhov}
{
Yu. N. Obukhov and J. G. Pereira, Metric\hyph affine approach to teleparallel gravity,
\href{http://scitation.aip.org/getabs/servlet/GetabsServlet?prog=normal&id=PRVDAQ000067000004044016000001&idtype=cvips&gifs=Yes}
{Phys. Rev. D 67, 044016} (2003),
eprint \href{http://arxiv.org/abs/gr-qc/0212080}{arXiv:gr-qc/0212080} (2002)
}%

\BiblioItem{Sardanashvily}
{
Giovanni Giachetta, Gennadi Sardanashvily, Dirac Equation in Gauge and Affine-Metric Gravitation Theories,
eprint \href{http://arxiv.org/abs/gr-qc/9511035}{arXiv:gr-qc/9511035} (1995)
}%

\BiblioItem{Gauge}
{
Frank Gronwald and Friedrich W. Hehl, On the Gauge Aspects of Gravity, eprint
\href{http://arxiv.org/abs/gr-qc/9602013}{arXiv:gr-qc/9602013} (1996)
}%

\BiblioItem{Neeman}
{
Yuval Neeman, Friedrich W. Hehl, Test Matter in a Spacetime with Nonmetricity, eprint
\href{http://arxiv.org/abs/gr-qc/9604047}{arXiv:gr-qc/9604047} (1996)
}%

\BiblioItem{torsion}
{
F. W. Hehl, P. von der Heyde, G. D. Kerlick, and J. M. Nester,
General relativity with spin and torsion: Foundations and prospects,\\
\href{http://prola.aps.org/abstract/RMP/v48/i3/p393_1}{Rev. Mod. Phys. 48, 393} (1976)
}%

\BiblioItem{Megged}
{
O. Megged, Post-Riemannian Merger of Yang-Mills Interactions with Gravity,
eprint \href{http://arxiv.org/abs/hep-th/0008135}{arXiv:hep-th/0008135} (2001)
}%

%\BiblioItem{Hehl}
%{
%Friedrich W. Hehl, Uwe Muench,
%eprint \href{http://arxiv.org/abs/gr-qc/9708007}{arXiv:gr-qc/9708007} (1997)
%}%

\BiblioItem{gr-qc-9604027}
{
Yu.N. Obukhov, E.J. Vlachynsky, W. Esser, R. Tresguerres and F.W. Hehl,
An exact solution of the metric\hyph affine gauge theory with dilation, shear, and spin charges,
eprint \href{http://arxiv.org/abs/gr-qc/9604027}{arXiv:gr-qc/9604027} (1996)
}%

\BiblioItem{4419-7514}
{
Mari\'an Fabian, Petr Habala, Petr H\'ajek, Vicente Montesinos, V\'aclav Zizler.
Banach Space Theory: The Basis for Linear and Nonlinear Analysis.
\\
Springer; New York, 2010; ISBN-13: 978-1441975140
}%

\BiblioItem{Weinberg I}
{
Steven Weinberg.
The Quantum Theory of Fields. Volume I. Foundations.
Cambridge university press, 1995
}%

\BiblioItem{Weinberg II}
{
Steven Weinberg.
The Quantum Theory of Fields. Volume II. Modern applications.
Cambridge university press, 1996
}%

\BiblioItem{Reinhardt}
{
Walter Greiner, Joachim Reinhardt. Field Quantization. Springer.
}%

\BiblioItem{978-3540875604}
{
Walter Greiner, Joachim Reinhardt. Quantum Electrodynamics. Springer, 2009.
}%

\BiblioItem{978-1898563020}
{
H. Robert Mills. Practical Astronomy. Woodhead Publishing, 1994. ISBN-13: 978-1898563020.
}%

\BiblioItem{Landau}
{
L. D. Landau, E. M. Lifshich, The classical theory of fields.
Oxford, New York, Pergamon Press
}%

\BiblioItem{Landau III}
{
L. D. Landau, E. M. Lifshich,
Course of Theoretical Physics, Volume 3.
Quantum Mechanics Non-Relativistic Theory, Third Edition.
\\
Translated from the Russian by J. B. Sykes and J. S. Bell.
Butterworth-Heinemann, 1981, ISBN 978-0750635394.
}%

\BiblioItem{Wheeler}
{
Ignazio Ciufolini, John Wheeler. Gravitation and Inertia.
Princeton university press.
}%

\BiblioItem{Gravitation MTW}
{
Charles W. Misner, Kip S. Thorne, John Archibald Wheeler.
Gravitation.
W. H. Freeman and Company, San Francisco, 1973.
}%

\BiblioItem{Anderson98}
{
J. D. Anderson, P. A. Laing, E. L. Lau, A. S. Liu, M. M. Nieto, and S. G. Turyshev,
Indication, from Pioneer 10/11, Galileo, and Ulysses Data, of an Apparent Anomalous, Weak, Long-Range Acceleration,
\href{http://prola.aps.org/abstract/PRL/v81/i14/p2858_1}{Phys. Rev. Lett. 81, 2858}, (1998),
eprint \href{http://arxiv.org/abs/gr-qc/9808081}{arXiv:gr-qc/9808081} (1998)
}%

\BiblioItem{Anderson02}
{
J. D. Anderson, P. A. Laing, E. L. Lau, A. S. Liu, M. M. Nieto, and S. G. Turyshev,
Study of the anomalous acceleration of Pioneer 10 and 11,
\href{http://prola.aps.org/searchabstract/PRD/v65/i8/e082004}{Phys. Rev. D 65, 082004, 50 pp.}, (2002),
eprint \href{http://arxiv.org/abs/gr-qc/0104064}{arXiv:gr-qc/0104064} (2001)
}%

%\BiblioItem{Havas} Peter Havas, The Classical Equations of Motion of Point Particles, I,
%{
%\href{http://prola.aps.org/abstract/PR/v87/i2/p309_1}{Phys. Rev. 87, 309} (1952)
%}%

\BiblioItem{H. Aslaksen}
{
H. Aslaksen.  Quaternionic determinants \textit{Math.
Intelligencer} {\bf 18}(3), pp.57-65, (1996).
}%

\BiblioItem{L. Chen: Definition of determinant}
{
L. Chen, Definition of determinant and Cramer solutions over
quaternion field, \textit{Acta Math. Sinica (N.S.)} {\bf 7},
pp.171-180, (1991).
}%

\BiblioItem{L. Chen: Inverse matrix}
{
L. Chen,
Inverse matrix and properties of double determinant over quaternion
field, \textit{Sci. China, Ser. A} {\bf 34}, pp.528-540, (1991).
}%

\BiblioItem{N. Cohen S. De Leo}
{
N. Cohen, S. De Leo, The quaternionic determinant, \textit{The Electronic Journal Linear
Algebra} {\bf 7}, pp.100-111, (2000).
}%

\BiblioItem{Dyson: Quaternion determinants}
{
F. J. Dyson, Quaternion determinants, \textit{Helvetica Phys.
Acta} {\bf 45}, pp. 289-302, (1972).
}%

\BiblioItem{Melvin Hausner}
{
Melvin Hausner,
A Vector Space Approach to Geometry,
Dover Publications, 1998
}%

\BiblioItem{Serge Lang}
{
Serge Lang,
Algebra, Springer, 2002
}%

\BiblioItem{9780534423230}
{
Charles Lanski.
Concepts In Abstract Algebra.
American Mathematical Soc., 2005, ISBN 978-0534423230
}%

\BiblioItem{Burris Sankappanavar}
{
S. Burris, H.P. Sankappanavar,
A Course in Universal Algebra, Springer-Verlag (March, 1982),
\\eprint
\href{http://www.math.uwaterloo.ca/~snburris/htdocs/ualg.html}
{http://www.math.uwaterloo.ca/~snburris/htdocs/ualg.html}
\\(The Millennium Edition)
}%

\BiblioItem{Shilov single 3}
{
G. E. Shilov,
Calculus, Single Variable Functions, Part 3,
Moscow, Nauka, 1970
}%

\BiblioItem{Shilov}
{
G. E. Shilov,
Calculus, Multivariable Functions,
Moscow, Nauka, 1972
}%

\BiblioItem{Kolmogorov Fomin}
{
A. N. Kolmogorov and S. V. Fomin.
Introductory Real Analysis.
\\
Translated and edited by Richard A. Silverman.
\\
Dover Publication, 1975, ISBN-13: 978-0486612263
}%

\BiblioItem{Lebedev Vorovich}
{
L. P. Lebedev, I. I. Vorovich,
Functional Analysis in Mechanics,
Springer, 2002
}%

\BiblioItem
{Rashevsky}
{
P. K. Rashevsky, Riemann Geometry and Tensor Calculus,\\
Moscow, Nauka, 1967
}%

\BiblioItem
{Kurosh: High Algebra}
{
A. G. Kurosh, Higher Algebra,
\\
George Yankovsky translator,
\\
Mir Publishers, 1988, ISBN: 978-5030001319
}%

\BiblioItem
{Kurosh: General Algebra}
{
A. G. Kurosh, Lectures on General Algebra,
Chelsea Pub Co, 1965 
}%

\BiblioItem
{Sabinin: Smooth Quasigroups}
{
Lev V. Sabinin, Smooth Quasigroups and Loops,
Kluwer Academic Publisher, 1999 
}%

\BiblioItem{Dubrovin Fomenko Novikov part 1}
{
B. A. Dubrovin, A. T. Fomenko, S. P. Novikov,
Modern Geometry - Methods and Applications,\\
Part 1, The Geometry of Surfaces, Transformation Groups, and Fields,\\
Translated by Robert G. Burns,\\
Springer - New York, 1992
}%

\BiblioItem{Korn}
{
Granino A. Korn, Theresa M. Korn,
Mathematical Handbook for Scientists and Engineer,
McGraw-Hill Book Company, New York, San Francisco,
Toronto, London, Sydney, 1968
}%

\BiblioItem{Hocking Young Topology}
{
John G. Hocking, Gail S. Young,
Topology,\\
Courier Dover Publications, 1988
}%

\BiblioItem{Olver: Lie groups to differential equations}
{
Peter J. Olver,
Applications of Lie groups to differential equations,\\
Springer, 2000
}%

\BiblioItem{Tartaglia}
{
Angelo Tartaglia and Matteo Luca Ruggiero,
Angular Momentum Effects in Michelson\Hyph Morley Type Experiments,
Gen.Rel.Grav. 34, 1371-1382 (2002),\\
eprint \href{http://arxiv.org/abs/gr-qc/0110015}{arXiv:gr-qc/0110015} (2001)
}%

\BiblioItem{Tomozawa}
{
Yukio Tomozawa, Speed of Light in Gravitational Fields, eprint
\href{http://arxiv.org/abs/astro-ph/0303047}{arXiv:astro-ph/0303047} (2004)
}%

\BiblioItem{Magueijo}
{
Joao Magueijo,
Covariant and locally Lorentz-invariant varying speed of light theories,
\href{http://prola.aps.org/abstract/PRD/v62/i10/e103521}{Phys. Rev. D 62, 103521} (2000),
eprint \href{http://arxiv.org/abs/gr-qc/0007036}{arXiv:gr-qc/0007036} (2000)
}%

\BiblioItem{Bassett}
{
Bruce A. Bassett, Stefano Liberati, Carmen Molina-Paris, and Matt Visser,
Geometrodynamics of variable-speed-of-light cosmologies,
\href{http://prola.aps.org/abstract/PRD/v62/i10/e103518}{Phys. Rev. D 62}, 103518 (2000),
eprint \href{http://arxiv.org/abs/astro-ph/0001441}{arXiv:astro-ph/0001441} (2000)
}%

\BiblioItem{C.A. Deavours The Quaternion Calculus}
{
C.A. Deavours, The Quaternion Calculus, 
American Mathematical Monthly, {\bf 80} (1973), pp. 995 - 1008
}%

\BiblioItem{Straumann}
{
Lochlainn O'Raifeartaigh and Norbert Straumann,
Gauge theory: Historical origins and some modern developments,
\href{http://prola.aps.org/abstract/RMP/v72/i1/p1_1}{Rev. Mod. Phys. 72, 1} (2000)
}%

\BiblioItem{Lammerzahl}
{
Claus L\"ammerzahl, Mark P. Haugan,
On the interpretation of Michelson\Hyph Morley experiments,
%\href{http://www.sciencedirect.com/science?\_ob=ArticleURL&\_udi=B6TVM-42WP7CR-1&\_user=10&\_handle=W-WA-A-A-AZ-MsSAYZW-UUW-AUDDYZYZAU-WZCBYCEDW-AZ-U&\_fmt=summary&\_coverDate=04%2F23%2F2001&\_rdoc=1&\_orig=browse&\_srch=%23toc%235538%232001%23997179995%23246657!&\_cdi=5538&view=c&\_acct=C000050221&\_version=1&\_urlVersion=0&\_userid=10&md5=385478cda8c5568dea1aeaf0c43669da}
{Phys. Lett. A282 223-229} (2001),\\
eprint \href{http://arxiv.org/abs/gr-qc/0103052}{arXiv:gr-qc/0103052} (2001)
}%

\BiblioItem{0305117}
{
Holger Mueller, Sven Herrmann, Claus Braxmaier, Stephan Schiller, Achim Peters.
Modern Michelson-Morley Experiment using Cryogenic Optical Resonators.
eprint \href{http://arxiv.org/abs/physics/0305117}{arXiv:physics/0305117} (2003)
\\
Phys. Rev. Lett. 91:020401, 2003
}%

\BiblioItem{0706.2031}
{
Holger Mueller, Paul Louis Stanwix, Michael Edmund Tobar,
Eugene Ivanov, Peter Wolf, Sven Herrmann, Alexander Senger,
Evgeny Kovalchuk, Achim Peters.
Relativity tests by complementary rotating Michelson-Morley experiments.
eprint \href{http://arxiv.org/abs/0706.2031}{arXiv:0706.2031 [physics.class-ph]} (2006)
\\
Phys. Rev. Lett. 99:050401, 2007
}%

\BiblioItem{1008.1205}
{
M. Nagel, K. M\"ohle, K. D\"oringshoff, S. Herrmann, A. Senger, E.V. Kovalchuk, A. Peters.
Testing Lorentz Invariance by Comparing Light Propagation in Vacuum and Matter.
eprint \href{http://arxiv.org/abs/1008.1205}{arXiv:1008.1205 [physics.ins-det]} (2010)
}%

\BiblioItem{1109.4897}
{
The OPERA Collaboration.
Measurement of the neutrino velocity with the OPERA detector in the CNGS beam.
eprint \href{http://arxiv.org/abs/1109.4897}{arXiv:1109.4897 [hep-ex]} (2011)
}%

\BiblioItem{Ranada}
{
Antonio F. Ranada,
Pioneer acceleration and variation of light speed: experimental situation,
eprint \href{http://arxiv.org/abs/gr-qc/0402120}{arXiv:gr-qc/0402120} (2004)
}%

\BiblioItem{Gelfand Minlos: rotation and Lorentz groups}
{
Izrail Moiseevich Gelfand, Robert Adolfovich Minlos,
Representations of the rotation and Lorentz groups and their applications;\\
Engl. transl. ed. H. K. Farahat; Transl. by G. Cummins and T. Boddongton;\\
Pergamon Press, 1963
}%

\BiblioItem{math.QA-0208146}
{
I. Gelfand, S. Gelfand, V. Retakh, R. Wilson,
Quasideterminants,\\
eprint \href{http://arxiv.org/abs/math.QA/0208146}{arXiv:math.QA/0208146} (2002)
}%

\BiblioItem{q-alg-9705026}
{
I. Gelfand, V. Retakh,
Quasideterminants, I,\\
eprint \href{http://arxiv.org/abs/q-alg/9705026}{arXiv:q-alg/9705026} (1997)
}%

\BiblioItem{Gelfand Retakh 1991}
{
I. Gelfand and V. Retakh, Determinants of Matrices over Noncommutative Rings, Funct.
Anal. Appl. 25 (1991), no. 2, 91-102
}%

\BiblioItem{Gelfand Retakh 1992}
{
I. Gelfand and V. Retakh, A Theory of Noncommutative Determinants and Characteristic
Functions of Graphs, Funct. Anal. Appl. 26 (1992), no. 4, 1-20
}%

\BiblioItem{hep-th-9407124}
{
I. M. Gelfand, D. Krob, A. Lascoux, B. Leclerc, V.S. Retakh and J.-Y. Thibon,
Noncommutative symmetric functions,\\
eprint \href{http://arxiv.org/abs/hep-th/9407124}{arXiv:hep-th/9407124} (1994)
}%

\BiblioItem{Naimark Shtern: Theory of group representations}
{
Mark Aronovich Naimark, Aleksandr Isaakovich Shtern,
Theory of group representations;\\
Heidelberg, 1982
}%

\BiblioItem{Barut Raczka: Theory of group representations}
{
Asim Orhan Barut; Ryszard R\c{a}czka;
Theory of group representations and applications;\\
World Scientific Publishing Co. Pre. Ltd., 1986
}%

\BiblioItem{Mihalev Pilz: concise handbook of algebra}
{
Aleksandr Vasilevich Mikhalev; G\"{u}nter Pilz;
The concise handbook of algebra;\\
Kluwer Academic Publishers, 2002
}%

\BiblioItem{Shafarevich: Basic notions of algebra}
{
I. R. Shafarevich,
Basic notions of algebra,\\
Translated from the Russian by M. Reid,\\
Springer, 2005
}%

\BiblioItem{Elsgolts: Differential Equations}
{
Lev Elsgolts,
Differential Equations and the Calculus of Variations,\\
University Press of the Pacific, 2003 
}%

\BiblioItem{Baez Huerta: algebra of grand unified theories}
{
John Baez; John Huerta;
The algebra of grand unified theories;\\
Bull. Amer. Math. Soc. {\bf 47} (2010), 483-552
}%

\BiblioItem{J. Fan: Determinants}
{
J. Fan, Determinants and multiplicative functionals
on quaternion matrices, \textit{Linear Algebra and Its
Applications} {\bf 369}, pp. 193-201, (2003).
}%

\BiblioItem{Carl Faith 1}
{
Carl Faith, Algebra: Rings, Modules and Categories I,
Springer - Verlag, Berlin - Heidelberg - New York, 1973
}%

\BiblioItem{Gilson Nimmo Ohta}
{
 C.R.Gilson, J.J.C.Nimmo, Y.Ohta, Quasideterminant solutions of a non-Abelian Hirota-Miwa
 equation, \textit{Journal of Physics A: Mathematical and Theoretical} {\bf 40}(42), pp.
 12607-12617,(2007).
}%

\BiblioItem{Haider Hassan}
{
B. Haider, M. Hassan, Quasideterminant solutions of an integrable chiral model in two
 dimensions, \textit{Journal of Physics A: Mathematical and Theoretical} {\bf 42} (35), art. no.
 355211, (2009).
}%

%\BiblioItem{Pareigis}
%{
%Bodo Pareigis, Categories and Functors,
%Academic Press - New York - London, 1970
%}%

%\BiblioItem{Beachy}
%{
%John A. Beachy, Introductory Lectures on Rings i Modules,
%Cambridge University Press, 1999
%}%

\BiblioItem{0702447}
{
I.I. Kyrchei, Cramer's rule for quaternion systems of linear equations,
\textit{Journal of Mathematical Sciences} {\bf 155}(6), 839-858, (2008).
 Translated from  \textit{Fundamental and Appl. Math.}
 {\bf 13}(4), pp.67-94, (2007). (in Russian)\\
eprint
\href{http://arxiv.org/abs/math/0702447}{arXiv:math.RA/0702447}
(2007)
}%

\BiblioItem{1004.4380}
{
I.I. Kyrchei, Cramer's rule for some quaternion matrix
    equations,  \textit{Applied Mathematics and Computation} {\bf 217}(5), pp.2024-2030, (2010).\\eprint
\href{http://arxiv.org/abs/1004.4380
}{arXiv:math.RA/arXiv:1004.4380 } (2010)
}%

\BiblioItem{1005.0736}
{
I.I. Kyrchei,Determinantal representations of the Moore-Penrose inverse
 over the quaternion skew field and corresponding Cramer's rules,
 \\
eprint
\href{http://arxiv.org/abs/1005.0736}{arXiv:math.RA/1005.0736}
(2010)
}%

\BiblioItem{0412.391}
{
Aleks Kleyn,
Basis Manifold,
eprint \href{http://arxiv.org/abs/math.DG/0412391}{arXiv:math.DG/0412391} (2007)
}%

\BiblioItem{0405.027}
{
Aleks Kleyn,
Reference Frame in General Relativity,\\
eprint \href{http://arxiv.org/abs/gr-qc/0405027}{arXiv:gr-qc/0405027} (2008)
}%

\BiblioItem{0405.028}
{
Aleks Kleyn, Metric\hyph Affine Manifold,\\
eprint \href{http://arxiv.org/abs/gr-qc/0405028}{arXiv:gr-qc/0405028} (2008)
}%

\BiblioItem{0612.111}
{
Aleks Kleyn,
Biring of Matrices,\\
eprint \href{http://arxiv.org/abs/math.OA/0612111}{arXiv:math.OA/0612111} (2007)
}%

\BiblioItem{0701.238}
{
Aleks Kleyn,
Lectures on Linear Algebra over Division Ring,\\
eprint \href{http://arxiv.org/abs/math.GM/0701238}{arXiv:math.GM/0701238} (2010)
}%

\BiblioItem{0702.561}
{
Aleks Kleyn,
Fibered $\mathfrak{F}$\Hyph Algebra,\\
eprint \href{http://arxiv.org/abs/math.DG/0702561}{arXiv:math.DG/0702561} (2007)
}%

\BiblioItem{math.RA-0501237}
{
Aleks Kleyn,
Vector Space Over Division Ring,\\
eprint \href{http://arxiv.org/abs/math.RA/0412391}{arXiv:math.RA/0501237} (2007)
}%

\BiblioItem{math.RA-0501237v1}
{
Aleks Kleyn,
Module Over Division Ring, version 1,\\
eprint \href{http://arxiv.org/abs/math/0501237v1}{arXiv:math.RA/0501237v1} (2005)
}%

\BiblioItem{0707.2246}
{
Aleks Kleyn,
Fibered Correspondence,\\
eprint \href{http://arxiv.org/abs/0707.2246}{arXiv:0707.2246} (2007)
}%

\BiblioItem{0803.2620}
{
Aleks Kleyn,
Morphism of \Ts Representations,\\
eprint \href{http://arxiv.org/abs/0803.2620}{arXiv:0803.2620} (2008)
}%

\BiblioItem{0803.3276}
{
Aleks Kleyn,
Lorentz Transformation and General Covariance Principle,\\
eprint \href{http://arxiv.org/abs/0803.3276}{arXiv:0803.3276} (2009)
}%

\BiblioItem{0812.4763}
{
Aleks Kleyn,
Introduction into Calculus over Division Ring,\\
eprint \href{http://arxiv.org/abs/0812.4763}{arXiv:0812.4763} (2010)
}%

\BiblioItem{0906.0135}
{
Aleks Kleyn,
Introduction into Geometry over Division Ring,\\
eprint \href{http://arxiv.org/abs/0906.0135}{arXiv:0906.0135} (2010)
}%

\BiblioItem{0909.0855}
{
Aleks Kleyn,
Quaternion Rhapsody,\\
eprint \href{http://arxiv.org/abs/0909.0855}{arXiv:0909.0855} (2010)
}%

\BiblioItem{0912.3315}
{
Aleks Kleyn,
Representation of Universal Algebra,\\
eprint \href{http://arxiv.org/abs/0912.3315}{arXiv:0912.3315} (2009)
}%

\BiblioItem{0912.4061}
{
Aleks Kleyn,
Linear Equation in Finite Dimensional Algebra,\\
eprint \href{http://arxiv.org/abs/0912.4061}{arXiv:0912.4061} (2010)
}%

\BiblioItem{1001.4852}
{
Aleks Kleyn,
The Matrix of Linear Maps,\\
eprint \href{http://arxiv.org/abs/1001.4852}{arXiv:1001.4852} (2010)
}%

\BiblioItem{1003.1544}
{
Aleks Kleyn,
Linear Maps of Free Algebra,\\
eprint \href{http://arxiv.org/abs/1003.1544}{arXiv:1003.1544} (2010)
}%

\BiblioItem{1006.2597}
{
Aleks Kleyn,
The G\^ateaux Derivative and Integral over Banach Algebra,\\
eprint \href{http://arxiv.org/abs/1006.2597}{arXiv:1006.2597} (2010)
}%

\BiblioItem{1011.3102}
{
Aleks Kleyn,
Polylinear Map of Free Algebra,\\
eprint \href{http://arxiv.org/abs/1011.3102}{arXiv:1011.3102} (2010)
}%

\BiblioItem{1104.5197}
{
Aleks Kleyn,
$C^*$-Rhapsody,\\
eprint \href{http://arxiv.org/abs/1104.5197}{arXiv:1104.5197} (2011)
}%

\BiblioItem{1105.4307}
{
Aleks Kleyn,
Algebra with Conjugation,\\
eprint \href{http://arxiv.org/abs/1105.4307}{arXiv:1105.4307} (2011)
}%

\BiblioItem{1107.1139}
{
Aleks Kleyn,
Linear Maps of Quaternion Algebra,\\
eprint \href{http://arxiv.org/abs/1107.1139}{arXiv:1107.1139} (2011)
}%

\BiblioItem{1107.5037}
{
Aleks Kleyn,
Orthogonal Basis and Motion in Finsler Geometry,\\
eprint \href{http://arxiv.org/abs/1107.5037}{arXiv:1107.5037} (2011)
}%

\BiblioItem{1202.6021}
{
Aleks Kleyn,
Maps of Conjugation of Quaternion Algebra,\\
eprint \href{http://arxiv.org/abs/1202.6021}{arXiv:1202.6021} (2012)
}%

\BiblioItem{1211.6965}
{
Aleks Kleyn,
Free Algebra with Countable Basis,\\
eprint \href{http://arxiv.org/abs/1211.6965}{arXiv:1211.6965} (2012)
}%

\BiblioItem{8433-5163}
{
Aleks Kleyn,
Linear Maps of Free Algebra: First Steps in Noncommutative Linear Algebra,\\
Lambert Academic Publishing, 2010
}%

\BiblioItem{8443-0072}
{
Aleks Kleyn,
Representation Theory: Representation of Universal Algebra,\\
Lambert Academic Publishing, 2011
}%

\BiblioItem{CACAA.07.291}
{
Aleks Kleyn,
Introduction into Calculus over Division Ring.\\
Clifford Analysis, Clifford Algebras and their applications,
Vol 7, Issue 4, pages 291 - 355, 2012
}%

\BiblioItem{Lauve: Quantum coordinates}
{
A. Lauve, Quantum- and quasi-Plucker coordinates,
\textit{Journal of Algebra} {\bf 296}(2), pp.440-461,
(2006).
}%

\BiblioItem{Lewis D. W. Quaternion algebras}
{
Lewis D. W. Quaternion algebras and the algebraic legacy
of Hamilton's quaternions, \textit{Irish Math. Soc. Bulletin} {\bf
57}, pp. 41-64, (2006).
}%

\BiblioItem{0812.2865}
{
Jos\'e Miguel Figueroa-O'Farrill,
Three lectures on 3-algebras,
eprint \href{http://arxiv.org/abs/0812.2865}{arXiv:0812.2865} (2008)
}%

\BiblioItem{1202.0951}
{
Daniel Edward Clark,
Deconvolution of point processes,
eprint \href{http://arxiv.org/abs/1202.0951}{arXiv:1202.0951} (2012)
}%

\BiblioItem{1202.4546}
{
Ming-Liang Hu,
Disentanglement, Bell-nonlocality violation
and teleportation capacity of the decaying tripartite states,
eprint \href{http://arxiv.org/abs/1202.4546}{arXiv:1202.4546} (2012)
}%

\BiblioItem{1203.1629}
{
Borivoje Dakic, Yannick Ole Lipp, Xiaosong Ma, Martin Ringbauer,
Sebastian Kropatschek, Stefanie Barz, Tomasz Paterek, Vlatko Vedral,
Anton Zeilinger, Caslav Brukner, Philip Walther,
Quantum Discord as Optimal Resource for Quantum Communication,
eprint \href{http://arxiv.org/abs/1203.1629}{arXiv:1203.1629} (2012)
}%

\BiblioItem{Li Nimmo: Darboux transformations}
{
C.X.Li, J.J.C. Nimmo, Darboux transformations for a twisted
derivation and quasideterminant solutions to the super KdV
equation, \textit{Proceedings of the Royal Society A:
Mathematical, Physical and Engineering Sciences} {\bf 466} (2120),
pp. 2471-2493, (2010)
}%

\BiblioItem{Schiebold: Cauchy-type determinants}
{
C. Schiebold, Cauchy-type determinants and integrable
systems, \textit{Linear Algebra and Its Applications} {\bf 433}
(2), pp. 447-475, (2010)
}%

\BiblioItem{Suzuki: Noncommutative spectral decomposition}
{
T. Suzuki, Noncommutative
spectral decomposition with qua\-si\-de\-ter\-mi\-nant, \textit{Advances in
Mathematics} {\bf 217}(5), pp. 2141-2158, (2008)
}%

\BiblioItem{1105.3456}
{
C. W. F. Everitt, D. B. DeBra, B. W. Parkinson, J. P. Turneaure, J. W. Conklin,
M. I. Heifetz, G. M. Keiser, A. S. Silbergleit, T. Holmes, J. Kolodziejczak,
M. Al-Meshari, J. C. Mester, B. Muhlfelder, V. Solomonik, K. Stahl, P. Worden,
W. Bencze, S. Buchman, B. Clarke, A. Al-Jadaan, H. Al-Jibreen, J. Li, J. A. Lipa,
J. M. Lockhart, B. Al-Suwaidan, M. Taber, S. Wang,\\
Gravity Probe B: Final Results of a Space Experiment to Test General Relativity,\\
eprint \href{http://arxiv.org/abs/1105.3456}{arXiv:1105.3456[gr-qc]} (2011)
}%

\BiblioItem{0009305}
{
G. S. Asanov.
Can Neutrinos and High-Energy Particles Test Finsler Metric of Space-Time?\\
eprint \href{http://arxiv.org/abs/hep-ph/0009305}{arXiv:hep-ph/0009305} (2000)
}%

\BiblioItem{Asanov 2004}
{
G. S. Asanov.
Finsleroid - space supplemented by angle and scalar product.\\
Hypercomplex Numbers in Geometry and Physics, {\bf 1}, 2004, p. 40 - 62
}%

\BiblioItem{1004.3007}
{
Sergiu I. Vacaru,
Principles of Einstein-Finsler Gravity and Perspectives in Modern Cosmology,\\
eprint \href{http://arxiv.org/abs/1004.3007}{arXiv:1004.3007[math-ph]} (2010)
}%

\BiblioItem{1012.4148}
{
Sergiu I. Vacaru.
Principles of Einstein-Finsler Gravity and Cosmology.\\
eprint \href{http://arxiv.org/abs/1012.4148}{arXiv:1012.4148[physics.gen-ph]} (2010)
}%

\BiblioItem{1112.5641}
{
Christian Pfeifer, Mattias N.R. Wohlfarth.
Finsler geometric extension of Einstein gravity.\\
eprint \href{http://arxiv.org/abs/1112.5641}{arXiv:1112.5641[gr-qc]} (2011)
}%

\BiblioItem{0711.0056}
{
Zhe Chang, Xin Li.
Lorentz Invariance Violation and Symmetry in Randers\Hyph Finsler Spaces.\\
eprint \href{http://arxiv.org/abs/0711.0056}{arXiv:0711.0056[hep-th]} (2011)
}%

\BiblioItem{Rund Finsler geometry}
{
Hanno Rund,
The differential geometry of Finsler spaces.
\\
Springer - Verlag, Berlin - G\"ottingen - Heidelberg, 1959
}%

\BiblioItem{Smirnov vol 1}
{
V. I. Smirnov,
A Course of Higher Mathematics, volume I.
\\
Translated by D. E. Brown.
\\
Translation, edited and additions made by I. N. Sneddon.
\\
Pergamon Press, Addison-Wesley Publishing Company, 1964
}%

\BiblioItem{Beem Dostoglou Ehrlich}
{
John K. Beem, Stamatis A. Dostoglou, Paul E. Ehrlich,
Advances in differential geometry and general relativity.
\\
American Mathematical Society, 2004
}%

\BiblioItem{978-0719033414}
{
Malcolm Pemberton, Nicholas Rau,
Mathematics for economists: an introductory textbook.
\\
Manchester University Press, November 2001; ISBN-13: 978-0719033414
}%

\BiblioItem{0 521 59180 5}
{
Cyrus D. Cantrell,
Modern mathematical methods for physicists and engineers.
\\
Cambridge University Press, 2000
}%

\BiblioItem{Arveson spectral theory}
{
William Arveson,
A short course on spectral theory.
\\
Springer - Verlag, New York, 2002
}%

\BiblioItem{Robert Hermann}
{
Robert Hermann,
Topics in the mathematics of quantum mechanics.
\\
Math Sci Press, 1973
}%

\BiblioItem{9705.009}%q-alg-9705009
{
John C. Baez,
An Introduction to n-Categories,\\
eprint \href{http://arxiv.org/abs/q-alg/9705009}{arXiv:q-alg/9705009} (1997)
}%

\BiblioItem{0105.155}
{
John C. Baez,
The Octonions,\\
eprint \href{http://arxiv.org/abs/math.RA/0105155}{arXiv:math.RA/0105155} (2002)
}%

\BiblioItem{John Baez: Math Blogs}
{
John C. Baez,
What do mathematicians need to know about blogging?,\\
Notices of the American Mathematical Society,
(2010), 3, {\bf 57}, 333,\\
\url{http://www.ams.org/notices/201003/rtx100300333p.pdf}
}%

\BiblioItem{Tolstoi about Anna Karenina}
{
Tolstoi about Anna Karenina,
in book A Karenina Companion, by C. J. G. Turner,
published by Wilfrid Laurier University Press (August 1993)
}%

\BiblioItem
{Cohn: Universal Algebra}
{
Paul M. Cohn,
Universal Algebra,
Springer, 1981
}%

\BiblioItem
{Cohn: Skew Fields}
{
Paul M. Cohn,
Skew Fields,
Cambridge University Press, 1995
}%

\BiblioItem
{Maunder: Algebraic Topology}
{
C. R. F. Maunder,
Algebraic Topology,
Dover Publications, Inc, Mineola, New York, 1996
}%

\BiblioItem{Pommaret: Partial Differential Equations}
{
J.-F. Pommaret,
Partial Differential Equations and Group Theory,
Springer, 1994
}%

\BiblioItem{Bourbaki: Set Theory}
{
N. Bourbaki,
Theory of sets,
Springer, 2004
}%

\BiblioItem{Bourbaki: Algebra 1}
{
N. Bourbaki,
Algebra 1,
Springer, 2004
}%

\BiblioItem{Bourbaki: Algebra 2}
{
N. Bourbaki,
Algebra II, Chapters 4 - 7,//
Translated by P. M. Cohn & J. Howie,//
Springer, 2004
}%

\BiblioItem
{Bourbaki: General Topology 1}
{
N. Bourbaki,
General Topology, Chapters 1 - 4,
Springer, 1989
}

\BiblioItem{Bourbaki: General Topology: Chapter 5 - 10}
{
N. Bourbaki,
General Topology, Chapters 5 - 10,
Springer, 1989
}

\BiblioItem{Bourbaki: Topological Vector Space}
{
N. Bourbaki,
Topological Vector Spaces, Chapters 1 - 5,
Transl. by H. G. Eggleston $\&$ S. Madan,
Springer, 2003
}

\BiblioItem{Bourbaki: Coxeter Group Lie}
{
N. Bourbaki,
Lie Groups and Lie Algebras, Chapters 4 - 6,
Translator Andrew Pressley,
Springer, 2002
}

\BiblioItem{Bourbaki: Real Group Lie}
{
N. Bourbaki,
Lie Groups and Lie Algebras, Chapters 7 - 9,
Translator Andrew Pressley,
Springer, 2005
}

\BiblioItem{Shabat: Complex Analysis}
{
Shabat B. V.,
Introduction to Complex Analysis,
\\ \url{http://www.math.uchicago.edu/~ryzhik/shabat-all.pdf},
\\Translated from Russian by L.Ryzhik, 2003
(Moscow, Nauka, 1969)
}

\BiblioItem{Pontryagin: Topological Group}
{
L. S. Pontryagin,
Selected Works, Volume Two, Topological Groups,
Gordon and Breach Science Publishers, 1986
}

\BiblioItem
{Eisenhart: Riemannian Geometry}
{
Eisenhart,
Riemannian Geometry,
Princeton University Press, Princeton, 1949
}

\BiblioItem
{Eisenhart: Continuous Groups of Transformations}
{
Eisenhart,
Continuous Groups of Transformations,
Dover Publications, New York, 1961
}

\BiblioItem
{Condon Odabasi}
{
Edward Uhler Condon, Halis Odabasi,
Atomic Structure,
CUP Archive, 1980
}

\BiblioItem{Postnikov: Differential Geometry}
{
Postnikov M. M.,
Geometry IV: Differential geometry,
Moscow, Nauka, 1983
}

\BiblioItem{Fihtengolts: Calculus volume 1}
{
Fihtengolts G. M.,
Differential and Integral Calculus Course, volume 1,
Moscow, Nauka, 1969
}

\BiblioItem{Fihtengolts: Calculus volume 2}
{
Fihtengolts G. M.,
Differential and Integral Calculus Course, volume 2,
Moscow, Nauka, 1969
}

\BiblioItem{Hatcher: Algebraic Topology}
{
Allen Hatcher,
Algebraic Topology,
Cambridge University Press, 2002
}

\BiblioItem{geometry of differential equations}
{
Vinogradov, A. M., Krasil'shchik, I. S., and Lychagin, V. V.,
Introduction to geometry of nonlinear differential equations,
Nauka, Moscow, 1986
}

\BiblioItem{cohomological analysis}
{
A. M. Vinogradov,
Cohomological Analysis of Partial Differential Equations
and Secondary Calculus,
American Mathematical Society, 2001
}

\BiblioItem{0801.1734}
{
Brandon S. DiNunno, Richard A. Matzner,
The Volume Inside a Black Hole,\\
eprint \href{http://arxiv.org/abs/0801.1734v1}{arXiv:0801.1734v1} (2008)
}

\BiblioItem{0702.447}
{
Ivan Kyrchei,
Cramer's rule for some quaternion matrix equations,\\
eprint \href{http://arxiv.org/abs/math/0702447}{arXiv:math.RA/0702447} (2007)
}

\BiblioItem{Izrail M. Gelfand: Quaternion Groups}
{
I. M. Gelfand, M. I. Graev,
Representation of Quaternion Groups over Localy Compact and
Functional Fields,\\
Funct. Anal. Appl. {\bf 2} (1968) 19 - 33;\\
Izrail Moiseevich Gelfand, Semen Grigorevich Gindikin,\\
Izrail M. Gelfand: Collected Papers, volume II, 435 - 449,\\
Springer, 1989
}

\BiblioItem{Richard D. Schafer}
{
Richard D. Schafer,
An Introduction to Nonassociative Algebras,
Dover Publications, Inc., New York, 1995
}

\BiblioItem{Bamberg Sternberg}
{
Paul Bamberg, Shlomo Sternberg,
A course in mathematics for students of physics,
Cambridge University Press, 1991
}

\BiblioItem{Conway Smith}
{
John Horton Conway, Derek Alan Smith,
On quaternions and octonions: their geometry, arithmetic, and symmetry,
A K Peters, Natick, Massachussets, 2003
}

\BiblioItem{Fueter}
{
Fueter, R.
Die Funktionentheorie der Differentialgleichungen $\Delta u = 0$ und
$\Delta \Delta u = 0$ mit vier reellen Variablen.
Comment. Math. Helv. {\bf 7} (1935), 307-330
}

\BiblioItem{Sudbery Quaternionic Analysis}
{
A. Sudbery,
Quaternionic Analysis,
Math. Proc. Camb. Phil. Soc. (1979), {\bf 85}, 199 - 225
}

\BiblioItem{0902.4771}
{
Fabrizio Colombo, Graziano Gentili, Irene Sabadini,
A Cauchy kernel for slice regular functions,\\
eprint \href{http://arxiv.org/abs/0902.4771v1}{arXiv:0902.4771v1} (2009)
}

\BiblioItem{Vadim Komkov}
{
Vadim Komkov,
Variational Principles of Continuum Mechanics with Engineering Applications: Critical Points Theory,\\
Springer, 1986
}

\BiblioItem{Alain Connes 1994}
{
Alain Connes,
Noncommutative Geometry,\\
Academic Press, 1994
}

\BiblioItem{Hamilton papers 3}
{
Sir William Rowan Hamilton,
The Mathematical Papers, Vol. III, Algebra,\\
Cambridge at the University Press, 1967
}

\BiblioItem{Hamilton Elements of Quaternions 1}
{
Sir William Rowan Hamilton,
Elements of Quaternions, Volume I,\\
Longmans, Green, and Co., London, New York, and Bombay, 1899
}

\BiblioItem{Cartan geometry in reper}
{
Elie Cartan, Vladislav V. Goldberg, Serge\u{i} Pavlovich Finikov,\\
Riemannian geometry in an orthogonal frame:
from lectures delivered by Elie Cartan at the Sorbonne in 1926-1927,\\
translated by Vladislav V. Goldberg,\\
World Scientific, 2001
}

\BiblioItem{Cartan differential form}
{
Henri Cartan.
Differential calculus. Differential forms.\\
Moscow. Mir, 1971
}

\BiblioItem{Arnautov Glavatsky Mikhalev}
{
V. I. Arnautov, S. T. Glavatsky, A. V. Mikhalev,\\
Introduction to the theory of topological rings and modules,
Volume 1995,\\
Marcel Dekker, Inc, 1996
}

\BiblioItem{Moore Yaqub}
{
Hal G. Moore, Adil Yaqub,
A first course in linear algebra with applications,
Edition 3, Academic Press, 1998 
}

\BiblioItem{math.CV-0405471}
{
S. V. Ludkovsky,
Differentiable functions of Cayley-Dickson numbers,\\
eprint \href{http://arxiv.org/abs/math.CV/0405471}{arXiv:math.CV/0405471} (2004)
}%

\BiblioItem{W.Bertram H.Glockner K.Neeb}
{
W.Bertram, H.Glockner, K.Neeb,
Differential Calculus over General Base Fields and Rings,
Expositiones Mathematicae (2004), Volume 22, Issue 3, Pages 213-282
}

\CloseBiblio


==> Biblio.Russian.tex <==
%auto-ignore
\OpenBiblio

\BiblioItem{Einstein: Electrodynamics of Moving Bodies}
{
Альберт Эйнштейн,
К электродинамике движущихся тел, 1905,
Собрание научных трудов, I, 7 - 35,
М., Наука, 1965
\\
Zur Elektrodynamik der bewegter K\"orper. Ann. Phys., 1905, 17, 891-921. 
}%

\BiblioItem{Einstein: On the Relativity Principle}
{
Альберт Эйнштейн,
О принципе относительности и его следствиях, 1907,
Собрание научных трудов, I, 65 - 114,
М., Наука, 1965
\\
\"Uber das Relativit\"atsprinzip und die aus demselben gezogenen Folgerungen. 
Jahrb. d. Radioaktivit\"at u. Elektronik, 1907, 4, 411-462. 
}%

\BiblioItem{Einstein: Foundations of general relativity}
{
Альберт Эйнштейн,
Основы общей теории относительности, 1916,
Собрание научных трудов, I, 452 - 504,
М., Наука, 1965
}%

\BiblioItem{Einstein: Geometry and Experience}
{
Альберт Эйнштейн,
Геометрия и опыт, (1921)
Собрание научных трудов, II, 83 - 84,
М., Наука, 1966
}%

\BiblioItem{Einstein: Main problems of general relativity}
{
Альберт Эйнштейн,
Основные идеи и проблемы теории относительности, (1923)
Собрание научных трудов, II, 120 - 129,
М., Наука, 1966
}%

\BiblioItem{Einstein: Noneuclidean Geometry and Physics}
{
Альберт Эйнштейн,
Неэвклидова геометрия и физика, (1926)
Собрание научных трудов, II, 178 - 182,
М., Наука, 1966
}%

\BiblioItem{Einstein: Isaak Newton}
{
Альберт Эйнштейн,
Исаак Ньютон, 1927,
Собрание научных трудов, IV, 78 - 81,
М., Наука, 1967
}%

\BiblioItem{Einstein: On Science}
{
Альберт Эйнштейн,
О науке, 1931,
Собрание научных трудов, IV, 142 - 146,
М., Наука, 1967
}%

\BiblioItem{Einstein: Autobiographical Notes}
{
Альберт Эйнштейн,
Автобиографические заметки, 1949,
Собрание научных трудов, IV, 259 - 293,
М., Наука, 1967
}%

\BiblioItem{Feynman 3}
{
Фейнман Р., Лейтон Р., Сэндс М..
Фейнмановские лекции по физике (том 3). Излучение. Волны. Кванты.
М., Мир, 1976
}%

\BiblioItem{0538731877}
{
James Shipman, Jerry D. Wilson and Aaron Todd.
Introduction to Physical Science.
Cengage Learning, 2009; ISBN 0538731877.
}%

\BiblioItem{Cite: 104}
{
Ссылка 104, Источник неизвестен
}%

\BiblioItem{Ghez}
{
Ghez et al.,
The First Measurement of Spectral Lines in a Short-Period Star Bound to the Galaxy's Central Black Hole: A Paradox of Youth,
\href{http://www.journals.uchicago.edu/ApJ/journal/issues/ApJL/v586n2/16990/brief/16990.abstract.html}{ApJL, 586, L127} (2003),
eprint \href{http://arxiv.org/abs/astro-ph/0302299}{arXiv:astro-ph/0302299} (2003)
}%

\BiblioItem{Schodel}
{
R. Sch\"odel et al.,
A star in a 15.2-year orbit around the supermassive black hole at the centre of the Milky Way,
\href{http://www.nature.com/cgi-taf/DynaPage.taf?file=/nature/journal/v419/n6908/abs/nature01121_fs.html}{Nature 419, 694} (2002)
}%

\BiblioItem{Mielke}
{
Eckehard W. Mielke, Affine generalization of the Komar complex of general relativity,
\href{http://prola.aps.org/searchabstract/PRD/v63/i4/e044018}{Phys. Rev. D 63, 044018} (2001)
}%

\BiblioItem{Obukhov}
{
Yu. N. Obukhov and J. G. Pereira, Metric\hyph affine approach to teleparallel gravity,
\href{http://scitation.aip.org/getabs/servlet/GetabsServlet?prog=normal&id=PRVDAQ000067000004044016000001&idtype=cvips&gifs=Yes}
{Phys. Rev. D 67, 044016} (2003),
eprint \href{http://arxiv.org/abs/gr-qc/0212080}{arXiv:gr-qc/0212080} (2002)
}%

\BiblioItem{Sardanashvily}
{
Giovanni Giachetta, Gennadi Sardanashvily, Dirac Equation in Gauge and Affine-Metric Gravitation Theories,
eprint \href{http://arxiv.org/abs/gr-qc/9511035}{arXiv:gr-qc/9511035} (1995)
}%

\BiblioItem{Gauge}
{
Frank Gronwald and Friedrich W. Hehl, On the Gauge Aspects of Gravity, eprint
\href{http://arxiv.org/abs/gr-qc/9602013}{arXiv:gr-qc/9602013} (1996)
}%

\begin{otherlanguage}{english}
\BiblioItem{Neeman}
{
Yuval Neeman, Friedrich W. Hehl, Test Matter in a Spacetime with Nonmetricity, eprint
\href{http://arxiv.org/abs/gr-qc/9604047}{arXiv:gr-qc/9604047} (1996)
}%
\end{otherlanguage}

\BiblioItem{torsion}
{
F. W. Hehl, P. von der Heyde, G. D. Kerlick, and J. M. Nester,
General relativity with spin and torsion: Foundations and prospects,\\
\href{http://prola.aps.org/abstract/RMP/v48/i3/p393_1}{Rev. Mod. Phys. 48, 393} (1976)
}%

\BiblioItem{Megged}
{
O. Megged, Post-Riemannian Merger of Yang-Mills Interactions with Gravity,
eprint \href{http://arxiv.org/abs/hep-th/0008135}{arXiv:hep-th/0008135} (2001)
}%

%\BiblioItem{Hehl}
%{
%Friedrich W. Hehl, Uwe Muench,
%eprint \href{http://arxiv.org/abs/gr-qc/9708007}{arXiv:gr-qc/9708007} (1997)
%}%

\BiblioItem{gr-qc-9604027}
{
Yu.N. Obukhov, E.J. Vlachynsky, W. Esser, R. Tresguerres and F.W. Hehl,
An exact solution of the metric\hyph affine gauge theory with dilation, shear, and spin charges,
eprint \href{http://arxiv.org/abs/gr-qc/9604027}{arXiv:gr-qc/9604027} (1996)
}%

\BiblioItem{4419-7514}
{
Mari\'an Fabian, Petr Habala, Petr H\'ajek, Vicente Montesinos, V\'aclav Zizler.
Banach Space Theory: The Basis for Linear and Nonlinear Analysis.
\\
Springer; New York, 2010; ISBN-13: 978-1441975140
}%

\BiblioItem{Weinberg I}
{
Стивен Вайнберг.
Квантовая теория полей. Том 1. Основы.
\\
Перевод на русский язык А. В. Беркова под редакцией Б. Л. Воронова,
М., Физико-математическая литература, 2001
}%

\BiblioItem{Weinberg II}
{
Стивен Вайнберг.
Квантовая теория полей. Том 2. Современные приложения.
\\
Перевод на русский язык А. В. Беркова,
М., Физико-математическая литература, 2001
}%

\BiblioItem{Reinhardt}
{
Walter Greiner, Joachim Reinhardt. Field Quantization. Springer.
}%

\BiblioItem{978-3540875604}
{
Walter Greiner, Joachim Reinhardt. Quantum Electrodynamics. Springer, 2009.
}%

\BiblioItem{978-1898563020}
{
H. Robert Mills. Practical Astronomy. Woodhead Publishing, 1994. ISBN-13: 978-1898563020.v
}%

\BiblioItem{Landau}
{
Л. Д. Ландау, Е. М. Лифшич,
Теоретическая физика, теория поля,
М., Наука, 1988
}%

\BiblioItem{Landau III}
{
Л. Д. Ландау, Е. М. Лифшич,
Теоретическая физика, том III, квантовая механика,
нерелятивистская теория,
М., Наука, 1989
}%

\BiblioItem{Wheeler}
{
Ignazio Ciufolini, John Wheeler. Gravitation and Inertia.
Princeton university press.
}%

\BiblioItem{Gravitation MTW 1}
{
Ч. Мизнер, К. Торн, Дж. Уилер.
Гравитация, том $1$.
\\
Перевод с английского М. М. Баско
под редакцией В. Б. Брагинского и И. Д. Новикова.
\\
М. Мир, 1977.
}%

\BiblioItem{Gravitation MTW 2}
{
Ч. Мизнер, К. Торн, Дж. Уилер.
Гравитация, том $2$.
\\
Перевод с английского A. А. Рузмайкина 
под редакцией В. Б. Брагинского и И. Д. Новикова.
\\
М. Мир, 1977.
}%

\BiblioItem{Anderson98}
{
J. D. Anderson, P. A. Laing, E. L. Lau, A. S. Liu, M. M. Nieto, and S. G. Turyshev,
Indication, from Pioneer 10/11, Galileo, and Ulysses Data, of an Apparent Anomalous, Weak, Long-Range Acceleration,
\href{http://prola.aps.org/abstract/PRL/v81/i14/p2858_1}{Phys. Rev. Lett. 81, 2858}, (1998),
eprint \href{http://arxiv.org/abs/gr-qc/9808081}{arXiv:gr-qc/9808081} (1998)
}%

\BiblioItem{Anderson02}
{
J. D. Anderson, P. A. Laing, E. L. Lau, A. S. Liu, M. M. Nieto, and S. G. Turyshev,
Study of the anomalous acceleration of Pioneer 10 and 11,
\href{http://prola.aps.org/searchabstract/PRD/v65/i8/e082004}{Phys. Rev. D 65, 082004, 50 pp.}, (2002),
eprint \href{http://arxiv.org/abs/gr-qc/0104064}{arXiv:gr-qc/0104064} (2001)
}%

%\BiblioItem{Havas} Peter Havas, The Classical Equations of Motion of Point Particles, I,
%{
%\href{http://prola.aps.org/abstract/PR/v87/i2/p309_1}{Phys. Rev. 87, 309} (1952)
%}%

\BiblioItem{H. Aslaksen}
{
H. Aslaksen.  Quaternionic determinants \textit{Math.
Intelligencer} {\bf 18}(3), pp.57-65, (1996).
}%

\BiblioItem{L. Chen: Definition of determinant}
{
L. Chen, Definition of determinant and Cramer solutions over
quaternion field, \textit{Acta Math. Sinica (N.S.)} {\bf 7},
pp.171-180, (1991).
}%

\BiblioItem{L. Chen: Inverse matrix}
{
L. Chen,
Inverse matrix and properties of double determinant over quaternion
field, \textit{Sci. China, Ser. A} {\bf 34}, pp.528-540, (1991).
}%

\BiblioItem{N. Cohen S. De Leo}
{
N. Cohen, S. De Leo, The quaternionic determinant, \textit{The Electronic Journal Linear
Algebra} {\bf 7}, pp.100-111, (2000).
}%

\BiblioItem{Dyson: Quaternion determinants}
{
F. J. Dyson, Quaternion determinants, \textit{Helvetica Phys.
Acta} {\bf 45}, pp. 289-302, (1972).
}%

\BiblioItem{Melvin Hausner}
{
Melvin Hausner,
A Vector Space Approach to Geometry,
Dover Publications, 1998
}%

\BiblioItem{Serge Lang}
{
Серж Ленг,
Алгебра, М. Мир, 1968
}%

\BiblioItem{9780534423230}
{
Charles Lanski.
Concepts In Abstract Algebra.
American Mathematical Soc., 2005, ISBN 978-0534423230
}%

\BiblioItem{Burris Sankappanavar}
{
S. Burris, H.P. Sankappanavar,
A Course in Universal Algebra, Springer-Verlag (March, 1982),
\\eprint
\href{http://www.math.uwaterloo.ca/~snburris/htdocs/ualg.html}
{http://www.math.uwaterloo.ca/~snburris/htdocs/ualg.html}
\\(The Millennium Edition)
}%

\BiblioItem{Shilov single 3}
{
Г. Е. Шилов. Математический анализ,
Функции одного переменного, часть 3,
М., Наука, 1970
}%

\BiblioItem{Shilov}
{
Г. Е. Шилов. Математический анализ,
Функции нескольких вещественных переменных, части 1 - 2,
М., Наука, 1972
}%

\BiblioItem{Kolmogorov Fomin}
{
А. Н. Колмогоров, С. В. Фомин.
Элементы теории функций и функционального анализа.
М., Наука, 1976
}%

\BiblioItem{Lebedev Vorovich}
{
И. И. Ворович, Л. П. Лебедев,
Функциональный анализ и его приложения в механике сплошной среды,
М., Вузовская книга, 2000
}%

\BiblioItem
{Rashevsky}
{
П. К. Рашевский,
Риманова геометрия и тензорный анализ,\\
М., Наука, 1967
}%

\BiblioItem
{Kurosh: High Algebra}
{
А. Г. Курош,
Курс высшей алгебры,
М., Наука, 1968
}%

\BiblioItem
{Kurosh: General Algebra}
{
А. Г. Курош,
Общая алгебра, (лекции 1969 - 70 учебного года),
М., МГУ, 1970
}%

\BiblioItem
{Sabinin: Smooth Quasigroups}
{
Lev V. Sabinin, Smooth Quasigroups and Loops,
Kluwer Academic Publisher, 1999 
}%

\BiblioItem{Dubrovin Fomenko Novikov part 1}
{
Б. А. Дубровин, С. П. Новиков, А. Т. Фоменко,
Современная геометрия, Методы и приложения,\\
Том 1, Геометрия поверхностей, групп преобразований и полей,\\
Эдиториал УРСС, М. 1998
}%

\BiblioItem{Korn}
{
Г. Корн, Т. Корн,
Справочник по математике для научных работников и инженеров,
М., Наука, 1974
}%

\BiblioItem{Hocking Young Topology}
{
John G. Hocking, Gail S. Young,
Topology,\\
Courier Dover Publications, 1988
}%

\BiblioItem{Olver: Lie groups to differential equations}
{
П. Олвер,
Приложения групп Ли к дифференциальным уравнениям,\\
М. Мир, 1989
}%

\BiblioItem{Tartaglia}
{
Angelo Tartaglia and Matteo Luca Ruggiero,
Angular Momentum Effects in Michelson\Hyph Morley Type Experiments,
Gen.Rel.Grav. 34, 1371-1382 (2002),\\
eprint \href{http://arxiv.org/abs/gr-qc/0110015}{arXiv:gr-qc/0110015} (2001)
}%

\BiblioItem{Tomozawa}
{
Yukio Tomozawa, Speed of Light in Gravitational Fields, eprint
\href{http://arxiv.org/abs/astro-ph/0303047}{arXiv:astro-ph/0303047} (2004)
}%

\BiblioItem{Magueijo}
{
Joao Magueijo,
Covariant and locally Lorentz-invariant varying speed of light theories,
\href{http://prola.aps.org/abstract/PRD/v62/i10/e103521}{Phys. Rev. D 62, 103521} (2000),
eprint \href{http://arxiv.org/abs/gr-qc/0007036}{arXiv:gr-qc/0007036} (2000)
}%

\BiblioItem{Bassett}
{
Bruce A. Bassett, Stefano Liberati, Carmen Molina-Paris, and Matt Visser,
Geometrodynamics of variable-speed-of-light cosmologies,
\href{http://prola.aps.org/abstract/PRD/v62/i10/e103518}{Phys. Rev. D 62}, 103518 (2000),
eprint \href{http://arxiv.org/abs/astro-ph/0001441}{arXiv:astro-ph/0001441} (2000)
}%

\BiblioItem{C.A. Deavours The Quaternion Calculus}
{
C.A. Deavours, The Quaternion Calculus, 
American Mathematical Monthly, {\bf 80} (1973), pp. 995 - 1008
}%

\BiblioItem{Straumann}
{
Lochlainn O'Raifeartaigh and Norbert Straumann,
Gauge theory: Historical origins and some modern developments,
\href{http://prola.aps.org/abstract/RMP/v72/i1/p1_1}{Rev. Mod. Phys. 72, 1} (2000)
}%

\begin{otherlanguage}{english}
\BiblioItem{Lammerzahl}
{
Claus L\"ammerzahl, Mark P. Haugan,
On the interpretation of Michelson\Hyph Morley experiments,
%\href{http://www.sciencedirect.comyph /science?_ob=ArticleURL&_udi=B6TVM-42WP7CR-1&_user=10&_handle=W-WA-A-A-AZ-MsSAYZW-UUW-AUDDYZYZAU-WZCBYCEDW-AZ-U&_fmt=summary&_coverDate=04%2F23%2F2001&_rdoc=1&_orig=browse&_srch=%23toc%235538%232001%23997179995%23246657!&_cdi=5538&view=c&_acct=C000050221&_version=1&_urlVersion=0&_userid=10&md5=385478cda8c5568dea1aeaf0c43669da}
{Phys. Lett. A282 223-229} (2001),\\
eprint \href{http://arxiv.org/abs/gr-qc/0103052}{arXiv:gr-qc/0103052} (2001)
}%
\end{otherlanguage}

\begin{otherlanguage}{english}
\BiblioItem{0305117}
{
Holger Mueller, Sven Herrmann, Claus Braxmaier, Stephan Schiller, Achim Peters.
Modern Michelson-Morley Experiment using Cryogenic Optical Resonators.
eprint \href{http://arxiv.org/abs/physics/0305117}{arXiv:physics/0305117} (2003)
\\
Phys. Rev. Lett. 91:020401, 2003
}%
\end{otherlanguage}

\BiblioItem{0706.2031}
{
Holger Mueller, Paul Louis Stanwix, Michael Edmund Tobar,
Eugene Ivanov, Peter Wolf, Sven Herrmann, Alexander Senger,
Evgeny Kovalchuk, Achim Peters.
Relativity tests by complementary rotating Michelson-Morley experiments.
eprint \href{http://arxiv.org/abs/0706.2031}{arXiv:0706.2031 [physics.class-ph]} (2006)
\\
Phys. Rev. Lett. 99:050401, 2007
}%

\BiblioItem{1008.1205}
{
M. Nagel, K. M\"ohle, K. D\"oringshoff, S. Herrmann, A. Senger, E.V. Kovalchuk, A. Peters.
Testing Lorentz Invariance by Comparing Light Propagation in Vacuum and Matter.
eprint \href{http://arxiv.org/abs/1008.1205}{arXiv:1008.1205 [physics.ins-det]} (2010)
}%

\BiblioItem{1109.4897}
{
The OPERA Collaboration.
Measurement of the neutrino velocity with the OPERA detector in the CNGS beam.
eprint \href{http://arxiv.org/abs/1109.4897}{arXiv:1109.4897 [hep-ex]} (2011)
}%

\begin{otherlanguage}{english}
\BiblioItem{Ranada}
{
Antonio F. Ranada,
Pioneer acceleration and variation of light speed: experimental situation,
eprint \href{http://arxiv.org/abs/gr-qc/0402120}{arXiv:gr-qc/0402120} (2004)
}%
\end{otherlanguage}

\BiblioItem{Gelfand Minlos: rotation and Lorentz groups}
{
И. М. Гельфанд, Р. А. Минлос, З. Я. Шапиро,
Представления группы вращений и группы Лоренца, их применения,\\
М., Наука, 1958
}%

\BiblioItem{math.QA-0208146}
{
I. Gelfand, S. Gelfand, V. Retakh, R. Wilson,
Quasideterminants,\\
eprint \href{http://arxiv.org/abs/math.QA/0208146}{arXiv:math.QA/0208146} (2002)
}%

\BiblioItem{q-alg-9705026}
{
I. Gelfand, V. Retakh,
Quasideterminants, I,\\
eprint \href{http://arxiv.org/abs/q-alg/9705026}{arXiv:q-alg/9705026} (1997)
}%

\BiblioItem{Gelfand Retakh 1991}
{
И. М. Гельфанд, В. С. Ретах,  Детерминанты матриц над некоммутативными кольцами,
\textit{Функциональный анализ и его приложения} {\bf 25}(2), c. 13-35, (1991).
}%

\BiblioItem{Gelfand Retakh 1992}
{
И. М. Гельфанд, В. С. Ретах,  Теория некоммутативных
детерминантов и характеристические функции графов,\\
\textit{Функциональный анализ и его приложения} {\bf 26} (4), c.
33-45, (1992).
}%

\BiblioItem{hep-th-9407124}
{
I. M. Gelfand, D. Krob, A. Lascoux, B. Leclerc, V.S. Retakh and J.-Y. Thibon,
Noncommutative symmetric functions,\\
eprint \href{http://arxiv.org/abs/hep-th/9407124}{arXiv:hep-th/9407124} (1994)
}%

\BiblioItem{Naimark Shtern: Theory of group representations}
{
М. А. Наймарк,
Теория представления групп,\\
М., Наука, 1976
}%

\BiblioItem{Barut Raczka: Theory of group representations}
{
А. Барут, Р. Рончка,
Теория представления групп и её приложения,\\
Перевод с английского А. У. Климыка и А. М. Гаврилика
под редакцией Я. А. Смородинского,\\
М., Мир, 1980
}%

\BiblioItem{Mihalev Pilz: concise handbook of algebra}
{
Aleksandr Vasilevich Mikhalev; G\"{u}nter Pilz;
The concise handbook of algebra;\\
Kluwer Academic Publishers, 2002
}%

\BiblioItem{Shafarevich: Basic notions of algebra}
{
И. Р. Шафаревич,
Основные понятия алгебры,\\
В сборнике "Современные проблемы математики. Фундаментальные направления
(Итоги науки и техники. ВИНИТИ АН СССР",
М., 1986, {\bf 11} 3 - 289
М., Мир, 1980
}%

\BiblioItem{Elsgolts: Differential Equations}
{
Л. Э. Эльсгольц,
Дифференциальные уравнения и вариационное исчисление,
М., Наука, 1971 
}%

\BiblioItem{Baez Huerta: algebra of grand unified theories}
{
John Baez; John Huerta;
The algebra of grand unified theories;\\
Bull. Amer. Math. Soc. {\bf 47} (2010), 483-552
}%

\BiblioItem{J. Fan: Determinants}
{
J. Fan, Determinants and multiplicative functionals
on quaternion matrices, \textit{Linear Algebra and Its
Applications} {\bf 369}, pp. 193-201, (2003).
}%

\BiblioItem{Carl Faith 1}
{
К. Фейс, Алгебра: кольца, модули и категории, том I,
М., Мир, 1973
}%

\BiblioItem{Gilson Nimmo Ohta}
{
 C.R.Gilson, J.J.C.Nimmo, Y.Ohta, Quasideterminant solutions of a non-Abelian Hirota-Miwa
 equation, \textit{Journal of Physics A: Mathematical and Theoretical} {\bf 40}(42), pp.
 12607-12617,(2007).
}%

\BiblioItem{Haider Hassan}
{
B. Haider, M. Hassan, Quasideterminant solutions of an integrable chiral model in two
 dimensions, \textit{Journal of Physics A: Mathematical and Theoretical} {\bf 42} (35), art. no.
 355211, (2009).
}%

%\BiblioItem{Pareigis}
%{
%Bodo Pareigis, Categories and Functors,
%Academic Press - New York - London, 1970
%}%

%\BiblioItem{Beachy}
%{
%John A. Beachy, Introductory Lectures on Rings i Modules,
%Cambridge University Press, 1999
%}%

\BiblioItem{0702447}
{
I.I. Kyrchei, Cramer's rule for quaternion systems of linear equations,
\textit{Journal of Mathematical Sciences} {\bf 155}(6), 839-858, (2008).
 Translated from  \textit{Fundamental and Appl. Math.}
 {\bf 13}(4), pp.67-94, (2007). (in Russian)\\
eprint
\href{http://arxiv.org/abs/math/0702447}{arXiv:math.RA/0702447}
(2007)
}%

\BiblioItem{1004.4380}
{
I.I. Kyrchei, Cramer's rule for some quaternion matrix
    equations,  \textit{Applied Mathematics and Computation} {\bf 217}(5), pp.2024-2030, (2010).\\eprint
\href{http://arxiv.org/abs/1004.4380
}{arXiv:math.RA/arXiv:1004.4380 } (2010)
}%

\BiblioItem{1005.0736}
{
I.I. Kyrchei,Determinantal representations of the Moore-Penrose inverse
 over the quaternion skew field and corresponding Cramer's rules,
 \\
eprint
\href{http://arxiv.org/abs/1005.0736}{arXiv:math.RA/1005.0736}
(2010)
}%

\BiblioItem{0412.391}
{
Александр Клейн,
Многообразие базисов,\\
eprint \href{http://arxiv.org/abs/math.DG/0412391}{arXiv:math.DG/0412391} (2007)
}%

\BiblioItem{0405.027}
{
Александр Клейн,
Система отсчета в общей теории относительности,
eprint \href{http://arxiv.org/abs/gr-qc/0405027}{arXiv:gr-qc/0405027} (2008)
}%

\BiblioItem{0405.028}
{
Александр Клейн,
Метрико\hyph аффинное многообразие,\\
eprint \href{http://arxiv.org/abs/gr-qc/0405028}{arXiv:gr-qc/0405028} (2008)
}%

\BiblioItem{0612.111}
{
Александр Клейн,
Бикольцо матриц,\\
eprint \href{http://arxiv.org/abs/math.OA/0612111}{arXiv:math.OA/0612111} (2007)
}%

\BiblioItem{0701.238}
{
Александр Клейн,
Лекции по линейной алгебре над телом,\\
eprint \href{http://arxiv.org/abs/math.GM/0701238}{arXiv:math.GM/0701238} (2010)
}%

\BiblioItem{0702.561}
{
Александр Клейн,
Расслоенная $\mathfrak{F}$\Hyph алгебра,\\
eprint \href{http://arxiv.org/abs/math.DG/0702561}{arXiv:math.DG/0702561} (2007)
}%

\BiblioItem{math.RA-0501237}
{
Александр Клейн,
Векторное пространство над телом,\\
eprint \href{http://arxiv.org/abs/math.RA/0412391}{arXiv:math.RA/0501237} (2007)
}%

\BiblioItem{math.RA-0501237v1}
{
Aleks Kleyn,
Module Over Division Ring, version 1,\\
eprint \href{http://arxiv.org/abs/math/0501237v1}{arXiv:math.RA/0501237v1} (2005)
}%

\BiblioItem{0707.2246}
{
Александр Клейн,
Расслоенное соответствие,\\
eprint \href{http://arxiv.org/abs/0707.2246}{arXiv:0707.2246} (2007)
}%

\BiblioItem{0803.2620}
{
Александр Клейн,
Морфизм \Ts представлений,\\
eprint \href{http://arxiv.org/abs/0803.2620}{arXiv:0803.2620} (2008)
}%

\BiblioItem{0803.3276}
{
Александр Клейн,
Преобразование Лоренца и принцип общековариантности,\\
eprint \href{http://arxiv.org/abs/0803.3276}{arXiv:0803.3276} (2009)
}%

\BiblioItem{0812.4763}
{
Александр Клейн,
Введение в математический анализ над телом,\\
eprint \href{http://arxiv.org/abs/0812.4763}{arXiv:0812.4763} (2010)
}%

\BiblioItem{0906.0135}
{
Александр Клейн,
Введение в геометрию над телом,\\
eprint \href{http://arxiv.org/abs/0906.0135}{arXiv:0906.0135} (2010)
}%

\BiblioItem{0909.0855}
{
Александр Клейн,
Этюд о кватернионах,\\
eprint \href{http://arxiv.org/abs/0909.0855}{arXiv:0909.0855} (2010)
}%

\BiblioItem{0912.3315}
{
Александр Клейн,
Представление универсальной алгебры,\\
eprint \href{http://arxiv.org/abs/0912.3315}{arXiv:0912.3315} (2010)
}%

\BiblioItem{0912.4061}
{
Александр Клейн,
Линейное уравнение в конечномерной алгебре,\\
eprint \href{http://arxiv.org/abs/0912.4061}{arXiv:0912.4061} (2010)
}%

\BiblioItem{1001.4852}
{
Александр Клейн,
Матрица линейных отображений,\\
eprint \href{http://arxiv.org/abs/1001.4852}{arXiv:1001.4852} (2010)
}%

\BiblioItem{1003.1544}
{
Александр Клейн,
Линейные отображения свободной алгебры,\\
eprint \href{http://arxiv.org/abs/1003.1544}{arXiv:1003.1544} (2010)
}%

\BiblioItem{1006.2597}
{
Александр Клейн,
Производная Гато и интеграл над банаховой алгеброй,\\
eprint \href{http://arxiv.org/abs/1006.2597}{arXiv:1006.2597} (2010)
}%

\BiblioItem{1011.3102}
{
Александр Клейн,
Полилинейное отображение свободной алгебры,\\
eprint \href{http://arxiv.org/abs/1011.3102}{arXiv:1011.3102} (2010)
}%

\BiblioItem{1104.5197}
{
Александр Клейн,
$C^*$-рапсодия,\\
eprint \href{http://arxiv.org/abs/1104.5197}{arXiv:1104.5197} (2011)
}%

\BiblioItem{1105.4307}
{
Александр Клейн,
Алгебра с сопряжением,\\
eprint \href{http://arxiv.org/abs/1105.4307}{arXiv:1105.4307} (2011)
}%

\BiblioItem{1107.1139}
{
Александр Клейн,
Линейные отображения алгебры кватернионов,\\
eprint \href{http://arxiv.org/abs/1107.1139}{arXiv:1107.1139} (2011)
}%

\BiblioItem{1107.5037}
{
Александр Клейн,
Ортогональный базис и движение в финслеровой геометрии,\\
eprint \href{http://arxiv.org/abs/1107.5037}{arXiv:1107.5037} (2011)
}%

\BiblioItem{1202.6021}
{
Александр Клейн,
Отображения сопряжения алгебры кватернионов,\\
eprint \href{http://arxiv.org/abs/1202.6021}{arXiv:1202.6021} (2012)
}%

\BiblioItem{1211.6965}
{
Александр Клейн,
Свободная алгебра со счётным базисом,\\
eprint \href{http://arxiv.org/abs/1211.6965}{arXiv:1211.6965} (2012)
}%

\BiblioItem{8433-5163}
{
Aleks Kleyn,
Linear Maps of Free Algebra: First Steps in Noncommutative Linear Algebra,\\
Lambert Academic Publishing, 2010
}%

\BiblioItem{8443-0072}
{
Aleks Kleyn,
Representation Theory: Representation of Universal Algebra,\\
Lambert Academic Publishing, 2011
}%

\BiblioItem{CACAA.07.291}
{
Aleks Kleyn,
Introduction into Calculus over Division Ring.\\
Clifford Analysis, Clifford Algebras and their applications,
Vol 7, Issue 4, pages 291 - 355, 2012
}%

\BiblioItem{Lauve: Quantum coordinates}
{
A. Lauve, Quantum- and quasi-Plucker coordinates,
\textit{Journal of Algebra} {\bf 296}(2), pp.440-461,
(2006).
}%

\BiblioItem{Lewis D. W. Quaternion algebras}
{
Lewis D. W. Quaternion algebras and the algebraic legacy
of Hamilton's quaternions, \textit{Irish Math. Soc. Bulletin} {\bf
57}, pp. 41-64, (2006).
}%

\BiblioItem{0812.2865}
{
Jos\'e Miguel Figueroa-O'Farrill,
Three lectures on 3-algebras,
eprint \href{http://arxiv.org/abs/0812.2865}{arXiv:0812.2865} (2008)
}%

\BiblioItem{1202.0951}
{
Daniel Edward Clark,
Deconvolution of point processes,
eprint \href{http://arxiv.org/abs/1202.0951}{arXiv:1202.0951} (2012)
}%

\BiblioItem{1202.4546}
{
Ming-Liang Hu,
Disentanglement, Bell-nonlocality violation
and teleportation capacity of the decaying tripartite states,
eprint \href{http://arxiv.org/abs/1202.4546}{arXiv:1202.4546} (2012)
}%

\BiblioItem{1203.1629}
{
Borivoje Dakic, Yannick Ole Lipp, Xiaosong Ma, Martin Ringbauer,
Sebastian Kropatschek, Stefanie Barz, Tomasz Paterek, Vlatko Vedral,
Anton Zeilinger, Caslav Brukner, Philip Walther,
Quantum Discord as Optimal Resource for Quantum Communication,
eprint \href{http://arxiv.org/abs/1203.1629}{arXiv:1203.1629} (2012)
}%

\BiblioItem{Li Nimmo: Darboux transformations}
{
C.X.Li, J.J.C. Nimmo, Darboux transformations for a twisted
derivation and quasideterminant solutions to the super KdV
equation, \textit{Proceedings of the Royal Society A:
Mathematical, Physical and Engineering Sciences} {\bf 466} (2120),
pp. 2471-2493, (2010)
}%

\BiblioItem{Schiebold: Cauchy-type determinants}
{
C. Schiebold, Cauchy-type determinants and integrable
systems, \textit{Linear Algebra and Its Applications} {\bf 433}
(2), pp. 447-475, (2010)
}%

\BiblioItem{Suzuki: Noncommutative spectral decomposition}
{
T. Suzuki, Noncommutative
spectral decomposition with qua\-si\-de\-ter\-mi\-nant, \textit{Advances in
Mathematics} {\bf 217}(5), pp. 2141-2158, (2008)
}%

\BiblioItem{1105.3456}
{
C. W. F. Everitt, D. B. DeBra, B. W. Parkinson, J. P. Turneaure, J. W. Conklin,
M. I. Heifetz, G. M. Keiser, A. S. Silbergleit, T. Holmes, J. Kolodziejczak,
M. Al-Meshari, J. C. Mester, B. Muhlfelder, V. Solomonik, K. Stahl, P. Worden,
W. Bencze, S. Buchman, B. Clarke, A. Al-Jadaan, H. Al-Jibreen, J. Li, J. A. Lipa,
J. M. Lockhart, B. Al-Suwaidan, M. Taber, S. Wang,\\
Gravity Probe B: Final Results of a Space Experiment to Test General Relativity,\\
eprint \href{http://arxiv.org/abs/1105.3456}{arXiv:1105.3456[math-ph]} (2011)
}%

\BiblioItem{0009305}
{
G. S. Asanov.
Can Neutrinos and High-Energy Particles Test Finsler Metric of Space-Time?\\
eprint \href{http://arxiv.org/abs/hep-ph/0009305}{arXiv:hep-ph/0009305} (2000)
}%

\BiblioItem{Asanov 2004}
{
Г. С. Асанов.
Финслероид - пространство с углом и скалярным произведением.\\
Гиперкомплексные числа в геометрии и физике, {\bf 1}, 2004, с. 43 - 67
}%

\BiblioItem{1004.3007}
{
Sergiu I. Vacaru,
Principles of Einstein-Finsler Gravity and Perspectives in Modern Cosmology,\\
eprint \href{http://arxiv.org/abs/1004.3007}{arXiv:1004.3007[gr-qc]} (2010)
}%

\BiblioItem{1012.4148}
{
Sergiu I. Vacaru.
Principles of Einstein-Finsler Gravity and Cosmology.\\
eprint \href{http://arxiv.org/abs/1012.4148}{arXiv:1012.4148[physics.gen-ph]} (2010)
}%

\BiblioItem{1112.5641}
{
Christian Pfeifer, Mattias N.R. Wohlfarth.
Finsler geometric extension of Einstein gravity.\\
eprint \href{http://arxiv.org/abs/1112.5641}{arXiv:1112.5641[gr-qc]} (2011)
}%

\BiblioItem{0711.0056}
{
Zhe Chang, Xin Li.
Lorentz Invariance Violation and Symmetry in Randers\Hyph Finsler Spaces.\\
eprint \href{http://arxiv.org/abs/0711.0056}{arXiv:0711.0056[hep-th]} (2011)
}%

\BiblioItem{Rund Finsler geometry}
{
Х. Рунд,
Дифференциальная геометрия финслеровых пространств.
\\
Перевод с английского Г. С. Асанова под редакцией Э. Г. Позняка,
М., Наука, 1981
}%

\BiblioItem{Smirnov vol 1}
{
В. И. Смирнов,
Курс высшей математики, том первый.
\\
М., Наука, 1974
}%

\BiblioItem{Beem Dostoglou Ehrlich}
{
John K. Beem, Stamatis A. Dostoglou, Paul E. Ehrlich,
Advances in differential geometry and general relativity.
\\
American Mathematical Society, 2004
}%

\BiblioItem{978-0719033414}
{
Malcolm Pemberton, Nicholas Rau,
Mathematics for economists: an introductory textbook.
\\
Manchester University Press, November 2001; ISBN-13: 978-0719033414
}%

\BiblioItem{0 521 59180 5}
{
Cyrus D. Cantrell,
Modern mathematical methods for physicists and engineers.
\\
Cambridge University Press, 2000
}%

\BiblioItem{Arveson spectral theory}
{
William Arveson,
A short course on spectral theory.
\\
Springer - Verlag, New York, 2002
}%

\BiblioItem{Robert Hermann}
{
Robert Hermann,
Topics in the mathematics of quantum mechanics.
\\
Math Sci Press, 1973
}%

\BiblioItem{9705.009}%q-alg-9705009
{
John C. Baez,
An Introduction to n-Categories,\\
eprint \href{http://arxiv.org/abs/q-alg/9705009}{arXiv:q-alg/9705009} (1997)
}%

\BiblioItem{0105.155}
{
John C. Baez,
The Octonions,\\
eprint \href{http://arxiv.org/abs/math.RA/0105155}{arXiv:math.RA/0105155} (2002)
}%

\BiblioItem{John Baez: Math Blogs}
{
John C. Baez,
What do mathematicians need to know about blogging?,\\
Notices of the American Mathematical Society,
(2010), 3, {\bf 57}, 333,\\
\url{http://www.ams.org/notices/201003/rtx100300333p.pdf}
}%

\BiblioItem{Tolstoi about Anna Karenina}
{
Константин Паустовский. Золотая роза, в сборнике Книга скитаний.
Картя молдовеняскэ, Кишинёв, 1978
}%
%Л. Н. Толстой в воспоминаниях современиков, т. 1, М. 1955, с. 231 - 232

\BiblioItem
{Cohn: Universal Algebra}
{
П. Кон,
Универсальная алгебра,
М., Мир, 1968
}%

\BiblioItem
{Cohn: Skew Fields}
{
Paul M. Cohn,
Skew Fields,
Cambridge University Press, 1995
}%

\BiblioItem
{Maunder: Algebraic Topology}
{
C. R. F. Maunder,
Algebraic Topology,
Dover Publications, Inc, Mineola, New York, 1996
}%

\BiblioItem{Pommaret: Partial Differential Equations}
{
Ж. Поммаре,
Системы уравнений с частными производными и псевдогруппы Ли,
М., Мир, 1983
}%

\BiblioItem{Bourbaki: Set Theory}
{
Н. Бурбаки,
Теория множеств, перевод с французского Г. Н. Поварова и Ю. А.
Шихановича под редакцией В. А. Успенского,
М. Мир, 1965
}%

\BiblioItem{Bourbaki: Algebra 1}
{
Н. Бурбаки,
Алгебра: алгебраические структуры, линейная и полилинейная алгебра,
перевод с французского Д. А. Райкова,
М.,
государственное издательство физико\Hyph математической литературы, 1962
}%

\BiblioItem{Bourbaki: Algebra 2}
{
Н. Бурбаки,
Алгебра: алгебраические структуры, линейная и полилинейная алгебра,
перевод с французского Д. А. Райкова,
М.,
государственное издательство физико\Hyph математической литературы, 1962
}%

\BiblioItem
{Bourbaki: General Topology 1}
{
Н. Бурбаки,
Общая топология, основные структуры,
перевод с французского Д. А. Райкова,
М. Наука, 1968
}

\BiblioItem{Bourbaki: General Topology: Chapter 3 - 8}
{
Н. Бурбаки,
Общая топология. Топологические группы.
Числа и связанные с ними группы и пространства.
\\
перевод с французского С. Н. Крачковского под редакцией Д. А. Райкова,
\\
М. Наука, 1975
}

\BiblioItem{Bourbaki: General Topology: Chapter 5 - 10}
{
Н. Бурбаки,
Общая топология. Использование вещественных чисел в общей топологии.
\\
перевод с французского С. Н. Крачковского под редакцией Д. А. Райкова,
\\
М. Наука, 1975
}

\BiblioItem{Bourbaki: Topological Vector Space}
{
Н. Бурбаки,
Топологические векторные пространства,
перевод с французского Д. А. Райкова,
М. Иностранная литература, 1959
}

\BiblioItem{Bourbaki: Coxeter Group Lie}
{
Н. Бурбаки,
Группы и алгебры Ли, главы 4 - 6,
Перевод с французского А. И. Кострикина и А. Н. Тюрина
под редакцией А. И. Кострикина,
М. Мир, 1986
}

\BiblioItem{Bourbaki: Real Group Lie}
{
Н. Бурбаки,
Группы и алгебры Ли, Компактные вещественные группы,
Перевод с французского И. А. Кострикина под редакцией А. А. Кирилова,
М. Мир, 1986
}

\BiblioItem{Shabat: Complex Analysis}
{
Шабат Б. В.,
Введение в комплексный анализ,
М. Наука, 1969
}

\BiblioItem{Pontryagin: Topological Group}
{
Понтрягин Л. С.,
Непрерывные группы,
М. Едиториал УРСС, 2004
}

\BiblioItem
{Eisenhart: Riemannian Geometry}
{
Eisenhart,
Riemannian Geometry,
Princeton University Press, Princeton, 1949
}

\BiblioItem
{Eisenhart: Continuous Groups of Transformations}
{
Л. П. Эйзенхарт,
Непрерывные группы преобразований,
перевод с английского М. М. Постникова,
М. Иностранная литература, 1947
}

\BiblioItem
{Condon Odabasi}
{
Edward Uhler Condon, Halis Odabasi,
Atomic Structure,
CUP Archive, 1980
}

\BiblioItem{Postnikov: Differential Geometry}
{
Постников М. М.,
Лекции по геометрии, семестр IV, Дифференциальная геометрия,
М. Наука, 1983
}

\BiblioItem{Fihtengolts: Calculus volume 1}
{
Фихтенгольц Г. М.,
Курс дифференциального и интегрального исчисления, том 1,
М. Наука, 1969
}

\BiblioItem{Fihtengolts: Calculus volume 2}
{
Фихтенгольц Г. М.,
Курс дифференциального и интегрального исчисления, том 2,
М. Наука, 1969
}

\BiblioItem{Hatcher: Algebraic Topology}
{
Allen Hatcher,
Algebraic Topology,
Cambridge University Press, 2002
}

\BiblioItem{geometry of differential equations}
{
А. М. Виноградов, И. С. Красильщик, В. В. Лычагин,
Введение в геометрию нелинейных дифференциальных уравнений,
М. Наука, 1986
}

\BiblioItem{cohomological analysis}
{
A. M. Vinogradov,
Cohomological Analysis of Partial Differential Equations
and Secondary Calculus,
American Mathematical Society, 2001
}

\BiblioItem{0801.1734}
{
Brandon S. DiNunno, Richard A. Matzner,
The Volume Inside a Black Hole,\\
eprint \href{http://arxiv.org/abs/0801.1734v1}{arXiv:0801.1734v1} (2008)
}

\BiblioItem{0702.447}
{
Ivan Kyrchei,
Cramer's rule for some quaternion matrix equations,\\
eprint \href{http://arxiv.org/abs/math/0702447}{arXiv:math.RA/0702447} (2007)
}

\BiblioItem{Izrail M. Gelfand: Quaternion Groups}
{
I. M. Gelfand, M. I. Graev,
Representation of Quaternion Groups over Localy Compact and
Functional Fields,\\
Functs. Anal. Prilozh. {\bf 2} (1968) 20 - 35;\\
Izrail Moiseevich Gelfand, Semen Grigorevich Gindikin,\\
Izrail M. Gelfand: Collected Papers, volume II, 435 - 449,\\
Springer, 1989
}

\BiblioItem{Richard D. Schafer}
{
Richard D. Schafer,
An Introduction to Nonassociative Algebras,
Dover Publications, Inc., New York, 1995
}

\BiblioItem{Bamberg Sternberg}
{
Paul Bamberg, Shlomo Sternberg,
A course in mathematics for students of physics,
Cambridge University Press, 1991
}

\BiblioItem{Conway Smith}
{
John Horton Conway, Derek Alan Smith,
On quaternions and octonions: their geometry, arithmetic, and symmetry,
A K Peters, Natick, Massachussets, 2003
}

\BiblioItem{Fueter}
{
Fueter, R.
Die Funktionentheorie der Differentialgleichungen $\Delta u = 0$ und
$\Delta \Delta u = 0$ mit vier reellen Variablen.
Comment. Math. Helv. {\bf 7} (1935), 307-330
}

\BiblioItem{Sudbery Quaternionic Analysis}
{
A. Sudbery,
Quaternionic Analysis,
Math. Proc. Camb. Phil. Soc. (1979), {\bf 85}, 199 - 225
}

\BiblioItem{0902.4771}
{
Fabrizio Colombo, Graziano Gentili, Irene Sabadini,
A Cauchy kernel for slice regular functions,\\
eprint \href{http://arxiv.org/abs/0902.4771v1}{arXiv:0902.4771v1} (2009)
}

\BiblioItem{Vadim Komkov}
{
Vadim Komkov,
Variational Principles of Continuum Mechanics with Engineering Applications: Critical Points Theory,\\
Springer, 1986
}

\BiblioItem{Alain Connes 1994}
{
Alain Connes,
Noncommutative Geometry,\\
Academic Press, 1994
}

\BiblioItem{Hamilton papers 3}
{
Sir William Rowan Hamilton,
The Mathematical Papers, Vol. III, Algebra,\\
Cambridge at the University Press, 1967
}

\BiblioItem{Hamilton Elements of Quaternions 1}
{
Sir William Rowan Hamilton,
Elements of Quaternions, Volume I,\\
Longmans, Green, and Co., London, New York, and Bombay, 1899
}

\BiblioItem{Cartan geometry in reper}
{
Эли Картан,
Риманова геометрия в ортогональном репере,
По лекциям Эли Картана, читанным в Сорбонне в 1926 - 1927 гг.,\\
перевод и редакция проф. С. П. Финикова,\\
издательство МГУ, 1960
}

\BiblioItem{Cartan differential form}
{
Анри Картан.
Дифференцииальное исчисление. Дифференциальные формы.\\
М. Мир, 1971
}

\BiblioItem{Arnautov Glavatsky Mikhalev}
{
V. I. Arnautov, S. T. Glavatsky, A. V. Mikhalev,\\
Introduction to the theory of topological rings and modules,
Volume 1995,\\
Marcel Dekker, Inc, 1996
}

\BiblioItem{Moore Yaqub}
{
Hal G. Moore, Adil Yaqub,
A first course in linear algebra with applications,
Edition 3, Academic Press, 1998 
}

\BiblioItem{math.CV-0405471}
{
S. V. Ludkovsky,
Differentiable functions of Cayley-Dickson numbers,\\
eprint \href{http://arxiv.org/abs/math.CV/0405471}{arXiv:math.CV/0405471} (2004)
}%

\BiblioItem{W.Bertram H.Glockner K.Neeb}
{
W.Bertram, H.Glockner, K.Neeb,
Differential Calculus over General Base Fields and Rings,
Expositiones Mathematicae (2004), Volume 22, Issue 3, Pages 213-282
}

\CloseBiblio



==> Commands.tex <==
%auto-ignore
\def\Defined{}
\scrollmode
\ifx\FilePrefix\undefined
\newcommand{\FilePrefix}{}
\fi
\ifx\UseRussian\Defined
\usepackage{cmap}
%\usepackage{cmcyralt}
%\usepackage{cmcyr}
%\usepackage{lhcyr}
%\usepackage{cmlgc}
%\ifx\PublishBook\undefined
\usepackage[T2A,T2B]{fontenc}
%\fi
\usepackage[cp1251]{inputenc}
\usepackage[english,russian]{babel}
\selectlanguage{russian}
\fi
\ifx\GJSFRA\Defined
\paperheight 297mm\paperwidth 210mm
\usepackage[top=1.905cm,bottom=1.905cm,inner=1.65cm,outer=1.65cm]{geometry}
\fi
\ifx\Presentation\Defined
\paperheight 215pt
\paperwidth 480pt
\usepackage[margin=1cm]{geometry}
\fi
\ifx\CreateSpace\Defined
%page size  = 6    x 9   inches
%\paperheight 228.6mm\paperwidth 152.4mm
%page size  = 7    x 10   inches
\paperheight 254mm\paperwidth 177.8mm
%\paperheight 257mm\paperwidth 182mm
\usepackage[top=1.905cm,bottom=1.905cm,inner=1.905cm,outer=1.27cm]{geometry}
\fi
\ifx\PublishBook\Defined
%use class \documentclass[12pt]{amsbook}
\def\PrintPaper{}
%page size  = 8.27    x 11.69   inches
%           = 21.0    x 29.7    cm
%           = 600.0   x 848.36  pt
%1 inch/дюйм = 2.54 см
%1 pt = .35 mm = .035 cm
%1 pc = 12 pt
% left/right margin = 2 cm = 57.14 pt
\usepackage{setspace}
\ifx\UseRussian\undefined
\usepackage{pslatex}
\fi
\onehalfspacing
\paperheight 297mm\paperwidth 210mm
% текст начинается на расстоянии 1 дюйм + oddsidemargin от левого края
%%%%\oddsidemargin=-.54cm
%%%%\evensidemargin=-.54cm
%%%\marginparwidth=2cm
%%%%\textwidth=17cm
% top/bottom margin = 2 cm = 57.14pt
\usepackage[margin=2cm]{geometry}
\fi
\raggedbottom
%\usepackage{ifthen}
\usepackage{footmisc}
%\usepackage[fixpdftex]{xcolor}
\usepackage[all]{xy}
\usepackage{color}
\ifx\PrintPaper\undefined
\definecolor{UrlColor}{rgb}{.9,0,.3}
\definecolor{SymbColor}{rgb}{.4,0,.9}
\definecolor{IndexColor}{rgb}{1,.3,.6}
\newcommand\BlueText[1]{\textcolor{blue}{#1}}
\newcommand\RedText[1]{\textcolor{red}{#1}}
\else
\definecolor{UrlColor}{rgb}{.1,.1,.1}
\definecolor{SymbColor}{rgb}{.1,.1,.1}
\definecolor{IndexColor}{rgb}{.1,.1,.1}
\newcommand\BlueText[1]{#1}
\newcommand\RedText[1]{#1}
\fi

\usepackage{xr-hyper}
%\ifx\Presentation\undefined
\usepackage[unicode]{hyperref}
\hypersetup{pdfdisplaydoctitle=true}
%\hypersetup{pdftex}
\hypersetup{colorlinks}
\hypersetup{citecolor=UrlColor}
\hypersetup{urlcolor=UrlColor}
\hypersetup{linkcolor=UrlColor}
\hypersetup{pdffitwindow=true}
\hypersetup{pdfnewwindow=true}
\hypersetup{pdfstartview={FitH}}
%\fi

\newcounter{Index}
\newcounter{Symbol}

\def\hyph{\penalty0\hskip0pt\relax-\penalty0\hskip0pt\relax}
\def\Hyph{-\penalty0\hskip0pt\relax}

\renewcommand{\arraystretch}{1.5}

\def\ValueOff{off}
\def\ValueOn{on}
\def\Items#1{\ItemList#1,LastItem,}%
\def\LastItem{LastItem}%
\def\ItemList#1,{\def\ViewBook{#1}%
\ifx\ViewBook\LastItem%
\else%
\ifx\ViewBook\BookNumber%
\def\Semafor{on}%
\fi%
\expandafter\ItemList%
\fi%
}%

\newcommand{\ePrints}[1]
{%
\def\Semafor{off}%
\Items{#1}%
}%

\newcommand{\Basis}[1]{\overline{\overline{#1}}{}}
\newcommand{\Vector}[1]{\overline{#1}{}}
%\newcommand{\Basis}[1]{{}_\star #1^\star{}}
%\newcommand{\Vector}[1]{#1^\star{}}
%%\newcommand{\Basis}[1]{\boldsymbol{\overset{\rightarrow}{#1}}}
%%\newcommand{\Vector}[1]{\overset{\rightarrow}{#1}}
\ifx\PrintPaper\undefined
\newcommand{\gi}[1]{\boldsymbol{\textcolor{IndexColor}{#1}}}
\else
\newcommand{\gi}[1]{\boldsymbol{#1}}
\fi
\newcommand\gii{\gi i}
\newcommand\giI{\gi I}
\newcommand\gij{\gi j}
\newcommand\giJ{\gi J}
\newcommand\gik{\gi k}
\newcommand\gil{\gi l}
\newcommand\gin{\gi n}
\newcommand\gim{\gi m}
\newcommand\giA{\gi 1}
\newcommand{\bVector}[2]{\Vector{#1}_{\gi{#2}}}
\newcommand{\VX}[1]{\Vector{#1}_{[1]}}
\makeatletter
\newcommand{\NameDef}[1]{%
\expandafter\gdef\csname #1\endcsname%
}%
\newcommand{\xNameDef}[1]{%
\expandafter\xdef\csname #1\endcsname%
}%
\newcommand{\ShowSymbol}[1]{%
\@nameuse{ViewSymbol#1}%
}%
\newcommand{\symb}[3]{%
\@ifundefined{ViewSymbol#3}{%
\NameDef{ViewSymbol#3}{\textcolor{SymbColor}{#1}}%
\xNameDef{RefSymbol#3}{:}%
\@namedef{LabeSymbol}{\label{symbol: #3::}}%
}{%
\addtocounter{Symbol}{1}%
\xNameDef{RefSymbol#3}{\@nameuse{RefSymbol#3},\arabic{Symbol}}%
\@namedef{LabeSymbol}{\label{symbol: #3:\arabic{Symbol}}}%
}%
\ifcase#2%0
\or%1
$\@nameuse{ViewSymbol#3}$%
\or%2
\[\@nameuse{ViewSymbol#3}\]%
\else%
\fi%
\@nameuse{LabeSymbol}%
}%
\newcommand{\DefEq}[2]{%
\@ifundefined{ViewEq#2}{%
\NameDef{ViewEq#2}{#1}%
}{%
%\errmessage {second DefEq #2}%
}%
}%
\newcommand{\DefEquation}[2]{%
\DefEq
{
\begin{equation}
#1
\EqLabel{#2}
\end{equation}
}
{#2}
}%
\newcommand\EqRef[1]{\eqref{eq: #1}}%
\newcommand\eqRef[2]{\EqRef{#1, #2}}%
\newcommand\EqLabel[1]{\label{eq: #1}}%
\newcommand\ShowEq[1]{%
\@ifundefined{ViewEq#1}{%
\message {error: missed ShowEq #1}
  }{%
\@nameuse{ViewEq#1}%
}%
}%
\newcommand\DrawEq[2]{%
\@ifundefined{ViewEq#1}{%
\message {error: missed ShowEq #1}%
  }{%
\def\Temp{}%
\def\Tempa{#2}%
\ifx\Tempa\Temp%
\[%
\@nameuse{ViewEq#1}%
\]%
\else%
\begin{equation}%
\@nameuse{ViewEq#1}%
\EqLabel{#1, #2}%
\end{equation}%
\fi%
}%
}%
%%\newcommand{\ShowEq}[2]{%
%%\ifcase#1%0
%%$\@nameuse{ViewEq#2}$%
%%\or%1
%%\[%
%%\@nameuse{ViewEq#2}%
%%\]$%
%%\or%2
%%\begin{equation}%
%%\@nameuse{ViewSymbol#3}%
%%\@nameuse{LabelSymbol#3}%
%%\end{equation}
%%\else%
%%\fi%
%%}%
\makeatother
\DeclareMathOperator{\rank}{\mathrm{rank}} 
\DeclareMathOperator{\id}{\mathrm{id}} 
\DeclareMathOperator{\const}{\mathrm{const}} 
\newcommand{\subs}{${}_*$\Hyph}
\newcommand{\sups}{${}^*$\Hyph}
\newcommand{\gS}{$*$\Hyph}
\newcommand{\CRstar}{{}^*{}_*}
\newcommand{\RCstar}{{}_*{}^*}
\newcommand{\CRcirc}{{}^{\circ}{}_{\circ}}
\newcommand{\RCcirc}{{}_{\circ}{}^{\circ}}
\newcommand{\Star}{*}
\newcommand{\RC}{$\RCstar$\Hyph}
\newcommand{\CR}{$\CRstar$\Hyph}
\newcommand{\drc}{$D\RCstar$\Hyph}
\newcommand{\Drc}{$\mathcal D\RCstar$\Hyph}
\newcommand{\dcr}{$D\CRstar$\hyph}
\newcommand{\rcd}{$\RCstar D$\Hyph}
\newcommand{\crd}{$\CRstar D$\Hyph}
\newcommand{\Arc}{$A\RCcirc$\Hyph}
\newcommand{\Acr}{$A\CRcirc$\Hyph}
\newcommand{\rcA}{$\RCcirc A$\Hyph}
\newcommand{\crA}{$\CRcirc A$\Hyph}
\newcommand{\RCPower}[1]{#1\RCstar}
\newcommand{\CRPower}[1]{#1\CRstar}
\newcommand{\RCInverse}{\RCPower{-1}}
\newcommand{\CRInverse}{\CRPower{-1}}
\newcommand{\RCRank}{\rank_{\RCstar}}
\newcommand{\CRRank}{\rank_{\CRstar}}
%\newcommand{\RCDet}[1]{|#1,\RCstar|}
%\newcommand{\CRDet}[1]{|#1,\CRstar|}
%\newcommand{\RCDet}[1]{\det\left(#1,\RCstar\right)}
%\newcommand{\CRDet}[1]{\det\left(#1,\CRstar\right)}
\newcommand\RCDet{\det(\RCstar)}
\newcommand\CRDet{\det(\CRstar)}
\newcommand{\RCGL}[2]{GL_{#1}^{\RCstar #2}}
\newcommand{\CRGL}[2]{GL_{#1}^{\CRstar #2}}
\newcommand\sT{$\star T$\Hyph}%
\newcommand\Ts{$T\star$\Hyph}%
\newcommand\sD{$\star D$\Hyph}%
\newcommand\Ds{$D\star$\Hyph}%
\newcommand\VirtFrac{\vphantom{\overset{\rightarrow}{\frac 11}^{\frac 11}}}
\newcommand\VirtVar{\vphantom{\overset{\rightarrow}{1}^1}}
%%\newcommand\pC[2]{{}_{\underline{#1}}^{#2}}%
%%\newcommand\pC[2]{{}^{#1}_{#2}}%
%\newcommand\pC[2]{{}_{#1(#2)}}%
\newcommand\pC[2]{{}_{#1\cdot #2}}%
%\newcommand\pC[2]
%{
%\def\tempa{0}%
%\def\tempb{#2}%
%\ifx\tempa\tempb%
%{}^{#1}%
%\else%
%{}_{#1#2}
%\fi%
%}%
\newcommand\DcrPartial[1]%
{%
\def\tempa{}%
\def\tempb{#1}%
\ifx\tempa\tempc%
(\partial\CRstar)%
\else%
(\partial_{\gi{#1}}\CRstar)%
\fi%
}%
\newcommand\rcDPartial[1]%
{%
\def\tempa{}%
\def\tempb{#1}%
\ifx\tempa\tempc%
(\RCstar\partial)%
\else%
(\RCstar\partial_{\gi{#1}})%
\fi%
}%
%\newcommand\StandPartial[4]%
%{%
%\def\tempa{}%
%\def\tempb{#3}%
%\def\tempc{#4}%
%\ifx\tempa\tempb%
%\else%
%{\vphantom{\frac{#1}{#2}}}^{#3}\!%
%\fi%
%\left(\frac{\partial #1}{\partial #2}%
%\ifx\tempa\tempc%
%\right)%
%\else%
%\right)^{#4}%
%\fi%
%}%
\newcommand\StandPartial[3]%
{%
%\left(\frac{\partial #1}{\partial #2}\right)^{\gi{#3}}%
\frac{\partial^{\gi{#3}} #1}{\partial #2}%
}%

%\ifx\Presentation\undefined
\renewcommand{\uppercasenonmath}[1]{}
%\fi
\renewcommand{\MakeUppercase}[1]{#1}
\makeatletter
\newcommand\@dotsep{4.5}
\def\@tocline#1#2#3#4#5#6#7
{\relax
%\ifnum #1>\c@tocdepth % then omit
%\else
\par \addpenalty\@secpenalty\addvspace{#2}%
\begingroup %\hyphenpenalty\@M
\@ifempty{#4}{%
\@tempdima\csname r@tocindent\number#1\endcsname\relax
}{%
\@tempdima#4\relax
}%
\parindent\z@ \leftskip#3\relax \advance\leftskip\@tempdima\relax
\rightskip\@pnumwidth plus1em \parfillskip-\@pnumwidth
#5\leavevmode\hskip-\@tempdima #6\relax
\leaders\hbox{$\m@th
\mkern \@dotsep mu\hbox{.}\mkern \@dotsep mu$}\hfill
\hbox to\@pnumwidth{\@tocpagenum{#7}}\par
\nobreak
\endgroup
%\fi
}
\makeatother 

%I use macro PrintBook if I print book
%and chapter is primery counter.
%Otherwise section is primery counter.
\ifx\PrintBook\undefined
\def\Chapter{\section}
\def\Section{\subsection}
\makeatletter
%bibliography and index should be numbered sections
%\ifx\Presentation\undefined
\renewcommand{\@indextitlestyle}{%
\twocolumn[\section{\indexname}]%
\def\IndexSpace{off}%
}
%\fi
\makeatother 
%\ifx\Presentation\undefined
\ifx\PrintPaper\undefined
\thanks{\href{mailto:Aleks\_Kleyn@MailAPS.org}{Aleks\_Kleyn@MailAPS.org}}
\ePrints{1102.1776,1201.4158}
\ifx\Semafor\ValueOff
\thanks{\ \ \ \url{http://sites.google.com/site/AleksKleyn/}}
\thanks{\ \ \ \url{http://arxiv.org/a/kleyn\_a\_1}}
\thanks{\ \ \ \url{http://AleksKleyn.blogspot.com/}}
\fi
\fi
\else

\def\Chapter{\chapter}
\def\Section{\section}

%\ifx\Presentation\undefined
\pagestyle{headings}
%\fi
\makeatletter
%title page
\def\@maketitle{%
  \ifx\Title\undefined
  \else
	  \cleardoublepage \thispagestyle{empty}%
	  \begingroup \topskip\z@skip
	  \null\vfil
	  \begingroup
	  \LARGE\bfseries \centering
	  \openup\medskipamount
	  \Title
	  \par
	  \ifx\Subtitle\undefined
	  \else
	  \centerline{\emph\Subtitle}
	  \fi
	  \par\vspace{24pt}%
	  \def\and{\par\medskip}\centering
	  \mdseries\Authors\par\bigskip
	  \endgroup
	  \vfil
	  \ifx\@empty\addresses \else \@setaddresses \fi
	  \vfil
  \fi
  \cleardoublepage \thispagestyle{empty}%
  \begingroup \topskip\z@skip
  \null\vfil
  \begingroup
  \LARGE\bfseries \centering
  \openup\medskipamount
  \@title
  \par
  \ifx\subtitle\undefined
  \else
  \centerline{\emph\subtitle}
  \fi
  \ifx\subtitleA\undefined
  \else
  \centerline{\emph\subtitleA}
  \fi
  \ifx\titleNote\undefined
  \else
  \centerline{\mdseries\titleNote}
  \fi
  \par\vspace{24pt}%
  \def\and{\par\medskip}\centering
  \mdseries\authors\par\bigskip
  \endgroup
  \vfil
  \ifx\@empty\addresses \else \@setaddresses \fi
  \vfil
  \ifx\@empty\@dedicatory
  \else \begingroup
    \centering{\footnotesize\itshape\@dedicatory\@@par}%
    \endgroup
  \fi
  \vfill
  \newpage\thispagestyle{empty}
  \begin{center}
    \ifx\@empty\@subjclass\else\@setsubjclass\fi
    \ifx\@empty\@keywords\else\@setkeywords\fi
    \ifx\@empty\@translators\else\vfil\@settranslators\fi
    \ifx\@empty\thankses\else\vfil\@setthanks\fi
  \end{center}
  \vfil
  \@setabstract
  %\@setcopyright
\vfil
  \def\Temp{0000}
  \ifx\copyrightyear\Temp
  \else
  \begin{center}
\begin{tabular}{@{}c}
Copyright\ \copyright\ \copyrightyear\ \copyrightholder
\\
All rights reserved.
\end{tabular}
  \end{center}
  \fi
  \ifx\ISBN\undefined%
  \else%
  \begin{center}
\begin{tabular}{@{}r@{\ }l}
ISBN:&\ISBN
\\
ISBN-13:&\ISBNa
\end{tabular}
  \end{center}
  \fi%
  \endgroup}
%bibliography and index should be numbered chapters
\renewcommand{\@indextitlestyle}{%
\twocolumn[\chapter{\indexname}]%
\def\IndexSpace{off}%
\let\@secnumber\@empty
\chaptermark{\indexname}%
%\sectionmark{}%
}
\makeatother 
\email{\href{mailto:Aleks\_Kleyn@MailAPS.org}{Aleks\_Kleyn@MailAPS.org}}
\ePrints{1102.1776,1201.4158}
\ifx\Semafor\ValueOff
%\def\temp{1102.1776}
%\ifx\BookNumber\temp
%\else
\urladdr{\url{http://sites.google.com/site/alekskleyn/}}
\urladdr{\url{http://arxiv.org/a/kleyn\_a\_1}}
\urladdr{\url{http://AleksKleyn.blogspot.com/}}
\fi
\fi

\ifx\SelectlEnglish\undefined
\ifx\UseRussian\undefined
\def\SelectlEnglish{}
\fi
\fi

\newcommand\arXivRef{http://arxiv.org/PS_cache/}
\newcommand\wRefDef[2]
{
\def\Tempa{#1}
\def\Tempb{0405.027}
\ifx\Tempa\Tempb
\def\wRef{\arXivRef gr-qc/pdf/0405/0405027v3.pdf}
\fi
\def\Tempb{0405.028}
\ifx\Tempa\Tempb
\def\wRef{\arXivRef gr-qc/pdf/0405/0405028v5.pdf}
\fi
\def\Tempb{0412.391}
\ifx\Tempa\Tempb
\def\wRef{\arXivRef math/pdf/0412/0412391v4.pdf}
\fi
\def\Tempb{0612.111}
\ifx\Tempa\Tempb
\def\wRef{\arXivRef math/pdf/0612/0612111v2.pdf}
\fi
\def\Tempb{0701.238}
\ifx\Tempa\Tempb
\def\wRef{\arXivRef math/pdf/0701/0701238v4.pdf}
\fi
\def\Tempb{0702.561}
\ifx\Tempa\Tempb
\def\wRef{\arXivRef math/pdf/0702/0702561v3.pdf}
\fi
\def\Tempb{0707.2246}
\ifx\Tempa\Tempb
\def\wRef{\arXivRef arxiv/pdf/0707/0707.2246v2.pdf}
\fi
\def\Tempb{0803.3276}
\ifx\Tempa\Tempb
\def\wRef{\arXivRef arxiv/pdf/0803/0803.3276v3.pdf}
\fi
\def\Tempb{0812.4763}
\ifx\Tempa\Tempb
\def\wRef{\arXivRef arxiv/pdf/0812/0812.4763v6.pdf}
\fi
\def\Tempb{0906.0135}
\ifx\Tempa\Tempb
\def\wRef{\arXivRef arxiv/pdf/0906/0906.0135v3.pdf}
\fi
 \def\Tempb{0909.0855}
\ifx\Tempa\Tempb
\def\wRef{\arXivRef arxiv/pdf/0909/0909.0855v5.pdf}
\fi
 \def\Tempb{0912.3315}
\ifx\Tempa\Tempb
\def\wRef{\arXivRef arxiv/pdf/0912/0912.3315v2.pdf}
\fi
 \def\Tempb{0912.4061}
\ifx\Tempa\Tempb
\def\wRef{\arXivRef arxiv/pdf/0912/0912.4061v2.pdf}
\fi
 \def\Tempb{1003.1544}
\ifx\Tempa\Tempb
\def\wRef{\arXivRef arxiv/pdf/1003/1003.1544v2.pdf}
\fi
 \def\Tempb{1006.2597}
\ifx\Tempa\Tempb
\def\wRef{\arXivRef arxiv/pdf/1006/1006.2597v2.pdf}
\fi
 \def\Tempb{1104.5197}
\ifx\Tempa\Tempb
\def\wRef{\arXivRef arxiv/pdf/1104/1104.5197.pdf}
\fi
 \def\Tempb{1011.3102}
\ifx\Tempa\Tempb
\def\wRef{\arXivRef arxiv/pdf/1011/1011.3102.pdf}
\fi
 \def\Tempb{1105.4307}
\ifx\Tempa\Tempb
\def\wRef{\arXivRef arxiv/pdf/1105/1105.4307.pdf}
\fi
 \def\Tempb{1107.1139}
\ifx\Tempa\Tempb
\def\wRef{\arXivRef arxiv/pdf/1104/1107.1139.pdf}
\fi
 \def\Tempb{1107.5037}
\ifx\Tempa\Tempb
\def\wRef{\arXivRef arxiv/pdf/1107/1107.5037.pdf}
\fi
 \def\Tempb{1202.6021}
\ifx\Tempa\Tempb
\def\wRef{\arXivRef arxiv/pdf/1202/1202.6021.pdf}
\fi
 \def\Tempb{1211.6965}
\ifx\Tempa\Tempb
\def\wRef{\arXivRef arxiv/pdf/1211/1211.6965.pdf}
\fi
 \def\Tempb{8433-5163}
\ifx\Tempa\Tempb
\def\wRef{http://www.amazon.com/}
\fi
 \def\Tempb{8443-0072}
\ifx\Tempa\Tempb
\def\wRef{http://www.amazon.com/}
\fi
 \def\Tempb{CACAA.07.291}
\ifx\Tempa\Tempb
\def\wRef{http://www.cliffordanalysis.com/}
\fi
\externaldocument[#1-#2-]{\FilePrefix #1.#2}[\wRef]
}
\newcommand\LanguagePrefix{}%
\makeatletter
\newcommand\StartLabelItem[1]
{
\def\theenumi{\ref*{#1}.\@arabic\c@enumi}
\def\labelenumi{\theenumi:}
}
\newcommand\StopLabelItem
{
\def\theenumi{\@arabic\c@enumi}
\def\labelenumi{(\theenumi)}
}
\makeatother
\newcommand\RefItem[1]{\ref{item: #1}}
\ifx\SelectlEnglish\undefined
\newcommand\Input[1]{\input{\FilePrefix #1.Russian}}%
\newcommand\CurrentLanguage{Russian.}%
\author{Александр Клейн}
%\ifx\Presentation\undefined
\newtheorem{theorem}{Теорема}[section]
\newtheorem{corollary}[theorem]{Следствие}
\newtheorem{convention}[theorem]{Соглашение}
\theoremstyle{definition}
\newtheorem{definition}[theorem]{Определение}
\newtheorem{example}[theorem]{Пример}
\newtheorem{xca}[theorem]{Exercise}
\theoremstyle{remark}
\newtheorem{remark}[theorem]{Замечание}
%\theoremstyle{lemma}
\newtheorem{lemma}[theorem]{Лемма}
\newtheorem{Example}[theorem]{Example}
%\else
%\theoremstyle{remark}
%\newtheorem{remark}{Замечание}
%\fi
\newcommand\xRefDef[1]
{
\wRefDef{#1}{Russian}
\NameDef{xRefDef#1}{}%
}
\makeatletter
\newcommand\xRef[2]%
{%
\@ifundefined{xRefDef#1}{%
\ref{#2}%
}{% 
\citeBib{#1}-\ref{#1-Russian-#2}%
}%
}%
\newcommand\xEqRef[2]%
{%
\@ifundefined{xRefDef#1}{%
\eqref{eq: #2}%
}{%
\citeBib{#1}-\eqref{#1-Russian-eq: #2}%
}%
}%
\makeatother
\ifx\PrintBook\undefined
\newcommand{\BibTitle}{%
\section{Список литературы}%
}
\else
\newcommand{\BibTitle}{%
\chapter{Список литературы}%
}
\fi
\else
\newcommand\Input[1]{\input{\FilePrefix #1.English}}%
\newcommand\CurrentLanguage{English.}%
\author{Aleks Kleyn}
%\ifx\Presentation\undefined
\newtheorem{theorem}{Theorem}[section]
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{convention}[theorem]{Convention}
\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{example}[theorem]{Example}
\newtheorem{xca}[theorem]{Exercise}
\theoremstyle{remark}
\newtheorem{remark}[theorem]{Remark}
%\theoremstyle{lemma}
\newtheorem{lemma}[theorem]{Lemma}
%\else
%\theoremstyle{remark}
%\newtheorem{remark}{Remark}
%\fi
\newcommand\xRefDef[1]
{
\wRefDef{#1}{English}
\NameDef{xRefDef#1}{}%
}
\makeatletter
\newcommand\xRef[2]%
{%
\@ifundefined{xRefDef#1}{%
\ref{#2}%
}{% 
\citeBib{#1}-\ref{#1-English-#2}%
}%
}%
\newcommand\xEqRef[2]%
{%
\@ifundefined{xRefDef#1}{%
\eqref{eq: #2}%
}{%
\citeBib{#1}-\eqref{#1-English-eq: #2}%
}%
}%
\makeatother
\ifx\PrintBook\undefined
\newcommand{\BibTitle}{%
\section{References}%
}
\else
\newcommand{\BibTitle}{%
\chapter{References}%
}
\fi
\fi

\ifx\PrintBook\undefined
%\ifx\Presentation\undefined
\renewcommand\theHsection{\CurrentLanguage\arabic{section}}%
\numberwithin{Hfootnote}{section}
%\fi
\else
\numberwithin{section}{chapter}
\renewcommand\theHchapter{\CurrentLanguage\arabic{chapter}}%
\numberwithin{footnote}{chapter}
\numberwithin{Hfootnote}{chapter}
\fi

\ifx\Presentation\undefined
\numberwithin{equation}{section}
\numberwithin{figure}{section}
\numberwithin{table}{section}
\numberwithin{Item}{section}
\fi

\makeatletter
%to reuse the data of \maketitle:
\newcommand\org@maketitle{}
\let\org@maketitle\maketitle
\def\maketitle{%
\hypersetup{pdftitle={\@title}}%
\hypersetup{pdfauthor={\authors}}%
\hypersetup{pdfsubject=\@keywords}%
\ifx\UseRussian\Defined
\pdfbookmark[1]{\@title}{TitleRussian}
\else
\pdfbookmark[1]{\@title}{TitleEnglish}
\fi
\org@maketitle
}
%Let's patch \make@stripped@name so that the language-prefix
%gets inserted also:
\def\make@stripped@name#1{%
\begingroup
\escapechar\m@ne
\global\let\newname\@empty
%Formerly ---and that's the only modification---the
%next line was: "\protected@edef\Hy@tempa{#1}%"
\protected@edef\Hy@tempa{\CurrentLanguage #1}%
\edef\@tempb{%
\noexpand\@tfor\noexpand\Hy@tempa:=%
\expandafter\strip@prefix\meaning\Hy@tempa
}%
\@tempb\do{%
\if\Hy@tempa\else
\if\Hy@tempa\else
\xdef\newname{\newname\Hy@tempa}%
\fi
\fi
}%
\endgroup
}%
%I change environment for bibliography
%because labels for bibliography also need language prefix
\newenvironment{enumBib}{%
\BibTitle
\advance\@enumdepth \@ne
\edef\@enumctr{enum\romannumeral\the\@enumdepth}\list
{\csname biblabel\@enumctr\endcsname}{\usecounter
{\@enumctr}\def\makelabel##1{\hss\llap{\upshape##1}}}
}{%
\endlist
}
\let\endenumBib=\endlist % for efficiency
\def\biblabelenumi{[\LanguagePrefix \theenumi]}
\makeatletter

\newcommand{\BiblioItem}[2]
{
\def\Semafor{off}
\@ifundefined{\LanguagePrefix ViewCite#1}{}{%
\def\Semafor{on}%
}%
\ifx\Semafor\ValueOff
\@ifundefined{xRefDef#1}{}{% 
\def\Semafor{on}%
}%
\fi
\ifx\Semafor\ValueOn
\ifx\IndexState\ValueOff
\begin{enumBib}
\def\IndexState{on}
\fi
\item \label{\LanguagePrefix bibitem: #1}#2%
\fi
}
\makeatother
\newcommand{\OpenBiblio}
{
\def\IndexState{off}
}
\newcommand{\CloseBiblio}
{
\ifx\IndexState\ValueOn
\end{enumBib}
%\end{enumerate}
\def\IndexState{off}
\fi
}

\makeatletter
\def\StartCite{[}%
\def\citeBib#1{\protect\showCiteBib#1,endCite,}%
\def\endCite{endCite}%
\def\showCiteBib#1,{\def\temp{#1}%
\ifx\temp\endCite
]%
\def\StartCite{[}%
\else
\StartCite\LanguagePrefix \ref{\LanguagePrefix bibitem: #1}%
\@ifundefined{\LanguagePrefix ViewCite#1}{%
\NameDef{\LanguagePrefix ViewCite#1}{}%
}{%
}%
\def\StartCite{, }%
\expandafter\showCiteBib%
\fi}%
\makeatother

\newcommand\setPdfOutline[5]
{
%1-external link
%2-ref
%3-file
%4-anchor
%5-text in bookmark
\pdfstringdef\tempa{\ref{#1-#2} }
\pdfstringdef\tempb{#5}
\pdfoutline goto file{#3.pdf} name{#4} {\tempa\tempb}
}
\newcommand{\arp}{\ar @{-->}}
%\newcommand{\ars}{\ar @{{}*{*}>}}
%\newcommand{\ars}{\ar @*{[|(2)]}@{.>}}
\newcommand{\ars}{\ar @{.>}}
\newcommand\Bundle[1]{{\mathbb #1}}%{{\bf #1}}
\newcommand{\bundle}[4]%
{%
\def\tempa{}%
\def\tempb{#3}%
\def\tempc{#1}%
\ifx\tempa\tempb%
\ifx\tempa\tempc%
#2%
\else%
\xymatrix{#2:#1\arp[r]&#4}%
\fi%
\else%
\ifx\tempa\tempc%
#2[#3]%
\else%
\xymatrix{#2[#3]:#1\arp[r]&#4}%
\fi%
\fi%
}%
\makeatletter
\newcommand{\AddIndex}[2]%
{%
\@ifundefined{RefIndex#2}{%
\xNameDef{RefIndex#2}{:}%
\@namedef{LabelIndex}{\label{index: #2::}}%
}{%
\addtocounter{Index}{1}%
\xNameDef{RefIndex#2}{\@nameuse{RefIndex#2},\arabic{Index}}%
\@namedef{LabelIndex}{\label{index: #2:\arabic{Index}}}%
}%
\@nameuse{LabelIndex}%
{\bf #1}%
}%
\newcommand{\Index}[2]%
{%
\def\Semafor{off}%
\@ifundefined{RefIndex#2}{%
}{%
\def\Semafor{on}
}%
\ifx\Semafor\ValueOn%
\def\tempa{}%
\def\tempb{#2}%
\ifx\IndexState\ValueOff%
\begin{theindex}%
\def\IndexState{on}%
\fi%
\ifx\IndexSpace\ValueOn%
\indexspace%
\def\IndexSpace{off}%
\fi%
\item #1%
\ifx\tempa\tempb%
\else%
\edef\PageRefs{\@nameuse{RefIndex#2}}
\def\Sep{\ }%
\@for\PageRef:=\PageRefs\do{%
\Sep
\pageref{index: #2:\PageRef}%
\def\Sep{,\ }%
}%
\fi%
\fi%
}%
%\newcommand{\SubIndex}[3]
%{
%\def\Semafor{off}
%\Items{#1}
%\ifx\Semafor\ValueOn
%\subitem #2 \pageref{index: #3}%\RefPage{#3}
%\fi
%}%
%\newcommand{\AddIndexRef}[2]
%{%
%\def\Semafor{off}
%\Items{#1}
%\ifx\Semafor\ValueOn
%, \pageref{index: #2}%
%\fi%
%}%

\newcommand{\Symb}[2]
{
\def\Semafor{off}
\@ifundefined{ViewSymbol#2}{%
}{%
\def\Semafor{on}
}%
\ifx\Semafor\ValueOn
\ifx\IndexState\ValueOff
\begin{theindex}
\def\IndexState{on}
\fi
\ifx\IndexSpace\ValueOn
\indexspace
\def\IndexSpace{off}
\fi
\item $\displaystyle\@nameuse{ViewSymbol#2}$\ \ #1
\edef\PageRefs{\@nameuse{RefSymbol#2}}
\def\Sep{}%
\@for\PageRef:=\PageRefs\do{%
\Sep
\pageref{symbol: #2:\PageRef}%
\def\Sep{,\ }%
}%
\fi
}
%\def\CiteBibNote{\xdef\@thefnmark{}\@footnotetext}
\def\CiteBibNote{\footnote[0]}
\makeatother
%\newcommand{\SubSymb}[3]
%{
%\def\Semafor{off}
%\Items{#1}
%\ifx\Semafor\ValueOn
%\subitem #2 \pageref{symbol: #3}
%\fi
%}%
%\newcommand{\AddSymbRef}[2]
%{%
%\def\Semafor{off}
%\Items{#1}
%\ifx\Semafor\ValueOn
%, \pageref{symbol: #2}%
%\fi%
%}%

\newcommand{\SetIndexSpace}%
{%
\def\IndexSpace{on}%
}%

\newcommand{\OpenIndex}
{
\def\IndexState{off}
}
\newcommand{\CloseIndex}
{
\ifx\IndexState\ValueOn
\end{theindex}
\def\IndexState{off}
\fi
}
\newcommand\CiteQuotation[2]
{
\leftskip=40pt
\Memos{#1}
\begin{flushright}
\begin{tabular}{r}
\hline
\makebox[100pt][r]{#2}\\
\end{tabular}
\end{flushright}
\leftskip=0pt
}
\newcommand\CiteQuote[2]
{
\leftskip=40pt
\BlueText{#1}%
\begin{flushright}
\begin{tabular}{r}
\hline
\makebox[100pt][r]{#2}\\
\end{tabular}
\end{flushright}
\leftskip=0pt
}
\newcommand\epigraph[2]
{
%\leftskip=150pt
\Memos{#1}
\begin{flushright}
\begin{tabular}{r}
\hline
\makebox[100pt][r]{#2}\\
\end{tabular}
\end{flushright}
%\leftskip=0pt
}
\def\Memos#1{\MemoList#1//LastMemo//}%
\def\LastMemo{LastMemo}%
\def\MemoList#1//{\def\temp{#1}%
\ifx\temp\LastMemo
\else%
\begin{flushright}
\begin{minipage}{200pt}
\setlength{\parindent}{5mm}
%\par
%\setlength{\parindent}{12pt}
\BlueText{#1}%
\end{minipage}
\end{flushright}
\expandafter\MemoList%
\fi%
}%

%\newenvironment{epigraph1}
%{
%%    \leavevmode\unskip\penalty9999 \hbox{}\nobreak\hfill
%\begin{flushright}
%\begin{minipage}{200pt}
%\ \\
%
%}
%{
%\end{minipage}
%\end{flushright}
%}

\newenvironment{TextMath}
{
\begin{flushleft}
\begin{minipage}{\textwidth}
\setlength{\parindent}{12pt}
}
{
\end{minipage}
\end{flushleft}
}
\listfiles


==> Complex.Number.English.tex <==
%auto-ignore

\input{\FilePrefix Complex.Number.Eq}

\ePrints{Calculus.Paper}
\ifx\Semafor\ValueOn
\Section{Linear Function of Complex Field}
\else
\section{Linear Function of Complex Field}
\fi
\label{section: Function of Complex Field}

\begin{theorem}[the Cauchy\Hyph Riemann equations]
\label{theorem: complex field over real field}
Let us consider complex field $C$ as two-dimensional algebra over real field.
Let
\ShowEq{basis of complex field}
be the basis of algebra $C$.
\ePrints{Calculus.Paper}
\ifx\Semafor\ValueOff
Then in this basis product has form
\ShowEq{product of complex field}
and structural constants have form
\ShowEq{structural constants of complex field}
\fi%Calculus.Paper
Matrix of linear function
\[
y^{\gi i}=x^{\gi j}f_{\gi j}^{\gi i}
\]
of complex field over real field
satisfies relationship
\begin{align}
\EqLabel{complex field over real field, 0}
f_{\gi 0}^{\gi 0}&=f_{\giA}^{\giA}
\\
\EqLabel{complex field over real field, 1}
f_{\gi 0}^{\giA}&=-f_{\giA}^{\gi 0}
\end{align}
\end{theorem}
\begin{proof}
\ePrints{Calculus.Paper}
\ifx\Semafor\ValueOff
Equations
\EqRef{product of complex field} and
\EqRef{structural constants of complex field}
follow from equation $i^2=-1$.
Using equation
\xEqRef{0812.4763}{linear map over field, division ring, relation}
we get relationships
\ShowEq{complex field over real field}
\EqRef{complex field over real field, 0}
follows from equations
\EqRef{complex field over real field, 0, 0} and
\EqRef{complex field over real field, 0, 1}.
\EqRef{complex field over real field, 1}
follows from equations
\EqRef{complex field over real field, 1, 0} and
\EqRef{complex field over real field, 1, 1}.
\else%Calculus.Paper
See the proof of the theorem
\xRef{8433-5163}{theorem: complex field over real field}.
\fi%Calculus.Paper
\end{proof}

\ePrints{0701.238,1003.1544,8433-5163}
\ifx\Semafor\ValueOff
\begin{theorem}[the Cauchy\Hyph Riemann equations]
Since matrix
\ShowEq{Jacobian of map of complex variable}
is Jacobian matrix of map of complex variable
\[
x=x^{\gi 0}+x^{\giA}i\rightarrow y=y^{\gi 0}(x^{\gi 0},x^{\giA})+y^{\giA}(x^{\gi 0},x^{\giA})i
\]
over real field,
then
\ShowEq{Cauchy Riemann equations, complex field, 1}
\end{theorem}
\begin{proof}
The statement of theorem is
corollary of theorem
\ref{theorem: complex field over real field}.
\end{proof}

\begin{theorem}
Derivative of function of complex variable satisfyes to equation
\ShowEq{Cauchy Riemann equations, complex field, 2}
\end{theorem}
\begin{proof}
Equation
\ShowEq{Cauchy Riemann equations, complex field, 2, 1}
follows from equations
\EqRef{Cauchy Riemann equations, complex field, 1}.
\end{proof}

\ePrints{Calculus.Paper}
\ifx\Semafor\ValueOff
Equation \EqRef{Cauchy Riemann equations, complex field, 2}
is equivalent to equation
\ShowEq{Cauchy Riemann equations, complex field, 3}
\fi
\ifx\texFuture\Defined
The G\^ateaux derivative of function of complex variable is
total differential and has form
\ShowEq{Gateaux derivative, complex field}
where $dx$, $dy\in R$.
Therefore, a symbolic equation
\ShowEq{Cauchy Riemann equations, Gateaux derivative, complex field}
does not express relation between the G\^ateaux derivative
with the Cauchy\Hyph Riemann equations.
\fi
\fi

\ePrints{Calculus.Paper}
\ifx\Semafor\ValueOn
\Section{Quaternion Algebra}
\else
\section{Quaternion Algebra}
\label{section: Quaternion Algebra}
\fi

\ePrints{Calculus.Paper}
\ifx\Semafor\ValueOff
In this paper I explore the set of quaternion algebras
defined in \citeBib{Izrail M. Gelfand: Quaternion Groups}. 

\begin{definition}
Let $F$ be field.
Extension field $F(i,j,k)$ is called
\AddIndex{the quaternion algebra
\symb{E(F,a,b)}1{quaternion algebra over the field}
over the field $F$}{quaternion algebra over the field}\footnote{I
follow definition from \citeBib{Izrail M. Gelfand: Quaternion Groups}.}
if multiplication in algebra $E$ is defined according to rule
\ShowEq{product in E(F,a,b), table}
where $a$, $b\in F$, $ab\ne 0$.
\qed
\end{definition}

Elements of the algebra $E(F,a,b)$ have form
\[
x=x^{\gi 0}+x^{\giA}i+x^{\gi 2}j+x^{\gi 3}k
\]
where $x^{\gi i}\in F$, $\gi i=\gi 0$, $\giA$, $\gi 2$, $\gi 3$.
Quaternion
\[
\overline x=x^{\gi 0}-x^{\giA}i-x^{\gi 2}j-x^{\gi 3}k
\]
is called conjugate to the quaternion $x$.
We define
\AddIndex{the norm of the quaternion}{norm of quaternion}
$x$ using equation
\ShowEq{norm of quaternion E(F,a,b)}
From equation \EqRef{norm of quaternion E(F,a,b)}, it follows that
$E(F,a,b)$ is algebra with division only when $a<0$, $b<0$.
In this case we can renorm basis such that $a=-1$, $b=-1$.

We use symbol
\ShowEq{quaternion division algebra over the field}
to denote the quaternion division algebra
$E(F,-1,-1)$
over the field $F$.
\symb{H}0{quaternion algebra over real field}
We will use notation $\ShowSymbol{quaternion algebra over real field}=E(R,-1,-1)$.
\def\EF{E(F)}
\else
\def\EF{H}
\fi
Multiplication in quaternion algebra $\EF$ is defined according to rule
\begin{equation}
\begin{array}{c|ccc}
&i&j&k\\
\hline
i&-1&k&-j\\
j&-k&-1&i\\
k&j&-i&-1\\
\end{array}
\EqLabel{product of quaternions}
\end{equation}
In algebra $\EF$, the norm of the quaternion has form
\begin{equation}
\EqLabel{norm of quaternion}
|x|^2=x\overline x=(x^{\gi 0})^2+(x^{\giA})^2+(x^{\gi 2})^2+(x^{\gi 3})^2
\end{equation}
\ePrints{Calculus.Paper}
\ifx\Semafor\ValueOff
In this case inverse element has form
\begin{equation}
\EqLabel{inverce quaternion}
x^{-1}=|x|^{-2}\overline x
\end{equation}

The inner automorphism of quaternion algebra $H$\footnote{See
\citeBib{Hamilton papers 3}, p. 643.}
\ShowEq{Quaternion Rotation}
describes the rotation of the vector with coordinates $x$, $y$, $z$.
The norm of quaternion $q$ is irrelevant, although usually we assume $|q|=1$.
If $q$ is written as sum of scalar and vector
\ShowEq{Quaternion Rotation, 1}
then \EqRef{Quaternion Rotation} is a rotation
of the vector $(x,y,z)$ about the vector $(a,b,c)$ through an angle $2\alpha$.
\fi


==> Complex.Number.Eq.tex <==
%auto-ignore

\DefEq
{
\begin{equation}
\EqLabel{norm of quaternion E(F,a,b)}
|x|^2=x\overline x=(x^{\gi 0})^2-a(x^{\giA})^2-b(x^{\gi 2})^2+ab(x^{\gi 3})^2
\end{equation}
}
{norm of quaternion E(F,a,b)}

\DefEq
{
\symb{E(F)}1{quaternion division algebra over the field}
}
{quaternion division algebra over the field}

\DefEq
{
\begin{equation}
\EqLabel{structural constants of quaternion, complex field}
\begin{array}{r@{}rr@{}r}
C_{23\cdot}{}_{\gi{00}}^{\gi 0}=&1&C_{23\cdot}{}_{\gi{01}}^{\giA}=&1
\\
C_{23\cdot}{}_{\gi{10}}^{\giA}=&1&C_{23\cdot}{}_{\gi{11}}^{\gi 0}=&-1
\end{array}
\end{equation}
}
{structural constants of quaternion, complex field}

\DefEquation
{
\begin{array}{rr}
e_{C\cdot\gi 0}=1&e_{C\cdot\giA}=i
\end{array}
}
{basis of complex field}

\DefEquation
{
e_{C\cdot\giA}^2=-e_{C\cdot\gi 0}
}
{product of complex field}


\DefEquation
{
\begin{array}{r@{}rr@{}r}
C_{C\cdot}^{}{}_{\gi{00}}^{\gi 0}=&1&C_{C\cdot}^{}{}_{\gi{01}}^{\giA}=&1
\\
\VirtVar
C_{C\cdot}^{}{}_{\gi{10}}^{\giA}=&1&C_{C\cdot}^{}{}_{\gi{11}}^{\gi 0}=&-1
\end{array}
}
{structural constants of complex field}

\DefEq
{
\begin{equation}
\EqLabel{complex field over real field, 0, 0}
f_{\gi 0}^{\gi 0}=f^{\gi{kr}}C_{C\cdot}^{}{}_{\gi{k0}}^{\gi p}
C_{C\cdot}^{}{}_{\gi{pr}}^{\gi 0}
=f^{\gi{0r}}C_{C\cdot}^{}{}_{\gi{00}}^{\gi 0}C_{C\cdot}^{}{}_{\gi{0r}}^{\gi 0}
+f^{\gi{1r}}C_{C\cdot}^{}{}_{\gi{10}}^{\giA}C_{C\cdot}^{}{}_{\gi{1r}}^{\gi 0}
=f^{\gi{00}}-f^{\gi{11}}
\end{equation}
\begin{equation}
\EqLabel{complex field over real field, 1, 0}
f_{\gi 0}^{\giA}=f^{\gi{kr}}C_{C\cdot}^{}{}_{\gi{k0}}^{\gi p}
C_{C\cdot}^{}{}_{\gi{pr}}^{\giA}
=f^{\gi{0r}}C_{C\cdot}^{}{}_{\gi{00}}^{\gi 0}C_{C\cdot}^{}{}_{\gi{0r}}^{\giA}
+f^{\gi{1r}}C_{C\cdot}^{}{}_{\gi{10}}^{\giA}C_{C\cdot}^{}{}_{\gi{1r}}^{\giA}
=f^{\gi{01}}+f^{\gi{10}}
\end{equation}
\begin{equation}
\EqLabel{complex field over real field, 1, 1}
f_{\giA}^{\gi 0}=f^{\gi{kr}}C_{C\cdot}^{}{}_{\gi{k1}}^{\gi p}
C_{C\cdot}^{}{}_{\gi{pr}}^{\gi 0}
=f^{\gi{0r}}C_{C\cdot}^{}{}_{\gi{01}}^{\giA}C_{C\cdot}^{}{}_{\gi{1r}}^{\gi 0}
+f^{\gi{1r}}C_{C\cdot}^{}{}_{\gi{11}}^{\gi 0}C_{C\cdot}^{}{}_{\gi{0r}}^{\gi 0}
=-f^{\gi{01}}-f^{\gi{10}}
\end{equation}
\begin{equation}
\EqLabel{complex field over real field, 0, 1}
f_{\giA}^{\giA}=f^{\gi{kr}}C_{C\cdot}^{}{}_{\gi{k1}}^{\gi p}
C_{C\cdot}^{}{}_{\gi{pr}}^{\giA}
=f^{\gi{0r}}C_{C\cdot}^{}{}_{\gi{01}}^{\giA}C_{C\cdot}^{}{}_{\gi{1r}}^{\giA}
+f^{\gi{1r}}C_{C\cdot}^{}{}_{\gi{11}}^{\gi 0}C_{C\cdot}^{}{}_{\gi{0r}}^{\giA}
=f^{\gi{00}}-f^{\gi{11}}
\end{equation}
}
{complex field over real field}

\DefEq
{
\begin{equation}
\EqLabel{Cauchy Riemann equations, complex field, 1}
\begin{array}{r@{}r}
\displaystyle\frac{\partial y^{\giA}}{\partial x^{\gi 0}}=
&\displaystyle-\frac{\partial y^{\gi 0}}{\partial x^{\giA}}
\\
\VirtFrac
\displaystyle\frac{\partial y^{\gi 0}}{\partial x^{\gi 0}}=
&\displaystyle\frac{\partial y^{\giA}}{\partial x^{\giA}}
\end{array}
\end{equation}
}
{Cauchy Riemann equations, complex field, 1}

\DefEq
{
\begin{pmatrix}
\displaystyle\frac{\partial y^{\gi 0}}{\partial x^{\gi 0}}
&
\displaystyle\frac{\partial y^{\gi 0}}{\partial x^{\giA}} 
\\
\VirtFrac
\displaystyle\frac{\partial y^{\giA}}{\partial x^{\gi 0}}
&
\displaystyle\frac{\partial y^{\giA}}{\partial x^{\giA}}
\end{pmatrix}
}
{Jacobian of map, complex variable}

\DefEq
{
\[
\ShowEq{Jacobian of map, complex variable}
\]
}
{Jacobian of map of complex variable}

\DefEq
{
\begin{equation}
\EqLabel{Cauchy Riemann equations, complex field, 2}
\frac{\partial y}{\partial x^{\gi 0}}
+i\frac{\partial y}{\partial x^{\giA}}
=0
\end{equation}
}
{Cauchy Riemann equations, complex field, 2}

\DefEq
{
\[
\frac{\partial y^{\gi 0}}{\partial x^{\gi 0}}
+i\frac{\partial y^{\giA}}{\partial x^{\gi 0}}
+i\frac{\partial y^{\gi 0}}{\partial x^{\giA}}
-\frac{\partial y^{\giA}}{\partial x^{\giA}}
=0
\]
}
{Cauchy Riemann equations, complex field, 2, 1}

\DefEq
{
\begin{equation}
\EqLabel{Cauchy Riemann equations, complex field, 3}
\begin{pmatrix}
1&i
\end{pmatrix}
\ShowEq{Jacobian of map, complex variable}
\begin{pmatrix}
1\\i
\end{pmatrix}
=0
\end{equation}
}
{Cauchy Riemann equations, complex field, 3}

\DefEq
{
\begin{equation}
\EqLabel{Gateaux derivative, complex field}
\partial(f(x+yi))(dx,dy)=
\begin{pmatrix}
1&i
\end{pmatrix}
\ShowEq{Jacobian of map, complex variable}
\begin{pmatrix}
dx\\dy
\end{pmatrix}
\end{equation}
}
{Gateaux derivative, complex field}

\DefEq
{
\begin{equation}
\EqLabel{Cauchy Riemann equations, Gateaux derivative, complex field}
\partial(f(x+yi))(1,i)=0
\end{equation}
}
{Cauchy Riemann equations, Gateaux derivative, complex field}

\DefEq
{
\begin{equation}
\begin{array}{c|ccc}
&i&j&k\\
\hline
i&a&k&aj\\
j&-k&b&-bi\\
k&-aj&bi&-ab\\
\end{array}
\EqLabel{product in E(F,a,b), table}
\end{equation}
}
{product in E(F,a,b), table}

\DefEq
{
\frac{\partial f}{\partial x^{\gi 0}}
+i\frac{\partial f}{\partial x^{\giA}}
+j\frac{\partial f}{\partial x^{\gi 2}}
+k\frac{\partial f}{\partial x^{\gi 3}}
}
{Regular quaternion function}

\DefEq
{
\begin{pmatrix}
\displaystyle\frac{\partial f^{\gi 0}}{\partial x^{\gi 0}}
&\displaystyle\frac{\partial f^{\gi 0}}{\partial x^{\giA}}
&\displaystyle\frac{\partial f^{\gi 0}}{\partial x^{\gi 2}}
&\displaystyle\frac{\partial f^{\gi 0}}{\partial x^{\gi 3}}
\\
\displaystyle\VirtFrac\frac{\partial f^{\giA}}{\partial x^{\gi 0}}
&\displaystyle\frac{\partial f^{\giA}}{\partial x^{\giA}}
&\displaystyle\frac{\partial f^{\giA}}{\partial x^{\gi 2}}
&\displaystyle\frac{\partial f^{\giA}}{\partial x^{\gi 3}}
\\
\displaystyle\VirtFrac\frac{\partial f^{\gi 2}}{\partial x^{\gi 0}}
&\displaystyle\frac{\partial f^{\gi 2}}{\partial x^{\giA}}
&\displaystyle\frac{\partial f^{\gi 2}}{\partial x^{\gi 2}}
&\displaystyle\frac{\partial f^{\gi 2}}{\partial x^{\gi 3}}
\\
\displaystyle\VirtFrac\frac{\partial f^{\gi 3}}{\partial x^{\gi 0}}
&\displaystyle\frac{\partial f^{\gi 3}}{\partial x^{\giA}}
&\displaystyle\frac{\partial f^{\gi 3}}{\partial x^{\gi 2}}
&\displaystyle\frac{\partial f^{\gi 3}}{\partial x^{\gi 3}}
\end{pmatrix}
}
{Jacobian of quaternion function}

\DefEq
{
\begin{equation}%
\begin{matrix}
p\rightarrow qpq^{-1}
\\
\VirtVar
q(ix+jy+kz)q^{-1}=ix'+jy'+kz'
\end{matrix}
\EqLabel{Quaternion Rotation}%
\end{equation}%
}%
{Quaternion Rotation}%

\DefEq
{
\[
q=\cos\alpha+(ia+jb+kc)\sin\alpha\ \ \ a^2+b^2+c^2=1
\]
}
{Quaternion Rotation, 1}

\DefEq
{
\begin{align*}
(a,b)&=-\frac 12(ab+aibi+ajbj+akbk)
\\
&=-\frac 12((a^{\gi 0}+a^{\giA}i+a^{\gi 2}j+a^{\gi 3}k)
(b^{\gi 0}+b^{\giA}i+b^{\gi 2}j+b^{\gi 3}k)
\\
&+(-a^{\giA}+a^{\gi 0}i+a^{\gi 3}j-a^{\gi 2}k)
(-b^{\giA}+b^{\gi 0}i+b^{\gi 3}j-b^{\gi 2}k)
\\
&+(-a^{\gi 2}-a^{\gi 3}i+a^{\gi 0}j+a^{\giA}k)
(-b^{\gi 2}-b^{\gi 3}i+b^{\gi 0}j+b^{\giA}k)
\\
&+(-a^{\gi 3}+a^{\gi 2}i-a^{\giA}j+a^{\gi 0}k)
(-b^{\gi 3}+b^{\gi 2}i-b^{\giA}j+b^{\gi 0}k)
\\
&=a^{\gi 0}b^{\gi 0}-a^{\giA}b^{\giA}-a^{\gi 2}b^{\gi 2}-a^{\gi 3}b^{\gi 3}
+(a^{\gi 0}b^{\giA}+a^{\giA}b^{\gi 0}+a^{\gi 2}b^{\gi 3}-a^{\gi 3}b^{\gi 2})i
\\
&+(a^{\gi 0}b^{\gi 2}+a^{\gi 2}b^{\gi 0}+a^{\gi 3}b^{\giA}-a^{\giA}b^{\gi 3})j
+(a^{\gi 0}b^{\gi 3}+a^{\gi 3}b^{\gi 0}+a^{\giA}b^{\gi 2}-a^{\gi 2}b^{\giA})k
\end{align*}
}
{scalar product, quaternion algebra, old}



==> Complex.Number.Russian.tex <==
%auto-ignore

\input{\FilePrefix Complex.Number.Eq}

\ePrints{Calculus.Paper}
\ifx\Semafor\ValueOn
\Section{Линейная функция комплексного поля}
\else
\section{Линейная функция комплексного поля}
\fi
\label{section: Linear Function of Complex Field}

\begin{theorem}[Уравнения Коши\Hyph Римана]
\label{theorem: complex field over real field}
Рассмотрим поле комплексных чисел $C$ как двумерную алгебру над полем действительных чисел.
Положим
\ShowEq{basis of complex field}
базис алгебры $C$.
\ePrints{Calculus.Paper}
\ifx\Semafor\ValueOff
Тогда в этом базисе произведение имеет вид
\ShowEq{product of complex field}
и структурные константы имеют вид
\ShowEq{structural constants of complex field}
\fi%Calculus.Paper
Матрица линейной функции
\[
y^{\gi i}=x^{\gi j}f_{\gi j}^{\gi i}
\]
поля комплексных чисел над полем действительных чисел
удовлетворяет соотношению
\begin{align}
\EqLabel{complex field over real field, 0}
f_{\gi 0}^{\gi 0}&=f_{\giA}^{\giA}
\\
\EqLabel{complex field over real field, 1}
f_{\gi 0}^{\giA}&=-f_{\giA}^{\gi 0}
\end{align}
\end{theorem}
\begin{proof}
\ePrints{Calculus.Paper}
\ifx\Semafor\ValueOff
Равенства
\EqRef{product of complex field} и
\EqRef{structural constants of complex field}
следуют из равенства $i^2=-1$.
Пользуясь равенством
\xEqRef{0812.4763}{linear map over field, division ring, relation}
получаем соотношения
\ShowEq{complex field over real field}
Из равенств
\EqRef{complex field over real field, 0, 0} и
\EqRef{complex field over real field, 0, 1}
следует \EqRef{complex field over real field, 0}.
Из равенств
\EqRef{complex field over real field, 1, 0} и
\EqRef{complex field over real field, 1, 1}
следует \EqRef{complex field over real field, 1}.
\else%Calculus.Paper
Смотри доказательство теоремы
\xRef{8433-5163}{theorem: complex field over real field}.
\fi%Calculus.Paper
\end{proof}

\ePrints{0701.238,1003.1544,8433-5163}
\ifx\Semafor\ValueOff
\begin{theorem}[Уравнения Коши\Hyph Римана]
Если матрица
\ShowEq{Jacobian of map of complex variable}
является матрицей Якоби функции комплексного переменного
\[
x=x^{\gi 0}+x^{\giA}i\rightarrow y=y^{\gi 0}(x^{\gi 0},x^{\giA})+y^{\giA}(x^{\gi 0},x^{\giA})i
\]
над полем действительных чисел,
то
\ShowEq{Cauchy Riemann equations, complex field, 1}
\end{theorem}
\begin{proof}
Следствие теоремы
\ref{theorem: complex field over real field}.
\end{proof}

\begin{theorem}
Производная функции комплексного переменного удовлетворяет равенству
\ShowEq{Cauchy Riemann equations, complex field, 2}
\end{theorem}
\begin{proof}
Равенство
\ShowEq{Cauchy Riemann equations, complex field, 2, 1}
следует из равенств
\EqRef{Cauchy Riemann equations, complex field, 1}.
\end{proof}

\ePrints{Calculus.Paper}
\ifx\Semafor\ValueOff
Равенство \EqRef{Cauchy Riemann equations, complex field, 2}
эквивалентно равенству
\ShowEq{Cauchy Riemann equations, complex field, 3}
\fi
\ifx\texFuture\Defined
Производная Гато функции комплексного переменного является
полным дифференциалом и имеет вид
\ShowEq{Gateaux derivative, complex field}
где $dx$, $dy\in R$.
Поэтому символическое уравнение
\ShowEq{Cauchy Riemann equations, Gateaux derivative, complex field}
не выражает связь производной Гато с уравнения Коши\Hyph Римана.
\fi
\fi

\ePrints{Calculus.Paper}
\ifx\Semafor\ValueOn
\Section{Алгебра кватернионов}
\else
\section{Алгебра кватернионов}
\label{section: Quaternion Algebra}
\fi

\ePrints{Calculus.Paper}
\ifx\Semafor\ValueOff
В этой статье я рассматриваю множество кватернионных алгебр,
определённых в \citeBib{Izrail M. Gelfand: Quaternion Groups}.

\begin{definition}
Пусть $F$ - поле.
Расширение $F(i,j,k)$ поля $F$ называется
\AddIndex{алгеброй
\symb{E(F,a,b)}1{quaternion algebra over the field}
кватернионов над полем $F$}{quaternion algebra over the field}\footnote{Я
буду следовать определению из \citeBib{Izrail M. Gelfand: Quaternion Groups}.},
если произведение в алгебре $E$ определено согласно правилам
\ShowEq{product in E(F,a,b), table}
где $a$, $b\in F$, $ab\ne 0$.
\qed
\end{definition}

Элементы алгебры $E(F,a,b)$ имеют вид
\[
x=x^{\gi 0}+x^{\giA}i+x^{\gi 2}j+x^{\gi 3}k
\]
где $x^{\gi i}\in F$, $\gi i=\gi 0$, $\giA$, $\gi 2$, $\gi 3$.
Кватернион
\[
\overline x=x^{\gi 0}-x^{\giA}i-x^{\gi 2}j-x^{\gi 3}k
\]
называется сопряжённым кватерниону $x$.
Мы определим
\AddIndex{норму кватерниона}{norm of quaternion}
$x$ равенством
\ShowEq{norm of quaternion E(F,a,b)}
Из равенства \EqRef{norm of quaternion E(F,a,b)} следует, что
$E(F,a,b)$ является алгеброй с делением только когда $a<0$, $b<0$.
Тогда мы можем пронормировать базис так, что $a=-1$, $b=-1$.

Мы будем обозначать символом
\ShowEq{quaternion division algebra over the field}
алгебру $E(F,-1,-1)$
кватернионов с делением над полем $F$.
\symb{H}0{quaternion algebra over real field}
Мы будем полагать $\ShowSymbol{quaternion algebra over real field}=E(R,-1,-1)$.
\def\EF{E(F)}
\else
\def\EF{H}
\fi
Произведение в алгебре кватернионов $\EF$ определено согласно правилам
\begin{equation}
\begin{array}{c|ccc}
&i&j&k\\
\hline
i&-1&k&-j\\
j&-k&-1&i\\
k&j&-i&-1\\
\end{array}
\EqLabel{product of quaternions}
\end{equation}
В алгебре $\EF$ норма кватерниона имеет вид
\begin{equation}
\EqLabel{norm of quaternion}
|x|^2=x\overline x=(x^{\gi 0})^2+(x^{\giA})^2+(x^{\gi 2})^2+(x^{\gi 3})^2
\end{equation}
\ePrints{Calculus.Paper}
\ifx\Semafor\ValueOff
При этом обратный элемент имеет вид
\begin{equation}
\EqLabel{inverce quaternion}
x^{-1}=|x|^{-2}\overline x
\end{equation}

Внутренний автоморфизм алгебры кватернионов $H$\footnote{См.
\citeBib{Hamilton papers 3}, с. 643.}
\ShowEq{Quaternion Rotation}
описывает вращение вектора с координатами $x$, $y$, $z$.
Если $q$ записан в виде суммы скаляра и вектора
\ShowEq{Quaternion Rotation, 1}
то \EqRef{Quaternion Rotation} описывает вращение
вектора $(x,y,z)$ вокруг вектора $(a,b,c)$ на угол $2\alpha$.
\fi


==> Convention.English.tex <==
%auto-ignore
\input{\FilePrefix Convention.Eq}

\section{Conventions}

\ePrints{0812.4763,0906.0135,0908.3307,0909.0855,0912.3315,1003.1544}
\Items{1006.2597}
\ifx\Semafor\ValueOn
\begin{convention}
Function and map are synonyms. However according to
tradition, correspondence between either rings or vector
spaces is called map and a map of
either real field or quaternion algebra is called function.
\qed
\end{convention}
\fi

\ePrints{0701.238,0812.4763,0908.3307,0912.4061,1001.4852}
\Items{1003.1544,4776-3181}
\ifx\Semafor\ValueOn
\begin{convention}
In any expression where we use index I assume
that this index may have internal structure.
For instance, considering the algebra $A$ we enumerate coordinates of
$a\in A$ relative to basis $\Basis e$ by an index $i$.
This means that $a$ is a vector. However, if $a$
is matrix, then we need two indexes, one enumerates
rows, another enumerates columns. In the case, when index has
structure, we begin the index from symbol $\cdot$ in
the corresponding position. 
For instance, if I consider the matrix $a^i_j$ as an element of a vector
space, then I can write the element of matrix as $a^{\cdot}{}^i_j$.
\qed
\end{convention}
\fi

\ePrints{0701.238,0812.4763,0908.3307,0912.4061,1006.2597,1011.3102}
\Items{Calculus.Paper,1211.6965,GJSFRF.Basis}
\ifx\Semafor\ValueOn
\begin{convention}
I assume sum over index $s$ in expression like
\ShowEq{Sum over repeated index}
\qed
\end{convention}
\fi

\ePrints{0701.238,0812.4763,0906.0135,0908.3307,0909.0855}
\ifx\Semafor\ValueOn
\begin{convention}
We can consider division ring $D$ as $D$\Hyph vector space
of dimension $1$. According to this statement, we can explore not only
homomorphisms of division ring $D_1$ into division ring $D_2$,
but also linear maps of division rings.
\qed
\end{convention}
\fi

\ePrints{0912.4061}
\ifx\Semafor\ValueOn
\begin{convention}
For given field $F$, unless otherwise stated,
we consider finite dimensional $F$\Hyph algebra.
%without zero divisors.
\qed
\end{convention}
\fi

\ePrints{0701.238,0812.4763,0906.0135,0908.3307,4776-3181}
\ifx\Semafor\ValueOn
\begin{convention}
In spite of noncommutativity of product a lot of statements
remain to be true if we substitute, for instance, right representation by
left representation or right vector space by left
vector space.
To keep this symmetry in statements of theorems
I use symmetric notation.
For instance, I consider \Ds vector space
and \sD vector space.
We can read notation \Ds vector space
as either D\Hyph star\Hyph vector space or
left vector space.
We can read notation \Ds linear dependent vectors
as either D\Hyph star\Hyph linear dependent vectors or
vectors that are linearly dependent from left.
\qed
\end{convention}
\fi

\ePrints{0701.238,0812.4763,0906.0135,0908.3307,0909.0855,0912.4061}
\Items{1001.4852,1003.1544,1006.2597,1104.5197,1105.4307,1107.1139}
\Items{1202.6021,MQuater,1211.6965,CACAA.07.195,GJSFRF.Basis,MPoly}
\ifx\Semafor\ValueOn
\begin{convention}
\label{convention: we use separate color for index of element}
Let $A$ be free algebra
with finite or countable basis.
Considering expansion of element of algebra $A$ relative basis $\Basis e$
we use the same root letter to denote this element and its coordinates.
In expression $a^2$, it is not clear whether this is component
of expansion of element
$a$ relative basis, or this is operation $a^2=aa$.
To make text clearer we use separate color for index of element
of algebra. For instance,
\ShowEq{Expansion relative basis in algebra}
\qed
\end{convention}
\fi

\ePrints{0701.238,0812.4763,GJSFRF.Basis}
\ifx\Semafor\ValueOn
\begin{convention}
%\label{convention: }
It is very difficult to draw the line between the module and the algebra.
Especially since sometimes in the process of constructing, we must first
prove that the set $A$ is a module,
and then we prove that this set is an algebra.
Therefore, to write the element of the module,
we will also use the convention
\ref{convention: we use separate color for index of element}.
\qed
\end{convention}
\fi

\ePrints{MPoly}
\ifx\Semafor\ValueOn
\begin{convention}
Element of
\ePrints{MPoly}
\ifx\Semafor\ValueOn
$D$\Hyph algebra
\else
$\Omega$\Hyph group
\fi
$A$ is called
\AddIndex{$A$\Hyph number}{A number}.
For instance, complex number is also called
$C$\Hyph number, and quaternion is called $H$\Hyph number.
\qed
\end{convention}
\fi

\ePrints{0701.238,0812.4763}
\ifx\Semafor\ValueOn
\begin{convention}
The identification of the vector and matrix of its coordinates
can lead to ambiguity in the equation
\ShowEq{Identification can lead to ambiguity, 1}
where $\Basis e$ is a basis of vector space.
Therefore, we write the equation
\EqRef{Identification can lead to ambiguity, 1}
in the following form
\ShowEq{Identification can lead to ambiguity, 2}
in order to see where we wrote vector.
\qed
\end{convention}
\fi

\ePrints{0701.238,0812.4763,0906.0135,0908.3307,0909.0855,0912.4061}
\Items{1001.4852,1003.1544,1006.2597,1104.5197,1105.4307,1107.1139}
\Items{1202.6021,MQuater,CACAA.07.195}
\ifx\Semafor\ValueOn
\begin{convention}
If free finite dimensional algebra has unit, then we identify
the vector of basis $\Vector e_{\gi 0}$ with unit of algebra.
\qed
\end{convention}
\fi

\ePrints{1104.5197,1105.4307}
\ifx\Semafor\ValueOn
\begin{convention}
Although the algebra is a free module over some
ring, we do not use the vector notation
to write elements of algebra. In the case when I consider the
matrix of coordinates of element of algebra, I will use vector
notation to write corresponding element.
In order to avoid ambiguity when I use conjugation,
I denote $a^*$ element conjugated to element $a$.
\qed
\end{convention}
\fi

\ePrints{0906.0135,0912.3315,8443-0072,1111.6035,1102.5168}
\ifx\Semafor\ValueOn
\begin{convention}
In \citeBib{Cohn: Universal Algebra},
an arbitrary operation of algebra is denoted by letter $\omega$,
and $\Omega$ is the set of operations of some universal algebra.
Correspondingly, the universal algebra with the set of operations
$\Omega$ is denoted as $\Omega$\Hyph algebra.
Similar notations we see in
\citeBib{Burris Sankappanavar} with small difference
that an operation in the algebra is denoted by letter $f$
and $\mathcal F$ is the set of operations.
I preferred first case of notations because in this case it is
easier to see where I use operation.
\qed
\end{convention}
\fi

\ePrints{0906.0135,0912.3315,8443-0072}
\ifx\Semafor\ValueOn
\begin{convention}
Since the number of universal algebras
in the tower of representations is varying,
then we use vector notation for a tower of
representations. We denote the set
$(A_1,...,A_n)$ of $\Omega_i$\Hyph algebras $A_i$, $i=1$, ..., $n$
as $\Vector A$. We denote the set of representations
$(f_{1,2},...,f_{n-1,n})$ of these algebras as $\Vector f$.
Since different algebras have different type, we also
talk about the set of $\Vector{\Omega}$\Hyph algebras.
\ePrints{8443-0072}
\ifx\Semafor\ValueOn
We
\else
In relation to the set $\Vector A$,
we also use matrix notations 
that we discussed
in section \xRef{0701.238}{section: Concept of Generalized Index}.
For instance, we
\fi
use the symbol $\Vector A_{[1]}$ to denote the
set of $\Vector{\Omega}$\Hyph algebras $(A_2,...,A_n)$.
In the corresponding notation $(\VX A,\Vector f)$ of tower
of representation, we assume that $\Vector f=(f_{2,3},...,f_{n-1,n})$.
\qed
\end{convention}

\begin{convention}
Since we use vector notation for elements of the
tower of representations, we need convention about notation of operation.
We assume that we get result of operation componentwise. For instance,
\ShowEq{vector notation in tower of representations}
\qed
\end{convention}
\fi

\ePrints{8443-0072,1111.6035,0906.0135,NewAffine,1102.5168,MOmega}
\ifx\Semafor\ValueOn
\begin{convention}
Let $A$ be $\Omega_1$\Hyph algebra.
Let $B$ be $\Omega_2$\Hyph algebra.
Notation
\ShowEq{A->*B}
means that there is representation of $\Omega_1$\Hyph algebra $A$
in $\Omega_2$\Hyph algebra $B$.
\qed
\end{convention}
\fi

\ePrints{0702.561,0707.2246,0803.2620}
\ifx\Semafor\ValueOn
\begin{convention}
I use arrow $\xymatrix{\arp[r]&}$ to represent
projection of bundle on diagram.
I use arrow $\xymatrix{\ars[r]&}$ to represent
section of bundle on diagram.
\qed
\end{convention}
\fi

\ePrints{0912.3315}
\ifx\Semafor\ValueOn
\begin{remark}
I believe that diagrams of maps are an important tool.
However, sometimes I want
to see the diagram as three dimensional figure
and I expect that this would increase its expressive
power. Who knows what surprises the future holds.
In 1992, at a conference in Kazan, I have described to my colleagues
what advantages the computer preparation of papers has.
8 years later I learned from the letter from Kazan that now we can
prepare paper using LaTeX.
\qed
\end{remark}
\fi

\ePrints{1001.4852,1003.1544,1006.2597,1011.3102}
\Items{Calculus.Paper}
\ifx\Semafor\ValueOn
\begin{convention}
If, in a certain expression, we use several operations
which include the operation $\circ$, then
it is assumed that the operation $\circ$ is executed first.
Below is an example of equivalent expressions.
\ShowEq{list circ expressions}
\qed
\end{convention}
\fi

%\ePrints{0906.0135,NewAffine}
%\ifx\Semafor\ValueOn
%\item
%Let $\VX X$ be the basis of the tower of representations $(\Vector A,\Vector f)$.
%A $\Omega_n$\Hyph word
%$w_n(\Vector f,\VX X,x_n)$ is called coordinates $x_n\in A_n$
%relative to basis $\VX X$.
%\fi

\ePrints{1107.1139}
\ifx\Semafor\ValueOn
\begin{convention}
For given $D$\Hyph algebra $A$
we define left shift
\ShowEq{left shift, D algebra}
by the equation
\ShowEq{left shift 1, D algebra}
and right shift
\ShowEq{right shift, D algebra}
by the equation
\ShowEq{right shift 1, D algebra}
\qed
\end{convention}
\fi

\ifx\PrintPaper\undefined
Without a doubt, the reader may have questions,
comments, objections. I will appreciate any response.
\fi



==> Convention.Eq.tex <==
%auto-ignore

\DefEq
{
\[
\Vector r(\Vector a)=(r_1(a_1),...,r_n(a_n))
\]
}
{vector notation in tower of representations}

\DefEq
{
\[
\xymatrix
{
A\ar[r]|{*}&B
}
\]
}
{A->*B}

\DefEq
{
\[
\begin{array}{r@{\ }lr@{\ }l}
f\circ xy&\equiv f(x)y
&
f\circ(xy)&\equiv f(xy)
\\
f\circ x+y&\equiv f(x)+y
&
f\circ (x+y)&\equiv f(x+y)
\end{array}
\]
}
{list circ expressions}

\DefEq
{
\[
a\pC s0xa\pC s1
\]
}
{Sum over repeated index}

\DefEq
{
\[
a=a^{\gi i}e_{\gi i}
\]
}
{Expansion relative basis in algebra}

\DefEquation
{
a=a\CRstar e
}
{Identification can lead to ambiguity, 1}

\DefEq
{
\[\Vector a=a\CRstar e\]
}
{Identification can lead to ambiguity, 2}

\DefEq
{
\symb{a\circ}1{left shift, D algebra}
}
{left shift, D algebra}

\DefEq
{
\symb{a\star}1{right shift, D algebra}
}
{right shift, D algebra}

\DefEq
{
\[
\ShowSymbol{left shift, D algebra}x=ax
\]
}
{left shift 1, D algebra}

\DefEq
{
\[
\ShowSymbol{right shift, D algebra}x=xa
\]
}
{right shift 1, D algebra}


==> Convention.Russian.tex <==
%auto-ignore
\input{\FilePrefix Convention.Eq}

\section{Соглашения}

\ePrints{0812.4763,0906.0135,0908.3307,0909.0855,0912.3315,1003.1544}
\Items{1006.2597}
\ifx\Semafor\ValueOn
\begin{convention}
Функция и отображение - синонимы. Однако существует
традиция соответствие между кольцами или векторными
пространствами называть отображением, а отображение
поля действительных чисел или алгебры кватернионов называть функцией.
Я тоже следую этой традиции,
хотя встречается текст, в котором неясно, какому термину надо
отдать предпочтение.
\qed
\end{convention}
\fi

\ePrints{0701.238,0812.4763,0908.3307,0912.4061,1001.4852}
\Items{1003.1544,4776-3181}
\ifx\Semafor\ValueOn
\begin{convention}
В любом выражении, где появляется индекс, я предполагаю,
что этот индекс может иметь внутреннюю структуру.
Например, при рассмотрении алгебры $A$ координаты $a\in A$
относительно базиса $\Basis e$ пронумерованы индексом $i$.
Это означает, что $a$ является вектором. Однако, если $a$
является матрицей, нам необходимо два индекса, один нумерует
строки, другой - столбцы. В том случае, когда мы уточняем структуру
индекса, мы будем начинать индекс с символа $\cdot$ в соответствующей
позиции.
Например, если я рассматриваю матрицу $a^i_j$ как элемент векторного
пространства, то я могу записать элемент матрицы в виде $a^{\cdot}{}^i_j$.
\qed
\end{convention}
\fi

\ePrints{0701.238,0812.4763,0908.3307,0912.4061,1006.2597,1011.3102}
\Items{Calculus.Paper,1211.6965,GJSFRF.Basis}
\ifx\Semafor\ValueOn
\begin{convention}
В выражении вида
\ShowEq{Sum over repeated index}
предполагается сумма по индексу $s$.
\qed
\end{convention}
\fi

\ePrints{0701.238,0812.4763,0906.0135,0908.3307,0909.0855}
\ifx\Semafor\ValueOn
\begin{convention}
Тело $D$ можно рассматривать как $D$\Hyph векторное пространство
размерности $1$. Соответственно этому, мы можем изучать не только
гомоморфизм тела $D_1$ в тело $D_2$, но и линейное отображение тел.
\qed
\end{convention}
\fi

\ePrints{0912.4061}
\ifx\Semafor\ValueOn
\begin{convention}
Для данного поля $F$, если не оговорено противное,
мы будем рассматривать конечномерную $F$\Hyph алгебру.
%без делителей нуля.
\qed
\end{convention}
\fi

\ePrints{0701.238,0812.4763,0906.0135,0908.3307,4776-3181}
\ifx\Semafor\ValueOn
\begin{convention}
Несмотря на некоммутативность произведения многие утверждения
сохраняются, если заменить например правое представление на
левое представление или правое векторное пространство на левое
векторное пространство.
Чтобы сохранить эту симметрию в формулировках теорем
я пользуюсь симметричными обозначениями.
Например, я рассматриваю \Ds векторное пространство
и \sD векторное пространство.
Запись \Ds векторное пространство можно прочесть
как D\Hyph star\Hyph векторное пространство либо
как левое векторное пространство.
Запись \Ds линейно зависимые векторы можно прочесть
как D\Hyph star\Hyph линейно зависимые векторы либо
как векторы, линейно зависимые слева.
\qed
\end{convention}
\fi

\ePrints{0701.238,0812.4763,0906.0135,0908.3307,0909.0855,0912.4061}
\Items{1001.4852,1003.1544,1006.2597,1104.5197,1105.4307,1107.1139}
\Items{1202.6021,MQuater,1211.6965,CACAA.07.195,GJSFRF.Basis,MPoly}
\ifx\Semafor\ValueOn
\begin{convention}
\label{convention: we use separate color for index of element}
Пусть $A$ - свободная алгебра
с конечным или счётным базисом.
При разложении элемента алгебры $A$ относительно базиса $\Basis e$
мы пользуемся одной и той же корневой буквой для обозначения этого
элемента и его координат.
В выражении $a^2$ не ясно - это компонента разложения элемента
$a$ относительно базиса или это операция возведения в степень.
Для облегчения чтения текста мы будем индекс элемента алгебры выделять
цветом. Например,
\ShowEq{Expansion relative basis in algebra}
\qed
\end{convention}
\fi

\ePrints{0701.238,0812.4763,GJSFRF.Basis}
\ifx\Semafor\ValueOn
\begin{convention}
%\label{convention: }
Очень трудно провести границу между модулем и алгеброй.
Тем более, иногда в процессе построения мы должны сперва
доказать, что множество $A$ является модулем,
а потом мы доказываем, что это множество является алгеброй.
Поэтому для записи координат элемента модуля
мы также будем пользоваться соглашением
\ref{convention: we use separate color for index of element}.
\qed
\end{convention}
\fi

\ePrints{MPoly}
\ifx\Semafor\ValueOn
\begin{convention}
Элемент
\ePrints{MPoly}
\ifx\Semafor\ValueOn
$D$\Hyph алгебры
\else
$\Omega$\Hyph группы
\fi
$A$ называется
\AddIndex{$A$\Hyph числом}{A number}.
Например, комплексное число также называется
$C$\Hyph число, а кватернион называется $H$\Hyph число.
\qed
\end{convention}
\fi

\ePrints{0701.238,0812.4763}
\ifx\Semafor\ValueOn
\begin{convention}
Отождествление вектора и матрицы его координат
может привести к неоднозначности в равенстве
\ShowEq{Identification can lead to ambiguity, 1}
где $\Basis e$ - базис векторного пространства.
Поэтому мы будем записывать равенство
\EqRef{Identification can lead to ambiguity, 1}
в виде
\ShowEq{Identification can lead to ambiguity, 2}
чтобы видеть, где записан вектор.
\qed
\end{convention}
\fi

\ePrints{0701.238,0812.4763,0906.0135,0908.3307,0909.0855,0912.4061}
\Items{1001.4852,1003.1544,1006.2597,1104.5197,1105.4307,1107.1139}
\Items{1202.6021,MQuater,CACAA.07.195}
\ifx\Semafor\ValueOn
\begin{convention}
Если свободная конечномерная алгебра имеет единицу,
то мы будем отождествлять
вектор базиса $\Vector e_{\gi 0}$ с единицей алгебры.
\qed
\end{convention}
\fi

\ePrints{1104.5197,1105.4307}
\ifx\Semafor\ValueOn
\begin{convention}
Хотя алгебра является свободным модулем над некоторым
кольцом, мы не пользуемся векторными обозначениями
при записи элементов алгебры. В тех случаях, когда я рассматриваю
матрицу координат элемента алгебры, я буду пользоваться векторными
обозначениями для записи соответствующего элемента.
Чтобы не возникала неоднозначность при записи сопряжения,
я буду обозначать $a^*$ элемент, сопряжённый элементу $a$.
\qed
\end{convention}
\fi

\ePrints{0906.0135,0912.3315,8443-0072,1111.6035,1102.5168}
\ifx\Semafor\ValueOn
\begin{convention}
В \citeBib{Cohn: Universal Algebra}
произвольная операция алгебры обозначена буквой $\omega$,
и $\Omega$ - множество операций некоторой универсальной алгебры.
Соответственно, универсальная алгебра с множеством операций
$\Omega$ обозначается $\Omega$\Hyph алгебра.
Аналогичные обозначения мы видим в
\citeBib{Burris Sankappanavar} с той небольшой разницей,
что операция в алгебре обозначена буквой $f$
и $\mathcal F$ - множество операций.
Я выбрал первый вариант обозначений, так как в этом случае
легче видно, где я использую операцию.
\qed
\end{convention}
\fi

\ePrints{0906.0135,0912.3315,8443-0072}
\ifx\Semafor\ValueOn
\begin{convention}
Так как число универсальных алгебр в башне представлений переменно,
то мы будем пользоваться векторными обозначениями для башни
представлений. Множество
$(A_1,...,A_n)$ $\Omega_i$\Hyph алгебр $A_i$, $i=1$, ..., $n$
мы будем обозначать $\Vector A$. Множество представлений
$(f_{1,2},...,f_{n-1,n})$ этих алгебр мы будем обозначать $\Vector f$.
Так как разные алгебры имеют разный тип, мы также
будем говорить о множестве $\Vector{\Omega}$\Hyph алгебр.
\ePrints{8443-0072}
\ifx\Semafor\ValueOn
Символом
\else
По отношению к множеству $\Vector A$
мы также будем пользоваться матричными обозначениями, предложенными
в разделе \xRef{0701.238}{section: Concept of Generalized Index}.
Например, символом
\fi
$\Vector A_{[1]}$ мы будем обозначать
множество $\Vector{\Omega}$\Hyph алгебр $(A_2,...,A_n)$.
В соответствующем обозначении $(\VX A,\Vector f)$ башни
представлений подразумевается, что $\Vector f=(f_{2,3},...,f_{n-1,n})$.
\qed
\end{convention}

\begin{convention}
Так как мы пользуемся векторными обозначениями для элементов
башни представлений, необходимо соглашение о записи операций.
Предполагается, что операции выполняются покомпонентно. Например,
\ShowEq{vector notation in tower of representations}
\qed
\end{convention}
\fi

\ePrints{8443-0072,1111.6035,0906.0135,NewAffine,1102.5168,MOmega}
\ifx\Semafor\ValueOn
\begin{convention}
Пусть $A$ - $\Omega_1$\Hyph алгебра.
Пусть $B$ - $\Omega_2$\Hyph алгебра.
Запись
\ShowEq{A->*B}
означает, что определено представление $\Omega_1$\Hyph алгебры $A$
в $\Omega_2$\Hyph алгебре $B$.
\qed
\end{convention}
\fi

\ePrints{0702.561,0707.2246,0803.2620}
\ifx\Semafor\ValueOn
\begin{convention}
Я пользуюсь стрелкой $\xymatrix{\arp[r]&}$
на диаграмме для обозначения проекции расслоения.
Я пользуюсь стрелкой $\xymatrix{\ars[r]&}$
на диаграмме для обозначения сечения расслоения.
\qed
\end{convention}
\fi

\ePrints{0912.3315}
\ifx\Semafor\ValueOn
\begin{remark}
Я считаю диаграммы отображений важным инструментом. Однако временами возникает
желание увидеть диаграмму трёх мерной, что увеличило бы её выразительную
мощность. Кто знает какие сюрпризы готовит будущее.
В 1992 на конференции в Казани я рассказывал своим коллегам
какие преимущества имеет компьютерная подготовка статей.
Спустя 8 лет из письма из Казани я узнал, что теперь можно
готовить статьи с помощью LaTeX.
\qed
\end{remark}
\fi

\ePrints{1001.4852,1003.1544,1006.2597,1011.3102}
\Items{Calculus.Paper}
\ifx\Semafor\ValueOn
\begin{convention}
Если в некотором выражении используется несколько
операций, среди которых есть операция $\circ$, то предполагается,
что операция $\circ$ выполняется первой.
Ниже приведен пример эквивалентных выражений.
\ShowEq{list circ expressions}
\qed
\end{convention}
\fi

%\ePrints{0906.0135,NewAffine}
%\ifx\Semafor\ValueOn
%\item
%Пусть $\VX X$ - базис башни представлений $(\Vector A,\Vector f)$.
%Мы будем называть $\Omega_n$\Hyph слово
%$w_n(\Vector f,\VX X,x_n)$ координатами $x_n\in A_n$
%относительно базиса $\VX X$.
%\fi

\ePrints{1107.1139}
\ifx\Semafor\ValueOn
\begin{convention}
Для данной $D$\Hyph алгебры $A$
левый сдвиг
\ShowEq{left shift, D algebra}
определён равенством
\ShowEq{left shift 1, D algebra}
и правый сдвиг
\ShowEq{right shift, D algebra}
определён равенством
\ShowEq{right shift 1, D algebra}
\qed
\end{convention}
\fi

\ifx\PrintPaper\undefined
Без сомнения, у читателя могут быть вопросы,
замечания, возражения. Я буду признателен любому отзыву.
\fi



==> Differential.English.tex <==
%auto-ignore

\input{Differential.Eq}

\ifx\PrintBook\undefined
\else
\chapter{Differentiable Maps}
\label{chapter: Differentiable maps}
\fi
\section{Topological Division Ring}
\label{section: Topological Division Ring}

\begin{definition}
Division ring $D$ is called 
\AddIndex{topological division ring}{topological division ring}\footnote{I
made definition according to definition
from \citeBib{Pontryagin: Topological Group},
chapter 4}
if $D$ is topological space and the algebraic operations
defined in $D$ are continuous in the topological space $D$.
\qed
\end{definition}

According to definition, for arbitrary elements $a, b\in D$
and for arbitrary neighborhoods $W_{a-b}$ of the element $a-b$,
$W_{ab}$ of the element $ab$ there exists neighborhoods $W_a$
of the element $a$ and $W_b$ of the element $b$ such
that $W_a-W_b\subset W_{a-b}$,
$W_aW_b\subset W_{ab}$. For any $a\ne 0$ and for arbitrary
neighborhood $W_{a^{-1}}$ there exists neighborhood $W_a$ of the element $a$,
satisfying the condition $W_a^{-1}\subset W_{a^{-1}}$.

\begin{definition}
\label{definition: absolute value on division ring}
\AddIndex{Absolute value on division ring}
{absolute value on division ring} $D$\footnote{I
made definition according to definition
from \citeBib{Bourbaki: General Topology: Chapter 5 - 10},
IX, \S 3.2} is a map
\[d\in D\rightarrow |d|\in R\]
which satisfies the following axioms
\begin{itemize}
\item $|a|\ge 0$
\item $|a|=0$ if, and only if, $a=0$
\item $|ab|=|a|\ |b|$
\item $|a+b|\le|a|+|b|$
\end{itemize}

Division ring $D$, endowed with the structure defined by a given absolute value on
$D$, is called \AddIndex{valued division ring}{valued division ring}.
\qed
\end{definition}

Invariant distance on additive group of division ring $D$
\[d(a,b)=|a-b|\]
defines topology of metric space,
compatible with division ring structure of $D$.

\begin{definition}
\label{definition: limit of sequence, valued division ring}
Let $D$ be valued division ring.
Element $a\in D$ is called 
\AddIndex{limit of a sequence}{limit of sequence}
\ShowEq{limit of sequence, valued division ring}
if for every $\epsilon\in R$, $\epsilon>0$,
there exists positive integer $n_0$ depending on $\epsilon$ and such,
that $|a_n-a|<\epsilon$ for every $n>n_0$.
\qed
\end{definition}

\ePrints{0908.3307}%
\ifx\Semafor\ValueOff%
\begin{theorem}
\label{theorem: limit of sequence, valued division ring, product on scalar}
Let $D$ be valued division ring of characteristic $0$ and let $d\in D$.
Let $a\in D$ be limit of a sequence $\{a_n\}$.
Then
\[
\lim_{n\rightarrow\infty}(a_nd)=ad
\]
\[
\lim_{n\rightarrow\infty}(da_n)=da
\]
\end{theorem}
\begin{proof}
Statement of the theorem is trivial, however I give this proof
for completeness sake. 
Since $a\in D$ is limit of the sequence $\{a_n\}$,
then according to definition \ref{definition: limit of sequence, valued division ring}
for given $\epsilon\in R$, $\epsilon>0$,
there exists positive integer $n_0$ such,
that $|a_n-a|<\epsilon/|d|$ for every $n>n_0$.
According to definition \ref{definition: absolute value on division ring}
the statement of theorem follows from inequalities
\[
|a_nd-ad|=|(a_n-a)d|=|a_n-a||d|<\epsilon/|d||d|=\epsilon
\]
\[
|da_n-da|=|d(a_n-a)|=|d||a_n-a|<|d|\epsilon/|d|=\epsilon
\]
for any $n>n_0$.
\end{proof}
\fi

\begin{definition}
Let $D$ be valued division ring.
The sequence $\{a_n\}$, $a_n\in D$ is called 
\AddIndex{fundamental}{fundamental sequence}
or \AddIndex{Cauchy sequence}{Cauchy sequence},
if for every $\epsilon\in R$, $\epsilon>0$,
there exists positive integer $n_0$ depending on $\epsilon$ and such,
that $|a_p-a_q|<\epsilon$ for every $p$, $q>n_0$.
\qed
\end{definition}

\begin{definition}
Valued division ring $D$ is called
\AddIndex{complete}{complete division ring}
if any fundamental sequence of elements
of division ring $D$ converges, i.e.
has limit in division ring $D$.
\qed
\end{definition}

\ePrints{0908.3307}%
\ifx\Semafor\ValueOff%
So far everything was good. Ring of characteristic $0$ contains ring of integers.
Division ring of characteristic $0$
contains field of rational numbers.
However this does not mean that complete division ring $D$ of characteristic $0$
contains field of real numbers.
For instance, absolute value $|x|=1$
determines discrete topology on valued
division ring and is not interesting for us,
because any fundamental sequence is
constant map.
\fi

Later on, speaking about valued division ring of characteristic $0$,
we will assume that homeomorphism of field of rational numbers $Q$
into division ring $D$ is defined.

\begin{theorem}
\label{theorem: division ring contains real number}
Complete division ring $D$ of characteristic $0$
contains as subfield an isomorphic image of the field $R$ of
real numbers.
It is customary to identify it with $R$.
\end{theorem}
\begin{proof}
Consider fundamental sequence of rational numbers $\{p_n\}$.
Let $p'$ be limit of this sequence in division ring $D$.
Let $p$ be limit of this sequence in field $R$.
Since immersion of field $Q$ into division ring $D$ is homeomorphism,
then we may identify $p'\in D$ and $p\in R$.
\end{proof}

\begin{theorem}
\label{theorem: division ring, real number}
Let $D$ be complete division ring of characteristic $0$ and let $d\in D$.
Then any real number $p\in R$ commute with $d$.
\end{theorem}
\begin{proof}
Let us represent real number $p\in R$ as
fundamental sequence of rational numbers $\{p_n\}$.
Statement of theorem follows from chain of equations
\[
pd=\lim_{n\rightarrow\infty}(p_nd)=\lim_{n\rightarrow\infty}(dp_n)=dp
\]
based on statement of theorem
\xRef{0812.4763}{theorem: limit of sequence, valued division ring, product on scalar}.
\end{proof}

\begin{theorem}
\label{theorem: real subring of center}
Let $D$ be complete division ring of characteristic $0$.
Then field of real numbers $R$ is subfield of center $Z(D)$ of division ring $D$.
\end{theorem}
\begin{proof}
Corollary of theorem \ref{theorem: division ring, real number}.
\end{proof}

\begin{definition}
Let $D$ be complete division ring of characteristic $0$.
Set of elements $d\in D$, $|d|=1$, is called
\AddIndex{unit sphere in division ring}{unit sphere in division ring} $D$.
\qed
\end{definition}

\begin{definition}
\label{definition: continuous map, division ring}
Let $D_1$ be complete division ring of characteristic $0$ with absolute value $|x|_1$.
Let $D_2$ be complete division ring of characteristic $0$ with absolute value $|x|_2$.
A map \[f:D_1\rightarrow D_2\]
is called \AddIndex{continuous}{continuous map}, if
for every as small as we please $\epsilon>0$
there exist such $\delta>0$, that
\[
|x'-x|_1<\delta
\]
implies
\[
|f(x')-f(x)|_2<\epsilon
\]
\qed
\end{definition}

\begin{theorem}
\label{theorem: continuous map of division ring}
Let $D$ be complete division ring of characteristic $0$.
Since index $s$ in expansion
\ePrints{0812.4763,0908.3307}
\ifx\Semafor\ValueOn
\EqRef{linear map, division ring, canonical morphism}
\else
\xEqRef{0701.238}{linear map, division ring, canonical morphism}
\fi
of linear map \[f:D\rightarrow D\]
belongs to finite range,
then linear map $f$
is continuous.
\end{theorem}
\begin{proof}
Suppose $x'=x+a$. Then
\[
f(x')-f(x)=f(x+a)-f(x)=f(a)=\pC{s}{0}f\ a\ \pC{s}{1}f
\]
\[
|f(x')-f(x)|=|\pC{s}{0}f\ a\ \pC{s}{1}f|<(|\pC{s}{0}f|\ |\pC{s}{1}f|)|a|
\]
Let us denote $F=|\pC{s}{0}f|\ |\pC{s}{1}f|$. Then
\[
|f(x')-f(x)|<F|a|
\]
Suppose $\epsilon>0$ and let us assume $\displaystyle a=\frac{\epsilon}Fe$.
Then $\displaystyle\delta=|a|=\frac{\epsilon}F$.
According to definition \ref{definition: continuous map, division ring},
linear map $f$ is continuous.
\end{proof}

\ePrints{0908.3307}%
\ifx\Semafor\ValueOff%
Similarly, since index $s$ belongs to countable range,
then for continuity of additive map $f$ it is necessary that series
$|\pC{s}{0}f|\ |\pC{s}{1}f|$ converges.
Since index $s$ belongs to continues range,
then for continuity of additive map $f$ it is necessary that integral
$\int|\pC{s}{0}f|\ |\pC{s}{1}f|ds$ exist.
\fi

\begin{definition}
\label{definition: norm of map, division ring}
Let
\[f:D_1\rightarrow D_2\]
be map of complete division ring $D_1$ of characteristic $0$ with absolute value $|x|_1$
into complete division ring $D_2$ of characteristic $0$ with absolute value $|y|_2$.
Value
\ShowEq{norm of map}
\ShowEq{norm of map, division ring}
is called
\AddIndex{norm of map $f$}{norm of map}.
\qed
\end{definition}

\begin{theorem}
\label{theorem: continuity of linear map, finite norm, division ring}
Let
\[f:D_1\rightarrow D_2\]
be linear map of complete division ring $D_1$
into complete division ring $D_2$.
Since $\|f\|<\infty$, then map $f$ is continuous.
\end{theorem}
\begin{proof}
Because map $f$ is additive, then
according to definition \ref{definition: norm of map, division ring}
\[
|f(x)-f(y)|_2=|f(x-y)|_2\le \|f\|\ |x-y|_1
\]
Let us assume arbitrary $\epsilon>0$. Assume $\displaystyle\delta=\frac\epsilon{\|f\|}$.
Then
\[
|f(x)-f(y)|_2\le \|f\|\ \delta=\epsilon
\]
follows from inequality
\[
|x-y|_1<\delta
\]
According to definition \ref{definition: continuous map, division ring},
map $f$ is continuous.
\end{proof}

\begin{theorem}
\label{theorem: continuous linear map, real number, division ring}
Let map
\ShowEq{f d1 d2}
be continuous linear map of division ring $D_1$ of characteristic $0$
into division ring $D_2$ of characteristic $0$.
Then
\[
f(ax)=af(x)
\]
for any real number $a$.
\end{theorem}
\begin{proof}
According to the theorem
\ref{theorem: real subring of center},
real field is subfield of the center $Z(D)$ of division ring $D$.
Let us represent real number $p\in R$ as
fundamental sequence of rational numbers $\{p_n\}$.
The statement of theorem
follows from theorems
\ref{theorem: linear map, division ring, rational},
\xRef{0812.4763}{theorem: limit of sequence, valued division ring, product on scalar}
and chain of equations
\ShowEq{continuous linear map, real number, division ring, 1}
\end{proof}

\ifx\texFuture\Defined
\begin{theorem}
\label{theorem: continuity of map, norm, division ring}
Let
\[f:D_1\rightarrow D_2\]
map of complete division ring $D_1$
в complete division ring $D_2$.
map $f$ is continuous, if $\|f\|<\infty$.
\end{theorem}
\begin{proof}
Since map $f$ is additive, then
according to definition \ref{definition: norm of map, division ring}
\[
|f(x)-f(y)|_2=|f(x-y)|_2\le \|f\|\ |x-y|_1
\]
Let $\epsilon>0$ be arbitrary. Assume $\displaystyle\delta=\frac\epsilon{\|f\|}$.
Then from inequality
\[
|x-y|_1<\delta
\]
follows
\[
|f(x)-f(y)|_2\le \|f\|\ \delta=\epsilon
\]
According to definition \ref{definition: continuous map, division ring},
map $f$ is continuous.
\end{proof}
\fi

\ePrints{0812.4763}
\ifx\Semafor\ValueOn

\begin{theorem}
\label{theorem: projective map in 0, division ring}
Let $D$ be complete division ring of characteristic $0$.
Either continuous map $f$ of division ring which is projective over field $P$,
does not depend on direction over field $P$,
or value $f(0)$ is not defined.
\end{theorem}
\begin{proof}
According to definition
\ref{definition: map projective over commutative ring, ring},
map $f$
is constant on direction $Pa$. Since $0\in Pa$,
then we may assume
\[
f(0)=f(a)
\]
based on continuity.
However this leads to uncertainty of value
of map $f$ in direction $0$,
when map $f$ has different values for different directions $a$.
\end{proof}

If projective over field $R$ map $f$ is continuous,
then we say that
\AddIndex{map $f$ is continuous in direction over field}
{projective map is continuous in direction over field} $R$.
Since for any $a\in D$, $a\ne 0$ we may choose
$a_1=|a|^{-1}a$, $f(a_1)=f(a)$, then it is possible to make definition more accurate.

\begin{definition}
\label{definition: projective function is continuous in direction over field R, division ring}
Let $D$ be complete division ring of characteristic $0$.
Projective over field $R$ function $f$ is continuous
in direction over field $R$, if
for every as small as we please $\epsilon>0$
there exists such $\delta>0$, that
\[
|x'-x|_1<\delta\ \ \ |x'|_1=|x|_1=1
\]
implies
\[
|f(x')-f(x)|_2<\epsilon
\]
\qed
\end{definition}

\begin{theorem}
\label{theorem: projective function is continuous in direction over field R, division ring}
Let $D$ be complete division ring of characteristic $0$.
Projective over field $R$ function $f$ is continuous
in direction over field $R$ iif
this function is continuous on unit sphere of division ring $D$.
\end{theorem}
\begin{proof}
Corollary of definitions \ref{definition: continuous map, division ring},
\ref{definition: map projective over commutative ring, ring},
\ref{definition: projective function is continuous in direction over field R, division ring}.
\end{proof}
\fi

\section{Differentiable Map of Division Ring}
\label{section: Differentiable maps of Division Ring}

\ePrints{0812.4763}
\ifx\Semafor\ValueOn
\begin{definition}
\label{definition: differentiable functions, division ring}
Let $D$ be valued division ring.\footnote{I
made definition according to definition
\citeBib{Lebedev Vorovich}-3.1.1,
page 177.}
Function \[f:D\rightarrow D\] is called
\AddIndex{\Ds differentiable in the Fr\'echet sense}
{function Dstar differentiable in Frechet sense, division ring}
on the set $U\subset D$\footnote{Like in remark
\xRef{0701.238}{remark: drc linear map}
we may define \Ds differentiability of map \[f:S\rightarrow D\]
of valued division ring $S$
into valued division ring $D$ according to rule
\[
f(x+h)-f(x)
=F(h)\frac{d f(x)}{d_*x}
+o(h)
\]
where \[F:S\rightarrow D\] is homomorphism of division rings.
However, based on isomorphism theorem, we may confine ourselves by case of
maps of division ring $D$ into $D$.},
if at every point $x\in U$ the increment of the function $f$ can be represented as
\symb{\frac{d f(x)}{d_*x}}0{Frechet Dstar derivative of map, division ring}
\begin{equation}
\EqLabel{Dstar derivative, division ring}
f(x+h)-f(x)
=h\ShowSymbol{Frechet Dstar derivative of map, division ring}
+o(h)
\end{equation}
where $o$ is such continuous map
\[o:D\rightarrow D\]
that
\begin{equation}
\EqLabel{infinitesimal, division ring}
\lim_{h\rightarrow 0}\frac{|o(h)|}{|h|}=0
\end{equation}
\qed
\end{definition}

According to definition \ref{definition: differentiable functions, division ring},
\AddIndex{the Fr\'echet \Ds derivative of map $f$ at point $x$}
{Frechet Dstar derivative of map, division ring}
\[
\ShowSymbol{Frechet Dstar derivative of map, division ring}\in {}_*\mathcal L(D,D)
\]
generates a homomorphism
\[
\Delta f
=\Delta x\frac{d f(x)}{d_*x}
\]
which maps increment of argument into increment of function.

If we multiply both sides of equation
\EqRef{Dstar derivative, division ring}
by $h^{-1}$, then we get equation
\begin{equation}
\EqLabel{Dstar derivative, division ring, 1}
h^{-1}(f(x+h)-f(x))
=\frac{d f(x)}{d_*x}
+h^{-1}o(h)
\end{equation}
Alternative definition of the Fr\'echet \Ds derivative
\begin{equation}
\EqLabel{Dstar derivative, division ring, 2}
\frac{d f(x)}{d_*x}
=\lim_{h\rightarrow 0}(h^{-1}(f(x+h)-f(x)))
\end{equation}
follows from equations \EqRef{Dstar derivative, division ring, 1} and
\EqRef{infinitesimal, division ring}.

In contrast to derivative of map over field $F$
the Fr\'echet \Ds derivative of map of division ring $D$ is not
linear map. Indeed, the Fr\'echet \Ds derivative is \sD
linear map; however, in general, it is not \Ds
linear map. In fact,
\[
f(x+h)a-f(x)a=h\frac{df}{d_*x}a+o(h)
\]
\begin{equation}
\EqLabel{Dstar derivative, division ring, 3}
af(x+h)-af(x)=ah\frac{df}{d_*x}+o(h)
\end{equation}
However, in general,
\[
ah\frac{df}{d_*x}\ne ha\frac{df}{d_*x}
\]

Similar problem arises when we differentiate product of maps.
According to definition \ref{definition: differentiable functions, division ring}
\begin{equation}
f(x+h)g(x+h)-f(x)g(x)
=h\frac{df(x)g(x)}{d_*x}+o(h)
\EqLabel{product of maps, derivative, 0}
\end{equation}
It is possible to represent expression in left side as
\begin{align}
&f(x+h)g(x+h)-f(x)g(x)\nonumber\\
\EqLabel{product of maps, derivative, 1}
=&f(x+h)g(x+h)-f(x)g(x+h)+f(x)g(x+h)-f(x)g(x)\\
=&(f(x+h)-f(x))g(x+h)+f(x)(g(x+h)-g(x))\nonumber
\end{align}
According to definition \ref{definition: differentiable functions, division ring},
it is possible to represent \EqRef{product of maps, derivative, 1} as
\begin{align}
&f(x+h)g(x+h)-f(x)g(x)\nonumber\\
\EqLabel{product of maps, derivative, 2}
=&\left(h\frac{df(x)}{d_*x}+o(h)\right)
\left(g(x)+h\frac{dg(x)}{d_*x}+o(h)\right)\\
+&f(x)\left(h\frac{dg(x)}{d_*x}+o(h)\right)\nonumber
\end{align}
Since, in general,
\[
f(x)h\frac{dg}{d_*x}\ne hf(x)\frac{dg}{d_*x}
\]
then it is natural to anticipate that map $f(x)g(x)$
is not \Ds differentiable in the Fr\'echet sense.

Thus definition the Fr\'echet \Ds derivative is extremely restricted
and does not satisfy standard definition of differentiation.
To find solution of problem of differentiation,
Consider this problem on the other hand.
\fi

\begin{example}
\label{example: differential dxx}
Consider increment of map $f(x)=x^2$.
\begin{align*}
f(x+h)-f(x)
&=(x+h)^2-x^2
\\
&=xh+hx+h^2
\\
&=xh+hx+o(h)
\end{align*}
As can be easily seen, the component of the increment of the function $f(x)=x^2$
that is linearly dependent on the increment of the argument, is of the form
\[
xh+hx
\]
Since product is non commutative,
we cannot represent increment of map $f(x+h)-f(x)$
as $Ah$ or $hA$
where $A$ does not depend on $h$.
It results in the unpredictable behavior of
the increment of the function $f(x)=x^2$ when
the increment of the argument converges to $0$.
However, since infinitesimal $h$ is infinitesimal like
$h=ta$, $a\in D$, $t\in R$, $t\rightarrow 0$, the answer becomes
more definite
\[
(xa+ax)t
\]
\qed
\end{example}

\begin{definition}
\label{definition: map differentiable in Gateaux sense, division ring}
Let $D$ be complete division ring of characteristic $0$.\footnote{I
made definition according to definition
\citeBib{Lebedev Vorovich}-3.1.2,
page 177.}
The map \[f:D\rightarrow D\]
is called \AddIndex{differentiable in the G\^ateaux sense}
{map differentiable in Gateaux sense} on the set $U\subset D$,
if at every point $x\in U$
the increment of the function $f$ can be represented as
\ShowEq{Gateaux derivative of map, division ring, def}
\ShowEq{Gateaux differential of map, division ring}
where
\AddIndex{the G\^ateaux derivative
$\ShowSymbol{Gateaux derivative of map}$
of map $f$}
{Gateaux derivative of map}
is linear map of increment $a$ and
$o:D\rightarrow D$ is such continuous map that
\[
\lim_{a\rightarrow 0}\frac{|o(a)|}{|a|}=0
\]
\qed
\end{definition}

\begin{remark}
\label{remark: differential L(D,D)}
According to definition
\ref{definition: map differentiable in Gateaux sense, division ring}
for given $x$, the G\^ateaux derivative $\partial f(x)\in\mathcal L(D;D)$.
Therefore, the G\^ateaux derivative of map $f$ is map
\ShowEq{differential L(D,D)}
Expressions $\partial f(x)$ and $\displaystyle\frac{\partial f(x)}{\partial x}$
are different notations for the same function.
We will use notation $\displaystyle\frac{\partial f(x)}{\partial x}$
to underline that this is  the G\^ateaux derivative with respect to variable $x$.
\qed
\end{remark}

\begin{theorem}
\label{theorem: map differentiable in Gateaux sense, division ring}
It is possible to represent the G\^ateaux derivative
of map $f$ as
\ShowEq{Gateaux derivative, representation}
\end{theorem}
\begin{proof}
Corollary of definition
\ref{definition: map differentiable in Gateaux sense, division ring}
and theorem
\ePrints{0812.4763,0908.3307}
\ifx\Semafor\ValueOn
\ref{theorem: linear map, division ring, canonical morphism}.
\else
\xRef{0701.238}{theorem: linear map, division ring, canonical morphism}.
\fi
\end{proof}

\begin{definition}
\begin{sloppypar}
Expression
\ShowEq{component of Gateaux derivative of map, division ring}
is called
\AddIndex{component of the G\^ateaux derivative of map $f(x)$}
{component of Gateaux derivative of map, division ring}.
\qed
\end{sloppypar}
\end{definition}

\begin{theorem}
\label{theorem: Gateaux derivative is linear over field R, division ring}
Let $D$ be division ring of characteristic $0$.
Let function \[f:D\rightarrow D\]
be differentiable in the G\^ateaux sense
Then
\ShowEq{Gateaux derivative is linear over field R, division ring}
for any real number $a$.
\end{theorem}
\begin{proof}
Corollary of theorem
\ref{theorem: continuous linear map, real number, division ring} and
definition
\ref{definition: map differentiable in Gateaux sense, division ring}.
\end{proof}

Combining equation
\EqRef{Gateaux derivative is linear over field R, division ring}
and definition
\ref{definition: map differentiable in Gateaux sense, division ring},
we get known definition of the G\^ateaux
differential
\ShowEq{Gateaux derivative, representation, 2}
Definitions of the G\^ateaux derivative \EqRef{Gateaux differential of map, division ring}
and \EqRef{Gateaux derivative, representation, 2}
are equivalent. Using this equivalence we tell
that map $f$
is called differentiable in the G\^ateaux sense on the set $U\subset D$,
if at every point $x\in U$
the increment of the function $f$ can be represented as
\begin{equation}
\EqLabel{Gateaux differential of map, t, division ring}
f(x+ta)-f(x)
=t\partial f(x)(a)
+o(t)
\end{equation}
where
$o:R\rightarrow D$ is such continuous map that
\[
\lim_{t\rightarrow 0}\frac{|o(t)|}{|t|}=0
\]

Since infinitesimal $a$ in the equation
\EqRef{Gateaux derivative, representation}
is differential $dx$,
then equation
\EqRef{Gateaux derivative, representation}
becomes definition of
\AddIndex{the G\^ateaux differential}{Gateaux differential of map}
\ShowEq{Gateaux differential, division ring}
\ShowEq{Gateaux differential, form}

\begin{theorem}
\label{theorem: Gateaux derivative, standard form, division ring}
Let $D$ be division ring of characteristic $0$.
Let $\Basis e$ be basis of division ring $D$ over center $Z(D)$ of division ring $D$.
\symb{\StandPartial{f(x)}{x}{ij}}0
{standard component of Gateaux derivative}
\AddIndex{Standard representation of the G\^ateaux derivative}
{Gateaux derivative, standard representation}
\EqRef{Gateaux derivative, representation}
of map\[f:D\rightarrow D\]
has form
\ShowEq{Gateaux derivative, division ring, standard representation}
Expression
$\displaystyle
\ShowSymbol{standard component of Gateaux derivative}$
in equation \EqRef{Gateaux derivative, division ring, standard representation}
is called
\AddIndex{standard component of the G\^ateaux derivative}
{standard component of Gateaux derivative} of map $f$.
\end{theorem}
\begin{proof}
Statement of theorem is corollary of theorem
\ePrints{0812.4763,0908.3307}
\ifx\Semafor\ValueOn
\ref{theorem: linear map, standard form, division ring}.
\else
\xRef{0701.238}{theorem: linear map, standard form, division ring}.
\fi
\end{proof}

\begin{theorem}
Let $D$ be division ring of characteristic $0$.
Let $\Basis e$ be basis of division ring $D$ over
field $F\subset Z(D)$.
Then it is possible to represent the G\^ateaux differential of map
\[
f:D\rightarrow D
\]
as
\ShowEq{Gateaux derivative and Jacobian, division ring}
where $a\in D$ has expansion
\ShowEq{expansion a  in D}
relative to basis $\Basis e$ and Jacobian matrix of map $f$ has form
\begin{equation}
\EqLabel{standard components and Jacobian, division ring}
\frac{\partial f^{\gij}}{\partial x^{\gii}}=
\StandPartial{f(x)}{x}{kr}\ C^{\gi p}_{\gi{ki}}\ C^{\gij}_{\gi{pr}}
\end{equation}
\end{theorem}
\begin{proof}
Statement of theorem is corollary of theorem
\ePrints{0812.4763,0908.3307}
\ifx\Semafor\ValueOn
\ref{theorem: linear map over field, division ring}.
\else
\xRef{0701.238}{theorem: linear map over field, division ring}.
\fi
\end{proof}

\ePrints{0908.3307}%
\ifx\Semafor\ValueOff%
To find structure similar to derivative in commutative calculus
we need extract derivative from differential
of map. For this purpose we need
take the increment of argument outside brackets.\footnote{It is possible when all
$\displaystyle \frac{\pC{s}{0}\partial f(x)}{\partial x}=e$
or all
$\displaystyle \frac{\pC{s}{1}\partial f(x)}{\partial x}=e$.
Therefore definition
\citeBib{Lebedev Vorovich}-3.1.2,
page 177, leads us either to definition of
the Fr\'echet \Ds derivative,
or to definition of
the Fr\'echet \sD derivative.}
It is possible to take $a$ outside brackets
using equations
\ShowEq{need extract derivative from differential}
\fi

\begin{definition}
\label{definition: Gateaux Dstar derivative, division ring}
Let $D$ be complete division ring of characteristic $0$
and $a\in D$.
\symb{\frac{\partial f(x)(a)}{\partial_* x}}
0{Gateaux Dstar derivative of map, division ring}
We define \AddIndex{the G\^ateaux \Ds derivative
$\displaystyle\ShowSymbol{Gateaux Dstar derivative of map, division ring}$
of map $f:D\rightarrow D$}
{Gateaux Dstar derivative of map, division ring}
using equation
\begin{equation}
\EqLabel{Gateaux Dstar derivative, division ring}
\partial f(x)(a)
=a\ShowSymbol{Gateaux Dstar derivative of map, division ring}
\end{equation}
\symb{\frac{\partial f(x)(a)}{{}_*\partial x}}
0{Gateaux starD derivative of map, division ring}
We define \AddIndex{the G\^ateaux \sD derivative
$\displaystyle\ShowSymbol{Gateaux starD derivative of map, division ring}$
of map $f:D\rightarrow D$}
{Gateaux starD derivative of map, division ring}
using equation
\begin{equation}
\EqLabel{Gateaux starD derivative, division ring}
\partial f(x)(a)
=\ShowSymbol{Gateaux starD derivative of map, division ring}a
\end{equation}
\qed
\end{definition}

\ePrints{0908.3307}%
\ifx\Semafor\ValueOff%
For representation of the G\^ateaux \Ds derivative
we also use notation
\[
\frac{\partial f(x)(a)}{\partial_* x}=\frac{\partial}{\partial_* x} f(x)(a)=\partial_* f(x)(a)
\]

For representation of the G\^ateaux \sD derivative
we also use notation
\[
\frac{\partial f(x)(a)}{{}_*\partial x}=\frac{\partial}{{}_*\partial x} f(x)(a)={}_*\partial f(x)(a)
\]

Based on duality principle
\xRef{0701.238}{theorem: duality principle, vector space},
we will study \Ds derivative, keeping in mind that dual statement
is true for \sD derivative.

Because product is not commutative, concept of fraction is not defined in division ring.
We need explicitly show from which side denominator has an effect on numerator.
Symbol $*$ in denominator of fraction implements this function.
According to definition
\[
\frac{\partial f}{\partial_* x}=(\partial_* x)^{-1}\partial f
\]
\[
\frac{\partial f}{{}_*\partial x}=\partial f({}_*\partial x)^{-1}
\]
Thus, we may represent
the G\^ateaux \Ds derivative of function $f$
as ratio of change of function to change of argument.
We do not extend this remark to
components of the G\^ateaux differential.
In this case we consider notation
$\displaystyle\frac{\partial}{\partial_* x}$
and $\displaystyle\frac{\partial}{{}_*\partial x}$ not
as fraction, but as symbol of operator.

Then we can write equation \EqRef{Gateaux Dstar derivative, division ring}
as
\begin{equation}
\EqLabel{Gateaux differential, division ring, 1}
\partial f(x)(dx)
=dx(\partial_* x)^{-1}\partial f(x)(dx)
\end{equation}
It is easy to see that
we wrote \Ds differential of variable $x$
in denominator of fraction in equation
\EqRef{Gateaux differential, division ring, 1},
however we multiply fraction by
differential of variable $x$.
\fi

\begin{theorem}
\label{theorem: Dstar derivative is multiplicative over field R, division ring}
Let $D$ be complete division ring of characteristic $0$.
The G\^ateaux \Ds derivative is projective
over field of real numbers $R$.
\end{theorem}
\begin{proof}
Corollary of theorems
\ref{theorem: Gateaux derivative is linear over field R, division ring}
and example
\ePrints{0812.4763,0908.3307}
\ifx\Semafor\ValueOn
\ref{example: map projective over commutative ring, ring}.
\else
\xRef{0701.238}{example: map projective over commutative ring, ring}.
\fi
\end{proof}

From theorem \ref{theorem: Dstar derivative is multiplicative over field R, division ring}
it follows
\begin{equation}
\EqLabel{Dstar derivative is multiplicative over field R, division ring}
\frac{\partial f(x)(ra)}{\partial_* x}
=\frac{\partial f(x)(a)}{\partial_* x}
\end{equation}
for every $r\in R$, $r\ne 0$ and  $a\in D$, $a\ne 0$.
Therefore the G\^ateaux \Ds derivative
is well defined in direction $a$ over field $R$, $a\in D$, $a\ne 0$,
and does not depend on the choice of value in this direction.

\begin{theorem}
Let $D$ be complete division ring of characteristic $0$
and $a\ne 0$.
The G\^ateaux \Ds derivative and the G\^ateaux \sD derivative of map $f$ of division ring $D$
are bounded by relationship
\begin{equation}
\EqLabel{Dstar derivative and starD derivative in direction, division ring}
\frac{\partial f(x)(a)}{{}_*\partial x} 
=a\frac{\partial f(x)(a)}{\partial_* x} a^{-1}
\end{equation}
\end{theorem}
\begin{proof}
From equations \EqRef{Gateaux Dstar derivative, division ring}
and \EqRef{Gateaux starD derivative, division ring}
it follows
\[
\frac{\partial f(x)(a)}{{}_*\partial x}
=\partial f(x)(a)a^{-1}
=a\frac{\partial f(x)(a)}{\partial_* x}a^{-1}
\]
\end{proof}

\begin{theorem}
Let $D$ be complete division ring of characteristic $0$.
The G\^ateaux derivative satisfies to relationship
\begin{equation}
\EqLabel{Gateaux derivative of product, division ring}
\partial (f(x)g(x))(a)
=\partial f(x)(a)\ g(x)+f(x)\ \partial g(x)(a)
\end{equation}
\end{theorem}
\begin{proof}
Equation \EqRef{Gateaux derivative of product, division ring}
follows from chain of equations
\begin{align*}
\partial (f(x)g(x))(a)
&=\lim_{t\rightarrow 0}(t^{-1}(f(x+ta)g(x+ta)-f(x)g(x)))
\\
&=\lim_{t\rightarrow 0}(t^{-1}(f(x+ta)g(x+ta)-f(x)g(x+ta)))
\\
&+\lim_{t\rightarrow 0}(t^{-1}(f(x)g(x+ta)-f(x)g(x)))
\\
&=\lim_{t\rightarrow 0}(t^{-1}(f(x+ta)-f(x)))g(x)
\\
&+f(x)\lim_{t\rightarrow 0}(t^{-1}(g(x+ta)-g(x)))
\end{align*}
based on definition \EqRef{Gateaux derivative, representation, 2}.
\end{proof}

\begin{theorem}
Let $D$ be complete division ring of characteristic $0$.
Suppose the G\^ateaux derivative
of map $f:D\rightarrow D$
has expansion
\ShowEq{Gateaux derivative of f, division ring}
Suppose the G\^ateaux derivative
of map $g:D\rightarrow D$
has expansion
\ShowEq{Gateaux derivative of g, division ring}
Components of the G\^ateaux derivative of map $f(x)g(x)$
have form
\ShowEq{component of Gateaux derivative, fg, division ring}
\end{theorem}
\begin{proof}
Let us substitute \EqRef{Gateaux derivative of f, division ring}
and \EqRef{Gateaux derivative of g, division ring}
into equation \EqRef{Gateaux derivative of product, division ring}
\ShowEq{Gateaux derivative of fg, division ring}
Based \EqRef{Gateaux derivative of fg, division ring},
we define equations
\EqRef{0 component of Gateaux derivative, fg, division ring},
\EqRef{1 component of Gateaux derivative, fg, division ring}.
\end{proof}

\begin{theorem}
Let $D$ be complete division ring of characteristic $0$.
The G\^ateaux \Ds derivative satisfy to relationship
\begin{equation}
\EqLabel{Gateaux Dstar derivative of product, division ring}
\frac{\partial f(x)g(x)}{\partial_* x}(a)
=\frac{\partial f(x)(a)}{\partial_* x}g(x)+a^{-1}f(x)a\frac{\partial g(x)(a)}{\partial_* x}
\end{equation}
\end{theorem}
\begin{proof}
Equation \EqRef{Gateaux Dstar derivative of product, division ring}
follows from chain of equations
\begin{align*}
\frac{\partial f(x)g(x)}{\partial_* x}(a)
&=a^{-1}\partial f(x)g(x)(a)
\\
&=a^{-1}(\partial f(x)(a)g(x)+f(x)\partial g(x)(a))
\\
&=a^{-1}\partial f(x)(a)g(x)+a^{-1}f(x)aa^{-1}\partial g(x)(a)
\\
&=\frac{\partial f(x)(a)}{\partial_* x}g(x)+a^{-1}f(x)a\frac{\partial g(x)(a)}{\partial_* x}
\end{align*}
\end{proof}

\begin{theorem}
Let $D$ be complete division ring of characteristic $0$.
Either the G\^ateaux \Ds derivative  does not depend on direction,
or the G\^ateaux \Ds derivative in direction $0$ is not defined.
\end{theorem}
\begin{proof}
Statement of theorem is corollary
of theorem \ref{theorem: Dstar derivative is multiplicative over field R, division ring}
and theorem \ref{theorem: projective map in 0, division ring}.
\end{proof}

\begin{theorem}
\label{theorem: norm of Gateaux differential, division ring}
Let $D$ be complete division ring of characteristic $0$.
Let unit sphere of division ring $D$ be compact.
If the G\^ateaux \Ds derivative
$\displaystyle\frac{\partial f(x)(a)}{\partial_* x}$
exists in point $x$ and is continuous in direction over field $R$,
then there exist norm $\|\partial f(x)\|$ of the G\^ateaux \Ds differential.
\end{theorem}
\begin{proof}
From definition \ref{definition: Gateaux Dstar derivative, division ring}
it follows
\begin{equation}
\EqLabel{norm of Gateaux differential, division ring, 1}
|\partial f(x)(a)|
=|a|\ \left|\frac{\partial f(x)(a)}{\partial_* x}\right|
\end{equation}
From theorems
\xRef{0812.4763}{theorem: projective function is continuous in direction over field R, division ring},
\ref{theorem: Dstar derivative is multiplicative over field R, division ring}
it follows, that the G\^ateaux \Ds derivative is continuous
on unit sphere.
Since unit sphere is compact, then range
the G\^ateaux \Ds derivative of function $f$ at point $x$ is bounded
\[
\left|
\frac{\partial f(x)(a)}{\partial_* x}
\right|
<F=\text{sup}\left|
\frac{\partial f(x)(a)}{\partial_* x}
\right|
\]
According to definition \ref{definition: norm of map, division ring}
\[
\|\partial f(x)\|=F
\]
\end{proof}

\begin{theorem}
\label{theorem: Dstar derivative and continuos function, division ring}
Let $D$ be complete division ring of characteristic $0$.
Let unit sphere of division ring $D$ be compact.
If the G\^ateaux \Ds derivative
$\displaystyle\frac{\partial f(x)(a)}{\partial_* x}$
exists in point $x$ and is continuous in direction over field $R$,
then function $f$ is continuous at point $x$.
\end{theorem}
\begin{proof}
From theorem \ref{theorem: norm of Gateaux differential, division ring}
it follows
\begin{equation}
\EqLabel{Dstar derivative and continuos function, division ring, 1}
|\partial f(x)(a)|
\le\|\partial f(x)\| |a|
\end{equation}
From \EqRef{Gateaux differential of map, division ring},
\EqRef{Dstar derivative and continuos function, division ring, 1}
it follows
\begin{equation}
\EqLabel{Dstar derivative and continuos function, division ring, 2}
|f(x+a)-f(x)|<|a|\ \|\partial f(x)\|
\end{equation}
Let us assume arbitrary $\epsilon>0$. Assume
\[\delta=\frac\epsilon{\|\partial f(x)\|}\]
Then from inequality
\[
|a|<\delta
\]
it follows
\[
|f(x+a)-f(x)|\le \|\partial f(x)\|\ \delta=\epsilon
\]
According to definition \ref{definition: continuous map, division ring},
map $f$ is continuous at point $x$.
\end{proof}

\ePrints{0908.3307}%
\ifx\Semafor\ValueOff%
Theorem \ref{theorem: Dstar derivative and continuos function, division ring}
has interesting generalization. If unit sphere of division ring $D$ is not compact,
then we may consider compact set of directions instead of unit sphere.
In this case we may speak about continuity of function $f$ along selected set
of directions.
\fi

\section{Table of Derivatives of Map of Division Ring}

\begin{theorem}
\label{theorem: Gateaux differential of const, division ring}
Let $D$ be complete division ring of characteristic $0$.
Then for any $b\in D$
\begin{equation}
\EqLabel{Gateaux differential of const, division ring}
\partial (b)(a)
=0
\end{equation}
\end{theorem}
\begin{proof}
Immediate corollary of definition
\ref{definition: map differentiable in Gateaux sense, division ring}.
\end{proof}

\begin{theorem}
\label{theorem: Gateaux differential, product over constant, division ring}
Let $D$ be complete division ring of characteristic $0$.
Then for any $b$, $c\in D$
\ShowEq{Gateaux differential, product over constant, division ring}
\end{theorem}
\begin{proof}
Immediate corollary of equations
\EqRef{Gateaux derivative of product, division ring},
\EqRef{0 component of Gateaux derivative, fg, division ring},
\EqRef{1 component of Gateaux derivative, fg, division ring},
\EqRef{Gateaux Dstar derivative of product, division ring}
because $\partial b=\partial c=0$.
\end{proof}

\begin{theorem}
\label{theorem: Gateaux differential, product over constant, fx=x, division ring}
Let $D$ be complete division ring of characteristic $0$.
Then for any $b$, $c\in D$
\ShowEq{Gateaux differential, product over constant, fx=x, division ring}
\end{theorem}
\begin{proof}
Corollary of theorem
\ref{theorem: Gateaux differential, product over constant, division ring},
when $f(x)=x$.
\end{proof}

\begin{theorem}
%\label{theorem: Gateaux differential, product over constant, fx=x, division ring}
Let $D$ be complete division ring of characteristic $0$.
Then for any $b\in D$
\ShowEq{Gateaux differential, xb-bx, division ring}
\end{theorem}
\begin{proof}
Corollary of theorem
\ref{theorem: Gateaux differential, product over constant, division ring},
when $f(x)=x$.
\end{proof}

\begin{theorem}
Let $D$ be complete division ring of characteristic $0$.
Then\footnote{The statement of the theorem is similar to example VIII,
\citeBib{Hamilton Elements of Quaternions 1}, p. 451.
If product is commutative, then the equation
\EqRef{derivative x2, division ring}
gets form
\ShowEq{derivative x2, field}}
\ShowEq{derivative x2, division ring}
\ShowEq{derivative x2, component of Gateaux differential, division ring}
\end{theorem}
\begin{proof}
\EqRef{derivative x2, division ring} follows from example \ref{example: differential dxx}
and definition \ref{definition: Gateaux Dstar derivative, division ring}.
\EqRef{derivative x2, component of Gateaux differential, division ring}
follows from example \ref{example: differential dxx}
and equation \EqRef{Gateaux differential, form}.
\end{proof}

\begin{theorem}
Let $D$ be complete division ring of characteristic $0$.
Then\footnote{The statement of the theorem is similar to example IX,
\citeBib{Hamilton Elements of Quaternions 1}, p. 451.
If product is commutative, then the equation
\EqRef{derivative x power -1, division ring}
gets form
\ShowEq{derivative x power -1, field}}
\ShowEq{derivative x power -1, division ring}
\end{theorem}
\begin{proof}
Let us substitute $f(x)=x^{-1}$ in definition
\EqRef{Gateaux derivative, representation, 2}.
\begin{align}
\partial f(x)(h)
&=\lim_{t\rightarrow 0,\ t\in R}(t^{-1}((x+th)^{-1}-x^{-1}))
\nonumber
\\
&=\lim_{t\rightarrow 0,\ t\in R}(t^{-1}((x+th)^{-1}-x^{-1}(x+th)(x+th)^{-1}))
\nonumber
\\
&=\lim_{t\rightarrow 0,\ t\in R}(t^{-1}(1-x^{-1}(x+th))(x+th)^{-1})
\EqLabel{derivative x power -1, division ring, 1}
\\
&=\lim_{t\rightarrow 0,\ t\in R}(t^{-1}(1-1-x^{-1}th)(x+th)^{-1})
\nonumber
\\
&=\lim_{t\rightarrow 0,\ t\in R}(-x^{-1}h(x+th)^{-1})
\nonumber
\end{align}
Equation \EqRef{derivative x power -1, division ring}
follows from chain of equations
\EqRef{derivative x power -1, division ring, 1}.
\end{proof}

\begin{theorem}
Let $D$ be complete division ring of characteristic $0$.
Then\footnote{If product is commutative, then
\[
y=xax^{-1}=a
\]
Accordingly, the derivative is $0$.}
\ShowEq{derivative xax power -1, division ring}
\end{theorem}
\begin{proof}
Equation \EqRef{derivative xax power -1, division ring}
is corollary of equations \EqRef{Gateaux derivative of product, division ring},
\EqRef{Gateaux differential, product over constant, fx=x, division ring},
\EqRef{derivative xax power -1, division ring}.
\end{proof}


==> Differential.Eq.tex <==
%auto-ignore

\ePrints{0812.4763,0908.3307}
\ifx\Semafor\ValueOn

\DefEq
{
\[f:D_1\rightarrow D_2\]
}
{f d1 d2}

\DefEquation
{
\partial f(x)(a)=a^{\gii}\ \frac{\partial f^{\gij}}{\partial x^{\gii}}
e_{\gij}
}
{Gateaux derivative and Jacobian, division ring}

\DefEq
{
\symb{\|f\|}0{norm of map}
}
{norm of map}

\DefEquation
{
\ShowSymbol{norm of map}=
\text{sup}\frac{|f(x)|_2}{|x|_1}
}
{norm of map, division ring}

\DefEq
{
$\{a_n\}$
\symb{\lim_{n\rightarrow\infty}a_n}0{limit of sequence}
\[
a=\ShowSymbol{limit of sequence}
\]
}
{limit of sequence, valued division ring}

\fi

\DefEquation
{
\partial f(x)(ah)=a\partial f(x)(h)
}
{Gateaux derivative is linear over field R, division ring}

\DefEquation
{
f(x+a)-f(x)
=\ShowSymbol{Gateaux derivative of map}(a)
+o(a)
=\ShowSymbol{Gateaux derivative of map, fraction}(a)
+o(a)
}
{Gateaux differential of map, division ring}

\DefEq
{
\symb{\partial f(x)(dx)}0{Gateaux differential of map, scalar}
}
{Gateaux differential, division ring}

\DefEquation
{
\partial f(x)(a)
=\frac{\partial_{s\cdot 0} f(x)}{\partial x}
\ a
\ \frac{\partial_{s\cdot 1} f(x)}{\partial x}
}
{Gateaux derivative, representation}

\DefEquation
{
\ShowSymbol{Gateaux differential of map, scalar}
=\frac{\partial_{s\cdot 0} f(x)}{\partial x}
dx
\frac{\partial_{s\cdot 1} f(x)}{\partial x}
}
{Gateaux differential, form}

\DefEquation
{
\partial f(x)(a)=\lim_{t\rightarrow 0,\ t\in R}(t^{-1}(f(x+ta)-f(x)))
}
{Gateaux derivative, representation, 2}

\DefEquation
{
\partial f(x)(a)
=\ShowSymbol{standard component of Gateaux derivative}
\ e_{\gii}\ a\ e_{\gij}
}
{Gateaux derivative, division ring, standard representation}

\DefEq
{
\[
\frac{\partial_{s\cdot 0} f(x)}{\partial x}a
\frac{\partial_{s\cdot 1} f(x)}{\partial x}
=\frac{\partial_{s\cdot 0} f(x)}{\partial x}a
\frac{\partial_{s\cdot 1} f(x)}{\partial x}a^{-1}a
\]
\[
\frac{\partial_{s\cdot 0} f(x)}{\partial x}a
\frac{\partial_{s\cdot 1} f(x)}{\partial x}
=aa^{-1}\frac{\partial_{s\cdot 0} f(x)}{\partial x}a
\frac{\partial_{s\cdot 1} f(x)}{\partial x}
\]
}
{need extract derivative from differential}

\DefEquation
{
\partial f(x)(a)
=\frac{\partial_{s\cdot 0} f(x)}{\partial x}
a
\frac{\partial_{s\cdot 1} f(x)}{\partial x}
}
{Gateaux derivative of f, division ring}

\DefEquation
{
\partial g(x)(a)
=\frac{\partial_{t\cdot 0} g(x)}{\partial x}
a
\frac{\partial_{t\cdot 1} g(x)}{\partial x}
}
{Gateaux derivative of g, division ring}

\DefEq
{
\begin{align}
\EqLabel{0 component of Gateaux derivative, fg, division ring}
\frac{\partial_{s\cdot 0} f(x)g(x)}{\partial x}
&
=\frac{\partial_{s\cdot 0} f(x)}{\partial x}
&
\frac{\partial_{t\cdot 0} f(x)g(x)}{\partial x}
&
=f(x)\frac{\partial_{t\cdot 0} g(x)}{\partial x}
\\
\EqLabel{1 component of Gateaux derivative, fg, division ring}
\frac{\partial_{s\cdot 1} f(x)g(x)}{\partial x}
&
=\frac{\partial_{s\cdot 1} f(x)}{\partial x}
g(x)
&
\frac{\partial_{t\cdot 1} f(x)g(x)}{\partial x}
&
=\frac{\partial_{t\cdot 1} g(x)}{\partial x}
\end{align}
}
{component of Gateaux derivative, fg, division ring}

\DefEquation
{
\begin{split}
\partial (f(x) g(x))(a)
&=\partial f(x)(a)\ g(x)+f(x)\ \partial g(x)(a)
\\
&=\frac{\partial_{s\cdot 0} f(x)}{\partial x}a
\frac{\partial_{s\cdot 1} f(x)}{\partial x}
g(x)
+f(x)\frac{\partial_{t\cdot 0} g(x)}{\partial x}a
\frac{\partial_{t\cdot 1} g(x)}{\partial x}
\end{split}
}
{Gateaux derivative of fg, division ring}

\DefEq
{
\begin{align}
\EqLabel{Gateaux differential, product over constant, division ring}
\partial (bf(x)c)(a)
&=b\partial f(x)(a)c
\\
\EqLabel{0 component of Gateaux differential, product over constant, division ring}
\frac{\partial_{s\cdot 0} bf(x)c}{\partial x}
&=b\frac{\partial_{s\cdot 0} f(x)}{\partial x}
\\
\EqLabel{1 component of Gateaux differential, product over constant, division ring}
\frac{\partial_{s\cdot 1} bf(x)c}{\partial x}
&=\frac{\partial_{s\cdot 1} f(x)}{\partial x}c
\\
\EqLabel{Gateaux derivative, product over constant, division ring}
\frac{\partial bf(x)c}{\partial_* x}(a)
&=a^{-1}ba\frac{\partial f(x)(a)}{\partial_* x}c
\end{align}
}
{Gateaux differential, product over constant, division ring}

\DefEq
{
\begin{align}
\EqLabel{Gateaux differential, xb-bx, division ring}
\partial (xb-bx)(h)
&=hb-bh
\\
\nonumber
\frac{\partial_{1\cdot 0} (xb-bx)}{\partial x}
&=1
&
\frac{\partial_{1\cdot 1} (xb-bx)}{\partial x}
&=b
\\
\nonumber
\frac{\partial_{2\cdot 0} (xb-bx)}{\partial x}
&=-b
&
\frac{\partial_{2\cdot 1} (xb-bx)}{\partial x}
&=1
\\
\nonumber
\frac{\partial (xb-bx)}{\partial_* x}(h)
&=h^{-1}bhc
\end{align}
}
{Gateaux differential, xb-bx, division ring}

\DefEquation
{
 \begin{array}{rl}
\partial (x^2)(a)&=xa+ax
\\
\displaystyle\frac{\partial x^2}{\partial_*x}(a)
&=a^{-1}xa+x
\end{array}
}
{derivative x2, division ring}

\DefEq
{
\begin{align}
\partial (x^{-1})(h)&=-x^{-1}hx^{-1}
\EqLabel{derivative x power -1, division ring}
\\
\displaystyle\frac{\partial x^{-1}}{\partial_*x}(h)
&=-h^{-1}x^{-1}hx^{-1}
\nonumber
\end{align}
\[
 \begin{array}{ccc}
\displaystyle\frac{\partial_{1\cdot 0} x^{-1}}{\partial x}=-x^{-1}
&
\displaystyle\frac{\partial_{1\cdot 1} x^{-1}}{\partial x}=x^{-1}
\end{array}
\]
}
{derivative x power -1, division ring}

\DefEq
{
\begin{align}
\partial (xax^{-1})(h)&=hax^{-1}-xax^{-1}hx^{-1}
\EqLabel{derivative xax power -1, division ring}
\\
\displaystyle\frac{\partial xax^{-1}}{\partial_*x}(h)
&=ax^{-1}-h^{-1}xax^{-1}hx^{-1}
\nonumber
\end{align}
\[
 \begin{array}{lll}
\displaystyle\frac{\partial_{1\cdot 0} x^{-1}}{\partial x}=1
&
\displaystyle\frac{\partial_{1\cdot 1} x^{-1}}{\partial x}=ax^{-1}
\\
\displaystyle\frac{\partial_{2\cdot 0} x^{-1}}{\partial x}=-xax^{-1}
&
\displaystyle\frac{\partial_{2\cdot 1} x^{-1}}{\partial x}=x^{-1}
\end{array}
\]
}
{derivative xax power -1, division ring}

\DefEquation
{
 \begin{array}{ccc}
\displaystyle\frac{\partial_{1\cdot 0} x^2}{\partial x}=x
&
\displaystyle\frac{\partial_{1\cdot 1} x^2}{\partial x}=e
\\ \\
\displaystyle\frac{\partial_{2\cdot 0} x^2}{\partial x}=e
&
\displaystyle\frac{\partial_{2\cdot 1} x^2}{\partial x}=x
\end{array}
}
{derivative x2, component of Gateaux differential, division ring}

\DefEq
{
\begin{align}
\EqLabel{Gateaux differential, product over constant, fx=x, division ring}
\partial (bxc)(h)
&=bhc
\\
\EqLabel{0 component of Gateaux differential, product over constant, fx=x, division ring}
\frac{\partial_{1\cdot 0} bxc}{\partial x}
&=b
\\
\EqLabel{1 component of Gateaux differential, product over constant, fx=x, division ring}
\frac{\partial_{1\cdot 1} bxc}{\partial x}
&=c
\\
\EqLabel{Gateaux derivative, product over constant, fx=x, division ring}
\frac{\partial bxc}{\partial_* x}(h)
&=h^{-1}bhc
\end{align}
}
{Gateaux differential, product over constant, fx=x, division ring}

\DefEq
{
\[
\begin{array}{ccc}
a=a^{\gii}\ e_{\gii}&&a^{\gii}\in F
\end{array}
\]
}
{expansion a  in D}

\DefEq
{
\symb{\frac{\partial_{s\cdot p} f(x)}{\partial x}}0
{component of Gateaux derivative}
$\displaystyle\ShowSymbol{component of Gateaux derivative}$,
$p=0$, $1$,
}
{component of Gateaux derivative of map, division ring}

\DefEq
{
\symb{\partial f(x)}0{Gateaux derivative of map}
\symb{\frac{\partial f(x)}{\partial x}}
0{Gateaux derivative of map, fraction}
}
{Gateaux derivative of map, division ring, def}

\DefEquation
{
f(ph)=\lim_{n\rightarrow\infty}f(p_nh)=\lim_{n\rightarrow\infty}(p_nf(h))=pf(h)
}
{continuous linear map, real number, division ring, 1}

\DefEq
{
\[
\partial f:D\rightarrow \mathcal L(D;D)
\]
}
{differential L(D,D)}

\DefEq
{
\begin{align*}
\partial (x^{-1})(h)&=-hx^{-2}
\\
\frac{dx^{-1}}{dx}&=-x^{-2}
\end{align*}
}
{derivative x power -1, field}

\DefEq
{
\begin{align*}
\partial (x^2)(h)&=2hx
\\
\frac{dx^2}{dx}&=2x
\end{align*}
}
{derivative x2, field}



==> Differential.Russian.tex <==
%auto-ignore

\input{Differential.Eq}

\ifx\PrintBook\undefined
\else
\chapter{Дифференцируемые отображения}
\label{chapter: Differentiable maps}
\fi
\section{Топологическое тело}
\label{section: Topological Division Ring}

\begin{definition}
Тело $D$ называется 
\AddIndex{топологическим телом}{topological division ring}\footnote{Определение
дано согласно
определению из \citeBib{Pontryagin: Topological Group},
глава 4},
если $D$ является топологическим пространством, и алгебраические операции,
определённые в $D$, непрерывны в топологическом пространстве $D$.
\qed
\end{definition}

Согласно определению, для произвольных элементов $a, b\in D$
и для произвольных окрестностей $W_{a-b}$ элемента $a-b$,
$W_{ab}$ элемента $ab$ существуют такие окрестности $W_a$
элемента $a$ и $W_b$ элемента $b$, что $W_a-W_b\subset W_{a-b}$,
$W_aW_b\subset W_{ab}$. Если $a\ne 0$, то для произвольной
окрестности $W_{a^{-1}}$ существует окрестность $W_a$ элемента $a$,
удовлетворяющая условию $W_a^{-1}\subset W_{a^{-1}}$.

\begin{definition}
\label{definition: absolute value on division ring}
\AddIndex{Норма на теле}
{absolute value on division ring} $D$\footnote{Определение
дано согласно
определению из \citeBib{Bourbaki: General Topology: Chapter 5 - 10},
гл. IX, \S 3, п${}^\circ$2} - это отображение
\[d\in D\rightarrow |d|\in R\]
такое, что
\begin{itemize}
\item $|a|\ge 0$
\item $|a|=0$ равносильно $a=0$
\item $|ab|=|a|\ |b|$
\item $|a+b|\le|a|+|b|$
\end{itemize}

Тело $D$, наделённое структурой, определяемой заданием на
$D$ нормы, называется \AddIndex{нормированным телом}{valued division ring}.
\qed
\end{definition}

Инвариантное расстояние на аддитивной группе тела $D$
\[d(a,b)=|a-b|\]
определяет топологию метрического пространства,
согласующуюся со структурой тела в $D$.

\begin{definition}
\label{definition: limit of sequence, valued division ring}
Пусть $D$ - нормированное тело.
Элемент $a\in D$ называется 
\AddIndex{пределом последовательности}{limit of sequence}
\ShowEq{limit of sequence, valued division ring}
если для любого $\epsilon\in R$, $\epsilon>0$,
существует, зависящее от $\epsilon$, натуральное число $n_0$ такое,
что $|a_n-a|<\epsilon$ для любого $n>n_0$.
\qed
\end{definition}

\ePrints{0908.3307}%
\ifx\Semafor\ValueOff%
\begin{theorem}
\label{theorem: limit of sequence, valued division ring, product on scalar}
Пусть $D$ - нормированное тело характеристики $0$ и пусть $d\in D$.
Пусть $a\in D$ - предел последовательности $\{a_n\}$.
Тогда
\[
\lim_{n\rightarrow\infty}(a_nd)=ad
\]
\[
\lim_{n\rightarrow\infty}(da_n)=da
\]
\end{theorem}
\begin{proof}
Утверждение теоремы тривиально, однако я привожу доказательство
для полноты текста. 
Поскольку $a\in D$ - предел последовательности $\{a_n\}$,
то согласно определению \ref{definition: limit of sequence, valued division ring}
для заданного $\epsilon\in R$, $\epsilon>0$,
существует натуральное число $n_0$ такое,
что $|a_n-a|<\epsilon/|d|$ для любого $n>n_0$.
Согласно определению \ref{definition: absolute value on division ring}
утверждение теоремы следует из неравенств
\[
|a_nd-ad|=|(a_n-a)d|=|a_n-a||d|<\epsilon/|d||d|=\epsilon
\]
\[
|da_n-da|=|d(a_n-a)|=|d||a_n-a|<|d|\epsilon/|d|=\epsilon
\]
для любого $n>n_0$.
\end{proof}
\fi

\begin{definition}
Пусть $D$ - нормированное тело.
Последовательность $\{a_n\}$, $a_n\in D$ называется 
\AddIndex{фундаментальной}{fundamental sequence}
или \AddIndex{последовательностью Коши}{Cauchy sequence},
если для любого $\epsilon\in R$, $\epsilon>0$,
существует, зависящее от $ \epsilon$, натуральное число $n_0$ такое,
что $|a_p-a_q|<\epsilon$ для любых $p$, $q>n_0$.
\qed
\end{definition}

\begin{definition}
Нормированное тело $D$ называется 
\AddIndex{полным}{complete division ring}
если любая фундаментальная последовательность элементов
данного тела сходится, т. е.
имеет предел в этом теле.
\qed
\end{definition}

\ePrints{0908.3307}%
\ifx\Semafor\ValueOff%
До сих пор всё было хорошо. Кольцо целых чисел содержится в кольце
характеристики $0$. Поле рациональных чисел содержится в теле
характеристики $0$. Однако это не означает, что поле действительных
чисел содержится в полном теле $D$ характеристики $0$.
Например, мы можем определить норму на теле,
тождественно равную $1$. Эта норма определяет на нормированном
теле дискретную топологию и не представляет для нас интереса,
так как любая фундаментальная последовательность является
постоянным отображением.
\fi

В дальнейшем, говоря о нормированном теле характеристики $0$,
мы будем предполагать, что определён гомеоморфизм поля рациональных чисел $Q$
в тело $D$.

\begin{theorem}
\label{theorem: division ring contains real number}
Полное тело $D$ характеристики $0$
содержит в качестве подполя изоморфный образ поля $R$
действительных чисел.
Это поле обычно отождествляют с $R$.
\end{theorem}
\begin{proof}
Рассмотрим фундаментальную последовательность рациональных чисел $\{p_n\}$.
Пусть $p'$ - предел этой последовательности в теле $D$.
Пусть $p$ - предел этой последовательности в поле $R$.
Так как вложение поля $Q$ в тело $D$ гомеоморфно,
то мы можем отождествить $p'\in D$ и $p\in R$.
\end{proof}

\begin{theorem}
\label{theorem: division ring, real number}
Пусть $D$ - полное тело характеристики $0$ и пусть $d\in D$.
Тогда любое действительное число $p\in R$ коммутирует с $d$.
\end{theorem}
\begin{proof}
Мы можем представить действительное число $p\in R$ в
виде фундаментальной последовательности рациональных чисел $\{p_n\}$.
Утверждение теоремы следует из цепочки равенств
\[
pd=\lim_{n\rightarrow\infty}(p_nd)=\lim_{n\rightarrow\infty}(dp_n)=dp
\]
основанной на утверждении теоремы
\xRef{0812.4763}{theorem: limit of sequence, valued division ring, product on scalar}.
\end{proof}

\begin{theorem}
\label{theorem: real subring of center}
Пусть $D$ - полное тело характеристики $0$.
Тогда поле действительных чисел $R$ является подполем центра $Z(D)$ тела $D$.
\end{theorem}
\begin{proof}
Следствие теоремы \ref{theorem: division ring, real number}.
\end{proof}

\begin{definition}
Пусть $D$ - полное тело характеристики $0$.
Множество элементов $d\in D$, $|d|=1$, называется
\AddIndex{единичной сферой в теле}{unit sphere in division ring} $D$.
\qed
\end{definition}

\begin{definition}
\label{definition: continuous map, division ring}
Пусть $D_1$ - полное тело характеристики $0$ с нормой $|x|_1$.
Пусть $D_2$ - полное тело характеристики $0$ с нормой $|x|_2$.
Отображение \[f:D_1\rightarrow D_2\]
называется \AddIndex{непрерывной}{continuous map}, если
для любого сколь угодно малого $\epsilon>0$
существует такое $\delta>0$, что
\[
|x'-x|_1<\delta
\]
влечёт
\[
|f(x')-f(x)|_2<\epsilon
\]
\qed
\end{definition}

\begin{theorem}
\label{theorem: continuous map of division ring}
Пусть $D$ - полное тело характеристики $0$.
Если в разложении
\ePrints{0812.4763,0908.3307}
\ifx\Semafor\ValueOn
\EqRef{linear map, division ring, canonical morphism}
\else
\xEqRef{0701.238}{linear map, division ring, canonical morphism}
\fi
линейного отображения \[f:D\rightarrow D\]
индекс $s$ принимает конечное множество значений,
то линейное отображение $f$
непрерывно.
\end{theorem}
\begin{proof}
Положим $x'=x+a$. Тогда
\[
f(x')-f(x)=f(x+a)-f(x)=f(a)=\pC{s}{0}f\ a\ \pC{s}{1}f
\]
\[
|f(x')-f(x)|=|\pC{s}{0}f\ a\ \pC{s}{1}f|<(|\pC{s}{0}f|\ |\pC{s}{1}f|)|a|
\]
Положим $F=|\pC{s}{0}f|\ |\pC{s}{1}f|$. Тогда
\[
|f(x')-f(x)|<F|a|
\]
Выберем $\epsilon>0$ и положим $\displaystyle a=\frac{\epsilon}Fe$.
Тогда $\displaystyle\delta=|a|=\frac{\epsilon}F$.
Согласно определению \ref{definition: continuous map, division ring}
линейное отображение $f$ непрерывно.
\end{proof}

\ePrints{0908.3307}%
\ifx\Semafor\ValueOff%
Аналогично, если индекс $s$ принимает счётное множество значений,
то для непрерывности аддитивного отображения $f$ мы требуем, что бы ряд
$|\pC{s}{0}f|\ |\pC{s}{1}f|$ сходился.
Если индекс $s$ принимает непрерывное множество значений,
то для непрерывности аддитивного отображения $f$ мы требуем, что бы интеграл
$\int|\pC{s}{0}f|\ |\pC{s}{1}f|ds$ существовал.
\fi

\begin{definition}
\label{definition: norm of map, division ring}
Пусть
\[f:D_1\rightarrow D_2\]
отображение полного тела $D_1$ характеристики $0$ с нормой $|x|_1$
в полное тело $D_2$ характеристики $0$ с нормой $|y|_2$.
Величина
\ShowEq{norm of map}
\ShowEq{norm of map, division ring}
называется
\AddIndex{нормой отображения $f$}{norm of map}.
\qed
\end{definition}

\begin{theorem}
\label{theorem: continuity of linear map, finite norm, division ring}
Пусть
\[f:D_1\rightarrow D_2\]
линейное отображение полного тела $D_1$
в полное тело $D_2$.
Отображение $f$ непрерывно, если $\|f\|<\infty$.
\end{theorem}
\begin{proof}
Поскольку отображение $f$ аддитивно, то
согласно определению \ref{definition: norm of map, division ring}
\[
|f(x)-f(y)|_2=|f(x-y)|_2\le \|f\|\ |x-y|_1
\]
Возьмём произвольное $\epsilon>0$. Положим $\displaystyle\delta=\frac\epsilon{\|f\|}$.
Тогда из неравенства
\[
|x-y|_1<\delta
\]
следует
\[
|f(x)-f(y)|_2\le \|f\|\ \delta=\epsilon
\]
Согласно определению \ref{definition: continuous map, division ring}
отображение $f$ непрерывно.
\end{proof}

\begin{theorem}
\label{theorem: continuous linear map, real number, division ring}
Пусть отображение
\ShowEq{f d1 d2}
является непрерывным линейным отображением
тела $D_1$ характеристики $0$ в тело $D_2$ характеристики $0$.
Тогда
\[
f(ax)=af(x)
\]
для любого действительного числа $a$.
\end{theorem}
\begin{proof}
Согласно теореме
\ref{theorem: real subring of center},
поле действительных чисел является подполем центра $Z(D)$ тела $D$.
Мы можем представить действительное число $p\in R$ в
виде фундаментальной последовательности рациональных чисел $\{p_n\}$.
Утверждение теоремы
следует из теорем
\ref{theorem: linear map, division ring, rational},
\xRef{0812.4763}{theorem: limit of sequence, valued division ring, product on scalar}
и цепочки равенств
\ShowEq{continuous linear map, real number, division ring, 1}
\end{proof}

\ifx\texFuture\Defined
\begin{theorem}
\label{theorem: continuity of map, norm, division ring}
Пусть
\[f:D_1\rightarrow D_2\]
отображение полного тела $D_1$
в полное тело $D_2$.
Отображение $f$ непрерывно, если $\|f\|<\infty$.
\end{theorem}
\begin{proof}
Поскольку отображение $f$ аддитивно, то
согласно определению \ref{definition: norm of map, division ring}
\[
|f(x)-f(y)|_2=|f(x-y)|_2\le \|f\|\ |x-y|_1
\]
Возьмём произвольное $\epsilon>0$. Положим $\displaystyle\delta=\frac\epsilon{\|f\|}$.
Тогда из неравенства
\[
|x-y|_1<\delta
\]
следует
\[
|f(x)-f(y)|_2\le \|f\|\ \delta=\epsilon
\]
Согласно определению \ref{definition: continuous map, division ring}
отображение $f$ непрерывно.
\end{proof}
\fi

\ePrints{0812.4763}
\ifx\Semafor\ValueOn

\begin{theorem}
\label{theorem: projective map in 0, division ring}
Пусть $D$ - полное тело характеристики $0$.
Либо непрерывное отображение $f$ тела, проективное над полем $P$,
не зависит от направления над полем $P$,
либо значение $f(0)$ не определено.
\end{theorem}
\begin{proof}
Согласно определению
\ref{definition: map projective over commutative ring, ring},
отображение $f$
постоянно на направлении $Pa$. Так как $0\in Pa$,
то естественно положить по непрерывности
\[
f(0)=f(a)
\]
Однако это приводит к неопределённости значения
отображения $f$ в направлении $0$,
если отображение $f$ имеет разное значение для разных направлений $a$.
\end{proof}

Если проективное над полем $R$ отображение $f$ непрерывно,
то мы будем говорить, что
\AddIndex{отображение $f$ непрерывно по направлению над полем}
{projective map is continuous in direction over field} $R$.
Поскольку для любого $a\in D$, $a\ne 0$ мы можем выбрать
$a_1=|a|^{-1}a$, $f(a_1)=f(a)$, то мы можем сделать определение более точным.

\begin{definition}
\label{definition: projective function is continuous in direction over field R, division ring}
Пусть $D$ - полное тело характеристики $0$.
Проективная над полем $R$ функция $f$ непрерывна
по направлению над полем $R$, если
для любого сколь угодно малого $\epsilon>0$
существует такое $\delta>0$, что
\[
|x'-x|_1<\delta\ \ \ |x'|_1=|x|_1=1
\]
влечёт
\[
|f(x')-f(x)|_2<\epsilon
\]
\qed
\end{definition}

\begin{theorem}
\label{theorem: projective function is continuous in direction over field R, division ring}
Пусть $D$ - полное тело характеристики $0$.
Проективная над полем $R$ функция $f$ непрерывна
по направлению над полем $R$ тогда и только тогда, когда
эта функция непрерывна на единичной сфере тела $D$.
\end{theorem}
\begin{proof}
Следствие определений \ref{definition: continuous map, division ring},
\ref{definition: map projective over commutative ring, ring},
\ref{definition: projective function is continuous in direction over field R, division ring}.
\end{proof}
\fi

\section{Дифференцируемое отображение тела}
\label{section: Differentiable maps of Division Ring}

\ePrints{0812.4763}
\ifx\Semafor\ValueOn
\begin{definition}
\label{definition: differentiable functions, division ring}
Пусть $D$ - нормированное тело.\footnote{Определение
дано согласно
определению \citeBib{Lebedev Vorovich}-3.1.1,
стр. 256.}
Функция \[f:D\rightarrow D\] называется
\AddIndex{\Ds дифференцируемой по Фреше}
{function Dstar differentiable in Frechet sense, division ring}
на множестве $U\subset D$\footnote{Так же как в замечании
\xRef{0701.238}{remark: drc linear map}
мы можем определить \Ds дифференцируемость отображения \[f:S\rightarrow D\]
нормированного тела $S$
в нормированное тело $D$ согласно правилу
\[
f(x+h)-f(x)
=F(h)\frac{d f(x)}{d_*x}
+o(h)
\]
где \[F:S\rightarrow D\] гомоморфизм тел.
Однако, опираясь на теоремы об изоморфизмах, мы можем ограничиться случаем
отображений тела $D$ в $D$.},
если в каждой точке $x\in U$ изменение функции $f$ может быть представлено в виде
\symb{\frac{d f(x)}{d_*x}}0{Frechet Dstar derivative of map, division ring}
\begin{equation}
\EqLabel{Dstar derivative, division ring}
f(x+h)-f(x)
=h\ShowSymbol{Frechet Dstar derivative of map, division ring}
+o(h)
\end{equation}
где $o$ - такое непрерывное отображение
\[o:D\rightarrow D\]
что
\begin{equation}
\EqLabel{infinitesimal, division ring}
\lim_{h\rightarrow 0}\frac{|o(h)|}{|h|}=0
\end{equation}
\qed
\end{definition}

Согласно определению \ref{definition: differentiable functions, division ring},
\AddIndex{\Ds производная Фреше отображения $f$ в точке $x$}
{Frechet Dstar derivative of map, division ring}
\[
\ShowSymbol{Frechet Dstar derivative of map, division ring}\in {}_*\mathcal L(D,D)
\]
порождает гомоморфизм
\[
\Delta f
=\Delta x\frac{d f(x)}{d_*x}
\]
отображающий приращение аргумента в приращение функции.

Если мы умножим обе части равенства
\EqRef{Dstar derivative, division ring}
на $h^{-1}$, то мы получим равенство
\begin{equation}
\EqLabel{Dstar derivative, division ring, 1}
h^{-1}(f(x+h)-f(x))
=\frac{d f(x)}{d_*x}
+h^{-1}o(h)
\end{equation}
Из равенств \EqRef{Dstar derivative, division ring, 1} и
\EqRef{infinitesimal, division ring} следует
альтернативное определение \Ds производной Фреше
\begin{equation}
\EqLabel{Dstar derivative, division ring, 2}
\frac{d f(x)}{d_*x}
=\lim_{h\rightarrow 0}(h^{-1}(f(x+h)-f(x)))
\end{equation}

Отличие \Ds производной Фреше отображения тела $D$ от производной отображения
поля $F$ состоит в том, что прежде всего \Ds производная Фреше не является
линейным отображением. Более точно, \Ds производная Фреше является \sD
линейным отображением, однако, вообще говоря, не является \Ds
линейным отображением. Действительно,
\[
f(x+h)a-f(x)a=h\frac{df}{d_*x}a+o(h)
\]
\begin{equation}
\EqLabel{Dstar derivative, division ring, 3}
af(x+h)-af(x)=ah\frac{df}{d_*x}+o(h)
\end{equation}
Однако, вообще говоря,
\[
ah\frac{df}{d_*x}\ne ha\frac{df}{d_*x}
\]

Подобная проблема возникает при дифференцировании произведения функций.
Согласно определению \ref{definition: differentiable functions, division ring}
\begin{equation}
f(x+h)g(x+h)-f(x)g(x)
=h\frac{df(x)g(x)}{d_*x}+o(h)
\EqLabel{product of maps, derivative, 0}
\end{equation}
Выражение в левой части можно представить в виде
\begin{align}
&f(x+h)g(x+h)-f(x)g(x)\nonumber\\
\EqLabel{product of maps, derivative, 1}
=&f(x+h)g(x+h)-f(x)g(x+h)+f(x)g(x+h)-f(x)g(x)\\
=&(f(x+h)-f(x))g(x+h)+f(x)(g(x+h)-g(x))\nonumber
\end{align}
Согласно определению \ref{definition: differentiable functions, division ring},
мы можем представить \EqRef{product of maps, derivative, 1} в виде
\begin{align}
&f(x+h)g(x+h)-f(x)g(x)\nonumber\\
\EqLabel{product of maps, derivative, 2}
=&\left(h\frac{df(x)}{d_*x}+o(h)\right)
\left(g(x)+h\frac{dg(x)}{d_*x}+o(h)\right)\\
+&f(x)\left(h\frac{dg(x)}{d_*x}+o(h)\right)\nonumber
\end{align}
Так как, вообще говоря,
\[
f(x)h\frac{dg}{d_*x}\ne hf(x)\frac{dg}{d_*x}
\]
то естественно ожидать, что функция $f(x)g(x)$
не является \Ds дифференцируемой по Фреше.

Таким образом, определение \Ds производной Фреше весьма ограничено
и не удовлетворяет стандартному определению операции дифференцирования.
Чтобы найти решение проблемы дифференцирования,
рассмотрим эту проблему с другой стороны.
\fi

\begin{example}
\label{example: differential dxx}
Рассмотрим приращение функции $f(x)=x^2$.
\begin{align*}
f(x+h)-f(x)
&=(x+h)^2-x^2
\\
&=xh+hx+h^2
\\
&=xh+hx+o(h)
\end{align*}
Как мы видим компонента приращения функции $f(x)=x^2$, линейно зависящая
от приращения аргумента, имеет вид
\[
xh+hx
\]
Так как произведение некомутативно,
то мы не можем представить приращение функции $f(x+h)-f(x)$
в виде $Ah$ или $hA$,
где $A$ не зависит от $h$.
Следствием этого является непредсказуемость поведения приращения функции $f(x)=x^2$,
когда приращение аргумента стремится к $0$.
Однако, если бесконечно малая величина $h$ будет бесконечно малой величиной
вида $h=ta$, $a\in D$, $t\in R$, $t\rightarrow 0$, то ответ становится
более определённым
\[
(xa+ax)t
\]
\qed
\end{example}

\begin{definition}
\label{definition: map differentiable in Gateaux sense, division ring}
Пусть $D$ - полное тело характеристики $0$.\footnote{Определение
дано согласно
определению \citeBib{Lebedev Vorovich}-3.1.2,
стр. 256.}
Отображение \[f:D\rightarrow D\]
\AddIndex{дифференцируемо по Гато}
{map differentiable in Gateaux sense} на множестве $U\subset D$,
если в каждой точке $x\in U$
изменение функции $f$ может быть представлено в виде
\ShowEq{Gateaux derivative of map, division ring, def}
\ShowEq{Gateaux differential of map, division ring}
где
\AddIndex{производная Гато
$\ShowSymbol{Gateaux derivative of map}$
отображения $f$}
{Gateaux derivative of map}
- линейное отображение приращения $a$ и
$o:D\rightarrow D$ - такое непрерывное отображение, что
\[
\lim_{a\rightarrow 0}\frac{|o(a)|}{|a|}=0
\]
\qed
\end{definition}

\begin{remark}
\label{remark: differential L(D,D)}
Согласно определению
\ref{definition: map differentiable in Gateaux sense, division ring}
при заданном $x$ производная Гато $\partial f(x)\in\mathcal L(D;D)$.
Следовательно, производная Гато отображения $f$ является отображением
\ShowEq{differential L(D,D)}
Выражения $\partial f(x)$ и $\displaystyle\frac{\partial f(x)}{\partial x}$
являются разными обозначениями одной и той же функции.
Мы будем пользоваться обозначением $\displaystyle\frac{\partial f(x)}{\partial x}$,
если хотим подчеркнуть, что мы берём производную Гато по переменной $x$.
\qed
\end{remark}

\begin{theorem}
\label{theorem: map differentiable in Gateaux sense, division ring}
Мы можем представить производную Гато
отображения $f$ в виде
\ShowEq{Gateaux derivative, representation}
\end{theorem}
\begin{proof}
Следствие определения
\ref{definition: map differentiable in Gateaux sense, division ring}
и теоремы
\ePrints{0812.4763,0908.3307}
\ifx\Semafor\ValueOn
\ref{theorem: linear map, division ring, canonical morphism}.
\else
\xRef{0701.238}{theorem: linear map, division ring, canonical morphism}.
\fi
\end{proof}

\begin{definition}
Выражение
\ShowEq{component of Gateaux derivative of map, division ring}
называется
\AddIndex{компонентой производной Гато отображения $f(x)$}
{component of Gateaux derivative of map, division ring}.
\qed
\end{definition}

\begin{theorem}
\label{theorem: Gateaux derivative is linear over field R, division ring}
Пусть $D$ - тело характеристики $0$.
Пусть функция \[f:D\rightarrow D\]
дифференцируема по Гато.
Тогда
\ShowEq{Gateaux derivative is linear over field R, division ring}
для любого действительного числа $a$.
\end{theorem}
\begin{proof}
Следствие теоремы
\ref{theorem: continuous linear map, real number, division ring} и
определения
\ref{definition: map differentiable in Gateaux sense, division ring}.
\end{proof}

Комбинируя равенство
\EqRef{Gateaux derivative is linear over field R, division ring}
и определение
\ref{definition: map differentiable in Gateaux sense, division ring},
мы получим знакомое определение производной
Гато
\ShowEq{Gateaux derivative, representation, 2}
Определения производной Гато \EqRef{Gateaux differential of map, division ring}
и \EqRef{Gateaux derivative, representation, 2}
эквивалентны. На основе этой эквивалентности мы будем говорить,
что отображение $f$
дифференцируемо по Гато на множестве $U\subset D$,
если в каждой точке $x\in U$
изменение функции $f$ может быть представлено в виде
\begin{equation}
\EqLabel{Gateaux differential of map, t, division ring}
f(x+ta)-f(x)
=t\partial f(x)(a)
+o(t)
\end{equation}
где
$o:R\rightarrow D$ - такое непрерывное отображение, что
\[
\lim_{t\rightarrow 0}\frac{|o(t)|}{|t|}=0
\]

Если бесконечно малая $a$ в равенстве
\EqRef{Gateaux derivative, representation}
является дифференциалом $dx$,
то равенство
\EqRef{Gateaux derivative, representation}
становится определением
\AddIndex{дифференциала Гато}{Gateaux differential of map}
\ShowEq{Gateaux differential, division ring}
\ShowEq{Gateaux differential, form}

\begin{theorem}
\label{theorem: Gateaux derivative, standard form, division ring}
Пусть $D$ - тело характеристики $0$.
Пусть $\Basis e$ - базис тела $D$ над центром $Z(D)$ тела $D$.
\symb{\StandPartial{f(x)}{x}{ij}}0
{standard component of Gateaux derivative}
\AddIndex{Стандартное представление производной Гато}
{Gateaux derivative, standard representation}
\EqRef{Gateaux derivative, representation}
отображения\[f:D\rightarrow D\]
имеет вид
\ShowEq{Gateaux derivative, division ring, standard representation}
Выражение
$\displaystyle\ShowSymbol{standard component of Gateaux derivative}$
в равенстве \EqRef{Gateaux derivative, division ring, standard representation}
называется \AddIndex{стандартной компонентой производной Гато}
{standard component of Gateaux derivative} отображения $f$.
\end{theorem}
\begin{proof}
Утверждение теоремы является следствием теоремы
\ePrints{0812.4763,0908.3307}
\ifx\Semafor\ValueOn
\ref{theorem: linear map, standard form, division ring}.
\else
\xRef{0701.238}{theorem: linear map, standard form, division ring}.
\fi
\end{proof}

\begin{theorem}
Пусть $D$ - тело характеристики $0$.
Пусть $\Basis e$ - базис тела $D$
над полем $F\subset Z(D)$.
Тогда дифференциал Гато отображения
\[
f:D\rightarrow D
\]
можно записать в виде
\ShowEq{Gateaux derivative and Jacobian, division ring}
где $a\in D$ имеет разложение
\ShowEq{expansion a  in D}
относительно базиса $\Basis e$ и матрица Якоби отображения $f$ имеет вид
\begin{equation}
\EqLabel{standard components and jacobian, division ring}
\frac{\partial f^{\gij}}{\partial x^{\gii}}=
\StandPartial{f(x)}{x}{kr}\ C^{\gi p}_{\gi{ki}}\ C^{\gij}_{\gi{pr}}
\end{equation}
\end{theorem}
\begin{proof}
Утверждение теоремы является следствием теоремы
\ePrints{0812.4763,0908.3307}
\ifx\Semafor\ValueOn
\ref{theorem: linear map over field, division ring}.
\else
\xRef{0701.238}{theorem: linear map over field, division ring}.
\fi
\end{proof}

\ePrints{0908.3307}%
\ifx\Semafor\ValueOff%
Чтобы найти конструкцию, подобную производной в коммутативном случае,
мы должны выделить производную из дифференциала
отображения. Для этого мы должны вынести приращение аргумента за
скобки.\footnote{Это возможно в том случае, если все
$\displaystyle \frac{\pC{s}{0}\partial f(x)}{\partial x}=e$
либо все
$\displaystyle \frac{\pC{s}{1}\partial f(x)}{\partial x}=e$.
Поэтому определение \citeBib{Lebedev Vorovich}-3.1.2,
стр. 256, приводит нас либо к определению
\Ds производной Фреше,
либо к определению
\sD производной Фреше.}
Мы можем вынести $a$ за скобки,
опираясь на равенства
\ShowEq{need extract derivative from differential}
\fi

\begin{definition}
\label{definition: Gateaux Dstar derivative, division ring}
Пусть $D$ - полное тело характеристики $0$
и $a\in D$.
\symb{\frac{\partial f(x)(a)}{\partial_* x}}
0{Gateaux Dstar derivative of map, division ring}
\AddIndex{\Ds производная Гато
$\displaystyle\ShowSymbol{Gateaux Dstar derivative of map, division ring}$
отображения $f:D\rightarrow D$}
{Gateaux Dstar derivative of map, division ring}
определена равенством
\begin{equation}
\EqLabel{Gateaux Dstar derivative, division ring}
\partial f(x)(a)
=a\ShowSymbol{Gateaux Dstar derivative of map, division ring}
\end{equation}
\symb{\frac{\partial f(x)(a)}{{}_*\partial x}}
0{Gateaux starD derivative of map, division ring}
\AddIndex{\sD производная Гато
$\displaystyle\ShowSymbol{Gateaux starD derivative of map, division ring}$
отображения $f:D\rightarrow D$}
{Gateaux starD derivative of map, division ring}
определена равенством
\begin{equation}
\EqLabel{Gateaux starD derivative, division ring}
\partial f(x)(a)
=\ShowSymbol{Gateaux starD derivative of map, division ring}a
\end{equation}
\qed
\end{definition}

\ePrints{0908.3307}%
\ifx\Semafor\ValueOff%
Для представления \Ds производной Гато
мы также будем пользоваться записью
\[
\frac{\partial f(x)(a)}{\partial_* x}=\frac{\partial}{\partial_* x} f(x)(a)=\partial_* f(x)(a)
\]

Для представления \sD производной Гато
мы также будем пользоваться записью
\[
\frac{\partial f(x)(a)}{{}_*\partial x}=\frac{\partial}{{}_*\partial x} f(x)(a)={}_*\partial f(x)(a)
\]

Опираясь на принцип двойственности
\xRef{0701.238}{theorem: duality principle, vector space},
мы будем изучать \Ds производную, имея в виду, что двойственное утверждение
справедливо для \sD производной.

Поскольку произведение не коммутативно, понятие дроби не определено в теле.
Мы должны явно указать, с какой стороны знаменатель действует на числитель.
Эту функцию выполняет символ $*$ в знаменателе дроби.
Согласно определению
\[
\frac{\partial f}{\partial_* x}=(\partial_* x)^{-1}\partial f
\]
\[
\frac{\partial f}{{}_*\partial x}=\partial f({}_*\partial x)^{-1}
\]
Таким образом, мы можем представить
\Ds производную Гато функции $f$
как отношение изменения функции к изменению аргумента.
Это замечание не распространяется на
компоненты дифференциала Гато.
В этом случае мы рассматриваем запись
$\displaystyle\frac{\partial}{\partial_* x}$
и $\displaystyle\frac{\partial}{{}_*\partial x}$ не
как дроби, а как символы операторов.

При этом равенство \EqRef{Gateaux Dstar derivative, division ring}
можно записать в виде
\begin{equation}
\EqLabel{Gateaux differential, division ring, 1}
\partial f(x)(dx)
=dx(\partial_* x)^{-1}\partial f(x)(dx)
\end{equation}
Нетрудно видеть, что в знаменателе дроби в равенстве
\EqRef{Gateaux differential, division ring, 1}
мы записали \Ds дифференциал переменной $x$, а умножаем дробь на
дифференциал переменной $x$.
\fi

\begin{theorem}
\label{theorem: Dstar derivative is multiplicative over field R, division ring}
Пусть $D$ - полное тело характеристики $0$.
\Ds производная Гато проективна
над полем действительных чисел $R$.
\end{theorem}
\begin{proof}
Следствие теоремы
\ref{theorem: Gateaux derivative is linear over field R, division ring}
и примера
\ePrints{0812.4763,0908.3307}
\ifx\Semafor\ValueOn
\ref{example: map projective over commutative ring, ring}.
\else
\xRef{0701.238}{example: map projective over commutative ring, ring}.
\fi
\end{proof}

Из теоремы \ref{theorem: Dstar derivative is multiplicative over field R, division ring}
следует
\begin{equation}
\EqLabel{Dstar derivative is multiplicative over field R, division ring}
\frac{\partial f(x)(ra)}{\partial_* x}
=\frac{\partial f(x)(a)}{\partial_* x}
\end{equation}
для любых $r\in R$, $r\ne 0$ и  $a\in D$, $a\ne 0$.
Следовательно, \Ds производная Гато
хорошо определена в направлении $a$ над полем $R$, $a\in D$, $a\ne 0$, 
и не зависит от выбора значения в этом направлении.

\begin{theorem}
Пусть $D$ - полное тело характеристики $0$
и $a\ne 0$.
\Ds производная Гато и \sD производная Гато отображения $f$ тела $D$
связаны соотношением
\begin{equation}
\EqLabel{Dstar derivative and starD derivative in direction, division ring}
\frac{\partial f(x)(a)}{{}_*\partial x} 
=a\frac{\partial f(x)(a)}{\partial_* x} a^{-1}
\end{equation}
\end{theorem}
\begin{proof}
Из равенств \EqRef{Gateaux Dstar derivative, division ring}
и \EqRef{Gateaux starD derivative, division ring}
следует
\[
\frac{\partial f(x)(a)}{{}_*\partial x}
=\partial f(x)(a)a^{-1}
=a\frac{\partial f(x)(a)}{\partial_* x}a^{-1}
\]
\end{proof}

\begin{theorem}
Пусть $D$ - полное тело характеристики $0$.
Производная Гато удовлетворяет соотношению
\begin{equation}
\EqLabel{Gateaux derivative of product, division ring}
\partial (f(x)g(x))(a)
=\partial f(x)(a)\ g(x)+f(x)\ \partial g(x)(a)
\end{equation}
\end{theorem}
\begin{proof}
Равенство \EqRef{Gateaux derivative of product, division ring}
следует из цепочки равенств
\begin{align*}
\partial (f(x)g(x))(a)
&=\lim_{t\rightarrow 0}(t^{-1}(f(x+ta)g(x+ta)-f(x)g(x)))
\\
&=\lim_{t\rightarrow 0}(t^{-1}(f(x+ta)g(x+ta)-f(x)g(x+ta)))
\\
&+\lim_{t\rightarrow 0}(t^{-1}(f(x)g(x+ta)-f(x)g(x)))
\\
&=\lim_{t\rightarrow 0}(t^{-1}(f(x+ta)-f(x)))g(x)
\\
&+f(x)\lim_{t\rightarrow 0}(t^{-1}(g(x+ta)-g(x)))
\end{align*}
основанной на определении \EqRef{Gateaux derivative, representation, 2}.
\end{proof}

\begin{theorem}
Пусть $D$ - полное тело характеристики $0$.
Допустим производная Гато
отображения $f:D\rightarrow D$
имеет разложение
\ShowEq{Gateaux derivative of f, division ring}
Допустим проиводная Гато
отображения $g:D\rightarrow D$
имеет разложение
\ShowEq{Gateaux derivative of g, division ring}
Компоненты производной Гато отображения $f(x)g(x)$
имеют вид
\ShowEq{component of Gateaux derivative, fg, division ring}
\end{theorem}
\begin{proof}
Подставим \EqRef{Gateaux derivative of f, division ring}
и \EqRef{Gateaux derivative of g, division ring}
в равенство \EqRef{Gateaux derivative of product, division ring}
\ShowEq{Gateaux derivative of fg, division ring}
Опираясь на \EqRef{Gateaux derivative of fg, division ring},
мы определяем равенства
\EqRef{0 component of Gateaux derivative, fg, division ring},
\EqRef{1 component of Gateaux derivative, fg, division ring}.
\end{proof}

\begin{theorem}
Пусть $D$ - полное тело характеристики $0$.
\Ds производная Гато удовлетворяет соотношению
\begin{equation}
\EqLabel{Gateaux Dstar derivative of product, division ring}
\frac{\partial f(x)g(x)}{\partial_* x}(a)
=\frac{\partial f(x)(a)}{\partial_* x}g(x)+a^{-1}f(x)a\frac{\partial g(x)(a)}{\partial_* x}
\end{equation}
\end{theorem}
\begin{proof}
Равенство \EqRef{Gateaux Dstar derivative of product, division ring}
следует из цепочки равенств
\begin{align*}
\frac{\partial f(x)g(x)}{\partial_* x}(a)
&=a^{-1}\partial f(x)g(x)(a)
\\
&=a^{-1}(\partial f(x)(a)g(x)+f(x)\partial g(x)(a))
\\
&=a^{-1}\partial f(x)(a)g(x)+a^{-1}f(x)aa^{-1}\partial g(x)(a)
\\
&=\frac{\partial f(x)(a)}{\partial_* x}g(x)+a^{-1}f(x)a\frac{\partial g(x)(a)}{\partial_* x}
\end{align*}
\end{proof}

\begin{theorem}
Пусть $D$ - полное тело характеристики $0$.
Либо \Ds производная Гато не зависит от направления,
либо \Ds производная Гато в направлении $0$ не определена.
\end{theorem}
\begin{proof}
Утверждение теоремы является следствием
теоремы \ref{theorem: Dstar derivative is multiplicative over field R, division ring}
и теоремы \ref{theorem: projective map in 0, division ring}.
\end{proof}

\begin{theorem}
\label{theorem: norm of Gateaux differential, division ring}
Пусть $D$ - полное тело характеристики $0$.
Пусть единичная сфера тела $D$ - компактна.
Если \Ds производная Гато
$\displaystyle\frac{\partial f(x)(a)}{\partial_* x}$
существует в точке $x$ и непрерывна по направлению над полем $R$,
то существует норма $\|\partial f(x)\|$ дифференциала Гато.
\end{theorem}
\begin{proof}
Из определения \ref{definition: Gateaux Dstar derivative, division ring}
следует
\begin{equation}
\EqLabel{norm of Gateaux differential, division ring, 1}
|\partial f(x)(a)|
=|a|\ \left|\frac{\partial f(x)(a)}{\partial_* x}\right|
\end{equation}
Из теорем
\xRef{0812.4763}{theorem: projective function is continuous in direction over field R, division ring},
\ref{theorem: Dstar derivative is multiplicative over field R, division ring}
следует, что \Ds производная Гато непрерывна
на единичной сфере.
Так как единичная сфера компактна, то множество значений
\Ds производной Гато функции $f$ в точке $x$ ограниченно
\[
\left|
\frac{\partial f(x)(a)}{\partial_* x}
\right|
<F=\text{sup}\left|
\frac{\partial f(x)(a)}{\partial_* x}
\right|
\]
Согласно определению \ref{definition: norm of map, division ring}
\[
\|\partial f(x)\|=F
\]
\end{proof}

\begin{theorem}
\label{theorem: Dstar derivative and continuos function, division ring}
Пусть $D$ - полное тело характеристики $0$.
Пусть единичная сфера тела $D$ - компактна.
Если \Ds производная Гато
$\displaystyle\frac{\partial f(x)(a)}{\partial_* x}$
существует в точке $x$ и непрерывна по направлению над полем $R$,
то отображение $f$ непрерывно в точке $x$.
\end{theorem}
\begin{proof}
Из теоремы \ref{theorem: norm of Gateaux differential, division ring}
следует
\begin{equation}
\EqLabel{Dstar derivative and continuos function, division ring, 1}
|\partial f(x)(a)|
\le\|\partial f(x)\| |a|
\end{equation}
Из \EqRef{Gateaux differential of map, division ring},
\EqRef{Dstar derivative and continuos function, division ring, 1}
следует
\begin{equation}
\EqLabel{Dstar derivative and continuos function, division ring, 2}
|f(x+a)-f(x)|<|a|\ \|\partial f(x)\|
\end{equation}
Возьмём произвольное $\epsilon>0$. Положим
\[\delta=\frac\epsilon{\|\partial f(x)\|}\]
Тогда из неравенства
\[
|a|<\delta
\]
следует
\[
|f(x+a)-f(x)|\le \|\partial f(x)\|\ \delta=\epsilon
\]
Согласно определению \ref{definition: continuous map, division ring}
отображение $f$ непрерывно в точке $x$.
\end{proof}

\ePrints{0908.3307}%
\ifx\Semafor\ValueOff%
Теорема \ref{theorem: Dstar derivative and continuos function, division ring}
имеет интересное обобщение. Если единичная сфера тела $D$ не является компактной,
то мы можем рассмотреть компактное множество направлений вместо единичной сферы.
В этом случае, мы можем говорить о непрерывности функции $f$ вдоль заданного множества
направлений.
\fi

\section{Таблица производных Гато отображения тела}

\begin{theorem}
\label{theorem: Gateaux differential of const, division ring}
Пусть $D$ - полное тело характеристики $0$.
Тогда для любого $b\in D$
\begin{equation}
\EqLabel{Gateaux differential of const, division ring}
\partial (b)(a)
=0
\end{equation}
\end{theorem}
\begin{proof}
Непосредственное следствие определения
\ref{definition: map differentiable in Gateaux sense, division ring}.
\end{proof}

\begin{theorem}
\label{theorem: Gateaux differential, product over constant, division ring}
Пусть $D$ - полное тело характеристики $0$.
Тогда для любых $b$, $c\in D$
\ShowEq{Gateaux differential, product over constant, division ring}
\end{theorem}
\begin{proof}
Непосредственное следствие равенств
\EqRef{Gateaux derivative of product, division ring},
\EqRef{0 component of Gateaux derivative, fg, division ring},
\EqRef{1 component of Gateaux derivative, fg, division ring},
\EqRef{Gateaux Dstar derivative of product, division ring},
так как $\partial b=\partial c=0$.
\end{proof}

\begin{theorem}
\label{theorem: Gateaux differential, product over constant, fx=x, division ring}
Пусть $D$ - полное тело характеристики $0$.
Тогда для любых $b$, $c\in D$
\ShowEq{Gateaux differential, product over constant, fx=x, division ring}
\end{theorem}
\begin{proof}
Следствие теоремы
\ref{theorem: Gateaux differential, product over constant, division ring},
когда $f(x)=x$.
\end{proof}

\begin{theorem}
%\label{theorem: Gateaux differential, product over constant, fx=x, division ring}
Пусть $D$ - полное тело характеристики $0$.
Тогда для любого $b\in D$
\ShowEq{Gateaux differential, xb-bx, division ring}
\end{theorem}
\begin{proof}
Следствие теоремы
\ref{theorem: Gateaux differential, product over constant, division ring},
когда $f(x)=x$.
\end{proof}

\begin{theorem}
Пусть $D$ - полное тело характеристики $0$.
Тогда\footnote{Утверждение теоремы аналогично примеру VIII,
\citeBib{Hamilton Elements of Quaternions 1}, с. 451.
Если произведение коммутативно, то равенство
\EqRef{derivative x2, division ring}
принимает вид
\ShowEq{derivative x2, field}}
\ShowEq{derivative x2, division ring}
\ShowEq{derivative x2, component of Gateaux differential, division ring}
\end{theorem}
\begin{proof}
\EqRef{derivative x2, division ring} следует из примера \ref{example: differential dxx}
и определения \ref{definition: Gateaux Dstar derivative, division ring}.
\EqRef{derivative x2, component of Gateaux differential, division ring}
следует из примера \ref{example: differential dxx}
и равенства \EqRef{Gateaux differential, form}.
\end{proof}

\begin{theorem}
Пусть $D$ - полное тело характеристики $0$.
Тогда\footnote{Утверждение теоремы аналогично примеру IX,
\citeBib{Hamilton Elements of Quaternions 1}, с. 451.
Если произведение коммутативно, то равенство
\EqRef{derivative x power -1, division ring}
принимает вид
\ShowEq{derivative x power -1, field}}
\ShowEq{derivative x power -1, division ring}
\end{theorem}
\begin{proof}
Подставим $f(x)=x^{-1}$ в определение
\EqRef{Gateaux derivative, representation, 2}.
\begin{align}
\partial f(x)(h)
&=\lim_{t\rightarrow 0,\ t\in R}(t^{-1}((x+th)^{-1}-x^{-1}))
\nonumber
\\
&=\lim_{t\rightarrow 0,\ t\in R}(t^{-1}((x+th)^{-1}-x^{-1}(x+th)(x+th)^{-1}))
\nonumber
\\
&=\lim_{t\rightarrow 0,\ t\in R}(t^{-1}(1-x^{-1}(x+th))(x+th)^{-1})
\EqLabel{derivative x power -1, division ring, 1}
\\
&=\lim_{t\rightarrow 0,\ t\in R}(t^{-1}(1-1-x^{-1}th)(x+th)^{-1})
\nonumber
\\
&=\lim_{t\rightarrow 0,\ t\in R}(-x^{-1}h(x+th)^{-1})
\nonumber
\end{align}
Равенство \EqRef{derivative x power -1, division ring}
следует из цепочки равенств
\EqRef{derivative x power -1, division ring, 1}.
\end{proof}

\begin{theorem}
Пусть $D$ - полное тело характеристики $0$.
Тогда\footnote{Если произведение коммутативно, то
\[
y=xax^{-1}=a
\]
Соответственно производная обращается в $0$.}
\ShowEq{derivative xax power -1, division ring}
\end{theorem}
\begin{proof}
Равенство \EqRef{derivative xax power -1, division ring}
является следствием равенств \EqRef{Gateaux derivative of product, division ring},
\EqRef{Gateaux differential, product over constant, fx=x, division ring},
\EqRef{derivative xax power -1, division ring}.
\end{proof}


==> Differential.Vector.English.tex <==
%auto-ignore

\input{Differential.Vector.Eq}

\ifx\PrintBook\undefined
\else
\chapter{Differentiable Maps of \texorpdfstring{$D$}{D}-Vector Space}
\label{chapter: Differentiable maps of D Vector Space}
\fi

\section{Topological \texorpdfstring{$D$}{D}-Vector Space}
\label{section: topological D vector space}

\begin{definition}
Given a topological division ring $D$ and
$D$\Hyph vector space $V$
such that $V$ has
a topology compatible with the structure of the additive
group of $V$ and maps
\ShowEq{topological D vector space}
are continuous,
then $V$ is called a
\AddIndex{topological $D$\Hyph vector space}
{topological D vector space}\footnote{I
made definition according to definition
from \citeBib{Bourbaki: Topological Vector Space},
p. TVS I.1}.
\qed
\end{definition}

\begin{definition}
The map \[f:F\rightarrow A\]
of set $F$
to an arbitrary algebra $A$ is called
\AddIndex{$A$\Hyph valued function}{A valued function}.
The map \[f:F\rightarrow V\]
of set $F$
to $D$\Hyph vector space $V$ is called
\AddIndex{$D$\Hyph vector function}{d vector function}.
\qed
\end{definition}

We consider following definitions in this
section for topological $D$\Hyph vector space.
However definitions do not change, if we consider
topological \dcr vector space.

\begin{definition}
Let $V$ be $D$\Hyph vector space of dimension $n$.
Let $\Basis e$ be basis of \dcr vector space $V$.
We represent an arbitrary map
\ShowEq{f:V->A}
$D$\Hyph vector space $V$
to set $A$
as \AddIndex{map}{map of n D valued variables}
\[f':D^n\rightarrow A\]
of $n$
\AddIndex{$D$\Hyph valued variables}{D valued variable};
function $f'$ is defined by equation
\ShowEq{map of n D valued variables}
\qed
\end{definition}

\begin{definition}
A map
\ShowEq{f:V->A}
of topological $D$\Hyph vector space $V$ of dimension $n$
to topological space $A$
is called \AddIndex{continuous with respect to set 
of the arguments}
{map continuous with respect to set of arguments}
if for arbitrary neighbourhood $U$ of image of element
\ShowEq{a=a CRstar e in V}
for every $a_i\in D$
there exist such neighbourhood $V_i$,
that \[f'(V_1, ..., V_n)\subset U\]
\qed
\end{definition}

\begin{theorem}
Continuous map
\ShowEq{f:V->A}
of topological $D$\Hyph vector space $V$
of dimension $n$
to topological space $A$
is continuous with respect to set of arguments.
\end{theorem}
\begin{proof}
Let
\ShowEq{b=f(a)}
and $U$ be neigborhood of point $b$.
Since map $f$ is continuous, there exists such neighborhood
$V$ of vector
\ShowEq{a=a CRstar e}
that $f(V)\subseteq U$.
Since additive operation is continues, then there exists such neighborhood
$E_i$ of vector $e_i$ and neighborhood $W_i$
of $a_i\in D$ that $W\RCstar E\subset V$.
\end{proof}

\begin{definition}
\label{definition: norm on d vector space}
\AddIndex{Norm on $D$\Hyph vector space}
{norm on D vector space} $\Vector V$
over non\Hyph discrete valued division ring $D$\footnote{I
made definition according to definition
from \citeBib{Bourbaki: General Topology: Chapter 5 - 10},
IX, \S 3.3} is a map
\ShowEq{norm on d vector space}
which satisfies the following axioms
\begin{itemize}
\ShowEq{|v| ge 0}
\item $\|v\|=0$ if, and only if, $v=0$
\ShowEq{|v+w|}
\ShowEq{|av|}
for all $a\in D$ and all $v\in V$
\end{itemize}

If $D$ is a non\Hyph discrete valued division ring,
$D$\Hyph vector space $V$,
endowed with the structure defined by a given norm on
$V$, is called
\AddIndex{normed $D$\Hyph vector space}{normed D vector space}.
\qed
\end{definition}

Invariant distance on additive group of
$D$\Hyph vector space $V$
\ShowEq{Invariant distance}
defines topology of metric space
compatible with structure of $D$\Hyph vector space $V$.

\begin{definition}
\label{definition: norm of map, D vector space}
Let $D$ be complete division ring of characteristic $0$.
Let
\ShowEq{f:V->W}
be map of normed $D$\hyph vector space $V$ with norm $\|x\|_1$
to normed $D$\hyph vector space $\Vector W$ with norm $\|\Vector y\|_2$.
Value
\ShowEq{norm of map, D vector space}
is called
\AddIndex{norm of map}{norm of map} $f$.
\qed
\end{definition}

\section{Differentiable Maps of \texorpdfstring{$D$}{D}-Vector Space}
\label{section: Differentiable maps of D Vector Space}

\begin{definition}
\label{definition: map differentiable in Gateaux sense, D vector space}
The map
\ShowEq{f:V->W}
of normed $D$\Hyph vector space $V$
with norm $\|x\|_1$
to normed $D$\Hyph vector space $W$
with norm $\|x\|_2$\footnote{When dimension of $D$\Hyph vector space $V$
equal $1$, we can identify it with division ring $D$. Then we
speak about map of division ring $D$ into $D$\Hyph vector space $W$.
When dimension of $D$\Hyph vector space $W$
equal $1$, we can identify it with division ring $D$. Then we
speak about map of $D$\Hyph vector space $V$ into division ring $D$.
In both cases we will omit corresponding index,
because this index has single value.}
is called
\AddIndex{differentiable in the G\^ateaux sense on the set $U\subset V$}
{map differentiable in Gateaux sense},
if at every point $x\in U$
the increment of the map $f$ can be represented as
\ShowEq{Gateaux derivative of map, D vector space, def}
\ShowEq{Gateaux derivative of map, D vector space}
where
\AddIndex{the G\^ateaux derivative
$\ShowSymbol{Gateaux derivative of map}$
of map $f$}
{Gateaux derivative of map}
is linear map of increment $a$ and
\ShowEq{o:V->W}
is such continuous map that
\ShowEq{o:V->W 1}
\qed
\end{definition}

\begin{remark}
\label{remark: differential L(D,V,W)}
According to definition
\ref{definition: map differentiable in Gateaux sense, D vector space}
for given $x$, the G\^ateaux derivative
\ShowEq{df in L(V,W)}
Therefore, the G\^ateaux derivative of map $f$ is map
\ShowEq{differential L(D,V,W)}
\qed
\end{remark}

\begin{theorem}
\label{theorem: map differentiable in Gateaux sense, D vector space}
Let $D$ be division ring of characteristic $0$.
Let $V$, $W$ be $D$\Hyph vector spaces.
Let \eV V be basis of \dcr vector space $V$ and
\ShowEq{h in V}
Let \eV W be basis of \dcr vector space $W$.
It is possible to represent the G\^ateaux derivative
of map $f$ as
\ShowEq{Gateaux differential of map, D vector space, representation}
\end{theorem}
\begin{proof}
Corollary of definition
\ref{definition: map differentiable in Gateaux sense, D vector space}
and theorem
\ePrints{0812.4763}
\ifx\Semafor\ValueOn
\ref{theorem: linear map, D vector space}.
\else
\xRef{0701.238}{theorem: linear map, D vector space}.
\fi
\end{proof}

\begin{definition}
\begin{sloppypar}
Expression
\ShowEq{component of Gateaux derivative of map, D vector space}
is called
\AddIndex{component of the G\^ateaux derivative}
{component of Gateaux derivative} of map $f(x)$.
\qed
\end{sloppypar}
\end{definition}

\begin{theorem}
\label{theorem: Gateaux derivative over field F, D vector space}
Let complete division ring $D$ of characteristic $0$
is algebra over field $F\subset Z(D)$.
The G\^ateaux derivative of the map
\ShowEq{f:V->W}
of normed $D$\Hyph vector space $V$
to normed $D$\Hyph vector space $W$
satisfies to equation
\ShowEq{Gateaux derivative over field F, D vector space}
\end{theorem}
\begin{proof}
Corollary of definitions
\ePrints{0812.4763}
\ifx\Semafor\ValueOn
\ref{definition: linear map, vector space},
\else
\xRef{0701.238}{definition: linear map, vector space},
\fi
\ref{definition: map differentiable in Gateaux sense, D vector space}.
\end{proof}

\begin{theorem}
\label{theorem: Gateaux derivative is multiplicative over field R, D vector space}
Let $D$ be complete division ring of characteristic $0$.
The G\^ateaux derivative
of the function
\ShowEq{f:V->W}
of normed $D$\Hyph vector space $V$
to normed $D$\Hyph vector space $W$
satisfies to equation
\ShowEq{Gateaux differential is multiplicative over field R, D vector space}
for every $r\in R$, $r\ne 0$ and  $a\in V$, $a\ne 0$.
\end{theorem}
\begin{proof}
Corollary of theorems
\ref{theorem: real subring of center},
\ePrints{0812.4763}
\ifx\Semafor\ValueOn
\ref{theorem: Gateaux derivative over field F, D vector space}.
\else
\xRef{0812.4763}{theorem: Gateaux derivative over field F, D vector space}.
\fi
\end{proof}

Combining equation
\EqRef{Gateaux differential is multiplicative over field R, D vector space}
and definition
\ref{definition: map differentiable in Gateaux sense, D vector space},
we get known definition of the G\^ateaux derivative
\ShowEq{Gateaux differential, D vector space, representation, 2}
Definitions of the G\^ateaux derivative
\EqRef{Gateaux derivative of map, D vector space}
and \EqRef{Gateaux differential, D vector space, representation, 2}
are equivalent. Using this equivalence we tell
that map $f$
is called differentiable in the G\^ateaux sense on the set $U\subset D$,
if at every point $x\in U$
the increment of the function $f$ can be represented as
\ShowEq{Gateaux differential of map, t, D vector space}
where
\ShowEq{o:R->W}
is such continuous map that
\ShowEq{o:R->W 1}

Since infinitesimal $a$ is differential $dx$,
then equation
\EqRef{Gateaux differential of map, D vector space, representation}
becomes definition of
\AddIndex{the G\^ateaux differential}{Gateaux differential of map}
\ShowEq{Gateaux differential of map, D vector space}
\ShowEq{Gateaux differential of map, D vector space, form}

\begin{definition}
\label{definition: Gateaux partial derivative, D vector space}
\ShowEq{Gateaux partial derivative; D vector space}
Let $D$ be division ring of characteristic $0$.
Let $V$, $W$ be $D$\Hyph vector spaces.
Let \eV V be basis of \dcr vector space $V$ and
\ShowEq{h in V}
Let \eV W be basis of \dcr vector space $W$.
If we consider the G\^ateaux derivative of map $f$
with respect to variable $v^{\gii}$ assuming that other coordinates of vector
$v$ are fixed, then corresponding additive map
\ShowEq{Gateaux partial derivative, D vector space}
is called
\AddIndex{the G\^ateaux partial derivative}{Gateaux partial derivative}
of map $f^{\gij}$
with respect to variable $v^{\gii}$.
\qed
\end{definition}

\begin{theorem}
\label{theorem: expansion of Gateaux differential, D vector space}
Let $D$ be division ring of characteristic $0$.
Let \eV V be basis of $D$\Hyph vector space $V$ and
\ShowEq{h in V}
Let \eV W be basis of $D$\Hyph vector space $W$.
Let the G\^ateaux partial derivatives of map
\ShowEq{f:V->W}
are continuous on the set $U\in V$.
Then, on the set $U$, the G\^ateaux derivative of map $f$
and the G\^ateaux partial derivatives hold
\ShowEq{expansion of Gateaux differential, D vector space}
\end{theorem}
\begin{proof}
From theorem
\ePrints{0812.4763}
\ifx\Semafor\ValueOn
\ref{theorem: partial linear map of variable},
\else
\xRef{0701.238}{theorem: partial linear map of variable},
\fi
it follows that we can expand the G\^ateaux derivative of map $f$
into sum \EqRef{expansion of Gateaux differential, D vector space}
of partial linear maps. Our task is to clarify when
these partial linear maps become the G\^ateaux partial derivatives.

According to definitions
\ref{eq: Gateaux differential, D vector space, representation, 2},
\ShowEq{expansion of Gateaux differential, D vector space, 1}
From equations \EqRef{Gateaux partial derivative, D vector space} and
\EqRef{expansion of Gateaux differential, D vector space, 1},
up to infinitesimal with respect to $t$, it follows that
\ShowEq{expansion of Gateaux differential, D vector space, 2}
Therefore, for the equation
\EqRef{expansion of Gateaux differential, D vector space}
to follow from the equation
\EqRef{expansion of Gateaux differential, D vector space, 2}
it is necessary that the G\^ateaux partial derivatives be continuous.
\end{proof}

\begin{definition}
\label{definition: Gateaux dcr derivative of map, D vector space}
Let map
\ShowEq{f:V->W}
of normed $D$\Hyph vector space $V$
to normed $D$\Hyph vector space $W$
be differentiable in the G\^ateaux sense on the set $U\times W$.
Assume we selected basis \eV V
in \dcr vector space $V$.
Assume we selected basis \eV W
in \dcr vector space $W$.
\ShowEq{Gateaux dcr derivative of map}
We define \AddIndex{the G\^ateaux \dcr derivative
$\displaystyle\ShowSymbol{Gateaux dcr derivative of map, D vector space}$
of map $f$}
{Gateaux dcr derivative of map, D vector space}.
using equation
\ShowEq{Gateaux dcr derivative, D vector space}
Expression $\displaystyle
\ShowSymbol{Gateaux partial dcr derivative of map, 2, D vector space}$
in equation
\EqRef{Gateaux dcr derivative, D vector space}
is called
\AddIndex{the G\^ateaux partial \dcr derivative of map $f^{\gij}$
with respect to variable $x^{\gii}$}
{Gateaux partial dcr derivative of map with respect to variable, D vector space}.
\qed
\end{definition}

For representation of the G\^ateaux \dcr derivative
we also use notation
\ShowEq{Gateaux dcr derivative 1, D vector space}

\begin{definition}
\label{definition: Gateaux rcd derivative of map, D vector space}
Let map
\ShowEq{f:V->W}
of normed $D$\hyph vector space $V$
to normed $D$\hyph vector space $W$
be differentiable in the G\^ateaux sense on the set $U\times W$.
Assume we selected basis \eV V
in \rcd vector space $V$.
Assume we selected basis \eV W
in \rcd vector space $W$.
\ShowEq{Gateaux rcd derivative of map}
We define \AddIndex{the G\^ateaux \rcd derivative
$\displaystyle\ShowSymbol{Gateaux rcd derivative of map, D vector space}$
of map $f$}
{Gateaux rcd derivative of map, D vector space}.
using equation
\ShowEq{Gateaux rcd derivative, D vector space}
Expression $\displaystyle
\ShowSymbol{Gateaux partial rcd derivative of map, 2, D vector space}$
in equation
\EqRef{Gateaux rcd derivative, D vector space}
is called
\AddIndex{the G\^ateaux partial \rcd derivative of map $f^{\gij}$
with respect to variable $x^{\gii}$}
{Gateaux partial rcd derivative of map with respect to variable, D vector space}.
\qed
\end{definition}

For representation of the G\^ateaux \rcd derivative
we also use notation
\ShowEq{Gateaux rcd derivative 1, D vector space}

\ifx\texFuture\Defined
\begin{theorem}
\label{theorem: increment of diferentiable function, D vector space}
Let function \[\Vector f:\Vector U\rightarrow\Vector V\]
of normed $D$\Hyph vector space $\Vector U$
to normed $D$\Hyph vector space $\Vector V$
be differentiable in the G\^ateaux sense at point
$\Vector x$.
Let unit sphere of normed $D$\Hyph vector space $\Vector U$ be compact.
Let $\Vector a$, $\Vector b\in\Vector U$,
$\|\Vector a\|_1=\|\Vector a\|_2=1$.
Then
\begin{equation}
\EqLabel{increment of diferentiable function, D vector space}
\|\Vector f(\Vector x+t\Vector a)-\Vector f(\Vector x+s\Vector b)\|_2
\le|t-s|\ \|\partial \Vector f\|
\end{equation}
\end{theorem}
\begin{proof}
According to definition
\EqRef{Gateaux derivative of map, D vector space}
\end{proof}
\fi

\begin{theorem}
\label{theorem: Gateaux differential, 0, D vector space}
Let $D$ be division ring  of characteristic $0$.
Let function
\ShowEq{f:U->V}
of normed $D$\Hyph vector space $U$
to normed $D$\Hyph vector space $V$
be differentiable in the G\^ateaux sense at point
$x$.
Then
\ShowEq{df(x)0=0}
\end{theorem}
\begin{proof}
Corollary of definitions
\ref{definition: map differentiable in Gateaux sense, D vector space}
and theorem
\ePrints{0812.4763}
\ifx\Semafor\ValueOn
\ref{theorem: linear map, 0, D vector space}.
\else
\xRef{0701.238}{theorem: linear map, 0, D vector space}.
\fi
\end{proof}

\begin{theorem}
\label{theorem: composite map, differential, D vector space}
Let $D$ be division ring  of characteristic $0$.
Let $U$ be normed $D$\Hyph vector space with norm $\|x\|_1$.
Let $V$ be normed $D$\Hyph vector space with norm $\|y\|_2$.
Let $W$ be normed $D$\Hyph vector space with norm $\|z\|_3$.
Let map
\ShowEq{f:U->V}
be differentiable in the G\^ateaux sense at point
$x$
and norm of the G\^ateaux derivative of map $f$
be finite
\ShowEq{composite map, norm f, D vector space}
Let map
\ShowEq{g:V->W}
be differentiable in the G\^ateaux sense at point
\ShowEq{composite map, y fx, D vector space}
and norm of the G\^ateaux derivative of map $g$
be finite
\ShowEq{composite map, norm g, D vector space}
Map
\ShowEq{composite map, gfx, D vector space}
is differentiable in the G\^ateaux sense at point
$x$
\ShowEq{composite map, differential, D vector space}
\ShowEq{composite map, Gateaux dcr derivative, D vector space}
\ShowEq{composite map, Gateaux dcr derivative 1, D vector space}
\ShowEq{composite map, Gateaux derivative 0, D vector space}
\ShowEq{composite map, Gateaux derivative 1, D vector space}
\end{theorem}
\begin{proof}
According to definition
\ref{definition: map differentiable in Gateaux sense, D vector space}
\ShowEq{Gateaux differential of map g, D vector space}
where
\ShowEq{o1:V->W}
is such continuous map that
\ShowEq{o1:V->W 1}
According to definition
\ref{definition: map differentiable in Gateaux sense, D vector space}
\ShowEq{Gateaux differential of map f, D vector space}
where
\ShowEq{o2:U->V}
is such continuous map that
\ShowEq{o2:U->V 1}
According to
\EqRef{Gateaux differential of map f, D vector space}
increment of vector $x\in U$ in direction $a$
leads to increment of vector
$y$
in direction
\ShowEq{composite map, b fxa, D vector space}
Using \EqRef{composite map, y fx, D vector space},
\EqRef{composite map, b fxa, D vector space}
in equation \EqRef{Gateaux differential of map g, D vector space},
we get
\ShowEq{Gateaux differential of map gf, 1, D vector space}
According to definitions
\ref{definition: map differentiable in Gateaux sense, D vector space},
\ePrints{0812.4763}
\ifx\Semafor\ValueOn
\ref{definition: linear map, vector space}
\else
\xRef{0701.238}{definition: linear map, vector space}
\fi
from equation \EqRef{Gateaux differential of map gf, 1, D vector space}
it follows
\ShowEq{Gateaux differential of map gf, 2, D vector space}
Let us find limit
\ShowEq{Gateaux differential of map gf, 2 1, D vector space}
According to definition \ref{definition: norm on d vector space}
\ShowEq{Gateaux differential of map gf, 3, D vector space}
From \EqRef{composite map, norm g, D vector space}
it follows that
\ShowEq{Gateaux differential of map gf, 4, D vector space}
From \EqRef{composite map, norm f, D vector space}
it follows that
\ShowEq{Gateaux differential of map gf, 5 1, D vector space}
According to the theorem \ref{theorem: Gateaux differential, 0, D vector space}
\ShowEq{Gateaux differential of map gf, 5 2, D vector space}
Therefore,
\ShowEq{Gateaux differential of map gf, 5, D vector space}
From equations
\EqRef{Gateaux differential of map gf, 3, D vector space},
\EqRef{Gateaux differential of map gf, 4, D vector space},
\EqRef{Gateaux differential of map gf, 5, D vector space}
it follows that
\ShowEq{Gateaux differential of map gf, 6, D vector space}
According to definition
\ref{definition: map differentiable in Gateaux sense, D vector space}
\ShowEq{Gateaux differential of map gf, 7, D vector space}
where
\ShowEq{o:U->W}
is such continuous map that
\ShowEq{o:U->W 1}
Equation \EqRef{composite map, differential, D vector space}
follows from
\EqRef{Gateaux differential of map gf, 2, D vector space},
\EqRef{Gateaux differential of map gf, 6, D vector space},
\EqRef{Gateaux differential of map gf, 7, D vector space}.

From equation \EqRef{composite map, differential, D vector space}
and the definition
\ref{definition: Gateaux dcr derivative of map, D vector space}
it follows that
\ShowEq{composite map, differential 1, D vector space}
Since increment $a$ is arbitrary, then equation
\EqRef{composite map, Gateaux dcr derivative, D vector space}
follows from equation
\EqRef{composite map, differential 1, D vector space}.

From equation \EqRef{composite map, differential, D vector space}
and the theorem
\ref{theorem: map differentiable in Gateaux sense, D vector space}
it follows that
\ShowEq{composite map, differential 2, D vector space}
\EqRef{composite map, Gateaux derivative 0, D vector space},
\EqRef{composite map, Gateaux derivative 1, D vector space}
follow from equation
\EqRef{composite map, differential 2, D vector space}.
\end{proof}


==> Differential.Vector.Eq.tex <==
%auto-ignore

\DefEq
{
\[
\partial f:V\rightarrow \mathcal L(D;V;W)
\]
}
{differential L(D,V,W)}

\DefEq
{
$h\in V$
\[
\Vector h=h \CRstar e_V
\]
}
{h in V}

\DefEq
{
\symb{\partial f(x)(dx)}
0{Gateaux differential of map, vector}
}
{Gateaux differential of map, D vector space}

\DefEquation
{
\partial f(x)(h)
=\partial_{s\cdot 0\cdot\gii} f^{\gij}(x)
\ h^{\gii}
\ \partial_{s\cdot 1\cdot\gii} f^{\gij}(x)
\ \EV Wj
=\frac{\partial_{s\cdot 0} f^{\gij}(x)}{\partial x^{\gii}}
\ h^{\gii}
\ \frac{\partial_{s\cdot 1} f^{\gij}(x)}{\partial x^{\gii}}
\ \EV Wj
}
{Gateaux differential of map, D vector space, representation}

\DefEq
{
\symb{\frac{\partial_{s\cdot p} f^{\gij}(x)}{\partial x^{\gii}}}0
{component of Gateaux derivative, vector space}
\symb{\partial_{s\cdot p\cdot\gii} f^{\gij}(x)}0
{component of Gateaux derivative of map, D vector space, short}
$\displaystyle
\ShowSymbol{component of Gateaux derivative of map, D vector space, short}
=
\ShowSymbol{component of Gateaux derivative, vector space}$,
$p=0$, $1$,
}
{component of Gateaux derivative of map, D vector space}

\DefEq
{
\symb{\|f\|}0{norm of map}
\[
\ShowSymbol{norm of map}=
\text{sup}\frac{\|f(x)\|_2}{\|x\|_1}
\]
}
{norm of map, D vector space}

\DefEq
{
\[
\begin{matrix}
\partial f(x)(ph)=
p\partial f(x)(h)
&p\in F
\end{matrix}
\]
}
{Gateaux derivative over field F, D vector space}

\DefEq
{
\[f:V\rightarrow W\]
}
{f:V->W}

\DefEquation
{
\partial f(x)(h)=
\left(\frac{\partial f^{\gij}(x)}{\partial x^{\gii}}(h^{\gii})\right)
\EV Wj
}
{expansion of Gateaux differential, D vector space}

\DefEquation
{
\begin{split}
\partial f(x)(h)
=&\lim_{t\rightarrow 0}(t^{-1}(f(x+th)-f(x)))
\\
=&\lim_{t\rightarrow 0}(t^{-1}
(f^{\gij}(x^{\giA}+th^{\giA},x^{\gi 2}+th^{\gi 2},...,x^{\gin}+th^{\gin})
\\
-&f^{\gij}(x^{\giA},x^{\gi 2}+th^{\gi 2},...,x^{\gin}+th^{\gin})
\\
+&f^{\gij}(x^{\giA},x^{\gi 2}+th^{\gi 2},...,x^{\gin}+th^{\gin})
-...
\\
-&f^{\gij}(x^{\giA},...,x^{\gin})))\EV Wj
\end{split}
}
{expansion of Gateaux differential, D vector space, 1}

\DefEquation
{
\begin{split}
\partial f(x)(h)
=\lim_{t\rightarrow 0}&\left(
\frac{\partial f^{\gij}
(x^{\giA},x^{\gi 2}+th^{\gi 2},...,x^{\gin}+th^{\gin})}
{\partial x^{\giA}}( h^{\giA})\right.
\\
+...&+
\left.\frac{\partial f^{\gij}(x^{\giA},...,x^{\gin})}{\partial x^{\gin}}
(h^{\gin})
\right)\EV Wj
\end{split}
}
{expansion of Gateaux differential, D vector space, 2}

\DefEquation
{
\partial f(x)(ra)
=
r\partial f(x)(a)
}
{Gateaux differential is multiplicative over field R, D vector space}

\DefEquation
{
\partial f(x)(a)=
\lim_{t\rightarrow 0}(t^{-1}(f(x+ta)-f(x)))
}
{Gateaux differential, D vector space, representation, 2}

\DefEquation
{
f(x+ta)-f(x)
=t\partial f(x)(a)
+o(t)
}
{Gateaux differential of map, t, D vector space}

\DefEq
{
$o:R\rightarrow W$
}
{o:R->W}

\DefEq
{
\[
\lim_{t\rightarrow 0}\frac{\|o(t)\|_2}{|t|}=0
\]
}
{o:R->W 1}

\DefEquation
{
\ShowSymbol{Gateaux differential of map, vector}
=\frac{\partial_{s\cdot 0} f^{\gij}(x)}{\partial x^{\gii}}
\ dx^{\gii}
\ \frac{\partial_{s\cdot 1} f^{\gij}(x)}{\partial x^{\gii}}
\ \EV Wj
}
{Gateaux differential of map, D vector space, form}

\DefEq
{
\symb{\frac{\partial f^{\gij}(v)}{\partial v^{\gii}}}
0{Gateaux partial derivative}
}
{Gateaux partial derivative; D vector space}

\DefEquation
{
\ShowSymbol{Gateaux partial derivative}(h^{\gii})
=\lim_{t\rightarrow 0}
(t^{-1}(f^{\gij}(v^{\giA},...,v^{\gii}+th^{\gii},...,v^{\gin})
-f^{\gij}(v)))
}
{Gateaux partial derivative, D vector space}

\DefEq
{
\[f:V\rightarrow A\]
}
{f:V->A}

\DefEq
{
\item $\|v+w\|\le \|v\|+\|w\|$
}
{|v+w|}

\DefEq
{
\[d(a,b)=\|a-b\|\]
}
{Invariant distance}

\DefEq
{
\item $\|av\|=|a|\|v\|$
}
{|av|}

\DefEq
{
\[v\in V\rightarrow \|v\|\in R\]
}
{norm on d vector space}

\DefEq
{
\item $\|v\|\ge 0$
}
{|v| ge 0}

\DefEq
{
$\Vector a=a\CRstar e$
}
{a=a CRstar e}

\DefEq
{
$\Vector a=a\CRstar e\in V$
}
{a=a CRstar e in V}

\DefEq
{
\[
f'(a^1,...,a^n)=f(a\CRstar e)
\]
}
{map of n D valued variables}

\DefEq
{
\begin{align*}
(a,v)&\in D\times V\rightarrow av\in V
\\
(v,a)&\in V\times D\rightarrow va\in V
\end{align*}
}
{topological D vector space}

\DefEq
{
\[f:U\rightarrow V\]
}
{f:U->V}

\DefEquation
{
\partial f(x)(a)
=a\CRstar\ShowSymbol{Gateaux dcr derivative of map, D vector space}
=a^{\gii}\ \ShowSymbol{Gateaux partial dcr derivative of map, 2, D vector space}
\ \EV Wj
}
{Gateaux dcr derivative, D vector space}

\DefEq
{
\[
\begin{array}{lll}
\displaystyle
\frac{\partial f(x)(a)}{\DcrPartial{}x}
&\displaystyle=
\frac{\partial}{\DcrPartial{}x}f(x)(a)
&\displaystyle=
\ShowSymbol{Gateaux partial dcr derivative of map, 3, D vector space}
\\
\displaystyle
\frac{\partial f^{\gij}(x)(a^{\gii})}{\DcrPartial{} x^{\gii}}
&\displaystyle=
\frac{\partial}{\DcrPartial{} x^{\gii}} f^{\gij}(x)(a)
&\displaystyle=
\ShowSymbol{Gateaux partial dcr derivative of map, 1, D vector space}
\end{array}
\]
}
{Gateaux dcr derivative 1, D vector space}

\DefEq
{
\[
\begin{array}{lll}
\displaystyle
\frac{\partial f(x)(a)}{\rcDPartial{}x}
&\displaystyle=
\frac{\partial}{\rcDPartial{}x}f(x)(a)
&\displaystyle=
\ShowSymbol{Gateaux partial rcd derivative of map, 3, D vector space}
\\
\displaystyle
\frac{\partial f^{\gij}(x)(a)}{\rcDPartial{} x^{\gii}}
&\displaystyle=
\frac{\partial}{\rcDPartial{} x^{\gii}} f^{\gij}(x)(a)
&\displaystyle=
\ShowSymbol{Gateaux partial rcd derivative of map, 1, D vector space}
\end{array}
\]
}
{Gateaux rcd derivative 1, D vector space}

\DefEquation
{
\begin{split}
a\CRstar\frac{\partial gf(x)(a)}{\DcrPartial{}x}
&=
\partial f(x)(a)\CRstar
\frac{\partial g(f(x))(\partial f(x)(a)}
{\DcrPartial{} f(x)}
\\
&=
a\CRstar\frac{\partial f(x)(a)}{\DcrPartial{}x}
\CRstar
\frac{\partial g(f(x))(\partial f(x)(a)}
{\DcrPartial{} f(x)}
\end{split}
}
{composite map, differential 1, D vector space}

\DefEquation
{
\frac{\partial(gf)^{\gik}(x)(a)}{\DcrPartial{} x^{\gii}}
=
\frac{\partial f^{\gij}(x)(a)}{\DcrPartial{} x^{\gii}}
\frac{\partial g^{\gik}(f(x))(\partial f(x)(a))}
{\DcrPartial{} f^{\gij}(x)}
}
{composite map, Gateaux dcr derivative 1, D vector space}

\DefEquation
{
\frac{\partial gf(x)(a)}{\DcrPartial{}x}
=
\frac{\partial f(x)(a)}{\DcrPartial{}x}
\CRstar
\frac{\partial g(f(x))(\partial f(x)(a))}
{\DcrPartial{} f(x)}
}
{composite map, Gateaux dcr derivative, D vector space}

\DefEquation
{
\partial f(x)(a)
=\ShowSymbol{Gateaux rcd derivative of map, D vector space}\RCstar\Vector a
=\EV Wj\ \ShowSymbol{Gateaux partial rcd derivative of map, 2, D vector space}
\ a^{\gii}
}
{Gateaux rcd derivative, D vector space}

\DefEq
{
\symb{\frac{\partial f(x)(a)}{\rcDPartial{} x}}
0{Gateaux rcd derivative of map, D vector space}
\symb{\rcDPartial{\gii}\ f^{\gij}(x)(a)}0
{Gateaux partial rcd derivative of map, 1, D vector space}
\symb{\rcDPartial{}f(x)(a)}0
{Gateaux partial rcd derivative of map, 3, D vector space}
\symb{\frac{\partial f^{\gij}(x)(a)}{\rcDPartial{} x^{\gii}}}0
{Gateaux partial rcd derivative of map, 2, D vector space}
}
{Gateaux rcd derivative of map}

\DefEq
{
$b=f(a\CRstar e)\in A$
}
{b=f(a)}

\DefEq
{
\symb{\frac{\partial f(x)(a)}{\DcrPartial{} x}}%
0{Gateaux dcr derivative of map, D vector space}%
\symb{\DcrPartial{i} f^{\gij}(x)(a)}0%
{Gateaux partial dcr derivative of map, 1, D vector space}%
\symb{\DcrPartial{} f(x)(a)}0%
{Gateaux partial dcr derivative of map, 3, D vector space}%
\symb{\frac{\partial f^{\gij}(x)(a)}{\DcrPartial{} x^{\gii}}}0%
{Gateaux partial dcr derivative of map, 2, D vector space}%
}
{Gateaux dcr derivative of map}

\DefEq
{
\[
\partial f(x)(0)=0
\]
}
{df(x)0=0}

\DefEquation
{
\|\partial f(x)\|=F\le\infty
}
{composite map, norm f, D vector space}

\DefEq
{
\[g:V\rightarrow W\]
}
{g:V->W}

\DefEquation
{
y=f(x)
}
{composite map, y fx, D vector space}

\DefEquation
{
\|\partial g(y)\|=G\le\infty
}
{composite map, norm g, D vector space}

\DefEquation
{
gf(x)=g(f(x))
}
{composite map, gfx, D vector space}

\DefEquation
{
\partial gf(x)(a)
=\partial g(f(x))(\partial f(x)(a))
}
{composite map, differential, D vector space}

\DefEquation
{
\frac{\partial_{st\cdot 0} (gf)^{\gik}(x)}{\partial x^{\gii}}=
\frac{\partial_{s\cdot 0} g^{\gik}(f(x))}{\partial f^{\gij}(x)}
\frac{\partial_{t\cdot 0} f^{\gij}(x)}{\partial x^{\gii}}
}
{composite map, Gateaux derivative 0, D vector space}

\DefEquation
{
\frac{\partial_{st\cdot 1} (gf)^{\gik}(x)}{\partial x^{\gii}}=
\frac{\partial_{t\cdot 1} f^{\gij}(x)}{\partial x^{\gii}}
\frac{\partial_{s\cdot 1} g^{\gik}(f(x))}{\partial f^{\gij}(x)}
}
{composite map, Gateaux derivative 1, D vector space}

\DefEquation
{
g(y+b)-g(y)
=\partial g(y)(b)
+o_1(b)
}
{Gateaux differential of map g, D vector space}

\DefEq
{
$o_1:V\rightarrow W$
}
{o1:V->W}

\DefEq
{
\[
\lim_{b\rightarrow 0}\frac{\|o_1(b)\|_3}{\|b\|_2}=0
\]
}
{o1:V->W 1}

\DefEq
{
$o_2:U\rightarrow V$
}
{o2:U->V}

\DefEquation
{
b=\partial f(x)(a)+o_2(a)
}
{composite map, b fxa, D vector space}

\DefEquation
{
\begin{array}{r@{\,}l}
&g(f(x+a))-g(f(x))
\\
=&g(f(x)+\partial f(x)(a)
+o_2(a))
-g(f(x))
\\
=&\partial g(f(x))(\partial f(x)(a)
+o_2(a))
-o_1(\partial f(x)(a)
+o_2(a))
\end{array}
}
{Gateaux differential of map gf, 1, D vector space}

\DefEq
{
\[
\lim_{a\rightarrow 0}
\frac
{\|\partial g(f(x))(o_2(a))
-o_1(\partial f(x)(a)
+o_2(a))\|_3}
{\|a\|_1}
\]
}
{Gateaux differential of map gf, 2 1, D vector space}

\DefEquation
{
\begin{array}{r@{\,}l}
&\displaystyle\lim_{a\rightarrow 0}
\frac
{\|\partial g(f(x))(o_2(a))
-o_1(\partial f(x)(a)
+o_2(a))\|_3}
{\|a\|_1}
\\
\le
&\displaystyle\lim_{a\rightarrow 0}
\frac
{\|\partial g(f(x))(o_2(a))\|_3}
{\|a\|_1}
+\lim_{a\rightarrow 0}
\frac
{\|o_1(\partial f(x)(a)
+o_2(a))\|_3}
{\|a\|_1}
\end{array}
}
{Gateaux differential of map gf, 3, D vector space}

\DefEquation
{
\lim_{a\rightarrow 0}
\frac
{\|\partial g(f(x))(o_2(a))\|_3}
{\|a\|_1}
\le
G\lim_{a\rightarrow 0}
\frac
{\|o_2(a)\|_2}
{\|a\|_1}=0
}
{Gateaux differential of map gf, 4, D vector space}

\DefEq
{
\begin{align*}
&\lim_{a\rightarrow 0}
\frac
{\|o_1(\partial f(x)(a)
+o_2(a))\|_3}
{\|a\|_1}
\\
=&
\lim_{a\rightarrow 0}
\frac
{\|o_1(\partial f(x)(a)
+o_2(a))\|_3}
{\|\partial f(x)(a)
+o_2(a)\|_2}
\lim_{a\rightarrow 0}
\frac
{\|\partial f(x)(a)
+o_2(a)\|_2}
{\|a\|_1}
\\
\le&
\lim_{a\rightarrow 0}
\frac
{\|o_1(\partial f(x)(a)
+o_2(a))\|_3}
{\|\partial f(x)(a)
+o_2(a)\|_2}
\lim_{a\rightarrow 0}
\frac
{\|\partial f(x)\|\|a\|_1
+\|o_2(a)\|_2}
{\|a\|_1}
\\
=&
\lim_{a\rightarrow 0}
\frac
{\|o_1(\partial f(x)(a)
+o_2(a))\|_3}
{\|\partial f(x)(a)
+o_2(a)\|_2}
\|\partial f(x)\|
\end{align*}
}
{Gateaux differential of map gf, 5 1, D vector space}

\DefEq
{
\[
\lim_{a\rightarrow 0}
(\partial f(x)(a)
+o_2(a))=0
\]
}
{Gateaux differential of map gf, 5 2, D vector space}

\DefEquation
{
\lim_{a\rightarrow 0}
\frac
{\|o_1(\partial f(x)(a)
+o_2(a))\|_3}
{\|a\|_1}=0
}
{Gateaux differential of map gf, 5, D vector space}

\DefEquation
{
\lim_{a\rightarrow 0}
\frac
{\|\partial g(f(x))(o_2(a))
-o_1(\partial f(x)(a)
+o_2(a))\|_3}
{\|a\|_1}=0
}
{Gateaux differential of map gf, 6, D vector space}

\DefEquation
{
gf(x+a)-gf(x)
=\partial gf(x)(a)
+o(a)
}
{Gateaux differential of map gf, 7, D vector space}

\DefEq
{
$o:U\rightarrow W$
}
{o:U->W}

\DefEq
{
\[
\lim_{a\rightarrow 0}\frac{\|o(a)\|_3}{\|a\|_1}=0
\]
}
{o:U->W 1}

\DefEquation
{
\begin{array}{r@{\,}l}
&\displaystyle\frac{\partial_{st\cdot 0} gf^{\gik}(x)}{\partial x^{\gii}}
\ a^{\gii}
\ \frac{\partial_{st\cdot 1} gf^{\gik}(x)}{\partial x^{\gii}}
\ \EV Wk
\\
=&\displaystyle
\frac{\partial_{s\cdot 0} g^{\gik}(f(x))}{\partial f^{\gij}(x)}
\ \partial f^{\gij}(x)(a)
\ \frac{\partial_{s\cdot 1} g^{\gik}(f(x))}{\partial f^{\gij}(x)}
\ \EV Wk
\\
=&\displaystyle
\frac{\partial_{s\cdot 0} g^{\gik}(f(x))}{\partial f^{\gij}(x)}
\frac{\partial_{t\cdot 0} f^{\gij}(x)}{\partial x^{\gii}}
\ a^{\gii}
\ \frac{\partial_{t\cdot 1} f^{\gij}(x)}{\partial x^{\gii}}
\ \frac{\partial_{s\cdot 1} g^{\gik}(f(x))}{\partial f^{\gij}(x)}
\ \EV Wk
\end{array}
}
{composite map, differential 2, D vector space}

\DefEquation
{
f(x+a)-f(x)
=\ShowSymbol{Gateaux derivative of map}(a)
+o(a)
}
{Gateaux derivative of map, D vector space}

\DefEq
{
\symb{\partial f(x)}0{Gateaux derivative of map}
}
{Gateaux derivative of map, D vector space, def}

\DefEq
{
$\partial f(x)\in\mathcal L(D;V;W)$.
}
{df in L(V,W)}

\DefEq
{
\[
\lim_{a\rightarrow 0}\frac{\|o(a)\|_2}{\|a\|_1}=0
\]
}
{o:V->W 1}

\DefEq
{
$o:V\rightarrow W$
}
{o:V->W}

\DefEquation
{
\begin{array}{r@{\,}l}
&g(f(x+a))-g(f(x))
\\
=&\partial g(f(x))(\partial f(x)(a))
+\partial g(f(x))(o_2(a))
-o_1(\partial f(x)(a)
+o_2(a))
\end{array}
}
{Gateaux differential of map gf, 2, D vector space}

\DefEq
{
\[
\lim_{a\rightarrow 0}\frac{\|o_2(a)\|_2}{\|a\|_1}=0
\]
}
{o2:U->V 1}

\DefEquation
{
f(x+a)-f(x)
=\partial f(x)(a)
+o_2(a)
}
{Gateaux differential of map f, D vector space}


==> Differential.Vector.Russian.tex <==
%auto-ignore

\input{Differential.Vector.Eq}
\ifx\PrintBook\undefined
\else
\chapter{Дифференцируемые отображения \texorpdfstring{$D$}{D}-векторного пространства}
\label{chapter: Differentiable maps of D Vector Space}
\fi

\section{Топологическое \texorpdfstring{$D$}{D}-векторное пространство}
\label{section: topological D vector space}

\begin{definition}
\begin{sloppypar}
Пусть $D$ - топологическое тело.
$D$\Hyph векторное пространство $V$ называется 
\AddIndex{топологическим $D$\Hyph векторным пространством}
{topological D vector space}\footnote{Определение
дано согласно
определению из \citeBib{Bourbaki: Topological Vector Space}, с. 21},
если $V$ наделено топологией, согласующейся со
структурой аддитивной группы в $V$,
и отображения
\ShowEq{topological D vector space}
непрерывны.
\qed
\end{sloppypar}
\end{definition}

\begin{definition}
Отображение \[f:F\rightarrow A\]
множества $F$
в произвольную алгебру $A$
называется
\AddIndex{$A$\Hyph значной функцией}{A valued function}.
Отображение \[f:F\rightarrow V\]
множества $F$ в $D$\Hyph векторное пространство $V$
называется
\AddIndex{$D$\Hyph вектор\Hyph функцией}{d vector function}.
\qed
\end{definition}

Мы рассматриваем последующие определения в этом
разделе для топологического $D$\Hyph векторного пространства.
Однако определения не изменятся, если мы будем рассматривать
топологическое \dcr векторное пространство.

\begin{definition}
Пусть $V$ - $D$\Hyph векторное пространство размерности $n$.
Пусть $\Basis e$ - базис \dcr векторного пространства $V$.
Произвольное отображение
\ShowEq{f:V->A}
$D$\Hyph векторного пространства $V$
в множество $A$
можно представить в виде \AddIndex{отображения}{map of n D valued variables}
\[f':D^n\rightarrow A\]
$n$
\AddIndex{$D$\Hyph значных переменных}{D valued variable};
функция $f'$ определена равенством
\ShowEq{map of n D valued variables}
\qed
\end{definition}

\begin{definition}
Отображение
\ShowEq{f:V->A}
топологического $D$\Hyph векторного пространства $V$ размерности $n$
в топологическое пространство $A$
называется \AddIndex{непрерывным по совокупности аргументов}
{map continuous with respect to set of arguments},
если для произвольной окрестности $U$ образа элемента
\ShowEq{a=a CRstar e in V}
для каждого $a_i\in D$
существуют такие окрестности $V_i$,
что \[f'(V_1, ..., V_n)\subset U\]
\qed
\end{definition}

\begin{theorem}
Непрерывное отображение
\ShowEq{f:V->A}
топологического $D$\Hyph векторного пространства $V$
размерности $n$
в топологическое пространство $A$
непрерывна по совокупности аргументов.
\end{theorem}
\begin{proof}
Пусть
\ShowEq{b=f(a)}
и $U$ окрестность точки $b$.
Так как отображение $f$ непрерывно, то существует такая окрестность
$V$ вектора
\ShowEq{a=a CRstar e},
что $f(V)\subseteq U$.
Так как аддитивная операция непрерывна, то существуют такие окрестности
$E_i$ вектора $e_i$ и окрестности $W_i$
элемента $a_i\in D$, что $W\RCstar E\subset V$.
\end{proof}

\begin{definition}
\label{definition: norm on d vector space}
\AddIndex{Норма на $D$\Hyph векторном пространстве}
{norm on D vector space} $\Vector V$
над недискретным нормированным телом $D$\footnote{Определение
дано согласно
определению из \citeBib{Bourbaki: General Topology: Chapter 5 - 10},
гл. IX, \S 3, п${}^\circ$3} - это отображение
\ShowEq{norm on d vector space}
такое, что
\begin{itemize}
\ShowEq{|v| ge 0}
\item $\|v\|=0$ равносильно $v=0$
\ShowEq{|v+w|}
\ShowEq{|av|}
для всех $a\in D$ и $v\in V$
\end{itemize}

$D$\Hyph векторное пространство $V$
над недискретным нормированным телом $D$,
наделённое структурой, определяемой заданием на
$V$ нормы, называется
\AddIndex{нормированным $D$\Hyph векторным пространством}{normed D vector space}.
\qed
\end{definition}

Инвариантное расстояние на аддитивной группе
$D$\Hyph векторного пространства $V$
\ShowEq{Invariant distance}
определяет в $V$ топологию метрического пространства,
согласующуюся со структурой $D$\Hyph векторного пространства в $V$.

\begin{definition}
\label{definition: norm of map, D vector space}
Пусть $D$ - полное тело характеристики $0$.
Пусть
\ShowEq{f:V->W}
отображение нормированного $D$\hyph векторного пространства $V$ с нормой $\|x\|_1$
в нормированное $D$\hyph векторное пространство $W$ с нормой $\|y\|_2$.
Величина
\ShowEq{norm of map, D vector space}
называется
\AddIndex{нормой отображения}{norm of map} $f$.
\qed
\end{definition}

\section{Дифференцируемые отображения \texorpdfstring{$D$}{D}-векторного пространства}
\label{section: Differentiable maps of D Vector Space}

\begin{definition}
\label{definition: map differentiable in Gateaux sense, D vector space}
Отображение
\ShowEq{f:V->W}
нормированного $D$\Hyph векторного пространства $V$
с нормой $\|x\|_1$
в нормированное $D$\Hyph векторное пространство $W$
с нормой $\|x\|_2$\footnote{Если размерность $D$\Hyph векторного пространства $V$
равна $1$, то мы можем отождествить его с телом $D$. Тогда мы будем
говорить об отображении тела $D$ в $D$\Hyph векторное пространство $W$.
Если размерность $D$\Hyph векторного пространства $W$
равна $1$, то мы можем отождествить его с телом $D$. Тогда мы будем
говорить об отображении $D$\Hyph векторного пространства $V$ в тело $D$.
В обоих случаях мы будем опускать соответствующие индексы,
так как эти индексы имеют единственное значение.}
называется \AddIndex{дифференцируемой по Гато}
{map differentiable in Gateaux sense}
на множестве $U\subset V$,
если в каждой точке $x\in U$
изменение отображения $f$ может быть представлено в виде
\ShowEq{Gateaux derivative of map, D vector space, def}
\ShowEq{Gateaux derivative of map, D vector space}
где
\AddIndex{производная Гато
$\ShowSymbol{Gateaux derivative of map}$
отображения $f$}
{Gateaux derivative of map}
- линейное отображение приращения $a$ и
\ShowEq{o:V->W}
- такое непрерывное отображение, что
\ShowEq{o:V->W 1}
\qed
\end{definition}

\begin{remark}
\label{remark: differential L(D,V,W)}
Согласно определению
\ref{definition: map differentiable in Gateaux sense, D vector space}
при заданном $x$ производная Гато
\ShowEq{df in L(V,W)}
Следовательно, производная Гато отображения $f$ является отображением
\ShowEq{differential L(D,V,W)}
\qed
\end{remark}

\begin{theorem}
\label{theorem: map differentiable in Gateaux sense, D vector space}
Пусть $D$ - тело характеристики $0$.
Пусть $V$, $W$ - $D$\Hyph векторные пространства.
Допустим \eV V - базис в \dcr векторном пространстве $V$ и
\ShowEq{h in V}
Допустим \eV W - базис в \dcr векторном пространстве $W$.
Мы можем представить производную Гато
отображения $f$ в виде
\ShowEq{Gateaux differential of map, D vector space, representation}
\end{theorem}
\begin{proof}
Следствие определения
\ref{definition: map differentiable in Gateaux sense, D vector space}
и теоремы
\ePrints{0812.4763}
\ifx\Semafor\ValueOn
\ref{theorem: linear map, D vector space}.
\else
\xRef{0701.238}{theorem: linear map, D vector space}.
\fi
\end{proof}

\begin{definition}
Выражение
\ShowEq{component of Gateaux derivative of map, D vector space}
называется
\AddIndex{компонентой производной Гато}
{component of Gateaux derivative} отображения $f(x)$.
\qed
\end{definition}

\begin{theorem}
\label{theorem: Gateaux derivative over field F, D vector space}
Пусть полное тело $D$ характеристики $0$ является
алгеброй над полем $F\subset Z(D)$.
Производная Гато отображения
\ShowEq{f:V->W}
нормированного $D$\Hyph векторного пространства $V$
в нормированное $D$\Hyph векторное пространство $W$
удовлетворяет равенству
\ShowEq{Gateaux derivative over field F, D vector space}
\end{theorem}
\begin{proof}
Следствие определений
\ePrints{0812.4763}
\ifx\Semafor\ValueOn
\ref{definition: linear map, vector space},
\else
\xRef{0701.238}{definition: linear map, vector space},
\fi
\ref{definition: map differentiable in Gateaux sense, D vector space}.
\end{proof}

\begin{theorem}
\label{theorem: Gateaux derivative is multiplicative over field R, D vector space}
Пусть $D$ - полное тело характеристики $0$.
Производная Гато
функции
\ShowEq{f:V->W}
нормированного $D$\Hyph векторного пространства $V$
в нормированное $D$\Hyph векторное пространство $W$
удовлетворяет равенству
\ShowEq{Gateaux differential is multiplicative over field R, D vector space}
для любых $r\in R$, $r\ne 0$ и  $a\in V$, $a\ne 0$.
\end{theorem}
\begin{proof}
Следствие теорем
\ref{theorem: real subring of center},
\ePrints{0812.4763}
\ifx\Semafor\ValueOn
\ref{theorem: Gateaux derivative over field F, D vector space}.
\else
\xRef{0812.4763}{theorem: Gateaux derivative over field F, D vector space}.
\fi
\end{proof}

Комбинируя равенство
\EqRef{Gateaux differential is multiplicative over field R, D vector space}
и определение
\ref{definition: map differentiable in Gateaux sense, D vector space},
мы получим знакомое определение производной Гато
\ShowEq{Gateaux differential, D vector space, representation, 2}
Определения производной Гато
\EqRef{Gateaux derivative of map, D vector space}
и \EqRef{Gateaux differential, D vector space, representation, 2}
эквивалентны. На основе этой эквивалентности мы будем говорить,
что отображение $f$
дифференцируемо по Гато на множестве $U\subset D$,
если в каждой точке $x\in U$
изменение функции $f$ может быть представлено в виде
\ShowEq{Gateaux differential of map, t, D vector space}
где
\ShowEq{o:R->W}
- такое непрерывное отображение, что
\ShowEq{o:R->W 1}

Если бесконечно малая $a$ является дифференциалом $dx$,
то равенство
\EqRef{Gateaux differential of map, D vector space, representation}
становится определением
\AddIndex{дифференциала Гато}{Gateaux differential of map}
\ShowEq{Gateaux differential of map, D vector space}
\ShowEq{Gateaux differential of map, D vector space, form}

\begin{definition}
\label{definition: Gateaux partial derivative, D vector space}
\ShowEq{Gateaux partial derivative; D vector space}
Пусть $D$ - тело характеристики $0$.
Пусть $V$, $W$ - $D$\Hyph векторные пространства.
Допустим \eV V - базис в \dcr векторном пространстве $V$ и
\ShowEq{h in V}
Допустим \eV W - базис в \dcr векторном пространстве $W$.
Если мы рассмотрим производную Гато отображения $f$
по переменной $v^{\gi i}$ при условии, что остальные координаты вектора
$v$ постояны, то соответствующий аддитивный оператор
\ShowEq{Gateaux partial derivative, D vector space}
называется
\AddIndex{частной производной Гато}
{Gateaux partial derivative}
отображения $f^{\gi j}$
по переменной $v^{\gi i}$.
\qed
\end{definition}

\begin{theorem}
\label{theorem: expansion of Gateaux differential, D vector space}
Пусть $D$ - тело характеристики $0$.
Допустим \eV V - базис в $D$\Hyph векторном пространстве $V$ и
\ShowEq{h in V}
Допустим \eV W - базис в $D$\Hyph векторном пространстве $W$.
Пусть частные производные Гато отображения
\ShowEq{f:V->W}
непрерывны в области $U\in V$.
Тогда на множестве $U$ производная Гато отображения $f$
и частные производные Гато связаны соотношением
\ShowEq{expansion of Gateaux differential, D vector space}
\end{theorem}
\begin{proof}
Из теоремы
\ePrints{0812.4763}
\ifx\Semafor\ValueOn
\ref{theorem: partial linear map of variable}
\else
\xRef{0701.238}{theorem: partial linear map of variable}
\fi
следует, что мы можем разложить производную Гато отображения $f$
в сумму \EqRef{expansion of Gateaux differential, D vector space}
частных линейных отображений. Наша задача: выяснить, при каком условии
эти частные линейные отображения становятся частными производными Гато.

Согласно определению
\ref{eq: Gateaux differential, D vector space, representation, 2},
\ShowEq{expansion of Gateaux differential, D vector space, 1}
Из равенств \EqRef{Gateaux partial derivative, D vector space} и
\EqRef{expansion of Gateaux differential, D vector space, 1}
с точностью до бесконечно малой по сравнению с $t$ следует
\ShowEq{expansion of Gateaux differential, D vector space, 2}
Следовательно, для того, чтобы из равенства
\EqRef{expansion of Gateaux differential, D vector space, 2}
следовало равенство
\EqRef{expansion of Gateaux differential, D vector space},
необходимо, чтобы частные производные Гато были непрерывны.
\end{proof}

\begin{definition}
\label{definition: Gateaux dcr derivative of map, D vector space}
Пусть отображение
\ShowEq{f:V->W}
нормированного $D$\Hyph векторного пространства $V$
в нормированное $D$\Hyph векторное пространство $W$
дифференцируема по Гато на множестве $U\times W$.
Допустим мы выбрали базис \eV V
в \dcr векторном пространстве $V$.
Допустим мы выбрали базис \eV W
в \dcr векторном пространстве $W$.
\ShowEq{Gateaux dcr derivative of map}
\AddIndex{\dcr производная Гато
$\displaystyle\ShowSymbol{Gateaux dcr derivative of map, D vector space}$
отображения $f$}
{Gateaux dcr derivative of map, D vector space}
определена равенством
\ShowEq{Gateaux dcr derivative, D vector space}
Выражение $\displaystyle
\ShowSymbol{Gateaux partial dcr derivative of map, 2, D vector space}$
в равенстве
\EqRef{Gateaux dcr derivative, D vector space}
называется
\AddIndex{частными \dcr производными Гато отображения $f^{\gij}$
по переменной $x^{\gii}$}
{Gateaux partial dcr derivative of map with respect to variable, D vector space}.
\qed
\end{definition}

Для представления \dcr производной Гато
мы также будем пользоваться записью
\ShowEq{Gateaux dcr derivative 1, D vector space}

\begin{definition}
\label{definition: Gateaux rcd derivative of map, D vector space}
Пусть отображение
\ShowEq{f:V->W}
нормированного $D$\hyph векторного пространства $V$
в нормированное $D$\hyph векторное пространство $W$
дифференцируема по Гато на множестве $U\times W$.
Допустим мы выбрали базис \eV V
в \rcd векторном пространстве $V$.
Допустим мы выбрали базис \eV W
в \rcd векторном пространстве $W$.
\ShowEq{Gateaux rcd derivative of map}
\AddIndex{\rcd производная Гато
$\displaystyle\ShowSymbol{Gateaux rcd derivative of map, D vector space}$
отображения $f$}
{Gateaux rcd derivative of map, D vector space}
определена равенством
\ShowEq{Gateaux rcd derivative, D vector space}
Выражение $\displaystyle
\ShowSymbol{Gateaux partial rcd derivative of map, 2, D vector space}$
в равенстве
\EqRef{Gateaux rcd derivative, D vector space}
называется
\AddIndex{частными \rcd производными Гато отображения $f^{\gij}$
по переменной $x^{\gii}$}
{Gateaux partial rcd derivative of map with respect to variable, D vector space}.
\qed
\end{definition}

Для представления \rcd производной Гато
мы также будем пользоваться записью
\ShowEq{Gateaux rcd derivative 1, D vector space}

\ifx\texFuture\Defined
\begin{theorem}
\label{theorem: increment of diferentiable function, D vector space}
Пусть функция \[\Vector f:\Vector U\rightarrow\Vector V\]
нормированного $D$\Hyph векторного пространства $\Vector U$
в нормированное $D$\Hyph векторное пространство $\Vector V$
дифференцируема по Гато в точке
$\Vector x$.
Пусть единичная сфера нормированного $D$\Hyph векторного пространства $\Vector U$ - компактна.
Пусть $\Vector a$, $\Vector b\in\Vector U$,
$\|\Vector a\|_1=\|\Vector a\|_2=1$.
Тогда
\begin{equation}
\EqLabel{increment of diferentiable function, D vector space}
\|\Vector f(\Vector x+t\Vector a)-\Vector f(\Vector x+s\Vector b)\|_2
\le|t-s|\ \|\partial \Vector f\|
\end{equation}
\end{theorem}
\begin{proof}
Согласно определению
\EqRef{Gateaux derivative of map, D vector space}
\end{proof}
\fi

\begin{theorem}
\label{theorem: Gateaux differential, 0, D vector space}
Пусть $D$ - тело характеристики $0$.
Пусть функция
\ShowEq{f:U->V}
нормированного $D$\Hyph векторного пространства $U$
в нормированное $D$\Hyph векторное пространство $V$
дифференцируема по Гато в точке
$x$.
Тогда
\ShowEq{df(x)0=0}
\end{theorem}
\begin{proof}
Следствие определения
\ref{definition: map differentiable in Gateaux sense, D vector space}
и теоремы
\ePrints{0812.4763}
\ifx\Semafor\ValueOn
\ref{theorem: linear map, 0, D vector space}.
\else
\xRef{0701.238}{theorem: linear map, 0, D vector space}.
\fi
\end{proof}

\begin{theorem}
\label{theorem: composite map, differential, D vector space}
Пусть $D$ - тело характеристики $0$.
Пусть $U$ - нормированное $D$\Hyph векторное пространство с нормой $\|x\|_1$.
Пусть $V$ - нормированное $D$\Hyph векторное пространство с нормой $\|y\|_2$.
Пусть $W$ - нормированное $D$\Hyph векторное пространство с нормой $\|z\|_3$.
Пусть отображение
\ShowEq{f:U->V}
дифференцируемо по Гато в точке
$x$
и норма производной Гато отображения $f$
конечна
\ShowEq{composite map, norm f, D vector space}
Пусть отображение
\ShowEq{g:V->W}
дифференцируемо по Гато в точке
\ShowEq{composite map, y fx, D vector space}
и норма производной Гато отображения $g$
конечна
\ShowEq{composite map, norm g, D vector space}
Функция
\ShowEq{composite map, gfx, D vector space}
дифференцируема по Гато в точке
$x$
\ShowEq{composite map, differential, D vector space}
\ShowEq{composite map, Gateaux dcr derivative, D vector space}
\ShowEq{composite map, Gateaux dcr derivative 1, D vector space}
\ShowEq{composite map, Gateaux derivative 0, D vector space}
\ShowEq{composite map, Gateaux derivative 1, D vector space}
\end{theorem}
\begin{proof}
Согласно определению
\ref{definition: map differentiable in Gateaux sense, D vector space}
\ShowEq{Gateaux differential of map g, D vector space}
где
\ShowEq{o1:V->W}
- такое непрерывное отображение, что
\ShowEq{o1:V->W 1}
Согласно определению
\ref{definition: map differentiable in Gateaux sense, D vector space}
\ShowEq{Gateaux differential of map f, D vector space}
где
\ShowEq{o2:U->V}
- такое непрерывное отображение, что
\ShowEq{o2:U->V 1}
Согласно
\EqRef{Gateaux differential of map f, D vector space}
смещение вектора $x\in U$ в направлении $a$
приводит к смещению вектора
$y$
в направлении
\ShowEq{composite map, b fxa, D vector space}
Используя \EqRef{composite map, y fx, D vector space},
\EqRef{composite map, b fxa, D vector space}
в равенстве \EqRef{Gateaux differential of map g, D vector space},
мы получим
\ShowEq{Gateaux differential of map gf, 1, D vector space}
Согласно определениям
\ref{definition: map differentiable in Gateaux sense, D vector space},
\ePrints{0812.4763}
\ifx\Semafor\ValueOn
\ref{definition: linear map, vector space}
\else
\xRef{0701.238}{definition: linear map, vector space}
\fi
из равенства \EqRef{Gateaux differential of map gf, 1, D vector space}
следует
\ShowEq{Gateaux differential of map gf, 2, D vector space}
Найдём предел
\ShowEq{Gateaux differential of map gf, 2 1, D vector space}
Согласно определению \ref{definition: norm on d vector space}
\ShowEq{Gateaux differential of map gf, 3, D vector space}
Из \EqRef{composite map, norm g, D vector space}
следует
\ShowEq{Gateaux differential of map gf, 4, D vector space}
Из \EqRef{composite map, norm f, D vector space}
следует
\ShowEq{Gateaux differential of map gf, 5 1, D vector space}
Согласно теореме \ref{theorem: Gateaux differential, 0, D vector space}
\ShowEq{Gateaux differential of map gf, 5 2, D vector space}
Следовательно,
\ShowEq{Gateaux differential of map gf, 5, D vector space}
Из равенств
\EqRef{Gateaux differential of map gf, 3, D vector space},
\EqRef{Gateaux differential of map gf, 4, D vector space},
\EqRef{Gateaux differential of map gf, 5, D vector space}
следует
\ShowEq{Gateaux differential of map gf, 6, D vector space}
Согласно определению
\ref{definition: map differentiable in Gateaux sense, D vector space}
\ShowEq{Gateaux differential of map gf, 7, D vector space}
где
\ShowEq{o:U->W}
- такое непрерывное отображение, что
\ShowEq{o:U->W 1}
Равенство \EqRef{composite map, differential, D vector space}
следует из
\EqRef{Gateaux differential of map gf, 2, D vector space},
\EqRef{Gateaux differential of map gf, 6, D vector space},
\EqRef{Gateaux differential of map gf, 7, D vector space}.

Из равенства \EqRef{composite map, differential, D vector space}
и определения
\ref{definition: Gateaux dcr derivative of map, D vector space}
следует
\ShowEq{composite map, differential 1, D vector space}
Так как приращение $a$ произвольно, то равенство
\EqRef{composite map, Gateaux dcr derivative, D vector space}
следует из равенства
\EqRef{composite map, differential 1, D vector space}.

Из равенства \EqRef{composite map, differential, D vector space}
и теоремы
\ref{theorem: map differentiable in Gateaux sense, D vector space}
следует
\ShowEq{composite map, differential 2, D vector space}
\EqRef{composite map, Gateaux derivative 0, D vector space},
\EqRef{composite map, Gateaux derivative 1, D vector space}
следуют из равенства
\EqRef{composite map, differential 2, D vector space}.
\end{proof}


==> Index.English.tex <==
%auto-ignore
\OpenIndex
\SetIndexSpace%
\Index%1%1%1-form
   {$1$\Hyph form}%
   {1-form}%
\SetIndexSpace%
\Index%2%2%2- ary fibered relation
   {$2$\Hyph ary fibered relation}%
   {2 ary fibered relation}%
\SetIndexSpace%
\Index%819%A%A algebra of polynomials over D algebra
   {$A$\Hyph algebra of polynomials over $D$\Hyph algebra $A$}%
   {algebra of polynomials over algebra}%
\Index%693%A%A linear mapping of modules
   {$A$\Hyph linear mapping of modules}%
   {A linear map of modules}%
\Index%818%A%A number
   {$A$\Hyph number}%
   {A number}%
\Index%603%A%A(A) mapping
   {$\mathcal A(A)$\Hyph mapping}%
   {A(A) mapping}%
\Index%685%A%A- module
   {$A$\Hyph module}%
   {module over algebra}%
\Index%5%A%A- valued function
   {$A$\Hyph valued function}%
   {A valued function}%
\Index%645%A%Abelian Omega group
   {Abelian $\Omega$\Hyph group}%
   {Abelian Omega group}%
\Index%284%A%absolute value on division ring
   {absolute value on division ring}%
   {absolute value on division ring}%
\Index%680%A%Acr linear mapping of modules
   {\Acr linear mapping of modules}%
   {Acr linear map of modules}%
\Index%764%A%ACRcirc linear combination
   {$A\CRcirc$\Hyph linear combination}%
   {ACRcirc linear combination}%
\Index%100%A%active representation
   {active representation}%
   {active representation}%
\Index%569%A%active representation of group in basis manifold of representation
   {active representation of group $G(f)$ in basis manifold of representation}%
   {active representation in basis manifold}%
\Index%716%A%active representation of group in basis manifold of tower of representations
   {active representation of group $G(\Vector f)$ in basis manifold of tower of representations}%
   {active representation in basis manifold, tower of representations}%
\Index%99%A%active starT- representation
   {active \sT representation}%
   {active representation, vector space}%
\Index%326%A%active transformation of basis manifold of representation
   {active transformation of basis manifold of representation}%
   {active transformation of basis, representation}%
\Index%715%A%active transformation of basis manifold of tower of representations
   {active transformation of basis manifold of tower of representations}%
   {active transformation of basis, tower of representations}%
\Index%101%A%active transformation on basis manifold
   {active transformation on basis manifold}%
   {active transformation}%
\Index%102%A%active transformation on the set of rcd bases
   {active transformation on the set of \rcd bases}%
   {active transformation, vector space}%
\Index%805%A%additive map
   {additive map}%
   {additive map}%
\Index%110%A%affine basis
   {affine basis}%
   {Affine Basis}%
\Index%733%A%affine structure on set
   {affine structure on set}%
   {affine structure on set}%
\Index%141%A%affine transformation group
   {affine transformation group}%
   {drc affine transformation group}%
\Index%142%A%affine transformation group
   {affine transformation group}%
   {affine transformation group}%
\Index%109%A%affine transformation on basis manifold
   {affine transformation on basis manifold}%
   {affine transformation}%
\Index%400%A%algebra of fractions of algebra with conjugation
   {algebra of fractions of algebra with conjugation}%
   {algebra of fractions of algebra with conjugation}%
\Index%487%A%algebra of polynomials over D algebra
   {algebra of polynomials over $D$\Hyph algebra}%
   {algebra of polynomials over D algebra}%
\Index%618%A%algebra of rational mappings of algebra
   {algebra of rational mappings of algebra}%
   {algebra of rational mappings of algebra}%
\Index%797%A%algebra of sets
   {algebra of sets}%
   {algebra of sets}%
\Index%607%A%algebra over ring
   {algebra over ring}%
   {algebra over ring}%
\Index%780%A%algebra with conjugation
   {algebra with conjugation}%
   {algebra with conjugation}%
\Index%105%A%alternative representation of matrix
   {alternative representation of matrix}%
   {Alternative representation}%
\Index%275%A%anholonomic coordinate
   {anholonomic coordinate}%
   {anholonomic coordinate}%
\Index%278%A%anholonomic coordinates of connection
   {anholonomic coordinates of connection}%
   {anholonomic coordinates of connection}%
\Index%276%A%anholonomic coordinates of vector
   {anholonomic coordinates of vector}%
   {vector anholonomic coordinates}%
\Index%277%A%anholonomic coordinates on manifold
   {anholonomic coordinates on manifold}%
   {anholonomic coordinates on manifold}%
\Index%293%A%anholonomity object
   {anholonomity object}%
   {anholonomity object}%
\Index%106%A%antihomomorphism of fibered groups
   {antihomomorphism of fibered groups}%
   {antihomomorphism of fibered groups}%
\Index%107%A%antisymmetric 2- ary fibered relation
   {antisymmetric $2$\Hyph ary fibered relation}%
   {antisymmetric 2 ary fibered relation}%
\Index%582%A%Arc basis for vector space
   {$A\RCstar$\Hyph basis for vector space}%
   {Arc basis, vector space}%
\Index%108%A%arity of operation
   {arity of operation}%
   {arity of operation}%
\Index%617%A%associative D algebra
   {associative $D$\Hyph algebra}%
   {associative D algebra}%
\Index%585%A%associative law for Astar linear mappings of vector spaces
   {associative law for $A\star$\Hyph linear mappings of vector spaces}%
   {associative law for Astar linear mappings of vector spaces}%
\Index%662%A%associative law for Astar- module
   {associative law for $A\star$\Hyph module}%
   {associative law, Astar module over algebra}%
\Index%576%A%associative law for Astar- vector space
   {associative law for $A\star$\Hyph vector space}%
   {associative law, Astar vector space}%
\Index%165%A%associative law for covariant starT- representation
   {associative law for covariant \sT representation}%
   {associative law for covariant starT representation}%
\Index%166%A%associative law for covariant Tstar- representation
   {associative law for covariant \Ts representation}%
   {associative law for covariant Tstar representation}%
\Index%654%A%associative law for D- module
   {associative law for $D$\Hyph module}%
   {associative law, D module}%
\Index%162%A%associative law for Drc linear maps of vector bundles
   {associative law for \Drc linear maps of vector bundles}%
   {associative law for drc linear maps of vector bundles}%
\Index%164%A%associative law for Dstar- vector fields
   {associative law for $\mathcal D\star$\Hyph vector fields}%
   {associative law, Dstar vector fields}%
\Index%163%A%associative law for Dstar- vector space
   {associative law for $D\star$\Hyph vector space}%
   {associative law, Dstar vector space}%
\Index%161%A%associative law for rcd linear maps of vector spaces
   {associative law for \rcd linear maps of vector spaces}%
   {associative law for rcd linear maps of vector spaces}%
\Index%671%A%associative law for starA- module
   {associative law for $\star A$\Hyph module}%
   {associative law, starA module over algebra}%
\Index%501%A%associative law for starD- vector space
   {associative law for $\star D$\Hyph vector space}%
   {associative law, starD vector space}%
\Index%167%A%associative law for twin representations
   {associative law for twin representations}%
   {associative law for twin representations}%
\Index%168%A%associative law of composition of fibered correspondences
   {associative law of composition of fibered correspondences}%
   {associative law, composition of fibered correspondences}%
\Index%616%A%associator of D algebra
   {associator of $D$\Hyph algebra}%
   {associator of algebra}%
\Index%789%A%Astar antilinear mapping of algebra with conjugation
   {$A\star$\Hyph antilinear mapping of algebra with conjugation}%
   {antilinear mapping of algebra with conjugation}%
\Index%583%A%Astar linear map of vector spaces
   {$A\star$\Hyph linear map of vector spaces}%
   {Astar linear map of vector spaces}%
\Index%575%A%Astar vector space
   {$A\star$\Hyph vector space}%
   {Astar vector space}%
\Index%660%A%Astar- module
   {$A\star$\Hyph module}%
   {Astar-module}%
\Index%665%A%Astar- product of vector over scalar
   {$A\star$\Hyph product of vector over scalar}%
   {Astar product of vector over scalar, Astar module}%
\Index%579%A%Astar-product of vector over scalar
   {$A\star$\hyph product of vector over scalar}%
   {Astar product of vector over scalar, vector space}%
\Index%95%A%auto parallel line
   {auto parallel line}%
   {auto parallel line}%
\Index%94%A%automorphism of representation of Omega algebra
   {automorphism of representation of $\Omega$\Hyph algebra}%
   {automorphism of representation}%
\Index%560%A%automorphism of tower of representations
   {automorphism of tower of representations}%
   {automorphism of tower of representations}%
\Index%3%A%j i-CR quasideterminant
   {$(^j_i)$\hyph \CR quasideterminant}%
   {j i cr-quasideterminant}%
\Index%282%A%norm of quaternion
   {norm of quaternion}%
   {norm of quaternion}%
\SetIndexSpace%
\Index%799%B%b set
   {$B$\Hyph set}%
   {B set}%
\Index%503%B%Banach D- algebra
   {Banach $D$\Hyph algebra}%
   {Banach algebra}%
\Index%313%B%Banach D- module
   {Banach $D$\Hyph module}%
   {Banach module}%
\Index%114%B%base of fibered correspondence
   {base of fibered correspondence}%
   {base of fibered correspondence}%
\Index%113%B%base of mapping
   {base of mapping}%
   {base of map}%
\Index%49%B%basis dual to basis
   {basis dual to basis}%
   {basis dual to basis}%
\Index%223%B%basis dual to basis
   {basis dual to basis}%
   {dual basis}%
\Index%25%B%basis for c rows rcd vector space
   {basis for \sups rows \rcd vector space}%
   {basis, c rows rcd vector space}%
\Index%197%B%basis for D vector space
   {basis for $D$\Hyph vector space}%
   {basis, D vector space}%
\Index%659%B%basis for module
   {basis for module}%
   {basis, module}%
\Index%24%B%basis for rcd vector space
   {basis for \rcd vector space}%
   {basis, rcd vector space}%
\Index%256%B%basis manifold of affine space
   {basis manifold of affine space}%
   {Basis Manifold, Affine Space}%
\Index%261%B%basis manifold of central affine space
   {basis manifold of central affine space}%
   {Basis Manifold, Central Affine Space, division ring}%
\Index%262%B%basis manifold of central affine space
   {basis manifold of central affine space}%
   {Basis Manifold, Central Affine Space}%
\Index%259%B%basis manifold of Euclid space
   {basis manifold of Euclid space}%
   {Basis Manifold, Euclid Space}%
\Index%260%B%basis manifold of Euclid space
   {basis manifold of Euclid space}%
   {Basis Manifold, Euclid Space, division ring}%
\Index%257%B%basis manifold of rcd affine space
   {basis manifold of \rcd affine space}%
   {Basis Manifold, rcd Affine Space, division ring}%
\Index%255%B%basis manifold of rcd vector space
   {basis manifold of \rcd vector space}%
   {basis manifold of rcd vector space}%
\Index%536%B%basis manifold of representation
   {basis manifold of representation}%
   {basis manifold representation F algebra}%
\Index%714%B%basis manifold of tower of representations
   {basis manifold of tower of representations}%
   {basis manifold tower of representations}%
\Index%258%B%basis manifold of vector space
   {basis manifold of vector space}%
   {basis manifold of vector space}%
\Index%653%B%basis of algebra L(A,A)
   {basis of algebra $\mathcal L(A;A)$}%
   {basis of algebra L(A,A)}%
\Index%16%B%basis of r rows drc vector space
   {basis of \subs rows \drc vector space}%
   {basis, r rows drc vector space}%
\Index%329%B%basis of representation
   {basis of representation}%
   {basis of representation}%
\Index%567%B%basis of tower of representations
   {basis of tower of representations}%
   {basis of tower of representations}%
\Index%115%B%basis of vector space
   {basis of vector space}%
   {Basis}%
\Index%117%B%basis vector of representation of Lie group
   {basis vector of representation of Lie group}%
   {basis vector of representation of Lie group}%
\Index%116%B%basis vector of representation of Lie group over algebra A
   {basis vector of representation of Lie group over algebra $A$}%
   {basis vector of representation of Lie group over algebra A}%
\Index%122%B%biring
   {biring}%
   {biring}%
\Index%808%B%Borel algebra
   {Borel algebra}%
   {Borel algebra}%
\Index%798%B%borel set
   {Borel set}%
   {Borel set}%
\Index%803%B%Borel-measurable map
   {Borel\Hyph measurable map}%
   {Borel-measurable map}%
\Index%419%B%bundle of level 2
   {bundle of level $2$}%
   {bundle of level 2}%
\Index%418%B%bundle of level n
   {bundle of level $n$}%
   {bundle of level n}%
\SetIndexSpace%
\Index%6%C%c row of matrix
   {\subs row of matrix}%
   {c row}%
\Index%29%C%c rows rcd vector space
   {\sups rows \rcd vector space}%
   {sups rows rcd vector space}%
\Index%12%C%c-row of matrix
   {$c$\hyph row of matrix}%
   {c-row}%
\Index%443%C%Cartan connection
   {Cartan connection}%
   {Cartan connection}%
\Index%227%C%Cartan curvature
   {Cartan curvature}%
   {Cartan curvature}%
\Index%401%C%Cartan derivative
   {Cartan derivative}%
   {Cartan derivative}%
\Index%444%C%Cartan symbol
   {Cartan symbol}%
   {Cartan symbol}%
\Index%338%C%Cartan transport
   {Cartan transport}%
   {Cartan transport}%
\Index%149%C%Cartesian power A of bundle B
   {Cartesian power $\Bundle A$ of bundle $\Bundle B$}%
   {Cartesian power A of bundle B}%
\Index%148%C%Cartesian power A of set B
   {Cartesian power $A$ of set $B$}%
   {Cartesian power of set}%
\Index%150%C%Cartesian power n of bundle E
   {Cartesian power $n$ of bundle $\Bundle E$}%
   {Cartesian power n of bundle E}%
\Index%594%C%Cartesian power n of H algebra
   {Cartesian power $n$ of $\mathfrak{H}$\Hyph algebra}%
   {Cartesian power of algebra}%
\Index%175%C%category of drc vector spaces
   {category of \drc vector spaces}%
   {category of drc vector spaces}%
\Index%179%C%category of fibered correspondences over diagonal
   {category of fibered correspondences over diagonal}%
   {category of fibered correspondences over diagonal}%
\Index%178%C%category of reduced fibered correspondences
   {category of reduced fibered correspondences}%
   {category of reduced fibered correspondences}%
\Index%176%C%category of Tstar- representations of Omega1 algebra A
   {category of \Ts representations of $\Omega_1$\Hyph algebra $A$}%
   {category of Tstar representations of Omega1 algebra}%
\Index%177%C%category of Tstar- representations of Omega1 algebra from category A
   {category of \Ts representations of $\Omega_1$\Hyph algebra from category $\mathcal A$}%
   {category of Tstar representations of Omega1 algebra from category}%
\Index%241%C%Cauchy sequence
   {Cauchy sequence}%
   {Cauchy sequence}%
\Index%620%C%center of algebra
   {center of $D$\Hyph algebra $A$}%
   {center of algebra}%
\Index%507%C%center of ring D
   {center of ring $D$}%
   {center of ring}%
\Index%508%C%central affine basis
   {central affine basis}%
   {Central Affine Basis, division ring}%
\Index%509%C%central affine basis
   {central affine basis}%
   {Central Affine Basis}%
\Index%807%C%closed ball
   {closed ball}%
   {closed ball}%
\Index%750%C%column determinant
   {column determinant}%
   {column determinant}%
\Index%124%C%column vector
   {column vector}%
   {column vector}%
\Index%615%C%commutative D algebra
   {commutative $D$\Hyph algebra}%
   {commutative D algebra}%
\Index%190%C%commutative diagram of correspondences
   {commutative diagram of correspondences}%
   {commutative diagram of correspondences}%
\Index%614%C%commutator of D algebra
   {commutator of $D$\Hyph algebra}%
   {commutator of algebra}%
\Index%815%C%compact set
   {compact set}%
   {compact set}%
\Index%191%C%compact-open topology
   {compact\hyph open topology}%
   {compact open topology}%
\Index%349%C%complete division ring
   {complete division ring}%
   {complete division ring}%
\Index%811%C%complete normed Omega group
   {complete normed $\Omega$\Hyph group}%
   {complete Omega group}%
\Index%270%C%complete ring
   {complete ring}%
   {complete ring}%
\Index%348%C%complete system of linear partial differential equations
   {complete system of linear partial differential equations}%
   {Complete System of Linear Partial Differential Equations}%
\Index%128%C%completely integrable system
   {completely integrable system}%
   {completely integrable system}%
\Index%193%C%component of linear map
   {component of linear map}%
   {component of linear map}%
\Index%647%C%component of polylinear map
   {component of polylinear map}%
   {component of polylinear map}%
\Index%629%C%component of the Gateaux derivative
   {component of the G\^ateaux derivative}%
   {component of Gateaux derivative}%
\Index%633%C%component of the Gateaux derivative of second order
   {component of the G\^ateaux derivative of second order}%
   {component of Gateaux derivative of Second Order}%
\Index%394%C%composition of fibered correspondences
   {composition of fibered correspondences}%
   {composition of fibered correspondences}%
\Index%393%C%composition of reduced fibered correspondences
   {composition of reduced fibered correspondences}%
   {composition of reduced fibered correspondences}%
\Index%495%C%condition of reducibility of products
   {condition of reducibility of products}%
   {condition of reducibility of products}%
\Index%746%C%conjugate of quaternion
   {conjugate of quaternion $x$}%
   {conjugate of quaternion}%
\Index%580%C%conjugated D module
   {conjugated $D$\Hyph  module}%
   {conjugated D module}%
\Index%788%C%conjugation in algebra
   {conjugation in algebra}%
   {conjugation in algebra}%
\Index%777%C%conjugation in ring
   {conjugation in ring}%
   {conjugation in ring}%
\Index%538%C%connection coefficients in D affine space
   {connection coefficients in $D$\Hyph affine space}%
   {connection coefficients, D affine space}%
\Index%668%C%continues basis
   {continues basis}%
   {continues basis}%
\Index%281%C%continuous correspondence
   {continuous correspondence}%
   {continuous correspondence}%
\Index%280%C%continuous map
   {continuous map}%
   {continuous map}%
\Index%610%C%continuous multivariable map
   {continuous multivariable map}%
   {continuous multivariable map}%
\Index%200%C%contravariant starT- representation of fibered group
   {contravariant \sT representation of fibered group}%
   {contravariant starT representation of fibered group}%
\Index%202%C%contravariant starT- representation of group
   {contravariant \sT representation of group}%
   {contravariant starT representation of group}%
\Index%203%C%contravariant Tstar- representation of fibered group
   {contravariant \Ts representation of fibered group}%
   {contravariant Tstar representation of fibered group}%
\Index%201%C%contravariant Tstar- representation of group
   {contravariant \Ts representation of group}%
   {contravariant Tstar representation of group}%
\Index%210%C%coordinate Drc vector bundle
   {coordinate \Drc vector bundle}%
   {coordinate drc vector bundle}%
\Index%215%C%coordinate isomorphism
   {coordinate isomorphism}%
   {coordinate isomorphism}%
\Index%206%C%coordinate matrix of set of vectors
   {coordinate matrix of set of vectors}%
   {coordinate matrix of set of vectors}%
\Index%691%C%coordinate matrix of vector
   {coordinate matrix of vector}%
   {coordinate matrix of vector}%
\Index%205%C%coordinate matrix of vector field in rcD basis
   {coordinate matrix of vector field in \rcD basis}%
   {coordinate matrix of vector field in drc basis}%
\Index%214%C%coordinate rcd isomorphism
   {coordinate \rcd isomorphism}%
   {coordinate rcd isomorphism}%
\Index%209%C%coordinate rcd vector space
   {coordinate \rcd vector space}%
   {coordinate rcd vector space}%
\Index%208%C%coordinate reference frame
   {coordinate reference frame}%
   {coordinate reference frame}%
\Index%697%C%coordinate representation in Omega_2- algebra
   {coordinate representation in $\Omega_2$\Hyph algebra}%
   {coordinate representation, Omega_2 algebra}%
\Index%212%C%coordinate representation in rcd vector space
   {coordinate representation in \rcd vector space}%
   {coordinate representation, rcd vector space}%
\Index%720%C%coordinate representation in tuple of Omega- algebras
   {coordinate representation in tuple of $\VX\Omega$\Hyph algebras}%
   {coordinate tower of representations, Omega algebra}%
\Index%213%C%coordinate representation of group in vector space
   {coordinate representation of group in vector space}%
   {coordinate representation, vector space}%
\Index%211%C%coordinate vector space
   {coordinate vector space}%
   {coordinate vector space}%
\Index%701%C%coordinates of a geometric object in Omega_2- algebra
   {coordinates of a geometric object in $\Omega_2$\Hyph algebra $M$}%
   {coordinates of geometric object, representation g}%
\Index%723%C%coordinates of a geometric object in tuple of Omega- algebras
   {coordinates of a geometric object in tuple of $\VX\Omega$\Hyph algebras}%
   {coordinates of geometric object, tower of representations g}%
\Index%325%C%coordinates of basis of representation
   {coordinates of basis of representation}%
   {coordinates of basis relative to basis, representation}%
\Index%558%C%coordinates of element of representation relative to set
   {coordinates of element $m$ of representation $f$ relative to set $X$}%
   {coordinates of element relative to set, representation}%
\Index%696%C%coordinates of endomorphism of representation
   {coordinates of endomorphism of representation}%
   {coordinates of endomorphism, representation}%
\Index%711%C%coordinates of endomorphism of tower of representations
   {coordinates of endomorphism of tower of representations}%
   {coordinates of endomorphism, tower of representations}%
\Index%218%C%coordinates of geometric object
   {coordinates of geometric object}%
   {coordinates of geometric object, vector space}%
\Index%220%C%coordinates of geometric object in coordinate rcd vector space
   {coordinates of geometric object in coordinate \rcd vector space}%
   {coordinates of geometric object, coordinate rcd vector space}%
\Index%221%C%coordinates of geometric object in coordinate representation
   {coordinates of geometric object in coordinate representation}%
   {coordinates of geometric object, coordinate vector space}%
\Index%699%C%coordinates of geometric object in coordinate space of representation
   {coordinates of geometric object in coordinate space of representation}%
   {coordinates of geometric object, coordinate representation}%
\Index%721%C%coordinates of geometric object in coordinate space of tower of representations
   {coordinates of geometric object in coordinate space of tower of representations}%
   {coordinates of geometric object, coordinate tower of representations}%
\Index%219%C%coordinates of geometric object in rcd vector space
   {coordinates of geometric object in \rcd vector space}%
   {coordinates of geometric object, rcd vector space}%
\Index%730%C%coordinates of point of affine space relative to basis)$
   {coordinates of point $A$ of affine space $\overset{\circ}{A}$ relative to basis $(O,\Basis e)$}%
   {coordinates in affine space}%
\Index%737%C%coordinates of point of rcd affine space relative to basis
   {coordinates of point of \rcd affine space relative to basis}%
   {coordinates in rcd affine space}%
\Index%224%C%coordinates of representation
   {coordinates of representation}%
   {coordinates of representation, drc vector space}%
\Index%225%C%coordinates of representation
   {coordinates of representation}%
   {coordinates of representation}%
\Index%222%C%coordinates of set of vectors
   {coordinates of set of vectors}%
   {coordinates of set of vectors}%
\Index%216%C%coordinates of vector
   {coordinates of vector}%
   {coordinates of vector}%
\Index%217%C%coordinates of vector field in Drc basis
   {coordinates of vector field in \Drc basis}%
   {coordinates of vector field in drc basis}%
\Index%286%C%coordinates of vector relative to Hamel basis
   {coordinates of vector relative to Hamel basis}%
   {coordinates of vector, Hamel basis}%
\Index%676%C%coordinates of vector relative to Schauder basis
   {coordinates of vector relative to Schauder basis}%
   {coordinates of vector, Schauder basis}%
\Index%455%C%correspondence continuous on the set
   {correspondence continuous on the set}%
   {correspondence continuous on the set}%
\Index%454%C%correspondence of homomorphism
   {correspondence of homomorphism}%
   {correspondence of homomorphism}%
\Index%185%C%covariant starT- representation of fibered group
   {covariant \sT representation of fibered group}%
   {covariant starT representation of fibered group}%
\Index%184%C%covariant starT- representation of group
   {covariant \sT representation of group}%
   {covariant starT representation of group}%
\Index%187%C%covariant Tstar- representation of fibered group
   {covariant \Ts representation of fibered group}%
   {covariant Tstar representation of fibered group}%
\Index%186%C%covariant Tstar- representation of group
   {covariant \Ts representation of group}%
   {covariant Tstar representation of group}%
\Index%8%C%CR inverse element of biring
   {\CR inverse element of biring}%
   {cr-inverse element}%
\Index%7%C%CR matrix group
   {\CR matrix group}%
   {cr-matrix group}%
\Index%10%C%CR power
   {\CR power}%
   {cr power}%
\Index%9%C%CR product of matrices
   {\CR product of matrices}%
   {cr-product of matrices}%
\Index%589%C%cr product of matrices of mappings
   {$\CRcirc$\Hyph product of matrices of mappings}%
   {cr product of matrices of mappings}%
\Index%11%C%crd vector space
   {\crd vector space}%
   {crd vector space}%
\Index%768%C%Cstar-algebra
   {$C^*$\Hyph algebra}%
   {Cstar-algebra}%
\Index%537%C%curvilinear coordinates of point in affine space
   {curvilinear coordinates of point in affine space}%
   {curvilinear coordinates of point in affine space}%
\Index%19%C%r rows drc vector space
   {\subs rows \drc vector space}%
   {subs rows drc vector space}%
\SetIndexSpace%
\Index%23%D%d affine space
   {$D$\Hyph affine space}%
   {d affine space}%
\Index%581%D%D linear functional
   {$D$\Hyph linear functional}%
   {D linear functional}%
\Index%549%D%D- affine connection on manifold with affine connections
   {$D$\Hyph affine connection on manifold with affine connections}%
   {D affine connection, affine manifold}%
\Index%251%D%D- algebra
   {$D$\Hyph algebra}%
   {D algebra}%
\Index%71%D%D- module
   {$D$\Hyph module}%
   {D-module}%
\Index%584%D%D- module
   {$D$\Hyph module}%
   {D module}%
\Index%48%D%D- valued variable
   {$D$\Hyph valued variable}%
   {D valued variable}%
\Index%14%D%D- vector function
   {$D$\Hyph vector function}%
   {d vector function}%
\Index%550%D%D-affine connection coefficients on manifold
   {$D$\Hyph affine connection coefficients on manifold}%
   {D affine connection coefficients, manifold}%
\Index%15%D%D-vector space
   {$D$\hyph vector space}%
   {D vector space}%
\Index%18%D%dcr vector space
   {\dcr vector space}%
   {dcr vector space}%
\Index%303%D%determinant of matrix
   {determinant of matrix}%
   {determinant}%
\Index%309%D%deviation of trajectories
   {deviation of trajectories}%
   {deviation of trajectories}%
\Index%153%D%diagonal in bundle
   {diagonal in bundle}%
   {diagonal in bundle}%
\Index%154%D%diagram of correspondences
   {diagram of correspondences}%
   {diagram of correspondences}%
\Index%725%D%diagram of representations
   {diagram of representations}%
   {diagram of representations}%
\Index%417%D%dimension of rcd vector space
   {dimension of \rcd vector space}%
   {dimension of vector space}%
\Index%151%D%direct product of bundles
   {direct product of bundles}%
   {Cartesian product of bundles}%
\Index%410%D%direct product of D- vector spaces
   {direct product of $D$\Hyph vector spaces}%
   {direct product of D vector spaces}%
\Index%415%D%direct product of division rings
   {direct product of division rings}%
   {direct product of division rings}%
\Index%411%D%direct product of rcd vector spaces
   {direct product of \rcd vector spaces}%
   {direct product, rcd vector space}%
\Index%414%D%direct product of representations of fibered group
   {direct product of representations of fibered group}%
   {direct product of representations of fibered group}%
\Index%413%D%direct product of representations of group
   {direct product of representations of group}%
   {direct product of representations of group}%
\Index%152%D%direct product of total spaces
   {direct product of total spaces}%
   {Cartesian product of total spaces}%
\Index%412%D%direct product of Tstar- representations of group
   {direct product of \Ts representations of group}%
   {direct product of Tstar representations of group}%
\Index%409%D%direct sum of representations
   {direct sum of representations}%
   {direct sum of representations}%
\Index%763%D%direction over commutative ring
   {direction over commutative ring}%
   {direction over commutative ring}%
\Index%663%D%distributive law for Astar- module
   {distributive law for $A\star$\Hyph module}%
   {distributive law, Astar module over algebra}%
\Index%577%D%distributive law for Astar- vector space
   {distributive law for $A\star$\Hyph vector space}%
   {distributive law, Astar vector space}%
\Index%655%D%distributive law for D- module
   {distributive law for $D$\Hyph module}%
   {distributive law, D module}%
\Index%170%D%distributive law for Dstar- vector fields
   {distributive law for $\mathcal D\star$\Hyph vector fields}%
   {distributive law, Dstar vector fields}%
\Index%169%D%distributive law for Dstar- vector space
   {distributive law for $D\star$\Hyph vector space}%
   {distributive law, Dstar vector space}%
\Index%672%D%distributive law for starA- module
   {distributive law for $\star A$\Hyph module}%
   {distributive law, starA module over algebra}%
\Index%625%D%distributive law for starD- vector space
   {distributive law for $\star D$\Hyph vector space}%
   {distributive law, starD vector space}%
\Index%820%D%divisor of polynomial
   {divisor of polynomial}%
   {divisor of polynomial}%
\Index%755%D%double determinant
   {double determinant}%
   {double determinant}%
\Index%26%D%Drc basis for vector  bundle
   {\Drc basis for vector  bundle}%
   {drc basis, vector bundle}%
\Index%36%D%Drc linear map of vector bundles
   {\Drc linear map of vector bundles}%
   {drc linear map of vector bundles}%
\Index%70%D%drc representation of group
   {\drc representation of group}%
   {drc linear representation of group}%
\Index%17%D%drc vector
   {\drc vector}%
   {drc vector}%
\Index%28%D%drc vector space
   {\drc vector space}%
   {drc vector space}%
\Index%734%D%Dstar affine space
   {$D\star$\Hyph affine space}%
   {Dstar affine space}%
\Index%771%D%Dstar antilinear homomorphism
   {$D\star$\Hyph antilinear homomorphism}%
   {Dstar antilinear homomorphism}%
\Index%779%D%Dstar antilinear mapping of ring with conjugation
   {$D\star$\Hyph antilinear mapping of ring with conjugation}%
   {antilinear mapping of ring with conjugation}%
\Index%769%D%Dstar linear homomorphism
   {$D\star$\Hyph linear homomorphism}%
   {Dstar linear homomorphism}%
\Index%41%D%Dstar- vector bundle
   {$\mathcal D\star$\Hyph vector bundle}%
   {Dstar vector bundle}%
\Index%39%D%Dstar- vector field
   {$\mathcal D\star$\Hyph vector field}%
   {Dstar vector field}%
\Index%40%D%Dstar- vector space
   {$D\star$\hyph  vector space}%
   {Dstar vector space}%
\Index%43%D%Dstar-linear composition of vector fields
   {$\mathcal D\star$\hyph linear composition of vector fields}%
   {linear composition of vector fields}%
\Index%156%D%Dstar-module
   {$D\star$\Hyph module}%
   {Dstar-module}%
\Index%45%D%Dstar-product of vector field over scalar
   {$\mathcal D\star$\hyph product of vector field over scalar}%
   {Dstar product of vector field over scalar, vector space}%
\Index%44%D%Dstar-product of vector over scalar
   {$D\star$\hyph product of vector over scalar}%
   {Dstar product of vector over scalar, vector space}%
\Index%159%D%dual space of rcd vector space
   {dual space of \rcd vector space}%
   {dual space of rcd vector space}%
\Index%382%D%duality principle for biring
   {duality principle for biring}%
   {duality principle for biring}%
\Index%383%D%duality principle for biring of matrices
   {duality principle for biring of matrices}%
   {duality principle for biring of matrices}%
\Index%32%D%rcd linear span in vector space
   {\rcd linear span in vector space}%
   {linear span, vector space}%
\SetIndexSpace%
\Index%521%E%effective representation of division ring
   {effective representation of division ring}%
   {effective representation of division ring}%
\Index%519%E%effective representation of fibered Omega- algebra
   {effective representation of fibered $\Omega$\Hyph algebra}%
   {effective representation of fibered Omega-algebra}%
\Index%518%E%effective representation of group
   {effective representation of group}%
   {effective representation of group}%
\Index%517%E%effective representation of Omega- algebra A
   {effective representation of $\Omega$\Hyph algebra $A$}%
   {effective representation of algebra}%
\Index%622%E%effective representation of ring
   {effective representation of ring}%
   {effective representation of ring}%
\Index%500%E%effective Tstar representation of Omega- algebra A
   {effective \Ts representation of $\Omega$\Hyph algebra $A$}%
   {effective Tstar representation of algebra}%
\Index%514%E%effective Tstar- representation of fibered division ring
   {effective \Ts representation of fibered division ring}%
   {effective representation of fibered division ring}%
\Index%520%E%effective Tstar- representation of fibered group
   {effective \Ts representation of fibered group}%
   {effective representation of fibered group}%
\Index%516%E%effective Tstar- representation of group
   {effective \Ts representation of group}%
   {effective Tstar representation of group}%
\Index%557%E%endomorphism of representation of Omega algebra
   {endomorphism of representation of $\Omega$\Hyph algebra}%
   {endomorphism of representation}%
\Index%327%E%endomorphism of representation regular on generating set X
   {endomorphism of representation regular on generating set $X$}%
   {endomorphism of representation, regular on set}%
\Index%328%E%endomorphism of representation singular on generating set X
   {endomorphism of representation singular on generating set $X$}%
   {endomorphism of representation, singular on set}%
\Index%559%E%endomorphism of tower of representations
   {endomorphism of tower of representations}%
   {endomorphism of tower of representations}%
\Index%564%E%endomorphism of tower of representations regular on tuple of generating sets
   {endomorphism of tower of representations regular on tuple of generating sets}%
   {endomorphism of representation, regular on tuple}%
\Index%565%E%endomorphism of tower of representations singular on tuple of generating sets
   {endomorphism of tower of representations singular on tuple of generating sets}%
   {endomorphism of representation, singular on tuple}%
\Index%50%E%enhanced Lie group
   {enhanced Lie group}%
   {enhanced Lie group}%
\Index%706%E%equivalence generated by representation
   {equivalence generated by representation $f$}%
   {equivalence of representation}%
\Index%51%E%essential parameters in a set of functions
   {essential parameters in a set of functions}%
   {essential parameters}%
\Index%539%E%Euclidean metric on division ring
   {Euclidean metric on division ring}%
   {Euclidean metric on division ring}%
\Index%547%E%Euclidean scalar product in D- vector space
   {Euclidean scalar product in $D$\Hyph vector space}%
   {Euclidean scalar product, vector space}%
\Index%542%E%Euclidean scalar product on division ring
   {Euclidean scalar product on division ring}%
   {Euclidean scalar product on division ring}%
\Index%204%E%expansion of vector relative to basis converges
   {expansion of vector relative to basis converges}%
   {expansion converges}%
\Index%621%E%expansion of vector relative to basis converges normally
   {expansion of vector relative to basis converges normally}%
   {expansion converges normally}%
\Index%437%E%extended matrix of drc linear equations
   {extended matrix of \drc linear equations}%
   {extended matrix, system of drc linear equations}%
\Index%438%E%extended matrix of rcd linear equations
   {extended matrix of \rcd linear equations}%
   {extended matrix, system of rcd linear equations}%
\Index%386%E%extension of correspondence
   {extension of correspondence}%
   {extension of correspondence}%
\Index%515%E%extreme line
   {extreme line}%
   {extreme line}%
\SetIndexSpace%
\Index%434%F%fibered coordinate Drc isomorphism
   {fibered coordinate \Drc isomorphism}%
   {fibered coordinate drc isomorphism}%
\Index%432%F%fibered correspondence from A to B
   {fibered correspondence from $\Bundle A$ to $\Bundle B$}%
   {fibered correspondence from A to B}%
\Index%430%F%fibered correspondence in A
   {fibered correspondence in $\Bundle{A}$}%
   {fibered correspondence in A}%
\Index%431%F%fibered correspondence of homomorphism
   {fibered correspondence of homomorphism}%
   {fibered correspondence of homomorphism}%
\Index%427%F%fibered equivalence
   {fibered equivalence}%
   {fibered equivalence}%
\Index%422%F%fibered group
   {fibered group}%
   {fibered group}%
\Index%436%F%fibered identification morphism
   {fibered identification morphism}%
   {fibered identification morphism}%
\Index%424%F%fibered little group
   {fibered little group}%
   {fibered little group}%
\Index%435%F%fibered morphism from bundle A into B
   {fibered morphism from bundle $\Bundle A$ into $\Bundle B$}%
   {fibered morphism from A into B}%
\Index%433%F%fibered natural morphism
   {fibered natural morphism}%
   {fibered natural morphism}%
\Index%420%F%fibered Omega- algebra
   {fibered $\Omega$\Hyph algebra}%
   {fibered Omega-algebra}%
\Index%421%F%fibered Omega- subalgebra
   {fibered $\Omega$\Hyph subalgebra}%
   {fibered Omega-subalgebra}%
\Index%426%F%fibered ordering
   {fibered ordering}%
   {fibered ordering}%
\Index%425%F%fibered preordering
   {fibered preordering}%
   {fibered preordering}%
\Index%428%F%fibered ring
   {fibered ring}%
   {fibered ring}%
\Index%423%F%fibered stability group
   {fibered stability group}%
   {fibered stability group}%
\Index%429%F%fibered subset
   {fibered subset}%
   {fibered subset}%
\Index%479%F%field-strength tensor
   {field-strength tensor}%
   {field-strength tensor}%
\Index%497%F%filter F converges to A
   {filter $\mathfrak{F}$ converges to $A$}%
   {filter converges}%
\Index%131%F%Finsler metric
   {Finsler metric}%
   {Finsler metric}%
\Index%77%F%Finsler space
   {Finsler space}%
   {Finsler space}%
\Index%574%F%Finsler structure
   {Finsler structure}%
   {Finsler structure}%
\Index%337%F%first Newton law
   {first Newton law}%
   {First Newton law}%
\Index%690%F%free A- module
   {free $A$\Hyph module}%
   {free A module}%
\Index%606%F%free algebra over ring
   {free algebra over ring}%
   {free algebra over ring}%
\Index%612%F%free module over ring
   {free module over ring}%
   {free module over ring}%
\Index%442%F%free Tstar- representation of fibered group
   {free \Ts representation of fibered group}%
   {free representation of fibered group}%
\Index%441%F%free Tstar- representation of group
   {free \Ts representation of group}%
   {free representation of group}%
\Index%339%F%Frenet transport
   {Frenet transport}%
   {Frenet transport}%
\Index%155%F%function homogeneous of degree
   {function homogeneous of degree $k$}%
   {function homogeneous}%
\Index%504%F%function of division ring Dstar differentiable in the Fr\'echet sense
   {function of division ring \Ds differentiable in the Fr\'echet sense}%
   {function Dstar differentiable in Frechet sense, division ring}%
\Index%243%F%fundamental sequence
   {fundamental sequence}%
   {fundamental sequence}%
\SetIndexSpace%
\Index%52%G%G- reference frame
   {$G$\Hyph reference frame}%
   {G reference frame}%
\Index%53%G%G-basis of vector space
   {$G$\Hyph basis of vector space}%
   {G-basis}%
\Index%54%G%G-coordinates of basis
   {$G$\Hyph coordinates of basis}%
   {G-coordinates}%
\Index%55%G%G-space
   {$G$\Hyph space}%
   {GSpace}%
\Index%38%G%Gateaux dcr derivative of map of D- vector space V to D- vector space W
   {the G\^ateaux \dcr derivative of map $f$ of $D$\Hyph vector space $V$ to $D$\Hyph vector space $W$}%
   {Gateaux dcr derivative of map, D vector space}%
\Index%627%G%Gateaux derivative of map
   {the G\^ateaux derivative of map}%
   {Gateaux derivative of map}%
\Index%399%G%Gateaux derivative of order n
   {the G\^ateaux derivative of order $n$}%
   {Gateaux derivative of Order n}%
\Index%396%G%Gateaux derivative of second order
   {the G\^ateaux derivative of second order}%
   {Gateaux derivative of Second Order}%
\Index%157%G%Gateaux differential of map
   {the G\^ateaux differential of map}%
   {Gateaux differential of map}%
\Index%46%G%Gateaux Dstar derivative of map f of division ring D
   {the G\^ateaux \Ds derivative of map $f$ of division ring $D$}%
   {Gateaux Dstar derivative of map, division ring}%
\Index%453%G%Gateaux mixed partial derivative
   {the G\^ateaux mixed partial derivative}%
   {Gateaux partial derivative of Second Order}%
\Index%511%G%Gateaux partial dcr derivative of map f^b with respect to variable x^a
   {the G\^ateaux partial \dcr derivative of map $f^{\gi b}$ with respect to variable $x^{\gi a}$}%
   {Gateaux partial dcr derivative of map with respect to variable, D vector space}%
\Index%512%G%Gateaux partial derivative
   {the G\^ateaux partial derivative}%
   {Gateaux partial derivative}%
\Index%510%G%Gateaux partial rcd derivative of map fb with respect to variable xa
   {the G\^ateaux partial \rcd derivative of map $f^{\gi b}$ with respect to variable $x^{\gi a}$}%
   {Gateaux partial rcd derivative of map with respect to variable, D vector space}%
\Index%13%G%Gateaux rcd derivative of map f of D-vector space V to D-vector space W
   {the G\^ateaux \rcd derivative of map $f$ of $D$\hyph vector space $V$ to $D$\hyph vector space $W$}%
   {Gateaux rcd derivative of map, D vector space}%
\Index%76%G%Gateaux starD derivative of map f of division ring D
   {the G\^ateaux \sD derivative of map $f$ of division ring $D$}%
   {Gateaux starD derivative of map, division ring}%
\Index%332%G%generating set of representation
   {generating set of representation}%
   {generating set of representation}%
\Index%331%G%generating set of subrepresentation
   {generating set of subrepresentation}%
   {generating set of subrepresentation}%
\Index%289%G%generator of linear map
   {generator of linear map}%
   {generator of linear map}%
\Index%700%G%geometric object defined in Omega_2- algebra
   {geometric object defined in $\Omega_2$\Hyph algebra $M$}%
   {geometric object, representation g}%
\Index%136%G%geometric object defined in rcd vector space
   {geometric object defined in \rcd vector space}%
   {geometric object, rcd vector space}%
\Index%722%G%geometric object defined in tuple of Omega- algebras
   {geometric object defined in tuple of $\VX\Omega$\Hyph algebras $\VX A$}%
   {geometric object, tower of representations g}%
\Index%133%G%geometric object in coordinate representation
   {geometric object in coordinate representation}%
   {geometric object, coordinate vector space}%
\Index%698%G%geometric object in coordinate representation defined in Omega_2- algebra
   {geometric object in coordinate representation defined in $\Omega_2$\Hyph algebra $M$}%
   {geometric object, coordinate representation g}%
\Index%134%G%geometric object in coordinate representation defined in rcd vector space
   {geometric object in coordinate representation defined in \rcd vector space}%
   {geometric object, coordinate rcd vector space}%
\Index%719%G%geometric object in coordinate representation defined in tuple of Omega- algebras
   {geometric object in coordinate representation defined in tuple of $\VX\Omega$\Hyph algebras $\VX A$}%
   {geometric object, coordinate tower of representations g}%
\Index%132%G%geometric object in vector space
   {geometric object in vector space}%
   {geometric object, vector space}%
\Index%704%G%geometric object of type
   {geometric object of type $H$}%
   {geometric object of type H, representation g}%
\Index%135%G%geometric object of type A
   {geometric object of type $A$ in vector space}%
   {geometric object of type A, vector space}%
\Index%146%G%group algebra
   {group algebra}%
   {group algebra}%
\Index%568%G%group of automorphisms of representation
   {group of automorphisms of representation}%
   {group of automorphisms of representation}%
\SetIndexSpace%
\Index%292%H%Hadamard inverse of matrix
   {Hadamard inverse of matrix}%
   {Hadamard inverse of matrix}%
\Index%783%H%Hamel basis
   {Hamel basis}%
   {Hamel basis}%
\Index%546%H%hermitian conjugated vector
   {hermitian conjugated vector}%
   {hermitian conjugated vector}%
\Index%541%H%hermitian conjugation in division ring
   {hermitian conjugation in division ring}%
   {hermitian conjugation, division ring}%
\Index%747%H%hermitian matrix
   {hermitian matrix}%
   {hermitian matrix}%
\Index%544%H%hermitian metric on division ring
   {hermitian metric on division ring}%
   {hermitian metric on division ring}%
\Index%350%H%hermitian scalar product in D- vector space
   {hermitian scalar product in $D$\Hyph vector space}%
   {hermitian scalar product, vector space}%
\Index%545%H%hermitian scalar product on division ring
   {hermitian scalar product on division ring}%
   {hermitian scalar product on division ring}%
\Index%138%H%holonomic coordinates of connection
   {holonomic coordinates of connection}%
   {holonomic coordinates of connection}%
\Index%137%H%holonomic coordinates of vector
   {holonomic coordinates of vector}%
   {vector holonomic coordinates}%
\Index%296%H%homogeneous bundle of fibered group
   {homogeneous bundle of fibered group}%
   {homogeneous bundle of fibered group}%
\Index%631%H%homogeneous linear geometric object
   {homogeneous linear geometric object}%
   {homogeneous linear geometric object}%
\Index%608%H%homogeneous linear representation of Lie group
   {homogeneous linear representation of Lie group}%
   {homogeneous Linear Representation of Lie Group}%
\Index%294%H%homogeneous map of degree k over field F
   {homogeneous map of degree $k$ over field $F$}%
   {homogeneous map of degree over field, D vector space}%
\Index%689%H%homogeneous polynomial of power
   {homogeneous polynomial of power $k$}%
   {homogeneous polynomial of power}%
\Index%295%H%homogeneous space of group
   {homogeneous space of group}%
   {homogeneous space of group}%
\Index%140%H%homomorphism of fibered groups
   {homomorphism of fibered groups}%
   {homomorphism of fibered groups}%
\Index%139%H%homomorphism of fibered universal algebras
   {homomorphism of fibered universal algebras}%
   {homomorphism of fibered universal algebras}%
\SetIndexSpace%
\Index%459%I%ideal of algebra
   {ideal of algebra}%
   {ideal of algebra}%
\Index%121%I%infinitesimal generator
   {infinitesimal generator}%
   {infinitesimal generator}%
\Index%174%I%infinitesimal generators of group Lie
   {infinitesimal generators of group Lie}%
   {infinitesimal generators of group Lie}%
\Index%705%I%invariance principle in drc vector space
   {invariance principle in \drc vector space}%
   {invariance principle}%
\Index%384%I%invariance principle in representation of universal algebra
   {invariance principle in representation of universal algebra}%
   {invariance principle, representation g}%
\Index%710%I%invariance principle in tower of representations of universal algebras
   {invariance principle in tower of representations of universal algebras}%
   {invariance principle, tower of representations g}%
\Index%385%I%invariance principle in vector space
   {invariance principle in vector space}%
   {invariance principle, vector space}%
\Index%291%I%inverse fibered correspondence
   {inverse fibered correspondence}%
   {inverse fibered correspondence}%
\Index%290%I%inverse reduced fibered correspondence
   {inverse reduced fibered correspondence}%
   {inverse reduced fibered correspondence}%
\Index%745%I%involution in quaternion algebra
   {involution in quaternion algebra}%
   {involution, quaternion algebra}%
\Index%173%I%isomorphism of fibered Omega- algebras
   {isomorphism of fibered $\Omega$\Hyph algebras}%
   {isomorphism of fibered Omega-algebras}%
\Index%266%I%isomorphism of repesentations of Omega- algebra
   {isomorphism of repesentations of $\Omega$\Hyph algebra}%
   {isomorphism of repesentations of Omega algebra}%
\Index%648%I%isotropic vector
   {isotropic vector}%
   {isotropic vector}%
\SetIndexSpace%
\Index%596%J%j i $RCcirc quasideterminant
   {$(^j_i)$\hyph $\RCcirc$\Hyph quasideterminant}%
   {j i RCcirc-quasideterminant}%
\Index%592%J%Jacobian complete system of differential equations
   {Jacobian complete system of differential equations}%
   {Jacobian complete system of differential equations}%
\Index%593%J%Jacobian complete system of drc differential equations
   {Jacobian complete system of \drv differential equations}%
   {Jacobian complete system of drc differential equations}%
\Index%678%J%ji- quasideterminant
   {$(ji)$\hyph quasideterminant}%
   {j i quasideterminant}%
\Index%527%J%the Jacobi Gateaux matrix of map
   {the Jacobi\Hyph G\^ateaux matrix of map}%
   {Jacobi Gateaux matrix of map}%
\SetIndexSpace%
\Index%526%K%kernel of inefficiency of representation of fibered group
   {kernel of inefficiency of representation of fibered group}%
   {kernel of inefficiency of representation of fibered group}%
\Index%525%K%kernel of inefficiency of representation of group
   {kernel of inefficiency of representation of group}%
   {kernel of inefficiency of representation of group}%
\Index%524%K%kernel of inefficiency of Tstar- representation of group G
   {kernel of inefficiency of \Ts representation of group $G$}%
   {kernel of inefficiency of Tstar representation of group}%
\Index%522%K%kernel of linear map
   {kernel of linear map}%
   {kernel of linear map}%
\Index%493%K%Killing equation
   {Killing equation}%
   {Killing equation}%
\Index%494%K%Killing equation of second type
   {Killing equation of second type}%
   {Killing equation second type}%
\Index%123%K%Killing vector of second type
   {Killing vector of second type}%
   {Killing vector second type}%
\Index%445%K%Kronecker symbol
   {Kronecker symbol}%
   {Kronecker symbol}%
\SetIndexSpace%
\Index%33%L%Drc linearly independent vector fields
   {linearly independent vector fields}%
   {linearly independent vector fields}%
\Index%754%L%left cofactor of entry of matrix
   {left cofactor of entry of matrix}%
   {left cofactor, matrix}%
\Index%301%L%left defined Lie algebra of Lie group
   {left defined Lie algebra of Lie group}%
   {left defined Lie algebra}%
\Index%756%L%left double cofactor of entry of matrix
   {left double cofactor of entry of matrix}%
   {left double cofactor}%
\Index%158%L%left fraction
   {left fraction}%
   {left fraction}%
\Index%681%L%left ideal of algebra
   {left ideal of algebra}%
   {left ideal of algebra}%
\Index%229%L%left invariant vector field
   {left invariant vector field}%
   {left invariant vector}%
\Index%661%L%left module over D- algebra A
   {left module over $D$\Hyph algebra $A$}%
   {left module over algebra}%
\Index%237%L%left module over ring
   {left module over a ring $D$}%
   {left module over ring}%
\Index%513%L%left principal ideal
   {left principal ideal}%
   {left principal ideal}%
\Index%731%L%left shift of R- module
   {left shift of $R$\Hyph module}%
   {left shift of module}%
\Index%240%L%left shift on fibered group
   {left shift on fibered group}%
   {Tstar shift, fibered group}%
\Index%238%L%left shift on group
   {left shift on group}%
   {left shift}%
\Index%239%L%left shift on group
   {left shift on group}%
   {left shift, group}%
\Index%236%L%left structural constant of Lie algebra
   {left structural constant of Lie algebra}%
   {left structural constant of Lie algebra}%
\Index%228%L%left vector space
   {left vector space}%
   {left vector space}%
\Index%812%L%left zero divisor
   {left zero divisor}%
   {left zero divisor}%
\Index%751%L%left-ordered cycle notation of permutation
   {left-ordered cycle notation of permutation}%
   {left-ordered cycle notation of permutation}%
\Index%231%L%left-side contravariant representation of group
   {left-side contravariant representation of group}%
   {left-side contravariant representation of group}%
\Index%230%L%left-side covariant representation of group
   {left-side covariant representation of group}%
   {left-side covariant representation of group}%
\Index%233%L%left-side representation of fibered Omega- algebra
   {left-side representation of fibered $\Omega$\Hyph algebra}%
   {left-side representation of fibered Omega-algebra}%
\Index%232%L%left-side representation of Omega1 algebra A in Omega2 algebra M
   {left-side representation of $\Omega_1$\Hyph algebra $A$ in $\Omega_2$\Hyph algebra $M$}%
   {left-side representation of algebra}%
\Index%234%L%left-side transformation
   {left-side transformation}%
   {left-side transformation}%
\Index%235%L%left-side transformation on bundle
   {left-side transformation on bundle}%
   {left-side transformation of bundle}%
\Index%104%L%Lie algebra of Lie group
   {Lie algebra of Lie group}%
   {algebra Lie group Lie}%
\Index%402%L%Lie derivative
   {Lie derivative}%
   {Lie derivative}%
\Index%404%L%Lie derivative of connection
   {Lie derivative of connection}%
   {Lie derivative of connection}%
\Index%403%L%Lie derivative of metric
   {Lie derivative of metric}%
   {Lie derivative of metric}%
\Index%118%L%Lie group basic operators
   {Lie group basic operators}%
   {Lie group basic operators}%
\Index%246%L%lift of correspondence
   {lift of correspondence}%
   {lift of correspondence}%
\Index%245%L%lift of mapping
   {lift of mapping}%
   {lift of map}%
\Index%365%L%limit of correspondence with respect to the filter
   {limit of correspondence with respect to the filter}%
   {limit of correspondence with respect to the filter}%
\Index%366%L%limit of filter
   {limit of filter}%
   {limit of filter}%
\Index%467%L%limit of sequence
   {limit of sequence}%
   {limit of sequence}%
\Index%367%L%limit set of filter
   {limit set of filter}%
   {limit set of filter}%
\Index%88%L%linear combination of  vectors
   {linear combination of  vectors}%
   {linear combination of  vectors}%
\Index%686%L%linear combination of vectors of A- module
   {linear combination of vectors of $A$\Hyph module}%
   {linear combination in A module}%
\Index%688%L%linear dependent vectors of A- module
   {linear dependent vectors of $A$\Hyph module}%
   {linear dependent vectors, module}%
\Index%397%L%linear functional on D module
   {linear functional on $D$\Hyph module}%
   {linear functional, D module}%
\Index%630%L%linear geometric object
   {linear geometric object}%
   {linear geometric object}%
\Index%687%L%linear independent vectors of A- module
   {linear independent vectors of $A$\Hyph module}%
   {linear independent vectors, module}%
\Index%613%L%linear map
   {linear map}%
   {linear map}%
\Index%98%L%linear map generated by map
   {linear map generated by map}%
   {linear map generated by map}%
\Index%398%L%linear map of D vector spaces
   {linear map of $D$\Hyph vector spaces}%
   {linear map of D vector spaces}%
\Index%97%L%linear map of division ring
   {linear map of division ring}%
   {linear map of division ring}%
\Index%35%L%linear map of rcd vector spaces
   {linear map of \rcd vector spaces}%
   {linear map of rcd vector spaces}%
\Index%244%L%linear representation of group
   {linear representation of group}%
   {linear representation of group}%
\Index%682%L%linear representation of Lie group
   {linear representation of Lie group}%
   {Linear Representation of Lie Group}%
\Index%740%L%linear transformation of rcd affine space
   {linear transformation of \rcd affine space}%
   {linear transformation, rcd affine space}%
\Index%20%L%linearly dependent vector fields
   {linearly dependent vector fields}%
   {linearly dependent vector fields}%
\Index%21%L%linearly dependent vectors
   {linearly dependent vectors}%
   {linearly dependent vectors}%
\Index%34%L%linearly independent vectors
   {linearly independent vectors}%
   {linearly independent vectors}%
\Index%250%L%little group
   {little group}%
   {little group}%
\Index%247%L%local reference frame
   {local reference frame}%
   {local reference frame}%
\Index%248%L%locally compact at point p space
   {locally compact at point $p$ space}%
   {locally compact at point space}%
\Index%249%L%locally compact space
   {locally compact space}%
   {locally compact space}%
\Index%373%L%Lorentz transformation
   {Lorentz transformation}%
   {Lorentz transformation}%
\SetIndexSpace%
\Index%56%M%m- dimensional parallelepiped
   {$m$\Hyph dimensional parallelepiped}%
   {m dimensional parallelepiped}%
\Index%57%M%m- vector
   {$m$\Hyph vector}%
   {m-vector}%
\Index%556%M%manifold with D- affine connections
   {manifold with $D$\Hyph affine connections}%
   {manifold with D- affine connections}%
\Index%506%M%map continuous with respect to set of arguments
   {map continuous with respect to set of arguments}%
   {map continuous with respect to set of arguments}%
\Index%505%M%map differentiable in Gateaux sense
   {map differentiable in the G\^ateaux sense}%
   {map differentiable in Gateaux sense}%
\Index%502%M%map of n D- valued variables
   {map of $\gi n$ $D$\Hyph valued variables}%
   {map of n D valued variables}%
\Index%316%M%map of type G on manifold
   {map of type $G$ on manifold}%
   {map of type G on manifold}%
\Index%572%M%map polylinear over finite dimensional algebras
   {map polylinear over finite dimensional algebras}%
   {map polylinear over finite dimensional algebras}%
\Index%677%M%map projective over commutative ring
   {map projective over commutative ring}%
   {map projective over commutative ring}%
\Index%312%M%mapping of rings polylinear over commutative ring
   {mapping of rings polylinear over commutative ring}%
   {map polylinear over commutative ring, ring}%
\Index%407%M%mapping space
   {mapping space}%
   {mapping space}%
\Index%772%M%matrix of antilinear homomorphism
   {matrix of antilinear homomorphism}%
   {matrix of antilinear homomorphism}%
\Index%252%M%matrix of bilinear function
   {matrix of bilinear function}%
   {matrix of bilinear function}%
\Index%595%M%matrix of endomorphisms of Omega algebra
   {matrix of endomorphisms of $\Omega$\Hyph algebra}%
   {matrix of endomorphisms of Omega algebra}%
\Index%253%M%matrix of fibered Drc linear map
   {matrix of fibered \Drc linear map}%
   {matrix of fibered drc linear map}%
\Index%770%M%matrix of linear homomorphism
   {matrix of linear homomorphism}%
   {matrix of linear homomorphism}%
\Index%194%M%matrix of linear map
   {matrix of linear map}%
   {matrix of linear map}%
\Index%591%M%matrix of linear mappings
   {matrix of linear mappings}%
   {matrix of linear mappings}%
\Index%588%M%matrix of mappings
   {matrix of mappings}%
   {matrix of mappings}%
\Index%552%M%matrix of quadratic map
   {matrix of quadratic map}%
   {matrix of quadratic map, division ring}%
\Index%800%M%measurable map
   {measurable map}%
   {measurable map}%
\Index%96%M%metric tensor in Minkowski space
   {metric tensor in Minkowski space}%
   {metric tensor, Minkowski space}%
\Index%254%M%metric-affine manifold
   {metric-affine manifold}%
   {metric-affine manifold}%
\Index%635%M%Minkowski space
   {Minkowski space}%
   {Minkowski space, Finsler}%
\Index%642%M%minor matrix
   {minor matrix}%
   {minor matrix}%
\Index%611%M%module over ring
   {module over ring}%
   {module over ring}%
\Index%766%M%monomial of power
   {monomial of power $k$}%
   {monomial of power}%
\Index%265%M%morphism from tower of Tstar- representations into tower of Tstar- representations
   {morphism from tower of \Ts representations into tower of \Ts representations}%
   {morphism from tower of representations into tower of representations}%
\Index%269%M%morphism of fibered Tstar- representations from F into G
   {morphism of fibered \Ts representations from $\Bundle F$ into $\Bundle G$}%
   {morphism of fibered representations from f into g}%
\Index%732%M%morphism of representation f
   {morphism of representation $f$}%
   {morphism of representation f}%
\Index%268%M%morphism of representations from f into g
   {morphism of representations from $f$ into $g$}%
   {morphism of representations from f into g}%
\Index%267%M%morphism of representations of Omega1 algebra in Omega2 algebra
   {morphism of representations of $\Omega_1$\Hyph algebra in $\Omega_2$\Hyph algebra}%
   {morphism of representations of Omega1 algebra in Omega2 algebra}%
\Index%264%M%morphism of Tstar- representations of fibered Omega- algebra
   {morphism of \Ts representations of fibered $\Omega$\Hyph algebra}%
   {morphism of representations of fibered Omega algebra}%
\Index%586%M%motion of Minkowski space
   {motion of Minkowski space}%
   {motion, Minkowski space}%
\Index%147%M%movement on basis manifold
   {movement on basis manifold}%
   {movement transformation}%
\SetIndexSpace%
\Index%726%N%n algebra over ring
   {$n$\Hyph algebra over the ring}%
   {n algebra over ring}%
\Index%58%N%n- ary fibered relation
   {$n$\Hyph ary fibered relation}%
   {fibered relation}%
\Index%279%N%nonmetricity
   {nonmetricity}%
   {nonmetricity}%
\Index%272%N%nonsingular bilinear function
   {nonsingular bilinear function}%
   {nonsingular bilinear function}%
\Index%273%N%nonsingular system of drc linear equations
   {nonsingular system of \rcd linear equations}%
   {nonsingular system of linear equations}%
\Index%643%N%nonsingular tensor
   {nonsingular tensor}%
   {nonsingular tensor}%
\Index%274%N%nonsingular transformation
   {nonsingular transformation}%
   {nonsingular transformation}%
\Index%742%N%norm in quaternion algebra
   {norm in quaternion algebra}%
   {norm, quaternion algebra}%
\Index%196%N%norm of functional
   {norm of functional}%
   {norm of functional}%
\Index%314%N%norm of map
   {norm of map}%
   {norm of map}%
\Index%657%N%norm of operation
   {norm of operation}%
   {norm of operation}%
\Index%285%N%norm of polylinear map
   {norm of polylinear map}%
   {norm of polymap}%
\Index%801%N%norm of representation
   {norm of representation}%
   {norm of representation}%
\Index%346%N%norm on D- algebra
   {norm on $D$\Hyph algebra}%
   {norm on D algebra}%
\Index%283%N%norm on D- vector space
   {norm on $D$\Hyph vector space}%
   {norm on D vector space}%
\Index%460%N%norm on D-module
   {norm on $D$\Hyph module}%
   {norm on D module}%
\Index%675%N%norm on Omega group
   {norm on $\Omega$\Hyph group}%
   {norm on Omega group}%
\Index%641%N%norm on ring
   {norm on ring}%
   {norm on ring}%
\Index%692%N%normal basis
   {normal basis}%
   {normal basis}%
\Index%343%N%normed D-algebra
   {normed $D$\Hyph algebra}%
   {normed D algebra}%
\Index%364%N%normed D-module
   {normed $D$\Hyph module}%
   {normed D module}%
\Index%287%N%normed D-vector space
   {normed $D$\Hyph vector space}%
   {normed D vector space}%
\Index%792%N%normed Omega group
   {normed $\Omega$\Hyph group}%
   {normed Omega group}%
\Index%640%N%normed ring
   {normed ring}%
   {normed ring}%
\Index%632%N%not complete group
   {not complete group}%
   {not complete group}%
\Index%649%N%not complete Omega algebra
   {not complete $\Omega$\Hyph algebra}%
   {not complete Omega algebra}%
\Index%619%N%nucleus of algebra
   {nucleus of $D$\Hyph algebra $A$}%
   {nucleus of algebra}%
\SetIndexSpace%
\Index%639%O%octonion algebra
   {octonion algebra}%
   {octonion algebra}%
\Index%793%O%open ball
   {open ball}%
   {open ball}%
\Index%300%O%operation on bundle
   {operation on bundle}%
   {operation on bundle}%
\Index%623%O%opposite algebra to algebra
   {opposite algebra to algebra $P$}%
   {opposite algebra}%
\Index%408%O%opposite fibered preordering
   {opposite fibered preordering}%
   {opposite fibered preordering}%
\Index%624%O%orbit of linear mapping
   {orbit of linear mapping}%
   {orbit of linear mapping}%
\Index%306%O%orbit of representation of fibered group
   {orbit of representation of fibered group}%
   {orbit of representation of fibered group}%
\Index%305%O%orbit of representation of group
   {orbit of representation of group}%
   {orbit of representation of group}%
\Index%304%O%orbit of Tstar- representation of group
   {orbit of \Ts representation of group}%
   {orbit of Tstar  representation of group}%
\Index%729%O%origin of coordinate system of affine space
   {origin of coordinate system of affine space}%
   {origin of coordinate system of affine space}%
\Index%738%O%origin of coordinate system of star D affine space
   {origin of coordinate system of $\star D$\Hyph affine space}%
   {origin of coordinate system of starD affine space}%
\Index%637%O%orthogonal basis in Minkowski space
   {orthogonal basis in Minkowski space}%
   {orthogonal basis, Minkowski space}%
\Index%636%O%orthogonality in Minkowski space
   {orthogonality in Minkowski space}%
   {Minkowski orthogonality}%
\Index%638%O%orthonormal basis in Minkowski space
   {orthonormal basis in Minkowski space}%
   {orthonormal basis, Minkowski space}%
\Index%307%O%orthonornal basis
   {orthonornal basis}%
   {Orthonornal Basis}%
\Index%308%O%orthonornal basis
   {orthonornal basis}%
   {Orthonornal Basis, division ring}%
\SetIndexSpace%
\Index%695%P%active representation of group in basis manifold of representation
   {passive representation of group $G(f)$ in basis manifold of representation}%
   {passive representation in basis manifold}%
\Index%739%P%parallel shift of rcd affine space
   {parallel shift of \rcd affine space}%
   {parallel shift, rcd affine space}%
\Index%317%P%parallelogram
   {parallelogram}%
   {parallelogram}%
\Index%475%P%partial linear map
   {partial linear map}%
   {partial linear map}%
\Index%333%P%passive representation
   {passive representation}%
   {passive representation}%
\Index%718%P%passive representation of group in basis manifold of tower of representations
   {passive representation of group $G(\Vector f)$ in basis manifold of tower of representations}%
   {passive representation in basis manifold, tower of representations}%
\Index%321%P%passive starT- representation
   {passive \sT representation}%
   {passive starT representation}%
\Index%570%P%passive transformation of the basis manifold of representation
   {passive transformation of the basis manifold of representation}%
   {passive transformation of basis, representation}%
\Index%717%P%passive transformation of the basis manifold of tower of representations
   {passive transformation of the basis manifold of tower of representations}%
   {passive transformation of basis, tower of representations}%
\Index%335%P%passive transformation on basis manifold
   {passive transformation on basis manifold}%
   {passive transformation}%
\Index%336%P%passive transformation on the set of rcd bases
   {passive transformation on the set of \rcd bases}%
   {passive transformation, vector space}%
\Index%744%P%permutability property of trace
   {permutability property of trace}%
   {permutability property of trace}%
\Index%416%P%pfaffian derivative
   {pfaffian derivative}%
   {pfaffian derivative}%
\Index%806%P%polyadditive map
   {polyadditive map}%
   {polyadditive map}%
\Index%609%P%polylinear map
   {polylinear map}%
   {polylinear map}%
\Index%345%P%polylinear skew symmetric map
   {polylinear skew symmetric map}%
   {polylinear map skew symmetric}%
\Index%347%P%polylinear symmetric map
   {polylinear symmetric map}%
   {polylinear map symmetric}%
\Index%760%P%polymorphism of representations
   {polymorphism of representations}%
   {polymorphism of representations}%
\Index%804%P%polynomial
   {polynomial}%
   {polynomial}%
\Index%344%P%polyvector
   {polyvector}%
   {polyvector}%
\Index%352%P%potential energy
   {potential energy}%
   {potential energy}%
\Index%767%P%principal ideal
   {principal ideal}%
   {principal ideal}%
\Index%388%P%product of geometric object and constant
   {product of geometric object and constant}%
   {product of geometric object and constant}%
\Index%389%P%product of geometric object and constant in vector space
   {product of geometric object and constant in vector space}%
   {product of geometric object and constant, vector space}%
\Index%390%P%product of groups
   {product of groups}%
   {product of groups}%
\Index%683%P%product of linear map over scalar
   {product of linear map over scalar}%
   {product of linear map over scalar}%
\Index%271%P%product of map over scalar
   {product of map over scalar}%
   {product of map over scalar}%
\Index%391%P%product of morphisms of representations of universal algebra
   {product of morphisms of representations of universal algebra}%
   {product of morphisms of representations of universal algebra}%
\Index%561%P%product of morphisms of tower of representations
   {product of morphisms of tower of representations}%
   {product of morphisms of tower of representations}%
\Index%392%P%product of morphisms of Tstar- representations of fibered Omega- algebra
   {product of morphisms of \Ts representations of fibered $\Omega$\Hyph algebra}%
   {product of morphisms of representations of fibered Omega algebra}%
\Index%395%P%product of objects in category
   {product of objects in category}%
   {product of objects in category}%
\Index%666%P%product of polynomials
   {product of polynomials}%
   {product of polynomials}%
\Index%387%P%projection of bundle E along fiber E
   {projection of bundle $\Bundle E$ along fiber $E$}%
   {projection of bundle along fiber}%
\Index%195%P%projective map is continuous in direction over field
   {projective map is continuous in direction over field}%
   {projective map is continuous in direction over field}%
\Index%540%P%pseudo-Euclidean metric on division ring
   {pseudo\Hyph Euclidean metric on division ring}%
   {pseudo-Euclidean metric on division ring}%
\Index%548%P%pseudo-Euclidean scalar product in D- vector space
   {pseudo\Hyph Euclidean scalar product in $D$\Hyph vector space}%
   {pseudo-Euclidean scalar product, vector space}%
\Index%543%P%pseudo-Euclidean scalar product on division ring
   {pseudo-Euclidean scalar product on division ring}%
   {pseudo-Euclidean scalar product on division ring}%
\SetIndexSpace%
\Index%555%Q%quadratic form in division ring
   {quadratic form in division ring}%
   {quadratic form, division ring}%
\Index%551%Q%quadratic map of division ring
   {quadratic map of division ring}%
   {Quadratic Map of Division Ring}%
\Index%180%Q%quasi affine transformation on basis manifold
   {quasi affine transformation on basis manifold}%
   {quasi affine transformation}%
\Index%181%Q%quasi affine transformation on basis manifold
   {quasi affine transformation on basis manifold}%
   {quasi affine drc transformation}%
\Index%182%Q%quasi movement on basis manifold
   {quasi movement on basis manifold}%
   {quasi movement, division ring}%
\Index%183%Q%quasi movement on basis manifold
   {quasi movement on basis manifold}%
   {quasi movement}%
\Index%604%Q%quasiclosed ring of mappings
   {quasiclosed ring of mappings}%
   {quasiclosed ring of mappings}%
\Index%679%Q%quasideterminant
   {quasideterminant}%
   {quasideterminant definition}%
\Index%75%Q%quasimotion of Minkowski space
   {quasimotion of Minkowski space}%
   {Quasimotion, Minkowski space}%
\Index%741%Q%quaternion algebra
   {quaternion algebra}%
   {quaternion algebra}%
\Index%103%Q%quaternion algebra E over the field F
   {quaternion algebra $E$ over the field $F$}%
   {quaternion algebra over the field}%
\Index%496%Q%quotient bundle
   {quotient bundle}%
   {quotient bundle}%
\SetIndexSpace%
\Index%4%R%j i-RC quasideterminant
   {$(^j_i)$\hyph \RC quasideterminant}%
   {j i RC-quasideterminant}%
\Index%59%R%r row of matrix
   {\sups row of matrix}%
   {r row}%
\Index%728%R%R- module
   {$R$\Hyph module}%
   {R- module}%
\Index%72%R%r-row of matrix
   {$r$\hyph row of matrix}%
   {r-row}%
\Index%749%R%rank of Hermitian matrix by principal minors
   {rank of Hermitian matrix by principal minors}%
   {rank of Hermitian matrix by principal minors}%
\Index%554%R%rank of quadratic map of division ring
   {rank of quadratic map of division ring}%
   {rank of quadratic map, division ring}%
\Index%65%R%RC inverse element of biring
   {\RC inverse element of biring}%
   {rc-inverse element}%
\Index%61%R%RC major minor matrix
   {\RC major minor matrix}%
   {RC-major minor}%
\Index%63%R%RC matrix group
   {\RC matrix group}%
   {rc-matrix group}%
\Index%64%R%RC nonsingular matrix
   {\RC nonsingular matrix}%
   {RC nonsingular matrix}%
\Index%68%R%RC power
   {\RC power}%
   {rc power}%
\Index%66%R%RC product of matrices
   {\RC product of matrices}%
   {rc-product of matrices}%
\Index%590%R%rc product of matrices of mappings
   {$\RCcirc$\Hyph product of matrices of mappings}%
   {rc product of matrices of mappings}%
\Index%62%R%RC quasideterminant
   {\RC quasideterminant}%
   {RC-quasideterminant}%
\Index%67%R%RC rank of matrix
   {\RC rank of matrix}%
   {rc-rank of matrix}%
\Index%60%R%RC singular matrix
   {\RC singular matrix}%
   {RC singular matrix}%
\Index%601%R%RCcirc nonsingular matrix of A(A) mappings
   {$\RCcirc$\Hyph nonsingular matrix of $\mathcal A(A)$\Hyph mappings}%
   {RCcirc nonsingular matrix of A(A) mappings}%
\Index%598%R%RCcirc nonsingular matrix of endomorphisms
   {$\RCcirc$\Hyph nonsingular matrix of endomorphisms}%
   {RCcirc nonsingular matrix of endomorphisms}%
\Index%602%R%RCcirc nonsingular system of additive equations
   {$\RCcirc$\Hyph nonsingular system of additive equations}%
   {RCcirc nonsingular system of additive equations}%
\Index%597%R%RCcirc quasideterminant
   {$\RCcirc$\Hyph quasideterminant}%
   {RCcirc-quasideterminant definition}%
\Index%600%R%RCcirc singular matrix of A(A) mappings
   {$\RCcirc$\Hyph singular matrix of $\mathcal A(A)$\Hyph mappings}%
   {RCcirc singular matrix of A(A) mappings}%
\Index%599%R%RCcirc singular matrix of endomorphisms
   {$\RCcirc$\Hyph singular matrix of endomorphisms}%
   {RCcirc singular matrix of endomorphisms}%
\Index%765%R%RCcircA linear combination
   {$\RCcirc A$\Hyph linear combination}%
   {RCcircA linear combination}%
\Index%111%R%rcd affine basis
   {\rcd affine basis}%
   {rcd affine basis, division ring}%
\Index%759%R%rcd affine plane
   {\rcd affine plane}%
   {rcd affine plane}%
\Index%736%R%rcd affine space
   {\rcd affine space}%
   {rcd affine space}%
\Index%758%R%rcd affine transformation
   {\rcd affine transformation}%
   {rcd affine transformation}%
\Index%22%R%rcd automorphism of vector space
   {\rcd automorphism of vector space}%
   {automorphism of vector space}%
\Index%31%R%rcd isomorphism of vector spaces
   {\rcd isomorphism of vector spaces}%
   {isomorphism of vector spaces}%
\Index%37%R%rcd linear Tstar- representation of group
   {\rcd linear \Ts representation of group}%
   {rcd linear Tstar representation of group}%
\Index%27%R%rcd vector
   {\rcd vector}%
   {rcd vector}%
\Index%69%R%rcd vector space
   {\rcd vector space}%
   {rcd vector space}%
\Index%377%R%reduced Cartesian product of bundles
   {reduced Cartesian product of bundles}%
   {reduced Cartesian product of bundles}%
\Index%378%R%reduced Cartesian product of total spaces
   {reduced Cartesian product of total spaces}%
   {reduced Cartesian product of total spaces}%
\Index%379%R%reduced fibered correspondence from A to B
   {reduced fibered correspondence from $\Bundle{A}$ to $\Bundle B$}%
   {reduced fibered correspondence from A to B}%
\Index%380%R%reduced fibered correspondence in A
   {reduced fibered correspondence in $\Bundle{A}$}%
   {reduced fibered correspondence in A}%
\Index%761%R%reduced polymorphism of representations
   {reduced polymorphism of representations}%
   {reduced polymorphism of representations}%
\Index%381%R%reducible biring
   {reducible biring}%
   {reducible biring}%
\Index%450%R%reference frame in event space
   {reference frame in event space}%
   {reference frame in event space}%
\Index%263%R%reference frame manifold
   {reference frame manifold}%
   {reference frame manifold}%
\Index%439%R%reflexive 2- ary fibered relation
   {reflexive $2$\Hyph ary fibered relation}%
   {reflexive 2 ary fibered relation}%
\Index%330%R%regular endomorphism of representation
   {regular endomorphism of representation}%
   {regular endomorphism of representation}%
\Index%566%R%regular endomorphism of tower of representations
   {regular endomorphism of tower of representations}%
   {regular endomorphism of tower of representations}%
\Index%553%R%regular quadratic map in division ring
   {regular quadratic map in division ring}%
   {regular quadratic map, division ring}%
\Index%372%R%representation of group
   {representation of group}%
   {representation of group}%
\Index%528%R%representation of Omega algebra in representation
   {representation of $\Omega$\Hyph algebra in representation}%
   {representation of Omega algebra in representation}%
\Index%529%R%representation of Omega algebra in tower of representations
   {representation of $\Omega$\Hyph algebra in tower of representations}%
   {representation of Omega algebra in tower of representations}%
\Index%370%R%representation of Omega- algebra A in category B
   {representation of $\Omega$\Hyph algebra $A$ in category $\mathcal B$}%
   {representation of Omega algebra in category}%
\Index%371%R%representation of Omega1 algebra A in Omega2 algebra M
   {representation of $\Omega_1$\Hyph algebra $A$ in $\Omega_2$\Hyph algebra $M$}%
   {representation of algebra}%
\Index%702%R%representative of geometric object in drc vector space
   {representative of geometric object in \drc vector space}%
   {representative of geometric object, drc vector space}%
\Index%703%R%representative of geometric object in Omega_2- algebra
   {representative of geometric object in $\Omega_2$\Hyph algebra}%
   {representative of geometric object, representation g}%
\Index%368%R%representative of geometric object in rcd vector space
   {representative of geometric object in \rcd vector space}%
   {representative of geometric object, rcd vector space}%
\Index%724%R%representative of geometric object in tuple of Omega- algebras
   {representative of geometric object in tuple of $\VX\Omega$\Hyph algebras}%
   {representative of geometric object, tower of representations g}%
\Index%369%R%representative of geometric object in vector space
   {representative of geometric object in vector space}%
   {representative of geometric object, vector space}%
\Index%474%R%restriction of correspondence \Phi to set C
   {restriction of correspondence $\Phi$ to set $C$}%
   {restriction of correspondence}%
\Index%753%R%right cofactor of entry of matrix
   {right cofactor of entry of matrix}%
   {right cofactor, matrix}%
\Index%302%R%right defined Lie algebra of Lie group
   {right defined Lie algebra of Lie group}%
   {right defined Lie algebra}%
\Index%757%R%right double cofactor of entry of matrix
   {right double cofactor of entry of matrix}%
   {right double cofactor}%
\Index%30%R%right fraction
   {right fraction}%
   {right fraction}%
\Index%42%R%right ideal of algebra
   {right ideal of algebra}%
   {right ideal of algebra}%
\Index%354%R%right invariant vector field
   {right invariant vector field}%
   {right invariant vector}%
\Index%670%R%right module over D- algebra A
   {right module over $D$\Hyph algebra $A$}%
   {right module over algebra}%
\Index%361%R%right module over ring
   {right module over a ring $D$}%
   {right module over ring}%
\Index%242%R%right principal ideal
   {right principal ideal}%
   {right principal ideal}%
\Index%362%R%right shift on group
   {right shift on group}%
   {right shift}%
\Index%363%R%right shift on group
   {right shift on group}%
   {right shift, group}%
\Index%360%R%right structural constant of Lie algebra
   {right structural constant of Lie algebra}%
   {right structural constant of Lie algebra}%
\Index%353%R%right vector space
   {right vector space}%
   {right vector space}%
\Index%813%R%right zero divisor
   {right zero divisor}%
   {right zero divisor}%
\Index%752%R%right-ordered cycle notation of permutation
   {right-ordered cycle notation of permutation}%
   {right-ordered cycle notation of permutation}%
\Index%356%R%right-side contravariant representation of group
   {right-side contravariant representation of group}%
   {right-side contravariant representation of group}%
\Index%355%R%right-side covariant representation of group
   {right-side covariant representation of group}%
   {right-side covariant representation of group}%
\Index%358%R%right-side representation of fibered Omega- algebra
   {right-side representation of fibered $\Omega$\Hyph algebra}%
   {right-side representation of fibered Omega-algebra}%
\Index%357%R%right-side representation of Omega1 algebra A in Omega2 algebra M
   {right-side representation of $\Omega_1$\Hyph algebra $A$ in $\Omega_2$\Hyph algebra $M$}%
   {right-side representation of algebra}%
\Index%359%R%right-side transformation
   {right-side transformation}%
   {right-side transformation}%
\Index%188%R%ring has characteristic 0
   {ring has characteristic $0$}%
   {ring has characteristic 0}%
\Index%189%R%ring has characteristic p
   {ring has characteristic $p$}%
   {ring has characteristic p}%
\Index%794%R%ring of sets
   {ring of sets}%
   {ring of sets}%
\Index%778%R%ring with conjugation
   {ring with conjugation}%
   {ring with conjugation}%
\Index%634%R%root of polynomial
   {root of polynomial}%
   {root of polynomial}%
\Index%748%R%row determinant
   {row determinant}%
   {row determinant}%
\Index%127%R%row vector
   {row vector}%
   {row vector}%
\SetIndexSpace%
\Index%669%S%$starA- module
   {$\star A$\Hyph module}%
   {starA-module}%
\Index%73%S%RCstarS,RCstarT- linear map of vector spaces
   {$(\RCstar S,\RCstar T)$\Hyph linear map of vector spaces}%
   {rcs rct linear map of vector spaces}%
\Index%786%S%scalar algebra of algebra
   {scalar algebra of algebra}%
   {scalar algebra of algebra}%
\Index%775%S%scalar algebra of ring
   {scalar algebra of ring}%
   {scalar algebra of ring}%
\Index%784%S%scalar of element of algebra
   {scalar of element of algebra}%
   {scalar of algebra}%
\Index%773%S%scalar of element of ring
   {scalar of element of ring}%
   {scalar of ring}%
\Index%781%S%scalar of mapping
   {scalar of mapping}%
   {scalar of mapping}%
\Index%451%S%scalar potential
   {scalar potential}%
   {scalar potential}%
\Index%791%S%Schauder basis
   {Schauder basis}%
   {Schauder basis}%
\Index%129%S%second Newton law
   {second Newton law}%
   {Second Newton law}%
\Index%694%S%section of bundle
   {section of bundle}%
   {section of bundle}%
\Index%816%S%sequence converges
   {sequence converges}%
   {sequence converges}%
\Index%817%S%sequence converges uniformly
   {sequence converges uniformly}%
   {sequence converges uniformly}%
\Index%562%S%set of coordinates of representation
   {set of coordinates of representation}%
   {coordinate set of representation}%
\Index%628%S%set of invertible elements of algebra
   {set of invertible elements of algebra}%
   {set of invertible elements of algebra}%
\Index%571%S%set of Omega_2- words of representation
   {set of $\Omega_2$\Hyph words of representation}%
   {word set of representation}%
\Index%563%S%set of tuples of coordinates of tower of representations
   {set of tuples of coordinates of tower of representations}%
   {coordinate set of tower of representations}%
\Index%709%S%set of tuples of Omega- words of tower of representations
   {set of tuples of $\Vector\Omega$\Hyph words of tower of representations}%
   {word set of tower of representations}%
\Index%626%S%set of zeros of algebra
   {set of zeros of algebra}%
   {set of zeros of algebra}%
\Index%810%S%simple map
   {simple map}%
   {simple map}%
\Index%405%S%simple polyvector
   {simple polyvector}%
   {simple polyvector}%
\Index%299%S%single transitive representation of fibered Omega- algebra
   {single transitive representation of fibered $\Omega$\Hyph algebra}%
   {single transitive representation of fibered Omega-algebra}%
\Index%298%S%single transitive representation of group
   {single transitive representation of group}%
   {single transitive representation of group}%
\Index%297%S%single transitive representation of Omega- algebra A
   {single transitive representation of $\Omega$\Hyph algebra $A$}%
   {single transitive representation of algebra}%
\Index%130%S%singular linear map
   {singular linear map}%
   {singular linear map}%
\Index%226%S%skew product of vectors
   {skew product of vectors}%
   {skew product of vectors}%
\Index%406%S%space of orbits of Tstar- representation
   {space of orbits of \Ts representation}%
   {space of orbits of Ts representation}%
\Index%342%S%spacelike vector
   {spacelike vector}%
   {spacelike vector}%
\Index%452%S%speed of deviation
   {speed of deviation}%
   {speed of deviation}%
\Index%74%S%SRCstar,TRCstar- linear map of vector bundles
   {$(\mathcal S\RCstar,\mathcal T\RCstar)$\Hyph linear map of vector bundles}%
   {src trc linear map of vector bundles}%
\Index%112%S%Sstar, star T-bimodule
   {($S\star$, $\star T$)\hyph bimodule}%
   {(Sstar,starT)-bimodule}%
\Index%145%S%stability group
   {stability group}%
   {stability group}%
\Index%457%S%stable set of representation
   {stable set of representation}%
   {stable set of representation}%
\Index%458%S%standard component of Gateaux derivative
   {standard component of the G\^ateaux derivative}%
   {standard component of Gateaux derivative}%
\Index%456%S%standard component of linear map
   {standard component of linear map}%
   {standard component of linear map}%
\Index%462%S%standard component of polylinear map
   {standard component of polylinear map}%
   {standard component of polylinear map}%
\Index%463%S%standard component of tensor
   {standard component of tensor}%
   {standard component of tensor}%
\Index%461%S%standard component over field F of bilitnear map f
   {standard component over field $F$ of bilitnear map $f$}%
   {standard component of bilinear map, division ring}%
\Index%472%S%standard coordinates of basis
   {standard coordinates of basis}%
   {standard coordinates of basis}%
\Index%471%S%standard coordinates of rcd basis
   {standard coordinates of \rcd basis}%
   {standard coordinates of rcd basis}%
\Index%465%S%standard representation of Gateaux derivative
   {standard representation of the G\^ateaux derivative}%
   {Gateaux derivative, standard representation}%
\Index%464%S%standard representation of linear map
   {standard representation of linear map}%
   {linear map, standard representation}%
\Index%468%S%standard representation of matrix
   {standard representation of matrix}%
   {Standard representation}%
\Index%470%S%standard representation of polylinear map
   {standard representation of polylinear map}%
   {polylinear map, standard representation}%
\Index%466%S%standard representation of quadratic map of division ring over field F
   {standard representation of quadratic map of division ring over field $F$}%
   {quadratic map, standard representation, division ring}%
\Index%469%S%standard representation over field F of bilinear map of division ring
   {standard representation over field $F$ of bilinear map of division ring}%
   {bilinear map, standard representation, division ring}%
\Index%78%S%star D-vector space
   {$\star D$\hyph vector space}%
   {starD-vector space}%
\Index%79%S%star R-module
   {$\star R$\hyph module}%
   {starR-module}%
\Index%674%S%starA- product of vector over scalar
   {$\star A$\Hyph product of vector over scalar}%
   {starA product of vector over scalar, starA module}%
\Index%735%S%starD affine space
   {$\star D$\Hyph affine space}%
   {starD affine space}%
\Index%192%S%starD- vector space
   {$\star D$\Hyph vector space}%
   {starD vector space}%
\Index%198%S%starD-product of vector over scalar
   {$\star D$\hyph product of vector over scalar}%
   {starD product of vector over scalar, vector space}%
\Index%84%S%starT- representation of fibered group
   {\sT representation of fibered group}%
   {starT representation of fibered group}%
\Index%83%S%starT- representation of fibered Omega- algebra
   {\sT representation of fibered $\Omega$\Hyph algebra}%
   {starT representation of fibered Omega-algebra}%
\Index%82%S%starT- representation of Omega1 algebra A in Omega2 algebra M
   {\sT representation of $\Omega_1$\Hyph algebra $A$ in $\Omega_2$\Hyph algebra $M$}%
   {starT representation of algebra}%
\Index%80%S%starT- shift
   {\sT shift}%
   {starT shift}%
\Index%81%S%starT- shift on fibered group
   {\sT shift on fibered group}%
   {starT shift, fibered group}%
\Index%85%S%starT- transformation
   {\sT transformation}%
   {starT transformation}%
\Index%86%S%starT- transformation on bundle
   {\sT transformation on bundle}%
   {starT transformation of bundle}%
\Index%473%S%structural constants
   {structural constants}%
   {structural constants}%
\Index%340%S%subbundle
   {subbundle}%
   {subbundle}%
\Index%341%S%subbundle of Dstar-vector space
   {subbundle of $\mathcal D\star$\hyph vector space}%
   {subbundle of Dstar vector bundle}%
\Index%322%S%subrepresentation generated by set X
   {subrepresentation generated by set $X$}%
   {subrepresentation generated by set}%
\Index%334%S%subrepresentation of representation
   {subrepresentation of representation}%
   {subrepresentation of representation}%
\Index%477%S%sum of geometric objects in vector space
   {sum of geometric objects in vector space}%
   {sum of geometric objects, vector space}%
\Index%476%S%sum of geometrical objects
   {sum of geometric objects}%
   {sum of geometric objects}%
\Index%351%S%sum of linear maps
   {sum of linear maps}%
   {sum of linear maps}%
\Index%667%S%sum of polynomials
   {sum of polynomials}%
   {sum of polynomials}%
\Index%323%S%superposition of coordinates of the representation and the element
   {superposition of coordinates of the representation $f$ and the element $m$}%
   {superposition of coordinates, representation}%
\Index%712%S%superposition of coordinates of the tower of representations and the element
   {superposition of coordinates of the tower of representations $\Vector f$ and the element $\VX a$}%
   {superposition of coordinates, tower of representations}%
\Index%446%S%symmetric 2- ary fibered relation
   {symmetric $2$\Hyph ary fibered relation}%
   {symmetric 2 ary fibered relation}%
\Index%447%S%symmetric bilinear map of D- vector space to division ring
   {symmetric bilinear map of $D$\Hyph vector space to division ring}%
   {symmetric bilinear map, vector space to division ring}%
\Index%650%S%symmetric polylinear mapping into associative algebra
   {symmetric polylinear mapping into associative algebra}%
   {polylinear map symmetric, associative algebra}%
\Index%143%S%symmetry group
   {symmetry group}%
   {symmetry group}%
\Index%144%S%symmetry group
   {symmetry group}%
   {SymmetryGroup}%
\Index%448%S%synchronization of reference frame
   {synchronization of reference frame}%
   {synchronization of reference frame}%
\Index%605%S%system of additive equations
   {system of additive equations}%
   {system of additive equations}%
\Index%449%S%system of drc linear equations
   {system of \drc linear equations}%
   {system of drc linear equations}%
\Index%311%S%system of rcd linear equations
   {system of \rcd linear equations}%
   {system of rcd linear equations}%
\SetIndexSpace%
\Index%499%T%Taylor polynomial
   {Taylor polynomial}%
   {Taylor polynomial, division ring}%
\Index%440%T%Taylor series
   {Taylor series}%
   {Taylor series, division ring}%
\Index%802%T%tensor inverse to tensor
   {tensor inverse to tensor}%
   {inverse tensor}%
\Index%652%T%tensor power
   {tensor power}%
   {tensor power}%
\Index%573%T%tensor product of algebras
   {tensor product of algebras}%
   {tensor product of algebras}%
\Index%480%T%tensor product of D- vector spaces
   {tensor product of $D$\Hyph vector spaces}%
   {tensor product of D vector spaces}%
\Index%484%T%tensor product of division rings
   {tensor product of division rings}%
   {tensor product of division rings}%
\Index%481%T%tensor product of Dstar vector spaces
   {tensor product of \Ds vector spaces}%
   {tensor product of Dstar vector spaces}%
\Index%483%T%tensor product of representations
   {tensor product of representations}%
   {tensor product of representations}%
\Index%762%T%tensor product of representations
   {tensor product of representations}%
   {tensor product of representations}%
\Index%482%T%tensor product of rings over commutative ring
   {tensor product of rings over commutative ring}%
   {tensor product of rings}%
\Index%207%T%tensor product of vector spaces
   {tensor product of vector spaces}%
   {tensor product of vector spaces}%
\Index%47%T%the Fr\'echet Dstar derivative of map f of division ring D at point x
   {the Fr\'echet \Ds derivative of map $f$ of division ring $D$ at point $x$}%
   {Frechet Dstar derivative of map, division ring}%
\Index%651%T%timelike vector
   {timelike vector}%
   {timelike vector}%
\Index%486%T%topological D- vector space
   {topological $D$\Hyph vector space}%
   {topological D vector space}%
\Index%310%T%topological D-algebra
   {topological $D$\Hyph algebra}%
   {topological D algebra}%
\Index%488%T%topological division ring
   {topological division ring}%
   {topological division ring}%
\Index%790%T%topological ring
   {topological ring}%
   {topological ring}%
\Index%498%T%torsion form
   {torsion form}%
   {torsion form}%
\Index%478%T%torsion tensor
   {torsion tensor}%
   {torsion tensor}%
\Index%120%T%tower of bundles
   {tower of bundles}%
   {tower of bundles}%
\Index%324%T%tower of effective representations
   {tower of effective representations}%
   {tower of effective representations}%
\Index%119%T%tower of representations of Omega algebras
   {tower of representations of $\Vector{\Omega}$\Hyph algebras}%
   {tower of representations of algebras}%
\Index%531%T%tower of subrepresentations
   {tower of subrepresentations}%
   {tower of subrepresentations}%
\Index%532%T%tower of subrepresentations of tower of representations generated by tuple of sets
   {tower of subrepresentations of tower of representations $\Vector f$ generated by tuple of sets $\VX X$}%
   {subrepresentation generated by tuple of sets}%
\Index%743%T%trace of quaternion
   {trace of quaternion}%
   {trace, quaternion algebra}%
\Index%376%T%transformation coordinated with equivalence
   {transformation coordinated with equivalence}%
   {transformation coordinated with equivalence}%
\Index%374%T%transformation of universal algebra
   {transformation of universal algebra}%
   {transformation of universal algebra}%
\Index%375%T%transformation on bundle
   {transformation on bundle}%
   {transformation of bundle}%
\Index%489%T%transitive 2- ary fibered relation
   {transitive $2$\Hyph ary fibered relation}%
   {transitive 2 ary fibered relation}%
\Index%492%T%transitive representation of fibered Omega- algebra
   {transitive representation of fibered $\Omega$\Hyph algebra}%
   {transitive representation of fibered Omega-algebra}%
\Index%491%T%transitive representation of group
   {transitive representation of group}%
   {transitive representation of group}%
\Index%490%T%transitive representation of Omega- algebra A
   {transitive representation of $\Omega$\Hyph algebra $A$}%
   {transitive representation of algebra}%
\Index%87%T%Tstar- matrices vector space
   {\Ts matrices vector space}%
   {matrices vector space}%
\Index%91%T%Tstar- representation of fibered Omega- algebra
   {\Ts representation of fibered $\Omega$\Hyph algebra}%
   {Tstar representation of fibered Omega-algebra}%
\Index%90%T%Tstar- representation of Omega1 algebra A in Omega2 algebra M
   {\Ts representation of $\Omega_1$\Hyph algebra $A$ in $\Omega_2$\Hyph algebra $M$}%
   {Tstar representation of algebra}%
\Index%89%T%Tstar- shift
   {\Ts shift}%
   {Tstar shift}%
\Index%92%T%Tstar- transformation
   {\Ts transformation}%
   {Tstar transformation}%
\Index%93%T%Tstar- transformation on bundle
   {\Ts transformation on bundle}%
   {Tstar transformation of bundle}%
\Index%535%T%tuple of coordinates of element relative to tuple of sets
   {tuple of coordinates of element $\Vector a$ relative to tuple of sets $\VX X$}%
   {coordinates of element, tower of representations}%
\Index%713%T%tuple of equivalence generated by tower of representations
   {tuple of equivalence generated by tower of representations $\Vector f$}%
   {tuple of equivalence of tower of representations}%
\Index%534%T%tuple of generating sets of tower of representations
   {tuple of generating sets of tower of representations}%
   {tuple of generating sets of tower of representations}%
\Index%533%T%tuple of generating sets of tower subrepresentations
   {tuple of generating sets of tower subrepresentations}%
   {tuple of generating sets of tower subrepresentations}%
\Index%708%T%tuple of Omega- words of elements of tower of representations relative to tuple of generating sets
   {tuple of $\Vector{\Omega}$\Hyph words of element of tower of representations relative to tuple of generating sets}%
   {tuple of words relative to tuple of generating sets, tower of representations}%
\Index%530%T%tuple of stable sets of tower of representation
   {tuple of stable sets of tower of representation}%
   {tuple of stable sets of tower of representations}%
\Index%587%T%twin representations of associative algebra
   {twin representations of associative algebra}%
   {twin representations of associative algebra}%
\Index%684%T%twin representations of D- algebra
   {twin representations of $D$\Hyph algebra}%
   {twin representations of D algebra}%
\Index%320%T%twin representations of division ring
   {twin representations of division ring}%
   {twin representations of division ring}%
\Index%319%T%twin representations of fibered group
   {twin representations of fibered group}%
   {twin representations of fibered group}%
\Index%318%T%twin representations of group
   {twin representations of group}%
   {twin representations of group}%
\SetIndexSpace%
\Index%796%U%unit of ring of sets
   {unit of ring of sets}%
   {unit of ring of sets}%
\Index%315%U%unit sphere in algebra
   {unit sphere in $D$\Hyph algebra}%
   {unit sphere in algebra}%
\Index%160%U%unit sphere in division ring
   {unit sphere in division ring}%
   {unit sphere in division ring}%
\Index%523%U%unit vector
   {unit vector}%
   {unit vector}%
\Index%172%U%unitarity law for  Dstar- vector fields
   {unitarity law for  $\mathcal D\star$\Hyph vector fields}%
   {unitarity law, Dstar vector fields}%
\Index%664%U%unitarity law for Astar- module
   {unitarity law for $A\star$\Hyph module}%
   {unitarity law, Astar module over algebra}%
\Index%578%U%unitarity law for Astar- vector space
   {unitarity law for $A\star$\Hyph vector space}%
   {unitarity law, Astar vector space}%
\Index%656%U%unitarity law for D- module
   {unitarity law for $D$\Hyph module}%
   {unitarity law, D module}%
\Index%171%U%unitarity law for Dstar- vector space
   {unitarity law for $D\star$\Hyph vector space}%
   {unitarity law, Dstar vector space}%
\Index%673%U%unitarity law for starA- module
   {unitarity law for $\star A$\Hyph module}%
   {unitarity law, starA module over algebra}%
\Index%199%U%unitarity law for starD- vector space
   {unitarity law for $\star D$\Hyph vector space}%
   {unitarity law, starD vector space}%
\SetIndexSpace%
\Index%288%V%valued division ring
   {valued division ring}%
   {valued division ring}%
\Index%125%V%vector bundle
   {vector bundle}%
   {vector bundle}%
\Index%787%V%vector module of algebra
   {vector module of algebra}%
   {vector module of algebra}%
\Index%776%V%vector module of ring
   {vector module of ring}%
   {vector module of ring}%
\Index%785%V%vector of element of algebra
   {vector of element of algebra}%
   {vector of algebra}%
\Index%774%V%vector of element of ring
   {vector of element of ring}%
   {vector of ring}%
\Index%782%V%vector of mapping
   {vector of mapping}%
   {vector of mapping}%
\Index%126%V%vector potential
   {vector potential}%
   {vector potential}%
\Index%727%V%vector space over field
   {vector space over field}%
   {vector space over field}%
\Index%485%V%vector space type
   {vector space type}%
   {vector space type}%
\SetIndexSpace%
\Index%814%Z%zero divisor
   {zero divisor}%
   {zero divisor}%
\SetIndexSpace%
\Index%809%M%mu measurable map
   {$\mu$\Hyph measurable map}%
   {mu measurable map}%
\SetIndexSpace%
\Index%644%O%Omega group
   {$\Omega$\Hyph group}%
   {Omega group}%
\Index%646%O%Omega linear mapping
   {$\Omega$\Hyph linear mapping}%
   {Omega linear map}%
\Index%707%O%Omega_2- word of element of representation relative to generating set
   {$\Omega_2$\Hyph word of element of representation relative to generating set}%
   {word of element relative to generating set, representation}%
\SetIndexSpace%
\Index%658%S%sigma algebra of sets
   {$\sigma$\Hyph algebra of sets}%
   {sigma algebra of sets}%
\Index%795%S%sigma ring of sets
   {$\sigma$\Hyph ring of sets}%
   {sigma ring of sets}%

\CloseIndex


==> Index.Russian.tex <==
%auto-ignore
\OpenIndex
\SetIndexSpace%
\Index%1%1%1-форма
   {$1$\Hyph форма}%
   {1-form}%
\SetIndexSpace%
\Index%2%2%2- арное расслоенное отношение
   {$2$\Hyph арное расслоенное отношение}%
   {2 ary fibered relation}%
\SetIndexSpace%
\Index%819%A%A алгебра многочленов над D алгеброй
   {$A$\Hyph алгебра многочленов над $D$\Hyph алгеброй $A$}%
   {algebra of polynomials over algebra}%
\Index%5%A%A- значная функция
   {$A$\Hyph значная функция}%
   {A valued function}%
\Index%693%A%A линейное отображение модулей
   {$A$\Hyph линейное отображение модулей}%
   {A linear map of modules}%
\Index%685%A%A- модуль
   {$A$\Hyph модуль}%
   {module over algebra}%
\Index%818%A%A число
   {$A$\Hyph число}%
   {A number}%
\Index%603%A%A(A) отображение
   {$\mathcal A(A)$\Hyph отображение}%
   {A(A) mapping}%
\Index%680%A%Acr линейное отображение модулей
   {\Acr линейное отображение модулей}%
   {Acr linear map of modules}%
\Index%764%A%ACRcirc линейная комбинация
   {$A\CRcirc$\Hyph линейная комбинация}%
   {ACRcirc linear combination}%
\Index%582%A%Arc базис в векторном пространстве
   {$A\RCstar$\Hyph базис в векторном пространстве}%
   {Arc basis, vector space}%
\Index%789%A%Astar антилинейное отображение алгебры с сопряжением
   {$A\star$\Hyph антилинейное отображение алгебры с сопряжением}%
   {antilinear mapping of algebra with conjugation}%
\Index%575%A%Astar векторное пространство
   {$A\star$\Hyph векторное пространство}%
   {Astar vector space}%
\Index%583%A%Astar линейное отображение векторных пространств
   {$A\star$\Hyph линейное отображение векторных пространств}%
   {Astar linear map of vector spaces}%
\Index%660%A%Astar- модуль
   {$A\star$\Hyph модуль}%
   {Astar-module}%
\Index%665%A%Astar- произведение вектора на скаляр
   {$A\star$\Hyph произведение вектора на скаляр}%
   {Astar product of vector over scalar, Astar module}%
\Index%579%A%Astar-произведение вектора на скаляр
   {$A\star$\hyph произведение вектора на скаляр}%
   {Astar product of vector over scalar, vector space}%
\Index%3%A%j i-CR квазидетерминант
   {$(^j_i)$\hyph \CR квазидетерминант}%
   {j i cr-quasideterminant}%
\SetIndexSpace%
\Index%799%B%b множество
   {$B$\Hyph множество}%
   {B set}%
\SetIndexSpace%
\Index%6%C%c строка матрицы
   {\subs строка матрицы}%
   {c row}%
\Index%7%C%CR матричная группа
   {\CR матричная группа}%
   {cr-matrix group}%
\Index%8%C%CR обратный элемент бикольца
   {\CR обратный элемент бикольца}%
   {cr-inverse element}%
\Index%9%C%CR произведение матриц
   {\CR произведение матриц}%
   {cr-product of matrices}%
\Index%589%C%cr произведение матриц отображений
   {$\CRcirc$\Hyph произведение матриц отображений}%
   {cr product of matrices of mappings}%
\Index%10%C%CR степень
   {\CR степень}%
   {cr power}%
\Index%11%C%crd векторное пространство
   {\crd векторное пространство}%
   {crd vector space}%
\Index%768%C%Cstar-алгебра
   {$C^*$\Hyph алгебра}%
   {Cstar-algebra}%
\Index%12%C%c-строка матрицы
   {$c$\hyph строка матрицы}%
   {c-row}%
\SetIndexSpace%
\Index%251%D%D- алгебра
   {$D$\Hyph алгебра}%
   {D algebra}%
\Index%549%D%D- аффинная связность на многообразии аффинной связности
   {$D$\Hyph аффинная связность на многообразии аффинной связности}%
   {D affine connection, affine manifold}%
\Index%23%D%d аффинное пространство
   {$D$\Hyph аффинное пространство}%
   {d affine space}%
\Index%14%D%D- вектор- функция
   {$D$\Hyph вектор\Hyph функция}%
   {d vector function}%
\Index%48%D%D- значная переменная
   {$D$\Hyph значная переменная}%
   {D valued variable}%
\Index%581%D%D линейный функционал
   {$D$\Hyph линейный функционал}%
   {D linear functional}%
\Index%584%D%D- модуль
   {$D$\Hyph модуль}%
   {D module}%
\Index%71%D%D- модуль
   {$D$\Hyph модуль}%
   {D-module}%
\Index%18%D%dcr векторное пространство
   {\dcr векторное пространство}%
   {dcr vector space}%
\Index%38%D%dcr производная Гато отображения f D- векторного пространства V в D- векторное пространство W
   {\dcr производная Гато отображения $\Vector f$ $D$\Hyph векторного пространства $V$ в $D$\Hyph векторное пространство $W$}%
   {Gateaux dcr derivative of map, D vector space}%
\Index%26%D%Drc базис в векторном расслоении
   {\Drc базис в векторном расслоении}%
   {drc basis, vector bundle}%
\Index%17%D%drc вектор
   {\drc вектор}%
   {drc vector}%
\Index%28%D%drc векторное пространство
   {\drc векторное пространство}%
   {drc vector space}%
\Index%19%D%drc векторное пространство r строк
   {\drc векторное пространство \subs строк}%
   {subs rows drc vector space}%
\Index%36%D%Drc линейное отображение векторных расслоений
   {\Drc линейное отображение векторных расслоений}%
   {drc linear map of vector bundles}%
\Index%70%D%drc представление группы
   {\drc представление группы}%
   {drc linear representation of group}%
\Index%779%D%Dstar антилинейное отображение кольца с сопряжением
   {$D\star$\Hyph антилинейное отображение кольца с сопряжением}%
   {antilinear mapping of ring with conjugation}%
\Index%771%D%Dstar антилинейный гомоморфизм
   {$D\star$\Hyph антилинейный гомоморфизм}%
   {Dstar antilinear homomorphism}%
\Index%734%D%Dstar аффинное пространство
   {$D\star$\Hyph аффинное пространство}%
   {Dstar affine space}%
\Index%39%D%Dstar- векторное поле
   {$\mathcal D\star$\Hyph векторное поле}%
   {Dstar vector field}%
\Index%41%D%Dstar- векторное расслоение
   {$\mathcal D\star$\Hyph векторное расслоение}%
   {Dstar vector bundle}%
\Index%769%D%Dstar линейный гомоморфизм
   {$D\star$\Hyph линейный гомоморфизм}%
   {Dstar linear homomorphism}%
\Index%46%D%Dstar производная Гато функции f тела D
   {\Ds производная Гато функции $f$ тела $D$}%
   {Gateaux Dstar derivative of map, division ring}%
\Index%47%D%Dstar производная Фреше отображения f тела D в точке x
   {\Ds производная Фреше отображения $f$ тела $D$ в точке $x$}%
   {Frechet Dstar derivative of map, division ring}%
\Index%40%D%Dstar-векторное пространство
   {$D\star$\hyph векторное пространство}%
   {Dstar vector space}%
\Index%43%D%Dstar-линейная комбинация векторных полей
   {$\mathcal D\star$\hyph линейная комбинация векторных полей}%
   {linear composition of vector fields}%
\Index%156%D%Dstar-модуль
   {$D\star$\Hyph модуль}%
   {Dstar-module}%
\Index%44%D%Dstar-произведение вектора на скаляр
   {$D\star$\hyph произведение вектора на скаляр}%
   {Dstar product of vector over scalar, vector space}%
\Index%45%D%Dstar-произведение векторного поля на скаляр
   {$\mathcal D\star$\hyph произведение векторного поля на скаляр}%
   {Dstar product of vector field over scalar, vector space}%
\Index%15%D%D-векторное пространство
   {$D$\hyph векторное пространство}%
   {D vector space}%
\Index%32%D%rcd линейная оболочка в векторном пространстве
   {\rcd линейная оболочка в векторном пространстве}%
   {linear span, vector space}%
\SetIndexSpace%
\Index%50%E%enhanced Lie group
   {enhanced Lie group}%
   {enhanced Lie group}%
\SetIndexSpace%
\Index%55%G%$G$\Hyph пространство
   {$G$\Hyph пространство}%
   {GSpace}%
\Index%52%G%G- система отсчёта
   {$G$\Hyph система отсчёта}%
   {G reference frame}%
\Index%53%G%G-basis векторного пространства
   {$G$\Hyph базис векторного пространства}%
   {G-basis}%
\Index%54%G%G-координаты базиса
   {$G$\Hyph координаты базиса}%
   {G-coordinates}%
\SetIndexSpace%
\Index%596%J%j i RCcirc квазидетерминант
   {$(^j_i)$\hyph $\RCcirc$\Hyph квазидетерминант}%
   {j i RCcirc-quasideterminant}%
\Index%678%J%ji- квазидетерминант
   {$(ji)$\hyph квазидетерминант}%
   {j i quasideterminant}%
\SetIndexSpace%
\Index%57%M%m- вектор
   {$m$\Hyph вектор}%
   {m-vector}%
\Index%56%M%m- мерный параллепипед
   {$m$\Hyph мерный параллепипед}%
   {m dimensional parallelepiped}%
\SetIndexSpace%
\Index%726%N%n алгебра над кольцом
   {$n$\Hyph алгебра над кольцом}%
   {n algebra over ring}%
\Index%58%N%n- арное расслоенное отношение
   {$n$\Hyph арное расслоенное отношение}%
   {fibered relation}%
\SetIndexSpace%
\Index%4%R%j i-RC квазидетерминант
   {$(^j_i)$\hyph \RC квазидетерминант}%
   {j i RC-quasideterminant}%
\Index%728%R%R- модуль
   {$R$\Hyph модуль}%
   {R- module}%
\Index%59%R%r строка матрицы
   {\sups строка матрицы}%
   {r row}%
\Index%60%R%RC вырожденная матрица
   {\RC вырожденная матрица}%
   {RC singular matrix}%
\Index%61%R%RC главная минорная матрица
   {\RC главная минорная матрица}%
   {RC-major minor}%
\Index%62%R%RC квазидетерминант
   {\RC квазидетерминант}%
   {RC-quasideterminant}%
\Index%63%R%RC матричная группа
   {\RC матричная группа}%
   {rc-matrix group}%
\Index%64%R%RC невырожденная матрица
   {\RC невырожденная матрица}%
   {RC nonsingular matrix}%
\Index%65%R%RC обратный элемент бикольца
   {\RC обратный элемент бикольца}%
   {rc-inverse element}%
\Index%66%R%RC произведение матриц
   {\RC произведение матриц}%
   {rc-product of matrices}%
\Index%590%R%rc произведение матриц отображений
   {$\RCcirc$\Hyph произведение матриц отображений}%
   {rc product of matrices of mappings}%
\Index%67%R%RC ранг матрицы
   {\RC ранг матрицы}%
   {rc-rank of matrix}%
\Index%68%R%RC степень
   {\RC степень}%
   {rc power}%
\Index%600%R%RCcirc вырожденная матрица A(A) отображений
   {$\RCcirc$\Hyph вырожденная матрица $\mathcal A(A)$\Hyph отображений}%
   {RCcirc singular matrix of A(A) mappings}%
\Index%599%R%RCcirc вырожденная матрица эндоморфизмов
   {$\RCcirc$\Hyph вырожденная матрица эндоморфизмов}%
   {RCcirc singular matrix of endomorphisms}%
\Index%597%R%RCcirc квазидетерминант
   {$\RCcirc$\Hyph квазидетерминант}%
   {RCcirc-quasideterminant definition}%
\Index%601%R%RCcirc невырожденная матрица A(A) отображений
   {$\RCcirc$\Hyph невырожденная матрица $A(A)$\Hyph отображений}%
   {RCcirc nonsingular matrix of A(A) mappings}%
\Index%598%R%RCcirc невырожденная матрица эндоморфизмов
   {$\RCcirc$\Hyph невырожденная матрица эндоморфизмов}%
   {RCcirc nonsingular matrix of endomorphisms}%
\Index%602%R%RCcirc невырожденная система аддитивных уравнений
   {$\RCcirc$\Hyph невырожденная система аддитивных уравнений}%
   {RCcirc nonsingular system of additive equations}%
\Index%765%R%RCcircA линейная комбинация
   {$\RCcirc A$\Hyph линейная комбинация}%
   {RCcircA linear combination}%
\Index%22%R%rcd автоморфизм векторного пространства
   {\rcd автоморфизм векторного пространства}%
   {automorphism of vector space}%
\Index%759%R%rcd аффинная плоскость
   {\rcd аффинная плоскость}%
   {rcd affine plane}%
\Index%758%R%rcd аффинное преобразование
   {\rcd аффинное преобразование}%
   {rcd affine transformation}%
\Index%736%R%rcd аффинное пространство
   {\rcd аффинное пространство}%
   {rcd affine space}%
\Index%111%R%rcd аффинный базис
   {\rcd аффинный базис}%
   {rcd affine basis, division ring}%
\Index%27%R%rcd вектор
   {\rcd вектор}%
   {rcd vector}%
\Index%69%R%rcd векторное пространство
   {\rcd векторное пространство}%
   {rcd vector space}%
\Index%29%R%rcd векторное пространство c строк
   {\rcd векторное пространство \sups строк}%
   {sups rows rcd vector space}%
\Index%31%R%rcd изоморфизм векторных пространств
   {\rcd изоморфизм векторных пространств}%
   {isomorphism of vector spaces}%
\Index%37%R%rcd линейным Tstar- представление группы
   {\rcd линейным \Ts представление группы}%
   {rcd linear Tstar representation of group}%
\Index%13%R%rcd производная Гато отображения f D-векторного пространства V в D-векторное пространство W
   {\rcd производная Гато отображения $f$ $D$\hyph векторного пространства $V$ в $D$\hyph векторное пространство $W$}%
   {Gateaux rcd derivative of map, D vector space}%
\Index%72%R%r-строка матрицы
   {$r$\hyph строка матрицы}%
   {r-row}%
\Index%510%R%частная rcd производная Гато отображения fb по переменной xa
   {частная \rcd производная Гато отображения $f^{\gi b}$ по переменной $x^{\gi a}$}%
   {Gateaux partial rcd derivative of map with respect to variable, D vector space}%
\SetIndexSpace%
\Index%73%S%RCstarS,RCstarT- линейное отображение векторных пространств
   {$(\RCstar S,\RCstar T)$\Hyph линейное отображение векторных пространств}%
   {rcs rct linear map of vector spaces}%
\Index%74%S%SRCstar,TRCstar- линейное отображение векторных расслоений
   {$(\mathcal S\RCstar,\mathcal T\RCstar)$\Hyph линейное отображение векторных расслоений}%
   {src trc linear map of vector bundles}%
\Index%112%S%Sstar, star T-бимодуль
   {($S\star$, $\star T$)\hyph бимодуль}%
   {(Sstar,starT)-bimodule}%
\Index%669%S%star A- модуль
   {$\star A$\Hyph модуль}%
   {starA-module}%
\Index%78%S%star D-векторное пространство
   {$\star D$\hyph векторное пространство}%
   {starD-vector space}%
\Index%79%S%star R-модуль
   {$\star R$\hyph модуль}%
   {starR-module}%
\Index%674%S%starA- произведение вектора на скаляр
   {$\star A$\Hyph произведение вектора на скаляр}%
   {starA product of vector over scalar, starA module}%
\Index%735%S%starD аффинное пространство
   {$\star D$\Hyph аффинное пространство}%
   {starD affine space}%
\Index%192%S%starD- векторное пространство
   {$\star D$\Hyph векторное пространство}%
   {starD vector space}%
\Index%76%S%starD производная Гато функции f тела D
   {\sD производная Гато функции $f$ тела $D$}%
   {Gateaux starD derivative of map, division ring}%
\Index%198%S%starD-произведение вектора на скаляр
   {$\star D$\hyph произведение вектора на скаляр}%
   {starD product of vector over scalar, vector space}%
\Index%82%S%starT- представление Omega1 алгебры A в Omega2 алгебре M
   {\sT представление $\Omega_1$\Hyph алгебры $A$ в $\Omega_2$\Hyph алгебре $M$}%
   {starT representation of algebra}%
\Index%83%S%starT- представление расслоенной Omega- алгебры
   {\sT представление расслоенной $\Omega$\Hyph алгебры}%
   {starT representation of fibered Omega-algebra}%
\Index%84%S%starT- представление расслоенной группы
   {\sT представление расслоенной группы}%
   {starT representation of fibered group}%
\Index%85%S%starT- преобразование
   {\sT преобразование}%
   {starT transformation}%
\Index%86%S%starT- преобразование расслоения
   {\sT преобразование расслоения}%
   {starT transformation of bundle}%
\Index%80%S%starT- сдвиг
   {\sT сдвиг}%
   {starT shift}%
\Index%81%S%starT- сдвиг на расслоении групп
   {\sT сдвиг на расслоении групп}%
   {starT shift, fibered group}%
\SetIndexSpace%
\Index%87%T%Tstar- векторное пространство матриц
   {\Ts векторное пространство матриц}%
   {matrices vector space}%
\Index%90%T%Tstar- представление Omega1 алгебры A в Omega2 алгебре M
   {\Ts представление $\Omega_1$\Hyph алгебры $A$ в $\Omega_2$\Hyph алгебре $M$}%
   {Tstar representation of algebra}%
\Index%91%T%Tstar- представление расслоенной Omega- алгебры
   {\Ts представление расслоенной $\Omega$\Hyph алгебры}%
   {Tstar representation of fibered Omega-algebra}%
\Index%92%T%Tstar- преобразование
   {\Ts преобразование}%
   {Tstar transformation}%
\Index%93%T%Tstar- преобразование расслоения
   {\Ts преобразование расслоения}%
   {Tstar transformation of bundle}%
\Index%89%T%Tstar- сдвиг
   {\Ts сдвиг}%
   {Tstar shift}%
\SetIndexSpace%
\Index%645%А%абелевая Omega группа
   {абелевая $\Omega$\Hyph группа}%
   {Abelian Omega group}%
\Index%560%А%автоморфизм башни представлений
   {автоморфизм башни представлений}%
   {automorphism of tower of representations}%
\Index%94%А%автоморфизм представления Omega алгебры
   {автоморфизм представления $\Omega$\Hyph алгебры}%
   {automorphism of representation}%
\Index%95%А%автопараллельная кривая
   {автопараллельная кривая}%
   {auto parallel line}%
\Index%805%А%аддитивное отображение
   {аддитивное отображение}%
   {additive map}%
\Index%99%А%активное starT- представление
   {активное \sT представление}%
   {active representation, vector space}%
\Index%100%А%активное представление
   {активное представление}%
   {active representation}%
\Index%716%А%активное представление группы в многообразии базисов башни представлений
   {активное представление группы $G(\Vector  f)$ в многообразии базисов  башни представлений}%
   {active representation in basis manifold, tower of representations}%
\Index%569%А%активное представление группы в многообразии базисов представления
   {активное представление группы $G(f)$ в многообразии базисов представления}%
   {active representation in basis manifold}%
\Index%715%А%активное преобразование многообразия базисов башни представлений
   {активное преобразование многообразия базисов башни представлений}%
   {active transformation of basis, tower of representations}%
\Index%326%А%активное преобразование многообразия базисов представления
   {активное преобразование многообразия базисов представления}%
   {active transformation of basis, representation}%
\Index%101%А%активное преобразование на многообразии базисов
   {активное преобразование на многообразии базисов}%
   {active transformation}%
\Index%102%А%активное преобразование на множестве rcd базисов
   {активное преобразование на множестве \rcd базисов}%
   {active transformation, vector space}%
\Index%103%А%алгебра E кватернионов над полем F
   {алгебра $E$ кватернионов над полем $F$}%
   {quaternion algebra over the field}%
\Index%808%А%алгебра Бореля
   {алгебра Бореля}%
   {Borel algebra}%
\Index%104%А%алгебра Ли группы Ли
   {алгебра Ли группы Ли}%
   {algebra Lie group Lie}%
\Index%487%А%алгебра многочленов над D алгеброй
   {алгебра многочленов над $D$\Hyph алгеброй}%
   {algebra of polynomials over D algebra}%
\Index%797%А%алгебра множеств
   {алгебра множеств}%
   {algebra of sets}%
\Index%607%А%алгебра над кольцом
   {алгебра над кольцом}%
   {algebra over ring}%
\Index%639%А%алгебра октонионов
   {алгебра октонионов}%
   {octonion algebra}%
\Index%618%А%алгебра рациональных отображений алгебры
   {алгебра рациональных отображений алгебры}%
   {algebra of rational mappings of algebra}%
\Index%780%А%алгебра с сопряжением
   {алгебра с сопряжением}%
   {algebra with conjugation}%
\Index%786%А%алгебра скаляров алгебры
   {алгебра скаляров алгебры}%
   {scalar algebra of algebra}%
\Index%775%А%алгебра скаляров кольца
   {алгебра скаляров кольца}%
   {scalar algebra of ring}%
\Index%400%А%алгебра частных алгебры с сопряжением
   {алгебра частных алгебры с сопряжением}%
   {algebra of fractions of algebra with conjugation}%
\Index%623%А%алгебра, противоположная алгебре
   {алгебра, противоположная алгебре $P$}%
   {opposite algebra}%
\Index%105%А%альтернативное представление матрицы
   {альтернативное представление матрицы}%
   {Alternative representation}%
\Index%106%А%антигомоморфизм расслоенных групп
   {антигомоморфизм расслоенных групп}%
   {antihomomorphism of fibered groups}%
\Index%107%А%антисимметричное 2- арное расслоенное отношение
   {антисимметричное $2$\Hyph арное расслоенное отношение}%
   {antisymmetric 2 ary fibered relation}%
\Index%108%А%арность операции
   {арность операции}%
   {arity of operation}%
\Index%617%А%ассоциативная D алгебра
   {ассоциативная $D$\Hyph алгебра}%
   {associative D algebra}%
\Index%616%А%ассоциатор D алгебры
   {ассоциатор $D$\Hyph алгебры}%
   {associator of algebra}%
\Index%733%А%аффинная структура на множестве
   {аффинная структура на множестве}%
   {affine structure on set}%
\Index%109%А%аффинное преобразование на многообразии базисов
   {аффинное преобразование на многообразии базисов}%
   {affine transformation}%
\Index%110%А%аффинный базис
   {аффинный базис}%
   {Affine Basis}%
\SetIndexSpace%
\Index%113%Б%база отображения
   {база отображения}%
   {base of map}%
\Index%114%Б%база расслоенного соответствия
   {база расслоенного соответствия}%
   {base of fibered correspondence}%
\Index%16%Б%базис drc векторного пространства r строк
   {базис \drc векторного пространства \subs строк}%
   {basis, r rows drc vector space}%
\Index%653%Б%базис алгебры L(A;A)
   {базис алгебры $\mathcal L(A;A)$}%
   {basis of algebra L(A,A)}%
\Index%567%Б%базис башни представлений
   {базис башни представлений}%
   {basis of tower of representations}%
\Index%197%Б%базис в D векторном пространстве
   {базис в $D$\Hyph векторном пространстве}%
   {basis, D vector space}%
\Index%24%Б%базис в rcd векторном пространстве
   {базис в \rcd векторном пространстве}%
   {basis, rcd vector space}%
\Index%25%Б%базис в rcd векторном пространстве c строк
   {базис в \rcd векторном пространстве \sups строк}%
   {basis, c rows rcd vector space}%
\Index%115%Б%базис векторного пространства
   {базис векторного пространства}%
   {Basis}%
\Index%783%Б%базис Гамеля
   {базис Гамеля}%
   {Hamel basis}%
\Index%659%Б%базис модуля
   {базис модуля}%
   {basis, module}%
\Index%329%Б%базис представления
   {базис представления}%
   {basis of representation}%
\Index%791%Б%базис Шаудера
   {базис Шаудера}%
   {Schauder basis}%
\Index%223%Б%базис, двойственный базису
   {базис, двойственный базису}%
   {dual basis}%
\Index%49%Б%базис, дуальный базису
   {базис, дуальный базису}%
   {basis dual to basis}%
\Index%117%Б%базовый вектор представления группы Ли
   {базовый вектор представления группы Ли}%
   {basis vector of representation of Lie group}%
\Index%116%Б%базовый вектор представления группы Ли над алгеброй A
   {базовый вектор представления группы Ли над алгеброй $A$}%
   {basis vector of representation of Lie group over algebra A}%
\Index%118%Б%базовый оператор группы Ли
   {базовый оператор группы Ли}%
   {Lie group basic operators}%
\Index%503%Б%банахова D- алгебра
   {банахова $D$\Hyph алгебра}%
   {Banach algebra}%
\Index%313%Б%банаховый D- модуль
   {банаховый $D$\Hyph модуль}%
   {Banach module}%
\Index%531%Б%башня подпредставлений
   {башня подпредставлений}%
   {tower of subrepresentations}%
\Index%532%Б%башня подпредставлений башни представлений, порождённая кортежем множеств
   {башня подпредставлений башни представлений $\Vector f$, порождённая кортежем множеств $\VX X$}%
   {subrepresentation generated by tuple of sets}%
\Index%119%Б%башня представлений Omega алгебр
   {башня представлений $\Vector{\Omega}$\Hyph алгебр}%
   {tower of representations of algebras}%
\Index%120%Б%башня расслоений
   {башня расслоений}%
   {tower of bundles}%
\Index%324%Б%башня эффективных представлений
   {башня эффективных представлений}%
   {tower of effective representations}%
\Index%121%Б%бесконечно малый генератор
   {бесконечно малый генератор}%
   {infinitesimal generator}%
\Index%122%Б%бикольцо
   {бикольцо}%
   {biring}%
\Index%798%Б%борелевское множество
   {борелевское множество}%
   {Borel set}%
\Index%803%Б%борелевское отображение
   {борелевское отображение}%
   {Borel-measurable map}%
\SetIndexSpace%
\Index%123%В%вектор Килинга второго рода
   {вектор Килинга второго рода}%
   {Killing vector second type}%
\Index%782%В%вектор отображения
   {вектор отображения}%
   {vector of mapping}%
\Index%785%В%вектор элемента алгебры
   {вектор элемента алгебры}%
   {vector of algebra}%
\Index%774%В%вектор элемента кольца
   {вектор элемента кольца}%
   {vector of ring}%
\Index%727%В%векторное пространство над полем
   {векторное пространство над полем}%
   {vector space over field}%
\Index%125%В%векторное расслоение
   {векторное расслоение}%
   {vector bundle}%
\Index%126%В%векторный потенциал
   {векторный потенциал}%
   {vector potential}%
\Index%124%В%вектор-столбец
   {вектор\hyph столбец}%
   {column vector}%
\Index%127%В%вектор-строка
   {вектор\hyph строка}%
   {row vector}%
\Index%128%В%вполне интегрируемая система
   {вполне интегрируемая система}%
   {completely integrable system}%
\Index%651%В%времениподобный вектор
   {времениподобный вектор}%
   {timelike vector}%
\Index%129%В%второй закон Ньютона
   {второй закон Ньютона}%
   {Second Newton law}%
\Index%130%В%вырожденное линейное отображение
   {вырожденное линейное отображение}%
   {singular linear map}%
\SetIndexSpace%
\Index%132%Г%геометрический объект в векторном пространстве
   {геометрический объект в векторном пространстве}%
   {geometric object, vector space}%
\Index%133%Г%геометрический объект в координатном представлении
   {геометрический объект в координатном представлении}%
   {geometric object, coordinate vector space}%
\Index%698%Г%геометрический объект в координатном представлении, определённом в Omega_2- алгебре
   {геометрический объект в координатном представлении, определённом в $\Omega_2$\Hyph алгебре $M$}%
   {geometric object, coordinate representation g}%
\Index%134%Г%геометрический объект в координатном представлении, определённом в rcd векторном пространстве
   {геометрический объект в координатном представлении, определённом в \rcd векторном пространстве}%
   {geometric object, coordinate rcd vector space}%
\Index%719%Г%геометрический объект в координатном представлении, определённом в кортеже Omega- алгебр
   {геометрический объект в координатном представлении, определённом в кортеже $\VX\Omega$\Hyph алгебр $\VX A$}%
   {geometric object, coordinate tower of representations g}%
\Index%704%Г%геометрический объект типа
   {геометрический объект типа $H$}%
   {geometric object of type H, representation g}%
\Index%135%Г%геометрический объект типа A
   {геометрический объект типа $A$ в векторном пространстве}%
   {geometric object of type A, vector space}%
\Index%700%Г%геометрический объект, определённый в Omega_2- алгбре
   {геометрический объект, определённый в $\Omega_2$\Hyph алгбре $M$}%
   {geometric object, representation g}%
\Index%136%Г%геометрический объект, определённый в rcd векторном пространстве
   {геометрический объект, определённый в \rcd векторном пространстве}%
   {geometric object, rcd vector space}%
\Index%722%Г%геометрический объект, определённый в кортеже Omega- алгебр
   {геометрический объект, определённый в кортеже $\VX\Omega$\Hyph алгебр $\VX A$}%
   {geometric object, tower of representations g}%
\Index%767%Г%главный идеал
   {главный идеал}%
   {principal ideal}%
\Index%137%Г%голономные координаты вектора
   {голономные координаты вектора}%
   {vector holonomic coordinates}%
\Index%138%Г%голономные координаты связности
   {голономные координаты связности}%
   {holonomic coordinates of connection}%
\Index%140%Г%гомоморфизм расслоенных групп
   {гомоморфизм расслоенных групп}%
   {homomorphism of fibered groups}%
\Index%139%Г%гомоморфизм расслоенных универсальных алгебр
   {гомоморфизм расслоенных универсальных алгебр}%
   {homomorphism of fibered universal algebras}%
\Index%568%Г%группа автоморфизмов представления
   {группа автоморфизмов представления}%
   {group of automorphisms of representation}%
\Index%141%Г%группа аффинных преобразований
   {группа аффинных преобразований}%
   {drc affine transformation group}%
\Index%142%Г%группа аффинных преобразований
   {группа аффинных преобразований}%
   {affine transformation group}%
\Index%143%Г%группа симметрии
   {группа симметрии}%
   {symmetry group}%
\Index%144%Г%группа симметрии
   {группа симметрии}%
   {SymmetryGroup}%
\Index%145%Г%группа стабилизации
   {группа стабилизации}%
   {stability group}%
\Index%146%Г%групповая алгебра
   {групповая алгебра}%
   {group algebra}%
\SetIndexSpace%
\Index%147%Д%движение на многообразии базисов
   {движение на многообразии базисов}%
   {movement transformation}%
\Index%586%Д%движение пространства Минковского
   {движение пространства Минковского}%
   {motion, Minkowski space}%
\Index%755%Д%двойной определитель
   {двойной определитель}%
   {double determinant}%
\Index%148%Д%декартова степень A множества B
   {декартова степень $A$ множества $B$}%
   {Cartesian power of set}%
\Index%149%Д%декартова степень A расслоения B
   {декартова степень $\Bundle A$ расслоения $\Bundle B$}%
   {Cartesian power A of bundle B}%
\Index%594%Д%декартова степень n H алгебры
   {декартова степень $n$ $\mathfrak{H}$\Hyph алгебры}%
   {Cartesian power of algebra}%
\Index%150%Д%декартова степень n расслоения E
   {декартова степень $n$ расслоения $\Bundle E$}%
   {Cartesian power n of bundle E}%
\Index%151%Д%декартово произведение расслоений
   {декартово произведение расслоений}%
   {Cartesian product of bundles}%
\Index%152%Д%декартово произведение расслоенных пространств
   {декартово произведение расслоенных пространств}%
   {Cartesian product of total spaces}%
\Index%820%Д%делитель многочлена
   {делитель многочлена}%
   {divisor of polynomial}%
\Index%814%Д%делитель нуля
   {делитель нуля}%
   {zero divisor}%
\Index%153%Д%диагональ в расслоении
   {диагональ в расслоении}%
   {diagonal in bundle}%
\Index%725%Д%диаграмма представлений
   {диаграмма представлений}%
   {diagram of representations}%
\Index%154%Д%диаграмма соответствий
   {диаграмма соответствий}%
   {diagram of correspondences}%
\Index%157%Д%дифференциал Гато отображения
   {дифференциал Гато отображения}%
   {Gateaux differential of map}%
\Index%159%Д%дуальное пространство к rcd векторному пространству
   {дуальное пространство к \rcd векторному пространству}%
   {dual space of rcd vector space}%
\SetIndexSpace%
\Index%796%Е%единица кольца множеств
   {единица кольца множеств}%
   {unit of ring of sets}%
\Index%315%Е%единичная сфера в алгебре
   {единичная сфера в $D$\Hyph алгебре}%
   {unit sphere in algebra}%
\Index%160%Е%единичная сфера в теле
   {единичная сфера в теле}%
   {unit sphere in division ring}%
\Index%523%Е%единичный вектор
   {единичный вектор}%
   {unit vector}%
\SetIndexSpace%
\Index%576%З%закон ассоциативности для Astar- векторного пространства
   {закон ассоциативности для $A\star$\Hyph векторного пространства}%
   {associative law, Astar vector space}%
\Index%585%З%закон ассоциативности для Astar линейных отображений векторных пространств
   {закон ассоциативности для $A\star$\Hyph линейных отображений векторных пространств}%
   {associative law for Astar linear mappings of vector spaces}%
\Index%662%З%закон ассоциативности для Astar- модуля
   {закон ассоциативности для $A\star$\Hyph модуля}%
   {associative law, Astar module over algebra}%
\Index%654%З%закон ассоциативности для D- модуля
   {закон ассоциативности для $D$\Hyph модуля}%
   {associative law, D module}%
\Index%162%З%закон ассоциативности для Drc линейных отображений векторных расслоений
   {закон ассоциативности для \Drc линейных отображений векторных расслоений}%
   {associative law for drc linear maps of vector bundles}%
\Index%163%З%закон ассоциативности для Dstar- векторного пространства
   {закон ассоциативности для $D\star$\Hyph векторного пространства}%
   {associative law, Dstar vector space}%
\Index%164%З%закон ассоциативности для Dstar- векторных полей
   {закон ассоциативности для $\mathcal D\star$\Hyph векторных полей}%
   {associative law, Dstar vector fields}%
\Index%161%З%закон ассоциативности для rcd линейных отображений векторных пространств
   {закон ассоциативности для \rcd линейных отображений векторных пространств}%
   {associative law for rcd linear maps of vector spaces}%
\Index%671%З%закон ассоциативности для starA- модуля
   {закон ассоциативности для $\star A$\Hyph модуля}%
   {associative law, starA module over algebra}%
\Index%501%З%закон ассоциативности для starD- векторного пространства
   {закон ассоциативности для $\star D$\Hyph векторного пространства}%
   {associative law, starD vector space}%
\Index%165%З%закон ассоциативности для ковариантного starT- представления
   {закон ассоциативности для ковариантного \sT представления}%
   {associative law for covariant starT representation}%
\Index%166%З%закон ассоциативности для ковариантного Tstar- представления
   {закон ассоциативности для ковариантного \Ts представления}%
   {associative law for covariant Tstar representation}%
\Index%167%З%закон ассоциативности для парных представлений
   {закон ассоциативности для парных представлений}%
   {associative law for twin representations}%
\Index%168%З%закон ассоциативности произведения расслоенных соответствий
   {закон ассоциативности произведения расслоенных соответствий}%
   {associative law, composition of fibered correspondences}%
\Index%577%З%закон дистрибутивности для Astar- векторного пространства
   {закон дистрибутивности для $A\star$\Hyph векторного пространства}%
   {distributive law, Astar vector space}%
\Index%663%З%закон дистрибутивности для Astar- модуля
   {закон дистрибутивности для $A\star$\Hyph модуля}%
   {distributive law, Astar module over algebra}%
\Index%655%З%закон дистрибутивности для D- модуля
   {закон дистрибутивности для $D$\Hyph модуля}%
   {distributive law, D module}%
\Index%169%З%закон дистрибутивности для Dstar- векторного пространства
   {закон дистрибутивности для $D\star$\Hyph векторного пространства}%
   {distributive law, Dstar vector space}%
\Index%170%З%закон дистрибутивности для Dstar- векторных полей
   {закон дистрибутивности для $\mathcal D\star$\Hyph векторных полей}%
   {distributive law, Dstar vector fields}%
\Index%672%З%закон дистрибутивности для starA- модуля
   {закон дистрибутивности для $\star A$\Hyph модуля}%
   {distributive law, starA module over algebra}%
\Index%625%З%закон дистрибутивности для starD- векторного пространства
   {закон дистрибутивности для $\star D$\Hyph векторного пространства}%
   {distributive law, starD vector space}%
\Index%578%З%закон унитарности для Astar- векторного пространства
   {закон унитарности для $A\star$\Hyph векторного пространства}%
   {unitarity law, Astar vector space}%
\Index%664%З%закон унитарности для Astar- модуля
   {закон унитарности для $A\star$\Hyph модуля}%
   {unitarity law, Astar module over algebra}%
\Index%656%З%закон унитарности для D- модуля
   {закон унитарности для $D$\Hyph модуля}%
   {unitarity law, D module}%
\Index%171%З%закон унитарности для Dstar- векторного пространства
   {закон унитарности для $D\star$\Hyph векторного пространства}%
   {unitarity law, Dstar vector space}%
\Index%172%З%закон унитарности для Dstar- векторных полей
   {закон унитарности для $\mathcal D\star$\Hyph векторных полей}%
   {unitarity law, Dstar vector fields}%
\Index%673%З%закон унитарности для starA- модуля
   {закон унитарности для $\star A$\Hyph модуля}%
   {unitarity law, starA module over algebra}%
\Index%199%З%закон унитарности для starD- векторного пространства
   {закон унитарности для $\star D$\Hyph векторного пространства}%
   {unitarity law, starD vector space}%
\Index%807%З%замкнутый шар
   {замкнутый шар}%
   {closed ball}%
\SetIndexSpace%
\Index%459%И%идеал алгебры
   {идеал алгебры}%
   {ideal of algebra}%
\Index%800%И%измеримое отображение
   {измеримое отображение}%
   {measurable map}%
\Index%266%И%изоморфизм представлений Omega- алгебры
   {изоморфизм представлений $\Omega$\Hyph алгебры}%
   {isomorphism of repesentations of Omega algebra}%
\Index%173%И%изоморфизм расслоенных Omega- алгебр
   {изоморфизм расслоенных $\Omega$\Hyph алгебр}%
   {isomorphism of fibered Omega-algebras}%
\Index%648%И%изотропный вектор
   {изотропный вектор}%
   {isotropic vector}%
\Index%745%И%инволюция в кватернионной алгебре
   {инволюция в кватернионной алгебре}%
   {involution, quaternion algebra}%
\Index%174%И%инфинитезимальные образующие группы Ли
   {инфинитезимальные образующие группы Ли}%
   {infinitesimal generators of group Lie}%
\SetIndexSpace%
\Index%175%К%категория drc векторных пространств
   {категория \drc векторных пространств}%
   {category of drc vector spaces}%
\Index%176%К%категория Tstar- представлений Omega1 алгебры A
   {категория \Ts представлений $\Omega$\Hyph алгебры $A$}%
   {category of Tstar representations of Omega1 algebra}%
\Index%177%К%категория Tstar- представлений Omega1 алгебры из категории A
   {категория \Ts представлений $\Omega_1$\Hyph алгебры из категории $\mathcal A$}%
   {category of Tstar representations of Omega1 algebra from category}%
\Index%178%К%категория приведенных расслоенных соответствий
   {категория приведенных расслоенных соответствий}%
   {category of reduced fibered correspondences}%
\Index%179%К%категория расслоенных соответствий над диагональю
   {категория расслоенных соответствий над диагональю}%
   {category of fibered correspondences over diagonal}%
\Index%555%К%квадратичная форма на теле
   {квадратичная форма на теле}%
   {quadratic form, division ring}%
\Index%551%К%квадратичное отображение тела
   {квадратичное отображение тела}%
   {Quadratic Map of Division Ring}%
\Index%180%К%квазиаффинное преобразование на многообразии базисов
   {квазиаффинное преобразование на многообразии базисов}%
   {quasi affine transformation}%
\Index%181%К%квазиаффинное преобразование на многообразии базисов
   {квазиаффинное преобразование на многообразии базисов}%
   {quasi affine drc transformation}%
\Index%182%К%квазидвижение на многообразии базисов
   {квазидвижение на многообразии базисов}%
   {quasi movement, division ring}%
\Index%183%К%квазидвижение на многообразии базисов
   {квазидвижение на многообразии базисов}%
   {quasi movement}%
\Index%75%К%квазидвижение пространства Минковского
   {квазидвижение пространства Минковского}%
   {Quasimotion, Minkowski space}%
\Index%679%К%квазидетерминант
   {квазидетерминант}%
   {quasideterminant definition}%
\Index%604%К%квазизамкнутое кольцо отображений
   {квазизамкнутое кольцо отображений}%
   {quasiclosed ring of mappings}%
\Index%746%К%кватернион, сопряженный к кватерниону
   {кватернион, сопряженный к кватерниону $x$}%
   {conjugate of quaternion}%
\Index%741%К%кватернионная алгебра
   {кватернионная алгебра}%
   {quaternion algebra}%
\Index%184%К%ковариантное starT- представление группы
   {ковариантное \sT представление группы}%
   {covariant starT representation of group}%
\Index%185%К%ковариантное starT- представление расслоенной группы
   {ковариантное \sT представление расслоенной группы}%
   {covariant starT representation of fibered group}%
\Index%186%К%ковариантное Tstar- представление группы
   {ковариантное \Ts представление группы}%
   {covariant Tstar representation of group}%
\Index%187%К%ковариантное Tstar- представление расслоенной группы
   {ковариантное \Ts представление расслоенной группы}%
   {covariant Tstar representation of fibered group}%
\Index%188%К%кольцо имеет характеристику 0
   {кольцо имеет характеристику $0$}%
   {ring has characteristic 0}%
\Index%189%К%кольцо имеет характеристику p
   {кольцо имеет характеристику $p$}%
   {ring has characteristic p}%
\Index%794%К%кольцо множеств
   {кольцо множеств}%
   {ring of sets}%
\Index%778%К%кольцо с сопряжением
   {кольцо с сопряжением}%
   {ring with conjugation}%
\Index%615%К%коммутативная D алгебра
   {коммутативная $D$\Hyph алгебра}%
   {commutative D algebra}%
\Index%190%К%коммутативная диаграмма соответствий
   {коммутативная диаграмма соответствий}%
   {commutative diagram of correspondences}%
\Index%614%К%коммутатор D алгебры
   {коммутатор $D$\Hyph алгебры}%
   {commutator of algebra}%
\Index%815%К%компактное множество
   {компактное множество}%
   {compact set}%
\Index%191%К%компактно-открытая топология
   {компактно\hyph открытая топология}%
   {compact open topology}%
\Index%193%К%компонента линейного отображения
   {компонента линейного отображения}%
   {component of linear map}%
\Index%647%К%компонента полилинейного отображения
   {компонента полилинейного отображения}%
   {component of polylinear map}%
\Index%629%К%компонента производной Гато
   {компонента производной Гато}%
   {component of Gateaux derivative}%
\Index%633%К%компонента производной Гато второго порядка
   {компонента производной Гато второго порядка}%
   {component of Gateaux derivative of Second Order}%
\Index%202%К%контравариантное starT- представление группы
   {контравариантное \sT представление группы}%
   {contravariant starT representation of group}%
\Index%200%К%контравариантное starT- представление расслоенной группы
   {контравариантное \sT представление расслоенной группы}%
   {contravariant starT representation of fibered group}%
\Index%201%К%контравариантное Tstar- представление группы
   {контравариантное \Ts представление группы}%
   {contravariant Tstar representation of group}%
\Index%203%К%контравариантное Tstar- представление расслоенной группы
   {контравариантное \Ts представление расслоенной группы}%
   {contravariant Tstar representation of fibered group}%
\Index%691%К%координатная матрица вектора
   {координатная матрица вектора}%
   {coordinate matrix of vector}%
\Index%205%К%координатная матрица векторного поля в Drc базисе
   {координатная матрица векторного поля в \Drc базисе}%
   {coordinate matrix of vector field in drc basis}%
\Index%206%К%координатная матрица множества векторов
   {координатная матрица множества векторов}%
   {coordinate matrix of set of vectors}%
\Index%208%К%координатная система отсчёта
   {координатная система отсчёта}%
   {coordinate reference frame}%
\Index%210%К%координатное Drc векторное расслоение
   {координатное \Drc векторное расслоение}%
   {coordinate drc vector bundle}%
\Index%209%К%координатное rcd векторное пространство
   {координатное \rcd векторное пространство}%
   {coordinate rcd vector space}%
\Index%211%К%координатное векторное пространство
   {координатное векторное пространство}%
   {coordinate vector space}%
\Index%697%К%координатное представление в Omega_2- алгебре
   {координатное представление в $\Omega_2$\Hyph алгебре}%
   {coordinate representation, Omega_2 algebra}%
\Index%212%К%координатное представление в rcd векторном пространстве
   {координатное представление в \rcd векторном пространстве}%
   {coordinate representation, rcd vector space}%
\Index%720%К%координатное представление в кортеже Omega- алгебр
   {координатное представление в кортеже $\VX\Omega$\Hyph алгебр}%
   {coordinate tower of representations, Omega algebra}%
\Index%213%К%координатное представление группы в векторном пространстве
   {координатное представление группы в векторном пространстве}%
   {coordinate representation, vector space}%
\Index%214%К%координатный rcd изоморфизм
   {координатный \rcd изоморфизм}%
   {coordinate rcd isomorphism}%
\Index%215%К%координатный изоморфизм
   {координатный изоморфизм}%
   {coordinate isomorphism}%
\Index%325%К%координаты базиса представления
   {координаты базиса представления}%
   {coordinates of basis relative to basis, representation}%
\Index%216%К%координаты вектора
   {координаты вектора}%
   {coordinates of vector}%
\Index%286%К%координаты вектора относительно базиса Гамеля
   {координаты вектора относительно базиса Гамеля}%
   {coordinates of vector, Hamel basis}%
\Index%676%К%координаты вектора относительно базиса Шаудера
   {координаты вектора относительно базиса Шаудера}%
   {coordinates of vector, Schauder basis}%
\Index%217%К%координаты векторного поля в Drc базисе
   {координаты векторного поля в \Drc базисе}%
   {coordinates of vector field in drc basis}%
\Index%218%К%координаты геометрического объекта
   {координаты геометрического объекта}%
   {coordinates of geometric object, vector space}%
\Index%701%К%координаты геометрического объекта в Omega_2- алгбре
   {координаты геометрического объекта в $\Omega_2$\Hyph алгбре $M$}%
   {coordinates of geometric object, representation g}%
\Index%219%К%координаты геометрического объекта в rcd векторном пространстве
   {координаты геометрического объекта в \rcd векторном пространстве}%
   {coordinates of geometric object, rcd vector space}%
\Index%220%К%координаты геометрического объекта в координатном rcd векторном пространстве
   {координаты геометрического объекта в координатном \rcd векторном пространстве}%
   {coordinates of geometric object, coordinate rcd vector space}%
\Index%221%К%координаты геометрического объекта в координатном представлении
   {координаты геометрического объекта в координатном представлении}%
   {coordinates of geometric object, coordinate vector space}%
\Index%721%К%координаты геометрического объекта в координатном пространстве башни представлений
   {координаты геометрического объекта в координатном пространстве башни представлений}%
   {coordinates of geometric object, coordinate tower of representations}%
\Index%699%К%координаты геометрического объекта в координатном пространстве представления
   {координаты геометрического объекта в координатном пространстве представления}%
   {coordinates of geometric object, coordinate representation}%
\Index%723%К%координаты геометрического объекта в кортеже Omega- алгебр
   {координаты геометрического объекта в кортеже $\VX\Omega$\Hyph алгебр}%
   {coordinates of geometric object, tower of representations g}%
\Index%222%К%координаты множества векторов
   {координаты множества векторов}%
   {coordinates of set of vectors}%
\Index%224%К%координаты представления
   {координаты представления}%
   {coordinates of representation, drc vector space}%
\Index%225%К%координаты представления
   {координаты представления}%
   {coordinates of representation}%
\Index%737%К%координаты точки rcd аффинного пространства относительно базиса
   {координаты точки \rcd аффинного пространства относительно базиса}%
   {coordinates in rcd affine space}%
\Index%730%К%координаты точки аффинного пространства относительно базиса
   {координаты точки $A$ аффинного пространства $\overset{\circ}{A}$ относительно базиса $(O,\Basis e)$}%
   {coordinates in affine space}%
\Index%558%К%координаты элемента представления относительно множества
   {координаты элемента $m$ представления $f$ относительно множества $X$}%
   {coordinates of element relative to set, representation}%
\Index%711%К%координаты эндоморфизма башни представлений
   {координаты эндоморфизма башни представлений}%
   {coordinates of endomorphism, tower of representations}%
\Index%696%К%координаты эндоморфизма представления
   {координаты эндоморфизма представления}%
   {coordinates of endomorphism, representation}%
\Index%634%К%корень полинома
   {корень полинома}%
   {root of polynomial}%
\Index%708%К%кортеж Omega слов элементов башни представления относительно кортежа множеств образующих
   {кортеж $\Vector{\Omega}$\Hyph слов элемента башни представления относительно кортежа множеств образующих}%
   {tuple of words relative to tuple of generating sets, tower of representations}%
\Index%535%К%кортеж координат элемента относительно кортежа множеств
   {кортеж координат элемента $\Vector a$ относительно кортежа множеств $\VX X$}%
   {coordinates of element, tower of representations}%
\Index%533%К%кортеж множеств образующих башни подпредставлений
   {кортеж множеств образующих башни подпредставлений}%
   {tuple of generating sets of tower subrepresentations}%
\Index%534%К%кортеж множеств образующих башни представлений
   {кортеж множеств образующих башни представлений}%
   {tuple of generating sets of tower of representations}%
\Index%713%К%кортеж отношений эквивалентности, порождённых башней представлений
   {кортеж отношений эквивалентности, порождённых башней представлений $\Vector f$}%
   {tuple of equivalence of tower of representations}%
\Index%530%К%кортеж стабильных множеств башни представлений
   {кортеж стабильных множеств башни представлений}%
   {tuple of stable sets of tower of representations}%
\Index%226%К%косое произведение векторов
   {косое произведение векторов}%
   {skew product of vectors}%
\Index%550%К%коэффициенты D- аффинной связности на многообразии
   {коэффициенты $D$\Hyph аффинной связности на многообразии}%
   {D affine connection coefficients, manifold}%
\Index%538%К%коэффициенты связности в D аффинном пространстве
   {коэффициенты связности в $D$\Hyph аффинном пространстве}%
   {connection coefficients, D affine space}%
\Index%227%К%кривизна Картана
   {кривизна Картана}%
   {Cartan curvature}%
\Index%537%К%криволинейные координаты точки аффинного пространства
   {криволинейные координаты точки аффинного пространства}%
   {curvilinear coordinates of point in affine space}%
\SetIndexSpace%
\Index%33%Л%Drc линейно независимые векторные поля
   {линейно независимые векторные поля}%
   {linearly independent vector fields}%
\Index%158%Л%левая дробь
   {левая дробь}%
   {left fraction}%
\Index%754%Л%левое алгебраическое дополнение элемента матрицы
   {левое алгебраическое дополнение элемента матрицы}%
   {left cofactor, matrix}%
\Index%228%Л%левое векторное пространство
   {левое векторное пространство}%
   {left vector space}%
\Index%756%Л%левое двойное алгебраическое дополнение элемента матрицы
   {левое двойное алгебраическое дополнение элемента матрицы}%
   {left double cofactor}%
\Index%229%Л%левоинвариантное векторное поле
   {левоинвариантное векторное поле}%
   {left invariant vector}%
\Index%230%Л%левостороннее ковариантное представление группы
   {левостороннее ковариантное представление группы}%
   {left-side covariant representation of group}%
\Index%231%Л%левостороннее контравариантное представление группы
   {левостороннее контравариантное представление группы}%
   {left-side contravariant representation of group}%
\Index%232%Л%левостороннее представление Omega1 алгебры A в Omega2 алгебре M
   {левостороннее представление $\Omega_1$\Hyph алгебры $A$ в $\Omega_2$\Hyph алгебре $M$}%
   {left-side representation of algebra}%
\Index%233%Л%левостороннее представление расслоенной Omega- алгебры
   {левостороннее представление расслоенной $\Omega$\Hyph алгебры}%
   {left-side representation of fibered Omega-algebra}%
\Index%234%Л%левостороннее преобразование
   {левостороннее преобразование}%
   {left-side transformation}%
\Index%235%Л%левостороннее преобразование расслоения
   {левостороннее преобразование расслоения}%
   {left-side transformation of bundle}%
\Index%236%Л%левые структурные константы алгебры Ли
   {левые структурные константы алгебры Ли}%
   {left structural constant of Lie algebra}%
\Index%513%Л%левый главный идеал
   {левый главный идеал}%
   {left principal ideal}%
\Index%812%Л%левый делитель нуля
   {левый делитель нуля}%
   {left zero divisor}%
\Index%681%Л%левый идеал алгебры
   {левый идеал алгебры}%
   {left ideal of algebra}%
\Index%237%Л%левый модуль нaд кольцом
   {левый модуль нaд кольцом $D$}%
   {left module over ring}%
\Index%661%Л%левый модуль над D- алгеброй A
   {левый модуль над $D$\Hyph алгеброй $A$}%
   {left module over algebra}%
\Index%731%Л%левый сдвиг R- модуля
   {левый сдвиг $R$\Hyph модуля}%
   {left shift of module}%
\Index%238%Л%левый сдвиг на группе
   {левый сдвиг на группе}%
   {left shift}%
\Index%239%Л%левый сдвиг на группе
   {левый сдвиг на группе}%
   {left shift, group}%
\Index%240%Л%левый сдвиг на расслоении групп
   {левый сдвиг на расслоении групп}%
   {Tstar shift, fibered group}%
\Index%88%Л%линейная комбинация векторов
   {линейная комбинация векторов}%
   {linear combination of  vectors}%
\Index%686%Л%линейная комбинация векторов A- модуля
   {линейная комбинация векторов $A$\Hyph модуля}%
   {linear combination in A module}%
\Index%98%Л%линейнное отображение, порождённое отображением
   {линейное отображение, порождённое отображением}%
   {linear map generated by map}%
\Index%688%Л%линейно зависимое множество A- модуля
   {линейно зависимое множество $A$\Hyph модуля}%
   {linear dependent vectors, module}%
\Index%20%Л%линейно зависимые векторные поля
   {линейно зависимые векторные поля}%
   {linearly dependent vector fields}%
\Index%21%Л%линейно зависимые векторы
   {линейно зависимые векторы}%
   {linearly dependent vectors}%
\Index%687%Л%линейно независимое множество A- модуля
   {линейно независимое множество $A$\Hyph модуля}%
   {linear independent vectors, module}%
\Index%34%Л%линейно независимые векторы
   {линейно независимые векторы}%
   {linearly independent vectors}%
\Index%613%Л%линейное отображение
   {линейное отображение}%
   {linear map}%
\Index%398%Л%линейное отображение D векторных пространств
   {линейное отображение $D$\Hyph векторных пространств}%
   {linear map of D vector spaces}%
\Index%35%Л%линейное отображение rcd векторных пространств
   {линейное отображение \rcd векторных пространств}%
   {linear map of rcd vector spaces}%
\Index%97%Л%линейное отображение тела
   {линейное отображение тела}%
   {linear map of division ring}%
\Index%244%Л%линейное представление группы
   {линейное представление группы}%
   {linear representation of group}%
\Index%682%Л%линейное представление группы Ли
   {линейное представление группы Ли}%
   {Linear Representation of Lie Group}%
\Index%740%Л%линейное преобразование rcd аффинного пространства
   {линейное преобразование \rcd аффинного пространства}%
   {linear transformation, rcd affine space}%
\Index%630%Л%линейный геометрический объект
   {линейный геометрический объект}%
   {linear geometric object}%
\Index%397%Л%линейный функционал на D модуле
   {линейный функционал на $D$\Hyph модуле}%
   {linear functional, D module}%
\Index%245%Л%лифт отображения
   {лифт отображения}%
   {lift of map}%
\Index%246%Л%лифт соответствия
   {лифт соответствия}%
   {lift of correspondence}%
\Index%247%Л%локальная система отсчёта
   {локальная система отсчёта}%
   {local reference frame}%
\Index%248%Л%локально компактное в точке p пространство
   {локально компактное в точке $p$ пространство}%
   {locally compact at point space}%
\Index%249%Л%локально компактное пространство
   {локально компактное пространство}%
   {locally compact space}%
\SetIndexSpace%
\Index%250%М%малая группа
   {малая группа}%
   {little group}%
\Index%772%М%матрица антилинейного гомоморфизма
   {матрица антилинейного гомоморфизма}%
   {matrix of antilinear homomorphism}%
\Index%252%М%матрица билинейной функции
   {матрица билинейной функции}%
   {matrix of bilinear function}%
\Index%552%М%матрица квадратичного отображения
   {матрица квадратичного отображения}%
   {matrix of quadratic map, division ring}%
\Index%770%М%матрица линейного гомоморфизма
   {матрица линейного гомоморфизма}%
   {matrix of linear homomorphism}%
\Index%194%М%матрица линейного отображения
   {матрица линейного отображения}%
   {matrix of linear map}%
\Index%591%М%матрица линейных отображений
   {матрица линейных отображений}%
   {matrix of linear mappings}%
\Index%588%М%матрица отображений
   {матрица отображений}%
   {matrix of mappings}%
\Index%253%М%матрица расслоенного Drc линейного отображения
   {матрица расслоенного \Drc линейного отображения}%
   {matrix of fibered drc linear map}%
\Index%595%М%матрица эндоморфизмов Omega алгебры
   {матрица эндоморфизмов $\Omega$\Hyph алгебры}%
   {matrix of endomorphisms of Omega algebra}%
\Index%527%М%матрица Якоби Гато отображения
   {матрица Якоби\Hyph Гато отображения}%
   {Jacobi Gateaux matrix of map}%
\Index%254%М%метрико-аффинное многообразие
   {метрико-аффинное многообразие}%
   {metric-affine manifold}%
\Index%96%М%метрический тензор в пространстве Минковского
   {метрический тензор в пространстве Минковского}%
   {metric tensor, Minkowski space}%
\Index%642%М%минорная матрица
   {минорная матрица}%
   {minor matrix}%
\Index%556%М%многообразие D- аффинной связности
   {многообразие $D$\Hyph аффинной связности}%
   {manifold with D- affine connections}%
\Index%257%М%многообразие базисов \rcd аффинного пространства
   {многообразие базисов \rcd аффинного пространства}%
   {Basis Manifold, rcd Affine Space, division ring}%
\Index%255%М%многообразие базисов rcd векторного пространства
   {многообразие базисов \rcd векторного пространства}%
   {basis manifold of rcd vector space}%
\Index%256%М%многообразие базисов аффинного пространства
   {многообразие базисов аффинного пространства}%
   {Basis Manifold, Affine Space}%
\Index%714%М%многообразие базисов башни представлений
   {многообразие базисов башни представлений}%
   {basis manifold tower of representations}%
\Index%258%М%многообразие базисов векторного пространства
   {многообразие базисов векторного пространства}%
   {basis manifold of vector space}%
\Index%259%М%многообразие базисов евклидова пространства
   {многообразие базисов евклидова пространства}%
   {Basis Manifold, Euclid Space}%
\Index%260%М%многообразие базисов евклидова пространства
   {многообразие базисов евклидова пространства}%
   {Basis Manifold, Euclid Space, division ring}%
\Index%536%М%многообразие базисов представления
   {многообразие базисов представления}%
   {basis manifold representation F algebra}%
\Index%261%М%многообразие базисов центро-аффинного пространства
   {многообразие базисов центро-аффинного пространства}%
   {Basis Manifold, Central Affine Space, division ring}%
\Index%262%М%многообразие базисов центро-аффинного пространства
   {многообразие базисов центро-аффинного пространства}%
   {Basis Manifold, Central Affine Space}%
\Index%263%М%многообразие систем отсчёта
   {многообразие систем отсчёта}%
   {reference frame manifold}%
\Index%804%М%многочлен
   {многочлен}%
   {polynomial}%
\Index%571%М%множество Omega_2- слов представления
   {множество $\Omega_2$\Hyph слов представления}%
   {word set of representation}%
\Index%562%М%множество координат представления
   {множество координат представления}%
   {coordinate set of representation}%
\Index%709%М%множество кортежей Omega- слов башни представлений
   {множество кортежей $\Vector\Omega$\Hyph слов башни представлений}%
   {word set of tower of representations}%
\Index%563%М%множество кортежей координат башни представлений
   {множество кортежей координат башни представлений}%
   {coordinate set of tower of representations}%
\Index%626%М%множество нулей алгебры
   {множество нулей алгебры}%
   {set of zeros of algebra}%
\Index%331%М%множество образующих подпредставления
   {множество образующих подпредставления}%
   {generating set of subrepresentation}%
\Index%332%М%множество образующих представления
   {множество образующих представления}%
   {generating set of representation}%
\Index%628%М%множество обратимых элементов алгебры
   {множество обратимых элементов алгебры}%
   {set of invertible elements of algebra}%
\Index%787%М%модуль векторов алгебры
   {модуль векторов алгебры}%
   {vector module of algebra}%
\Index%776%М%модуль векторов кольца
   {модуль векторов кольца}%
   {vector module of ring}%
\Index%611%М%модуль над кольцом
   {модуль над кольцом}%
   {module over ring}%
\Index%264%М%морфизм Tstar- представлений расслоенной Omega- алгебры
   {морфизм \Ts представлений расслоенной $\Omega$\Hyph алгебры}%
   {morphism of representations of fibered Omega algebra}%
\Index%265%М%морфизм из башни Tstar- представлений в башню Tstar- представлений
   {морфизм из башни \Ts представлений в башню \Ts представлений}%
   {morphism from tower of representations into tower of representations}%
\Index%267%М%морфизм представлений Omega1 алгебры в Omega2 алгебре
   {морфизм представлений $\Omega_1$\Hyph алгебры в $\Omega_2$\Hyph алгебре}%
   {morphism of representations of Omega1 algebra in Omega2 algebra}%
\Index%268%М%морфизм представлений из f в g
   {морфизм представлений из $f$ в $g$}%
   {morphism of representations from f into g}%
\Index%732%М%морфизм представления f
   {морфизм представления $f$}%
   {morphism of representation f}%
\Index%269%М%морфизм расслоенных Tstar- представлений из F в G
   {морфизм расслоенных \Ts представлений из $\Bundle F$ в $\Bundle G$}%
   {morphism of fibered representations from f into g}%
\SetIndexSpace%
\Index%763%Н%направление над коммутативным кольцом
   {направление над коммутативным кольцом}%
   {direction over commutative ring}%
\Index%738%Н%начало системы координат star D аффинного пространства
   {начало системы координат $\star D$\Hyph аффинного пространства}%
   {origin of coordinate system of starD affine space}%
\Index%729%Н%начало системы координат аффинного пространства
   {начало системы координат аффинного пространства}%
   {origin of coordinate system of affine space}%
\Index%649%Н%не полная Omega алгебра
   {не полная $\Omega$\Hyph алгебра}%
   {not complete Omega algebra}%
\Index%632%Н%не полная группа
   {не полная группа}%
   {not complete group}%
\Index%272%Н%невырожденная билинейная функция
   {невырожденная билинейная функция}%
   {nonsingular bilinear function}%
\Index%273%Н%невырожденная система drc линейных уравнений
   {невырожденная система \rcd линейных уравнений}%
   {nonsingular system of linear equations}%
\Index%553%Н%невырожденное квадратичное отображение тела
   {невырожденное квадратичное отображение тела}%
   {regular quadratic map, division ring}%
\Index%274%Н%невырожденное преобразование
   {невырожденное преобразование}%
   {nonsingular transformation}%
\Index%643%Н%невырожденный тензор
   {невырожденный тензор}%
   {nonsingular tensor}%
\Index%330%Н%невырожденный эндоморфизм представления
   {невырожденный эндоморфизм представления}%
   {regular endomorphism of representation}%
\Index%275%Н%неголономная координата
   {неголономная координата}%
   {anholonomic coordinate}%
\Index%276%Н%неголономные координаты вектора
   {неголономные координаты вектора}%
   {vector anholonomic coordinates}%
\Index%277%Н%неголономные координаты на многообразии
   {неголономные координаты на многообразии}%
   {anholonomic coordinates on manifold}%
\Index%278%Н%неголономные координаты связности
   {неголономные координаты связности}%
   {anholonomic coordinates of connection}%
\Index%279%Н%неметричность
   {неметричность}%
   {nonmetricity}%
\Index%280%Н%непрерывное отображение
   {непрерывное отображение}%
   {continuous map}%
\Index%610%Н%непрерывное отображение нескольких переменных
   {непрерывное отображение нескольких переменных}%
   {continuous multivariable map}%
\Index%281%Н%непрерывное соответствие
   {непрерывное соответствие}%
   {continuous correspondence}%
\Index%668%Н%непрерывный базис
   {непрерывный базис}%
   {continues basis}%
\Index%346%Н%норма в D- алгебре
   {норма в $D$\Hyph алгебре}%
   {norm on D algebra}%
\Index%460%Н%норма в D-модуле
   {норма в $D$\Hyph модуле}%
   {norm on D module}%
\Index%742%Н%норма в кватернионной алгебре
   {норма в кватернионной алгебре}%
   {norm, quaternion algebra}%
\Index%282%Н%норма кватерниона
   {норма кватерниона}%
   {norm of quaternion}%
\Index%283%Н%норма на D- векторном пространстве
   {норма на $D$\Hyph векторном пространстве}%
   {norm on D vector space}%
\Index%675%Н%норма на Omega группе
   {норма на $\Omega$\Hyph группе}%
   {norm on Omega group}%
\Index%641%Н%норма на кольце
   {норма на кольце}%
   {norm on ring}%
\Index%284%Н%норма на теле
   {норма на теле}%
   {absolute value on division ring}%
\Index%657%Н%норма операции
   {норма операции}%
   {norm of operation}%
\Index%314%Н%норма отображения
   {норма отображения}%
   {norm of map}%
\Index%285%Н%норма полилинейного отображения
   {норма полилинейного отображения}%
   {norm of polymap}%
\Index%801%Н%норма представления
   {норма представления}%
   {norm of representation}%
\Index%196%Н%норма функционала
   {норма функционала}%
   {norm of functional}%
\Index%343%Н%нормированная D-алгебра
   {нормированная $D$\Hyph алгебра}%
   {normed D algebra}%
\Index%792%Н%нормированная Omega группа
   {нормированная $\Omega$\Hyph группа}%
   {normed Omega group}%
\Index%287%Н%нормированное D-векторное пространство
   {нормированное $D$\Hyph векторное пространство}%
   {normed D vector space}%
\Index%640%Н%нормированное кольцо
   {нормированное кольцо}%
   {normed ring}%
\Index%288%Н%нормированное тело
   {нормированное тело}%
   {valued division ring}%
\Index%364%Н%нормированный D-модуль
   {нормированный $D$\Hyph модуль}%
   {normed D module}%
\Index%692%Н%нормированный базис
   {нормированный базис}%
   {normal basis}%
\SetIndexSpace%
\Index%289%О%образующая линейного отображения
   {образующая линейного отображения}%
   {generator of linear map}%
\Index%290%О%обратное приведенное расслоенное соответствие
   {обратное приведенное расслоенное соответствие}%
   {inverse reduced fibered correspondence}%
\Index%291%О%обратное расслоенное соответствие
   {обратное расслоенное соответствие}%
   {inverse fibered correspondence}%
\Index%292%О%обращение Адамара матрицы
   {обращение Адамара матрицы}%
   {Hadamard inverse of matrix}%
\Index%293%О%объект неголономности
   {объект неголономности}%
   {anholonomity object}%
\Index%608%О%однородное линейное представление группы Ли
   {однородное линейное представление группы Ли}%
   {homogeneous Linear Representation of Lie Group}%
\Index%294%О%однородное отображение степени k над полем F
   {однородное отображение степени $k$ над полем $F$}%
   {homogeneous map of degree over field, D vector space}%
\Index%295%О%однородное пространство группы
   {однородное пространство группы}%
   {homogeneous space of group}%
\Index%296%О%однородное расслоение расслоенной группы
   {однородное расслоение расслоенной группы}%
   {homogeneous bundle of fibered group}%
\Index%631%О%однородный линейный геометрический объект
   {однородный линейный геометрический объект}%
   {homogeneous linear geometric object}%
\Index%689%О%однородный многочлен степени
   {однородный многочлен степени $n$}%
   {homogeneous polynomial of power}%
\Index%297%О%однотранзитивное представление Omega- алгебры A
   {однотранзитивное представление $\Omega$\Hyph алгебры $A$}%
   {single transitive representation of algebra}%
\Index%298%О%однотранзитивное представление группы
   {однотранзитивное представление группы}%
   {single transitive representation of group}%
\Index%299%О%однотранзитивное представление расслоенной Omega- алгебры
   {однотранзитивное представление расслоенной $\Omega$\Hyph алгебры}%
   {single transitive representation of fibered Omega-algebra}%
\Index%766%О%одночлен степени
   {одночлен степени $k$}%
   {monomial of power}%
\Index%300%О%операция на расслоении
   {операция на расслоении}%
   {operation on bundle}%
\Index%301%О%определённая слева алгебра Ли группы Ли
   {определённая слева алгебра Ли группы Ли}%
   {left defined Lie algebra}%
\Index%302%О%определённая справа алгебра Ли группы Ли
   {определённая справа алгебра Ли группы Ли}%
   {right defined Lie algebra}%
\Index%303%О%определитель матрицы
   {определитель матрицы}%
   {determinant}%
\Index%304%О%орбита Tstar- представления группы
   {орбита \Ts представления группы}%
   {orbit of Tstar  representation of group}%
\Index%624%О%орбита линейного отображения
   {орбита линейного отображения}%
   {orbit of linear mapping}%
\Index%305%О%орбита представления группы
   {орбита представления группы}%
   {orbit of representation of group}%
\Index%306%О%орбита представления расслоенной группы
   {орбита представления расслоенной группы}%
   {orbit of representation of fibered group}%
\Index%636%О%ортогональность в пространстве Минковского
   {ортогональность в пространстве Минковского}%
   {Minkowski orthogonality}%
\Index%637%О%ортогональный базис в пространстве Минковского
   {ортогональный базис в пространстве Минковского}%
   {orthogonal basis, Minkowski space}%
\Index%307%О%ортонормированный базис
   {ортонормированный базис}%
   {Orthonornal Basis}%
\Index%308%О%ортонормированный базис
   {ортонормированный базис}%
   {Orthonornal Basis, division ring}%
\Index%638%О%ортонормированный базис в пространстве Минковского
   {ортонормированный базис в пространстве Минковского}%
   {orthonormal basis, Minkowski space}%
\Index%309%О%отклонение траекторий
   {отклонение траекторий}%
   {deviation of trajectories}%
\Index%793%О%открытый шар
   {открытый шар}%
   {open ball}%
\Index%706%О%отношение эквивалентности порождённое представлением
   {отношение эквивалентности, порождённое представлением $f$}%
   {equivalence of representation}%
\Index%502%О%отображение n D- значных переменных
   {отображение $\gi n$ $D$\Hyph значных переменных}%
   {map of n D valued variables}%
\Index%312%О%отображение колец полилинейное над коммутативным кольцом
   {отображение колец полилинейное над коммутативным кольцом}%
   {map polylinear over commutative ring, ring}%
\Index%316%О%отображение типа G на многообразии
   {отображение типа $G$ на многообразии}%
   {map of type G on manifold}%
\Index%505%О%отображение, дифференцируемое по Гато
   {отображение, дифференцируемое по Гато}%
   {map differentiable in Gateaux sense}%
\Index%506%О%отображение, непрерывное по совокупности аргументов
   {отображение, непрерывное по совокупности аргументов}%
   {map continuous with respect to set of arguments}%
\Index%572%О%отображение, полилинейное над конечномерными алгебрами
   {отображение, полилинейное над конечномерными алгебрами}%
   {map polylinear over finite dimensional algebras}%
\Index%677%О%отображение, проективное над коммутативным кольцом
   {отображение, проективное над коммутативным кольцом}%
   {map projective over commutative ring}%
\SetIndexSpace%
\Index%317%П%параллелограмм
   {параллелограмм}%
   {parallelogram}%
\Index%739%П%параллельный сдвиг rcd аффинного пространства
   {параллельный сдвиг \rcd аффинного пространства}%
   {parallel shift, rcd affine space}%
\Index%684%П%парные представления D- алгебры
   {парные представления $D$\Hyph алгебры}%
   {twin representations of D algebra}%
\Index%587%П%парные представления ассоциативной алгебры
   {парные представления ассоциативной алгебры}%
   {twin representations of associative algebra}%
\Index%318%П%парные представления группы
   {парные представления группы}%
   {twin representations of group}%
\Index%319%П%парные представления расслоенной группы
   {парные представления расслоенной группы}%
   {twin representations of fibered group}%
\Index%320%П%парные представления тела
   {парные представления тела}%
   {twin representations of division ring}%
\Index%321%П%пассивное starT- представление
   {пассивное \sT представление}%
   {passive starT representation}%
\Index%333%П%пассивное представление
   {пассивное представление}%
   {passive representation}%
\Index%718%П%пассивное представление группы в многообразии базисов башни представлений
   {пассивное представление группы $G(\Vector f)$ в многообразии базисов башни представлений}%
   {passive representation in basis manifold, tower of representations}%
\Index%695%П%пассивное представление группы в многообразии базисов представления
   {пассивное представление группы $G(f)$ в многообразии базисов представления}%
   {passive representation in basis manifold}%
\Index%717%П%пассивное преобразование многообразия базисов башни представлений
   {пассивное преобразование многообразия базисов башни представлений}%
   {passive transformation of basis, tower of representations}%
\Index%570%П%пассивное преобразование многообразия базисов представления
   {пассивное преобразование многообразия базисов представления}%
   {passive transformation of basis, representation}%
\Index%335%П%пассивное преобразование на многообразии базисов
   {пассивное преобразование на многообразии базисов}%
   {passive transformation}%
\Index%336%П%пассивное преобразование на множестве rcd базисов
   {пассивное преобразование на множестве \rcd базисов}%
   {passive transformation, vector space}%
\Index%337%П%первый закон Ньютона
   {первый закон Ньютона}%
   {First Newton law}%
\Index%338%П%перенос Картана
   {перенос Картана}%
   {Cartan transport}%
\Index%339%П%перенос Френе
   {перенос Френе}%
   {Frenet transport}%
\Index%334%П%подпредставление представления
   {подпредставление представления}%
   {subrepresentation of representation}%
\Index%322%П%подпредставление, порождённое множеством X
   {подпредставление, порождённое множеством $X$}%
   {subrepresentation generated by set}%
\Index%340%П%подрасслоение
   {подрасслоение}%
   {subbundle}%
\Index%341%П%подрасслоение Dstar-векторного расслоения
   {подрасслоение $\mathcal D\star$\hyph векторного расслоения}%
   {subbundle of Dstar vector bundle}%
\Index%806%П%полиаддитивное отображение
   {полиаддитивное отображение}%
   {polyadditive map}%
\Index%345%П%полиалинейное косо симметричное отображение
   {полиалинейное косо симметричное отображение}%
   {polylinear map skew symmetric}%
\Index%344%П%поливектор
   {поливектор}%
   {polyvector}%
\Index%609%П%полилинейное отображение
   {полилинейное отображение}%
   {polylinear map}%
\Index%347%П%полилинейное симметричное отображение
   {полилинейное симметричное отображение}%
   {polylinear map symmetric}%
\Index%760%П%полиморфизм представлений
   {полиморфизм представлений}%
   {polymorphism of representations}%
\Index%811%П%полная нормированная Omega группа
   {полная нормированная $\Omega$\Hyph группа}%
   {complete Omega group}%
\Index%348%П%полная система линейных дифференциальных уравнений в частных производны
   {полная система линейных дифференциальных уравнений в частных производны}%
   {Complete System of Linear Partial Differential Equations}%
\Index%270%П%полное кольцо
   {полное кольцо}%
   {complete ring}%
\Index%349%П%полное тело
   {полное тело}%
   {complete division ring}%
\Index%241%П%последовательность Коши
   {последовательность Коши}%
   {Cauchy sequence}%
\Index%816%П%последовательность сходится
   {последовательность сходится}%
   {sequence converges}%
\Index%817%П%последовательность сходится равномерно
   {последовательность сходится равномерно}%
   {sequence converges uniformly}%
\Index%352%П%потенциальная энергия
   {потенциальная энергия}%
   {potential energy}%
\Index%30%П%правая дробь
   {правая дробь}%
   {right fraction}%
\Index%753%П%правое алгебраическое дополнение элемента матрицы
   {правое алгебраическое дополнение элемента матрицы}%
   {right cofactor, matrix}%
\Index%353%П%правое векторное пространство
   {правое векторное пространство}%
   {right vector space}%
\Index%757%П%правое двойное алгебраическое дополнение элемента матрицы
   {правое двойное алгебраическое дополнение элемента матрицы}%
   {right double cofactor}%
\Index%354%П%правоинвариантное векторное поле
   {правоинвариантное векторное поле}%
   {right invariant vector}%
\Index%355%П%правостороннее ковариантное представление группы
   {правостороннее ковариантное представление группы}%
   {right-side covariant representation of group}%
\Index%356%П%правостороннее контравариантное представление группы
   {правостороннее контравариантное представление группы}%
   {right-side contravariant representation of group}%
\Index%357%П%правостороннее представление Omega1 алгебры A в Omega2 алгебре M
   {правостороннее представление $\Omega_1$\Hyph алгебры $A$ в $\Omega_2$\Hyph алгебре $M$}%
   {right-side representation of algebra}%
\Index%358%П%правостороннее представление расслоенной Omega- алгебры
   {правостороннее представление расслоенной $\Omega$\Hyph алгебры}%
   {right-side representation of fibered Omega-algebra}%
\Index%359%П%правостороннее преобразование
   {правостороннее преобразование}%
   {right-side transformation}%
\Index%360%П%правые структурные константы алгебры Ли
   {правые структурные константы алгебры Ли}%
   {right structural constant of Lie algebra}%
\Index%242%П%правый главный идеал
   {правый главный идеал}%
   {right principal ideal}%
\Index%813%П%правый делитель нуля
   {правый делитель нуля}%
   {right zero divisor}%
\Index%42%П%правый идеал алгебры
   {правый идеал алгебры}%
   {right ideal of algebra}%
\Index%361%П%правый модуль нaд кольцом
   {правый модуль нaд кольцом $D$}%
   {right module over ring}%
\Index%362%П%правый сдвиг на группе
   {правый сдвиг на группе}%
   {right shift}%
\Index%363%П%правый сдвиг на группе
   {правый сдвиг на группе}%
   {right shift, group}%
\Index%670%П%праый модуль над D- алгеброй A
   {правый модуль над $D$\Hyph алгеброй $A$}%
   {right module over algebra}%
\Index%467%П%предел последовательности
   {предел последовательности}%
   {limit of sequence}%
\Index%365%П%предел соответствия по фильтру
   {предел соответствия по фильтру}%
   {limit of correspondence with respect to the filter}%
\Index%366%П%предел фильтра
   {предел фильтра}%
   {limit of filter}%
\Index%367%П%предельное множество фильтра
   {предельное множество фильтра}%
   {limit set of filter}%
\Index%702%П%представитель геометрического объекта в drc векторном пространстве
   {представитель геометрического объекта в \drc векторном пространстве}%
   {representative of geometric object, drc vector space}%
\Index%703%П%представитель геометрического объекта в Omega_2- алгбре
   {представитель геометрического объекта в $\Omega_2$\Hyph алгбре}%
   {representative of geometric object, representation g}%
\Index%368%П%представитель геометрического объекта в rcd векторном пространстве
   {представитель геометрического объекта в \rcd векторном пространстве}%
   {representative of geometric object, rcd vector space}%
\Index%369%П%представитель геометрического объекта в векторном пространстве
   {представитель геометрического объекта в векторном пространстве}%
   {representative of geometric object, vector space}%
\Index%724%П%представитель геометрического объекта в кортеже Omega- алгебр
   {представитель геометрического объекта в кортеже $\VX\Omega$\Hyph алгебр}%
   {representative of geometric object, tower of representations g}%
\Index%370%П%представление Omega- алгебры A в категории B
   {представление $\Omega$\Hyph алгебры $A$ в категории $\mathcal B$}%
   {representation of Omega algebra in category}%
\Index%529%П%представление Omega алгебры в башне представлений
   {представление $\Omega$\Hyph алгебры в башне представлений}%
   {representation of Omega algebra in tower of representations}%
\Index%528%П%представление Omega алгебры в представлении
   {представление $\Omega$\Hyph алгебры в представлении}%
   {representation of Omega algebra in representation}%
\Index%371%П%представление Omega1 алгебры A в Omega2 алгебре M
   {представление $\Omega_1$\Hyph алгебры $A$ в $\Omega_2$\Hyph алгебре $M$}%
   {representation of algebra}%
\Index%372%П%представление группы
   {представление группы}%
   {representation of group}%
\Index%373%П%преобразование Лоренца
   {преобразование Лоренца}%
   {Lorentz transformation}%
\Index%375%П%преобразование расслоения
   {преобразование расслоения}%
   {transformation of bundle}%
\Index%374%П%преобразование универсальной алгебры
   {преобразование универсальной алгебры}%
   {transformation of universal algebra}%
\Index%376%П%преобразование, согласованное с эквивалентностью 
   {преобразование, согласованное с эквивалентностью }%
   {transformation coordinated with equivalence}%
\Index%377%П%приведенное декартово произведение расслоений
   {приведенное декартово произведение расслоений}%
   {reduced Cartesian product of bundles}%
\Index%378%П%приведенное декартово произведение расслоенных пространств
   {приведенное декартово произведение расслоенных пространств}%
   {reduced Cartesian product of total spaces}%
\Index%380%П%приведенное расслоенное соответствие в A
   {приведенное расслоенное соответствие в $\Bundle{A}$}%
   {reduced fibered correspondence in A}%
\Index%379%П%приведенное расслоенное соответствие из A в B
   {приведенное расслоенное соответствие из $\mathcal{A}$ в $\Bundle{B}$}%
   {reduced fibered correspondence from A to B}%
\Index%761%П%приведенный полиморфизм представлений
   {приведенный полиморфизм представлений}%
   {reduced polymorphism of representations}%
\Index%381%П%приводимое бикольцо
   {приводимое бикольцо}%
   {reducible biring}%
\Index%382%П%принцип двойственности для бикольца
   {принцип двойственности для бикольца}%
   {duality principle for biring}%
\Index%383%П%принцип двойственности для бикольца матриц
   {принцип двойственности для бикольца матриц}%
   {duality principle for biring of matrices}%
\Index%705%П%принцип инвариантности в \drc векторном пространстве
   {принцип инвариантности в \drc векторном пространстве}%
   {invariance principle}%
\Index%710%П%принцип инвариантности в башне представлений универсальных алгебр
   {принцип инвариантности в башне представлений универсальных алгебр}%
   {invariance principle, tower of representations g}%
\Index%385%П%принцип инвариантности в векторном пространстве
   {принцип инвариантности в векторном пространстве}%
   {invariance principle, vector space}%
\Index%384%П%принцип инвариантности в представлении универсальной алгебры
   {принцип инвариантности в представлении универсальной алгебры}%
   {invariance principle, representation g}%
\Index%386%П%продолжение соответствия
   {продолжение соответствия}%
   {extension of correspondence}%
\Index%195%П%проективное отображение непрерывно по направлению над полем
   {проективное отображение непрерывно по направлению над полем}%
   {projective map is continuous in direction over field}%
\Index%387%П%проекция расслоения E вдоль слоя E
   {проекция расслоения $\Bundle E$ вдоль слоя $E$}%
   {projection of bundle along fiber}%
\Index%388%П%произведение геометрического объекта и константы
   {произведение геометрического объекта и константы}%
   {product of geometric object and constant}%
\Index%389%П%произведение геометрического объекта и константы в векторном пространстве
   {произведение геометрического объекта и константы в векторном пространстве}%
   {product of geometric object and constant, vector space}%
\Index%390%П%произведение групп
   {произведение групп}%
   {product of groups}%
\Index%683%П%произведение линейного отображения на скаляр
   {произведение линейного отображения на скаляр}%
   {product of linear map over scalar}%
\Index%666%П%произведение многочленов
   {произведение многочленов}%
   {product of polynomials}%
\Index%392%П%произведение морфизмов Tstar- представлений расслоенной Omega- алгебры
   {произведение морфизмов \Ts представлений расслоенной $\Omega$\Hyph алгебры}%
   {product of morphisms of representations of fibered Omega algebra}%
\Index%561%П%произведение морфизмов башни представлений
   {произведение морфизмов башни представлений}%
   {product of morphisms of tower of representations}%
\Index%391%П%произведение морфизмов представлений универсальной алгебры
   {произведение морфизмов представлений универсальной алгебры}%
   {product of morphisms of representations of universal algebra}%
\Index%271%П%произведение отображения на скаляр
   {произведение отображения на скаляр}%
   {product of map over scalar}%
\Index%393%П%произведение приведенных расслоенных соответствий
   {произведение приведенных расслоенных соответствий}%
   {composition of reduced fibered correspondences}%
\Index%394%П%произведение расслоенных соответствий
   {произведение расслоенных соответствий}%
   {composition of fibered correspondences}%
\Index%395%П%произведением объектов в категории
   {произведением объектов в категории}%
   {product of objects in category}%
\Index%396%П%производная Гато второго порядка
   {производная Гато второго порядка}%
   {Gateaux derivative of Second Order}%
\Index%627%П%производная Гато отображения
   {производная Гато отображения}%
   {Gateaux derivative of map}%
\Index%399%П%производная Гато порядка n
   {производная Гато порядка $n$}%
   {Gateaux derivative of Order n}%
\Index%401%П%производная Картана
   {производная Картана}%
   {Cartan derivative}%
\Index%402%П%производная Ли
   {производная Ли}%
   {Lie derivative}%
\Index%403%П%производная Ли метрики
   {производная Ли метрики}%
   {Lie derivative of metric}%
\Index%404%П%производная Ли связности
   {производная Ли связности}%
   {Lie derivative of connection}%
\Index%810%П%простое отображение
   {простое отображение}%
   {simple map}%
\Index%405%П%простой поливектор
   {простой поливектор}%
   {simple polyvector}%
\Index%342%П%пространственноподобный вектор
   {пространственноподобный вектор}%
   {spacelike vector}%
\Index%635%П%пространство Минковского
   {пространство Минковского}%
   {Minkowski space, Finsler}%
\Index%406%П%пространство орбит Tstar- представления
   {пространство орбит \Ts представления}%
   {space of orbits of Ts representation}%
\Index%407%П%пространство отображений
   {пространство отображений}%
   {mapping space}%
\Index%408%П%противоположная расслоенная предупорядоченность
   {противоположная расслоенная предупорядоченность}%
   {opposite fibered preordering}%
\Index%409%П%прямая сумма представлений
   {прямая сумма представлений}%
   {direct sum of representations}%
\Index%410%П%прямое произведение D- векторных пространств
   {прямое произведение $D$\Hyph векторных пространств}%
   {direct product of D vector spaces}%
\Index%411%П%прямое произведение rcd векторных пространств
   {прямое произведение \rcd векторных пространств}%
   {direct product, rcd vector space}%
\Index%412%П%прямое произведение Tstar- представлений группы
   {прямое произведение \Ts представлений группы}%
   {direct product of Tstar representations of group}%
\Index%413%П%прямое произведение представлений группы
   {прямое произведение представлений группы}%
   {direct product of representations of group}%
\Index%414%П%прямое произведение представлений расслоенной группы
   {прямое произведение представлений расслоенной группы}%
   {direct product of representations of fibered group}%
\Index%415%П%прямое произведение тел
   {прямое произведение тел}%
   {direct product of division rings}%
\Index%540%П%псевдоэвклидова метрика на теле
   {псевдоэвклидова метрика на теле}%
   {pseudo-Euclidean metric on division ring}%
\Index%548%П%псевдоэвклидово скалярное произведение в D- векторном пространстве
   {псевдоэвклидово скалярное произведение в $D$\Hyph векторном пространстве}%
   {pseudo-Euclidean scalar product, vector space}%
\Index%543%П%псевдоэвклидово скалярное произведение на теле
   {псевдоэвклидово скалярное произведение на теле}%
   {pseudo-Euclidean scalar product on division ring}%
\Index%416%П%пфаффова производная
   {пфаффова производная}%
   {pfaffian derivative}%
\SetIndexSpace%
\Index%204%Р%разложение вектора относительно базиса сходится
   {разложение вектора относительно базиса сходится}%
   {expansion converges}%
\Index%621%Р%разложение вектора относительно базиса сходится нормально
   {разложение вектора относительно базиса сходится нормально}%
   {expansion converges normally}%
\Index%417%Р%размерность rcd векторного пространства
   {размерность \rcd векторного пространства}%
   {dimension of vector space}%
\Index%554%Р%ранг квадратичного отображения тела
   {ранг квадратичного отображения тела}%
   {rank of quadratic map, division ring}%
\Index%749%Р%ранг эрмитовой матрицы по главным минорам
   {ранг эрмитовой матрицы по главным минорам}%
   {rank of Hermitian matrix by principal minors}%
\Index%419%Р%расслоение уровня 2
   {расслоение уровня $2$}%
   {bundle of level 2}%
\Index%418%Р%расслоение уровня n
   {расслоение уровня $n$}%
   {bundle of level n}%
\Index%420%Р%расслоенная Omega- алгебра
   {расслоенная $\Omega$\Hyph алгебра}%
   {fibered Omega-algebra}%
\Index%421%Р%расслоенная Omega- подалгебра
   {расслоенная $\Omega$\Hyph подалгебра}%
   {fibered Omega-subalgebra}%
\Index%422%Р%расслоенная группа
   {расслоенная группа}%
   {fibered group}%
\Index%423%Р%расслоенная группа стабилизации
   {расслоенная группа стабилизации}%
   {fibered stability group}%
\Index%424%Р%расслоенная малая группа
   {расслоенная малая группа}%
   {fibered little group}%
\Index%425%Р%расслоенная предупорядоченность
   {расслоенная предупорядоченность}%
   {fibered preordering}%
\Index%426%Р%расслоенная упорядоченность
   {расслоенная упорядоченность}%
   {fibered ordering}%
\Index%427%Р%расслоенная эквивалентность
   {расслоенная эквивалентность}%
   {fibered equivalence}%
\Index%428%Р%расслоенное кольцо
   {расслоенное кольцо}%
   {fibered ring}%
\Index%429%Р%расслоенное подмножество
   {расслоенное подмножество}%
   {fibered subset}%
\Index%430%Р%расслоенное соответствие в A
   {расслоенное соответствие в $\Bundle{A}$}%
   {fibered correspondence in A}%
\Index%431%Р%расслоенное соответствие гомоморфизма
   {расслоенное соответствие гомоморфизма}%
   {fibered correspondence of homomorphism}%
\Index%432%Р%расслоенное соответствие из A в B
   {расслоенное соответствие из $\Bundle A$ в $\Bundle B$}%
   {fibered correspondence from A to B}%
\Index%433%Р%расслоенный естественный морфизм
   {расслоенный естественный морфизм}%
   {fibered natural morphism}%
\Index%434%Р%расслоенный координатный Drc изоморфизм
   {расслоенный координатный \Drc изоморфизм}%
   {fibered coordinate drc isomorphism}%
\Index%435%Р%расслоенный морфизм из расслоения A в B
   {расслоенный морфизм из расслоения $\Bundle A$ в $\Bundle B$}%
   {fibered morphism from A into B}%
\Index%436%Р%расслоенный морфизм отождествления
   {расслоенный морфизм отождествления}%
   {fibered identification morphism}%
\Index%437%Р%расширенная матрица drc линейных уравнений
   {расширенная матрица \drc линейных уравнений}%
   {extended matrix, system of drc linear equations}%
\Index%438%Р%расширенная матрица rcd линейных уравнений
   {расширенная матрица \rcd линейных уравнений}%
   {extended matrix, system of rcd linear equations}%
\Index%439%Р%рефлексивное 2- арное расслоенное отношение
   {рефлексивное $2$\Hyph арное расслоенное отношение}%
   {reflexive 2 ary fibered relation}%
\Index%440%Р%ряд Тейлора
   {ряд Тейлора}%
   {Taylor series, division ring}%
\SetIndexSpace%
\Index%606%С%свободная алгебра над кольцом
   {свободная алгебра над кольцом}%
   {free algebra over ring}%
\Index%441%С%свободное Tstar- представление группы
   {свободное \Ts представление группы}%
   {free representation of group}%
\Index%442%С%свободное Tstar- представление расслоенной группы
   {свободное \Ts представление расслоенной группы}%
   {free representation of fibered group}%
\Index%690%С%свободный A- модуль
   {свободный $A$\Hyph модуль}%
   {free A module}%
\Index%612%С%свободный модуль над кольцом
   {свободный модуль над кольцом}%
   {free module over ring}%
\Index%443%С%связность Картана
   {связность Картана}%
   {Cartan connection}%
\Index%694%С%сечение расслоения
   {сечение расслоения}%
   {section of bundle}%
\Index%444%С%символ Картана
   {символ Картана}%
   {Cartan symbol}%
\Index%445%С%символ Кронекерa
   {символ Кронекерa}%
   {Kronecker symbol}%
\Index%446%С%симметричное 2- арное расслоенное отношение
   {симметричное $2$\Hyph арное расслоенное отношение}%
   {symmetric 2 ary fibered relation}%
\Index%447%С%симметричное билинейное отображение D- векторного пространства в тело
   {симметричное билинейное отображение $D$\Hyph векторного пространства в тело}%
   {symmetric bilinear map, vector space to division ring}%
\Index%650%С%симметричное полилинейное отображение в ассоциативную алгебру
   {симметричное полилинейное отображение в ассоциативную алгебру}%
   {polylinear map symmetric, associative algebra}%
\Index%448%С%синхронизация системы отсчёта
   {синхронизация системы отсчёта}%
   {synchronization of reference frame}%
\Index%449%С%система drc линейных уравнений
   {система \drc линейных уравнений}%
   {system of drc linear equations}%
\Index%311%С%система rcd линейных уравнений
   {система \rcd линейных уравнений}%
   {system of rcd linear equations}%
\Index%605%С%система аддитивных уравнений
   {система аддитивных уравнений}%
   {system of additive equations}%
\Index%450%С%система отсчёта в пространстве событий
   {система отсчёта в пространстве событий}%
   {reference frame in event space}%
\Index%781%С%скаляр отображения
   {скаляр отображения}%
   {scalar of mapping}%
\Index%784%С%скаляр элемента алгебры
   {скаляр элемента алгебры}%
   {scalar of algebra}%
\Index%773%С%скаляр элемента кольца
   {скаляр элемента кольца}%
   {scalar of ring}%
\Index%451%С%скалярный потенциал
   {скалярный потенциал}%
   {scalar potential}%
\Index%452%С%скорость отклонения
   {скорость отклонения}%
   {speed of deviation}%
\Index%743%С%след кватерниона
   {след кватерниона}%
   {trace, quaternion algebra}%
\Index%453%С%смешанная частная производная Гато
   {смешанная частная производная Гато}%
   {Gateaux partial derivative of Second Order}%
\Index%454%С%соответствие гомоморфизма
   {соответствие гомоморфизма}%
   {correspondence of homomorphism}%
\Index%455%С%соответствие, непрерывное на множестве
   {соответствие, непрерывное на множестве}%
   {correspondence continuous on the set}%
\Index%788%С%сопряжение в алгебре
   {сопряжение в алгебре}%
   {conjugation in algebra}%
\Index%777%С%сопряжение в кольце
   {сопряжение в кольце}%
   {conjugation in ring}%
\Index%580%С%сопряжённый D  модуль
   {сопряжённый $D$\Hyph  модуль}%
   {conjugated D module}%
\Index%457%С%стабильное множество представления
   {стабильное множество представления}%
   {stable set of representation}%
\Index%458%С%стандартная компонента дифференциала Гато
   {стандартная компонента производной Гато}%
   {standard component of Gateaux derivative}%
\Index%456%С%стандартная компонента линейного отображения
   {стандартная компонента линейного отображения}%
   {standard component of linear map}%
\Index%461%С%стандартная компонента над полем F билинейного отображения f
   {стандартная компонента над полем $F$ билинейного отображения $f$}%
   {standard component of bilinear map, division ring}%
\Index%462%С%стандартная компонента полилинейного отображения
   {стандартная компонента полилинейного отображения}%
   {standard component of polylinear map}%
\Index%463%С%стандартная компонента тензора
   {стандартная компонента тензора}%
   {standard component of tensor}%
\Index%466%С%стандартное представление квадратичного отображения тела над полем F
   {стандартное представление квадратичного отображения тела над полем $F$}%
   {quadratic map, standard representation, division ring}%
\Index%464%С%стандартное представление линейного отображения
   {стандартное представление линейного отображения}%
   {linear map, standard representation}%
\Index%468%С%стандартное представление матрицы
   {стандартное представление матрицы}%
   {Standard representation}%
\Index%469%С%стандартное представление над полем F билинейного отображения тела
   {стандартное представление над полем $F$ билинейного отображения тела}%
   {bilinear map, standard representation, division ring}%
\Index%470%С%стандартное представление полилинейного отображения
   {стандартное представление полилинейного отображения}%
   {polylinear map, standard representation}%
\Index%465%С%стандартное представление производной Гато
   {стандартное представление производной Гато}%
   {Gateaux derivative, standard representation}%
\Index%471%С%стандартные координаты rcd базиса
   {стандартные координаты \rcd базиса}%
   {standard coordinates of rcd basis}%
\Index%472%С%стандартные координаты базиса
   {стандартные координаты базиса}%
   {standard coordinates of basis}%
\Index%750%С%столбцовый определитель
   {столбцовый определитель}%
   {column determinant}%
\Index%748%С%строчный определитель
   {строчный определитель}%
   {row determinant}%
\Index%473%С%структурные константы
   {структурные константы}%
   {structural constants}%
\Index%474%С%сужение соответствия \Phi на множество C
   {сужение соответствия $\Phi$ на множество $C$}%
   {restriction of correspondence}%
\Index%476%С%сумма геометрических объектов
   {сумма геометрических объектов}%
   {sum of geometric objects}%
\Index%477%С%сумма геометрических объектов в векторном пространстве
   {сумма геометрических объектов в векторном пространстве}%
   {sum of geometric objects, vector space}%
\Index%351%С%сумма линейных отображений
   {сумма линейных отображений}%
   {sum of linear maps}%
\Index%667%С%сумма многочленов
   {сумма многочленов}%
   {sum of polynomials}%
\Index%712%С%суперпозиция координат эндоморфизма башни представлений и элемента
   {суперпозиция координат эндоморфизма башни представлений $\Vector f$ и элемента $\VX a$}%
   {superposition of coordinates, tower of representations}%
\Index%323%С%суперпозиция координат эндоморфизма представления и элемента
   {суперпозиция координат эндоморфизма представления $f$ и элемента $m$}%
   {superposition of coordinates, representation}%
\Index%51%С%существенные параметры  семейства функций
   {существенные параметры  семейства функций}%
   {essential parameters}%
\SetIndexSpace%
\Index%478%Т%тензор кручения
   {тензор кручения}%
   {torsion tensor}%
\Index%479%Т%тензор напряжённости поля
   {тензор напряжённости поля}%
   {field-strength tensor}%
\Index%802%Т%тензор, обратный тензору
   {тензор, обратный тензору}%
   {inverse tensor}%
\Index%652%Т%тензорная степень
   {тензорная степень}%
   {tensor power}%
\Index%480%Т%тензорное произведение D- векторных пространств
   {тензорное произведение $D$\Hyph векторных пространств}%
   {tensor product of D vector spaces}%
\Index%481%Т%тензорное произведение Dstar векторных пространств
   {тензорное произведение \Ds векторных пространств}%
   {tensor product of Dstar vector spaces}%
\Index%573%Т%тензорное произведение алгебр
   {тензорное произведение алгебр}%
   {tensor product of algebras}%
\Index%207%Т%тензорное произведение векторных пространств
   {тензорное произведение векторных пространств}%
   {tensor product of vector spaces}%
\Index%482%Т%тензорное произведение колец над коммутативным кольцом
   {тензорное произведение колец над коммутативным кольцом}%
   {tensor product of rings}%
\Index%483%Т%тензорное произведение представлений
   {тензорное произведение представлений}%
   {tensor product of representations}%
\Index%762%Т%тензорное произведение представлений
   {тензорное произведение представлений}%
   {tensor product of representations}%
\Index%484%Т%тензорное произведение тел
   {тензорное произведение тел}%
   {tensor product of division rings}%
\Index%485%Т%тип векторного пространства
   {тип векторного пространства}%
   {vector space type}%
\Index%310%Т%топологическая D-алгебра
   {топологическая $D$\Hyph алгебра}%
   {topological D algebra}%
\Index%486%Т%топологическое D- векторное пространство
   {топологическое $D$\Hyph векторное пространство}%
   {topological D vector space}%
\Index%790%Т%топологическое кольцо
   {топологическое кольцо}%
   {topological ring}%
\Index%488%Т%топологическое тело
   {топологическое тело}%
   {topological division ring}%
\Index%489%Т%транзитивное 2- арное расслоенное отношение
   {транзитивное $2$\Hyph арное расслоенное отношение}%
   {transitive 2 ary fibered relation}%
\Index%490%Т%транзитивное представление Omega- алгебры A
   {транзитивное представление $\Omega$\Hyph алгебры $A$}%
   {transitive representation of algebra}%
\Index%491%Т%транзитивное представление группы
   {транзитивное представление группы}%
   {transitive representation of group}%
\Index%492%Т%транзитивное представление расслоенной Omega- алгебры
   {транзитивное представление расслоенной $\Omega$\Hyph алгебры}%
   {transitive representation of fibered Omega-algebra}%
\SetIndexSpace%
\Index%751%У%упорядоченное слева представление подстановки произведением циклов
   {упорядоченное слева представление подстановки произведением циклов}%
   {left-ordered cycle notation of permutation}%
\Index%752%У%упорядоченное справа представление подстановки произведением циклов
   {упорядоченное справа представление подстановки произведением циклов}%
   {right-ordered cycle notation of permutation}%
\Index%493%У%уравнение Килинга
   {уравнение Килинга}%
   {Killing equation}%
\Index%494%У%уравнение Килинга второго рода
   {уравнение Килинга второго рода}%
   {Killing equation second type}%
\Index%744%У%условие перестановочности следа
   {условие перестановочности следа}%
   {permutability property of trace}%
\Index%495%У%условие приводимости произведений
   {условие приводимости произведений}%
   {condition of reducibility of products}%
\SetIndexSpace%
\Index%496%Ф%фактор расслоение
   {фактор расслоение}%
   {quotient bundle}%
\Index%497%Ф%фильтр F сходится к A
   {фильтр $\mathfrak{F}$ сходится к $A$}%
   {filter converges}%
\Index%131%Ф%финслерова метрика
   {финслерова метрика}%
   {Finsler metric}%
\Index%574%Ф%финслерова структура
   {финслерова структура}%
   {Finsler structure}%
\Index%77%Ф%финслерово пространство
   {финслерово пространство}%
   {Finsler space}%
\Index%498%Ф%форма кручение
   {форма кручение}%
   {torsion form}%
\Index%499%Ф%формула Тейлора для многочлена
   {формула Тейлора для многочлена}%
   {Taylor polynomial, division ring}%
\Index%243%Ф%фундаментальная последовательность
   {фундаментальная последовательность}%
   {fundamental sequence}%
\Index%504%Ф%функция тела, Dstar дифференцируемая по Фреше
   {функция тела, \Ds дифференцируемая по Фреше}%
   {function Dstar differentiable in Frechet sense, division ring}%
\Index%155%Ф%функция, однородная степени
   {функция, однородная степени $k$}%
   {function homogeneous}%
\SetIndexSpace%
\Index%620%Ц%центр алгебры
   {центр $D$\Hyph алгебры $A$}%
   {center of algebra}%
\Index%507%Ц%центр кольца D
   {центр кольца $D$}%
   {center of ring}%
\Index%508%Ц%центро-аффинный базис
   {центро-аффинный базис}%
   {Central Affine Basis, division ring}%
\Index%509%Ц%центро-аффинный базис
   {центро-аффинный базис}%
   {Central Affine Basis}%
\SetIndexSpace%
\Index%511%Ч%частная dcr производная Гато отображения f^b по переменной x^a
   {частная \dcr производная Гато отображения $f^{\gi b}$ по переменной $x^{\gi a}$}%
   {Gateaux partial dcr derivative of map with respect to variable, D vector space}%
\Index%512%Ч%частная производная Гато
   {частная производная Гато}%
   {Gateaux partial derivative}%
\Index%475%Ч%частное линейное отображение
   {частное линейное отображение}%
   {partial linear map}%
\SetIndexSpace%
\Index%566%Э%невырожденный эндоморфизм башни представлений
   {невырожденный эндоморфизм башни представлений}%
   {regular endomorphism of tower of representations}%
\Index%539%Э%эвклидова метрика на теле
   {эвклидова метрика на теле}%
   {Euclidean metric on division ring}%
\Index%547%Э%эвклидово скалярное произведение в D- векторном пространстве
   {эвклидово скалярное произведение в $D$\Hyph векторном пространстве}%
   {Euclidean scalar product, vector space}%
\Index%542%Э%эвклидово скалярное произведение на теле
   {эвклидово скалярное произведение на теле}%
   {Euclidean scalar product on division ring}%
\Index%515%Э%экстремальная кривая
   {экстремальная кривая}%
   {extreme line}%
\Index%559%Э%эндоморфизм башни представлений
   {эндоморфизм башни представлений}%
   {endomorphism of tower of representations}%
\Index%565%Э%эндоморфизм башни представлений, вырожденный на кортеже множеств образующих
   {эндоморфизм башни представлений, вырожденный на кортеже множеств образующих}%
   {endomorphism of representation, singular on tuple}%
\Index%564%Э%эндоморфизм башни представлений, невырожденный на кортеже множеств образующих
   {эндоморфизм башни представлений, невырожденный на кортеже множеств образующих}%
   {endomorphism of representation, regular on tuple}%
\Index%557%Э%эндоморфизм представления Omega алгебры
   {эндоморфизм представления $\Omega$\Hyph алгебры}%
   {endomorphism of representation}%
\Index%328%Э%эндоморфизм представления, вырожденный на множестве образующих X
   {эндоморфизм представления, вырожденный на множестве образующих $X$}%
   {endomorphism of representation, singular on set}%
\Index%327%Э%эндоморфизм представления, невырожденный на множестве образующих X
   {эндоморфизм представления, невырожденный на множестве образующих $X$}%
   {endomorphism of representation, regular on set}%
\Index%747%Э%эрмитова матрица
   {эрмитова матрица}%
   {hermitian matrix}%
\Index%544%Э%эрмитова метрика на теле
   {эрмитова метрика на теле}%
   {hermitian metric on division ring}%
\Index%350%Э%эрмитово скалярное произведение в D- векторном пространстве
   {эрмитово скалярное произведение в $D$\Hyph векторном пространстве}%
   {hermitian scalar product, vector space}%
\Index%545%Э%эрмитово скалярное произведение на теле
   {эрмитово скалярное произведение на теле}%
   {hermitian scalar product on division ring}%
\Index%541%Э%эрмитово сопряжение в теле
   {эрмитово сопряжение в теле}%
   {hermitian conjugation, division ring}%
\Index%546%Э%эрмитово сопряжённый вектор
   {эрмитово сопряжённый вектор}%
   {hermitian conjugated vector}%
\Index%500%Э%эффективное Tstar представление Omega- алгебры A
   {эффективное \Ts представление $\Omega$\Hyph алгебры $A$}%
   {effective Tstar representation of algebra}%
\Index%516%Э%эффективное Tstar- представление группы
   {эффективное \Ts представление группы}%
   {effective Tstar representation of group}%
\Index%514%Э%эффективное Tstar- представление расслоенного тела
   {эффективное \Ts представление расслоенного тела}%
   {effective representation of fibered division ring}%
\Index%520%Э%эффективное Tstar- представление расслоенной группы
   {эффективное \Ts представление расслоенной группы}%
   {effective representation of fibered group}%
\Index%517%Э%эффективное представление Omega- алгебры A
   {эффективное представление $\Omega$\Hyph алгебры $A$}%
   {effective representation of algebra}%
\Index%518%Э%эффективное представление группы
   {эффективное представление группы}%
   {effective representation of group}%
\Index%622%Э%эффективное представление кольца
   {эффективное представление кольца}%
   {effective representation of ring}%
\Index%519%Э%эффективное представление расслоенной Omega- алгебры
   {эффективное представление расслоенной $\Omega$\Hyph алгебры}%
   {effective representation of fibered Omega-algebra}%
\Index%521%Э%эффективное представление тела
   {эффективное представление тела}%
   {effective representation of division ring}%
\SetIndexSpace%
\Index%619%Я%ядро алгебры
   {ядро $D$\Hyph алгебры $A$}%
   {nucleus of algebra}%
\Index%522%Я%ядро линейного отображения
   {ядро линейного отображения}%
   {kernel of linear map}%
\Index%524%Я%ядро неэффективности Tstar- представления группы G
   {ядро неэффективности \Ts представления группы $G$}%
   {kernel of inefficiency of Tstar representation of group}%
\Index%525%Я%ядро неэффективности представления группы
   {ядро неэффективности представления группы}%
   {kernel of inefficiency of representation of group}%
\Index%526%Я%ядро неэффективности представления расслоенной группы
   {ядро неэффективности представления расслоенной группы}%
   {kernel of inefficiency of representation of fibered group}%
\Index%593%Я%якобиевая полная система drc дифференциальных уравнений
   {якобиевая полная система \drc дифференциальных уравнений}%
   {Jacobian complete system of drc differential equations}%
\Index%592%Я%якобиевая полная система дифференциальных уравнений
   {якобиевая полная система дифференциальных уравнений}%
   {Jacobian complete system of differential equations}%
\SetIndexSpace%
\Index%809%M%mu измеримое отображение
   {$\mu$\Hyph измеримое отображение}%
   {mu measurable map}%
\SetIndexSpace%
\Index%644%O%Omega группа
   {$\Omega$\Hyph группа}%
   {Omega group}%
\Index%646%O%Omega линейное отображение
   {$\Omega$\Hyph линейное отображение}%
   {Omega linear map}%
\Index%707%O%Omega_2- слово элемента представления относительно множества образующих
   {$\Omega_2$\Hyph слово элемента представления относительно множества образующих}%
   {word of element relative to generating set, representation}%
\SetIndexSpace%
\Index%658%S%sigma алгебра множеств
   {$\sigma$\Hyph алгебра множеств}%
   {sigma algebra of sets}%
\Index%795%S%sigma кольцо множеств
   {$\sigma$\Hyph кольцо множеств}%
   {sigma ring of sets}%

\CloseIndex


==> Linear.Map.English.tex <==
%auto-ignore
\input{Linear.Map.Eq}
\chapter{Linear Map
of \texorpdfstring{$\RCstar D$}{Rcd}\hyph Vector Space}
\label{chapter: rcd Linear Map}

\section{Linear Map
of \texorpdfstring{$\RCstar D$}{Rcd}\hyph Vector Space}
\label{section: rcd Linear Map}

In this subsection we assume $V$, $W$ are \rcd vector spaces.

\begin{definition}
Let us denote by
\ShowEq{set linear maps, rcd vector space}
set of linear maps
\ShowEq{A:V->W}
of \rcd vector space $V$
into \rcd vector space $W$.
Let us denote by
\ShowEq{set linear maps, drc vector space}
set of linear maps
\ShowEq{A:V->W}
of \drc vector space $V$
into \drc vector space $W$.
\qed
\end{definition}

%In the literature this is also referred to
%В литературе используется также обозначение $Hom_{D\RCstar}(V,W)$.
%Однако я предпочёл предложенное обозначение с точки зрения излагаемого материала.
We can consider division ring $D$ as \rcd vector space of dimension $1$.
Correspondingly we can consider set
$\mathcal L(D\RCstar;D;W)$ and $\LDVD$.

\begin{definition}
Let us denote by \symb{\mathcal L(*T;S;R)}1{set sT representations, division ring}
set of \sT representations of division ring $S$
in additive group of division ring $R$.
Let us denote by \symb{\mathcal L(T*;S;R)}1{set Ts representations, division ring}
set of \Ts representations of division ring $S$
in additive group of division ring $R$.
\qed
\end{definition}

\begin{theorem}
\label{theorem: sum of linear maps, rcd vector spaces}
Suppose $V$, $W$ are \rcd vector spaces.
Then set
$\LDVW$
is an Abelian group
relative composition law
\ShowEq{sum of linear maps, rcd vector space}
Linear map $A+B$ is called
\AddIndex{sum of linear maps}{sum of linear maps}
$A$ and $B$.
\end{theorem}
\begin{proof}
We need to show that mapping
\ShowEq{A+B:V->W}
defined by equation \EqRef{sum of linear maps, rcd vector space}
is linear map of \rcd vector spaces.
According to the definition
\xRef{0701.238}{definition: linear map of rcd vector spaces}
\ShowEq{sum of linear maps 1, rcd vector space}
We see that
\ShowEq{sum of linear maps 2, rcd vector space}
We need to show also that this operation is commutative.
\ShowEq{sum of linear maps 3, rcd vector space}
\end{proof}

\begin{theorem}
\label{theorem: matrix of linear map of rcd vector spaces}
Let
\ShowEq{basis in vector space V}
be a basis in \rcd vector space $V$
and
\ShowEq{basis in vector space W}
be a basis in \rcd vector space $W$.
Let
\ShowEq{matrix of linear map}
be arbitrary matrix.
Then map
\ShowEq{linear map of rcd vector spaces}
defined by equation
\ShowEq{linear map of rcd vector spaces, presentation}
relative to selected bases
is a linear map of \rcd vector spaces.
\end{theorem}
\begin{proof}
Theorem \ref{theorem: matrix of linear map of rcd vector spaces}
is inverse statement to theorem
\xRef{0701.238}{theorem: linear map of rcd vector space}.
Suppose
\ShowEq{linear map 1}
Then
\ShowEq{linear map 2}
\end{proof}

\begin{theorem}
\label{theorem: product of linear map over scalar, rcd vector space}
Let \ShowEq{basis in vector space V}
be a basis in \rcd vector space $V$
and \ShowEq{basis in vector space W}
be a basis in \rcd vector space $W$.
Suppose linear map $A$ has matrix
\ShowEq{matrix of linear map}
relative to selected bases.
Let $m\in D$.
Then matrix
\ShowEq{matrix mA of linear map}
defines linear map
\ShowEq{right action on linear map of rcd vector spaces}
which we call
\AddIndex{product of linear map $A$ over scalar}
{product of linear map over scalar}.
\end{theorem}
\begin{proof}
The statement of the theorem is corollary of the theorem
\ref{theorem: matrix of linear map of rcd vector spaces}.
\end{proof}

\begin{theorem}
\label{theorem: linear maps of rcd vector space}
Set $\LDVW$ is \drc vector space.
\end{theorem}
\begin{proof}
Theorem \ref{theorem: sum of linear maps, rcd vector spaces} states
that $\LDVW$ is an Abelian group.
It follows from theorem
\ref{theorem: product of linear map over scalar, rcd vector space}
that element of division ring $D$
defines \Ts transformation on the Abelian group
$\LDVW$.
From theorems \ref{theorem: matrix of linear map of rcd vector spaces},
\xRef{0701.238}{theorem: Ts representation of the ring}, and
\xRef{0701.238}{theorem: effective Ts representation of the division ring}
it follows that set $\LDVW$ is $D\star$\Hyph vector space.

\begin{sloppypar}
Writing elements of basis $D\star$\Hyph vector space $\LDVW$
as \subs rows or \sups rows, we represent
$D\star$\Hyph vector space $\LDVW$
as \dcr\ or \rcd vector space.
I want to stress that choice between \drc\ and \dcr linear
combination in $D\star$\Hyph vector space
$\LDVW$ does not depend on type of
vector spaces $V$ and $W$.
\end{sloppypar}

To select the type of vector space 
$\LDVW$
I draw attention to the following observation.
let $V$ and $W$ be \rcd vector spaces.
Suppose $\LDVW$ is \drc vector space.
Then we can represent the operation of \sups row of \rcd linear maps ${}^jA$
on \subs row of vectors $f_i$ as matrix
\ShowEq{linear maps of rcd vector space}
This notation is coordinated with matrix notation of action of \drc linear combination
$a\RCstar A$ of \rcd linear maps $A$.
\end{proof}

We can also define $\star D$\Hyph product of \rcd linear map $A$ over scalar.
However in general we cannot carry this
\sT representation of division ring $D$
in $D\star$\Hyph vector space
$\LDVW$ 
into \rcd vector space $W$. Indeed,
in case of $\star D$\Hyph product we get
\ShowEq{linear maps of rcd vector space, 1}
Since product in division ring is noncommutative, we cannot express
this expression as product of $A\RCstar v$ over $m$.

Ambiguity of notation
\ShowEq{linear maps of rcd vector space, 2}
is corollary of theorem \ref{theorem: linear maps of rcd vector space}.
We may assume that meaning of this notation is clear from the text.
To make notation more clear we will use
brackets. Expression
\ShowEq{linear maps of rcd vector space, 3}
means that \drc linear composition of \rcd linear maps ${}^iA$
maps the vector $v$ to the vector $w$.
Expression
\ShowEq{linear maps of rcd vector space, 4}
means that \RC product of \rcd linear mappings $A$ and $B$
maps the vector $v$ to the vector $w$.

\section{\texorpdfstring{$1$}{1}\hyph Form
on \texorpdfstring{$\RCstar D$}{rcd}\hyph Vector Space}
\label{section: 1-Form on a Vector Space}

\begin{definition}
\label{definition: left vector space}
\AddIndex{$1$\Hyph form}{1-form} on \rcd vector space $V$
is linear map
\ShowEq{1-form on rcd vector space}
\qed
\end{definition} 

We can write value of $1$\Hyph form $b$, defined for
vector $a$, as
\ShowEq{1-form on rcd vector space, 1}

\begin{theorem}
Set $\LDVD$ is $D\star$\Hyph vector space.
\end{theorem}
\begin{proof}
\rcd vector space of dimension 1 is equivalent to division ring $D$
\end{proof}

\begin{theorem}
\label{theorem: presentation of 1-form relative frame}
Let $\Basis e$ be a basis in \rcd vector space $V$.
$1$\Hyph form $b$ has presentation
\ShowEq{1-form on rcd vector space, presentation}
relative to selected basis, where vector $a$ has expansion
\ShowEq{1-form on rcd vector space, 2}
and
\ShowEq{1-form and vector of basis}
\end{theorem}
\begin{proof}
Because $b$ is $1$\Hyph form,
it follows from \EqRef{1-form on rcd vector space, 2} that
\ShowEq{1-form and vector a}
\EqRef{1-form on rcd vector space, presentation} follows from
\EqRef{1-form and vector a} and \EqRef{1-form and vector of basis}.
\end{proof}

\begin{theorem}
\label{theorem: 1-form is uniquely defined}
Let $\Basis e$ be a basis in \rcd vector space $V$.
$1$\Hyph form \EqRef{1-form on rcd vector space} is uniquely defined
by values \EqRef{1-form and vector of basis}
into which $1$\Hyph form $b$ maps vectors of basis.
\end{theorem}
\begin{proof}
Statement follows from theorems
\ref{theorem: presentation of 1-form relative frame} and
\xRef{0701.238}{theorem: expansion relative basis, vector space}.
\end{proof}

\begin{theorem}
Let $\Basis e$ be a basis in \rcd vector space $V$.
The set of $1$\Hyph forms
\ShowEq{basis d}
such that
\ShowEq{basis of dual vector space}
is basis $\Basis d$ of \drc vector space $\LDVD$.
\end{theorem}
\begin{proof}
Since we assume
\ShowEq{basis of dual vector space, 1},
then according to theorem \ref{theorem: 1-form is uniquely defined}
there exists the $1$\Hyph form
${}^{\gij}d$ for given $\gij$.
If we assume that there exists $1$\Hyph form
\ShowEq{basis of dual vector space, 2}
then
\ShowEq{basis of dual vector space, 3}
According to equation
\EqRef{basis of dual vector space},
\ShowEq{basis of dual vector space, 4}
Therefore, $1$\Hyph forms
${}^{\gij}d$ are linearly independent.
\end{proof}

\begin{definition}
Let $V$ be \rcd vector space.
\drc vector space
\symb{V^*}0{dual space of rcd vector space}
\[
\ShowSymbol{dual space of rcd vector space}=\LDVD
\]
is called \AddIndex{dual space of \rcd vector space}
{dual space of rcd vector space}
$V$.
Let $\Basis e$ be a basis in \rcd vector space $V$.
basis $\Basis d$ of \drc vector space $V^*$,
satisfying to equation \EqRef{basis of dual vector space},
is called \AddIndex{basis dual to basis}
{basis dual to basis} $\Basis e$.
\qed
\end{definition}

\begin{theorem}
Let $A$ be passive transformation of basis manifold
$\mathcal{B}(V,\RCGL nD)$.
Let basis
\ShowEq{dual space, image of basis}
be image of basis $\Basis e$.
Let $B$ be passive transformation of basis manifold
$\mathcal{B}(V^*,\RCGL nD)$ such, that basis
\ShowEq{dual space, image of dual basis}
is dual to basis.
Then
\begin{equation}
B=A^{\RCInverse}
\EqLabel{dual space, dual passive transformation}
\end{equation}
\end{theorem}
\begin{proof}
From equations
\EqRef{basis of dual vector space},
\EqRef{dual space, image of basis},
\EqRef{dual space, image of dual basis}
it follows
\ShowEq{dual space, passive transformations}
Equation \EqRef{dual space, dual passive transformation}
follows from equation \EqRef{dual space, passive transformations}.
\end{proof}

\section{Twin Representations of Division Ring}

\begin{theorem}
\label{theorem: Tstar structure of rcd vector space}
We can introduce structure of $D\star$\Hyph vector space
in any \rcd vector space defining
$D\star$\Hyph product of vector over scalar using equation
\ShowEq{Tstar structure of rcd vector space}
\end{theorem}
\begin{proof}
We verify directly that the map
\[
f:D\rightarrow V^\star
\]
defined by equation
\[
f(m)=m\delta
\]
defines \Ts representation of the ring $D$.
\end{proof}

We can formulate the theorem \ref{theorem: Tstar structure of rcd vector space} by other way.

\begin{theorem}
\label{theorem: twin representations of division ring}
%\begin{sloppypar}
Suppose we defined an effective \sT representation $f$ of ring $D$
on the Abelian group $V$.
Then we can uniquely define an effective \Ts representation $h$ of ring $D$
on the Abelian group $V$
such that diagram
\ShowEq{twin representations of division ring}
is commutative for any $a$, $b\in D$.
\qed
%\end{sloppypar}
\end{theorem}
%\begin{proof}
%\end{proof}

We call representations $f$ and $h$
\AddIndex{twin representations of the division ring}{twin representations of division ring} $D$.

\begin{theorem}
\label{theorem: twin representations, vector space}
In vector space
$V$ over division ring $D$ we
can define $D\star$\Hyph product and $\star D$\Hyph product of vector over scalar.
According to theorem \ref{theorem: twin representations of division ring} these operations 
satisfy equation
\begin{equation}
(am)b=a(mb)
\EqLabel{associative law for twin representations}
\end{equation}
\end{theorem}
Equation \EqRef{associative law for twin representations}
represents \AddIndex{associative law for twin representations}
{associative law for twin representations}.
This allows us writing of such expressions without using of brackets.
\begin{proof}
In section \ref{section: rcd Linear Map} there is definition of
$D\star$\Hyph product of \rcd linear map $A$ over scalar.
According to theorem \ref{theorem: Tstar structure of rcd vector space}
\Ts representation of division ring $D$ in $D\star$\Hyph vector space
$\LDVW$ can be carried
into \rcd vector space $W$ according to rule
\ShowEq{twin representations, vector space}
\end{proof}

The analogy of the vector space over field goes so far
that we can assume an existence of the concept of basis which
serves for $D\star$\Hyph product and $\star D$\Hyph product of vector over skalar.

\begin{theorem}
\label{theorem: rcd dcr basis, vector space}
Basis manifold of \rcd vector space $V$
and basis manifold of \crd vector space $V$ are different
\[
\mathcal{B}(V,D\RCstar)\ne\mathcal{B}(V,\CRstar D)
\]
\end{theorem}
\begin{proof}
To prove this theorem we use the standard representation of a matrix.
Without loss of generality we prove theorem in coordinate vector space
$D^n$.

Let
\ShowEq{e=delta}
be the set of vectors of vector space $D^{\gin}$.
$\Basis e$ is evidently basis of \rcd vector space
and basis of \crd vector space.
For arbitrary set of vectors
\ShowEq{set of vectors f}
\rcd coordinate matrix 
\ShowEq{set of vectors f 1}
relative to basis $\Basis e$ coincide with \crd coordinate matrix
relative to basis $\Basis e$.

Let the set of vectors
\ShowEq{set of vectors f}
be basis of \rcd vector space.
According to theorem \xRef{0701.238}{theorem: coordinate matrix of basis}
matrix \EqRef{set of vectors f 1} is \RC nonsingular matrix.

Let the set of vectors
\ShowEq{set of vectors f}
be basis of \crd vector space.
According to theorem \xRef{0701.238}{theorem: coordinate matrix of basis}
matrix \EqRef{set of vectors f 1} is \CR nonsingular matrix.

Therefore, if the set of vectors
\ShowEq{set of vectors f}
is basis \rcd of vector space and basis of \crd vector space,
their coordinate matrix \EqRef{set of vectors f 1}
is \RC nonsingular and \CR nonsingular matrix.
The statement follows from theorem \xRef{0701.238}{theorem: CR RC singular matrix}.
\end{proof}

From theorem \ref{theorem: rcd dcr basis, vector space}, it follows that
there exists basis $\Basis e$ of \drc vector space $V$
which is not basis of \crd vector space $V$.

\section{\texorpdfstring{$D$}{D}\hyph Vector Space}
\label{section: D Vector Space}

For many problems we may confine ourselves to
considering of $D\star$\Hyph vector space or $\star D$\Hyph vector space.
However there are problems where we forced to reject simple model and
consider both structures of vector space at the same time.

Twin representations of division ring $D$
in Abelian group $V$
determine the structure of
\AddIndex{$D$\hyph vector space}{D vector space}.
From this definition, it follows that if
$v$, $w\in V$, then for any $a$, $b$, $c$, $d\in D$
\ShowEq{D linear combination}
The expression
\EqRef{D linear combination}
is called
\AddIndex{linear combination of  vectors}
{linear combination of  vectors} of $D$\hyph vector space $V$.

\begin{definition}
\label{definition: linearly independent, D vector space}
Vectors
\ShowEq{Vector A subs row 02}
of $D$\Hyph vector space
$V$ are \AddIndex{linearly independent}
{linearly independent vectors}
if
\ShowEq{D linearly independent 1}
follows from the equation
\ShowEq{D linearly independent}
Otherwise vectors $a_i$
are \AddIndex{linearly dependent}{linearly dependent vectors}.
\qed
\end{definition}

\begin{definition}
We call set of vectors
\ShowEq{basis, vector space 01}
\AddIndex{basis for $D$\Hyph vector space}{basis, D vector space}
if vectors $e_{\gi i}$ are
linearly independent and adding to this system any other vector
we get a new system which is linearly dependent.
\qed
\end{definition}

\begin{theorem}
\label{theorem: D vector space has dcr basis}
A basis of $D$\Hyph vector space $V$
is basis of \dcr vector space $V$.
\end{theorem}
\begin{proof}
Let vectors
$a_i$, $i\in I$ are linear dependent in \dcr vector space.
Then there exists \subs row
\ShowEq{D dimension 0}
such that
\ShowEq{D dimension 1}
From the equation
\EqRef{D dimension 1},
it folows that
\ShowEq{D dimension 2}
According to the definition
\ref{definition: linearly independent, D vector space},
vectors $a_i$ are
linear dependent in $D$\Hyph vector space.

Let \dcr dimension of vector space $V$ is equal to $\gin$.
Let $\Basis e$ be basis of \dcr vector space.
Let
\[
\begin{pmatrix}
1&...&0
\\...&...&...\\
0&...&1
\end{pmatrix}
\]
be coordinate matrix of basis $\Basis e$.
It is evident that we cannot
present vector $e_{\gin}$ as
$D$\Hyph linear combination of vectors $e_{\giA}$,
..., $e_{\gi{n-1}}$.
%\[(c_0^{ki}\otimes c_1^{ki})f_k\]
%
%\[c_{0\cdot ki}=c_{0\cdot ki}^ne_n\]
%\[c_{1\cdot ki}=c_{1\cdot ki}^me_m\]
%\[e_ne_m=C_{nm}^pe_p\]
%\[f_k=h_k^rf_{kr}\]
%
%\[=>\]
%
%\[a^{ki}c_{0\cdot ki}^nc_{1\cdot ki}^mC_{nm}^pe_ph_k^rf_{kr}\]
\end{proof}

Whether the set of vectors
\ShowEq{ei, i in I}
is a basis of \rcd vector space
or a basis of \dcr vector space
is of no concern to us.
So we will use index in standard format
to represent coordinates of vector.
Based on the theorem
\ref{theorem: D vector space has dcr basis},
considering a basis of $D$\Hyph vector space $V$ we will consider it
as a basis of \dcr vector space $V$.



==> Linear.Map.Eq.tex <==
%auto-ignore

\def\LDVW{\mathcal L(\RCstar D;V;W)}
\def\LDVD{\mathcal L(\RCstar D;V;D)}
\def\Ii{\gii\in\giI}
\def\Jj{\gij\in\giJ}

\DefEq
{
\symb{\LDVW}1{set linear maps, rcd vector space}
}
{set linear maps, rcd vector space}

\DefEq
{
$b_{\gii}={}^{\gij}\delta_{\gii}$
}
{basis of dual vector space, 1}

\DefEquation
{
avb+cwd\in V
}
{D linear combination}

\DefEq
{
\[b^ia_ic^i=0\]
}
{D linearly independent}

\DefEq
{
\symb{\Basis{e}}0
{basis, vector space}
\[
\ShowSymbol{basis, vector space}
=(e_{\gi i},\gii\in\giI)
\]
}
{basis, vector space 01}

\DefEquation
{
c\CRstar a=0
}
{D dimension 1}

\DefEquation
{
c^ia_i1=0
}
{D dimension 2}

\DefEquation
{
\begin{pmatrix}
c^i&i\in I
\end{pmatrix}
\ne 0
}
{D dimension 0}

\DefEq
{
$b^ic^i=0$, $i=1$, ..., $n$,
}
{D linearly independent 1}

\DefEq
{
$a_i$, $i\in I$,
}
{Vector A subs row 02}

\DefEq
{
$A\RCstar v=e\RCstar A\RCstar v$.
}
{linear map 1}

\DefEq
{
\[
{}^{\gij}(mA)_{\gii}=m\ {}^{\gij}A_{\gii}
\]
}
{matrix mA of linear map}

\DefEq
{
\begin{align*}
A\RCstar(v\RCstar a)&=e\RCstar A\RCstar v\RCstar a\\
&=(A\RCstar v)\RCstar a
\end{align*}
}
{linear map 2}

\DefEq
{
$A=({}^{\gij}A_{\gii})$, $\Ii$, $\Jj$,
}
{matrix of linear map}

\DefEq
{
$\Basis e_W=(e_{W\cdot\gij},\Jj)$
}
{basis in vector space W}

\DefEq
{
$\Basis e_V=(e_{V\cdot\gii},\Ii)$
}
{basis in vector space V}

\DefEq
{
$(e_{\gii}, \gii\in \giI)$
}
{ei, i in I}

\DefEq
{
\[
mA:V\rightarrow W
\]
}
{right action on linear map of rcd vector spaces}

\DefEq
{
\[
\begin{pmatrix}
{}^1A \\
...  \\
{}^mA
\end{pmatrix}
\RCstar
\begin{pmatrix}
f_1 &
...  &
f_n
\end{pmatrix}
=
\begin{pmatrix}
{}^1A\RCstar f_1 & ... & {}^1A\RCstar f_n \\
... & ... & ...  \\
{}^mA\RCstar f_1 & ... &{}^mA\RCstar f_n 
\end{pmatrix}
\]
}
{linear maps of rcd vector space}

\DefEquation
{
<b,a>=b\RCstar a
}
{1-form on rcd vector space, presentation}

\DefEquation
{
a=e\RCstar a
}
{1-form on rcd vector space, 2}

\DefEq
{
\[
b_{\gii}=b_{\gij}\ {}^{\gij}\delta_{\gii}= 0
\]
}
{basis of dual vector space, 4}

\DefEq
{
\[
mv
=m\delta\RCstar v
\]
}
{Tstar structure of rcd vector space}

\DefEq
{
$\Basis e=(e_{\gii}=(\delta_{\gii}^{\gij})$,
$\gii$, $\gij\in \giI$, $|\giI|=\gin)$
}
{e=delta}

\DefEquation
{
f=
\left(
 \begin{array}{ccc}
f_{\giA}^{\giA} &...&f_{\giA}^{\gin}\\
... &...&...\\
f_{\gin}^{\giA} &...&f_{\gin}^{\gin}
\end{array}
\right)
}
{set of vectors f 1}

\DefEq
{
$(f_{\gii},\gii\in \giI,|\giI|=\gin)$
}
{set of vectors f}

\DefEq
{
\[
[mA]\RCstar v
=[m\delta]\RCstar(A\RCstar v)
=m(A\RCstar v)
\]
}
{twin representations, vector space}

\DefEquation
{
\begin{split}
{}^{\gij}\delta_{\gii}=&<{}^{\gij}d',e'_{\gii}>
\\
=&{}^{\gij}B_{\gil}\ <{}^{\gil}d,e_{\gik}>\ {}^{\gik}A_{\gii}
\\
=&{}^{\gij}B_{\gil}\ {}^{\gil}\delta_{\gik}\ {}^{\gik}A_{\gii}
\\
=&{}^{\gij}B_{\gik}\ {}^{\gik}A_{\gii}
\end{split}
}
{dual space, passive transformations}

\DefEquation
{
\Basis d'=B\RCstar\Basis d 
}
{dual space, image of dual basis}

\DefEquation
{
\Basis e'=\Basis e\RCstar A
}
{dual space, image of basis}

\DefEquation
{
<{}^{\gij}d,e_{\gii}>={}^{\gij}\delta_{\gii}
}
{basis of dual vector space}

\DefEq
{
\[
b_{\gij}<{}^{\gij}d,e_{\gii}>=0
\]
}
{basis of dual vector space, 3}

\DefEq
{
\[
b=b\RCstar d=0
\]
}
{basis of dual vector space, 2}

\DefEquation
{
<b,a>=<b,e\RCstar a>=<b,e_{\gii}>\ {}^{\gii}a
}
{1-form and vector a}

\DefEquation
{
b_{\gii}=<b,e_{\gii}>
}
{1-form and vector of basis}

\DefEq
{
${}^{\gii}d$
}
{basis d}

\DefEq
{
\[
b(a)=<b,a>
\]
}
{1-form on rcd vector space, 1}

\DefEquation
{
b:V\rightarrow D
}
{1-form on rcd vector space}

\DefEq
{
\[w=[m\RCstar A]\RCstar v\]
}
{linear maps of rcd vector space, 3}

\DefEq
{
\[w=B\RCstar A\RCstar v\]
}
{linear maps of rcd vector space, 4}

\DefEq
{
\[m\RCstar A\RCstar v\]
}
{linear maps of rcd vector space, 2}

\DefEq
{
\[
(Am)\RCstar v
=(Am)\RCstar f\RCstar v
=e\RCstar(Am)\RCstar v
\]
}
{linear maps of rcd vector space, 1}

\DefEq
{
\[
b=A\RCstar a
\]
}
{linear map of rcd vector spaces, presentation}

\DefEq
{
\begin{align*}
(A+B)\RCstar x
&=A\RCstar x+B\RCstar x\\
&=B\RCstar x+A\RCstar x\\
&=(B+A)\RCstar x
\end{align*}
}
{sum of linear maps 3, rcd vector space}

\DefEq
{
\begin{align*}
(A+B)\RCstar (x\RCstar a)
&=A\RCstar(x\RCstar a) +B\RCstar (x\RCstar a)\\
&=(A\RCstar x)\RCstar a+(B\RCstar x)\RCstar a\\
&=(A\RCstar x+B\RCstar x)\RCstar a\\
&=((A+B)\RCstar x)\RCstar a
\end{align*}
}
{sum of linear maps 2, rcd vector space}

\DefEq
{
\begin{align*}
A\RCstar(x\RCstar a)&=(A\RCstar x)\RCstar a
\\
B\RCstar(x\RCstar a)&=(B\RCstar x)\RCstar a
\end{align*}
}
{sum of linear maps 1, rcd vector space}

\DefEq
{
\[
A:V\rightarrow W
\]
}
{linear map of rcd vector spaces}

\DefEq
{
\[
\xymatrix{
V\ar[rr]^{h(a)}\ar[d]^{f(b)} & & V\ar[d]^{f(b)}\\
V\ar[rr]_{h(a)}& &V
}
\]
}
{twin representations of division ring}

\DefEquation
{
(A+B)\RCstar x=A\RCstar x+B\RCstar x
}
{sum of linear maps, rcd vector space}

\DefEq
{
\symb{\mathcal L(D\RCstar;V;W)}1{set linear maps, drc vector space}
}
{set linear maps, drc vector space}

\DefEq
{
\[
A+B:V\rightarrow W
\]
}
{A+B:V->W}

\DefEq
{
\[
A:V\rightarrow W
\]
}
{A:V->W}


==> Linear.Map.Russian.tex <==
%auto-ignore
\input{Linear.Map.Eq}
\chapter{Линейное отображение
\texorpdfstring{$\RCstar D$}{Rcd}\hyph векторного пространства}
\label{chapter: rcd Linear Map}

\section{Линейное отображение
\texorpdfstring{$\RCstar D$}{Rcd}\hyph векторного пространства}
\label{section: rcd Linear Map}

В этом разделе мы положим, что $V$, $W$ - это \rcd векторные пространства.

\begin{definition}
Обозначим
\ShowEq{set linear maps, rcd vector space}
множество линейных отображений
\ShowEq{A:V->W}
\rcd векторного пространства $V$
в \rcd векторное пространство $W$.
Обозначим
\ShowEq{set linear maps, drc vector space}
множество линейных отображений
\ShowEq{A:V->W}
\rcd векторного пространства $V$
в \rcd векторное пространство $W$.
\qed
\end{definition}

\begin{sloppypar}
%В литературе используется также обозначение $Hom_{D\RCstar}(V,W)$.
%Однако я предпочёл предложенное обозначение с точки зрения излагаемого материала.
Мы можем рассматривать тело $D$ как одномерное \rcd векторное пространство.
Соответственно мы можем рассматривать множества
$\mathcal L(\RCstar D;D;W)$ и $\LDVD$.
\end{sloppypar}

\begin{definition}
Обозначим \symb{\mathcal L(*T;S;R)}1{set sT representations, division ring}
множество \sT представлений тела $S$
в аддитивной группе тела $R$.
Обозначим \symb{\mathcal L(T*;S;R)}1{set Ts representations, division ring}
множество \Ts представлений тела $S$
в аддитивной группе тела $R$.
\qed
\end{definition}

\begin{theorem}
\label{theorem: sum of linear maps, rcd vector spaces}
Предположим, что $V$, $W$ - \rcd векторные пространства.
Тогда множество
$\LDVW$
является абелевой группой
относительно закона композиции
\ShowEq{sum of linear maps, rcd vector space}
Линейное отображение $A+B$ называется
\AddIndex{суммой линейных отображений}{sum of linear maps}
$A$ и $B$.
\end{theorem}
\begin{proof}
Нам надо показать, что отображение
\ShowEq{A+B:V->W}
определённое равенством \EqRef{sum of linear maps, rcd vector space},
- это линейное отображение \rcd векторных пространств.
Согласно определению
\xRef{0701.238}{definition: linear map of rcd vector spaces}
\ShowEq{sum of linear maps 1, rcd vector space}
Мы видим, что
\ShowEq{sum of linear maps 2, rcd vector space}
Нам надо показать так же, что эта операция коммутативна.
\ShowEq{sum of linear maps 3, rcd vector space}
\end{proof}

\begin{theorem}
\label{theorem: matrix of linear map of rcd vector spaces}
Пусть
\ShowEq{basis in vector space V}
- базис в \rcd векторном пространстве $V$
и
\ShowEq{basis in vector space W}
- базис в \rcd векторном пространстве $W$.
Пусть
\ShowEq{matrix of linear map}
- произвольная матрица.
Тогда отображение
\ShowEq{linear map of rcd vector spaces}
определённое равенством
\ShowEq{linear map of rcd vector spaces, presentation}
относительно выбранных базисов,
является линейным отображением \rcd векторных пространств.
\end{theorem}
\begin{proof}
Теорема \ref{theorem: matrix of linear map of rcd vector spaces}
является обратным утверждением теореме
\xRef{0701.238}{theorem: linear map of rcd vector space}.
Предположим
\ShowEq{linear map 1}
Тогда
\ShowEq{linear map 2}
\end{proof}

\begin{theorem}
\label{theorem: product of linear map over scalar, rcd vector space}
Пусть \ShowEq{basis in vector space V}
- базис в \rcd векторном пространстве $V$
и \ShowEq{basis in vector space W}
- базис в \rcd векторном пространстве $W$.
Предположим линейное отображение $A$ имеет матрицу
\ShowEq{matrix of linear map}
относительно выбранных базисов.
Пусть $m\in D$.
Тогда матрица
\ShowEq{matrix mA of linear map}
определяет линейное отображение
\ShowEq{right action on linear map of rcd vector spaces}
которое мы будем называть
\AddIndex{произведением линейного отображения $A$ на скаляр}
{product of linear map over scalar}.
\end{theorem}
\begin{proof}
Утверждение теоремы является следствием теоремы
\ref{theorem: matrix of linear map of rcd vector spaces}.
\end{proof}

\begin{theorem}
\label{theorem: linear maps of rcd vector space}
Множество $\LDVW$ является \drc векторным пространством.
\end{theorem}
\begin{proof}
Теорема \ref{theorem: sum of linear maps, rcd vector spaces} утверждает,
что $\LDVW$ - абелевая группа.
Из теоремы
\ref{theorem: product of linear map over scalar, rcd vector space} следует,
что элемент тела $D$
порождает \Ts преобразование на абелевой группе
$\LDVW$.
Из теорем \ref{theorem: matrix of linear map of rcd vector spaces},
\xRef{0701.238}{theorem: Ts representation of the ring} и
\xRef{0701.238}{theorem: effective Ts representation of the division ring}
следует, что множество $\LDVW$ является $D\star$\Hyph векторным пространством.

\begin{sloppypar}
Выписывая элементы базиса $D\star$\Hyph векторного пространства $\LDVW$
в виде \subs строки или \sups строки, мы представим
$D\star$\Hyph векторное пространство
$\LDVW$
как \dcr\ или \drc векторное пространство.
При этом надо иметь в виду, что выбор между \drc\ и \dcr линейной
зависимостью в $D\star$\Hyph векторном пространстве
$\LDVW$ не зависит от типа
векторных пространств $V$ и $W$.
\end{sloppypar}

Для того, чтобы выбрать тип векторного пространства
$\LDVW$
мы обратим внимание на следующее обстоятельство.
Допустим $V$ и $W$ - \rcd векторные пространства.
Допустим $\LDVW$ - \drc векторное пространство.
Тогда действие \sups строки \rcd линейных отображений ${}^jA$
на \subs строку векторов $f_i$ можно представить в виде матрицы
\ShowEq{linear maps of rcd vector space}
Эта запись согласуется с матричной записью действия \drc линейной комбинации
$a\RCstar A\ $ \rcd линейных отображений $A$.
\end{proof}

Мы можем также определить $\star D$\Hyph произведение
\rcd линейного отображения $A$ на скаляр.
Однако, вообще говоря, это \sT представление тела $D$
в $D\star$\Hyph векторном пространстве
$\LDVW$ не может быть перенесено
в \rcd векторное пространство $W$. Действительно,
в случае $\star D$\Hyph произведения мы имеем
\ShowEq{linear maps of rcd vector space, 1}
Поскольку произведение в теле не коммутативно, мы не можем выразить
полученное выражение как произведение $A\RCstar v$ на скаляр $m$.

Следствием теоремы \ref{theorem: linear maps of rcd vector space}
является неоднозначность записи
\ShowEq{linear maps of rcd vector space, 2}
Мы можем предположить, что смысл этой записи ясен из контекста.
Однако желательно неоднозначность избежать. Мы будем пользоваться для этой цели
скобками. Выражение
\ShowEq{linear maps of rcd vector space, 3}
означает, что \drc линейная комбинация \rcd линейных отображений ${}^iA$
отображает вектор $v$ в вектор $w$.
Выражение
\ShowEq{linear maps of rcd vector space, 4}
означает, что \RC произведение \rcd линейных отображений $A$ и $B$
отображает вектор $v$ в вектор $w$.

\section{\texorpdfstring{$1$}{1}\hyph форма
на \texorpdfstring{$\RCstar D$}{rcd}\hyph векторном пространстве}
\label{section: 1-Form on a Vector Space}

\begin{definition}
\label{definition: left vector space}
\AddIndex{$1$\Hyph форма}{1-form} на \rcd векторном пространстве $V$
- это линейное отображение
\ShowEq{1-form on rcd vector space}
\qed
\end{definition} 

Мы можем значение $1$\Hyph формы $b$, определённое для
вектора $a$, записывать в виде
\ShowEq{1-form on rcd vector space, 1}

\begin{theorem}
Множество $\LDVD$ является $D\star$\Hyph векторным пространством.
\end{theorem}
\begin{proof}
\rcd векторное пространство размерности 1 эквивалентно телу $D$
\end{proof}

\begin{theorem}
\label{theorem: presentation of 1-form relative frame}
Пусть $\Basis e$ - базис в \rcd векторном пространстве $V$.
$1$\Hyph форма $b$ имеет представление
\ShowEq{1-form on rcd vector space, presentation}
относительно выбранного базиса, где вектор $a$ имеет разложение
\ShowEq{1-form on rcd vector space, 2}
и
\ShowEq{1-form and vector of basis}
\end{theorem}
\begin{proof}
Так как $b$ - $1$\Hyph форма,
из \EqRef{1-form on rcd vector space, 2} следует, что
\ShowEq{1-form and vector a}
\EqRef{1-form on rcd vector space, presentation} следует из
\EqRef{1-form and vector a} и \EqRef{1-form and vector of basis}.
\end{proof}

\begin{theorem}
\label{theorem: 1-form is uniquely defined}
Пусть $\Basis e$ - базис в \rcd векторном пространстве $V$.
$1$\Hyph форма \EqRef{1-form on rcd vector space} однозначно определена
значениями \EqRef{1-form and vector of basis},
в которые $1$\Hyph форма $b$ отображает вектора базиса.
\end{theorem}
\begin{proof}
Утверждение является следствием теорем
\ref{theorem: presentation of 1-form relative frame} и
\xRef{0701.238}{theorem: expansion relative basis, vector space}.
\end{proof}

\begin{theorem}
Пусть $\Basis e$ - базис в \rcd векторном пространстве $V$.
Множество $1$\Hyph форм
\ShowEq{basis d}
таких, что
\ShowEq{basis of dual vector space}
является базисом $\Basis d$ \drc векторного пространства $\LDVD$.
\end{theorem}
\begin{proof}
$1$\Hyph форма ${}^{\gij}d$ существует для данного $\gij$ согласно теореме
\ref{theorem: 1-form is uniquely defined},
если положить
\ShowEq{basis of dual vector space, 1}.
Если предположить, что существует $1$\Hyph форма
\ShowEq{basis of dual vector space, 2}
то
\ShowEq{basis of dual vector space, 3}
Согласно равенству
\EqRef{basis of dual vector space}
\ShowEq{basis of dual vector space, 4}
Следовательно, $1$\Hyph формы
${}^{\gij}d$ линейно независимы.
\end{proof}

\begin{definition}
Пусть $V$ - \rcd векторное пространство.
\drc векторное пространство
\symb{V^*}0{dual space of rcd vector space}
\[
\ShowSymbol{dual space of rcd vector space}=\LDVD
\]
называется \AddIndex{дуальным пространством к \rcd векторному пространству}
{dual space of rcd vector space}
$V$.
Пусть $\Basis e$ - базис в \rcd векторном пространстве $V$.
базис $\Basis d$ \drc векторного пространства $V^*$,
удовлетворяющий равенству \EqRef{basis of dual vector space},
называется \AddIndex{базисом, дуальным базису}
{basis dual to basis} $\Basis e$.
\qed
\end{definition}

\begin{theorem}
Пусть $A$ - пассивное преобразование многообразия базисов
$\mathcal{B}(V,\RCGL nD)$.
Допустим базис
\ShowEq{dual space, image of basis}
является образом базиса $\Basis e$.
Пусть $B$ - пассивное преобразование многообразия базисов
$\mathcal{B}(V^*,\RCGL nD)$ такое, что базис
\ShowEq{dual space, image of dual basis}
дуален базису.
Тогда
\begin{equation}
B=A^{\RCInverse}
\EqLabel{dual space, dual passive transformation}
\end{equation}
\end{theorem}
\begin{proof}
Из равенств
\EqRef{basis of dual vector space},
\EqRef{dual space, image of basis},
\EqRef{dual space, image of dual basis}
следет
\ShowEq{dual space, passive transformations}
Равенство \EqRef{dual space, dual passive transformation}
следует из равенства \EqRef{dual space, passive transformations}.
\end{proof}

\section{Парные представления тела}

\begin{theorem}
\label{theorem: Tstar structure of rcd vector space}
\begin{sloppypar}
В любом \rcd векторном пространстве можно определить структуру
$D\star$\Hyph векторного пространства, определив
$D\star$\Hyph произведение вектора на скаляр равенством
\ShowEq{Tstar structure of rcd vector space}
\end{sloppypar}
\end{theorem}
\begin{proof}
Непосредственная проверка доказывает, что отображение
\[
f:D\rightarrow V^\star
\]
определённое равенством
\[
f(m)=m\delta
\]
определяет \Ts представление кольца $D$.
\end{proof}

Мы можем иначе сформулировать теорему \ref{theorem: Tstar structure of rcd vector space}.

\begin{theorem}
\label{theorem: twin representations of division ring}
%\begin{sloppypar}
Если мы определили эффективное \sT представление $f$ тела $D$
на абелевой группе $V$,
то мы можем однозначно определить эффективное \Ts представление $h$ тела $D$
на абелевой группе $V$
такое, что диаграмма
\ShowEq{twin representations of division ring}
коммутативна для любых $a$, $b\in D$.
\qed
%\end{sloppypar}
\end{theorem}
%\begin{proof}
%\end{proof}

Мы будем называть представления $f$ и $h$
\AddIndex{парными представлениями тела}{twin representations of division ring} $D$.

\begin{theorem}
\label{theorem: twin representations, vector space}
В векторном пространстве
$V$ над телом $D$ мы
можем определить $D\star$\Hyph произведение и $\star D$\Hyph произведение вектора на скаляр.
Согласно теореме \ref{theorem: twin representations of division ring} эти операции 
удовлетворяют равенству
\begin{equation}
(am)b=a(mb)
\EqLabel{associative law for twin representations}
\end{equation}
\end{theorem}
Равенство \EqRef{associative law for twin representations}
представляет \AddIndex{закон ассоциативности для парных представлений}
{associative law for twin representations}.
Это позволяет нам писать подобные выражения не пользуясь скобками.
\begin{proof}
В разделе \ref{section: rcd Linear Map} дано определение
$D\star$\Hyph произведения \rcd линейного отображения $A$ на скаляр.
Согласно теореме \ref{theorem: Tstar structure of rcd vector space}
\Ts представление тела $D$ в $D\star$\Hyph векторном пространстве
$\LDVW$ может быть перенесено
в \rcd векторном пространство $W$ согласно правилу
\ShowEq{twin representations, vector space}
\end{proof}

Аналогия с векторными пространствами над полем заходит столь далеко,
что мы можем предположить существование концепции базиса, который
годится для $D\star$\Hyph произведения и $\star D$\Hyph произведения вектора на скаляр.

\begin{theorem}
\label{theorem: rcd dcr basis, vector space}
Многообразие базисов \drc векторного пространства $V$
и многообразие базисов \crd векторного пространства $V$ отличны
\[
\mathcal{B}(V,D\RCstar)\ne\mathcal{B}(V,\CRstar D)
\]
\end{theorem}
\begin{proof}
При доказательстве этой теоремы мы будем пользоваться стандартным представлением
матрицы. Не нарушая общности, мы проведём доказательство в координатном векторном
пространстве $D^n$.

Пусть
\ShowEq{e=delta}
множество векторов векторного пространства $D^{\gin}$.
Очевидно, $\Basis e$ является одновременно базисом \drc векторного пространства
и базисом \crd векторного пространства.
Для произвольного множества векторов
\ShowEq{set of vectors f}
\drc координатная матрица 
\ShowEq{set of vectors f 1}
относительно базиса $\Basis e$ совпадает с \crd координатной матрицей
относительно базиса $\Basis e$.

Если множество векторов
\ShowEq{set of vectors f}
- базис \rcd векторного пространства,
то согласно \xRef{0701.238}{theorem: coordinate matrix of basis}
матрица \EqRef{set of vectors f 1} - \RC невырожденная матрица.

Если множество векторов
\ShowEq{set of vectors f}
- базис \crd векторного пространства,
то согласно теореме \xRef{0701.238}{theorem: coordinate matrix of basis}
матрица \EqRef{set of vectors f 1} - \CR невырожденная матрица.

Следовательно, если множество векторов
\ShowEq{set of vectors f}
порождают базис \drc векторного пространства и базис \crd векторного пространства,
их координатная матрица \EqRef{set of vectors f 1}
является \RC невырожденной и \CR невырожденной матрицей.
Утверждение следует из теоремы \xRef{0701.238}{theorem: CR RC singular matrix}.
\end{proof}

Из теоремы \ref{theorem: rcd dcr basis, vector space} следует, что
существует базис $\Basis e$ \drc векторного пространства $V$,
который не является базисом \crd векторного пространства $V$.

\section{\texorpdfstring{$D$}{D}\hyph векторное пространство}
\label{section: D Vector Space}

При изучении многих задач мы вполне можем ограничиться рассмотрением
$D\star$\Hyph векторного пространства либо $\star D$\Hyph векторного пространства.
Однако есть задачи, в которых мы вынуждены отказаться от простой модели
и одновременно рассматривать обе структуры векторного пространства.

Парное представление тела $D$
в абелевой группе $V$
определяет структуру
\AddIndex{$D$\hyph векторного пространства}{D vector space}.
Из этого определения следует, что если
$v$, $w\in V$, то для любых $a$, $b$, $c$, $d\in D$
\ShowEq{D linear combination}
Выражение
\EqRef{D linear combination}
называется
\AddIndex{линейной комбинацией векторов}
{linear combination of  vectors} $D$\hyph векторного пространства $V$.

\begin{definition}
\label{definition: linearly independent, D vector space}
Векторы
\ShowEq{Vector A subs row 02}
$D$\Hyph векторного пространства
$V$ \AddIndex{линейно независимы}
{linearly independent vectors},
если из равенства
\ShowEq{D linearly independent}
следует
\ShowEq{D linearly independent 1}
В противном случае, векторы $a_i$
\AddIndex{линейно зависимы}{linearly dependent vectors}.
\qed
\end{definition}

\begin{definition}
Мы называем множество векторов
\ShowEq{basis, vector space 01}
\AddIndex{базисом $D$\Hyph векторного пространства}{basis, D vector space},
если векторы $e_{\gii}$
линейно независимы и, добавив к этой системе любого другого вектора,
мы получим новую систему, которая является линейно зависимой.
\qed
\end{definition}

\begin{theorem}
\label{theorem: D vector space has dcr basis}
Базис $D$\Hyph векторного пространства $V$
является базисом \dcr векторного пространства $V$.
\end{theorem}
\begin{proof}
Пусть векторы
$a_i$, $i\in I$ линейно зависимы в \dcr векторном пространстве.
Тогда существует \subs строка
\ShowEq{D dimension 0}
такая, что
\ShowEq{D dimension 1}
Из равенства
\EqRef{D dimension 1},
следует, что
\ShowEq{D dimension 2}
Согласно определению
\ref{definition: linearly independent, D vector space},
векторы $a_i$
линейно зависимы в $D$\Hyph векторном пространстве.

Пусть \dcr размерность векторного пространства $V$ равна $\gin$.
Пусть $\Basis e$ - базис \dcr векторного пространства.
Пусть
\[
\begin{pmatrix}
1&...&0
\\...&...&...\\
0&...&1
\end{pmatrix}
\]
координатная матрица базиса $\Basis e$.
Очевидно, что мы не можем
представить вектор $e_{\gin}$ как
$D$\Hyph линейную комбинацию векторов $e_{\giA}$,
..., $e_{\gi{n-1}}$.
%\[(c_0^{ki}\otimes c_1^{ki})f_k\]
%
%\[c_{0\cdot ki}=c_{0\cdot ki}^ne_n\]
%\[c_{1\cdot ki}=c_{1\cdot ki}^me_m\]
%\[e_ne_m=C_{nm}^pe_p\]
%\[f_k=h_k^rf_{kr}\]
%
%\[=>\]
%
%\[a^{ki}c_{0\cdot ki}^nc_{1\cdot ki}^mC_{nm}^pe_ph_k^rf_{kr}\]
\end{proof}

Для нас несущественно, является ли множество векторов
\ShowEq{ei, i in I}
базисом \rcd векторного пространства
или базисом \dcr векторного пространства.
Поэтому при записи координат вектора мы индексы будем записывать
в стандартном формате.
Рассматривая базис $D$\Hyph векторного пространства $V$ мы,
опираясь на теорему
\ref{theorem: D vector space has dcr basis},
будем рассматривать его как базис \dcr векторного пространства $V$.



==> Preface.0812.4763.English.tex <==
%auto-ignore

\chapter{Preface}

\section{Preface to Version 1}
\label{section: Preface to Version 1}

\epigraph
{
The way of charms and disappointments.
//
However I would put it another way.
When you understand that the reason for
your disappointments is in your expectations,
you start to examine surrounding landscape.
You found yourself on the path
where nobody went before.
New impressions are stronger
then impressions from travel along well known and trodden road.
}
{Author is unknown. The Adventures of an Explorer.}

In mathematics like in everyday life there are
statements that after studying become obvious.
It may appear surprising when you first time meet
that these statements are false in new conditions.\footnote{I experienced such
sensation when I
considered Rolle's theorem
in the calculus over division ring.
After numerous attempts to change statement of Rolle's theorem,
I came to a conclusion that it is false
even for complex numbers.
It is enough to consider function
$w=z^2$. $z=0$ is the only point where derivative equal $0$.
However we can connect points $z=0.5$ and $z=-0.5$ by curve that does not pass
through point $z=0$.

\ifx\texFuture\Defined
Любопытен сам вопрос, что означает равенство нулю derivative.
Ответ пришёл не сразу, но понимая, что derivative это оператор,
я пришёл к выводу, что равенство нулю derivative означает, что
derivative является вырожденным оператором.
Действительно, в тех точках, где
$\displaystyle\frac{dy}{dx}=0$, $\Delta y=0$ для любого $\Delta x$.
\fi
}

When I started to study linear algebra over division ring I
was ready to different surprises related with noncommutativity
of product. However large number of statements similar to statements
of linear algebra over field
%apparently
relaxed my attention.
Nevertheless I met first deep problem in linear algebra:
definition of polylinear form and tensor product assumes that product is
commutative.
The firm belief that solving of particular problems gives key
to solving of general problem, was main motive,
prompting me to consider calculus over division ring.
This book introduces technique of differentiation
of mapping over division ring.
Since the possibility of linear approximation of mapping
is at the heart of calculus,
this book is natural consequence
of book \citeBib{0701.238}.
In calculus like in linear algebra we see statements
that we know well. However we see a lot of new statements.

The first considered definition of derivative was
based on classic definition of derivative. However
considering of derivative of function $x^2$, I discovered
that I cannot express this derivative analytically.
To answer the question of existence of derivative I decided to conduct
calculating experiment.
The best candidate for calculating experiment is
division ring of quaternions. Simple calculations make it clear that
sometimes derivative does not exist.
It causes that the set of differentiable functions is
very small, and such theory of differentiation is not
interesting.\footnote{Search
in papers and books shows that this is a deep problem.
Mathematicians try to solve this problem suggesting
different definitions of derivative. These definitions are based on different properties
of derivative of function of real or complex variable.
These definitions are very interesting. However my task is the study of
common rules for differentiation of maps of complete division ring of characteristic $0$.}
Analysis of calculating experiment shows
that an expression that depends on
increment of argument appears even derivative does not exist. We know such tool
in functional analysis. This is
the Fr\'echet derivative and the G\^ateaux derivative
in the space of linear operators.

When I defined the G\^ateaux \Ds derivative\footnote{In
this book I use notations introduced in
\citeBib{0701.238}.}, I put attention
that differential does not depend on using of
the G\^ateaux \Ds derivative or the G\^ateaux \sD derivative.
This caused me to change text and I started from definition
of differential.

The concept of \drc vector space is
powerful tool for study of linear spaces over
division ring. However the G\^ateaux differential does not fit in frame
of \drc vector space.
It follows from example \ref{example: differential dxx}
that $D$\Hyph vector space is the most appropriate model
for studying of the G\^ateaux differential.

\ePrints{0812.4763}
\ifx\Semafor\ValueOn
\input{Preface.Additive.English}
\fi

Consideration of the G\^ateaux differential
as additive map leads to new structure for definition
of derivative. In contrast to the G\^ateaux \drc derivative
components of the G\^ateaux differential
do not depend on direction. However components of the G\^ateaux differential
are defined non\Hyph uniquely and their number is uncertain.
It is evident that when we consider calculus over field,
the G\^ateaux \Ds derivative and components of the G\^ateaux differential coincide with
derivative. These structures appear as result of different
constructions. When product is commutative these
structures coincide. However noncomutativity breaks
expected relationship.
In spite of difference in behavior, these structures are supplemental.

\begin{flushright}
December, 2008
\end{flushright}

\section{Preface to Version 3}

Discussing the notion of derivative which I introduced in this book, I realized
that the subject of the book is very complex.
This is the reason why in this part of preface
I want to consider in more detail the concept of differentiation.

When we study functions of one variable, the derivative in selected point
is a number. When we study function of multiple variables, we realize
that it is not enough to use number. The derivative becomes vector or gradient.
When we study maps of vector spaces, this is a first time that we tell about derivative
as operator. However since this operator is linear, then we can represent
derivative as product over matrix. Again we express the derivative
as a set of numbers.

Surely, such behavior of derivative weaken our attention.
When we consider objects which are more complex than fields or vector spaces,
we still try to see an object which can be written as a factor before an increment
and which does not depend on the increment.
Quaternion algebra is
the simplest model of continuous division ring. However, an attempt to define derivative
as linear map is doomed to failure. Only certain linear functions
are differentiable in this sense.

The question arises as to whether there exists an alternative method if the set of linear maps restricts
our ability to study infinitesimal behavior of map? The answer on this question is affirmative.
Let us consider the quaternion algebra. The quaternion algebra is normed space.
We know two types of derivative in normed space. Strong derivative or
the Fr\'echet derivative is analogue of the derivative which we know very well.
When I wrote about attempt to find derivative as linear map as increment of argument,
I meant the Fr\'echet derivative.
Besides strong derivative there exits weak derivative or the G\^ateaux derivative.
The main idea is that derivative may depend on direction.

Vadim Komkov defines the G\^ateaux derivative for quaternion algebra
(\citeBib{Vadim Komkov}, p. 322) at the point $q$
in the direction of $q_1$ to be the quantity $q_2$ such that, for $\epsilon>0$
\[
f(q+\epsilon q_1)-f(q)=\epsilon(q_1 q_2)
\]
He made this definition according to definition \citeBib{Lebedev Vorovich}-3.1.2,
page 177.
This definition does not have difference from the Fr\'echet derivative.
This phenomenon remains in general case. Every time when we try
to extract the G\^ateaux derivative as factor, the identification of the G\^ateaux derivative
and the Fr\'echet derivative occurs.

A linear map of division ring is homomorphism of its additive group and homomorphism of
its multiplicative group in one map.
Homomorphism of multiplicative group is restrictive factor.
This is why it is mind to get rid of homomorphism of multiplicatie group
and to consider only homomorphism of additive group.
It is evident that the set of homomorphisms of additive group is more
wide than the set of linear maps. However, because we defined two operations
in division ring, additive map has a special structure.
This is why I selected these map into separate set and called them
additive maps.

Even in this case some elements of linearity remain.
The center of division ring is field. As a consequence, additive map is
linear over center. When division ring has characteristic $0$
and does not have discrete topology, we can embed real field
into center of division ring. As a consequence, the definition of derivative as additive map
appears equivalent to the definition of the G\^ateaux derivative.

Qualitative change happens exactly here. In additive map
we cannot extract an argument as factor. We cannot extract increment
from derivative.
Is this idea fundamentally new? I do not think so.
Derivative is a map. It is the map of differential of an argument
to differential of function.
Even additive map of increment of argument allows approximate the increment of function by
polynomial of first power.
The structure of polynomial over division ring is different from structure of polynomial over field.
I consider some properties of polynomial in section
\ref{section: Taylor Series}.
Using obtained theorems I explore
Taylor series expansion of map and method
to find solution of differential equation.

In the beginning I also tried to define derivative of map over division ring as Fr\'echet derivative.
However, I saw that this derivative does not satisfy to basic rules of differentiation,
and I realized that this is wrong way.
To make sure that the problem is fundamental, and is not inherent in the logic of my research,
I made computation in the division ring of quaternions.
That is where I discovered that the derivative is dependent on the direction.

At this time I studied maps of $D$\Hyph vector spaces, and idea of additive
map became leading one in this research. In preface to version 1
(section \ref{section: Preface to Version 1}) I wrote
about impressions of explorer who found oneself for the first time in unfamiliar land.
Expecting to see familiar landscapes, explorer does not notice
initially the peculiarity of new places.
I experience such change of impressions during this year when I wrote the book.

I did not realize right away that derivative which I discovered is the G\^ateaux derivative.
I could see
difference between my derivative and the G\^ateaux derivative.
I had to come a long way before realizing that two definitions are equivalent.
Like explorer, who tried to see familiar landscapes,
I considered possibility to extract increment from derivative.
As a consequence, the G\^ateaux \Ds derivative emerged.

If we consider new concepts, what will survive in the future? Surely, 
the G\^ateaux derivative and the G\^ateaux partial derivative will be basic concepts.
Components of the G\^ateaux derivative are important for considering of
structure of the G\^ateaux derivative. I do not think that I will consider the G\^ateaux \Ds derivative
in other cases except the G\^ateaux derivative of first order. Primary advantage of the G\^ateaux \Ds derivative
is that it allows you to explore conditions when map is continuous.

\begin{flushright}
May, 2009
\end{flushright}

\ePrints{0812.4763}
\ifx\Semafor\ValueOn
\section{Preface to Version 4}

\input{Preface.Linear.English}

\section{Preface to Version 5}

Recently, in internet, I found the book
\citeBib{Hamilton Elements of Quaternions 1},
where Hamilton found similar description of
calculus in quaternion algebra.
Although this book was written more than 100 years ago,
I recommend to read this book everybody who are interested
in problems of calculus over quaternion algebra.

\begin{flushright}
December, 2009
\end{flushright}
\fi


==> Preface.0812.4763.Russian.tex <==
%auto-ignore

\chapter{Предисловие}

\section{Предисловие к изданию 1}
\label{section: Preface to Version 1}

\epigraph
{Дорога очарований и разочарований.
//
Но я бы сказал наоборот.
Когда ты понимаешь, что причина
твоих разочарований - в твоих ожиданиях,
ты начинаешь присматриваться к окружающему ландшафту.
Ты оказался на тропе,
по которой до тебя никто не ходил.
И новые впечатления куда сильнее,
чем если бы ты шёл по дороге многократно протоптанной
и хорошо изученной.}
{Автор неизвестен. Записки путешественника.}

В математике, как и в обычной жизни, есть утверждения,
которые после изучения становятся очевидными.
И когда эти утверждения в новых условиях не работают,
это в первый момент вызывает удивление.\footnote{Подобного
рода ощущение я испытал, когда пытался
сформулировать теорему Ролля при
изучении математического анализа над телом.
После многократных попыток изменить формулировку теоремы
Ролля я понял, что это утверждение
неверно даже в случае комплексных чисел.
Достаточно рассмотреть функцию
$w=z^2$. $z=0$ - единственная точка, где производная равна $0$.
Однако точки $z=0.5$ и $z=-0.5$ могут быть соединены кривой, не проходящей
через точку $z=0$.

\ifx\texFuture\Defined
Любопытен сам вопрос, что означает равенство нулю производной.
Ответ пришёл не сразу, но понимая, что производная это оператор,
я пришёл к выводу, что равенство нулю производной означает, что
производная является вырожденным оператором.
Действительно, в тех точках, где
$\displaystyle\frac{dy}{dx}=0$, $\Delta y=0$ для любого $\Delta x$.
\fi
}

Когда я начал изучать линейную алгебру над телом, я
был готов к разным сюрпризам, связанными с некоммутативностью
умножения. Но большое количество утверждений, похожих на утверждения
линейной алгебры над полем, повидимому ослабили моё внимание.
И тем не менее, уже в линейной алгебре я встретил первую серьёзную
проблему: определение полилинейных форм и тензорного произведения
подразумевает коммутативность произведения.
Твёрдая уверенность, что решение конкретных задач даст ключ
к решению общей задачи, была основным мотивом,
побуждающим меня изучать математический анализ над телом.
Предлагаемая книга вводит в методы дифференцирования
отображений над телом и является естественным следствием
книги \citeBib{0701.238}, поскольку в основе математического
анализа лежит возможность линейного приближения к отображению.
В анализе, как и в линейной алгебре, мы встречаем утверждения,
которые нам хорошо знакомы. Однако есть немало новых и неожиданных утверждений.

Первое определение производной, которое я рассмотрел, было
основано на классическом определении производной. Однако
при попытке рассмотреть производную функции $x^2$ я обнаружил,
что не могу эту производную выразить аналитически.
Чтобы ответить на вопрос, существует ли
производная, я решил провести
вычислительный эксперимент.
Самый лучший кандидат для вычислительного эксперимента - это
тело кватернионов. Несложные расчёты показали, что в некоторых
случаях производная действительно не существует.
Это приводит к тому, что множество дифференцируемых функций
крайне бедно, а сама теория дифференцирования не представляет
серьёзного интереса.\footnote{Поиск
в статьях и книгах показал, что это действительно серьёзная проблема.
Математики пытаются решать эту задачу, предлагая
разные определения производной, основанные на тех или иных свойствах
производной функции действительного или комплексного переменного.
Эти конструкции очень интересны. Но моя задача рассмотреть
общие закономерности для дифференцирования отображений полного тела характеристики $0$.}
Анализ вычислительного эксперимента обнаруживает,
что даже если производная не существует, возникает выражение,
зависящее от приращения аргумента. Подобная конструкция
известна в функциональном анализе. Речь идёт о
производных Фреше и Гато в пространстве линейных операторов.

Когда я определил \Ds производную\footnote{В
этой книге я использую обозначения, введенные в
\citeBib{0701.238}.} Гато, я обратил внимание,
что дифференциал не зависит от того, использую ли я
\Ds производную Гато или \sD производную Гато.
Поэтому я изменил характер изложения и начал с определения
дифференциала.

Концепция \drc векторного пространства
является мощным инструментом изучения линейных пространств над
телом. Однако дифференциал Гато не укладывается в рамках
\drc векторного пространства.
Пример \ref{example: differential dxx} приводит к выводу,
что $D$\Hyph векторное пространство - наиболее адекватная модель
для изучения дифференциала Гато.

\ePrints{0812.4763}
\ifx\Semafor\ValueOn
\input{Preface.Additive.Russian}
\fi

Рассмотрение дифференциала Гато
как аддитивное отображение приводит к новой конструкции для определения
производной. В отличии от \drc производной Гато компоненты дифференциала Гато
не зависят от направления. Однако компоненты дифференциала Гато определены
неоднозначно и неопределенно их количество.
Очевидно, что, когда мы рассматриваем математический анализ над полем,
\Ds производная Гато и компоненты дифференциала Гато совпадают
с производной. Эти конструкции возникают в результате различных
построений. Когда произведение коммутативно эти
конструкции совпадают. Но как только произведение
становится не коммутативным, ожидаемая связь разрушается.
Несмотря на различие в поведении, эти конструкции взаимно дополняют друг друга.

\begin{flushright}
Декабрь, 2008
\end{flushright}

\section{Предисловие к изданию 3}

Обсуждая понятие производной, приведенное в этой книге, я понял,
что это очень сложная тема.
Поэтому в этой части введения я хочу рассмотреть более подробно концепцию дифференцирования.

Когда мы изучаем функции одной переменной, то производная в заданной точке
является числом. Когда мы изучаем функцию нескольких переменных, выясняется,
что числа недостаточно. Производная становится вектором или градиентом.
При изучении отображений векторных пространств мы впервые говорим о производной
как об операторе. Но так как этот оператор линеен, то мы можем представить
производную как умножение на матрицу, т. е. опять мы выражаем производную
как набор чисел.

Без сомнения, подобное поведение производной ослабляет наше внимание.
Когда мы переходим к объектам, более сложным чем поля или векторные пространства,
мы по прежнему пытаемся увидеть объект, который можно записать как множитель
перед приращением и который от приращения не зависит. Алгебра кватернионов - это
самая простая модель непрерывного тела. Однако попытка определить производную
как линейное отображение обречена на неудачу. Только линейная функция, да и то
не любая, дифференцируема в этом смысле.

Если множество линейных отображений ограничивает нашу возможность изучения поведения
отображений в малом, существует ли альтернатива. Ответ на этот вопрос положительный.
Рассмотрим алгебру кватернионов. Алгебра кватернионов - это нормированное пространство.
Мы знаем два типа производных в нормированном пространстве. Сильная производная или
производная Фреше является аналогом той производной, к которой мы привыкли.
Когда я писал о попытке найти производную как линейное отображение приращения аргумента,
я имел в виду производную Фреше.
Помимо сильной производной существует слабая производная или производная Гато.
Основная идея состоит в том, что производная может зависеть от направления.

Вадим Комков даёт определение производной Гато для тела кватернионов
(\citeBib{Vadim Komkov}, с. 322) следующим образом. Положим $q_2$ является
производной Гато в направлении $q_1$, если для $\epsilon>0$ справедливо
\[
f(q+\epsilon q_1)-f(q)=\epsilon(q_1 q_2)
\]
Это определение сделано согласно определению \citeBib{Lebedev Vorovich}-3.1.2,
стр. 256
и не сильно отличается от производной Фреше.
Это явление сохраняется и в общем случае. Всякий раз, когда мы пытаемся
выделить производную Гато как множитель, происходит отождествление производной
Гато и производной Фреше.

Линейное отображение тела - это гомоморфизм его аддитивной группы и гомоморфизм
его мультипликативной группы в одном отображении.
Ограничивающим фактором является гомоморфизм мультипликативной группы.
Поэтому есть смысл отложить в сторону гомоморфизм мультипликативной группы
и рассматривать только гомоморфизм аддитивной группы.
Очевидно, что множество гомоморфизмов аддитивной группы гораздо
шире, чем множество линейных отображений. Однако, так как в теле определены
две операции, аддитивное отображение имеет специальную структуру.
Поэтому я выделил эти отображения в отдельный класс и назвал их
аддитивными отображениями.

Даже в этом случае сохраняются некоторые элементы линейности.
Центр тела является полем. В результате аддитивное отображение оказывается
линейным над центром. Если тело имеет характеристику $0$
и не имеет дискретную топологию, то мы можем вложить поле действительных чисел
в центр тела. В результате определение производной как аддитивного отображения
оказывается эквивалентным определению производной Гато.

Именно здесь происходит качественный скачок. В аддитивном отображении
мы не можем выделить аргумент как множитель. Мы не можем выделить приращение из
производной.
Является ли эта концепция принципиально новой? Я не думаю.
Производная - это отображение. Это отображение дифференциала аргумента
в дифференциал функции.
Даже аддитивная функция приращения аргумента позволяет аппроксимировать приращение функции
полиномом первой степени.
Структура полинома над телом отличается от структуры полинома над полем.
Я рассматриваю некоторые свойства полинома в разделе
\ref{section: Taylor Series}.
Опираясь на полученные результаты, я изучаю разложение
отображения в ряд Тейлора и метод
решения дифференциального уравнения.

Я вначале тоже пытался определить производную отображения над телом как производную Фреше.
Но увидев, что эта производная не удовлетворяет основным правилам дифференцирования,
я понял, что это неверный путь. Чтобы убедиться, что проблема фундаментальна, а не в логике моих
построений, я выполнил расчёт в теле кватернионов. Именно здесь я обнаружил, что производная зависит
от направления.

В это время я изучал отображения $D$\Hyph векторных пространств, и концепция аддитивного
отображения стала ведущей идеей в этом исследовании. В предисловии к изданию 1
(раздел \ref{section: Preface to Version 1}) я писал
о впечатлениях путешественника, оказавшегося впервые в незнакомых краях. Желая
увидеть знакомые пейзажи, путешественник не сразу замечает необычность новых мест.
Такую смену впечатлений я испытал на протяжении этого года пока я писал книгу.

Я не сразу осознал, что найденная мною производная является производной Гато. Я даже видел
различия между моей производной и производной Гато. Потребовался длинный путь, пока я понял,
что два определения эквивалентны. Подобно путешественнику, который пытался увидеть знакомые пейзажи,
я изучал варианты как можно выделить приращение из производной.
В результате появилась \Ds производная Гато.

Что уцелеет из введенных понятий в будущем? Без сомнения основными понятиями будет собственно
производная Гато и частные производные Гато. Компоненты производной Гато важны для исследования
структуры производной Гато. Я не думаю, что \Ds производная Гато будет меня интересовать за
пределами производных Гато первого порядка. Основное преимущество \Ds производной Гато
состоит в том, что она позволяет изучить условия, когда отображение непрерывно.

\begin{flushright}
Май, 2009
\end{flushright}

\ePrints{0812.4763}
\ifx\Semafor\ValueOn
\section{Предисловие к изданию 4}

\input{Preface.Linear.Russian}

\section{Предисловие к изданию 5}

Недавно в интернете я нашёл книгу
\citeBib{Hamilton Elements of Quaternions 1},
в которой Гамильтон нашёл аналогичное описание
дифференциального исчисления в алгебре кватернионов.
И хотя эта книга написана более чем 100 лет назад,
я рекомендую прочесть эту книгу всем, кому интересны
проблемы анализа в алгебре кватернионов.

\begin{flushright}
Декабрь, 2009
\end{flushright}
\fi

==> Preface.Additive.English.tex <==
%auto-ignore
The considering of \drc linear maps leads to the concept
of twin representations of division ring in Abelian group.
Abelian group, in which we define twin representation of division ring $D$,
is called $D$\Hyph vector space.
Since we define multiplication over elements of division ring $D$ from left,
as well as right, then homomorphisms of $D$\Hyph vector spaces
cannot keep this operation. This leads to concept
of additive map which is morphism of $D$\Hyph vector
space.\footnote{Design of additive mapping which I made proving theorem
\ref{theorem: linear map, D vector space},
is instructive methodically. From the time when I
started to learn differential geometry, I accepted
the fact that we can everything express using tensor,
that we enumerate components of tensor by
indexes and this relationship is permanent.
Once I saw that it was not the case,
I found myself unprepared to recognize it
It got month before I was able to write down expression that I saw by my eyes.
The problem was because I tried to write down this expression in
tensor form.}


==> Preface.Additive.Russian.tex <==
%auto-ignore
Изучение \drc линейных отображений приводит к концепции
парных представлений тела в абелевой группе.
Абелева группа, в которой определено парное представление тела $D$,
называется $D$\Hyph векторным пространством.
Поскольку умножение на элементы тела $D$ определено и слева,
и справа, гомоморфизмы $D$\Hyph векторных пространств
не могут сохранять эту операцию. Это приводит к концепции
аддитивного отображения, которое является морфизмом $D$\Hyph векторных
пространств.\footnote{Построение аддитивного отображения, выполненное при доказательстве теоремы
\ref{theorem: linear map, D vector space},
весьма поучительно методически. С того самого момента,
когда я начал изучать дифференциальную геометрию, я признал
факт, что всё сводится к тензорам, что компоненты тензора нумеруются с
помощью индексов и эта связь неразрывна.
В тот момент, когда это оказалось не так, я оказался не готов признать это.
Понадобился месяц прежде, чем я смог записать выражение, которое я видел глазами,
но которое я не мог записать до этого, так как пытался выразить его в тензорной
или операторной форме.}


==> Preface.Linear.English.tex <==
%auto-ignore

Quaternion algebra is the simplest example of division ring.
This is why I verify
theorems in quaternion algebra to see how they work.
Quaternion algebra is similar to complex field
and so it is natural to search some parallel.

In real field any additive map automatically turns out to be
linear over real field. This statement is caused by statement that real
field is completion of rational field and is corollary of
theorem \ref{theorem: linear map, division ring, rational}.

However the statement changes for complex field.
Not every additive map of complex field is
linear over complex field. Conjugation is the simplest example of
such map.
As soon as I discovered this extremely interesting statement, I returned to question about
analytical representation of additive map.

Exploring additive maps, I realized that I too abruptly
expanded the set of linear maps while switching from field to division ring.
The reason for this was not a very clear understanding
of how to overcome the noncommutativity of the product.
However during the process of research it became more evident
that any additive map is linear over some field.
For the first time I used this concept when constructing the
tensor product
and the concept took shape in a subsequent study.

During constructing the tensor product of division rings $D_1$, ..., $D_n$
I assumed existence of field $F$ such that additive
map of division ring $D_i$ is linear over this field for any $i$. If all division rings
have characteristic $0$, then according to theorem
\ref{theorem: linear map, division ring, rational}
such field always exists. However
dependence of tensor product on selected field $F$ arises here.
To get rid of this dependence, I assume
that field $F$ is maximal field that possesses stated property.

If $D_1=...=D_n=D$, then such field is center $Z(D)$
of division ring $D$.
If the product in division ring $D$ is commutative\footnote{In other words,
division ring is field.}, then $Z(D)=D$.
So, starting with additive map, I arrive at concept
of linear map, which is generalization of linear map over field.

\ePrints{0812.4763}
\ifx\Semafor\ValueOn
%The set of additive maps contains disjoint subsets
%of additive maps generated by one generator, as well as
%maps that are linear combination of maps of first group.
%The set  of generators depends on division ring, however
%always includes identity map.

%My decision to explore additive map generated only by identity
%map was influenced by following.

%\item Additive map is morphism of representations of division ring $D$ in
%$D$\Hyph vextor space. We explore additive map of division ring $D$
%considering division ring $D$ as one dimensional $D$\Hyph vector space.
%If division $D$ is field, then additive map has
%to be linear. As we noted above, conjugation is
%not linear map of complex field.

My decision to explore the G\^ateaux derivative as linear map
was influenced by following.

\begin{itemize}

\item Linear map of field is homogeneous polynomial of
degree one.
%Complex polynomial depends on $z$, however it does not depend on $\overline z$.
%Like linear map, additive map is coordinated with structure of
%polynomial.

\item For continuous field derivative of function of field is homogeneous
polynomial of degree one that is good approximation to change of function.
The same time we explore the derivative as linear map of
field. At the transition to division ring we can save the same link
between derivative and additive map.

\end{itemize}

%Because additive map generated by identity map is the main object of our course
%I do not introduce new terminology and when I use
%termin additive map I have in mind additive map
%generated by identity map.
\fi

Research in area of complex numbers and quaternions
revealed one more interesting phenomenon. In spite of the fact that
complex field is extension of real
field, the structure of linear map over complex
field is different from the structure of linear map
over real field. This difference leads to the statement
that conjugation of complex numbers is additive map
but not linear map over complex field.

Similarly, the structure of linear map over division ring of
quaternions is different from the structure of linear map
over complex field.
The source of difference is statement that the center of quaternion algebra
has more simple structure than complex field.
This difference leads to the statement that
conjugation of quaternion satisfies to equation
\[
\overline p =-\frac 12 (p+ipi+jpj+kpk) 
\]
Consequently, the problem  to find a mapping satisfying
to a theorem similar to the Riemann theorem
(theorem \ref{theorem: complex field over real field}),
is a nontrivial task for quaternions.

\begin{flushright}
August, 2009
\end{flushright}


==> Preface.Linear.Russian.tex <==
%auto-ignore

Алгебра кватернионов - самый простой пример тела. Поэтому я проверяю
полученные мной теоремы в алгебре кватернионов, чтобы увидеть как они работают.
Алгебра кватернионов похожа на поле комплексных чисел
и поэтому естественно искать некоторые параллели.

В поле действительных чисел любое аддитивное отображение автоматически оказывается
линейным над полем действительных чисел. Это связано с тем, что поле действительных
чисел является пополнением поля рациональных чисел и является следствием
теоремы \ref{theorem: linear map, division ring, rational}.

Однако в случае комплексных чисел ситуация меняется.
Не всякое аддитивное отображение поля комплексных чисел оказывается
линейным над полем комплексных чисел. Операция сопряжения - простейший пример
такого отображения.
Когда я обнаружил этот крайне интересный факт, я вернулся к вопросу об
аналитическом представлении аддитивного отображения.

Изучая аддитивные отображения, я понял, что я слишком резко
расширил множество линейных отображений при переходе от поля к телу.
Причиной этому было не вполне ясное понимание как преодолеть
некоммутативность произведения.
Однако в процессе построений становилось всё более очевидным,
что любое аддитивное отображение линейно над некоторым полем.
Впервые эта концепция появилась при построении
тензорных произведений
и отчётливо проявилась в
последующем исследовании.

При построении тензорного произведения тел $D_1$, ..., $D_n$
я предполагаю существование поля $F$, над которым аддитивное
преобразование тела $D_i$ линейно для любого $i$. Если все тела
имеют характеристику $0$, то согласно теореме
\ref{theorem: linear map, division ring, rational}
такое поле всегда существует. Однако здесь возникает
зависимость тензорного произведения от выбранного поля $F$.
Чтобы избавиться от этой зависимости, я предполагаю,
что поле $F$ - максимальное поле, обладающее указанным свойством.

Если $D_1=...=D_n=D$, то такое поле является центром $Z(D)$
тела $D$.
Если произведение в теле $D$ коммутативно\footnote{Иными словами,
тело является полем.}, то $Z(D)=D$.
Следовательно, начав с аддитивного отображения, я пришёл к концепции
линейного отображения, которая является обобщением линейного отображения над полем.

\ePrints{0812.4763}
\ifx\Semafor\ValueOn
%Множество аддитивных отображений содержит непересекающиеся классы
%аддитивных отображений, порождаемых одной образующией, а также
%отображения, являющиеся линейной комбинацией отображений первой группы.
%Множество образующих зависит от тела, но всегда включает тождественное отображение.

%На моё решение изучать аддитивные отображения, порождаемые только тождественным
%отображением, повлияли следующие обстоятельства.

%\item Аддитивное отображение - это морфизм представлений тела $D$ в
%$D$\Hyph векторном пространстве. Мы изучаем аддитивное отображение тела $D$,
%рассматривая тело $D$ как одномерное $D$\Hyph векторное пространство.
%Если тело $D$ является полем, то аддитивное отображение должно
%стать линейным. Как мы заметили выше, операция сопряжения не
%является линейным отображением поля комплексных чисел.

На моё решение изучать производную Гато как линейное отображение
повлияли следующие обстоятельства.

\begin{itemize}

\item Линейное отображение поля - это в тоже время однородный многочлен
первой степени.
%Комплексный многочлен зависит от $z$, но не зависит от $\overline z$.
%Так же как и линейное отображение, аддитивное отображение должно быть согласовано со структурой
%многочлена.

\item Для непрерывных полей производная функции поля - это однородный
многочлен первого порядка, аппроксимирующий изменение функции.
Одновременно мы рассматриваем производную как линейное отображение
поля. При переходе к телу мы можем сохранить ту же связь
производной и аддитивного отображения.

\end{itemize}

%Так как основным объектом нашего изучения являются аддитивные отображения,
%порождённые тождественным отображением, я не ввожу новой терминологии и,
%употребляя термин аддитивное отображение, имею в виду аддитивное отображение,
%порождённое тождественным отображением.
\fi

Исследование в области комплексных чисел и кватернионов
проявили ещё одно интересное явление. Несмотря на то,
что поле комплексных чисел является расширением поля
действительных чисел, структура линейного отображения над полем
комплексных чисел отличается от структуры линейного отображения
над полем действительных чисел. Это различие приводит к тому,
что операция сопряжения комплексных чисел является аддитивным отображением,
но не является линейным отображением над полем комплексных чисел.

Аналогично, структура линейного отображения над телом
кватернионов отличается от структуры линейного отображения
над полем комплексных чисел.
Причина различия в том, что центр алгебры кватернионов
имеет более простую структуру, чем поле комплексных чисел.
Это отличие приводит к тому, что операция сопряжения
кватерниона удовлетворяет равенству
\[
\overline p =-\frac 12 (p+ipi+jpj+kpk) 
\]
Вследствие этого задача найти отображения, удовлетворяющие
теореме подобной теореме Римана
(теорема \ref{theorem: complex field over real field}),
является нетривиальной задачей для кватернионов.

\begin{flushright}
Август, 2009
\end{flushright}


==> Quaternion.English.tex <==
%auto-ignore
\ePrints{1003.1544,8433-5163}
\Items{Calculus.Paper}
\ifx\Semafor\ValueOn
\Chapter{Division Algebra}
\ePrints{Calculus.Paper}
\ifx\Semafor\ValueOn
In this section, we consider equations that follow from the theorem
\ref{theorem: Gateaux differential and jacobian, algebra}.
We consider
complex field, quaternion algebra and octonion algebra.
Although in the section \ref{chapter: Differentiable maps},
we explored differentiable maps into associative algebra,
but, as noted in the subsection
\ref{Section: Linear Map into Nonassociative Algebra},
equations which we write in nonassociative algebra,
differ slightly from equations which we write in associative algebra.
\fi%Calculus.Paper
\else%1003.1544,8433-5163,Calculus.Paper
\chapter{Quaternion Algebra}
\label{chapter: Quaternion Algebra}
\fi%1003.1544,8433-5163,Calculus.Paper

\input{\FilePrefix Complex.Number.English}

\input{\FilePrefix Quaternion.Eq}

\ePrints{Calculus.Paper}
\ifx\Semafor\ValueOff
\Section{Linear Function of Quaternion Algebra}

\begin{theorem}
\label{theorem: Quaternion over real field}
Let
\ShowEq{basis of quaternion}
be basis of quaternion algebra $H$.
Then in the basis \EqRef{basis of quaternion}, structural constants have form
\ShowEq{structural constants, quaternion}
\end{theorem}
\begin{proof}
Value of structural constants follows from multiplication table
\EqRef{product of quaternions}.
\end{proof}

Since calculations in this section get a lot of space,
I put in one place references to theorems in this section.
\begin{description}
\item [Theorem \ref{theorem: Standard components of linear function, quaternion},
page \pageref{theorem: Standard components of linear function, quaternion}]
the definition of coordinates of linear map
of quaternion algebra $H$
using standard components of this map.
\item [Equation \EqRef{quaternion, 3, B->A},
page \pageref{eq: quaternion, 3, B->A}]
matrix form of dependence of coordinates of linear map
of quaternion algebra $H$
from standard components of this map.
\item [Equation \EqRef{quaternion, 3, A->B},
page \pageref{eq: quaternion, 3, A->B}]
matrix form of dependence of standard components of linear map
of quaternion algebra $H$
from coordinates of this map.
\item [Theorem \ref{theorem: coordinates of linear function, quaternion},
page \pageref{theorem: coordinates of linear function, quaternion}]
dependence of standard components of a linear map
of quaternion algebra $H$
from coordinates of this map.
\ePrints{0812.4763}
\ifx\Semafor\ValueOff
\item [Equation \EqRef{quaternion conjugation},
page \pageref{eq: quaternion conjugation}]
quaternion conjugation is a linear map
\fi
\end{description}

\begin{theorem}
\label{theorem: Standard components of linear function, quaternion}
Standard components of linear function
of quaternion algebra $H$ relative to basis
\EqRef{basis of quaternion}
and coordinates of corresponding linear map
satisfy relationship
\ShowEq{quaternion linear system, 1}
\end{theorem}
\begin{proof}
Using equation
\ePrints{1003.1544,8433-5163}
\ifx\Semafor\ValueOn
\EqRef{coordinates of map A}
\else%1003.1544,8433-5163
\EqRef{linear map over field, division ring, relation}
\fi%1003.1544,8433-5163
we get relationships
\ShowEq{Standard components of linear function, 1, quaternion}

Equations
\ShowEq{quaternion linear system ref, 0}
form the system of linear equations
\EqRef{quaternion linear system, 1, 0}.

Equations
\ShowEq{quaternion linear system ref, 1}
form the system of linear equations
\EqRef{quaternion linear system, 1, 1}.

Equations
\ShowEq{quaternion linear system ref, 2}
form the system of linear equations
\EqRef{quaternion linear system, 1, 2}.

Equations
\ShowEq{quaternion linear system ref, 3}
form the system of linear equations
\EqRef{quaternion linear system, 1, 3}.
\end{proof}

\begin{theorem}
\label{theorem: Quaternion over real field, matrix}
Consider quaternion algebra $H$ with the basis
\EqRef{basis of quaternion}.
Standard components of linear function over field $F$
and coordinates of this function over field $F$
satisfy relationship
\ShowEq{quaternion, 3}
where
\ShowEq{quaternion, 3, 1}
\end{theorem}
\begin{proof}
\ePrints{Calculus.Paper}
\ifx\Semafor\ValueOn
The statement of the theorem is corollary of theorems
\ref{theorem: coordinates of map A1 A2, algebra},
\ref{theorem: Quaternion over real field}.
\else
Let us write the system of linear equations
\EqRef{quaternion linear system, 1, 0}
as product of matrices
\ShowEq{quaternion matrix 0}
Let us write the system of linear equations
\EqRef{quaternion linear system, 1, 1}
as product of matrices
\ShowEq{quaternion matrix 1}
From the equation \EqRef{quaternion matrix 1},
it follows that
\ShowEq{quaternion over real field, 3, 1}
Let us write the system of linear equations
\EqRef{quaternion linear system, 1, 2}
as product of matrices
\ShowEq{quaternion matrix 2}
From the equation \EqRef{quaternion matrix 2},
it follows that
\ShowEq{quaternion over real field, 3, 2}
Let us write the system of linear equations
\EqRef{quaternion linear system, 1, 3}
as product of matrices
\ShowEq{quaternion matrix 3}
From the equation \EqRef{quaternion matrix 3},
it follows that
\ShowEq{quaternion over real field, 3, 3}
We join equations
\EqRef{quaternion matrix 0},
\EqRef{quaternion over real field, 3, 1},
\EqRef{quaternion over real field, 3, 2},
\EqRef{quaternion over real field, 3, 3}
into equation
\EqRef{quaternion, 3, B->A}.
\fi
\end{proof}

\begin{theorem}
\label{theorem: coordinates of linear function, quaternion}
Standard components of linear function
of quaternion algebra $H$ relative to basis
\EqRef{basis of quaternion}
and coordinates of corresponding linear map
satisfy relationship
\ShowEq{quaternion over real field}
\end{theorem}
\begin{proof}
We get systems of linear equations
\EqRef{quaternion over real field, 2, 0},
\EqRef{quaternion over real field, 2, 1},
\EqRef{quaternion over real field, 2, 2},
\EqRef{quaternion over real field, 2, 3}
as the product of matrices in equation
\EqRef{quaternion, 3, A->B}.
\end{proof}

\ePrints{0812.4763}
\ifx\Semafor\ValueOff
\begin{theorem}
\label{theorem: quaternion conjugation}
Quaternion conjugation satisfies equation
\ShowEq{quaternion conjugation}
\end{theorem}
\begin{proof}
Quaternion conjugation is linear map with matrix
\ShowEq{quaternion conjugation, matrix}
The statement of theorem follows from the equation
\EqRef{quaternion, 3, A->B}
and statement \eqref{f in L(A,A), 2, associative algebra}
of the theorem \ref{theorem: linear map in L(A,A), associative algebra}.
\end{proof}
\fi
\fi%Calculus.Paper

\ePrints{0812.4763,0908.3307}
\Items{Calculus.Paper}
\ifx\Semafor\ValueOn
\ePrints{0812.4763,0908.3307}
\ifx\Semafor\ValueOn
\Section{Differentiable Map of Division Ring of Quaternions}
\label{section: Differentiable Map of Division Ring of Quaternions}
\fi

\begin{theorem}
\ePrints{Calculus.Paper}
\ifx\Semafor\ValueOn
Consider quaternion algebra $H$ with the basis
\ShowEq{basis of quaternion}
\fi
Since matrix
$\displaystyle
\begin{pmatrix}
\displaystyle\frac{\partial y^{\gi i}}{\partial x^{\gi j}}
\end{pmatrix}
$
is Jacobian matrix of the map
$
x\rightarrow y
$
of division ring of quaternions over real field,
then
\ePrints{0812.4763,0908.3307}
\ifx\Semafor\ValueOn
\ShowEq{quaternion over real field, derivative}
\else
\ShowEq{quaternion over real field, Jacobian matrix}
\fi
\end{theorem}
\begin{proof}
The statement of theorem is
corollary of theorem
\ePrints{0812.4763,0908.3307}
\ifx\Semafor\ValueOn
\ref{theorem: Standard components of linear function, quaternion}.
\else%0812.4763,0908.3307
\ePrints{Calculus.Paper}
\ifx\Semafor\ValueOn
\xRef{8433-5163}{theorem: Quaternion over real field, matrix}.
\else%Calculus.Paper
\ref{theorem: Quaternion over real field, matrix}.
\fi%Calculus.Paper
\fi%0812.4763,0908.3307
\end{proof}

\begin{theorem}
\label{theorem: quaternion conjugation, derivative}
Quaternionic map
\[
f(x)=\overline x
\]
has the G\^ateaux derivative
\ShowEq{quaternion conjugation, derivative}
\end{theorem}
\begin{proof}
\ePrints{0812.4763,0908.3307}
\ifx\Semafor\ValueOn
Jacobian matrix of the map $f$ has form
\ShowEq{quaternion conjugation, matrix}
From equations
\EqRef{quaternion over real field, derivative, 2, 0}
it follows that
\begin{equation}
\EqLabel{quaternion conjugation, derivative, 1}
\SP 00=
\SP 11=
\SP 22=
\SP 33=
-\frac 12
\end{equation}
From equations
\EqRef{quaternion over real field, derivative, 2, 1},
\EqRef{quaternion over real field, derivative, 2, 2},
\EqRef{quaternion over real field, derivative, 2, 3}
it follows that
\begin{equation}
\EqLabel{quaternion conjugation, derivative, 2}
\SP ij=0
\ \ \ \gi i\ne\gi j
\end{equation}
Equation
\EqRef{quaternion conjugation, derivative}
follows from equations
\EqRef{Gateaux derivative, division ring, standard representation},
\EqRef{quaternion conjugation, derivative, 1},
\EqRef{quaternion conjugation, derivative, 2}.
\else
\ePrints{Calculus.Paper}
\ifx\Semafor\ValueOn
Jacobian matrix of the map $f$ has form
\ShowEq{quaternion conjugation, matrix}
The statement of the theorem follows from equations
\EqRef{Gateaux derivative, algebra, standard representation},
\EqRef{Jacobian, A->B},\EqRef{quaternion conjugation, matrix}.
\else%Calculus.Paper
The theorem is corollary of the theorem
\ref{theorem: Gateaux derivative of linear map},
\ref{theorem: quaternion conjugation}.
\fi%Calculus.Paper
\fi
\end{proof}

\begin{theorem}
The norm of quaternion satisfies equations\footnote{The statement of the
theorem is similar to example X,
\citeBib{Hamilton Elements of Quaternions 1}, p. 455.}
\ShowEq{norm of quaternion, derivative}
\end{theorem}
\begin{proof}
\ePrints{0812.4763}
\ifx\Semafor\ValueOff
The equation
\EqRef{norm2 of quaternion, derivative} follows from
equations
\EqRef{Gateaux derivative, fg, algebra},
\EqRef{Gateaux derivative, fx=axb, algebra},
\EqRef{norm of quaternion},
\EqRef{quaternion conjugation, derivative}.
\else
theorem
\ref{theorem: quaternion conjugation, derivative}
and equations
\EqRef{norm of quaternion},
\EqRef{Gateaux derivative of product, division ring}.
Since $\NormX\in R$,
than the equation
\EqRef{norm of quaternion, derivative}
follows from the equation
\EqRef{norm2 of quaternion, derivative}.
\fi
\end{proof}
\fi

\ePrints{0812.4763}
\begin{theorem}
In division ring of quaternions over real field $H$
with basis
\EqRef{basis of quaternion}
standard \Ds representation of the G\^ateaux differential of map $x^2$
has form
\[
\partial x^2(a)=(x+x_1)a+x_2ai+x_3aj+x_4ak
\]
\end{theorem}
\begin{proof}
The theorem follows from the definition
\ref{definition: Gateaux Dstar derivative, division ring}.
\end{proof}
\ifx\Semafor\ValueOn
\fi

\ePrints{1003.1544,8433-5163}
\Items{Calculus.Paper}
\ifx\Semafor\ValueOff
\begin{theorem}
We can identify quaternion
\ShowEq{quaternion a}
and matrix
\ShowEq{quaternion product ax, Jacobian}
\end{theorem}
\begin{proof}
The product of quaternions
\EqRef{quaternion a} and
\ShowEq{quaternion x}
has form
\ShowEq{quaternion product ax}
Therefore, function $f_a(x)=ax$ has Jacobian matrix
\EqRef{quaternion product ax, Jacobian}.
It is evident that $f_a\circ f_b=f_{ab}$. Similar equation
is true for matrices
\ShowEq{quaternion ab, Jacobian product}
Therefore, we can identify the quaternion $a$ and the matrix $J_a$.
\end{proof}
\fi



==> Quaternion.Eq.tex <==
%auto-ignore

\newcommand\FM[2]{f^{\gi #1}_{\gi #2}}%
\newcommand\FP[2]{\displaystyle\frac{\partial y^{\gi #1}}{\partial x^{\gi #2}}}%
\newcommand\FC[2]{f^{\gi{#1#2}}}%
\newcommand\SP[2]{\displaystyle\StandPartial{y}{x}{#1#2}}%

\input{\FilePrefix Algebra.Quaternion.Eq}

\DefEq
{
\begin{equation}
f:R\rightarrow H
\EqLabel{function from R to H}
\end{equation}
}
{function from R to H}

\DefEquation
{
\begin{array}{r@{\ }l}
\overline x
&\displaystyle
=-\frac 12(1\otimes 1+i\otimes i+j\otimes j+k\otimes k)\circ x
\\[6pt]
&\displaystyle%\VirtFrac
=-\frac 12(x+ixi+jxj+kxk)
\end{array}
}
{quaternion conjugation}

\DefEq
{
\begin{equation}
a=a^{\gi 0}+a^{\giA}i+a^{\gi 2}j+a^{\gi 3}k
\EqLabel{quaternion a}
\end{equation}
}
{quaternion a}

\DefEq
{
\[
x=x^{\gi 0}+x^{\giA}i+x^{\gi 2}j+x^{\gi 3}k
\]
}
{quaternion x}

\DefEq
{
\begin{align*}
ax
&=a^{\gi 0}x^{\gi 0}-a^{\giA}x^{\giA}-a^{\gi 2}x^{\gi 2}-a^{\gi 3}x^{\gi 3}
+(a^{\gi 0}x^{\giA}+a^{\giA}x^{\gi 0}+a^{\gi 2}x^{\gi 3}-a^{\gi 3}x^{\gi 2})i
\\
&+(a^{\gi 0}x^{\gi 2}+a^{\gi 2}x^{\gi 0}+a^{\gi 3}x^{\giA}-a^{\giA}x^{\gi 3})j
+(a^{\gi 0}x^{\gi 3}+a^{\gi 3}x^{\gi 0}+a^{\giA}x^{\gi 2}-a^{\gi 2}x^{\giA})k
\end{align*}
}
{quaternion product ax}

\DefEquation
{
J_a=
\left(
\begin{array}{rr@{}rr@{}rr@{}r}
a^{\gi 0}&-&a^{\giA}&-&a^{\gi 2}&-&a^{\gi 3}
\\
a^{\giA}&&a^{\gi 0}&-&a^{\gi 3}&&a^{\gi 2}
\\
a^{\gi 2}&&a^{\gi 3}&&a^{\gi 0}&-&a^{\giA}
\\
a^{\gi 3}&-&a^{\gi 2}&&a^{\giA}&&a^{\gi 0}
\end{array}
\right)
}
{quaternion product ax, Jacobian}

\DefEq
{
\begin{align*}
&
\left(
\begin{array}{rr@{}rr@{}rr@{}r}
a^{\gi 0}&-&a^{\giA}&-&a^{\gi 2}&-&a^{\gi 3}
\\
a^{\giA}&&a^{\gi 0}&-&a^{\gi 3}&&a^{\gi 2}
\\
a^{\gi 2}&&a^{\gi 3}&&a^{\gi 0}&-&a^{\giA}
\\
a^{\gi 3}&-&a^{\gi 2}&&a^{\giA}&&a^{\gi 0}
\end{array}
\right)
\left(
\begin{array}{rr@{}rr@{}rr@{}r}
b^{\gi 0}&-&b^{\giA}&-&b^{\gi 2}&-&b^{\gi 3}
\\
b^{\giA}&&b^{\gi 0}&-&b^{\gi 3}&&b^{\gi 2}
\\
b^{\gi 2}&&b^{\gi 3}&&b^{\gi 0}&-&b^{\giA}
\\
b^{\gi 3}&-&b^{\gi 2}&&b^{\giA}&&b^{\gi 0}
\end{array}
\right)
\\
=&
\left(
\begin{array}{rrrr}
a^{\gi 0}b^{\gi 0}-a^{\giA}b^{\giA}
&-a^{\gi 0}b^{\giA}-a^{\giA}b^{\gi 0}
&-a^{\gi 0}b^{\gi 2}+a^{\giA}b^{\gi 3}
&-a^{\gi 0}b^{\gi 3}-a^{\giA}b^{\gi 2}
\\
-a^{\gi 2}b^{\gi 2}-a^{\gi 3}b^{\gi 3}
&-a^{\gi 2}b^{\gi 3}+a^{\gi 3}b^{\gi 2}
&-a^{\gi 2}b^{\gi 0}-a^{\gi 3}b^{\giA}
&+a^{\gi 2}b^{\giA}-a^{\gi 3}b^{\gi 0}
\\
\\
a^{\gi 0}b^{\giA}+a^{\giA}b^{\gi 0}
&a^{\gi 0}b^{\gi 0}-a^{\giA}b^{\giA}
&-a^{\gi 0}b^{\gi 3}-a^{\giA}b^{\gi 2}
&a^{\gi 0}b^{\gi 2}-a^{\giA}b^{\gi 3}
\\
+a^{\gi 2}b^{\gi 3}-a^{\gi 3}b^{\gi 2}
&-a^{\gi 2}b^{\gi 2}-a^{\gi 3}b^{\gi 3}
&+a^{\gi 2}b^{\giA}-a^{\gi 3}b^{\gi 0}
&+a^{\gi 2}b^{\gi 0}+a^{\gi 3}b^{\giA}
\\
\\
a^{\gi 0}b^{\gi 2}-a^{\giA}b^{\gi 3}
&a^{\gi 0}b^{\gi 3}+a^{\giA}b^{\gi 2}
&a^{\gi 0}b^{\gi 0}-a^{\giA}b^{\giA}
&-a^{\gi 0}b^{\giA}-a^{\giA}b^{\gi 0}
\\
+a^{\gi 2}b^{\gi 0}+a^{\gi 3}b^{\giA}
&-a^{\gi 2}b^{\giA}+a^{\gi 3}b^{\gi 0}
&-a^{\gi 2}b^{\gi 2}-a^{\gi 3}b^{\gi 3}
&-a^{\gi 2}b^{\gi 3}-a^{\gi 3}b^{\gi 2}
\\
\\
a^{\gi 0}b^{\gi 3}+a^{\giA}b^{\gi 2}
&-a^{\gi 0}b^{\gi 2}+a^{\giA}b^{\gi 3}
&a^{\gi 0}b^{\giA}+a^{\giA}b^{\gi 0}
&a^{\gi 0}b^{\gi 0}-a^{\giA}b^{\giA}
\\
-a^{\gi 2}b^{\giA}+a^{\gi 3}b^{\gi 0}
&-a^{\gi 2}b^{\gi 0}-a^{\gi 3}b^{\giA}
&+a^{\gi 2}b^{\gi 3}-a^{\gi 3}b^{\gi 2}
&-a^{\gi 2}b^{\gi 2}-a^{\gi 3}b^{\gi 3}
\end{array}
\right)
\end{align*}
}
{quaternion ab, Jacobian product}

\DefEq
{
\begin{equation}
f=
\begin{pmatrix}
f^{\gi 0}&f^{\giA}&f^{\gi 2}&f^{\gi 3}
\end{pmatrix}
\EqLabel{function from R to H, coordinates}
\end{equation}
}
{function from R to H, coordinates}

\DefEq
{
\begin{equation}
G=
\begin{pmatrix}
G^{\gi 0}&G^{\giA}&G^{\gi 2}&G^{\gi 3}
\end{pmatrix}
\EqLabel{function from R to H, generator}
\end{equation}
}
{function from R to H, generator}

\DefEq
{
\begin{equation}
f^{\gi j}=&G^{\gil}\ \FC kr_G\ C^{\gi p}_{\gi{kl}}
C_{\gi{pr}}^{\gi j}
\EqLabel{function from R to H, relation}
\end{equation}
}
{function from R to H, relation}

\DefEq
{
\begin{equation}
\EqLabel{quaternion over real field, 2, 0}
\left\{
\begin{array}{r@{}l}
4\FC 00&=\FM 00+\FM 11+\FM 22+\FM 33
\\
\VirtVar
4\FC 11&=-\FM 00-\FM 11+\FM 22+\FM 33
\\
\VirtVar
4\FC 22&=-\FM 00+\FM 11-\FM 22+\FM 33
\\
\VirtVar
4\FC 33&=-\FM 00+\FM 11+\FM 22-\FM 33
\end{array}
\right.
\end{equation}
\begin{equation}
\EqLabel{quaternion over real field, 2, 1}
\left\{
\begin{array}{r@{}l}
4\FC 10&=-\FM 01+\FM 01-\FM 23+\FM 32
\\
\VirtVar
4\FC 01&=-\FM 01+\FM 01+\FM 23-\FM 32
\\
\VirtVar
4\FC 32&=-\FM 01-\FM 01-\FM 23-\FM 32
\\
\VirtVar
4\FC 23&=\FM 01+\FM 01-\FM 23-\FM 32
\end{array}
\right.
\end{equation}
\begin{equation}
\EqLabel{quaternion over real field, 2, 2}
\left\{
\begin{array}{r@{}l}
4\FC 20&=-\FM 02+\FM 13+\FM 20-\FM 31
\\
\VirtVar
4\FC 31&=\FM 02-\FM 13+\FM 20-\FM 31
\\
\VirtVar
4\FC 02&=-\FM 02-\FM 13+\FM 20+\FM 31
\\
\VirtVar
4\FC 13&=-\FM 02-\FM 13-\FM 20-\FM 31
\end{array}
\right.
\end{equation}
\begin{equation}
\EqLabel{quaternion over real field, 2, 3}
\left\{
\begin{array}{r@{}l}
4\FC 30&=-\FM 03-\FM 12+\FM 21+\FM 30
\\
\VirtVar
4\FC 21&=-\FM 03-\FM 12-\FM 21-\FM 30
\\
\VirtVar
4\FC 12&=\FM 03-\FM 12-\FM 21+\FM 30
\\
\VirtVar
4\FC 03&=-\FM 03+\FM 12-\FM 21+\FM 30
\end{array}
\right.
\end{equation}
}
{quaternion over real field}

\def\JacobianA
{
\left(
\begin{array}{rrrr}
\VirtFrac
\FP 00
&
\FP 01
&
\FP 02
&
\FP 03
\\
\VirtFrac
\FP 11
&
-\FP 01
&
\FP 13
&
\VirtFrac
-\FP 12
\\
\FP 22
&
-\FP 23
&
-\FP 20
&
\FP 21
\\
\VirtFrac
\FP 33
&
\FP 32
&
-\FP 31
&
-\FP 30
\end{array}
\right)
}

\def\JacobianB
{
\left(
\begin{array}{rrrr}
\VirtFrac
\SP 00
&
-\SP 01
&
-\SP 02
&
-\SP 03
\\
\VirtFrac
\SP 11
&
\SP 10
&
\SP 13
&
-\SP 12
\\
\VirtFrac
\SP 22
&
-\SP 23
&
\SP 20
&
\SP 21
\\
\VirtFrac
\SP 33
&
\SP 32
&
-\SP 31
&
\SP 30
\end{array}
\right)
}

\def\MatrixA
{
\left(
\begin{array}{rrrr}
\FM 00
&
\FM 01
&
\FM 02
&
\FM 03
\\
\FM 11
&
-\FM 01
&
\FM 13
&
-\FM 12
\\
\FM 22
&
-\FM 23
&
-\FM 20
&
\FM 21
\\
\FM 33
&
\FM 32
&
-\FM 31
&
-\FM 30
\end{array}
\right)
}

\def\MatrixB
{
\left(
\begin{array}{rrrr}
\FC 00
&
-\FC 01
&
-\FC 02
&
-\FC 03
\\
\FC 11
&
\FC 10
&
\FC 13
&
-\FC 12
\\
\FC 22
&
-\FC 23
&
\FC 20
&
\FC 21
\\
\FC 33
&
\FC 32
&
-\FC 31
&
\FC 30
\end{array}
\right)
}

\def\MatrixAB
{
\left(
\begin{array}{rrrr}
1&-1&-1&-1
\\
1&-1&1&1
\\
1&1&-1&1
\\
1&1&1&-1
\end{array}
\right)
}

\def\MatrixBA
{
\frac 14
\left(
\begin{array}{rrrr}
1&1&1&1
\\
-1&-1&1&1
\\
-1&1&-1&1
\\
-1&1&1&-1
\end{array}
\right)
}

\DefEq
{
\[
\MatrixAB^{-1}=\MatrixBA
\]
}
{quaternion, 3, 1}

\DefEq
{
\begin{equation}
\begin{array}{r@{}l}
&
\MatrixA
\\
=&
\MatrixAB
\MatrixB
\end{array}
\EqLabel{quaternion, 3, B->A}
\end{equation}
\begin{equation}
\begin{array}{r@{}l}
&
\MatrixB
\\
=&
\displaystyle
\MatrixBA
\MatrixA
\end{array}
\EqLabel{quaternion, 3, A->B}
\end{equation}
}
{quaternion, 3}

\DefEquation
{
\ePrints{Calculus.Paper}
\ifx\Semafor\ValueOn
\frac{\partial\overline x}{\partial x}=
\fi
\begin{pmatrix}
1&0&0&0
\\
0&-1&0&0
\\
0&0&-1&0
\\
0&0&0&-1
\end{pmatrix}
}
{quaternion conjugation, matrix}

\DefEq
{
\begin{align}
\left(
\begin{array}{r}
\FM 00
\\
\FM 11
\\
\FM 22
\\
\FM 33
\end{array}
\right)
=
\left(
\begin{array}{rrrr}
1&-1&-1&-1
\\
1&-1&1&1
\\
1&1&-1&1
\\
1&1&1&-1
\end{array}
\right)
\left(
\begin{array}{r}
\FC 00
\\
\FC 11
\\
\FC 22
\\
\FC 33
\end{array}
\right)
}
{quaternion matrix 0}

\DefEq
{
\begin{align*}
\left(
\begin{array}{r}
-\FM 01
\\
\FM 01
\\
\FM 32
\\
-\FM 23
\end{array}
\right)
&=
\left(
\begin{array}{rrrr}
-1&-1&-1&1
\\
-1&-1&1&-1
\\
-1&1&-1&-1
\\
-1&1&1&1
\end{array}
\right)
\left(
\begin{array}{r}
\FC 01
\\
\FC 10
\\
\FC 23
\\
\FC 32
\end{array}
\right)
\\
&=
\left(
\begin{array}{rrrr}
1&-1&1&1
\\
1&-1&-1&-1
\\
1&1&1&-1
\\
1&1&-1&1
\end{array}
\right)
\left(
\begin{array}{r}
-\FC 01
\\
\FC 10
\\
-\FC 23
\\
\FC 32
\end{array}
\right)
\end{align*}
\begin{equation}
\left(
\begin{array}{r}
\FM 01
\\
-\FM 01
\\
-\FM 23
\\
\FM 32
\end{array}
\right)
=
\left(
\begin{array}{rrrr}
1&-1&-1&-1
\\
1&-1&1&1
\\
1&1&-1&1
\\
1&1&1&-1
\end{array}
\right)
\left(
\begin{array}{r}
-\FC 01
\\
\FC 10
\\
-\FC 23
\\
\FC 32
\end{array}
\right)
\EqLabel{quaternion over real field, 3, 1}
\end{equation}
}
{quaternion over real field, 3, 1}

\DefEq
{
\begin{align*}
\left(
\begin{array}{r}
-\FM 20
\\
-\FM 31
\\
\FM 02
\\
\FM 13
\end{array}
\right)
&=
\left(
\begin{array}{rrrr}
-1&1&-1&-1
\\
-1&1&1&1
\\
-1&-1&-1&1
\\
-1&-1&1&-1
\end{array}
\right)
\left(
\begin{array}{r}
\FC 02
\\
\FC 13
\\
\FC 20
\\
\FC 31
\end{array}
\right)
\\
&=
\left(
\begin{array}{rrrr}
1&1&-1&1
\\
1&1&1&-1
\\
1&-1&-1&-1
\\
1&-1&1&1
\end{array}
\right)
\left(
\begin{array}{r}
-\FC 02
\\
\FC 13
\\
\FC 20
\\
-\FC 31
\end{array}
\right)
\end{align*}
\begin{equation}
\left(
\begin{array}{r}
\FM 02
\\
\FM 13
\\
-\FM 20
\\
-\FM 31
\end{array}
\right)
=
\left(
\begin{array}{rrrr}
1&-1&-1&-1
\\
1&-1&1&1
\\
1&1&-1&1
\\
1&1&1&-1
\end{array}
\right)
\left(
\begin{array}{r}
-\FC 02
\\
\FC 13
\\
\FC 20
\\
-\FC 31
\end{array}
\right)
\EqLabel{quaternion over real field, 3, 2}
\end{equation}
}
{quaternion over real field, 3, 2}

\DefEq
{
\begin{align*}
\left(
\begin{array}{r}
-\FM 30
\\
\FM 21
\\
-\FM 12
\\
\FM 03
\end{array}
\right)
&=
\left(
\begin{array}{rrrr}
-1&-1&1&-1
\\
-1&-1&-1&1
\\
-1&1&1&1
\\
-1&1&-1&-1
\end{array}
\right)
\left(
\begin{array}{r}
\FC 03
\\
\FC 12
\\
\FC 21
\\
\FC 30
\end{array}
\right)
\\
&=
\left(
\begin{array}{rrrr}
1&1&1&-1
\\
1&1&-1&1
\\
1&-1&1&1
\\
1&-1&-1&-1
\end{array}
\right)
\left(
\begin{array}{r}
-\FC 03
\\
-\FC 12
\\
\FC 21
\\
\FC 30
\end{array}
\right)
\end{align*}
\begin{equation}
\left(
\begin{array}{r}
\FM 03
\\
-\FM 12
\\
\FM 21
\\
-\FM 30
\end{array}
\right)
=
\left(
\begin{array}{rrrr}
1&-1&-1&-1
\\
1&-1&1&1
\\
1&1&-1&1
\\
1&1&1&-1
\end{array}
\right)
\left(
\begin{array}{r}
-\FC 03
\\
-\FC 12
\\
\FC 21
\\
\FC 30
\end{array}
\right)
\EqLabel{quaternion over real field, 3, 3}
\end{equation}
}
{quaternion over real field, 3, 3}

\DefEquation
{
\begin{matrix}
e_{\gi 0}=1&e_{\giA}=i&
e_{\gi 2}=j&e_{\gi 3}=k
\end{matrix}
}
{basis of quaternion}

\DefEq
{
\begin{equation}
\EqLabel{quaternion over real field, derivative, 1, 0}
\left\{
\begin{matrix}
\displaystyle
\frac{\partial y^{\gi 0}}{\partial x^{\gi 0}}=\SP 00-\SP 11-\SP 22-\SP 33
\\
\displaystyle
\vphantom{\overset{\rightarrow}{\frac{\partial}{\partial}}}
\frac{\partial y^{\giA}}{\partial x^{\giA}}=\SP 00-\SP 11+\SP 22+\SP 33
\\
\displaystyle
\vphantom{\overset{\rightarrow}{\frac{\partial}{\partial}}}
\frac{\partial y^{\gi 2}}{\partial x^{\gi 2}}=\SP 00+\SP 11-\SP 22+\SP 33
\\
\displaystyle
\vphantom{\overset{\rightarrow}{\frac{\partial}{\partial}}}
\frac{\partial y^{\gi 3}}{\partial x^{\gi 3}}=\SP 00+\SP 11+\SP 22-\SP 33
\end{matrix}
\right.
\end{equation}
\begin{equation}
\EqLabel{quaternion over real field, derivative, 1, 1}
\left\{
\begin{matrix}
\displaystyle
\frac{\partial y^{\giA}}{\partial x^{\gi 0}}=\SP 01+\SP 10+\SP 23-\SP 32
\\
\displaystyle
\vphantom{\overset{\rightarrow}{\frac{\partial}{\partial}}}
\frac{\partial y^{\gi 0}}{\partial x^{\giA}}=-\SP 01-\SP 10+\SP 23-\SP 32
\\
\displaystyle
\frac{\partial y^{\gi 3}}{\partial x^{\gi 2}}=-\SP 01+\SP 10-\SP 23-\SP 32
\\
\displaystyle
\vphantom{\overset{\rightarrow}{\frac{\partial}{\partial}}}
\frac{\partial y^{\gi 2}}{\partial x^{\gi 3}}=\SP 01-\SP 10-\SP 23-\SP 32
\end{matrix}
\right.
\end{equation}
\begin{equation}
\EqLabel{quaternion over real field, derivative, 1, 2}
\left\{
\begin{matrix}
\displaystyle
\frac{\partial y^{\gi 2}}{\partial x^{\gi 0}}=\SP 02-\SP 13+\SP 20+\SP 31
\\
\displaystyle
\vphantom{\overset{\rightarrow}{\frac{\partial}{\partial}}}
\frac{\partial y^{\gi 3}}{\partial x^{\giA}}=\SP 02-\SP 13-\SP 20-\SP 31
\\
\displaystyle
\vphantom{\overset{\rightarrow}{\frac{\partial}{\partial}}}
\frac{\partial y^{\gi 0}}{\partial x^{\gi 2}}=-\SP 02-\SP 13-\SP 20+\SP 31
\\
\displaystyle
\vphantom{\overset{\rightarrow}{\frac{\partial}{\partial}}}
\frac{\partial y^{\giA}}{\partial x^{\gi 3}}=-\SP 02-\SP 13+\SP 20-\SP 31
\end{matrix}
\right.
\end{equation}
\begin{equation}
\EqLabel{quaternion over real field, derivative, 1, 3}
\left\{
\begin{matrix}
\displaystyle
\FP 30=\SP 03+\SP 12-\SP 21+\SP 30
\\
\displaystyle
\vphantom{\overset{\rightarrow}{\frac{\partial}{\partial}}}
\FP 21=-\SP 03-\SP 12-\SP 21+\SP 30
\\
\displaystyle
\vphantom{\overset{\rightarrow}{\frac{\partial}{\partial}}}
\FP 12=\SP 03-\SP 12-\SP 21-\SP 30
\\
\displaystyle
\vphantom{\overset{\rightarrow}{\frac{\partial}{\partial}}}
\FP 03=-\SP 03+\SP 12-\SP 21-\SP 30
\end{matrix}
\right.
\end{equation}
\begin{equation}
\EqLabel{quaternion over real field, derivative, 2, 0}
\left\{
\begin{matrix}
\displaystyle
4\SP 00=\frac{\partial y^{\gi 0}}{\partial x^{\gi 0}}+\frac{\partial y^{\giA}}{\partial x^{\giA}}+\frac{\partial y^{\gi 2}}{\partial x^{\gi 2}}+\frac{\partial y^{\gi 3}}{\partial x^{\gi 3}}
\\
\displaystyle
\vphantom{\overset{\rightarrow}{\frac{\partial}{\partial}}}
4\SP 11=-\frac{\partial y^{\gi 0}}{\partial x^{\gi 0}}-\frac{\partial y^{\giA}}{\partial x^{\giA}}+\frac{\partial y^{\gi 2}}{\partial x^{\gi 2}}+\frac{\partial y^{\gi 3}}{\partial x^{\gi 3}}
\\
\displaystyle
\vphantom{\overset{\rightarrow}{\frac{\partial}{\partial}}}
4\SP 22=-\frac{\partial y^{\gi 0}}{\partial x^{\gi 0}}+\frac{\partial y^{\giA}}{\partial x^{\giA}}-\frac{\partial y^{\gi 2}}{\partial x^{\gi 2}}+\frac{\partial y^{\gi 3}}{\partial x^{\gi 3}}
\\
\displaystyle
\vphantom{\overset{\rightarrow}{\frac{\partial}{\partial}}}
4\SP 33=-\frac{\partial y^{\gi 0}}{\partial x^{\gi 0}}+\frac{\partial y^{\giA}}{\partial x^{\giA}}+\frac{\partial y^{\gi 2}}{\partial x^{\gi 2}}-\frac{\partial y^{\gi 3}}{\partial x^{\gi 3}}
\end{matrix}
\right.
\end{equation}
\begin{equation}
\EqLabel{quaternion over real field, derivative, 2, 1}
\left\{
\begin{matrix}
\displaystyle
4\SP 10=-\frac{\partial y^{\gi 0}}{\partial x^{\giA}}+\frac{\partial y^{\giA}}{\partial x^{\gi 0}}-\frac{\partial y^{\gi 2}}{\partial x^{\gi 3}}+\frac{\partial y^{\gi 3}}{\partial x^{\gi 2}}
\\
\displaystyle
\vphantom{\overset{\rightarrow}{\frac{\partial}{\partial}}}
4\SP 01=-\frac{\partial y^{\gi 0}}{\partial x^{\giA}}+\frac{\partial y^{\giA}}{\partial x^{\gi 0}}+\frac{\partial y^{\gi 2}}{\partial x^{\gi 3}}-\frac{\partial y^{\gi 3}}{\partial x^{\gi 2}}
\\
\displaystyle
\vphantom{\overset{\rightarrow}{\frac{\partial}{\partial}}}
4\SP 32=-\frac{\partial y^{\gi 0}}{\partial x^{\giA}}-\frac{\partial y^{\giA}}{\partial x^{\gi 0}}-\frac{\partial y^{\gi 2}}{\partial x^{\gi 3}}-\frac{\partial y^{\gi 3}}{\partial x^{\gi 2}}
\\
\displaystyle
\vphantom{\overset{\rightarrow}{\frac{\partial}{\partial}}}
4\SP 23=\frac{\partial y^{\gi 0}}{\partial x^{\giA}}+\frac{\partial y^{\giA}}{\partial x^{\gi 0}}-\frac{\partial y^{\gi 2}}{\partial x^{\gi 3}}-\frac{\partial y^{\gi 3}}{\partial x^{\gi 2}}
\end{matrix}
\right.
\end{equation}
\begin{equation}
\EqLabel{quaternion over real field, derivative, 2, 2}
\left\{
\begin{matrix}
\displaystyle
4\SP 20=-\frac{\partial y^{\gi 0}}{\partial x^{\gi 2}}+\frac{\partial y^{\giA}}{\partial x^{\gi 3}}+\frac{\partial y^{\gi 2}}{\partial x^{\gi 0}}-\frac{\partial y^{\gi 3}}{\partial x^{\giA}}
\\
\displaystyle
\vphantom{\overset{\rightarrow}{\frac{\partial}{\partial}}}
4\SP 31=+\frac{\partial y^{\gi 0}}{\partial x^{\gi 2}}-\frac{\partial y^{\giA}}{\partial x^{\gi 3}}+\frac{\partial y^{\gi 2}}{\partial x^{\gi 0}}-\frac{\partial y^{\gi 3}}{\partial x^{\giA}}
\\
\displaystyle
\vphantom{\overset{\rightarrow}{\frac{\partial}{\partial}}}
4\SP 02=-\frac{\partial y^{\gi 0}}{\partial x^{\gi 2}}-\frac{\partial y^{\giA}}{\partial x^{\gi 3}}+\frac{\partial y^{\gi 2}}{\partial x^{\gi 0}}+\frac{\partial y^{\gi 3}}{\partial x^{\giA}}
\\
\displaystyle
\vphantom{\overset{\rightarrow}{\frac{\partial}{\partial}}}
4\SP 13=-\frac{\partial y^{\gi 0}}{\partial x^{\gi 2}}-\frac{\partial y^{\giA}}{\partial x^{\gi 3}}-\frac{\partial y^{\gi 2}}{\partial x^{\gi 0}}-\frac{\partial y^{\gi 3}}{\partial x^{\giA}}
\end{matrix}
\right.
\end{equation}
\begin{equation}
\EqLabel{quaternion over real field, derivative, 2, 3}
\left\{
\begin{matrix}
\displaystyle
4\SP 30=-\FP 03-\FP 12+\FP 21+\FP 30
\\
\displaystyle
\vphantom{\overset{\rightarrow}{\frac{\partial}{\partial}}}
4\SP 21=-\FP 03-\FP 12-\FP 21-\FP 30
\\
\displaystyle
\vphantom{\overset{\rightarrow}{\frac{\partial}{\partial}}}
4\SP 12=\FP 03-\FP 12-\FP 21+\FP 30
\\
\displaystyle
\vphantom{\overset{\rightarrow}{\frac{\partial}{\partial}}}
4\SP 03=-\FP 03+\FP 12-\FP 21+\FP 30
\end{matrix}
\right.
\end{equation}
}
{quaternion over real field, derivative}

\DefEquation
{
\ePrints{0812.4763,0908.3307}
\ifx\Semafor\ValueOn
\partial (\overline x)(h)=-\frac 12(h+ihi+jhj+khk)
\else
\begin{array}{r@{\ }l}
\partial \overline x&\displaystyle=-\frac 12(1\otimes 1+i\otimes i+j\otimes j+k\otimes k)
\\
\VirtFrac
\partial \overline x\circ dx&\displaystyle=-\frac 12(dx+i\ dx\ i+j\ dx\ j+k\ dx\ k)
\\[6pt]
&=\overline {dx}
\end{array}
\fi
}
{quaternion conjugation, derivative}

\DefEq
{
\begin{equation}
\begin{array}{r@{}l}
&
\JacobianA
\\
=&
\MatrixAB
\JacobianB
\end{array}
\EqLabel{Jacobian, B->A}
\end{equation}
\begin{equation}
\begin{array}{r@{}l}
&
\JacobianB
\\
=&
\displaystyle
\MatrixBA
\JacobianA
\end{array}
\EqLabel{Jacobian, A->B}
\end{equation}
}
{quaternion over real field, Jacobian matrix}

\def\NormX{x\overline {dx}+\overline x dx}

\DefEq
{
\begin{align}
\partial (|x|^2)\circ dx=\NormX
\EqLabel{norm2 of quaternion, derivative}
\ePrints{0812.4763}
\ifx\Semafor\ValueOn
\\
\partial (|x|)(h)=\frac 1{2\sqrt{\NormX}}
\EqLabel{norm of quaternion, derivative}
\fi
\end{align}
}
{norm of quaternion, derivative}



==> Quaternion.Russian.tex <==
%auto-ignore
\ePrints{1003.1544,8433-5163}
\Items{Calculus.Paper}
\ifx\Semafor\ValueOn
\Chapter{Алгебра с делением}
\ePrints{Calculus.Paper}
\ifx\Semafor\ValueOn
В этом разделе мы рассмотрим равенства, которые следуют из теоремы
\ref{theorem: Gateaux differential and jacobian, algebra}.
Мы рассмотрим
поля комплексных чисел, алгебру кватернионов и алгебру октонионов.
Хотя в разделе \ref{chapter: Differentiable maps}
мы изучали дифференцируемые отображения в ассоциативную алгебру,
однако, как было отмечено в разделе
\ref{Section: Linear Map into Nonassociative Algebra},
равенства, которые мы записываем в неассоциативной алгебре,
незначительно отличаются от равенств, которые мы записываем в ассоциативной алгебре.
\fi%Calculus.Paper
\else%1003.1544,8433-5163,Calculus.Paper
\Chapter{Алгебра кватернионов}
\label{chapter: Quaternion Algebra}
\fi%1003.1544,8433-5163,Calculus.Paper

\input{\FilePrefix Complex.Number.Russian}

\input{\FilePrefix Quaternion.Eq}

\ePrints{Calculus.Paper}
\ifx\Semafor\ValueOff
\Section{Линейная функция алгебры кватернионов}

\begin{theorem}
\label{theorem: Quaternion over real field}
Положим
\ShowEq{basis of quaternion}
базис алгебры кватернионов $H$.
Тогда в базисе \EqRef{basis of quaternion} структурные константы имеют вид
\ShowEq{structural constants, quaternion}
\end{theorem}
\begin{proof}
Значение структурных констант следует из таблицы умножения
\EqRef{product of quaternions}.
\end{proof}

Так как вычисления в этом разделе занимают много места,
я собрал в одном месте ссылки на теоремы в этом разделе.
\begin{description}
\item [Теорема \ref{theorem: Standard components of linear function, quaternion},
страница \pageref{theorem: Standard components of linear function, quaternion}]
определение координат линейного отображения
алгебры кватернионов $H$
через стандартные компоненты этого отображения.
\item [Равенство \EqRef{quaternion, 3, B->A},
страница \pageref{eq: quaternion, 3, B->A}]
матричная форма зависимости координат линейного отображения
алгебры кватернионов $H$
от стандартных компонент этого отображения.
\item [Равенство \EqRef{quaternion, 3, A->B},
страница \pageref{eq: quaternion, 3, A->B}]
матричная форма зависимости стандартных компонент линейного отображения
алгебры кватернионов $H$
от координат этого отображения.
\item [Теорема \ref{theorem: coordinates of linear function, quaternion},
страница \pageref{theorem: coordinates of linear function, quaternion}]
зависимость стандартных компонент линейного отображения
алгебры кватернионов $H$
от координат этого отображения.
\ePrints{0812.4763}
\ifx\Semafor\ValueOff
\item [Равенство \EqRef{quaternion conjugation},
страница \pageref{eq: quaternion conjugation}]
сопряжения кватернионов - линейное отображение
\fi
\end{description}

\begin{theorem}
\label{theorem: Standard components of linear function, quaternion}
Стандартные компоненты линейной функции
алгебры кватернионов $H$ относительно базиса
\EqRef{basis of quaternion}
и координаты соответствующего линейного преобразования
удовлетворяют соотношениям
\ShowEq{quaternion linear system, 1}
\end{theorem}
\begin{proof}
Пользуясь равенством
\ePrints{1003.1544,8433-5163}
\ifx\Semafor\ValueOn
\EqRef{coordinates of map A}
\else%1003.1544,8433-5163
\EqRef{linear map over field, division ring, relation}
\fi%1003.1544,8433-5163
получаем соотношения
\ShowEq{Standard components of linear function, 1, quaternion}

Уравнения
\ShowEq{quaternion linear system ref, 0}
формируют систему линейных уравнений
\EqRef{quaternion linear system, 1, 0}.

Уравнения
\ShowEq{quaternion linear system ref, 1}
формируют систему линейных уравнений
\EqRef{quaternion linear system, 1, 1}.

Уравнения
\ShowEq{quaternion linear system ref, 2}
формируют систему линейных уравнений
\EqRef{quaternion linear system, 1, 2}.

Уравнения
\ShowEq{quaternion linear system ref, 3}
формируют систему линейных уравнений
\EqRef{quaternion linear system, 1, 3}.
\end{proof}

\begin{theorem}
\label{theorem: Quaternion over real field, matrix}
Рассмотрим алгебру кватернионов $H$ с базисом
\EqRef{basis of quaternion}.
Стандартные компоненты линейной функции над полем $F$
и координаты этой функции над полем $F$
удовлетворяют соотношениям
\ShowEq{quaternion, 3}
где
\ShowEq{quaternion, 3, 1}
\end{theorem}
\begin{proof}
\ePrints{Calculus.Paper}
\ifx\Semafor\ValueOn
Утверждение теоремы является следствием теорем
\ref{theorem: coordinates of map A1 A2, algebra},
\ref{theorem: Quaternion over real field}.
\else
Запишем систему линейных уравнений
\EqRef{quaternion linear system, 1, 0}
в виде произведения матриц
\ShowEq{quaternion matrix 0}
Запишем систему линейных уравнений
\EqRef{quaternion linear system, 1, 1}
в виде произведения матриц
\ShowEq{quaternion matrix 1}
Из равенства \EqRef{quaternion matrix 1}
следует
\ShowEq{quaternion over real field, 3, 1}
Запишем систему линейных уравнений
\EqRef{quaternion linear system, 1, 2}
в виде произведения матриц
\ShowEq{quaternion matrix 2}
Из равенства \EqRef{quaternion matrix 2}
следует
\ShowEq{quaternion over real field, 3, 2}
Запишем систему линейных уравнений
\EqRef{quaternion linear system, 1, 3}
в виде произведения матриц
\ShowEq{quaternion matrix 3}
Из равенства \EqRef{quaternion matrix 3}
следует
\ShowEq{quaternion over real field, 3, 3}
Мы объединяем равенства
\EqRef{quaternion matrix 0},
\EqRef{quaternion over real field, 3, 1},
\EqRef{quaternion over real field, 3, 2},
\EqRef{quaternion over real field, 3, 3}
в равенстве
\EqRef{quaternion, 3, B->A}.
\fi
\end{proof}

\begin{theorem}
\label{theorem: coordinates of linear function, quaternion}
Стандартные компоненты линейной функции
алгебры кватернионов $H$ относительно базиса
\EqRef{basis of quaternion}
и координаты соответствующего линейного преобразования
удовлетворяют соотношениям
\ShowEq{quaternion over real field}
\end{theorem}
\begin{proof}
Системы линейных уравнений
\EqRef{quaternion over real field, 2, 0},
\EqRef{quaternion over real field, 2, 1},
\EqRef{quaternion over real field, 2, 2},
\EqRef{quaternion over real field, 2, 3}
получены
в результате перемножения матриц в равенстве
\EqRef{quaternion, 3, A->B}.
\end{proof}

\ePrints{0812.4763}
\ifx\Semafor\ValueOff
\begin{theorem}
\label{theorem: quaternion conjugation}
Сопряжение кватернионов удовлетворяет равенству
\ShowEq{quaternion conjugation}
\end{theorem}
\begin{proof}
Сопряжение кватернионов является линейным отображением с матрицей
\ShowEq{quaternion conjugation, matrix}
Утверждение теоремы следует из равенства
\EqRef{quaternion, 3, A->B}
и утверждения \eqref{f in L(A,A), 2, associative algebra}
теоремы \ref{theorem: linear map in L(A,A), associative algebra}.
\end{proof}
\fi
\fi%Calculus.Paper

\ePrints{0812.4763,0908.3307}
\Items{Calculus.Paper}
\ifx\Semafor\ValueOn
\ePrints{0812.4763,0908.3307}
\ifx\Semafor\ValueOn
\Section{Дифференцируемое отображение тела кватернионов}
\label{section: Differentiable Map of Division Ring of Quaternions}
\fi

\begin{theorem}
\ePrints{Calculus.Paper}
\ifx\Semafor\ValueOn
Рассмотрим алгебру кватернионов $H$ с базисом
\ShowEq{basis of quaternion}
\fi
Если матрица
$\displaystyle
\begin{pmatrix}
\displaystyle\frac{\partial y^{\gi i}}{\partial x^{\gi j}}
\end{pmatrix}
$
является матрица Якоби функции
$
x\rightarrow y
$
тела кватернионов над полем действительных чисел,
то
\ePrints{0812.4763,0908.3307}
\ifx\Semafor\ValueOn
\ShowEq{quaternion over real field, derivative}
\else
\ShowEq{quaternion over real field, Jacobian matrix}
\fi
\end{theorem}
\begin{proof}
Следствие теоремы
\ePrints{0812.4763,0908.3307}
\ifx\Semafor\ValueOn
\ref{theorem: Standard components of linear function, quaternion}.
\else%0812.4763,0908.3307
\ePrints{Calculus.Paper}
\ifx\Semafor\ValueOn
\xRef{8433-5163}{theorem: Quaternion over real field, matrix}.
\else%Calculus.Paper
\ref{theorem: Quaternion over real field, matrix}.
\fi%Calculus.Paper
\fi%0812.4763,0908.3307
\end{proof}

\begin{theorem}
\label{theorem: quaternion conjugation, derivative}
Отображение кватернионов
\[
f(x)=\overline x
\]
имеет производную Гато
\ShowEq{quaternion conjugation, derivative}
\end{theorem}
\begin{proof}
\ePrints{0812.4763,0908.3307}
\ifx\Semafor\ValueOn
Матрица Якоби отображения $f$ имеет вид
\ShowEq{quaternion conjugation, matrix}
Из равенств
\EqRef{quaternion over real field, derivative, 2, 0}
следует
\begin{equation}
\EqLabel{quaternion conjugation, derivative, 1}
\SP 00=
\SP 11=
\SP 22=
\SP 33=
-\frac 12
\end{equation}
Из равенств
\EqRef{quaternion over real field, derivative, 2, 1},
\EqRef{quaternion over real field, derivative, 2, 2},
\EqRef{quaternion over real field, derivative, 2, 3}
следует
\begin{equation}
\EqLabel{quaternion conjugation, derivative, 2}
\SP ij=0
\ \ \ \gi i\ne\gi j
\end{equation}
Равенство
\EqRef{quaternion conjugation, derivative}
следует из равенств
\EqRef{Gateaux derivative, division ring, standard representation},
\EqRef{quaternion conjugation, derivative, 1},
\EqRef{quaternion conjugation, derivative, 2}.
\else
\ePrints{Calculus.Paper}
\ifx\Semafor\ValueOn
Матрица Якоби отображения $f$ имеет вид
\ShowEq{quaternion conjugation, matrix}
Утверждение теоремы следует из равенств
\EqRef{Gateaux derivative, algebra, standard representation},
\EqRef{Jacobian, A->B},\EqRef{quaternion conjugation, matrix}.
\else%Calculus.Paper
Следствие теорем
\ref{theorem: Gateaux derivative of linear map},
\ref{theorem: quaternion conjugation}.
\fi%Calculus.Paper
\fi
\end{proof}

\begin{theorem}
Норма кватерниона удовлетворяет равенствам\footnote{Утверждение
теоремы аналогично примеру X,
\citeBib{Hamilton Elements of Quaternions 1}, с. 455.}
\ShowEq{norm of quaternion, derivative}
\end{theorem}
\begin{proof}
Равенство
\EqRef{norm2 of quaternion, derivative} следует из
\ePrints{0812.4763}
\ifx\Semafor\ValueOff
равенств
\EqRef{Gateaux derivative, fg, algebra},
\EqRef{Gateaux derivative, fx=axb, algebra},
\EqRef{norm of quaternion},
\EqRef{quaternion conjugation, derivative}.
\else
теоремы
\ref{theorem: quaternion conjugation, derivative}
и равенств
\EqRef{norm of quaternion},
\EqRef{Gateaux derivative of product, division ring}.
Так как $\NormX\in R$,
то равенство
\EqRef{norm of quaternion, derivative}
следует из равенства
\EqRef{norm2 of quaternion, derivative}.
\fi
\end{proof}
\fi

\ePrints{0812.4763}
\begin{theorem}
В теле кватернионов над полем действительных чисел $H$
с базисом
\EqRef{basis of quaternion}
стандартное \Ds представление дифференциала Гато отображения $x^2$
имеет вид
\[
\partial x^2(a)=(x+x_1)a+x_2ai+x_3aj+x_4ak
\]
\end{theorem}
\begin{proof}
Следствие определения
\ref{definition: Gateaux Dstar derivative, division ring}.
\end{proof}

\ifx\Semafor\ValueOn
\fi

\ePrints{1003.1544,8433-5163}
\Items{Calculus.Paper}
\ifx\Semafor\ValueOff
\begin{theorem}
Мы можем отождествить кватернион
\ShowEq{quaternion a}
и матрицу
\ShowEq{quaternion product ax, Jacobian}
\end{theorem}
\begin{proof}
Произведение кватернионов
\EqRef{quaternion a} и
\ShowEq{quaternion x}
имеет вид
\ShowEq{quaternion product ax}
Следовательно, функция $f_a(x)=ax$ имеет матрицу Якоби
\EqRef{quaternion product ax, Jacobian}.
Очевидно, что $f_a\circ f_b=f_{ab}$. Аналогичное равенство
верно для матриц
\ShowEq{quaternion ab, Jacobian product}
Следовательно, мы можем отождествить кватернион $a$ и матрицу $J_a$.
\end{proof}
\fi


==> Ring.Linear.Map.English.tex <==
%auto-ignore
\input{Ring.Linear.Map.Eq}

\ifx\PrintBook\undefined
\else
\chapter{Linear Map of Division Ring}
\label{chapter: Linear map, Division Ring}
\fi

\section{Linear Map of Division Ring}
\label{section: linear map of division ring}

According to the remark
\xRef{0701.238}{remark: Geometry of Division Ring over Field},
we consider division ring $D$ as algebra over field \FZD.

\begin{definition}
\label{definition: linear map of division ring}
Let $D_1$, $D_2$ be division rings.
Let $F$ be field such that
\ShowEq{field division ring d1 d2}
Linear map
\ShowEq{f d1 d2}
of $F$\Hyph vector space $D_1$
into $F$\Hyph vector space $D_2$
is called
\AddIndex{linear map of division ring $D_1$
into division ring $D_2$}{linear map of division ring}.
\qed
\end{definition} 

According to definition \ref{definition: linear map of division ring},
linear map $f$ of division ring $D_1$ into division ring $D_2$
holds
\ShowEq{linear map of division ring}

\begin{theorem}
\label{theorem: linear map, division ring, integer}
Let map
\ShowEq{f d1 d2}
is linear map of division ring $D_1$ of characteristic $0$
into division ring $D_2$ of characteristic $0$.
Then\footnote{Let
\ShowEq{f d1 d2}
be a linear map of division ring $D_1$  of characteristic $2$
into division ring $D_2$  of characteristic $3$.
Then for any $a\in D_1$, $2a=0$, although $2 f(a)\ne 0$.
Therefore, if we assume that characteristic of division ring $D_1$ is
greater than $0$, then must demand that characteristic of division ring $D_1$
equal to characteristic of division ring $D_2$.}
\[
f(nx)=nf(x)
\]
for any integer $n$.
\end{theorem}
\begin{proof}
We prove the theorem by induction on $n$.
Statement is obvious for $n=1$ because
\[
f(1x)=f(x)=1f(x)
\]
Let statement is true for $n=k$. Then
\[
f((k+1)x)=f(kx+x)=f(kx)+f(x)=kf(x)+f(x)=(k+1)f(x)
\]
\end{proof}

\begin{theorem}
\label{theorem: linear map, division ring, rational}
Let map
\ShowEq{f d1 d2}
be linear map of division ring $D_1$ of characteristic $0$
into division ring $D_2$ of characteristic $0$.
Then
\[
f(ax)=af(x)
\]
for any rational $a$.
\end{theorem}
\begin{proof}
Let $a=\frac pq$.
Assume $y=\frac 1qx$. Then
according to the theorem \ref{theorem: linear map, division ring, integer}
\begin{equation}
f(x)=f(qy)=qf(y)=qf\left(\frac 1qx\right)
\EqLabel{additive map, division ring, rational, 1}
\end{equation}
From equation \EqRef{additive map, division ring, rational, 1}
it follows
\begin{equation}
\frac 1qf(x)=f\left(\frac 1qx\right)
\EqLabel{additive map, division ring, rational, 2}
\end{equation}
From equation \EqRef{additive map, division ring, rational, 2}
it follows
\[
f\left(\frac pqx\right)=pf\left(\frac 1qx\right)=\frac pqf(x)
\]
\end{proof}

We cannot extend the statement of theorem
\ref{theorem: linear map, division ring, rational}
for arbitrary subfield of center $Z(D)$ of division ring $D$.

\begin{theorem}
\label{theorem: exists linear map not linear over center, division ring}
Let division ring $D$ is algebra over field \FZD.
If $F\ne Z(D)$, then there exists linear map
\ShowEq{f D D}
which is not linear over field $Z(D)$.
\end{theorem}
\begin{proof}
To prove the theorem it is enough to consider the complex field
$C$ because $C=Z(C)$.
Because the complex field is algebra over real field,
then the function
\[
z\rightarrow \overline z
\]
is linear. However the equation
\[
\overline{az}=a\overline z
\]
is not true.
\end{proof}

Based on theorem
\ref{theorem: exists linear map not linear over center, division ring},
the question arises.
Why do we consider linear maps over field $F\ne Z(D)$,
if this leads us to sharp expansion of the set of linear maps?
The answer to this question is a rich experience
of the theory of complex function.

\begin{theorem}
\label{theorem: sum of linear maps, division ring}
Let maps
\ShowEq{f d1 d2}
\ShowEq{g d1 d2}
be linear maps of division ring $D_1$
into division ring $D_2$.
Then map $f+g$ is linear.
\end{theorem}
\begin{proof}
Statement of theorem follows from chain of equations
\ShowEq{sum of linear maps, division ring}
\end{proof}

\begin{theorem}
\label{theorem: linear map times constant, division ring}
Let map \ShowEq{f d1 d2}
be linear map of division ring $D_1$
into division ring $D_2$.
Then maps $af$, $fb$, $a$, $b\in R_2$ are linear.
\end{theorem}
\begin{proof}
Statement of theorem follows from chain of equations
\ShowEq{linear map times constant, division ring}
\end{proof}

\begin{definition}
Denote
\ShowEq{set linear maps, division ring}
set of linear maps
\ShowEq{f d1 d2}
of division ring $D_1$ into division ring $D_2$.
\qed
\end{definition}

\begin{theorem}
\label{theorem: linear map, division ring, morphism}
We may represent linear map
\ShowEq{f d1 d2}
of division ring $D_1$ into division ring $D_2$ as
\ShowEq{linear map, division ring, morphism}
where $(G_{k}, k\in K)$ is set of additive maps of
division ring $D_1$ into division ring $D_2$.\footnote{Here
and in the following text we assume
sum over index that is used in product few times.
Equation \EqRef{linear map, division ring, morphism}
is recursive definition and there is hope that it is possible
to simplify it.}
Expression
\ShowEq{component of linear map, division ring}
in equation \EqRef{linear map, division ring, morphism}
is called
\AddIndex{component of linear map}{component of linear map} $f$.
\end{theorem}
\begin{proof}
The statement of theorem follows from theorems
\ref{theorem: sum of linear maps, division ring} and
\ref{theorem: linear map times constant, division ring}. 
\end{proof}

If in the theorem
\ref{theorem: linear map, division ring, morphism}
$|K|=1$,
then the equation
\EqRef{linear map, division ring, morphism}
has form
\ShowEq{linear map, division ring, morphism G}
and map $f$ is called
\AddIndex{linear map generated by map}
{linear map generated by map} $G$.
Map $G$ is called
\AddIndex{generator of linear map}
{generator of linear map}.

\begin{theorem}
\label{theorem: linear map based G, standard form, division ring}
Let $D_1$, $D_2$ be division rings of characteristic $0$.
Let $F$, $F\subset Z(D_1)$, $F\subset Z(D_2)$, be field.
Let $G$ be linear map.
Let $\Basis e$ be basis of division ring $D_2$ over field $F$.
\AddIndex{Standard representation of linear map}
{linear map, standard representation}
\EqRef{linear map, division ring, morphism G}
has form\footnote{Representation of linear map of of division ring using
components of linear map
is ambiguous. We can increase or decrease number of summands
using algebraic operations.
Since dimension of division ring $D_2$ over field $F$ is finite, standard representation
of linear map guarantees finiteness of set
of items in the representation of map.}
\ShowEq{linear map, division ring, G, standard representation}
Expression
$\ShowSymbol{standard component of linear map, G}$
in equation \EqRef{linear map, division ring, G, standard representation}
is called
\AddIndex{standard component of linear map}
{standard component of linear map} $f$.
\end{theorem}
\begin{proof}
Components of linear map $f$
have expansion
\ShowEq{linear map, division ring, components extention}
relative to basis $\Basis e$.
If we substitute \EqRef{linear map, division ring, components extention}
into \EqRef{linear map, division ring, morphism G},
we get
\ShowEq{linear map, division ring, G, standard representation, 1}
If we substitute expression
\ShowEq{linear map, division ring, G, standard representation, 2}
into equation \EqRef{linear map, division ring, G, standard representation, 1}
we get equation \EqRef{linear map, division ring, G, standard representation}.
\end{proof}

\begin{theorem}
\label{theorem: linear map, G, coordinates and components, division ring}
Let $D_1$, $D_2$ be division rings of characteristic $0$.
Let $F$, $F\subset Z(D_1)$, $F\subset Z(D_2)$, be field
Let $G$ be linear map.
Let $\Basis e_1$ be basis of division ring $D_1$ over field $F$.
Let $\Basis e_2$ be basis of division ring $D_2$ over field $F$.
Let
\ShowEq{structural constants, division ring D2}
be structural constants of division ring $D_2$.
Then it is possible to represent linear map
\EqRef{linear map, division ring, morphism G}
generated by linear map $G$
as
\ShowEq{linear map, G, coordinates and components, division ring}
\end{theorem}
\begin{proof}
Consider map
\ShowEq{linear map D1 D2 generator}
According to the theorem \xRef{0701.238}{theorem: linear map of rcd vector space},
linear map $f(a)$ relative to bases $\Basis e_1$ and $\Basis e_2$
has form
\EqRef{linear map, G, coordinates and components, division ring}.
From equations \EqRef{linear map, division ring, G, standard representation}
and \EqRef{linear map D1 D2 generator},
it follows
\ShowEq{division ring, F linear map G, standard representation}
From equations \EqRef{linear map, G, coordinates and components, division ring}
and \EqRef{division ring, F linear map G, standard representation},
it follows
\ShowEq{linear map, G, coordinates and components, division ring, 1}
Since vectors $e_{2.\gi r}$ are linear independent over field $F$
and values $a^{\gik}$ are arbitrary, then
equation \EqRef{linear map, G, coordinates and components, division ring, relation}
follows from equation
\EqRef{linear map, G, coordinates and components, division ring, 1}.
\end{proof}

Considering map
\ShowEq{linear map, division ring}
we assume $G(x)=x$.

\begin{theorem}
\label{theorem: linear map, division ring, canonical morphism}
Let $D$ be division ring of characteristic $0$.
Linear map
\EqRef{linear map, division ring}
has form
\ShowEq{linear map, division ring, canonical morphism}
\end{theorem}

\begin{theorem}
\label{theorem: linear map, standard form, division ring}
Let $D$ be division ring of characteristic $0$.
Let $\Basis e$ be the basis of division ring $D$ over field $F\subset Z(D)$.
Standard representation of linear map
\EqRef{linear map, division ring, canonical morphism}
of division ring
has form
\ShowEq{linear map, division ring, standard representation}
\end{theorem}

\begin{theorem}
\label{theorem: linear map over field, division ring}
Let $D$ be division ring of characteristic $0$.
Let $\Basis e$ be basis of division ring $D$ over field $F\subset Z(D)$.
Then it is possible to represent linear map
\EqRef{linear map, division ring}
as
\ShowEq{linear map over field, division ring}
\end{theorem}

\begin{theorem}
\label{theorem: linear map over field, division ring, determinant}
Consider matrix
\ShowEq{linear map over field, division ring, matrix}
whose rows and columns are indexed by 
\ShowEq{linear map over field, division ring, row of matrix}
and
\ShowEq{linear map over field, division ring, column of matrix},
respectively.
If
\ShowEq{linear map over field, division ring, determinant},
then, for given coordinates of linear transformation $f_{\gi i}^{\gi j}$,
the system of linear equations
\EqRef{linear map over field, division ring, relation}
with standard components of this transformation
$f^{\gi{kr}}$ has the unique
solution.
If
\ShowEq{linear map over field, division ring, determinant=0},
then
the equation
\ShowEq{linear map over field, division ring, determinant=0, 1}
is the condition for the existence of solutions
of the system of linear equations
\EqRef{linear map over field, division ring, relation}.
In such case the system of linear equations
\EqRef{linear map over field, division ring, relation}
has infinitely many solutions and there exists linear
dependence between values $f_{\gi i}^{\gi j}$.
\end{theorem}
\begin{proof}
Equation
\EqRef{linear map, division ring, canonical morphism}
is special case of equation
\EqRef{linear map, division ring, morphism G}
when $G(x)=x$.
Theorem
\ref{theorem: linear map, standard form, division ring}
is special case of theorem
\ref{theorem: linear map based G, standard form, division ring}
when $G(x)=x$.
Theorem
\ref{theorem: linear map over field, division ring}
is special case of theorem
\ref{theorem: linear map, G, coordinates and components, division ring}
when $G(x)=x$.
The statement of the theorem
\ref{theorem: linear map over field, division ring, determinant}
is corollary of
the theory of linear equations over field.
\end{proof}

\begin{theorem}
\label{theorem: identity map, division ring}
Standard components of the identity map have the form
\ShowEq{identity map, division ring}
\end{theorem}
\begin{proof}
The equation
\EqRef{identity map, division ring}
is corollary of the equation
\ShowEq{identity map 0, division ring}
Let us show that the standard components
\EqRef{identity map, division ring}
of a linear transformation satisfy to the equation
\ShowEq{identity map 1, division ring}
which follows from the equation
\EqRef{linear map over field, division ring, relation}
if $f=\delta$.
From equations
\EqRef{identity map, division ring},
\EqRef{identity map 1, division ring},
it follows that
\ShowEq{identity map 2, division ring}
The equation
\EqRef{identity map 2, division ring}
is true, because, from equations
\ShowEq{identity map 3, division ring}
it follows that
\ShowEq{identity map 4, division ring}
If
\ShowEq{linear map over field, division ring, determinant},
then the solution
\EqRef{identity map, division ring}
is unique.
If
\ShowEq{linear map over field, division ring, determinant=0},
then the system of linear equations
\EqRef{identity map 1, division ring}
has infinitely many solutions.
However, we are looking for at least one solution.
\end{proof}

\begin{theorem}
\label{theorem: zero map, division ring}
If
\ShowEq{linear map over field, division ring, determinant},
then standard components of the zero map
\ShowEq{zero map, division ring}
are defined uniquely and have form
\ShowEq{zero map, division ring, 1}
If
\ShowEq{linear map over field, division ring, determinant=0},
then the set of standard components of the zero map
forms a vector space.
\end{theorem}
\begin{proof}
The theorem is true because standard components $z^{\gi{ij}}$
are solution of homogeneous system of linear equations
\ShowEq{zero map, division ring, 2}
\end{proof}

\begin{remark}
\label{remark: zero map, division ring}
Consider equation
\ShowEq{linear maps a=b, division ring}
From the theorem \ref{theorem: zero map, division ring},
it follows that only when condition
\ShowEq{linear map over field, division ring, determinant}
is true, from the equation
\EqRef{linear maps a=b, division ring},
it follows that
\ShowEq{linear maps a=b, 1, division ring}
Otherwise, we must assume equality
\ShowEq{linear maps a=b, 2, division ring}
%Это означает, что векторы
%\ShowEq{linear maps a=b, 3, division ring}
%линейно зависимы.
Despite this, in case
\ShowEq{linear map over field, division ring, determinant=0},
we also use standard representation
because in general it is very hard to show the set of linear
independent vectors.
If we want to define operation over linear maps
in standard representation,
then as well as in the case of the theorem
\ref{theorem: identity map, division ring}
we choose one element from the set of possible representations.
\qed
\end{remark}

\begin{theorem}
Expression
\ShowEq{fkr is tensor}
is tensor over field $F$
\begin{equation}
{}_{\gi i}f'^{\gi j}={}_{\gi i}A^{\gik}
\ {}_{\gik}f^{\gil}\ {}_{\gil}A^{-1}{}^{\gi j}
\EqLabel{fkr is tensor, division ring, transformation}
\end{equation}
\end{theorem}
\begin{proof}
$D$\Hyph linear map has form
\EqRef{linear map over field, division ring}
relative to basis $\Basis e$.
Let $\Basis e{}'$ be another basis. Let
\ShowEq{fkr is tensor, division ring, change basis}
be transformation map basis $\Basis e$ to
basis $\Basis e{}'$.
Since linear map $f$ is the same, then
\ShowEq{fkr is tensor, division ring, transformation, 1}
Let us substitute \xEqRef{0701.238}{division ring over field, change basis, 3},
\EqRef{fkr is tensor, division ring, change basis}
into equation \EqRef{fkr is tensor, division ring, transformation, 1}
\ShowEq{fkr is tensor, division ring, transformation, 2}
Because vectors $e_{\gi j}$ are linear independent and
components of vector $x^{\gi i}$ are arbitrary, the equation
\EqRef{fkr is tensor, division ring, transformation}
follows
from equation
\EqRef{fkr is tensor, division ring, transformation, 2}.
Therefore, expression
$f_k^r$
is tensor over field $F$.
\end{proof}

\ePrints{0908.3307}%
\ifx\Semafor\ValueOff%
\begin{definition}
The set
\ShowEq{kernel of linear map, division ring}
is called
\AddIndex{kernel of linear map}{kernel of linear map}
\ShowEq{f d1 d2}
of division ring $D_1$
into division ring $D_2$.
\qed
\end{definition}

\begin{theorem}
Kernel of linear map
\ShowEq{f d1 d2}
is subgroup of additive group of division ring $D_1$.
\end{theorem}
\begin{proof}
Let $a$, $b\in\text{ker}f$. Then
\begin{align*}
f(a)&=0
\\
f(b)&=0
\\
f(a+b)=f(a)+f(b)&=0
\end{align*}
Therefore, $a+b\in\text{ker}f$.
\end{proof}

\begin{definition}
The linear map
\ShowEq{f d1 d2}
of division ring $D_1$
into division ring $D_2$
is called
\AddIndex{singular}{singular linear map},
when
\[\text{ker}f\ne\{0\}\]
\qed
\end{definition}
\fi

\begin{theorem}
\label{theorem: product of linear map, D D D}
Let $D$ be division ring of characteristic $0$.
Let $\Basis e$ be basis of division ring $D$ over center $Z(D)$ of division ring $D$.
Let
\ShowEq{product of additive map, D D D}
be linear maps of division ring $D$.
Map
\begin{equation}
h(x)=gf(x)=g(f(x))
\EqLabel{D linear map, division ring, h1}
\end{equation}
is linear map
\ShowEq{D linear map, division ring, h2}
where
\ShowEq{D linear map, division ring, h gf}
\end{theorem}
\begin{proof}
Map \EqRef{D linear map, division ring, h1}
is linear because
\ShowEq{product of additive map, D D D, 1}

If we substitute
\EqRef{D linear map, division ring, f} and
\EqRef{D linear map, division ring, g} into
\EqRef{D linear map, division ring, h1},
we get
\ShowEq{additive map, division ring, h3}
Comparing \EqRef{additive map, division ring, h3}
and \EqRef{D linear map, division ring, h2},
we get \EqRef{D linear map, division ring, h gf, 0},
\EqRef{D linear map, division ring, h gf, 1}.

If we substitute
\EqRef{D linear map, division ring, standard representation, f} and
\EqRef{D linear map, division ring, standard representation, g} into
\EqRef{D linear map, division ring, h1},
we get
\ShowEq{D linear map, division ring, standard representation, h3}
Comparing \EqRef{D linear map, division ring, standard representation, h3}
and \EqRef{D linear map, division ring, standard representation, h2},
we get \EqRef{D linear map, division ring, standard representation, h gf}.
\end{proof}

\ePrints{0812.4763}
\ifx\Semafor\ValueOn

\begin{definition}
\label{definition: map projective over commutative ring, ring}
Let commutative ring $P$ be subring of center $Z(R)$ of ring $R$.
Map
\[f:R\rightarrow R\]
of ring $R$
is called
\AddIndex{projective over commutative ring}
{map projective over commutative ring} $P$, if
\[
f(px)=f(x)
\]
for any $p\in P$. Set
\[
Px=\{px:p\in P,x\in R\}
\]
is called
\AddIndex{direction $x$ over commutative ring}
{direction over commutative ring}\footnote{Direction
over commutative ring $P$ is subset of ring $R$.
However we denote direction $Px$ by element
$x\in R$ when this does not lead to ambiguity.
We tell about direction over commutative ring $Z(R)$
when we do not show commutative ring $P$ explicitly.} $P$.
\qed
\end{definition}

\begin{example}
\label{example: map projective over commutative ring, ring}
If map $f$
of ring $R$ is linear over commutative ring $P$,
then map
\[
g(x)=x^{-1}f(x)
\]
is projective over commutative ring $P$.
\qed
\end{example}
\fi

\section{Polylinear Map of Division Ring}

\begin{definition}
\label{definition: map polylinear over commutative ring, ring}
Let $R_1$, ..., $R_n$, $P$ be rings of characteristic $0$.
Let $S$ be module over ring $P$.
Let $F$ be commutative ring which is for any $i$ is subring of center
of ring $R_i$.
Map
\[
f:R_1\times...\times R_n\rightarrow
S
\]
is called \AddIndex{polylinear over commutative ring $F$}
{map polylinear over commutative ring, ring},
if
\ShowEq{map polylinear over commutative ring}
for any $i$, $1\le i\le n$, and any $p_i$, $q_i \in R_i$, $b\in F$.
Let us denote
\symb{\mathcal L(R_1,...,R_n;
S)}1{set polylinear maps, ring}
set of polylinear maps
of rings
$R_1$, ..., $R_n$
into module
$S$.
\qed
\end{definition}

\begin{theorem}
\label{theorem: polylinear map, division ring}
Let $D$ be division ring of characteristic $0$.
Polylinear map
\ShowEq{polylinear map, division ring}
has form
\ShowEq{polylinear map, division ring, canonical morphism}
$\sigma_s$ is a transposition of set of variables
$\{d_1,...,d_n\}$
\ShowEq{transposition of set of variables, division ring}
\end{theorem}
\begin{proof}
We prove statement by induction on $n$.

When $n=1$ the statement of theorem is corollary of theorem
\ref{theorem: linear map, division ring, canonical morphism}.
In such case we may identify\footnote{In representation
\EqRef{polylinear map, division ring, canonical morphism}
we will use following rules.
\begin{itemize}
\item If range of any index is set
consisting of one element, then we will omit corresponding
index.
\item If $n=1$, then $\sigma_s$ is identical transformation.
We will not show such transformation in the expression.
\end{itemize}}
\ShowEq{polylinear map, division ring, 1, canonical morphism}

Let statement of theorem be true for $n=k-1$.
Then it is possible to represent map
\EqRef{polylinear map, division ring}
as
\ShowEq{polylinear map, induction on n, 1, division ring}
According to statement of induction pollinear map
$h$ has form
\ShowEq{polylinear map, induction on n, 2, division ring}
According to construction $h=g(d_k)$.
Therefore, expressions $h\pC{t}{p}$
are functions of $d_k$.
Since $g(d_k)$ is linear map of $d_k$,
then only one expression $h\pC{t}{p}$
is linear map of $d_k$, and rest expressions
$\pC{t}{q}h$
do not depend on $d_k$.

Without loss of generality, assume $p=0$.
According to equation
\EqRef{linear map, division ring, canonical morphism}
for given $t$
\ShowEq{polylinear map, induction on n, 3, division ring}
Assume $s=tr$. Let us define transposition $\sigma_s$ according to rule
\ShowEq{polylinear map, induction on n, 4, division ring}
Suppose
\ShowEq{polylinear map, induction on n, 5, division ring}
We proved step of induction.
\end{proof}

\begin{definition}
\begin{sloppypar}
Expression
\ShowEq{component of polylinear map, division ring}
in equation \EqRef{polylinear map, division ring, canonical morphism}
is called
\AddIndex{component of polylinear map}
{component of polylinear map} $f$.
\qed
\end{sloppypar}
\end{definition}

\begin{theorem}
\label{theorem: standard representation of polylinear map, division ring}
Let $D$ be division ring of characteristic $0$.
Let $\Basis e$
be basis in division ring $D$ over field \FZD.
\AddIndex{Standard representation of polylinear map}
{polylinear map, standard representation} of division ring
has form
\ShowEq{polylinear map, division ring, standard representation}
Index $t$ enumerates every possible transpositions
$\sigma_t$ of the set of variables
$\{d_1,...,d_n\}$.
Expression
$\ShowSymbol{standard component of polylinear map}$
in equation \EqRef{polylinear map, division ring, standard representation}
is called
\AddIndex{standard component of polylinear map}
{standard component of polylinear map} $f$.
\end{theorem}
\begin{proof}
Components of polylinear map $f$
have expansion
\ShowEq{polylinear map, division ring, components extention}
relative to basis $\Basis e$.
If we substitute \EqRef{polylinear map, division ring, components extention}
into \EqRef{polylinear map, division ring, canonical morphism},
we get
\ShowEq{polylinear map, division ring, standard representation, 1}
Consider expression
\ShowEq{polylinear map, division ring, standard representation, 2}
The right-hand side is supposed to be the sum of the terms
with the index $s$, for which the transposition $\sigma_s$ is the same.
Each such sum
has a unique index $t$.
If we substitute expression
\EqRef{polylinear map, division ring, standard representation, 2}
into equation \EqRef{polylinear map, division ring, standard representation, 1}
we get equation \EqRef{polylinear map, division ring, standard representation}.
\end{proof}

\begin{theorem}
\label{theorem: polylinear map over field, division ring}
Let $\Basis e$ be basis of division ring $D$ over field \FZD.
Polylinear map
\EqRef{polylinear map, division ring}
can be represented as $D$-valued form of degree $n$
over field \FZD\footnote{We proved the theorem by analogy with
theorem in \citeBib{Rashevsky}, p. 107, 108}
\ShowEq{polylinear map over field, division ring}
where
\ShowEq{polylinear map over field, coordinates, division ring}
and values ${}_{\gi{i_1...i_n}}f$
are coordinates of $D$-valued covariant tensor over field $F$.
\end{theorem}
\begin{proof}
According to the definition
\ref{definition: map polylinear over commutative ring, ring},
the equation
\EqRef{polylinear map over field, division ring}
follows from the chain of equations
\ShowEq{polylinear map over field, 1, division ring}
Let $\Basis e'$ be another basis. Let
\ShowEq{polylinear map over field, division ring, change basis}
be transformation, mapping basis $\Basis e$ into
basis $\Basis e'$.
From equations \EqRef{polylinear map over field, division ring, change basis}
and \EqRef{polylinear map over field, coordinates, division ring}
it follows
\ShowEq{polylinear map over field, division ring, change coordinates}
From equation \EqRef{polylinear map over field, division ring, change coordinates}
the tensor law of transformation of coordinates of polylinear map follows.
From equation \EqRef{polylinear map over field, division ring, change coordinates}
and theorem \xRef{0701.238}{theorem: division ring over field, change basis}
it follows that value of the map $f(a_1,...,a_n)$ does not depend from
choice of basis.
\end{proof}

Polylinear map
\EqRef{polylinear map, division ring}
is \AddIndex{symmetric}
{polylinear map symmetric, division ring}, if
\[
f(d_1,...,d_n)=f(\sigma(d_1),...,\sigma(d_n))
\]
for any transposition $\sigma$ of set $\{d_1,...,d_n\}$.

\begin{theorem}
\label{theorem: polylinear map symmetric, division ring}
If polyadditive map $f$ is symmetric,
then
\ShowEq{polylinear map symmetric, division ring}
\end{theorem}
\begin{proof}
Equation
\EqRef{polylinear map symmetric, division ring}
follows from equation
\ShowEq{polylinear map symmetric, 1, division ring}
\end{proof}

Polylinear map
\EqRef{polylinear map, division ring}
is \AddIndex{skew symmetric}{polylinear map skew symmetric}, if
\[
f(d_1,...,d_n)=|\sigma|f(\sigma(d_1),...,\sigma(d_n))
\]
for any transposition $\sigma$ of set $\{d_1,...,d_n\}$.
Here
\[
|\sigma|=
\left\{
\begin{matrix}
1&\textrm{transposition }\sigma\textrm{ even}
\\
-1&\textrm{transposition }\sigma\textrm{ odd}
\end{matrix}
\right.
\]

\begin{theorem}
\label{theorem: polylinear map skew symmetric, division ring}
If polylinear map $f$ is skew symmetric,
then
\ShowEq{polylinear map skew symmetric, division ring}
\end{theorem}
\begin{proof}
Equation
\EqRef{polylinear map skew symmetric, division ring}
follows from equation
\ShowEq{polylinear map skew symmetric, 1, division ring}
\end{proof}

\begin{theorem}
\label{theorem: coordinates of polylinear map, division ring over field}
Coordinates of the polylinear over field $F$ map
\EqRef{polylinear map, division ring}
and its components relative basis $\Basis e$
satisfy to the equation
\ShowEq{coordinates of polylinear map, division ring over field}
\end{theorem}
\begin{proof}
In equation \EqRef{polylinear map, division ring, standard representation},
we assume
\ShowEq{coordinates of polylinear map, 1, division ring over field}
Then equation \EqRef{polylinear map, division ring, standard representation}
gets form
\ShowEq{polylinear map, division ring, standard representation, 1a}
From equation \EqRef{polylinear map over field, division ring}
it follows that
\ShowEq{polylinear map over field, division ring, 1a}
Equation
\EqRef{coordinates of polylinear map, division ring over field}
follows from comparison of equations
\EqRef{polylinear map, division ring, standard representation, 1a}
and
\EqRef{polylinear map over field, division ring}.
Equation
\EqRef{coordinates of polylinear map, division ring over field, 1}
follows from comparison of equations
\EqRef{polylinear map, division ring, standard representation, 1a}
and
\EqRef{polylinear map over field, division ring, 1a}.
\end{proof}



==> Ring.Linear.Map.Eq.tex <==
%auto-ignore

\def\FZD{$F\subset Z(D)$}

\DefEquation
{
f(x)=f\pC{k\cdot s_k}{0}\ G_k(x)\ f\pC{k\cdot s_k}{1}
}
{linear map, division ring, morphism}

\DefEq
{
\symb{\mathcal L(D_1;D_2)}1{set linear maps, scalar}
}
{set linear maps, division ring}

\DefEq
{
\[
\begin{array}{r@{\ }lc}
f(a+b)&=f(a)+f(b)&a, b\in D
\\
f(pa)&=pf(a)&p\in F
\end{array}
\]
}
{linear map of division ring}

\DefEq
{
\begin{align*}
(af)(x+y)
=&a(f(x+y))
=a(f(x)+f(y))
=af(x)+af(y)
\\
=&(af)(x)+(af)(y)
\\
(af)(px)
=&a(f(px))
=a(pf(x))
=p(af(x))
\\
=&p(af)(x)
\\
(fb)(x+y)
=&(f(x+y))b
=(f(x)+f(y))b
=f(x)b+f(y)b
\\
=&(fb)(x)+(fb)(y)
\\
(fb)(px)
=&(f(px))b
=(pf(x))b
=p(f(x)b)
\\
=&p(fb)(x)
\end{align*}
}
{linear map times constant, division ring}

\DefEq
{
\begin{align*}
(f+g)(x+y)
=&f(x+y)+g(x+y)
=f(x)+f(y)+g(x)+g(y)
\\
=&(f+g)(x)+(f+g)(y)
\\
(f+g)(px)
=&f(px)+g(px)
=pf(x)+pg(x)
=p(f(x)+g(x))
\\
=&p(f+g)(x)
\end{align*}
}
{sum of linear maps, division ring}

\DefEq
{
\[f:D_1\rightarrow D_2\]
}
{f d1 d2}

\DefEq
{
\[g:D_1\rightarrow D_2\]
}
{g d1 d2}

\DefEq
{
$F\subset Z(D_1)$, $F\subset Z(D_2)$.
}
{field division ring d1 d2}

\DefEquation
{
f(x)=f\pC{s}{0}\ G(x)\ f\pC{s}{1}
}
{linear map, division ring, morphism G}

\DefEq
{
\begin{align}
f(a)=&e_{\gi j}f_{\gi i}^{\gi j}a^{\gi i}
&f_{\gik}^{\gi j}&\in F
\EqLabel{linear map over field, division ring}
\\
a=&e_{\gi i}a^{\gi i}&a^{\gi i}&\in F\ \ \ a\in D
\nonumber
\\
f_{\gi i}^{\gi j}=&f^{\gi{kr}}C_{\gi{ki}}^{\gi p}
C_{\gi{pr}}^{\gi j}
\EqLabel{linear map over field, division ring, relation}
\end{align}
}
{linear map over field, division ring}

\DefEquation
{
\mathcal C
=
\left(
\mathcal C^{\cdot}{}_{\gi i}^{\gi j}{}_{\cdot\gi{kr}}
\right)
=\left(
C_{\gi{ki}}^{\gi p}C_{\gi{pr}}^{\gi j}
\right)
}
{linear map over field, division ring, matrix}

\DefEq
{
$\det\mathcal C\ne 0$%
}
{linear map over field, division ring, determinant}

\DefEq
{
$\det\mathcal C=0$%
}
{linear map over field, division ring, determinant=0}

\DefEquation
{
\rank
\begin{pmatrix}
\mathcal C^{\cdot}{}_{\gi i}^{\gi j}{}_{\cdot\gi{kr}}
&f_{\gi i}^{\gi j}
\end{pmatrix}
=\rank\mathcal C
}
{linear map over field, division ring, determinant=0, 1}

\DefEq
{
${}^{\cdot}{}_{\gi i}^{\gi j}$
}
{linear map over field, division ring, row of matrix}

\DefEq
{
$\cdot\gi{kr}$
}
{linear map over field, division ring, column of matrix}

\DefEq
{
\begin{equation}
f^{\gi{kr}}=\delta^{\gik}_{\gi 0}\delta^{\gi r}_{\gi 0}
\EqLabel{identity map, division ring}
\end{equation}
}
{identity map, division ring}

\DefEquation
{
\delta_{\gi i}^{\gi j}=f^{\gi{kr}}C_{\gi{ki}}^{\gi p}
C_{\gi{pr}}^{\gi j}
}
{identity map 1, division ring}

\DefEq
{
\[
z:A\rightarrow A\ \ \ z(x)=0
\]
}
{zero map, division ring}

\DefEq
{
$z^{\gi{ij}}=0$.
}
{zero map, division ring, 1}

\DefEq
{
\[
0=z^{\gi{kr}}C_{\gi{ki}}^{\gi p}
C_{\gi{pr}}^{\gi j}
\]
}
{zero map, division ring, 2}

\DefEq
{
\begin{equation}
a^{\gi{kr}}\ e_{\gik}\ x\ e_{\gi r}
=
b^{\gi{kr}}\ e_{\gik}\ x\ {}e_{\gi r}
\EqLabel{linear maps a=b, division ring}
\end{equation}
}
{linear maps a=b, division ring}

\DefEquation
{
f'{}_{\gi i}^{\gi j}=A_{\gi i}^{\gik}
f_{\gik}^{\gil}A^{-1\cdot}{}_{\gil}^{\gi j}
}
{fkr is tensor, division ring, transformation}

\DefEquation
{
e{}'_{\gi i}=e_{\gi j}A_{\gi i}^{\gi j}
}
{fkr is tensor, division ring, change basis}

\DefEquation
{
f(x)
=e_{\gi j}A_{\gil}^{\gi j}f'{}_{\gik}^{\gil}
A^{-1\cdot}{}_{\gi i}^{\gik}x^{\gi i}
}
{fkr is tensor, division ring, transformation, 2}

\DefEquation
{
f(x)=e{}'_{\gil}f'{}_{\gik}^{\gil}x'^{\gik}
}
{fkr is tensor, division ring, transformation, 1}

\DefEq
{
\[
f_{\gik}^{\gi r}=f^{\gi i\gi j}
C_{\gi{ik}}^{\gi p}C_{\gi{pj}}^{\gi r}
\]
}
{fkr is tensor}

\DefEq
{
$e_{\gik}\ x\ e_{\gi r}$
}
{linear maps a=b, 3, division ring}

\DefEq
{
\begin{equation}
a^{\gi{kr}}
=
b^{\gi{kr}}
\EqLabel{linear maps a=b, 1, division ring}
\end{equation}
}
{linear maps a=b, 1, division ring}

\DefEq
{
\symb{\text{ker}f}
0{kernel of linear map}
\[
\ShowSymbol{kernel of linear map}=\{x\in D_1:f(x)=0\}
\]
}
{kernel of linear map, division ring}

\DefEq
{
\begin{equation}
a^{\gi{kr}}
=
b^{\gi{kr}}
+
z^{\gi{kr}}
\EqLabel{linear maps a=b, 2, division ring}
\end{equation}
}
{linear maps a=b, 2, division ring}

\DefEq
{
$z^{\gi{ij}}=0$.
}
{zero map, division ring, 1}

\DefEquation
{
\delta_{\gi i}^{\gi j}=C_{\gi{0i}}^{\gi p}
C_{\gi{p0}}^{\gi j}
}
{identity map 2, division ring}

\DefEq
{
\[
e_{\gi j}e_{\gi 0}=
e_{\gi 0}\ e_{\gi j}=
e_{\gi j}
\]
}
{identity map 3, division ring}

\DefEq
{
\[
\begin{matrix}
C_{\gi{0r}}^{\gi j}=\delta_{\gi r}^{\gi j}
&
C_{\gi{r0}}^{\gi j}=\delta_{\gi r}^{\gi j}
\end{matrix}
\]
}
{identity map 4, division ring}

\DefEq
{
\[
x=e_{\gi 0}\ x\ e_{\gi 0}
\]
}
{identity map 0, division ring}

\DefEq
{
\begin{align}
f(a)&=e_{2\cdot\gi j}\,f_{\gi i}^{\gi j}a^{\gi i}
&f_{\gik}^{\gi j}&\in F
\EqLabel{linear map, G, coordinates and components, division ring}
\\
a&=e_{1\cdot\gi i}\,a^{\gi i}&a^{\gi i}&\in F\ \ \ a\in D_1
\nonumber
\\
f_{\gi i}^{\gi j}&=G_{\gi i}^{\gil}f^{\gi{kr}}_G C_{2\cdot}^{}{}_{\gi{kl}}^{\gi p}
C_{2\cdot}^{}{}_{\gi{pr}}^{\gi j}
\EqLabel{linear map, G, coordinates and components, division ring, relation}
\end{align}
}
{linear map, G, coordinates and components, division ring}

\DefEq
{
\begin{equation}
f:D\rightarrow D
\EqLabel{linear map, division ring}
\end{equation}
}
{linear map, division ring}

\DefEquation
{
f(x)=f\pC{s}{0}\ x\ f\pC{s}{1}
}
{linear map, division ring, canonical morphism}

\DefEquation
{
f(x)=f\pC{s}{0}^{\gi i}\ e_{\gi i}
\ G(x)\ f\pC{s}{1}^{\gi j}\ e_{\gi j}
}
{linear map, division ring, G, standard representation, 1}

\DefEq
{
\[
f^{\gi{ij}}_G=f\pC{s}{0}^{\gi i}\ f\pC{s}{1}^{\gi j}
\]
}
{linear map, division ring, G, standard representation, 2}

\DefEq
{
$C_{2\cdot}^{}{}_{\gi{kl}}^{\gi p}$
}
{structural constants, division ring D2}

\DefEquation
{
f\pC{s}{p}=f\pC{s}{p}^{\gi i}\ e_{\gi i}
}
{linear map, division ring, components extention}

\DefEquation
{
f(x)=f^{\gi{ij}}
\ e_{\gi i} xe_{\gi j}
}
{linear map, division ring, standard representation}

\DefEq
{
\symb{f^{\gi i\gi j}_G}0
{standard component of linear map, G}
\begin{equation}
f(x)=\ShowSymbol{standard component of linear map, G}
\ e_{\gi i}\ G(x)\ e_{\gi j}
\EqLabel{linear map, division ring, G, standard representation}
\end{equation}
}
{linear map, division ring, G, standard representation}

\DefEquation
{
\begin{matrix}
G:D_1\rightarrow D_2
&
a=e_{1\cdot\gi i}a^{\gi i} \rightarrow G(a)=
e_{2\cdot\gi j}G_{\gi i}^{\gi j}a^{\gi i}
\\
&
a^{\gi i}\in F\ \ \ G_{\gi i}^{\gi j}\in F
\end{matrix}
}
{linear map D1 D2 generator}

\DefEq
{
\symb{f\pC{k\cdot s_k}{p}}1
{component of linear map, division ring}, $p=0$, $1$,
}
{component of linear map, division ring}

\DefEquation
{
f(a)=G_{\gi i}^{\gil}a^{\gi i} f^{\gik\gi j}_G
e_{2\cdot\gik}e_{2\cdot\gil}e_{2\cdot\gi j}
}
{division ring, F linear map G, standard representation}

\DefEquation
{
e_{2\cdot\gi j}\ f_{\gi i}^{\gi j}\ a^{\gi i}
= G_{\gi i}^{\gil}a^{\gi i} f^{\gi{kr}}_G {}e_{2\cdot\gik}
e_{2\cdot\gil} e_{2\cdot\gi r}
=G_{\gi i}^{\gil}a^{\gi i}f^{\gi{kr}}_G C_{2\cdot}^{}{}_{\gi{kl}}^{\gi p}
C_{2\cdot}^{}{}_{\gi{pr}}^{\gi j}\ e_{2\cdot\gi j}
}
{linear map, G, coordinates and components, division ring, 1}

\DefEq
{
\[
h(x+y)=g(f(x+y))=g(f(x)+f(y))=g(f(x))+g(f(y))=h(x)+h(y)
\]
\[
h(ax)=g(f(ax))=g(af(x))=ag(f(x))=ah(x)
\]
}
{product of additive map, D D D, 1}

\DefEq
{
\begin{align}
h(x)=&g^{\gi{ij}}\ e_{\gi i}\ f(x)\ e_{\gi j}
\nonumber
\\
=&g^{\gi{ij}}\ e_{\gi i}\ f^{\gi{kl}}\ e_{\gik}
\ x\ e_{\gil} e_{\gi j}
\EqLabel{D linear map, division ring, standard representation, h3}
\\
=&g^{\gi{ij}} f^{\gi{kl}} C_{\gi{ik}}^{\gi p}
C_{\gi{lj}}^{\gi r}\ e_{\gi p}\ x\ e_{\gi r}
\nonumber
\end{align}
}
{D linear map, division ring, standard representation, h3}

\DefEquation
{
h(x)=g\pC{t}{0}\ f(x)\ g\pC{t}{1}
=g\pC{t}{0}\ f\pC{s}{0}\ x\ f\pC{s}{1}\ g\pC{t}{1}
}
{additive map, division ring, h3}

\DefEq
{
\begin{align}
f:D\rightarrow D\quad
f(x)&=f\pC{s}{0}\ x\ f\pC{s}{1}
\EqLabel{D linear map, division ring, f}
\\
&=f^{\gi{ij}}\ e_{\gi i} x e_{\gi j}
\EqLabel{D linear map, division ring, standard representation, f}
\\
g:D\rightarrow D\quad
g(x)&=g\pC{t}{0}\ x\ g\pC{t}{1}
\EqLabel{D linear map, division ring, g}
\\
&=g^{\gi{ij}}\ e_{\gi i} xe_{\gi j}
\EqLabel{D linear map, division ring, standard representation, g}
\end{align}
}
{product of additive map, D D D}

\DefEq
{
\begin{align}
h\pC{ts}{0}&=g\pC{t}{0}\ f\pC{s}{0}
\EqLabel{D linear map, division ring, h gf, 0}
\\
h\pC{ts}{1}&=f\pC{s}{1}\ g\pC{t}{1}
\EqLabel{D linear map, division ring, h gf, 1}
\\
h^{\gi{pr}}&=g^{\gi{ij}} f^{\gi{kl}}
C_{\gi{ik}}^{\gi p}C_{\gi{lj}}^{\gi r}
\EqLabel{D linear map, division ring, standard representation, h gf}
\end{align}
}
{D linear map, division ring, h gf}

\DefEq
{
\begin{align}
h(x)&=h\pC{ts}{0}\ x\ h\pC{ts}{1}
\EqLabel{D linear map, division ring, h2}
\\
&=h^{\gi{pr}}\ e_{\gi p}\ x\ e_{\gi r}
\EqLabel{D linear map, division ring, standard representation, h2}
\end{align}
}
{D linear map, division ring, h2}

\DefEq
{
\[
f:D\rightarrow D
\]
}
{f D D}

\DefEquation
{
f:D^n\rightarrow D,
d=f(d_1,...,d_n)
}
{polylinear map, division ring}

\DefEquation
{
f(a_1,...,a_n)=a^{\gi{i_1}}_1...a^{\gi{i_n}}_nf_{\gi{i_1...i_n}}
}
{polylinear map over field, division ring}

\DefEq
{
\begin{align*}
f(
p_1, ...,
p_i+ q_i, ...,
p_n)
&=
f(
p_1, ...,
p_i, ...,
p_n)
+
f(
p_1, ...,
q_i, ...,
p_n)
\\
f(a_1, ..., b a_i, ..., a_n)&=bf(a_1, ..., a_i, ..., a_n)
\end{align*}
}
{map polylinear over commutative ring}

\DefEquation
{
e'_{\gi i}=e_{\gi j}A_{\gi i}^{\gi j}
}
{polylinear map over field, division ring, change basis}

\DefEq
{
\begin{align}
f'_{\gi{i_1...i_n}}&=f(e'_{\gi{i_1}},...,e'_{\gi{i_n}})
\nonumber
\\
&=f(e_{\gi{j_1}}A_{\gi{i_1}}^{\gi{j_1}} ,...,
e'_{\gi{j_n}}A_{\gi{i_n}}^{\gi{j_n}})
\EqLabel{polylinear map over field, division ring, change coordinates}
\\
&=A_{\gi{i_1}}^{\gi{j_1}} ...
A_{\gi{i_n}}^{\gi{j_n}} f(e_{\gi{j_1}},...,e_{\gi{j_n}})
\nonumber
\\
&=A_{\gi{i_1}}^{\gi{j_1}} ... A_{\gi{i_n}}^{\gi{j_n}} f_{\gi{j_1...j_n}}
\nonumber
\end{align}
}
{polylinear map over field, division ring, change coordinates}

\DefEquation
{
f(a_1,...,a_n)
=e_{\gi p}
f_{\gi{i_1...i_n}}^{\gi p}a^{\gi{i_1}}_1...a^{\gi{i_n}}_n
}
{polylinear map over field, division ring, 1a}

\DefEq
{
\begin{align}
a_j&=e_{\gi i}a^{\gi i}_j
\nonumber
\\
f_{\gi{i_1...i_n}}&=f(e_{\gi{i_1}},...,e_{\gi{i_n}})
\EqLabel{polylinear map over field, coordinates, division ring}
\end{align}
}
{polylinear map over field, coordinates, division ring}

\DefEq
{
\[
f(a_1,...,a_n)=
f(e_{\gi{i_1}}a^{\gi{i_1}}_1,...,e_{\gi{i_n}}a^{\gi{i_n}}_n)
=a^{\gi{i_1}}_1...a^{\gi{i_n}}_nf(e_{\gi{i_1}},...,e_{\gi{i_n}})
\]
}
{polylinear map over field, 1, division ring}

\DefEq
{
\begin{equation}
f_{\gi{i_1,...,i_n}}=f_{\sigma(\gi{i_1}),...,\sigma(\gi{i_n})}
\EqLabel{polylinear map symmetric, division ring}
\end{equation}
}
{polylinear map symmetric, division ring}

\DefEq
{
\begin{align*}
a^{\gi{i_1}}_1 ... a^{\gi{i_n}}_n f_{\gi{i_1...i_n}}
=&f(a_1,...,a_n)
\\
=&|\sigma|f(\sigma(a_1),...,\sigma(a_n))
\\
=&a_1^{\gi{i_1}} ... a_n^{\gi{i_n}} |\sigma| f_{\sigma(\gi{i_1})...\sigma(\gi{i_n})}
\end{align*}
}
{polylinear map skew symmetric, 1, division ring}

\DefEq
{
\begin{align}
f_{\gi{j_1...j_n}}
=&f_t^{\gi{i_0...i_n}}
C_{\gi{i_0}\sigma_t(\gi{j_1})}^{\gi{k_1}}
C_{\gi{k_1i_1}}^{\gi{l_1}}
 ... B{}_{\gi{l_{n-1}}\sigma_t(\gi{j_n})}^{\gi{k_n}}
C_{\gi{k_ni_n}}^{\gi{l_n}}e_{\gi{l_n}}
\EqLabel{coordinates of polylinear map, division ring over field}
\\
f_{\gi{j_1...j_n}}^{\gi p}
=&f_t^{\gi{i_0...i_n}}
C_{\gi{i_0}\sigma_t(\gi{j_1})}^{\gi{k_1}}
C_{\gi{k_1i_1}}^{\gi{l_1}}
... C_{\gi{l_{n-1}}\sigma_t(\gi{j_n})}^{\gi{k_n}}
C_{\gi{k_ni_n}}^{\gi p}
\EqLabel{coordinates of polylinear map, division ring over field, 1}
\end{align}
}
{coordinates of polylinear map, division ring over field}

\DefEq
{
\[
d_i=e_{\gi{j_i}}d_i^{\gi{j_i}}
\]
}
{coordinates of polylinear map, 1, division ring over field}

\DefEquation
{
\begin{array}{r@{\ }l}
f(d_1,...,d_n)
=&f_t^{\gi{i_0...i_n}}
\ e_{\gi{i_0}} \sigma_t(d_1^{\gi{j_1}} e_{\gi{j_1}})
e_{\gi{i_1}} ... \sigma_t(d_n^{\gi{j_n}}
e_{\gi{j_n}}) e_{\gi{i_n}}
\\
=&d_1^{\gi{j_1}} ...d_n^{\gi{j_n}} f_t^{\gi{i_0...i_n}}
e_{\gi{i_0}} \sigma_t(e_{\gi{j_1}})
e_{\gi{i_1}} ... \sigma_t(e_{\gi{j_n}}) e_{\gi{i_n}}
\\
=&d_1^{\gi{j_1}} ...d_n^{\gi{j_n}} f_t^{\gi{i_0...i_n}}
C_{\gi{i_0}\sigma_t(\gi{j_1})}^{\gi{k_1}}
C_{\gi{k_1i_1}}^{\gi{l_1}}
\\
&...C_{\gi{l_{n-1}}\sigma_t(\gi{j_n})}^{\gi{k_n}}
C_{\gi{k_ni_n}}^{\gi{l_n}} e_{\gi{l_n}}
\end{array}
}
{polylinear map, division ring, standard representation, 1a}

\DefEquation
{
d=f\pC{s}{0}^{n\gi{j_1}}\ e_{\gi{j_1}}\ \sigma_s(d_1)
\ f\pC{s}{1}^{n\gi{j_2}}\ e_{\gi{j_2}}\ ...
\ \sigma_s(d_n)\ f\pC{s}{n}^{n\gi{j_n}}\ e_{\gi{j_n}}
}
{polylinear map, division ring, standard representation, 1}

\DefEquation
{
f_t^{\gi{j_0...j_n}}=
f\pC{s}{0}^{n\gi{j_1}}\ ...f\pC{s}{n}^{n\gi{j_n}}
}
{polylinear map, division ring, standard representation, 2}

\DefEquation
{
f\pC{s}{p}^n=e_{\gi i}f\pC{s}{p}^{n\gi i}
}
{polylinear map, division ring, components extention}

\DefEquation
{
f_{\gi{i_1,...,i_n}}=|\sigma|f_{\sigma(\gi{i_1}),...,\sigma(\gi{i_n})}
}
{polylinear map skew symmetric, division ring}

\DefEq
{
\begin{align*}
a^{\gi{i_1}}_1 ... a^{\gi{i_n}}_n f_{\gi{i_1...i_n}}
=&f(a_1,...,a_n)
\\
=&f(\sigma(a_1),...,\sigma(a_n))
\\
=&a_1^{\gi{i_1}} ... a_n^{\gi{i_n}} f_{\sigma(\gi{i_1})...\sigma(\gi{i_n})}
\end{align*}
}
{polylinear map symmetric, 1, division ring}

\DefEquation
{
d=f\pC{s}{0}^n\ \sigma_s(d_1)
\ f\pC{s}{1}^n\ ...\ \sigma_s(d_n)\ f\pC{s}{n}^n
}
{polylinear map, division ring, canonical morphism}

\DefEq
{
\[
\sigma_s=
\begin{pmatrix}
d_1&...&d_n
\\
\sigma_s(d_1)&...&\sigma_s(d_n)
\end{pmatrix}
\]
}
{transposition of set of variables, division ring}

\DefEq
{
\[
\begin{matrix}
f\pC{s}{p}^1=f\pC{s}{p}
&p=0, 1
\end{matrix}
\]
}
{polylinear map, division ring, 1, canonical morphism}

\DefEq
{
\[
\xymatrix{
D^k\ar[rr]^f\ar@{=>}[drr]_{g(d_k)}
& & D
\\
& &
\\
&&D^{k-1}\ar[uu]_h &
}
\]
\[
d=f(d_1,...,d_k)=g(d_k)(d_1,...,d_{k-1})
\]
}
{polylinear map, induction on n, 1, division ring}

\DefEq
{
\[
d=
h\pC{t}{0}^{k-1}\ \sigma_t(d_1)
\ h\pC{t}{1}^{k-1}\ ...
\ \sigma_t(d_{k-1})\ h\pC{t}{k-1}^{k-1}
\]
}
{polylinear map, induction on n, 2, division ring}

\DefEq
{
\[
h\pC{t}{0}^{k-1}
=g\pC{tr}{0}
\ d_k\ g\pC{tr}{1}
\]
}
{polylinear map, induction on n, 3, division ring}

\DefEq
{
\[
\sigma_s=\sigma_{tr}=
\left(
\begin{array}{cccc}
d_k&d_1&...&d_{k-1}
\\
d_k&\sigma_t(d_1)&...&\sigma_t(d_{k-1})
\end{array}
\right)
\]
}
{polylinear map, induction on n, 4, division ring}

\DefEq
{
\[
\begin{matrix}
f\pC{tr}{q+1}^k=h\pC{t}{q}^{k-1}
&q=1, ..., k-1
\\
f\pC{tr}{q}^k=g\pC{tr}{q}
&q=0, 1
\end{matrix}
\]
}
{polylinear map, induction on n, 5, division ring}

\DefEq
{
\symb{f_{s\cdot p}^n}1{component of polylinear map}
}
{component of polylinear map, division ring}

\DefEq
{
\symb{f_t^{\gi{i_0...i_n}}}0{standard component of polylinear map}
\begin{equation}
f(d_1,...,d_n)=
\ShowSymbol{standard component of polylinear map}
\ e_{\gi{i_0}}\ \sigma_t(d_1)\ 
e_{\gi{i_1}}
\ ...\ \sigma_t(d_n)\ e_{\gi{i_n}}
\EqLabel{polylinear map, division ring, standard representation}
\end{equation}
}
{polylinear map, division ring, standard representation}



==> Ring.Linear.Map.Russian.tex <==
%auto-ignore
\input{Ring.Linear.Map.Eq}

\ifx\PrintBook\undefined
\else
\chapter{Линейное отображение тела}
\label{chapter: Linear map, Division Ring}
\fi

\section{Линейное отображение тела}
\label{section: linear map of division ring}

Согласно замечанию
\xRef{0701.238}{remark: Geometry of Division Ring over Field},
мы рассматриваем тело $D$ как алгебру над полем \FZD.

\begin{definition}
\label{definition: linear map of division ring}
Пусть $D_1$, $D_2$ - тела.
Пусть $F$ - поле такое, что
\ShowEq{field division ring d1 d2}
Линейное отображение
\ShowEq{f d1 d2}
$F$\Hyph векторного пространства $D_1$
в $F$\Hyph векторное пространство $D_2$
называется
\AddIndex{линейным отображением
тела $D_1$ в тело $D_2$}{linear map of division ring}.
\qed
\end{definition} 

Согласно определению \ref{definition: linear map of division ring},
линейное отображение $f$ тела $D_1$ в тело $D_2$
удовлетворяет свойству
\ShowEq{linear map of division ring}

\begin{theorem}
\label{theorem: linear map, division ring, integer}
Пусть отображение
\ShowEq{f d1 d2}
является линейным отображением
тела $D_1$ характеристики $0$ в тело $D_2$ характеристики $0$.
Тогда\footnote{Допустим
\ShowEq{f d1 d2}
является линейным отображением
тела $D_1$ характеристики $2$ в тело $D_2$ характеристики $3$.
Тогда для любого $a\in D_1$, $2a=0$, хотя $2 f(a)\ne 0$.
Следовательно, если мы предположим, что характеристика тела $D_1$ больше
$0$, то мы должны потребовать, чтобы характеристика тела $D_1$
равнялась характеристике тела $D_2$.}
\[
f(nx)=nf(x)
\]
для любого целого $n$.
\end{theorem}
\begin{proof}
Мы докажем теорему индукцией по $n$.
При $n=1$ утверждение очевидно, так как
\[
f(1x)=f(x)=1f(x)
\]
Допустим уравнение справедливо при $n=k$. Тогда
\[
f((k+1)x)=f(kx+x)=f(kx)+f(x)=kf(x)+f(x)=(k+1)f(x)
\]
\end{proof}

\begin{theorem}
\label{theorem: linear map, division ring, rational}
Пусть отображение
\ShowEq{f d1 d2}
является линейным отображением
тела $D_1$ характеристики $0$ в тело $D_2$ характеристики $0$.
Тогда
\[
f(ax)=af(x)
\]
для любого рационального $a$.
\end{theorem}
\begin{proof}
Запишем $a$ в виде $a=\frac pq$.
Положим $y=\frac 1qx$. Тогда
согласно теореме \ref{theorem: linear map, division ring, integer}
\begin{equation}
f(x)=f(qy)=qf(y)=qf\left(\frac 1qx\right)
\EqLabel{additive map, division ring, rational, 1}
\end{equation}
Из равенства \EqRef{additive map, division ring, rational, 1}
следует
\begin{equation}
\frac 1qf(x)=f\left(\frac 1qx\right)
\EqLabel{additive map, division ring, rational, 2}
\end{equation}
Из равенства \EqRef{additive map, division ring, rational, 2}
следует
\[
f\left(\frac pqx\right)=pf\left(\frac 1qx\right)=\frac pqf(x)
\]
\end{proof}

Мы не можем распространить утверждение теоремы
\ref{theorem: linear map, division ring, rational}
на произвольное подполе центра $Z(D)$ тела $D$.

\begin{theorem}
\label{theorem: exists linear map not linear over center, division ring}
Пусть тело $D$ является алгеброй над полем \FZD.
Если $F\ne Z(D)$, то существует линейное отображение
\ShowEq{f D D}
которое нелинейно над полем $Z(D)$.
\end{theorem}
\begin{proof}
Для доказательства теоремы достаточно рассмотреть поле
комплексных чисел $C$ так как $C=Z(C)$.
Так как поле комплексных чисел является алгеброй над полем вещественных чисел,
то функция
\[
z\rightarrow \overline z
\]
линейна. Однако равенство
\[
\overline{az}=a\overline z
\]
неверно.
\end{proof}

Из теоремы
\ref{theorem: exists linear map not linear over center, division ring}
возникает вопрос.
Для чего мы рассматриваем линейные отображения над полем $F\ne Z(D)$,
если это приводит к резкому рассширению множества линейных отображений?
Ответом на этот вопрос служит богатый опыт
теории функции комплексного переменного.

\begin{theorem}
\label{theorem: sum of linear maps, division ring}
Пусть отображения
\ShowEq{f d1 d2}
\ShowEq{g d1 d2}
являются линейными отображениями
тела $D_1$ в тело $D_2$.
Тогда отображение $f+g$ также является линейным.
\end{theorem}
\begin{proof}
Утверждение теоремы следует из цепочки равенств
\ShowEq{sum of linear maps, division ring}
\end{proof}

\begin{theorem}
\label{theorem: linear map times constant, division ring}
Пусть отображение \ShowEq{f d1 d2}
является линейным отображением
тела $D_1$ в тело $D_2$.
Тогда отображения $af$, $fb$, $a$, $b\in R_2$, также являются линейными.
\end{theorem}
\begin{proof}
Утверждение теоремы следует из цепочки равенств
\ShowEq{linear map times constant, division ring}
\end{proof}

\begin{definition}
Обозначим
\ShowEq{set linear maps, division ring}
множество линейных отображений
\ShowEq{f d1 d2}
тела $D_1$ в тело $D_2$.
\qed
\end{definition}

\begin{theorem}
\label{theorem: linear map, division ring, morphism}
Мы можем представить линейное отображение
\ShowEq{f d1 d2}
тела $D_1$ в тело $D_2$ в виде
\ShowEq{linear map, division ring, morphism}
где $(G_{k}, k\in K)$ - множество аддитивных отображений
тела $D_1$ в тело $D_2$.\footnote{Здесь и в дальнейшем
мы будем предполагать
сумму по индексу, который встречается в произведении несколько раз.
Равенство \EqRef{linear map, division ring, morphism}
является рекурсивным определением и есть надежда, что мы можем
его упростить.}
Выражение
\ShowEq{component of linear map, division ring}
в равенстве \EqRef{linear map, division ring, morphism}
называется
\AddIndex{компонентой линейного отображения}{component of linear map} $f$.
\end{theorem}
\begin{proof}
Утверждение теоремы следует из теорем
\ref{theorem: sum of linear maps, division ring} и
\ref{theorem: linear map times constant, division ring}.
\end{proof}

Если в теореме
\ref{theorem: linear map, division ring, morphism}
$|K|=1$,
то равенство
\EqRef{linear map, division ring, morphism}
имеет вид
\ShowEq{linear map, division ring, morphism G}
и отображение $f$ называется
\AddIndex{линейным отображением, порождённым отображением}
{linear map generated by map} $G$.
Отображение $G$ мы будем называть
\AddIndex{образующей линейного отображения}
{generator of linear map}.

\begin{theorem}
\label{theorem: linear map based G, standard form, division ring}
Пусть $D_1$, $D_2$ - тела характеристики $0$.
Пусть $F$, $F\subset Z(D_1)$, $F\subset Z(D_2)$, - поле.
Пусть $G$ - линейное отображение.
Пусть $\Basis e$ - базис тела $D_2$ над полем $F$.
\AddIndex{Стандартное представление линейного отображения}
{linear map, standard representation}
\EqRef{linear map, division ring, morphism G}
имеет вид\footnote{Представление линейного отображения тела с помощью
компонент линейного отображения
неоднозначно. Чисто алгебраическими методами мы можем
увеличить либо уменьшить число слагаемых.
Если размерность тела $D_2$ над полем $F$ конечна, то стандартное представление
линейного отображения гарантирует конечность множества
слагаемых в представлении отображения.}
\ShowEq{linear map, division ring, G, standard representation}
Выражение
$\ShowSymbol{standard component of linear map, G}$
в равенстве \EqRef{linear map, division ring, G, standard representation}
называется
\AddIndex{стандартной компонентой линейного отображения}
{standard component of linear map} $f$.
\end{theorem}
\begin{proof}
Компоненты линейного отображения $f$
имеют разложение
\ShowEq{linear map, division ring, components extention}
относительно базиса $\Basis e$.
Если мы подставим \EqRef{linear map, division ring, components extention}
в \EqRef{linear map, division ring, morphism G},
мы получим
\ShowEq{linear map, division ring, G, standard representation, 1}
Подставив в равенство \EqRef{linear map, division ring, G, standard representation, 1}
выражение
\ShowEq{linear map, division ring, G, standard representation, 2}
мы получим равенство \EqRef{linear map, division ring, G, standard representation}.
\end{proof}

\begin{theorem}
\label{theorem: linear map, G, coordinates and components, division ring}
Пусть $D_1$, $D_2$ - тела характеристики $0$.
Пусть $F$, $F\subset Z(D_1)$, $F\subset Z(D_2)$, - поле.
Пусть $G$ - линейное отображение.
Пусть $\Basis e_1$ - базис тела $D_1$ над полем $F$.
Пусть $\Basis e_2$ - базис тела $D_2$ над полем $F$.
Пусть
\ShowEq{structural constants, division ring D2}
- структурные константы тела $D_2$.
Тогда линейное отображение
\EqRef{linear map, division ring, morphism G},
порождённое линейным отображением $G$,
можно записать в виде
\ShowEq{linear map, G, coordinates and components, division ring}
\end{theorem}
\begin{proof}
Выберем отображение
\ShowEq{linear map D1 D2 generator}
Согласно теореме \xRef{0701.238}{theorem: linear map of rcd vector space}
линейное отображение $f(a)$ относительно базисов $\Basis e_1$ и
$\Basis e_2$ принимает вид
\EqRef{linear map, G, coordinates and components, division ring}.
Из равенств \EqRef{linear map, division ring, G, standard representation}
и \EqRef{linear map D1 D2 generator}
следует
\ShowEq{division ring, F linear map G, standard representation}
Из равенств \EqRef{linear map, G, coordinates and components, division ring}
и \EqRef{division ring, F linear map G, standard representation}
следует
\ShowEq{linear map, G, coordinates and components, division ring, 1}
Так как векторы $e_{2.\gi r}$ линейно независимы над полем $F$ и величины
$a^{\gik}$ произвольны, то из равенства
\EqRef{linear map, G, coordinates and components, division ring, 1}
следует равенство
\EqRef{linear map, G, coordinates and components, division ring, relation}.
\end{proof}

При рассмотрении отображений
\ShowEq{linear map, division ring}
мы будем полагать $G(x)=x$.

\begin{theorem}
\label{theorem: linear map, division ring, canonical morphism}
Пусть $D$ является телом характеристики $0$.
Линейное отображение
\EqRef{linear map, division ring}
имеет вид
\ShowEq{linear map, division ring, canonical morphism}
\end{theorem}

\begin{theorem}
\label{theorem: linear map, standard form, division ring}
Пусть $D$ - тело характеристики $0$.
Пусть $\Basis e$ - базис тела $D$ над полем $F\subset Z(D)$.
Стандартное представление линейного отображения
\EqRef{linear map, division ring, canonical morphism}
тела
имеет вид
\ShowEq{linear map, division ring, standard representation}
\end{theorem}

\begin{theorem}
\label{theorem: linear map over field, division ring}
Пусть $D$ является телом характеристики $0$.
Пусть $\Basis e$ - базис тела $D$ над полем $F\subset Z(D)$.
Тогда линейное отображение
\EqRef{linear map, division ring}
можно записать в виде
\ShowEq{linear map over field, division ring}
\end{theorem}

\begin{theorem}
\label{theorem: linear map over field, division ring, determinant}
Рассмотрим матрицу
\ShowEq{linear map over field, division ring, matrix}
строки которой пронумерованы индексом
\ShowEq{linear map over field, division ring, row of matrix}
и столбцы пронумерованы индексом
\ShowEq{linear map over field, division ring, column of matrix}
Если
\ShowEq{linear map over field, division ring, determinant},
то для заданных координат линейного преобразования $f_{\gi i}^{\gi j}$
система линейных уравнений
\EqRef{linear map over field, division ring, relation}
относительно стандартных компонент этого преобразования
$f^{\gi{kr}}$ имеет единственное
решение.
Если
\ShowEq{linear map over field, division ring, determinant=0},
то условием существования решения
системы линейных уравнений
\EqRef{linear map over field, division ring, relation}
является равенство
\ShowEq{linear map over field, division ring, determinant=0, 1}
В этом случае система линейных уравнений
\EqRef{linear map over field, division ring, relation}
имеет бесконечно много решений и существует линейная
зависимость между величинами $f_{\gi i}^{\gi j}$.
\end{theorem}
\begin{proof}
Равенство
\EqRef{linear map, division ring, canonical morphism}
является частным случаем равенства
\EqRef{linear map, division ring, morphism G}
при условии $G(x)=x$.
Теорема
\ref{theorem: linear map, standard form, division ring}
является частным случаем теоремы
\ref{theorem: linear map based G, standard form, division ring}
при условии $G(x)=x$.
Теорема
\ref{theorem: linear map over field, division ring}
является частным случаем теоремы
\ref{theorem: linear map, G, coordinates and components, division ring}
при условии $G(x)=x$.
Утверждение теоремы
\ref{theorem: linear map over field, division ring, determinant}
является следствием
теории линейных уравнений над полем.
\end{proof}

\begin{theorem}
\label{theorem: identity map, division ring}
Стандартные компоненты тождественного отображения имеют вид
\ShowEq{identity map, division ring}
\end{theorem}
\begin{proof}
Равенство
\EqRef{identity map, division ring}
является следствием равенства
\ShowEq{identity map 0, division ring}
Убедимся, что стандартные компоненты
\EqRef{identity map, division ring}
линейного преобразования удовлетворяют уравнению
\ShowEq{identity map 1, division ring}
которое следует из уравнения
\EqRef{linear map over field, division ring, relation}
если $f=\delta$.
Из равенств
\EqRef{identity map, division ring},
\EqRef{identity map 1, division ring}
следует
\ShowEq{identity map 2, division ring}
Равенство
\EqRef{identity map 2, division ring}
верно, так как из равенств
\ShowEq{identity map 3, division ring}
следует
\ShowEq{identity map 4, division ring}
Если
\ShowEq{linear map over field, division ring, determinant},
то решение
\EqRef{identity map, division ring}
единственно.
Если
\ShowEq{linear map over field, division ring, determinant=0},
то система линейных уравнений
\EqRef{identity map 1, division ring}
имеет бесконечно много решений.
Однако нас интересует по крайней мере одно.
\end{proof}

\begin{theorem}
\label{theorem: zero map, division ring}
Если
\ShowEq{linear map over field, division ring, determinant},
то стандартные компоненты нулевого отображения
\ShowEq{zero map, division ring}
определены однозначно и имеют вид
\ShowEq{zero map, division ring, 1}
Если
\ShowEq{linear map over field, division ring, determinant=0},
то множество стандартных компонент нулевого отображения
порождает векторное пространство.
\end{theorem}
\begin{proof}
Теорема верна, поскольку стандартные компоненты $z^{\gi{ij}}$
являются решением однородной системы линейных уравнений
\ShowEq{zero map, division ring, 2}
\end{proof}

\begin{remark}
\label{remark: zero map, division ring}
Рассмотрим равенство
\ShowEq{linear maps a=b, division ring}
Из теоремы \ref{theorem: zero map, division ring}
следует, что только при условии
\ShowEq{linear map over field, division ring, determinant}
из равенства
\EqRef{linear maps a=b, division ring}
следует
\ShowEq{linear maps a=b, 1, division ring}
В противном случае мы должны предполагать равенство
\ShowEq{linear maps a=b, 2, division ring}
%Это означает, что векторы
%\ShowEq{linear maps a=b, 3, division ring}
%линейно зависимы.
Несмотря на это, мы и в случае
\ShowEq{linear map over field, division ring, determinant=0}
будем пользоваться стандартным представлением
так как в общем случае указать множество линейно
независимых векторов - задача достаточно сложная.
Если мы хотим определить операцию над линейными отображениями,
записанными в стандартном представлении,
то также как в случае теоремы
\ref{theorem: identity map, division ring}
мы будем выбирать представитель из множества возможных представлений.
\qed
\end{remark}

\begin{theorem}
Выражение
\ShowEq{fkr is tensor}
является тензором над полем $F$
\ShowEq{fkr is tensor, division ring, transformation}
\end{theorem}
\begin{proof}
$D$\Hyph линейное отображение относительно базиса $\Basis e$ имеет вид
\EqRef{linear map over field, division ring}.
Пусть $\Basis e{}'$ - другой базис. Пусть
\ShowEq{fkr is tensor, division ring, change basis}
преобразование, отображающее базис $\Basis e$ в
базис $\Basis e{}'$.
Так как линейное отображение $f$ не меняется, то
\ShowEq{fkr is tensor, division ring, transformation, 1}
Подставим \xEqRef{0701.238}{division ring over field, change basis, 3},
\EqRef{fkr is tensor, division ring, change basis}
в равенство \EqRef{fkr is tensor, division ring, transformation, 1}
\ShowEq{fkr is tensor, division ring, transformation, 2}
Так как векторы $e_{\gi j}$ линейно независимы и
компоненты вектора $x^{\gi i}$ произвольны, то равенство
\EqRef{fkr is tensor, division ring, transformation}
следует
из равенства
\EqRef{fkr is tensor, division ring, transformation, 2}.
Следовательно, выражение
$f_k^r$
является тензором над полем $F$.
\end{proof}

\ePrints{0908.3307}%
\ifx\Semafor\ValueOff%
\begin{definition}
Множество
\ShowEq{kernel of linear map, division ring}
называется
\AddIndex{ядром линейного отображения}{kernel of linear map}
\ShowEq{f d1 d2}
тела $D_1$
в тело $D_2$.
\qed
\end{definition}

\begin{theorem}
Ядро линейного отображения
\ShowEq{f d1 d2}
является подгруппой аддитивной группы тела $D_1$.
\end{theorem}
\begin{proof}
Пусть $a$, $b\in\text{ker}f$. Тогда
\begin{align*}
f(a)&=0
\\
f(b)&=0
\\
f(a+b)=f(a)+f(b)&=0
\end{align*}
Следовательно, $a+b\in\text{ker}f$.
\end{proof}

\begin{definition}
Линейное отображение
\ShowEq{f d1 d2}
тела $D_1$
в тело $D_2$
называется
\AddIndex{вырожденным}{singular linear map},
если
\[\text{ker}f\ne\{0\}\]
\qed
\end{definition}
\fi

\begin{theorem}
\label{theorem: product of linear map, D D D}
Пусть $D$ - тело характеристики $0$.
Пусть $\Basis e$ - базис тела $D$ над центром $Z(D)$ тела $D$.
Пусть
\ShowEq{product of additive map, D D D}
линейные отображения тела $D$.
Отображение
\begin{equation}
h(x)=gf(x)=g(f(x))
\EqLabel{D linear map, division ring, h1}
\end{equation}
является линейным отображением
\ShowEq{D linear map, division ring, h2}
где
\ShowEq{D linear map, division ring, h gf}
\end{theorem}
\begin{proof}
Отображение \EqRef{D linear map, division ring, h1}
линейно так как
\ShowEq{product of additive map, D D D, 1}

Если мы подставим
\EqRef{D linear map, division ring, f} и
\EqRef{D linear map, division ring, g} в
\EqRef{D linear map, division ring, h1},
то мы получим
\ShowEq{additive map, division ring, h3}
Сравнивая \EqRef{additive map, division ring, h3}
и \EqRef{D linear map, division ring, h2},
мы получим \EqRef{D linear map, division ring, h gf, 0},
\EqRef{D linear map, division ring, h gf, 1}.

Если мы подставим
\EqRef{D linear map, division ring, standard representation, f} и
\EqRef{D linear map, division ring, standard representation, g} в
\EqRef{D linear map, division ring, h1},
то мы получим
\ShowEq{D linear map, division ring, standard representation, h3}
Сравнивая \EqRef{D linear map, division ring, standard representation, h3}
и \EqRef{D linear map, division ring, standard representation, h2},
мы получим \EqRef{D linear map, division ring, standard representation, h gf}.
\end{proof}

\ePrints{0812.4763}
\ifx\Semafor\ValueOn

\begin{definition}
\label{definition: map projective over commutative ring, ring}
Пусть коммутативное кольцо $P$ является подкольцом центра $Z(R)$ кольца $R$.
Отображение
\[f:R\rightarrow R\]
кольца $R$
называется
\AddIndex{проективным над коммутативным кольцом}
{map projective over commutative ring} $P$, если
\[
f(px)=f(x)
\]
для любого $p\in P$. Множество
\[
Px=\{px:p\in P,x\in R\}
\]
называется
\AddIndex{направлением $x$ над коммутативным кольцом}
{direction over commutative ring}\footnote{Направление
над коммутативным кольцом $P$ является подможеством кольца $R$.
Однако мы будем обозначать направление $Px$ элементом
$x\in R$, когда это не приводит к неоднозначности.
Мы будем говорить о направлении над коммутативным кольцом $Z(R)$,
если мы явно не указываем коммутативное кольцо $P$.} $P$.
\qed
\end{definition}

\begin{example}
\label{example: map projective over commutative ring, ring}
Если отображение $f$
кольца $R$ линейно над коммутативным кольцом $P$,
то отображение
\[
g(x)=x^{-1}f(x)
\]
проективно над коммутативным кольцом $P$.
\qed
\end{example}
\fi

\section{Полилинейное отображение тела}

\begin{definition}
\label{definition: map polylinear over commutative ring, ring}
Пусть $R_1$, ..., $R_n$, $P$ - кольца характеристики $0$.
Пусть $S$ - модуль над кольцом $P$.
Пусть $F$ - коммутативное кольцо, которое для любого $i$ является подкольцом центра
кольца $R_i$.
Отображение
\[
f:R_1\times...\times R_n\rightarrow
S
\]
называется \AddIndex{полилинейным над коммутативным кольцом $F$}
{map polylinear over commutative ring, ring},
если
\ShowEq{map polylinear over commutative ring}
для любого $i$, $1\le i\le n$, и любых $p_i$, $q_i \in R_i$, $b\in F$.
Обозначим
\symb{\mathcal L(R_1,...,R_n;
S)}1{set polylinear maps, ring}
множество полилинейных отображений
колец
$R_1$, ..., $R_n$
в модуль
$S$.
\qed
\end{definition}

\begin{theorem}
\label{theorem: polylinear map, division ring}
Пусть $D$ - тело характеристики $0$.
Полилинейное отображение
\ShowEq{polylinear map, division ring}
имеет вид
\ShowEq{polylinear map, division ring, canonical morphism}
$\sigma_s$ - перестановка множества переменных
$\{d_1,...,d_n\}$
\ShowEq{transposition of set of variables, division ring}
\end{theorem}
\begin{proof}
Мы докажем утверждение индукцией по $n$.

При $n=1$ доказываемое утверждение является следствием теоремы
\ref{theorem: linear map, division ring, canonical morphism}.
При этом мы можем отождествить\footnote{В представлении
\EqRef{polylinear map, division ring, canonical morphism}
мы будем пользоваться следующими правилами.
\begin{itemize}
\item Если область значений какого-либо индекса - это множество,
состоящее из одного элемента, мы будем опускать соответствующий
индекс.
\item Если $n=1$, то $\sigma_s$ - тождественное преобразование.
Это преобразование можно не указывать в выражении.
\end{itemize}}
\ShowEq{polylinear map, division ring, 1, canonical morphism}

Допустим, что утверждение теоремы справедливо при $n=k-1$.
Тогда отображение
\EqRef{polylinear map, division ring}
можно представить в виде
\ShowEq{polylinear map, induction on n, 1, division ring}
Согласно предположению индукции полилинейное отображение
$h$ имеет вид
\ShowEq{polylinear map, induction on n, 2, division ring}
Согласно построению $h=g(d_k)$.
Следовательно, выражения $h\pC{t}{p}$
являются функциями $d_k$.
Поскольку $g(d_k)$ - линейная функция $d_k$,
то только одно выражение $h\pC{t}{p}$
является линейной функцией переменной $d_k$, и остальные выражения
$\pC{t}{q}h$
не зависят от $d_k$.

Не нарушая общности, положим $p=0$.
Согласно равенству
\EqRef{linear map, division ring, canonical morphism}
для заданного $t$
\ShowEq{polylinear map, induction on n, 3, division ring}
Положим $s=tr$ и определим перестановку $\sigma_s$ согласно правилу
\ShowEq{polylinear map, induction on n, 4, division ring}
Положим
\ShowEq{polylinear map, induction on n, 5, division ring}
Мы доказали шаг индукции.
\end{proof}

\begin{definition}
\begin{sloppypar}
Выражение
\ShowEq{component of polylinear map, division ring}
в равенстве \EqRef{polylinear map, division ring, canonical morphism}
называется \AddIndex{компонентой полилинейного отображения $f$}
{component of polylinear map, division ring}.
\qed
\end{sloppypar}
\end{definition}

\begin{theorem}
\label{theorem: standard representation of polylinear map, division ring}
Пусть $D$ - тело характеристики $0$.
Допустим $\Basis e$
- базис тела $D$ над полем \FZD.
\AddIndex{Стандартное представление полилинейного отображения}
{polylinear map, standard representation} тела
имеет вид
\ShowEq{polylinear map, division ring, standard representation}
Индекс $t$ нумерует всевозможные перестановки
$\sigma_t$ множества переменных
$\{d_1,...,d_n\}$.
Выражение
$\ShowSymbol{standard component of polylinear map}$
в равенстве \EqRef{polylinear map, division ring, standard representation}
называется \AddIndex{стандартной компонентой полилинейного отображения}
{standard component of polylinear map} $f$.
\end{theorem}
\begin{proof}
Компоненты полилинейного отображения $f$
имеют разложение
\ShowEq{polylinear map, division ring, components extention}
относительно базиса $\Basis e$.
Если мы подставим \EqRef{polylinear map, division ring, components extention}
в \EqRef{polylinear map, division ring, canonical morphism},
мы получим
\ShowEq{polylinear map, division ring, standard representation, 1}
Рассмотрим выражение
\ShowEq{polylinear map, division ring, standard representation, 2}
В правой части подразумевается сумма тех слагаемых с индексом $s$,
для которых перестановка $\sigma_s$ совпадает. Каждая такая сумма
будет иметь уникальный индекс $t$.
Подставив в равенство
\EqRef{polylinear map, division ring, standard representation, 1}
выражение
\EqRef{polylinear map, division ring, standard representation, 2}
мы получим равенство \EqRef{polylinear map, division ring, standard representation}.
\end{proof}

\begin{theorem}
\label{theorem: polylinear map over field, division ring}
Пусть $\Basis e$ - базис тела $D$ над полем \FZD.
Полилинейное отображение
\EqRef{polylinear map, division ring}
можно представить в виде $D$-значной формы степени $n$
над полем \FZD\footnote{Теорема доказана по аналогии
с теоремой в \citeBib{Rashevsky}, с. 107, 108}
\ShowEq{polylinear map over field, division ring}
где
\ShowEq{polylinear map over field, coordinates, division ring}
и величины $f_{\gi{i_1...i_n}}$
являются координатами $D$-значного ковариантнго тензора над полем $F$.
\end{theorem}
\begin{proof}
Согласно определению
\ref{definition: map polylinear over commutative ring, ring}
равенство
\EqRef{polylinear map over field, division ring}
следует из цепочки равенств
\ShowEq{polylinear map over field, 1, division ring}
Пусть $\Basis e'$ - другой базис. Пусть
\ShowEq{polylinear map over field, division ring, change basis}
преобразование, отображающее базис $\Basis e$ в
базис $\Basis e'$.
Из равенств \EqRef{polylinear map over field, division ring, change basis}
и \EqRef{polylinear map over field, coordinates, division ring}
следует
\ShowEq{polylinear map over field, division ring, change coordinates}
Из равенства \EqRef{polylinear map over field, division ring, change coordinates}
следует тензорный закон преобразования координат полилинейного отображения.
Из равенства \EqRef{polylinear map over field, division ring, change coordinates}
и теоремы \xRef{0701.238}{theorem: division ring over field, change basis}
следует, что значение отображения $f(a_1,...,a_n)$ не зависит от выбора
базиса.
\end{proof}

Полилинейное отображение
\EqRef{polylinear map, division ring}
\AddIndex{симметрично}
{polylinear map symmetric, division ring}, если
\[
f(d_1,...,d_n)=f(\sigma(d_1),...,\sigma(d_n))
\]
для любой перестановки $\sigma$ множества $\{d_1,...,d_n\}$.

\begin{theorem}
\label{theorem: polylinear map symmetric, division ring}
Если полилинейное отображение $f$ симметрично,
то
\ShowEq{polylinear map symmetric, division ring}
\end{theorem}
\begin{proof}
Равенство
\EqRef{polylinear map symmetric, division ring}
следует из равенства
\ShowEq{polylinear map symmetric, 1, division ring}
\end{proof}

Полилинейное отображение
\EqRef{polylinear map, division ring}
\AddIndex{косо симметрично}{polylinear map skew symmetric}, если
\[
f(d_1,...,d_n)=|\sigma|f(\sigma(d_1),...,\sigma(d_n))
\]
для любой перестановки $\sigma$ множества $\{d_1,...,d_n\}$.
Здесь
\[
|\sigma|=
\left\{
\begin{matrix}
1&\textrm{перестановка }\sigma\textrm{ чётная}
\\
-1&\textrm{перестановка }\sigma\textrm{ нечётная}
\end{matrix}
\right.
\]

\begin{theorem}
\label{theorem: polylinear map skew symmetric, division ring}
Если полилинейное отображение $f$ косо симметрично,
то
\ShowEq{polylinear map skew symmetric, division ring}
\end{theorem}
\begin{proof}
Равенство
\EqRef{polylinear map skew symmetric, division ring}
следует из равенства
\ShowEq{polylinear map skew symmetric, 1, division ring}
\end{proof}

\begin{theorem}
\label{theorem: coordinates of polylinear map, division ring over field}
Координаты полилинейного над полем $F$ отображения
\EqRef{polylinear map, division ring}
и его компоненты относительно базиса $\Basis e$
удовлетворяют равенству
\ShowEq{coordinates of polylinear map, division ring over field}
\end{theorem}
\begin{proof}
В равенстве \EqRef{polylinear map, division ring, standard representation}
положим
\ShowEq{coordinates of polylinear map, 1, division ring over field}
Тогда равенство \EqRef{polylinear map, division ring, standard representation}
примет вид
\ShowEq{polylinear map, division ring, standard representation, 1a}
Из равенства \EqRef{polylinear map over field, division ring}
следует
\ShowEq{polylinear map over field, division ring, 1a}
Равенство
\EqRef{coordinates of polylinear map, division ring over field}
следует из сравнения равенств
\EqRef{polylinear map, division ring, standard representation, 1a}
и
\EqRef{polylinear map over field, division ring}.
Равенство
\EqRef{coordinates of polylinear map, division ring over field, 1}
следует из сравнения равенств
\EqRef{polylinear map, division ring, standard representation, 1a}
и
\EqRef{polylinear map over field, division ring, 1a}.
\end{proof}


==> Second.Differential.English.tex <==
%auto-ignore

\input{Second.Differential.Eq}

\ifx\PrintBook\undefined
\else
\chapter{Derivative of Second Order of Map of Division Ring}
\label{chapter: Derivative of Second Order of Map of Division Ring}
\fi

\section{Derivative of Second Order of Map of Division Ring}

Let $D$ be valued division ring of characteristic $0$.
Let
\[f:D\rightarrow D\]
function differentiable in the G\^ateaux sense.
According to remark \ref{remark: differential L(D,D)}
the G\^ateaux derivative is map
\ShowEq{differential L(D,D)}
According to theorems
\ePrints{0812.4763,0908.3307}
\ifx\Semafor\ValueOn
\ref{theorem: sum of linear maps, division ring},
\ref{theorem: linear map times constant, division ring}
\else
\xRef{0701.238}{theorem: sum of linear maps, division ring},
\xRef{0701.238}{theorem: linear map times constant, division ring}
\fi
and definition \ref{definition: norm of map, division ring},
set $\mathcal L(D;D)$ is
normed $D$\Hyph vector space.
Therefore, we may consider the question,
if map $\partial f$ is differentiable in the G\^ateaux sense.

According to definition
\xRef{0812.4763}{definition: map differentiable in Gateaux sense, D vector space},
\ShowEq{Gateaux differential of map df, division ring}
where
\ShowEq{Gateaux differential of map df, division ring, o2}
is such continuous map, that
\ShowEq{Gateaux differential of map df, division ring, o2 lim}
According to definition
\xRef{0812.4763}{definition: map differentiable in Gateaux sense, D vector space},
map $\partial(\partial f(x)(a_1))(a_2)$
is linear map of variable $a_2$. From equation
\EqRef{Gateaux differential of map df, division ring},
it follows that map
$\partial(\partial f(x)(a_1))(a_2)$
is linear map of variable $a_1$.

\begin{definition}
\label{definition: Gateaux Differential of Second Order, division ring}
Polylinear map
\symb{\partial^2 f(x)}0{Gateaux derivative of Second Order}
\symb{\frac{\partial^2 f(x)}{\partial x^2}}
0{Gateaux derivative of Second Order, fraction, division ring}
\begin{equation}
\EqLabel{Gateaux derivative of Second Order, division ring}
\ShowSymbol{Gateaux derivative of Second Order}(a_1;a_2)
=\ShowSymbol{Gateaux derivative of Second Order, fraction, division ring}(a_1;a_2)
=\partial(\partial f(x)(a_1))(a_2)
\end{equation}
is called
\AddIndex{the G\^ateaux derivative of second order}
{Gateaux derivative of Second Order} of map $f$.
\qed
\end{definition}

\begin{remark}
\label{remark: differential L(D,D;D)}
According to definition
\ref{definition: Gateaux Differential of Second Order, division ring},
for given $x$ the G\^ateaux derivative of second order
\ShowEq{differential L(D,D;D), 1}.
Therefore, the G\^ateaux derivative of second order of map $f$ is map
\ShowEq{differential L(D,D;D)}
\end{remark}

\begin{theorem}
\label{theorem: Gateaux Differential of Second Order, division ring}
It is possible to represent
the G\^ateaux derivative of second order of map $f$
as
\ShowEq{Differential of Second Order, division ring, representation}
\end{theorem}
\begin{proof}
Corollary of definition \ref{definition: Gateaux Differential of Second Order, division ring}
and theorem
\ePrints{0812.4763}
\ifx\Semafor\ValueOn
\ref{theorem: polylinear map, D vector space}.
\else
\xRef{0701.238}{theorem: polylinear map, D vector space}.
\fi
\end{proof}

\begin{definition}
\begin{sloppypar}
Expression\footnote{We suppose
\ShowEq{component of Gateaux derivative of Second Order, 1, division ring}
}
\ShowEq{component of Gateaux derivative of Second Order, division ring}
is called
\AddIndex{component of the G\^ateaux derivative of second order}
{component of Gateaux derivative of Second Order} of map $f(x)$.
\qed
\end{sloppypar}
\end{definition}

By induction, assuming that we defined the G\^ateaux derivative
$\partial^{n-1} f(x)$ of order $n-1$, we define
\symb{\partial^n f(x)}
0{Gateaux derivative of Order n}
\symb{\frac{\partial^n f(x)}{\partial x^n}}
0{Gateaux derivative of Order n, fraction, division ring}
\begin{equation}
\EqLabel{Gateaux derivative of Order n, division ring}
\ShowSymbol{Gateaux derivative of Order n}(a_1;...;a_n)
=\ShowSymbol{Gateaux derivative of Order n, fraction, division ring}(a_1;...;a_n)
=\partial(\partial^{n-1} f(x)(a_1;...;a_{n-1}))(a_n)
\end{equation}
\AddIndex{the G\^ateaux derivative of order $n$}
{Gateaux derivative of Order n} of map $f$.
We also assume $\partial^0 f(x)=f(x)$.

\section{Taylor Series}
\label{section: Taylor Series}

Consider polynomial in one variable over division ring $D$ of power $n$, $n>0$. We
want to explore the structure of monomial $p_k(x)$ of polynomial of power $k$.

It is evident that monomial of power $0$ has form $a_0$, $a_0\in D$.
Let $k>0$. Let us prove that
\[
p_k(x)=p_{k-1}(x)xa_k
\]
where $a_k\in D$.
Actually, last factor of monomial $p_k(x)$ is either $a_k\in D$,
or has form $x^l$, $l\ge 1$.
In the later case we assume $a_k=1$.
Factor preceding $a_k$ has form $x^l$, $l\ge 1$.
We can represent this factor as $x^{l-1}x$.
Therefore, we proved the statement.

In particular, monomial of power $1$ has form $p_1(x)=a_0xa_1$.

Without loss of generality, we assume $k=n$.

\begin{theorem}
\label{theorem: Gateaux derivative of f(x)x, division ring}
For any $m>0$ the following equation is true
\begin{align}
&\partial^m (f(x)x)(h_1;...;h_m)
\nonumber \\
=&\partial^m f(x)(h_1;...;h_m)x
+\partial^{m-1} f(x)(h_1;...;h_{m-1})h_m
\EqLabel{Gateaux derivative of f(x)x, division ring}
\\ \nonumber
+&\partial^{m-1} f(x)(\widehat{h_1};...;h_{m-1};h_m)h_1
+...
\\ \nonumber
+&\partial^{m-1} f(x)(h_1;...;\widehat{h_{m-1}};h_m)h_{m-1}
\end{align}
where symbol $\widehat{h^i}$ means absense of variable $h^i$ in the list.
\end{theorem}
\begin{proof}
For $m=1$, this is corollary  of equation
\EqRef{Gateaux derivative of product, division ring}
\[
\partial (f(x)x)(h_1)=\partial f(x)(h_1)x+
f(x)h_1
\]
Assume, \EqRef{Gateaux derivative of f(x)x, division ring} is true
for $m-1$. Then
\begin{align}
&\partial^{m-1} (f(x)x)(h_1;...;h_{m-1})
\nonumber \\
=&\partial^{m-1} f(x)(h_1;...;h_{m-1})x
+\partial^{m-2} f(x)(h_1;...;h_{m-2})h_{m-1}
\EqLabel{Gateaux derivative of f(x)x, m-1, division ring}
\\ \nonumber
+&\partial^{m-2} f(x)(\widehat{h_1},...,h_{m-2},h_{m-1})h_1
+...
\\ \nonumber
+&\partial^{m-2} f(x)(h_1,...,\widehat{h_{m-2}},h_{m-1})h_{m-2}
\end{align}
Using equations \EqRef{Gateaux derivative of product, division ring}
and \EqRef{Gateaux differential, product over constant, division ring}
we get
\begin{align}
&\partial^m (f(x)x)(h_1;...;h_{m-1};h_m)
\nonumber \\
=&\partial^m f(x)(h_1;...;h_{m-1};h_m)x
+\partial^{m-1} f(x)(h_1;...;h_{m-2};h_{m-1})h_m
\nonumber \\
+&\partial^{m-1} f(x)(h_1;...;h_{m-2};\widehat{h_{m-1}};h_m)h_{m-1}
\EqLabel{Gateaux derivative of f(x)x, m, division ring}
\\ \nonumber
+&\partial^{m-2} f(x)(\widehat{h_1},...,h_{m-2},h_{m-1};h_m)h_1
+...
\\ \nonumber
+&\partial^{m-2} f(x)(h_1,...,\widehat{h_{m-2}},h_{m-1};h_m)h_{m-2}
\end{align}
The difference between
equations \EqRef{Gateaux derivative of f(x)x, division ring} and
\EqRef{Gateaux derivative of f(x)x, m, division ring}
is only in form of presentation.
We proved the theorem.
\end{proof}

\begin{theorem}
\label{theorem: Gateaux derivative of pn is symmetric, m less than n, division ring}
The G\^ateaux derivative $\partial^m p_n(x)(h_1,...,h_m)$
is symmetric polynomial with respect to variables $h_1$, ..., $h_m$.
\end{theorem}
\begin{proof}
To prove the theorem we consider algebraic properties
of the G\^ateaux derivative and give equivalent definition.
We start from construction of monomial.
For any monomial $p_n(x)$ we build symmetric
polynomial $r_n(x)$ according to following rules
\begin{itemize}
\item If $p_1(x)=a_0xa_1$, then $r_1(x_1)=a_0x_1a_1$
\item If $p_n(x)=p_{n-1}(x)a_n$, then
\[
r_n(x_1,...,x_n)=r_{n-1}(x_{[1},...,x_{n-1})x_{n]}a_n
\]
where square brackets express symmetrization of expression
with respect to variables $x_1$, ..., $x_n$.
\end{itemize}
It is evident that
\[
p_n(x)=r_n(x_1,...,x_n)\ \ \ x_1=...=x_n=x
\]
We define the G\^ateaux derivative of power $k$ according to rule
\begin{equation}
\partial^k p_n(x)(h_1,...,h_k)=r_n(h_1,...,h_k,x_{k+1},...,x_n)\ \ \ x_{k+1}=x_n=x
\EqLabel{Gateaux derivative of monomial, algebraic definition, division ring}
\end{equation}
According to construction, polynomial $r_n(h_1,...,h_k,x_{k+1},...,x_n)$
is symmetric with respect to variables $h_1$, ..., $h_k$, $x_{k+1}$, ..., $x_n$.
Therefore, polynomial
\EqRef{Gateaux derivative of monomial, algebraic definition, division ring}
is symmetric with respect to variables $h_1$, ..., $h_k$.

For $k=1$, we will prove that definition
\EqRef{Gateaux derivative of monomial, algebraic definition, division ring}
of the G\^ateaux derivative coincides with definition
\EqRef{Gateaux Dstar derivative, division ring}.

For $n=1$, $r_1(h_1)=a_0h_1a_1$. This expression coincides
with expression of the G\^ateaux derivative in theorem
\ref{theorem: Gateaux differential, product over constant, fx=x, division ring}.

Let the statement be true for $n-1$.
The following equation is true
\begin{equation}
r_n(h_1,x_2,...,x_n)=r_{n-1}(h_1,x_{[2},...,x_{n-1})x_{n]}a_n+r_{n-1}(x_2,...,x_n)h_1a_n
\EqLabel{Gateaux derivative of monomial, n, division ring}
\end{equation}
Assume $x_2=...=x_n=x$. 
According to suggestion of induction, from equations
\EqRef{Gateaux derivative of monomial, algebraic definition, division ring},
\EqRef{Gateaux derivative of monomial, n, division ring}
it follows that
\[
r_n(h_1,x_2,...,x_n)=\partial p_{n-1}(x)(h_1)xa_n+p_{n-1}(x)h_1a_n
\]

According to theorem
\ref{theorem: Gateaux derivative of f(x)x, division ring}
\[
r_n(h_1,x_2,...,x_n)=\partial p_n(x)(h_1)
\]
This proves the equation
\EqRef{Gateaux derivative of monomial, algebraic definition, division ring}
for $k=1$.

Let us prove now that definition
\EqRef{Gateaux derivative of monomial, algebraic definition, division ring}
of the G\^ateaux derivative coincides with definition
\EqRef{Gateaux derivative of Order n, division ring} for $k>1$.

Let equation
\EqRef{Gateaux derivative of monomial, algebraic definition, division ring}
be true for $k-1$.
Consider arbitrary monomial of polynomial $r_n(h_1,...,h_{k-1},x_k,...,x_n)$.
Identifying variables $h_1$, ..., $h_{k-1}$
with elements of division ring $D$, we consider polynomial
\begin{equation}
R_{n-k}(x_k,...,x_n)=r_n(h_1,...,h_{k-1},x_k,...,x_n)
\EqLabel{reduced polynom, division ring}
\end{equation}
Assume $P_{n-k}(x)=R_{n-k}(x_k,...,x_n)$, $x_k=...=x_n=x$.
Therefore
\[
P_{n-k}(x)=\partial^{k-1} p_n(x)(h_1;...;h_{k-1})
\]
According to definition of the G\^ateaux derivative
\EqRef{Gateaux derivative of Order n, division ring}
\begin{align}
\partial P_{n-k}(x)(h_k)
=&\partial(\partial^{k-1} p_n(x)(h_1;...;h_{k-1}))(h_k)
\nonumber\\
=&\partial^k p_n(x)(h_1;...;h_{k-1};h_k)
\EqLabel{Gateaux derivative of Order n, 1, division ring}
\end{align}
According to definition
\EqRef{Gateaux derivative of monomial, algebraic definition, division ring}
of the G\^ateaux derivative
\begin{equation}
\partial P_{n-k}(x)(h_k)=R_{n-k}(h_k,x_{k+1},...,x_n)\ \ \ x_{k+1}=x_n=x
\EqLabel{Gateaux derivative of monomial, algebraic definition, 1, division ring}
\end{equation}
According to definition \EqRef{reduced polynom, division ring},
from equation
\EqRef{Gateaux derivative of monomial, algebraic definition, 1, division ring}
it follows that
\begin{equation}
\partial P_{n-k}(x)(h_k)=r_n(h_1,...,h_k,x_{k+1},...,x_n)\ \ \ x_{k+1}=x_n=x
\EqLabel{Gateaux derivative of monomial, algebraic definition, 2, division ring}
\end{equation}
From comparison of equations \EqRef{Gateaux derivative of Order n, 1, division ring}
and \EqRef{Gateaux derivative of monomial, algebraic definition, 2, division ring}
it follows that
\[
\partial^k p_n(x)(h_1;...;h_k)=r_n(h_1,...,h_k,x_{k+1},...,x_n)\ \ \ x_{k+1}=x_n=x
\]
Therefore equation
\EqRef{Gateaux derivative of monomial, algebraic definition, division ring}
is true for any $k$ and $n$.

We proved the statement of theorem.
\end{proof}

\begin{theorem}
\label{theorem: Gateaux derivative of pn equal 0, division ring}
For any $n\ge 0$ following equation is true
\begin{equation}
\EqLabel{Gateaux derivative n1 of pn, division ring}
\partial^{n+1} p_n(x)(h_1;...;h_{n+1})=0
\end{equation}
\end{theorem}
\begin{proof}
Since $p_0(x)=a_0$, $a_0\in D$, then for $n=0$ theorem is corollary
of theorem \ref{theorem: Gateaux differential of const, division ring}.
Let statement of theorem is true for $n-1$. According to theorem
\ref{theorem: Gateaux derivative of f(x)x, division ring}
when $f(x)=p_{n-1}(x)$ we get
\begin{align*}
\partial^{n+1} p_n(x)(h_1;...;h_{n+1})
=&\partial^{n+1}(p_{n-1}(x)xa_n)(h_1;...;h_{n+1})
\\
=&\partial^{n+1} p_{n-1}(x)(h_1;...;h_m)xa_n
\\
+&\partial^n p_{n-1}(x)(h_1;...;h_{m-1})h_ma_n
\\
+&\partial^n p_{n-1}(x)(\widehat{h_1};...;h_{m-1};h_m)h_1a_n
+...
\\
+&\partial^{m-1} p_{n-1}(x)(h_1;...;\widehat{h_{m-1}};h_m)h_{m-1}a_n
\end{align*}
According to suggestion of induction all monomials are equal $0$.
\end{proof}

\begin{theorem}
\label{theorem: Gateaux derivative of pn equal 0, m less than n, division ring}
If $m<n$, then following equation is true
\begin{equation}
\partial^m p_n(0)(h)=0
\EqLabel{m Gateaux derivative of polinom pn, division ring}
\end{equation}
\end{theorem}
\begin{proof}
For $n=1$ following equation is true
\[
\partial^0 p_1(0)=a_0xa_1=0
\]
Assume that statement is true
for $n-1$. Then according to theorem \ref{theorem: Gateaux derivative of f(x)x, division ring}
\begin{align*}
&\partial^m (p_{n-1}(x)xa_n)(h_1;...;h_m)
\\
=&\partial^m p_{n-1}(x)(h_1;...;h_m)xa_n
+\partial^{m-1} p_{n-1}(x)(h_1;...;h_{m-1})h_ma_n
\\
+&\partial^{m-1} p_{n-1}(x)(\widehat{h_1};...;h_{m-1};h_m)h_1a_n
+...
\\
+&\partial^{m-1} p_{n-1}(x)(h_1;...;\widehat{h_{m-1}};h_m)h_{m-1}a_n
\end{align*}
First term equal $0$ because $x=0$.
Because $m-1<n-1$, then
rest terms equal $0$ according to suggestion of induction.
We proved the statement of theorem.
\end{proof}

When $h_1=...=h_n=h$, we assume
\[
\partial^nf(x)(h)=\partial^nf(x)(h_1;...;h_n)
\]
This notation does not create ambiguity, because we can determine function
according to number of arguments.

\begin{theorem}
\label{theorem: n Gateaux derivative of polinom pn, division ring}
For any $n>0$ following equation is true
\begin{equation}
\partial^n p_n(x)(h)=n!p_n(h)
\EqLabel{n Gateaux derivative of polinom pn, division ring}
\end{equation}
\end{theorem}
\begin{proof}
For $n=1$ following equation is true
\[
\partial p_1(x)(h)=\partial (a_0xa_1)(h)=a_0ha_1=1!p_1(h)
\]
Assume the statement is true
for $n-1$. Then according to theorem \ref{theorem: Gateaux derivative of f(x)x, division ring}
\begin{align}
\EqLabel{n Gateaux derivative of polinom pn, 1, division ring}
\partial^n p_n(x)(h)
=&\partial^n p_{n-1}(x)(h)xa_n
+\partial^{n-1} p_{n-1}(x)(h)ha_n
\\ \nonumber
+&...
+\partial^{n-1} p_{n-1}(x)(h)ha_n
\end{align}
First term equal $0$ according to theorem
\ref{theorem: Gateaux derivative of pn equal 0, division ring}.
The rest $n$ terms equal, and according to suggestion of induction
from equation \EqRef{n Gateaux derivative of polinom pn, 1, division ring}
it follows
\[
\partial^n p_n(x)(h)
=n\partial^{n-1} p_{n-1}(x)(h)ha_n=n(n-1)!p_{n-1}(h)ha_n=n!p_n(h)
\]
Therefore, statement of theorem is true for any $n$.
\end{proof}

Let $p(x)$ be polynomial of power $n$.\footnote{I consider
Taylor polynomial for polynomials by analogy with
construction of Taylor polynomial in \citeBib{Fihtengolts: Calculus volume 1}, p. 246.}
\[
p(x)=p_0+p_{1i_1}(x)+...+p_{ni_n}(x)
\]
We assume sum by index $i_k$ which enumerates terms
of power $k$.
According to theorem \ref{theorem: Gateaux derivative of pn equal 0, division ring},
\ref{theorem: Gateaux derivative of pn equal 0, m less than n, division ring},
\ref{theorem: n Gateaux derivative of polinom pn, division ring}
\ShowEq{dp(0)(x)}
Therefore, we can write
\[
p(x)=p_0+(1!)^{-1}\partial p(0)(x)+(2!)^{-1}\partial^2 p(0)(x)+...+(n!)^{-1}\partial^n p(0)(x)
\]
This representation of polynomial is called
\AddIndex{Taylor polynomial}{Taylor polynomial, division ring}.
If we consider substitution of variable $x=y-y_0$, then considered above construction
remain true for polynomial
\[
p(y)=p_0+p_{1i_1}(y-y_0)+...+p_{ni_n}(y-y_0)
\]
Therefore
\[
p(y)=p_0+(1!)^{-1}\partial p(y_0)(y-y_0)+(2!)^{-1}\partial^2 p(y_0)(y-y_0)+...+(n!)^{-1}\partial^n p(y_0)(y-y_0)
\]

Assume that function $f(x))$ is differentiable in the G\^ateaux sense at point $x_0$
up to any order.\footnote{I explore
construction of Taylor series by analogy with
construction of Taylor series in \citeBib{Fihtengolts: Calculus volume 1}, p. 248, 249.}

\begin{theorem}
\label{theorem: n Gateaux derivative equal 0, division ring}
If function $f(x)$ holds
\begin{equation}
f(x_0)=\partial f(x_0)(h)=...=\partial^n f(x_0)(h)=0
\EqLabel{n Gateaux derivatives of function, division ring}
\end{equation}
then for $t\rightarrow 0$ expression $f(x+th)$ is infinitesimal of order
higher then $n$ with respect to $t$
\[
f(x_0+th)=o(t^n)
\]
\end{theorem}
\begin{proof}
When $n=1$ this statement follows from equation
\EqRef{Gateaux differential of map, t, division ring}.

Let statement be true for $n-1$.
Map
\[
f_1(x)=\partial f(x)(h)
\]
satisfies to condition
\[
f_1(x_0)=\partial f_1(x_0)(h)=...=\partial^{n-1} f_1(x_0)(h)=0
\]
According to suggestion of induction
\[
f_1(x_0+th)=o(t^{n-1})
\]
Then equation \EqRef{Gateaux derivative, representation, 2}
gets form
\[
o(t^{n-1})=\lim_{t\rightarrow 0,\ t\in R}(t^{-1}f(x+th))
\]
Therefore,
\[
f(x+th)=o(t^n)
\]
\end{proof}

Let us form polynomial
\begin{equation}
\EqLabel{Taylor polynomial, f(x), division ring}
p(x)=f(x_0)+(1!)^{-1}\partial f(x_0)(x-x_0)+...+(n!)^{-1}\partial^n f(x_0)(x-x_0)
\end{equation}
According to theorem \ref{theorem: n Gateaux derivative equal 0, division ring}
\[
f(x_0+t(x-x_0))-p(x_0+t(x-x_0))=o(t^n)
\]
Therefore, polynomial $p(x)$ is good approximation of map $f(x)$.

If map $f(x)$ has the G\^ateaux derivative of any order, the passing to the limit
$n\rightarrow\infty$, we get expansion into series
\[
f(x)=\sum_{n=0}^{\infty}(n!)^{-1}\partial^n f(x_0)(x-x_0)
\]
which is called \AddIndex{Taylor series}{Taylor series, division ring}.

\section{Integral}

Concept of integral has different aspect. In this section we consider
integration as operation inverse to differentiation.
As a matter of fact, we consider procedure of solution of ordinary differential
equation
\[
\partial f(x)(h)=F(x;h)
\]

\begin{example}
I start from example of differential equation over real field.
\begin{equation}
\EqLabel{differential equation y=xx, 1, real number}
y'=3x^2
\end{equation}
\begin{equation}
\EqLabel{differential equation y=xx, initial, real number}
\begin{matrix}
x_0=0&y_0=0
\end{matrix}
\end{equation}
Differentiating one after another equation \EqRef{differential equation y=xx, 1, real number},
we get the chain of equations
\begin{align}
\EqLabel{differential equation y=xx, 2, real number}
y''&=6x
\\
\EqLabel{differential equation y=xx, 3, real number}
y'''&=6
\\
\EqLabel{differential equation y=xx, 4, real number}
y^{(n)}&=0&n&>3
\end{align}
From equations
\EqRef{differential equation y=xx, 1, real number},
\EqRef{differential equation y=xx, initial, real number},
\EqRef{differential equation y=xx, 2, real number},
\EqRef{differential equation y=xx, 3, real number},
\EqRef{differential equation y=xx, 4, real number}
it follows expansion into Taylor series
\[
y=x^3
\]
\qed
\end{example}

\begin{example}
Consider similar differential equation over division ring
\begin{equation}
\EqLabel{differential equation y=xx, 1, division ring}
\partial (y)(h)=hx^2+xhx+x^2h
\end{equation}
\begin{equation}
\EqLabel{differential equation y=xx, initial, division ring}
\begin{matrix}
x_0=0&y_0=0
\end{matrix}
\end{equation}
Differentiating one after another equation
\EqRef{differential equation y=xx, 1, division ring},
we get the chain of equations
\ShowEq{differential equation y=xx, division ring}
From equations
\EqRef{differential equation y=xx, 1, division ring},
\EqRef{differential equation y=xx, initial, division ring},
\EqRef{differential equation y=xx, 2, division ring},
\EqRef{differential equation y=xx, 3, division ring},
\EqRef{differential equation y=xx, 4, division ring}
expansion into Taylor series follows
\[
y=x^3
\]
\qed
\end{example}

\begin{remark}
Differential equation
\begin{equation}
\EqLabel{differential equation y=xx, 1, a, division ring}
\partial (y)(h)=3hx^2
\end{equation}
\begin{equation}
\EqLabel{differential equation y=xx, initial, a, division ring}
\begin{matrix}
x_0=0&y_0=0
\end{matrix}
\end{equation}
also leads to answer $y=x^3$. it is evident that this
map does not satisfies differential equation.
However, contrary to theorem
\ref{theorem: Gateaux derivative of pn is symmetric, m less than n, division ring}
second derivative is
not symmetric polynomial. This means that
equation \EqRef{differential equation y=xx, 1, a, division ring}
does not possess a solution.
\qed
\end{remark}

\begin{example}
\label{example: differential equation, additive function, division ring}
It is evident that, if function satisfies to differential equation
\ShowEq{differential equation, additive function, division ring}
then The G\^ateaux derivative of second order
\[
\partial^2 f(x)(h_1;h_2)=0
\]
In that case, if initial condition is $y(0)=0$,
then differential equation
\EqRef{differential equation, additive function, division ring} has solution
\ShowEq{differential equation, additive function, solution, division ring}
\qed
\end{example}

\section{Exponent}

In this section we consider one of possible models
of exponent.

In a field we can define exponent as solution of differential equation
\ShowEq{exponent over field}
It is evident that we cannot write such equation for division ring.
However we can use equation
\ShowEq{derivative over field}
From equations
\EqRef{exponent over field}, \EqRef{derivative over field}
it follows
\ShowEq{exponent derivative over field}
This equation is closer to our goal,
however there is the question: in which order
we should multiply $y$ and $h$?
To answer this question we change equation
\ShowEq{exponent derivative over division ring}
Hence, our goal is to solve differential equation
\EqRef{exponent derivative over division ring}
with initial condition $y(0)=1$.

For the statement and proof of the theorem
\ref{theorem: exponent derivative n over division ring}
I introduce following notation.
Let
\ShowEq{exponent derivative, transposition n}
be transposition of the tuple of variables
\ShowEq{exponent transposition tuple 1}
Let $p_{\sigma}(h_i)$ be position that
variable $h_i$ gets in the tuple
\ShowEq{exponent transposition tuple 2}
For instance, if transposition $\sigma$ has form
\ShowEq{exponent transposition tuple 3}
then following tuples equal
\ShowEq{exponent transposition tuple 4}

\begin{theorem}
\label{theorem: exponent derivative n over division ring}
If function $y$ is solution of differential equation
\EqRef{exponent derivative over division ring}
then the G\^ateaux derivative of order $n$ of function $y$
has form
\ShowEq{exponent derivative n over division ring}
where sum is over transpositions
\ShowEq{exponent derivative, transposition n}
of the set of variables $y$, $h_1$, ..., $h_n$.
Transposition $\sigma$ has following properties
\begin{enumerate}
\item If there exist $i$, $j$, $i\ne j$, such that
$p_{\sigma}(h_i)$ is situated in product
\EqRef{exponent derivative n over division ring}
on the left side of $p_{\sigma}(h_j)$ and $p_{\sigma}(h_j)$ is situated
on the left side of $p_{\sigma}(y)$, then $i<j$.
\label{enumerate: exponent derivative, transposition n, left}
\item If there exist $i$, $j$, $i\ne j$, such that
$p_{\sigma}(h_i)$ is situated in product
\EqRef{exponent derivative n over division ring}
on the right side of $p_{\sigma}(h_j)$ and $p_{\sigma}(h_j)$ is situated
on the right side of $p_{\sigma}(y)$, then $i>j$.
\label{enumerate: exponent derivative, transposition n, right}
\end{enumerate}
\end{theorem}
\begin{proof}
We prove this statement by induction.
For $n=1$ the statement is true because this is differential equation
\EqRef{exponent derivative over division ring}.
Let the statement be true for $n=k-1$.
Hence
\ShowEq{exponent derivative n=k-1 over division ring}
where the sum is over transposition
\ShowEq{exponent derivative, transposition n=k-1}
of the set of variables $y$, $h_1$, ..., $h_{k-1}$.
Transposition $\sigma$ satisfies to conditions
\eqref{enumerate: exponent derivative, transposition n, left},
\eqref{enumerate: exponent derivative, transposition n, right}
in theorem.
According to definition
\EqRef{Gateaux derivative of Order n, division ring}
the G\^ateaux derivative of order $k$ has form
\ShowEq{exponent derivative n=k over division ring, 1}
From equations
\EqRef{exponent derivative over division ring},
\EqRef{exponent derivative n=k over division ring, 1}
it follows that
\ShowEq{exponent derivative n=k over division ring, 2}
It is easy to see that arbitrary transposition $\sigma$
from sum
\EqRef{exponent derivative n=k over division ring, 2}
forms two transpositions
\ShowEq{exponent derivative, transposition n=k}
From \EqRef{exponent derivative n=k over division ring, 2}
and \EqRef{exponent derivative, transposition n=k}
it follows that
\ShowEq{exponent derivative n=k over division ring, 3}
In expression
\EqRef{exponent derivative n=k over division ring, 3}
$p_{\tau_1}(h_k)$ is written immediately before $p_{\tau_1}(y)$.
Since $k$ is smallest value of index
then transposition $\tau_1$ satisfies to conditions
\eqref{enumerate: exponent derivative, transposition n, left},
\eqref{enumerate: exponent derivative, transposition n, right}
in the theorem.
In expression
\EqRef{exponent derivative n=k over division ring, 3}
$p_{\tau_2}(h_k)$ is written immediately after $p_{\tau_2}(y)$.
Since $k$ is largest value of index
then transposition $\tau_2$ satisfies to conditions
\eqref{enumerate: exponent derivative, transposition n, left},
\eqref{enumerate: exponent derivative, transposition n, right}
in the theorem.

It remains to show that in the expression
\EqRef{exponent derivative n=k over division ring, 3}
we get all transpositions $\tau$ that satisfy to conditions
\eqref{enumerate: exponent derivative, transposition n, left},
\eqref{enumerate: exponent derivative, transposition n, right}
in the theorem.
Since $k$ is largest index then according to conditions
\eqref{enumerate: exponent derivative, transposition n, left},
\eqref{enumerate: exponent derivative, transposition n, right}
in the theorem $\tau(h_k)$
is written either immediately before or immediately after $\tau(y)$.
Therefore, any transposition $\tau$ has
either form $\tau_1$ or form $\tau_2$.
Using equation
\EqRef{exponent derivative, transposition n=k},
we can find corresponding
transposition $\sigma$ for given transposition $\tau$.
Therefore, the statement of theorem is true for $n=k$.
We proved the theorem.
\end{proof}

\begin{theorem}
The solution of differential equation
\EqRef{exponent derivative over division ring}
with initial condition $y(0)=1$
is exponent
\ShowEq{exponent over division ring}
that has following Taylor series expansion
\ShowEq{exponent Taylor series over division ring}
\end{theorem}
\begin{proof}
The G\^ateaux derivative of order $n$ has $2^n$ items.
In fact, the G\^ateaux derivative of order $1$ has $2$ items,
and each differentiation increase number of items twice.
From initial condition $y(0)=1$ and theorem
\ref{theorem: exponent derivative n over division ring}
it follows that the G\^ateaux derivative of order $n$
of required solution has form
\ShowEq{exponent derivative n over division ring, x=0}
Taylor series expansion
\EqRef{exponent Taylor series over division ring}
follows
from equation
\EqRef{exponent derivative n over division ring, x=0}.
\end{proof}

\begin{theorem}
\label{theorem: exponent of sum}
The equation
\ShowEq{exponent of sum}
is true iff
\ShowEq{exponent of sum, 1}
\end{theorem}
\begin{proof}
To prove the theorem it is enough to consider Taylor series
\ShowEq{exponent a b a+b}
Let us multiply expressions
\EqRef{exponent a} and \EqRef{exponent b}.
The sum of monomials of order $3$ has form
\ShowEq{exponent ab 3}
and in general does not equal expression
\ShowEq{exponent a+b 3}
The proof of statement that \EqRef{exponent of sum} follows from
\EqRef{exponent of sum, 1}
is trivial.
\end{proof}

The meaning of the theorem \ref{theorem: exponent of sum}
becomes more clear if we recall that there exist two
models of design of exponent. First model is
the solution of differential equation
\EqRef{exponent derivative over division ring}.
Second model is exploring of one parameter group of transformations.
For field both models lead to the same function.
I cannot state this now for general case. This is the subject of separate
research. However if we recall that quaternion is analogue
of transformation of three dimensional space then the statement of the theorem
becomes evident.


==> Second.Differential.Eq.tex <==
%auto-ignore

\DefEq
{
$o_2:D\rightarrow \mathcal L(D;D)$
}
{Gateaux differential of map df, division ring, o2}

\DefEq
{
\[
\frac{\partial_{s\cdot p}^2 f(x)}{\partial x^2}
=\frac{\partial_{s\cdot p}^2 f(x)}{\partial x\partial x}
\]
}
{component of Gateaux derivative of Second Order, 1, division ring}

\DefEq
{
\[
\lim_{a_2\rightarrow 0}\frac{\|o_2(a_2)\|}{|a_2|}=0
\]
}
{Gateaux differential of map df, division ring, o2 lim}

\DefEq
{
$\partial^2 f(x)\in\mathcal L(D,D;D)$%
}
{differential L(D,D;D), 1}

\DefEq
{
\[
\partial^2 f:D\rightarrow \mathcal L(D,D;D)
\]
}
{differential L(D,D;D)}

\DefEquation
{
\partial^2 f(x)(a_1;a_2)
=\frac{\partial^2_{s\cdot 0} f(x)}{\partial x^2}
\sigma_s(a_1)
\frac{\partial^2_{s\cdot 1} f(x)}{\partial x^2}
\sigma_s(a_2)
\frac{\partial^2_{s\cdot 2} f(x)}{\partial x^2}
}
{Differential of Second Order, division ring, representation}

\DefEq
{
\[
\partial^k p(0)(x)=k!p_{ki_k}(x)
\]
}
{dp(0)(x)}

\DefEq
{
\symb{\frac{\partial^2_{s\cdot p} f(x)}{\partial x^2}}0
{component of Gateaux derivative of Second Order}
$\displaystyle
\ShowSymbol{component of Gateaux derivative of Second Order}$,
$p=0$, $1$, $2$,
}
{component of Gateaux derivative of Second Order, division ring}

\DefEq
{
\begin{align}
\EqLabel{differential equation y=xx, 2, division ring}
&\partial^2 (y)(h_1;h_2)
\\ \nonumber
=&h_1h_2x+h_1xh_2
+h_2h_1x+xh_1h_2+h_2xh_1+xh_2h_1
\\
\EqLabel{differential equation y=xx, 3, division ring}
&\partial^3 (y)(h_1;h_2;h_3)
\\ \nonumber
=&h_1h_2h_3+h_1h_3h_2
+h_2h_1h_3+h_3h_1h_2+h_2h_3h_1+h_3h_2h_1
\\
\EqLabel{differential equation y=xx, 4, division ring}
&\partial^n (y)(h_1;...;h_n)=0\ \ \ n>3
\end{align}
}
{differential equation y=xx, division ring}

\DefEquation
{
\partial (y)(h)=f_{s\cdot 0}\ h\ f_{s\cdot 1}
}
{differential equation, additive function, division ring}

\DefEq
{
\[
y=f_{s\cdot 0} x f_{s\cdot 1}
\]
}
{differential equation, additive function, solution, division ring}

\DefEquation
{
y'=y
}
{exponent over field}

\DefEquation
{
\partial(y)(h)=y'h
}
{derivative over field}

\DefEquation
{
\partial(y)(h)=yh
}
{exponent derivative over field}

\DefEquation
{
\partial(y)(h)=\frac 12(yh+hy)
}
{exponent derivative over division ring}

\DefEq
{
\[
\sigma=
\begin{pmatrix}
y&h_1&...&h_n
\\
\sigma(y)&\sigma(h_1)&...&\sigma(h_n)
\end{pmatrix}
\]
}
{exponent derivative, transposition n}

\DefEq
{
\[
\begin{pmatrix}
y&h_1&...&h_n
\end{pmatrix}
\]
}
{exponent transposition tuple 1}

\DefEq
{
\[
\begin{pmatrix}
\sigma(y)&\sigma(h_1)&...&\sigma(h_n)
\end{pmatrix}
\]
}
{exponent transposition tuple 2}

\DefEq
{
\[
\begin{pmatrix}
y&h_1&h_2&h_3
\\
h_2&y&h_3&h_1
\end{pmatrix}
\]
}
{exponent transposition tuple 3}

\DefEq
{
\begin{align*}
\begin{pmatrix}
\sigma(y)&\sigma(h_1)&\sigma(h_2)&\sigma(h_3)
\end{pmatrix}
=&
\begin{pmatrix}
h_2&y&h_3&h_1
\end{pmatrix}
\\
=&
\begin{pmatrix}
p_{\sigma}(h_2)&p_{\sigma}(y)&p_{\sigma}(h_3)&p_{\sigma}(h_1)
\end{pmatrix}
\end{align*}
}
{exponent transposition tuple 4}

\DefEquation
{
\partial^n(y)(h_1,...,h_n)=\frac 1{2^n}
\sum_{\sigma} \sigma(y)\sigma(h_1) ... \sigma(h_n)
}
{exponent derivative n over division ring}

\DefEquation
{
\partial^{k-1}(y)(h_1,...,h_{k-1})=\frac 1{2^{k-1}}
\sum_{\sigma} \sigma(y)\sigma(h_1) ... \sigma(h_{k-1})
}
{exponent derivative n=k-1 over division ring}

\DefEq
{
\[
\sigma=
\begin{pmatrix}
y&h_1&...&h_{k-1}
\\
\sigma(y)&\sigma(h_1)&...&\sigma(h_{k-1})
\end{pmatrix}
\]
}
{exponent derivative, transposition n=k-1}

\DefEq
{
\begin{align}
\partial^k(y)(h_1,...,h_k)
=&\partial(\partial^{k-1}(y)(h_1,...,h_{k-1}))(h_k)
\nonumber
\\
=&\frac 1{2^{k-1}}\partial
\left(
\sum_{\sigma} \sigma(y)\sigma(h_1) ... \sigma(h_{k-1})
\right)
(h_k)
\EqLabel{exponent derivative n=k over division ring, 1}
\end{align}
}
{exponent derivative n=k over division ring, 1}

\DefEq
{
\begin{align}
&\partial^k(y)(h_1,...,h_k)
\nonumber
\\
=&\frac 1{2^{k-1}}\frac 12
\left(
\sum_{\sigma} \sigma(yh_k)\sigma(h_1) ... \sigma(h_{k-1})
+
\sum_{\sigma} \sigma(h_ky)\sigma(h_1) ... \sigma(h_{k-1})
\right)
\EqLabel{exponent derivative n=k over division ring, 2}
\end{align}
}
{exponent derivative n=k over division ring, 2}

\DefEquation
{
\begin{array}{rl}
\tau_1
&=
\begin{pmatrix}
y&h_1&...&h_{k-1}&h_k
\\
\tau_1(y)&\tau_1(h_1)&...&\tau_1(h_{k-1})&\tau_1(h_k)
\end{pmatrix}
\\
&=
\begin{pmatrix}
h_ky&h_1&...&h_{k-1}&
\\
\sigma(h_ky)&\sigma(h_1)&...&\sigma(h_{k-1})
\end{pmatrix}
\\
\tau_2
&=
\begin{pmatrix}
y&h_1&...&h_{k-1}&h_k
\\
\tau_2(y)&\tau_2(h_1)&...&\tau_2(h_{k-1})&\tau_2(h_k)
\end{pmatrix}
\\
&=
\begin{pmatrix}
yh_k&h_1&...&h_{k-1}&
\\
\sigma(yh_k)&\sigma(h_1)&...&\sigma(h_{k-1})
\end{pmatrix}
\end{array}
}
{exponent derivative, transposition n=k}

\DefEq
{
\begin{align}
&\partial^k(y)(h_1,...,h_k)
\nonumber
\\
=&\frac 1{2^k}
\Bigg(
\sum_{\tau_1} \tau_1(y)\tau_1(h_1) ... \tau_1(h_{k-1})\tau_1(h_k)
\EqLabel{exponent derivative n=k over division ring, 3}
\\
+&
\sum_{\tau_2} \tau_2(y)\tau_2(h_1) ... \tau_2(h_{k-1})\tau_2(h_k)
\Bigg)
\nonumber
\end{align}
}
{exponent derivative n=k over division ring, 3}

\DefEq
{
$y=e^x$
}
{exponent over division ring}

\DefEquation
{
e^x=\sum_{n=0}^{\infty}
\frac 1{n!}x^n
}
{exponent Taylor series over division ring}

\DefEquation
{
\partial^n(y(0))(h,...,h)=1
}
{exponent derivative n over division ring, x=0}

\DefEquation
{
e^{a+b}=e^ae^b
}
{exponent of sum}

\DefEquation
{
ab=ba
}
{exponent of sum, 1}

\DefEq
{
\begin{align}
e^a&=\sum_{n=0}^{\infty}\frac 1{n!}a^n
\EqLabel{exponent a}
\\
e^b&=\sum_{n=0}^{\infty}\frac 1{n!}b^n
\EqLabel{exponent b}
\\
e^{a+b}&=\sum_{n=0}^{\infty}\frac 1{n!}(a+b)^n
\EqLabel{exponent a+b}
\end{align}
}
{exponent a b a+b}

\DefEquation
{
\frac 16a^3+\frac 12a^2b+\frac 12ab^2+\frac 16b^3
}
{exponent ab 3}

\DefEquation
{
\frac 16(a+b)^3=\frac 16a^3+\frac 16a^2b+\frac 16aba+\frac 16ba^2
+\frac 16ab^2+\frac 16bab+\frac 16b^2a+\frac 16b^3
}
{exponent a+b 3}

\DefEquation
{
\partial f(x+a_2)(a_1)-\partial f(x)(a_1)
=\partial(\partial f(x)(a_1))(a_2)
+o_2(a_2)
}
{Gateaux differential of map df, division ring}



==> Second.Differential.Russian.tex <==
%auto-ignore

\input{Second.Differential.Eq}


\ifx\PrintBook\undefined
\else
\chapter{Производная второго порядка отображения тела}
\label{chapter: Derivative of Second Order of Map of Division Ring}
\fi

\section{Производная второго порядка отображения тела}

Пусть $D$ - нормированное тело характеристики $0$.
Пусть
\[f:D\rightarrow D\]
функция, дифференцируемая по Гато.
Согласно замечанию \ref{remark: differential L(D,D)}
производная Гато является отображением
\ShowEq{differential L(D,D)}
Согласно теоремам
\ePrints{0812.4763,0908.3307}
\ifx\Semafor\ValueOn
\ref{theorem: sum of linear maps, division ring},
\ref{theorem: linear map times constant, division ring}
\else
\xRef{0701.238}{theorem: sum of linear maps, division ring},
\xRef{0701.238}{theorem: linear map times constant, division ring}
\fi
и определению \ref{definition: norm of map, division ring}
множество $\mathcal L(D;D)$ является
нормированным $D$\Hyph векторным пространством.
Следовательно, мы можем рассмотреть вопрос,
является ли отображение $\partial f$ дифференцируемым по Гато.

Согласно определению
\xRef{0812.4763}{definition: map differentiable in Gateaux sense, D vector space}
\ShowEq{Gateaux differential of map df, division ring}
где
\ShowEq{Gateaux differential of map df, division ring, o2}
- такое непрерывное отображение, что
\ShowEq{Gateaux differential of map df, division ring, o2 lim}
Согласно определению
\xRef{0812.4763}{definition: map differentiable in Gateaux sense, D vector space}
отображение $\partial(\partial f(x)(a_1))(a_2)$
линейно по переменной $a_2$. Из равенства
\EqRef{Gateaux differential of map df, division ring}
следует, что отображение
$\partial(\partial f(x)(a_1))(a_2)$
линейно по переменной $a_1$.

\begin{definition}
\label{definition: Gateaux Differential of Second Order, division ring}
Полилинейное отображение
\symb{\partial^2 f(x)}0{Gateaux derivative of Second Order}
\symb{\frac{\partial^2 f(x)}{\partial x^2}}
0{Gateaux derivative of Second Order, fraction, division ring}
\begin{equation}
\EqLabel{Gateaux derivative of Second Order, division ring}
\ShowSymbol{Gateaux derivative of Second Order}(a_1;a_2)
=\ShowSymbol{Gateaux derivative of Second Order, fraction, division ring}(a_1;a_2)
=\partial(\partial f(x)(a_1))(a_2)
\end{equation}
называется
\AddIndex{производной Гато второго порядка}
{Gateaux derivative of Second Order} отображения $f$.
\qed
\end{definition}

\begin{remark}
\label{remark: differential L(D,D;D)}
Согласно определению
\ref{definition: Gateaux Differential of Second Order, division ring}
при заданном $x$ производная Гато второго порядка
\ShowEq{differential L(D,D;D), 1}.
Следовательно, производная Гато второго порядка отображения $f$ является отображением
\ShowEq{differential L(D,D;D)}
\end{remark}

\begin{theorem}
\label{theorem: Gateaux Differential of Second Order, division ring}
Мы можем представить
производную Гато второго порядка отображения $f$
в виде
\ShowEq{Differential of Second Order, division ring, representation}
\end{theorem}
\begin{proof}
Следствие определения \ref{definition: Gateaux Differential of Second Order, division ring}
и теоремы
\ePrints{0812.4763}
\ifx\Semafor\ValueOn
\ref{theorem: polylinear map, D vector space}.
\else
\xRef{0701.238}{theorem: polylinear map, D vector space}.
\fi
\end{proof}

\begin{definition}
Мы будем называть выражение\footnote{Мы полагаем
\ShowEq{component of Gateaux derivative of Second Order, 1, division ring}
}
\ShowEq{component of Gateaux derivative of Second Order, division ring}
\AddIndex{компонентой производной Гато второго порядка}
{component of Gateaux derivative of Second Order} отображения $f(x)$.
\qed
\end{definition}

По индукции, предполагая, что определена производная Гато
$\partial^{n-1} f(x)$ порядка $n-1$, мы определим
\symb{\partial^n f(x)}
0{Gateaux derivative of Order n}
\symb{\frac{\partial^n f(x)}{\partial x^n}}
0{Gateaux derivative of Order n, fraction, division ring}
\begin{equation}
\EqLabel{Gateaux derivative of Order n, division ring}
\ShowSymbol{Gateaux derivative of Order n}(a_1;...;a_n)
=\ShowSymbol{Gateaux derivative of Order n, fraction, division ring}(a_1;...;a_n)
=\partial(\partial^{n-1} f(x)(a_1;...;a_{n-1}))(a_n)
\end{equation}
\AddIndex{производную Гато порядка $n$}
{Gateaux derivative of Order n} отображения $f$.
Мы будем также полагать $\partial^0 f(x)=f(x)$.

\section{Ряд Тейлора}
\label{section: Taylor Series}

Рассмотрим многочлен одной переменной над телом $D$ степени $n$, $n>0$. Нас
интересует структура одночлена $p_k(x)$ многочлена степени $k$.

Очевидно, что одночлен степени $0$ имеет вид $a_0$, $a_0\in D$.
Пусть $k>0$. Докажем, что
\[
p_k(x)=p_{k-1}(x)xa_k
\]
где $a_k\in D$.
Действительно, последний множитель одночлена $p_k(x)$ является либо $a_k\in D$,
либо имеет вид $x^l$, $l\ge 1$.
В последнем случае мы положим $a_k=1$.
Множитель, предшествующий $a_k$, имеет вид $x^l$, $l\ge 1$.
Мы можем представить этот множитель в виде $x^{l-1}x$.
Следовательно, утверждение доказано.

В частности, одночлен степени $1$ имеет вид $p_1(x)=a_0xa_1$.

Не нарушая общности, мы можем положить $k=n$.

\begin{theorem}
\label{theorem: Gateaux derivative of f(x)x, division ring}
Для произвольного $m>0$ справедливо равенство
\begin{align}
&\partial^m (f(x)x)(h_1;...;h_m)
\nonumber \\
=&\partial^m f(x)(h_1;...;h_m)x
+\partial^{m-1} f(x)(h_1;...;h_{m-1})h_m
\EqLabel{Gateaux derivative of f(x)x, division ring}
\\ \nonumber
+&\partial^{m-1} f(x)(\widehat{h_1};...;h_{m-1};h_m)h_1
+...
\\ \nonumber
+&\partial^{m-1} f(x)(h_1;...;\widehat{h_{m-1}};h_m)h_{m-1}
\end{align}
где символ $\widehat{h^i}$ означает отсутствие переменной $h^i$ в списке.
\end{theorem}
\begin{proof}
Для $m=1$ - это следствие равенства
\EqRef{Gateaux derivative of product, division ring}
\[
\partial (f(x)x)(h_1)=\partial f(x)(h_1)x+
f(x)h_1
\]
Допустим, \EqRef{Gateaux derivative of f(x)x, division ring} справедливо
для $m-1$. Тогда
\begin{align}
&\partial^{m-1} (f(x)x)(h_1;...;h_{m-1})
\nonumber \\
=&\partial^{m-1} f(x)(h_1;...;h_{m-1})x
+\partial^{m-2} f(x)(h_1;...;h_{m-2})h_{m-1}
\EqLabel{Gateaux derivative of f(x)x, m-1, division ring}
\\ \nonumber
+&\partial^{m-2} f(x)(\widehat{h_1},...,h_{m-2},h_{m-1})h_1
+...
\\ \nonumber
+&\partial^{m-2} f(x)(h_1,...,\widehat{h_{m-2}},h_{m-1})h_{m-2}
\end{align}
Пользуясь равенствами \EqRef{Gateaux derivative of product, division ring}
и \EqRef{Gateaux differential, product over constant, division ring}
получим
\begin{align}
&\partial^m (f(x)x)(h_1;...;h_{m-1};h_m)
\nonumber \\
=&\partial^m f(x)(h_1;...;h_{m-1};h_m)x
+\partial^{m-1} f(x)(h_1;...;h_{m-2};h_{m-1})h_m
\nonumber \\
+&\partial^{m-1} f(x)(h_1;...;h_{m-2};\widehat{h_{m-1}};h_m)h_{m-1}
\EqLabel{Gateaux derivative of f(x)x, m, division ring}
\\ \nonumber
+&\partial^{m-2} f(x)(\widehat{h_1},...,h_{m-2},h_{m-1};h_m)h_1
+...
\\ \nonumber
+&\partial^{m-2} f(x)(h_1,...,\widehat{h_{m-2}},h_{m-1};h_m)h_{m-2}
\end{align}
Равенства \EqRef{Gateaux derivative of f(x)x, division ring} и
\EqRef{Gateaux derivative of f(x)x, m, division ring}
отличаются только формой записи.
Теорема доказана.
\end{proof}

\begin{theorem}
\label{theorem: Gateaux derivative of pn is symmetric, m less than n, division ring}
Производная Гато $\partial^m p_n(x)(h_1,...,h_m)$
является симметричным многочленом по переменным $h_1$, ..., $h_m$.
\end{theorem}
\begin{proof}
Для доказательства теоремы мы рассмотрим алгебраические свойства
производной Гато и дадим эквивалентное определение.
Мы начнём с построения одночлена.
Для произвольного одночлена $p_n(x)$ мы построим симметричный
многочлен $r_n(x)$ согласно следующим правилам
\begin{itemize}
\item Если $p_1(x)=a_0xa_1$, то $r_1(x_1)=a_0x_1a_1$
\item Если $p_n(x)=p_{n-1}(x)a_n$, то
\[
r_n(x_1,...,x_n)=r_{n-1}(x_{[1},...,x_{n-1})x_{n]}a_n
\]
где квадратные скобки выражают симметризацию выражения
по переменным $x_1$, ..., $x_n$.
\end{itemize}
Очевидно, что
\[
p_n(x)=r_n(x_1,...,x_n)\ \ \ x_1=...=x_n=x
\]
Мы определим производную Гато порядка $k$ согласно правилу
\begin{equation}
\partial^k p_n(x)(h_1,...,h_k)=r_n(h_1,...,h_k,x_{k+1},...,x_n)\ \ \ x_{k+1}=x_n=x
\EqLabel{Gateaux derivative of monomial, algebraic definition, division ring}
\end{equation}
Согласно построению многочлен $r_n(h_1,...,h_k,x_{k+1},...,x_n)$
симметричен по переменным $h_1$, ..., $h_k$, $x_{k+1}$, ..., $x_n$.
Следовательно, многочлен
\EqRef{Gateaux derivative of monomial, algebraic definition, division ring}
симметричен по переменным $h_1$, ..., $h_k$.

При $k=1$ мы докажем, что определение
\EqRef{Gateaux derivative of monomial, algebraic definition, division ring}
производной Гато совпадает с определением
\EqRef{Gateaux Dstar derivative, division ring}.

Для $n=1$, $r_1(h_1)=a_0h_1a_1$. Это выражение совпадает
с выражением производной Гато в теореме
\ref{theorem: Gateaux differential, product over constant, fx=x, division ring}.

Пусть утверждение справедливо для $n-1$.
Справедливо равенство
\begin{equation}
r_n(h_1,x_2,...,x_n)=r_{n-1}(h_1,x_{[2},...,x_{n-1})x_{n]}a_n+r_{n-1}(x_2,...,x_n)h_1a_n
\EqLabel{Gateaux derivative of monomial, n, division ring}
\end{equation}
Положим $x_2=...=x_n=x$. 
Согласно предположению индукции, из равенств
\EqRef{Gateaux derivative of monomial, algebraic definition, division ring},
\EqRef{Gateaux derivative of monomial, n, division ring}
следует
\[
r_n(h_1,x_2,...,x_n)=\partial p_{n-1}(x)(h_1)xa_n+p_{n-1}(x)h_1a_n
\]

Согласно теореме
\ref{theorem: Gateaux derivative of f(x)x, division ring}
\[
r_n(h_1,x_2,...,x_n)=\partial p_n(x)(h_1)
\]
что доказывает равенство
\EqRef{Gateaux derivative of monomial, algebraic definition, division ring}
для $k=1$.

Докажем теперь, что определение
\EqRef{Gateaux derivative of monomial, algebraic definition, division ring}
производной Гато совпадает с определением
\EqRef{Gateaux derivative of Order n, division ring} для $k>1$.

Пусть равенство
\EqRef{Gateaux derivative of monomial, algebraic definition, division ring}
верно для $k-1$.
Рассмотрим произвольное слагаемое многочлена $r_n(h_1,...,h_{k-1},x_k,...,x_n)$.
Отождествляя переменные $h_1$, ..., $h_{k-1}$
с элементами тела $D$, мы рассмотрим многочлен
\begin{equation}
R_{n-k}(x_k,...,x_n)=r_n(h_1,...,h_{k-1},x_k,...,x_n)
\EqLabel{reduced polynom, division ring}
\end{equation}
Положим $P_{n-k}(x)=R_{n-k}(x_k,...,x_n)$, $x_k=...=x_n=x$.
Следовательно
\[
P_{n-k}(x)=\partial^{k-1} p_n(x)(h_1;...;h_{k-1})
\]
Согласно определению
\EqRef{Gateaux derivative of Order n, division ring}
производной Гато
\begin{align}
\partial P_{n-k}(x)(h_k)
=&\partial(\partial^{k-1} p_n(x)(h_1;...;h_{k-1}))(h_k)
\nonumber\\
=&\partial^k p_n(x)(h_1;...;h_{k-1};h_k)
\EqLabel{Gateaux derivative of Order n, 1, division ring}
\end{align}
Согласно определению производной Гато
\EqRef{Gateaux derivative of monomial, algebraic definition, division ring}
\begin{equation}
\partial P_{n-k}(x)(h_k)=R_{n-k}(h_k,x_{k+1},...,x_n)\ \ \ x_{k+1}=x_n=x
\EqLabel{Gateaux derivative of monomial, algebraic definition, 1, division ring}
\end{equation}
Согласно определению \EqRef{reduced polynom, division ring},
из равенства
\EqRef{Gateaux derivative of monomial, algebraic definition, 1, division ring}
следует
\begin{equation}
\partial P_{n-k}(x)(h_k)=r_n(h_1,...,h_k,x_{k+1},...,x_n)\ \ \ x_{k+1}=x_n=x
\EqLabel{Gateaux derivative of monomial, algebraic definition, 2, division ring}
\end{equation}
Из сравнения равенств \EqRef{Gateaux derivative of Order n, 1, division ring}
и \EqRef{Gateaux derivative of monomial, algebraic definition, 2, division ring}
следует
\[
\partial^k p_n(x)(h_1;...;h_k)=r_n(h_1,...,h_k,x_{k+1},...,x_n)\ \ \ x_{k+1}=x_n=x
\]
Следовательно равенсто
\EqRef{Gateaux derivative of monomial, algebraic definition, division ring}
верно для любых $k$ и $n$.

Утверждение теоремы доказано.
\end{proof}

\begin{theorem}
\label{theorem: Gateaux derivative of pn equal 0, division ring}
Для произвольного $n\ge 0$ справедливо равенство
\begin{equation}
\EqLabel{Gateaux derivative n1 of pn, division ring}
\partial^{n+1} p_n(x)(h_1;...;h_{n+1})=0
\end{equation}
\end{theorem}
\begin{proof}
Так как $p_0(x)=a_0$, $a_0\in D$, то при $n=0$ теорема является следствием
теоремы \ref{theorem: Gateaux differential of const, division ring}.
Пусть утверждение теоремы верно для $n-1$. Согласно теореме
\ref{theorem: Gateaux derivative of f(x)x, division ring}
при условии $f(x)=p_{n-1}(x)$ мы имеем
\begin{align*}
\partial^{n+1} p_n(x)(h_1;...;h_{n+1})
=&\partial^{n+1}(p_{n-1}(x)xa_n)(h_1;...;h_{n+1})
\\
=&\partial^{n+1} p_{n-1}(x)(h_1;...;h_m)xa_n
\\
+&\partial^n p_{n-1}(x)(h_1;...;h_{m-1})h_ma_n
\\
+&\partial^n p_{n-1}(x)(\widehat{h_1};...;h_{m-1};h_m)h_1a_n
+...
\\
+&\partial^{m-1} p_{n-1}(x)(h_1;...;\widehat{h_{m-1}};h_m)h_{m-1}a_n
\end{align*}
Согласно предположению индукции все одночлены равны $0$.
\end{proof}

\begin{theorem}
\label{theorem: Gateaux derivative of pn equal 0, m less than n, division ring}
Если $m<n$, то справедливо равенство
\begin{equation}
\partial^m p_n(0)(h)=0
\EqLabel{m Gateaux derivative of polinom pn, division ring}
\end{equation}
\end{theorem}
\begin{proof}
Для $n=1$ справедливо равенство
\[
\partial^0 p_1(0)=a_0xa_1=0
\]
Допустим, утверждение справедливо
для $n-1$. Тогда согласно теореме \ref{theorem: Gateaux derivative of f(x)x, division ring}
\begin{align*}
&\partial^m (p_{n-1}(x)xa_n)(h_1;...;h_m)
\\
=&\partial^m p_{n-1}(x)(h_1;...;h_m)xa_n
+\partial^{m-1} p_{n-1}(x)(h_1;...;h_{m-1})h_ma_n
\\
+&\partial^{m-1} p_{n-1}(x)(\widehat{h_1};...;h_{m-1};h_m)h_1a_n
+...
\\
+&\partial^{m-1} p_{n-1}(x)(h_1;...;\widehat{h_{m-1}};h_m)h_{m-1}a_n
\end{align*}
Первое слагаемое равно $0$ так как $x=0$.
Так как $m-1<n-1$, то
остальные слагаемые равны $0$ согласно предположению индукции.
Утверждение теоремы доказано.
\end{proof}

Если $h_1=...=h_n=h$, то мы положим
\[
\partial^nf(x)(h)=\partial^nf(x)(h_1;...;h_n)
\]
Эта запись не будет приводить к неоднозначности, так как по числу аргументов
ясно, о какой функции идёт речь.

\begin{theorem}
\label{theorem: n Gateaux derivative of polinom pn, division ring}
Для произвольного $n>0$ справедливо равенство
\begin{equation}
\partial^n p_n(x)(h)=n!p_n(h)
\EqLabel{n Gateaux derivative of polinom pn, division ring}
\end{equation}
\end{theorem}
\begin{proof}
Для $n=1$ справедливо равенство
\[
\partial p_1(x)(h)=\partial (a_0xa_1)(h)=a_0ha_1=1!p_1(h)
\]
Допустим, утверждение справедливо
для $n-1$. Тогда согласно теореме \ref{theorem: Gateaux derivative of f(x)x, division ring}
\begin{align}
\EqLabel{n Gateaux derivative of polinom pn, 1, division ring}
\partial^n p_n(x)(h)
=&\partial^n p_{n-1}(x)(h)xa_n
+\partial^{n-1} p_{n-1}(x)(h)ha_n
\\ \nonumber
+&...
+\partial^{n-1} p_{n-1}(x)(h)ha_n
\end{align}
Первое слагаемое равно $0$ согласно теореме
\ref{theorem: Gateaux derivative of pn equal 0, division ring}.
Остальные $n$ слагаемых равны, и согласно предположению индукции
из равенства \EqRef{n Gateaux derivative of polinom pn, 1, division ring}
следует
\[
\partial^n p_n(x)(h)
=n\partial^{n-1} p_{n-1}(x)(h)ha_n=n(n-1)!p_{n-1}(h)ha_n=n!p_n(h)
\]
Следовательно, утверждение теоремы верно для любого $n$.
\end{proof}

Пусть $p(x)$ - многочлен степени $n$.\footnote{Я рассматриваю
формулу Тейлора для многочлена по аналогии с
построением формулы Тейлора в \citeBib{Fihtengolts: Calculus volume 1}, с. 246.}
\[
p(x)=p_0+p_{1i_1}(x)+...+p_{ni_n}(x)
\]
Мы предполагаем сумму по индексу $i_k$, который нумерует слагаемые
степени $k$.
Согласно теоремам \ref{theorem: Gateaux derivative of pn equal 0, division ring},
\ref{theorem: Gateaux derivative of pn equal 0, m less than n, division ring},
\ref{theorem: n Gateaux derivative of polinom pn, division ring}
\ShowEq{dp(0)(x)}
Следовательно, мы можем записать
\[
p(x)=p_0+(1!)^{-1}\partial p(0)(x)+(2!)^{-1}\partial^2 p(0)(x)+...+(n!)^{-1}\partial^n p(0)(x)
\]
Это представление многочлена называется
\AddIndex{формулой Тейлора для многочлена}{Taylor polynomial, division ring}.
Если рассмотреть замену переменных $x=y-y_0$, то рассмотренное построение
остаётся верным для многочлена
\[
p(y)=p_0+p_{1i_1}(y-y_0)+...+p_{ni_n}(y-y_0)
\]
откуда следует
\[
p(y)=p_0+(1!)^{-1}\partial p(y_0)(y-y_0)+(2!)^{-1}\partial^2 p(y_0)(y-y_0)+...+(n!)^{-1}\partial^n p(y_0)(y-y_0)
\]

Предположим, что функция $f(x))$ в точке $x_0$ дифференцируема в смысле Гато
до любого порядка.\footnote{Я рассматриваю
построение ряда Тейлора по аналогии с
построением ряда Тейлора в \citeBib{Fihtengolts: Calculus volume 1}, с. 248, 249.}

\begin{theorem}
\label{theorem: n Gateaux derivative equal 0, division ring}
Если для функции $f(x)$ выполняется условие
\begin{equation}
f(x_0)=\partial f(x_0)(h)=...=\partial^n f(x_0)(h)=0
\EqLabel{n Gateaux derivatives of function, division ring}
\end{equation}
то при $t\rightarrow 0$ выражение $f(x+th)$ является бесконечно малой порядка
выше $n$ по сравнению с $t$
\[
f(x_0+th)=o(t^n)
\]
\end{theorem}
\begin{proof}
При $n=1$ это утверждение следует из равенства
\EqRef{Gateaux differential of map, t, division ring}.

Пусть утверждение справедливо для $n-1$.
Для отображения
\[
f_1(x)=\partial f(x)(h)
\]
выполняется условие
\[
f_1(x_0)=\partial f_1(x_0)(h)=...=\partial^{n-1} f_1(x_0)(h)=0
\]
Согласно предположению индукции
\[
f_1(x_0+th)=o(t^{n-1})
\]
Тогда равенство \EqRef{Gateaux derivative, representation, 2}
примет вид
\[
o(t^{n-1})=\lim_{t\rightarrow 0,\ t\in R}(t^{-1}f(x+th))
\]
Следовательно,
\[
f(x+th)=o(t^n)
\]
\end{proof}

Составим многочлен
\begin{equation}
\EqLabel{Taylor polynomial, f(x), division ring}
p(x)=f(x_0)+(1!)^{-1}\partial f(x_0)(x-x_0)+...+(n!)^{-1}\partial^n f(x_0)(x-x_0)
\end{equation}
Согласно теореме \ref{theorem: n Gateaux derivative equal 0, division ring}
\[
f(x_0+t(x-x_0))-p(x_0+t(x-x_0))=o(t^n)
\]
Следовательно, полином $p(x)$ является хорошей апроксимацией отображения $f(x)$.

Если отображение $f(x)$ имеет производную Гато любого порядка, то переходя к пределу
$n\rightarrow\infty$, мы получим разложение в ряд
\[
f(x)=\sum_{n=0}^{\infty}(n!)^{-1}\partial^n f(x_0)(x-x_0)
\]
который называется \AddIndex{рядом Тейлора}{Taylor series, division ring}.

\section{Интеграл}

Понятие интеграла имеет разные аспекты. В этом разделе мы рассмотрим
интегрирование, как операцию, обратную дифференцированию.
По сути дела, мы рассмотрим процедуру решения обыкновенного дифференциального
уравнения
\[
\partial f(x)(h)=F(x;h)
\]

\begin{example}
Я начну с примера дифференциального уравнения над полем действительных чисел.
\begin{equation}
\EqLabel{differential equation y=xx, 1, real number}
y'=3x^2
\end{equation}
\begin{equation}
\EqLabel{differential equation y=xx, initial, real number}
\begin{matrix}
x_0=0&y_0=0
\end{matrix}
\end{equation}
Последовательно дифференцируя равенство \EqRef{differential equation y=xx, 1, real number},
мы получаем цепочку уравнений
\begin{align}
\EqLabel{differential equation y=xx, 2, real number}
y''&=6x
\\
\EqLabel{differential equation y=xx, 3, real number}
y'''&=6
\\
\EqLabel{differential equation y=xx, 4, real number}
y^{(n)}&=0&n&>3
\end{align}
Из уравнений
\EqRef{differential equation y=xx, 1, real number},
\EqRef{differential equation y=xx, initial, real number},
\EqRef{differential equation y=xx, 2, real number},
\EqRef{differential equation y=xx, 3, real number},
\EqRef{differential equation y=xx, 4, real number}
следует разложение в ряд Тейлора
\[
y=x^3
\]
\qed
\end{example}

\begin{example}
Рассмотрим аналогичное дифференциальное уравнение над телом
\begin{equation}
\EqLabel{differential equation y=xx, 1, division ring}
\partial (y)(h)=hx^2+xhx+x^2h
\end{equation}
\begin{equation}
\EqLabel{differential equation y=xx, initial, division ring}
\begin{matrix}
x_0=0&y_0=0
\end{matrix}
\end{equation}
Последовательно дифференцируя равенство
\EqRef{differential equation y=xx, 1, division ring},
мы получаем цепочку уравнений
\ShowEq{differential equation y=xx, division ring}
Из уравнений
\EqRef{differential equation y=xx, 1, division ring},
\EqRef{differential equation y=xx, initial, division ring},
\EqRef{differential equation y=xx, 2, division ring},
\EqRef{differential equation y=xx, 3, division ring},
\EqRef{differential equation y=xx, 4, division ring}
следует разложение в ряд Тейлора
\[
y=x^3
\]
\qed
\end{example}

\begin{remark}
Дифференциальное уравнение
\begin{equation}
\EqLabel{differential equation y=xx, 1, a, division ring}
\partial (y)(h)=3hx^2
\end{equation}
\begin{equation}
\EqLabel{differential equation y=xx, initial, a, division ring}
\begin{matrix}
x_0=0&y_0=0
\end{matrix}
\end{equation}
так же приводит к решению $y=x^3$. Очевидно, что это
отображение не удовлетворяет дифференциальному уравнению.
Однако, вопреки теореме
\ref{theorem: Gateaux derivative of pn is symmetric, m less than n, division ring}
вторая производная не
является симметричным многочленом. Это говорит о том,
что уравнение \EqRef{differential equation y=xx, 1, a, division ring}
не имеет решений.
\qed
\end{remark}

\begin{example}
\label{example: differential equation, additive function, division ring}
Очевидно, если функция удовлетворяет дифференциальному уравнению
\ShowEq{differential equation, additive function, division ring}
то вторая производная Гато
\[
\partial^2 f(x)(h_1;h_2)=0
\]
Следовательно, если задано начальное условие $y(0)=0$,
то дифференциальное уравнение
\EqRef{differential equation, additive function, division ring} имеет решение
\ShowEq{differential equation, additive function, solution, division ring}
\qed
\end{example}

\section{Экспонента}

В этом разделе мы рассмотрим одну из возможных моделей
построения экспоненты.

В поле мы можем определить экспоненту как решение дифференциального
уравнения
\ShowEq{exponent over field}
Очевидно, что мы не можем записать подобное уравнения для тела.
Однако мы можем воспользоваться равенством
\ShowEq{derivative over field}
Из уравнений
\EqRef{exponent over field}, \EqRef{derivative over field}
следует
\ShowEq{exponent derivative over field}
Это уравнение уже ближе к нашей цели,
однако остаётся открытым вопрос в каком порядке
мы должны перемножать $y$ и $h$.
Что бы ответить на этот вопрос, мы изменим запись уравнения
\ShowEq{exponent derivative over division ring}
Следовательно, наша задача - решить дифференциальное уравнение
\EqRef{exponent derivative over division ring}
при начальном условии $y(0)=1$.

Для формулировки и доказательства теоремы
\ref{theorem: exponent derivative n over division ring}
я введу следующее обозначение.
Пусть
\ShowEq{exponent derivative, transposition n}
перестановка кортежа переменных
\ShowEq{exponent transposition tuple 1}
Обозначим $p_{\sigma}(h_i)$ позицию, которую занимает
переменная $h_i$ в кортеже
\ShowEq{exponent transposition tuple 2}
Например, если перестановка $\sigma$ имеет вид
\ShowEq{exponent transposition tuple 3}
то следующие кортежи равны
\ShowEq{exponent transposition tuple 4}

\begin{theorem}
\label{theorem: exponent derivative n over division ring}
Производная Гато порядка $n$ функции $y$, удовлетворяющей дифференциальному уравнению
\EqRef{exponent derivative over division ring}
имеет вид
\ShowEq{exponent derivative n over division ring}
где сумма выполнена по перестановкам
\ShowEq{exponent derivative, transposition n}
множества переменных $y$, $h_1$, ..., $h_n$.
Перестановка $\sigma$ обладает следующими свойствами
\begin{enumerate}
\item Если существуют $i$, $j$, $i\ne j$, такие, что
$p_{\sigma}(h_i)$ располагается в произведении
\EqRef{exponent derivative n over division ring}
левее $p_{\sigma}(h_j)$ и $p_{\sigma}(h_j)$ располагается
левее $p_{\sigma}(y)$, то $i<j$.
\label{enumerate: exponent derivative, transposition n, left}
\item Если существуют $i$, $j$, $i\ne j$, такие, что
$p_{\sigma}(h_i)$ располагается в произведении
\EqRef{exponent derivative n over division ring}
правее $p_{\sigma}(h_j)$ и $p_{\sigma}(h_j)$ располагается
правее $p_{\sigma}(y)$, то $i>j$.
\label{enumerate: exponent derivative, transposition n, right}
\end{enumerate}
\end{theorem}
\begin{proof}
Мы докажем это утверждение индукцией.
Для $n=1$ утверждение верно, так как это дифференциальное уравнение
\EqRef{exponent derivative over division ring}.
Пусть утверждение верно для $n=k-1$.
Следовательно
\ShowEq{exponent derivative n=k-1 over division ring}
где сумма выполнена по перестановкам
\ShowEq{exponent derivative, transposition n=k-1}
множества переменных $y$, $h_1$, ..., $h_{k-1}$.
Перестановка $\sigma$ удовлетворяет условиям
\eqref{enumerate: exponent derivative, transposition n, left},
\eqref{enumerate: exponent derivative, transposition n, right},
сформулированным в теореме.
Согласно определению
\EqRef{Gateaux derivative of Order n, division ring}
производная Гато` порядка $k$ имеет вид
\ShowEq{exponent derivative n=k over division ring, 1}
Из равенств
\EqRef{exponent derivative over division ring},
\EqRef{exponent derivative n=k over division ring, 1}
следует
\ShowEq{exponent derivative n=k over division ring, 2}
Нетрудно видеть, что произвольная перестановка $\sigma$
из суммы
\EqRef{exponent derivative n=k over division ring, 2}
порождает две перестановки
\ShowEq{exponent derivative, transposition n=k}
Из \EqRef{exponent derivative n=k over division ring, 2}
и \EqRef{exponent derivative, transposition n=k}
следует
\ShowEq{exponent derivative n=k over division ring, 3}
В выражении
\EqRef{exponent derivative n=k over division ring, 3}
$p_{\tau_1}(h_k)$ записано непосредственно перед $p_{\tau_1}(y)$.
Так как $k$ - самое большое значение индекса,
то перестановка $\tau_1$ удовлетворяет условиям
\eqref{enumerate: exponent derivative, transposition n, left},
\eqref{enumerate: exponent derivative, transposition n, right},
сформулированным в теореме.
В выражении
\EqRef{exponent derivative n=k over division ring, 3}
$p_{\tau_2}(h_k)$ записано непосредственно после $p_{\tau_2}(y)$.
Так как $k$ - самое большое значение индекса,
то перестановка $\tau_2$ удовлетворяет условиям
\eqref{enumerate: exponent derivative, transposition n, left},
\eqref{enumerate: exponent derivative, transposition n, right},
сформулированным в теореме.

Нам осталось показать, что в выражении
\EqRef{exponent derivative n=k over division ring, 3}
перечислены все перестановки $\tau$, удовлетворяющие условиям
\eqref{enumerate: exponent derivative, transposition n, left},
\eqref{enumerate: exponent derivative, transposition n, right},
сформулированным в теореме.
Так как $k$ - самый большой индекс, то согласно условиям
\eqref{enumerate: exponent derivative, transposition n, left},
\eqref{enumerate: exponent derivative, transposition n, right},
сформулированным в теореме, $\tau(h_k)$
записано непосредственно перед или непосредственно после $\tau(y)$.
Следовательно, любая перестановка $\tau$ имеет
либо вид $\tau_1$, либо вид $\tau_2$.
Пользуясь равенством
\EqRef{exponent derivative, transposition n=k},
мы можем для заданной перестановки $\tau$ найти соответствующую
перестановку $\sigma$.
Следовательно, утверждение теоремы верно для $n=k$.
Теорема доказана.
\end{proof}

\begin{theorem}
Решением дифференциального уравнения
\EqRef{exponent derivative over division ring}
при начальном условии $y(0)=1$
является экспонента
\ShowEq{exponent over division ring}
которая имеет следующее разложение в ряд Тейлора
\ShowEq{exponent Taylor series over division ring}
\end{theorem}
\begin{proof}
Производная Гато порядка $n$ содержит $2^n$ слагаемых.
Действительно, производная Гато порядка $1$ содержит $2$ слагаемых,
и каждое дифференцирование увеличивает число слагаемых вдвое.
Из начального условия $y(0)=1$ и теоремы
\ref{theorem: exponent derivative n over division ring}
следует, что производная Гато порядка $n$ искомого решения имеет вид
\ShowEq{exponent derivative n over division ring, x=0}
Из равенства
\EqRef{exponent derivative n over division ring, x=0}
следует разложение
\EqRef{exponent Taylor series over division ring}.
в ряд Тейлора.
\end{proof}

\begin{theorem}
\label{theorem: exponent of sum}
Равенство
\ShowEq{exponent of sum}
справедливо тогда и только тогда, когда
\ShowEq{exponent of sum, 1}
\end{theorem}
\begin{proof}
Для доказательства теоремы достаточно рассмотреть ряды Тейлора
\ShowEq{exponent a b a+b}
Перемножим выражения
\EqRef{exponent a} и \EqRef{exponent b}.
Сумма одночленов порядка $3$ имеет вид
\ShowEq{exponent ab 3}
и не совпадает, вообще говоря, с выражением
\ShowEq{exponent a+b 3}
Доказательство утверждения, что
\EqRef{exponent of sum} следует из \EqRef{exponent of sum, 1}
тривиально.
\end{proof}

Смысл теоремы \ref{theorem: exponent of sum}
становится яснее, если мы вспомним, что существует две
модели построения экспоненты. Первая модель - это
решение дифференциального уравнения
\EqRef{exponent derivative over division ring}.
Вторая - это изучение однопараметрической группы преобразований.
В случае поля обе модели приводят к одной и той же функции.
Я не могу этого утверждать сейчас в общем случае. Это вопрос отдельного
исследования. Но если вспомнить, что кватернион является аналогом
преобразования трёхмерного пространства, то утверждение теоремы
становится очевидным.


==> Second.Differential.Vector.English.tex <==
%auto-ignore

\input{Second.Differential.Vector.Eq}

\ifx\PrintBook\undefined
\else
\chapter{Derivative of Second Order of Map of
\texorpdfstring{$D$}{D}-Vector Space}
\label{chapter: Derivative of Second Order of Map of D-Vector Space}
\fi
\section{Derivative of Second Order of Map of
\texorpdfstring{$D$}{D}-Vector Space}

Let $D$ be valued division ring of characteristic $0$.
Let $V$ be normed $D$\Hyph vector space with norm $\|y\|_V$.
Let $W$ be normed $D$\Hyph vector space with norm $\|z\|_W$.
Let
\ShowEq{f:V->W}
function differentiable in the G\^ateaux sense.
According to remark \ref{remark: differential L(D,V,W)}
the G\^ateaux derivative is map
\ShowEq{differential L(D,V,W)}
According to theorems
\ePrints{0812.4763}
\ifx\Semafor\ValueOn
\ref{theorem: sum of linear maps, division ring},
\else
\xRef{0701.238}{theorem: sum of linear maps, division ring},
\xRef{0701.238}{theorem: linear map times constant, division ring}
\fi
and definition \ref{definition: norm of map, D vector space}
set $\mathcal L(D;V;W)$ is
normed $D$\Hyph vector space.
Therefore, we may consider the question,
if map $\partial f$ is differentiable in the G\^ateaux sense.

According to the definition
\ref{definition: map differentiable in Gateaux sense, D vector space},
\ShowEq{Gateaux derivative of map df, D vector space}
where
\ShowEq{Gateaux derivative of map df, D vector space, o2}
is such continuous map, that
\ShowEq{Gateaux derivative of map df, D vector space, o2 lim}
According to the definition
\ref{definition: map differentiable in Gateaux sense, D vector space},
the map
\ShowEq{d(dfxa1)a2}
is linear map of variable $a_2$. From equation
\EqRef{Gateaux derivative of map df, D vector space},
it follows that map
\ShowEq{d(dfxa1)a2}
is linear map of variable $a_1$.

\begin{definition}
\label{definition: Gateaux derivative of Second Order, D vector space}
Polylinear map
\ShowEq{Gateaux derivative of Second Order, D vector space def}
\ShowEq{Gateaux derivative of Second Order, D vector space}
is called
\AddIndex{the G\^ateaux derivative of second order}
{Gateaux derivative of Second Order} of map $f$.
\qed
\end{definition}

\begin{remark}
\label{remark: differential L(D;V,V;W)}
According to definition
\ref{definition: Gateaux derivative of Second Order, D vector space}
for given $x$ the G\^ateaux derivative of second order
\ShowEq{differential L(D;V,V;W), 1}.
Therefore, the G\^ateaux derivative of second order of map $f$ is map
\ShowEq{differential L(D;V,V;W)}
\end{remark}

\begin{theorem}
\label{theorem: Gateaux Differential of Second Order, D vector space}
Let \eV V be basis of $D$\Hyph vector space $V$.
Let \eV W be basis of $D$\Hyph vector space $W$.
\AddIndex{The G\^ateaux differential of second order}
{Gateaux differential of Second Order} of map $f$
relative to basis \eV V and
basis \eV W
has form
\ShowEq{Gateaux differential of Second Order, D vector space}
\ShowEq{Differential of Second Order, D vector space, representation}
\end{theorem}
\begin{proof}
Corollary of definition
\ref{definition: Gateaux derivative of Second Order, D vector space}
and theorem
\ePrints{0812.4763}
\ifx\Semafor\ValueOn
\ref{theorem: polylinear map, D vector space}.
\else
\xRef{0701.238}{theorem: polylinear map, D vector space}.
\fi
\end{proof}

\begin{definition}
\begin{sloppypar}
Expression
\ShowEq{component of Gateaux derivative of Second Order, D vector space}
is called
\AddIndex{component of the G\^ateaux derivative of second order}
{component of Gateaux derivative of Second Order} of map $f(x)$.
\qed
\end{sloppypar}
\end{definition}

\begin{definition}
\ShowEq{Gateaux partial derivative of Second Order, D vector space}
Let $D$ be division ring of characteristic $0$.
Let \eV V be basis of $D$\Hyph vector space $V$.
Let \eV W be basis of $D$\Hyph vector space $W$.
The G\^ateaux partial derivative
\ShowEq{definition Gateaux partial derivative of Second Order, D vector space}
is called \AddIndex{the G\^ateaux mixed partial derivative}
{Gateaux partial derivative of Second Order}
of map $f^{\gik}$ with respect to variables $v^{\gii}$, $v^{\gij}$.
\qed
\end{definition}

\begin{theorem}
\label{theorem: Gateaux partial derivative of Second Order, D vector space}
Let $D$ be division ring of characteristic $0$.\footnote{I proved the theorem
the same way like it is done for theorem in \citeBib{Fihtengolts: Calculus volume 1},
p. 405, 406.}
Let \eV V be basis of $D$\Hyph vector space $V$.
Let \eV W be basis of $D$\Hyph vector space $W$.
Let the G\^ateaux partial derivatives of map
\ShowEq{f:V->W}
are continuous and differentiable in the G\^ateaux sense on the set $U\subset V$.
Let the G\^ateaux mixed partial derivatives of second order
is continuous on the set $U\subset V$.
Then on the set $U$ the G\^ateaux mixed partial derivatives
satisfy equation
\ShowEq{Gateaux partial derivatives equal, D vector space}
\end{theorem}
\begin{proof}
To prove theorem we will use notation
$f^{\gik}(v)=f^{\gik}(v^{\gii},v^{\gij})$,
assuming, that rest variables have given values.
The statement of theorem follows from following chain of equations
\ShowEq{Gateaux partial derivatives equal, 1, D vector space}

\ifx\texFuture\Defined
Let us consider expression
\begin{equation}
W=t^{-2}(f^k(x^i+th^i,x^j+th^j)-f^k(x^i+th^i,x^j)-f^k(x^i,x^j+th^j)+f^k(x^i,x^j))
\EqLabel{Gateaux partial derivative of Second Order, D vector space, 1}
\end{equation}
Because function $f^k$ is differentiable in the G\^ateaux sense
and the G\^ateaux partial derivatives are continuous,
then from theorem \ref{theorem: expansion of Gateaux differential, D vector space},
definition \ref{definition: Gateaux partial derivative, D vector space}
and equations \EqRef{Gateaux differential of map, t, division ring},
\EqRef{Gateaux partial derivative of Second Order, D vector space, 1}
it follows that
\begin{equation}
W=t^{-2}
\left(
\frac{\partial f^k(x^i+th^i,x^j)}{\partial tx^j}(th^j)
-\frac{\partial f^k(x^i,x^j)}{\partial tx^j}(th^j)
\right)
\EqLabel{Gateaux partial derivatives equal, D vector space, 2}
\end{equation}
Because the G\^ateaux derivatives
is multiplicative over real field,
from equation \EqRef{Gateaux partial derivative of Second Order, D vector space, 2}
it follows
\begin{equation}
W=t^{-1}
\left(
\frac{\partial f^k(x^i+th^i,x^j)}{\partial tx^j}(h^j)
-\frac{\partial f^k(x^i,x^j)}{\partial tx^j}(h^j)
\right)
\EqLabel{Gateaux partial derivative of Second Order, D vector space, 3}
\end{equation}
Because map
$\displaystyle\frac{\partial f^k(x^i,x^j)}{\partial x^j}(h^j)$
is differentiable and its partial derivatives are continues,
from theorem \ref{theorem: expansion of Gateaux differential, D vector space},
definition \ref{definition: Gateaux partial derivative, D vector space}
and equations \EqRef{Gateaux differential of map, t, division ring},
\EqRef{Gateaux partial derivative of Second Order, D vector space, 3}
it follows
\begin{equation}
W=t^{-1}
\frac{\partial}{\partial x^i}
\left(
\frac{\partial f^k(x^i+th^i,x^j)}{\partial x^j}(h^j)
\right)
(th^i)
\EqLabel{Gateaux partial derivative of Second Order, D vector space, 4}
\end{equation}
Because the G\^ateaux derivative
is multiplicative over real field,
using definition
\EqRef{definition Gateaux partial derivative of Second Order, D vector space},
we get
\begin{equation}
W=
\frac{\partial^2 f^k(x^i,x^j)}{\partial x^i\partial x^j}(h^j,h^i)
\EqLabel{Gateaux partial derivative of Second Order, D vector space, 5}
\end{equation}
Применяя к выражению
\EqRef{Gateaux partial derivative of Second Order, D vector space, 1}
приведенные выше преобразования сперва к переменной $x^i$, а затем
к переменной $x^j$, мы получим
\begin{equation}
W=
\frac{\partial^2 f^k(x^i,x^j)}{\partial x^j\partial x^i}(h^i,h^j)
\EqLabel{Gateaux partial derivative of Second Order, D vector space, 6}
\end{equation}
Equation \EqRef{Gateaux partial derivative of Second Order, D vector space}
follows from equations
\EqRef{Gateaux partial derivative of Second Order, D vector space, 5},
\EqRef{Gateaux partial derivative of Second Order, D vector space, 6}.
\fi
\end{proof}

By induction, assuming that the G\^ateaux derivative
$\partial^{n-1} f(x)$ of order $n-1$ is defined, we define
\ShowEq{Gateaux derivative of Order n, D vector space}
\AddIndex{the G\^ateaux derivative of order $n$}
{Gateaux derivative of Order n} of map $f$.
We also assume $\partial^0 f(x)=f(x)$.

\section{Homogeneous Map}

\begin{definition}
The map
\ShowEq{f:V->W}
of $D$\Hyph vector space $V$ into
$D$\Hyph vector space $W$
is called \AddIndex{homogeneous map of degree $k$ over field $F$}
{homogeneous map of degree over field, D vector space},
if for any $a\in F$
\ShowEq{homogeneous map of degree k, D vector space}
\qed
\end{definition}

\begin{theorem}[Euler's theorem]
\label{theorem: Euler theorem, homogeneous map, D vector space}
Let map
\ShowEq{f:V->W}
of $D$\Hyph vector space $V$ into
$D$\Hyph vector space $W$
be homogeneous map of degree $k$ over field $F\subset Z(D)$.
\ShowEq{Euler theorem, homogeneous map, D vector space}
\end{theorem}
\begin{proof}
Let us differentiate equation
\EqRef{homogeneous map of degree k, D vector space}
with respect to $a$\footnote{For map of field it is true that
\[
\partial f(x)(h)=\frac{df(x)}{dx}h
\]}
\ShowEq{homogeneous map of degree k, D vector space, 1}
From theorem
\ref{theorem: composite map, differential, D vector space}
it follows
\ShowEq{homogeneous map of degree k, D vector space, 2}
From theorem \ref{theorem: Gateaux derivative over field F, D vector space}
and equation \EqRef{homogeneous map of degree k, D vector space, 2}
it follows
\ShowEq{homogeneous map of degree k, D vector space, 3}
It is evident that
\ShowEq{homogeneous map of degree k, D vector space, 4}
Let us substitute \EqRef{homogeneous map of degree k, D vector space, 3}
and \EqRef{homogeneous map of degree k, D vector space, 4}
in \EqRef{homogeneous map of degree k, D vector space, 1}
\ShowEq{homogeneous map of degree k, D vector space, 5}
Because $\Delta a\ne 0$, then
\EqRef{Euler theorem, homogeneous map, D vector space}
follows from
\EqRef{homogeneous map of degree k, D vector space, 5}
under the condition $a=1$.
\end{proof}

%\begin{theorem}[Euler's theorem]
%\label{theorem: Euler theorem, homogeneous map}
Let map
\ShowEq{f:V->W}
from $D$\Hyph vector space $V$ into
$D$\Hyph vector space $W$
be homogeneous map of degree $k$ over field $F\subset Z(D)$.
%\end{theorem}
%\begin{proof}
From theorem \ref{theorem: Gateaux derivative over field F, D vector space}
it follows
\ShowEq{homogeneous map of degree k, D vector space, d1}
From equations \EqRef{Euler theorem, homogeneous map, D vector space},
\EqRef{homogeneous map of degree k, D vector space}
it follows
\ShowEq{homogeneous map of degree k, D vector space, d2}
From equations \EqRef{homogeneous map of degree k, D vector space, d1},
\EqRef{homogeneous map of degree k, D vector space, d2}
it follows
\ShowEq{homogeneous map of degree k, D vector space, d3}
However from equation
\EqRef{homogeneous map of degree k, D vector space, d3}
it does not follow
that map
\ShowEq{homogeneous map of degree k, D vector space, d4}
is homogeneous map of degree $k-1$ over field $F$.
%\end{proof}



==> Second.Differential.Vector.Eq.tex <==
%auto-ignore

\DefEquation
{
\partial f(x+a_2)(a_1)-\partial f(x)(a_1)
=\partial(\partial f(x)(a_1))(a_2)
+o_2(a_2)
}
{Gateaux derivative of map df, D vector space}

\DefEq
{
$o_2:V\rightarrow \mathcal L(D;V;W)$%
}
{Gateaux derivative of map df, D vector space, o2}

\DefEq
{
$\partial(\partial f(x)(a_1))(a_2)$
}
{d(dfxa1)a2}

\DefEq
{
\symb{\partial^2 f(x)}0{Gateaux derivative of Second Order}
}
{Gateaux derivative of Second Order, D vector space def}

\DefEquation
{
\ShowSymbol{Gateaux derivative of Second Order}(a_1;a_2)
=\partial(\partial f(x)(a_1))(a_2)
}
{Gateaux derivative of Second Order, D vector space}

\DefEq
{
\[
\lim_{a_2\rightarrow 0}\frac{\|o_2(a_2)\|_W}{\|a_2\|_V}=0
\]
}
{Gateaux derivative of map df, D vector space, o2 lim}

\DefEq
{
$\partial^2 f(x)\in
\mathcal L(D;V,V;W)$%
}
{differential L(D;V,V;W), 1}

\DefEq
{
\[
\partial^2 f:V\rightarrow \mathcal L(D;V,V;W)
\]
}
{differential L(D;V,V;W)}

\DefEq
{
\symb{\partial^2 f(x)(a_1;a_2)}
0{Gateaux differential of Second Order, D vector space}
}
{Gateaux differential of Second Order, D vector space}

\DefEquation
{
\ShowSymbol{Gateaux differential of Second Order, D vector space}
=\frac{\partial^2_{s\cdot 0} f^{\gij}(x)}
{\partial x^{\gi{i_1}}\partial x^{\gi{i_2}}}
\ \sigma_s(a_1^{\gi{i_1}})
\ \frac{\partial^2_{s\cdot 1} f^{\gij}(x)}
{\partial x^{\gi{i_1}}\partial x^{\gi{i_2}}}
\ \sigma_s(a_2^{\gi{i_2}})
\ \frac{\partial^2_{s\cdot 2} f^{\gij}(x)}
{\partial x^{\gi{i_1}}\partial x^{\gi{i_2}}}
\EV Wj
}
{Differential of Second Order, D vector space, representation}

\DefEq
{
\symb{\frac{\partial^2 f^{\gik}(v)}{\partial v^{\gij}\partial v^{\gii}}}
0{Gateaux partial derivative of Second Order}
}
{Gateaux partial derivative of Second Order, D vector space}

\DefEquation
{
\frac{\partial^2 f^{\gik}(v)}{\partial v^{\gij}\partial v^{\gii}}
(h^{\gii},h^{\gij})=
\frac{\partial^2 f^{\gik}(v)}{\partial v^{\gii}\partial v^{\gij}}
(h^{\gij},h^{\gii})
}
{Gateaux partial derivatives equal, D vector space}

\DefEq
{
\begin{align*}
&\frac{\partial^2 f(v^{\gii},v^{\gij})}{\partial v^{\gii}\partial v^{\gij}}
(h^{\gij},h^{\gii})
\\
=&\frac{\partial}{\partial v^{\gii}}
\left(
\frac{\partial f(v^{\gii},v^{\gij})}{\partial v^{\gij}}(h^{\gij})
\right)
(h^{\gii})
\\
=&\lim_{t\rightarrow 0}
\,t^{-1}
\left(
\frac{\partial f(v^{\gii}+h^{\gii}t,v^{\gij})}{\partial v^{\gij}}(h^{\gij})
-\frac{\partial f(v^{\gii},v^{\gij})}{\partial v^{\gij}}(h^{\gij})
\right)
\\
=&\lim_{t\rightarrow 0}
\,t^{-2}
\left(
f(v^{\gii}+h^{\gii}t,v^{\gij}+h^{\gij}t)
-f(v^{\gii}+h^{\gii}t,v^{\gij})
-f(v^{\gii},v^{\gij}+h^{\gij}t)
+f(v^{\gii},v^{\gij})
\right)
\\
=&\lim_{t\rightarrow 0}
\,t^{-2}
\left(
f(v^{\gii}+h^{\gii}t,v^{\gij}+h^{\gij}t)
-f(v^{\gii},v^{\gij}+h^{\gij}t)
-f(v^{\gii}+h^{\gii}t,v^{\gij})
+f(v^{\gii},v^{\gij})
\right)
\\
=&\lim_{t\rightarrow 0}
\,t^{-1}
\left(
\frac{\partial f(v^{\gii},v^{\gij}+h^{\gij}t)}{\partial v^{\gii}}(h^{\gii})
-\frac{\partial f(v^{\gii},v^{\gij})}{\partial v^{\gii}}(h^{\gii})
\right)
\\
=&\frac{\partial}{\partial v^{\gij}}
\left(
\frac{\partial f(v^{\gii},v^{\gij})}{\partial v^{\gii}}(h^{\gii})
\right)
(h^{\gij})
\\
=&\frac{\partial^2 f(v^{\gii},v^{\gij})}{\partial v^{\gij}\partial v^{\gii}}
(h^{\gii},h^{\gij})
\end{align*}
}
{Gateaux partial derivatives equal, 1, D vector space}

\DefEq
{
\symb{\partial^n f(x)}
0{Gateaux derivative of Order n}
\[
\ShowSymbol{Gateaux derivative of Order n}
(a_1;...;a_n)
=\partial(\partial^{n-1} f(x)(a_1;...;a_{n-1})) a_n
\]
}
{Gateaux derivative of Order n, D vector space}

\DefEquation
{
\partial f(av)(v)\Delta a=ka^{k-1}f(v)\Delta a
}
{homogeneous map of degree k, D vector space, 5}

\DefEquation
{
\partial f(av)(v)=a^{k-1}\partial f(v)(v)
}
{homogeneous map of degree k, D vector space, d3}

\DefEq
{
\[
\partial f:V\rightarrow\mathcal A(D;V;W)
\]
}
{homogeneous map of degree k, D vector space, d4}

\DefEquation
{
\partial f(av)(av)
=kf(av)
=ka^kf(v)
=a^k\partial f(v)(v)
}
{homogeneous map of degree k, D vector space, d2}

\DefEquation
{
\partial f(av)(av)
=a\partial f(av)(v)
}
{homogeneous map of degree k, D vector space, d1}

\DefEquation
{
\frac{d}{da}(a^kf(v))=ka^{k-1}f(v)
}
{homogeneous map of degree k, D vector space, 4}

\DefEquation
{
\frac{d}{da}(f(av))\Delta a
=\frac{d}{da}(a^kf(v))\Delta a
}
{homogeneous map of degree k, D vector space, 1}

\DefEquation
{
\begin{split}
\frac{d}{da}(f(av))\Delta a
&=\partial f(av)(\partial (av)(\Delta a))
\\
&=\partial f(av)\left(\frac {d(av)}{da}\Delta a\right)
\\
&=\partial f(av)(v\Delta a)
\end{split}
}
{homogeneous map of degree k, D vector space, 2}

\DefEquation
{
\frac{d}{da}(f(av))\Delta a
=\partial f(av)(v)\Delta a
}
{homogeneous map of degree k, D vector space, 3}

\DefEquation
{
\partial f(v)(v)=kf(v)
}
{Euler theorem, homogeneous map, D vector space}

\DefEquation
{
f(av)=a^kf(v)
}
{homogeneous map of degree k, D vector space}

\DefEq
{
$b=f(a\CRstar e)\in A$
}
{b=f(a)}

\DefEquation
{
\ShowSymbol{Gateaux partial derivative of Second Order}
(h^{\gii},h^{\gij})
=
\frac{\partial}{\partial v^{\gij}}
\left(
\frac{\partial f^{\gik}(v)}{\partial v^{\gii}}(h^{\gii})
\right)
(h^{\gij})
}
{definition Gateaux partial derivative of Second Order, D vector space}

\DefEq
{
\symb{\frac{\partial^2_{s\cdot p} f^{\gij}(x)}
{\partial x^{\gi{i_1}}\partial x^{\gi{i_2}}}}0
{component of Gateaux derivative of Second Order, D vector space}
$\displaystyle
\ShowSymbol{component of Gateaux derivative of Second Order, D vector space}$,
$p=0$, $1$, $2$,
}
{component of Gateaux derivative of Second Order, D vector space}


==> Second.Differential.Vector.Russian.tex <==
%auto-ignore

\input{Second.Differential.Vector.Eq}


\ifx\PrintBook\undefined
\else
\chapter{Производная второго порядка отображения
\texorpdfstring{$D$}{D}-векторного пространства}
\label{chapter: Derivative of Second Order of Map of D-Vector Space}
\fi

\section{Производная второго порядка отображения
\texorpdfstring{$D$}{D}-векторного пространства}

Пусть $D$ - нормированное тело характеристики $0$.
Пусть $V$ - нормированное $D$\Hyph векторное пространство с нормой $\|y\|_V$.
Пусть $W$ - нормированное $D$\Hyph векторное пространство с нормой $\|z\|_W$.
Пусть
\ShowEq{f:V->W}
функция, дифференцируемая по Гато.
Согласно замечанию \ref{remark: differential L(D,V,W)}
производная Гато является отображением
\ShowEq{differential L(D,V,W)}
Согласно теоремам
\ePrints{0812.4763}
\ifx\Semafor\ValueOn
\ref{theorem: sum of linear maps, division ring},
\ref{theorem: linear map times constant, division ring}
\else
\xRef{0701.238}{theorem: sum of linear maps, division ring},
\xRef{0701.238}{theorem: linear map times constant, division ring}
\fi
и определению \ref{definition: norm of map, D vector space}
множество $\mathcal L(D;V;W)$ является
нормированным $D$\Hyph векторным пространством.
Следовательно, мы можем рассмотреть вопрос,
является ли отображение $\partial f$ дифференцируемым по Гато.

Согласно определению
\ref{definition: map differentiable in Gateaux sense, D vector space}
\ShowEq{Gateaux derivative of map df, D vector space}
где
\ShowEq{Gateaux derivative of map df, D vector space, o2}
- такое непрерывное отображение, что
\ShowEq{Gateaux derivative of map df, D vector space, o2 lim}
Согласно определению
\ref{definition: map differentiable in Gateaux sense, D vector space}
отображение
\ShowEq{d(dfxa1)a2}
линейно по переменной $a_2$. Из равенства
\EqRef{Gateaux derivative of map df, D vector space}
следует, что отображение
\ShowEq{d(dfxa1)a2}
линейно по переменной $a_1$.

\begin{definition}
\label{definition: Gateaux derivative of Second Order, D vector space}
Полилинейное отображение
\ShowEq{Gateaux derivative of Second Order, D vector space def}
\ShowEq{Gateaux derivative of Second Order, D vector space}
называется
\AddIndex{производной Гато второго порядка}
{Gateaux derivative of Second Order} отображения $f$.
\qed
\end{definition}

\begin{remark}
\label{remark: differential L(D;V,V;W)}
Согласно определению
\ref{definition: Gateaux derivative of Second Order, D vector space}
при заданном $x$ производная Гато второго порядка
\ShowEq{differential L(D;V,V;W), 1}.
Следовательно, производная Гато второго порядка отображения $f$ является отображением
\ShowEq{differential L(D;V,V;W)}
\end{remark}

\begin{theorem}
\label{theorem: Gateaux Differential of Second Order, D vector space}
Допустим \eV V - базис в $D$\Hyph векторном пространстве $V$.
Допустим \eV W - базис в $D$\Hyph векторном пространстве $W$.
Производная Гато второго порядка отображения $f$
относительно базиса \eV V и
базиса \eV W
имеет вид
\ShowEq{Gateaux differential of Second Order, D vector space}
\ShowEq{Differential of Second Order, D vector space, representation}
\end{theorem}
\begin{proof}
Следствие определения
\ref{definition: Gateaux derivative of Second Order, D vector space}
и теоремы
\ePrints{0812.4763}
\ifx\Semafor\ValueOn
\ref{theorem: polylinear map, D vector space}.
\else
\xRef{0701.238}{theorem: polylinear map, D vector space}.
\fi
\end{proof}

\begin{definition}
Мы будем называть выражение
\ShowEq{component of Gateaux derivative of Second Order, D vector space}
\AddIndex{компонентой производной Гато второго порядка}
{component of Gateaux derivative of Second Order} отображения $f(x)$.
\qed
\end{definition}

\begin{definition}
\ShowEq{Gateaux partial derivative of Second Order, D vector space}
Пусть $D$ - тело характеристики $0$.
Допустим \eV V - базис в $D$\Hyph векторном пространстве $V$.
Допустим \eV W - базис в $D$\Hyph векторном пространстве $W$.
Частная производная Гато
\ShowEq{definition Gateaux partial derivative of Second Order, D vector space}
называется \AddIndex{смешанной частной производной Гато}
{Gateaux partial derivative of Second Order}
отображения $f^{\gik}$ по переменным $v^{\gii}$, $v^{\gij}$.
\qed
\end{definition}

\begin{theorem}
\label{theorem: Gateaux partial derivative of Second Order, D vector space}
Пусть $D$ - тело характеристики $0$.\footnote{Доказательство теоремы сделано
по аналогии с доказательством теоремы \citeBib{Fihtengolts: Calculus volume 1},
с. 405, 406.}
Допустим \eV V - базис в $D$\Hyph векторном пространстве $V$.
Допустим \eV W - базис в $D$\Hyph векторном пространстве $W$.
Пусть частные производные Гато отображения
\ShowEq{f:V->W}
непрерывны и дифференцируемы в смысле Гато в области $U\subset V$.
Пусть смешанные частные производные Гато второго порядка
непрерывны в области $U\subset V$.
Тогда на множестве $U$ смешанные частные производные Гато
удовлетворяют равенству
\ShowEq{Gateaux partial derivatives equal, D vector space}
\end{theorem}
\begin{proof}
Для доказательства теоремы мы будем пользоваться обозначением
$f^{\gik}(v)=f^{\gik}(v^{\gii},v^{\gij})$,
подразумевая, что остальные переменные имеют заданные значения.
Утверждение теоремы следует из следующей цепочки равенств
\ShowEq{Gateaux partial derivatives equal, 1, D vector space}

\ifx\texFuture\Defined
Рассмотрим выражение
\begin{equation}
W=t^{-2}(f^k(x^i+th^i,x^j+th^j)-f^k(x^i+th^i,x^j)-f^k(x^i,x^j+th^j)+f^k(x^i,x^j))
\EqLabel{Gateaux partial derivative of Second Order, D vector space, 1}
\end{equation}
Так как функция $f^k$ дифференцируема в смысле Гато и её частные производные Гато непрерывны,
то из теоремы \ref{theorem: expansion of Gateaux differential, D vector space},
определения \ref{definition: Gateaux partial derivative, D vector space}
и равенств \EqRef{Gateaux differential of map, t, division ring},
\EqRef{Gateaux partial derivative of Second Order, D vector space, 1}
следует
\begin{equation}
W=t^{-2}
\left(
\frac{\partial f^k(x^i+th^i,x^j)}{\partial x^j}(th^j)
-\frac{\partial f^k(x^i,x^j)}{\partial x^j}(th^j)
\right)
\EqLabel{Gateaux partial derivative of Second Order, D vector space, 2}
\end{equation}
Так как производная Гато
мультипликативна над полем действительных чисел,
то из равенства \EqRef{Gateaux partial derivative of Second Order, D vector space, 2}
следует
\begin{equation}
W=t^{-1}
\left(
\frac{\partial f^k(x^i+th^i,x^j)}{\partial tx^j}(h^j)
-\frac{\partial f^k(x^i,x^j)}{\partial tx^j}(h^j)
\right)
\EqLabel{Gateaux partial derivative of Second Order, D vector space, 3}
\end{equation}
Так как отображение
$\displaystyle\frac{\partial f^k(x^i,x^j)}{\partial x^j}(h^j)$
дифференцируемо и его частные производные непрерывны,
то из теоремы \ref{theorem: expansion of Gateaux differential, D vector space},
определения \ref{definition: Gateaux partial derivative, D vector space}
и равенств \EqRef{Gateaux differential of map, t, division ring},
\EqRef{Gateaux partial derivative of Second Order, D vector space, 3}
следует
\begin{equation}
W=t^{-1}
\frac{\partial}{\partial x^i}
\left(
\frac{\partial f^k(x^i+th^i,x^j)}{\partial x^j}(h^j)
\right)
(th^i)
\EqLabel{Gateaux partial derivative of Second Order, D vector space, 4}
\end{equation}
Так как производная Гато
мультипликативна над полем действительных чисел,
пользуясь определением
\EqRef{definition Gateaux partial derivative of Second Order, D vector space},
мы получим
\begin{equation}
W=
\frac{\partial^2 f^k(x^i,x^j)}{\partial x^i\partial x^j}(h^j,h^i)
\EqLabel{Gateaux partial derivative of Second Order, D vector space, 5}
\end{equation}
Применяя к выражению
\EqRef{Gateaux partial derivative of Second Order, D vector space, 1}
приведенные выше преобразования сперва к переменной $x^i$, а затем
к переменной $x^j$, мы получим
\begin{equation}
W=
\frac{\partial^2 f^k(x^i,x^j)}{\partial x^j\partial x^i}(h^i,h^j)
\EqLabel{Gateaux partial derivative of Second Order, D vector space, 6}
\end{equation}
Равенство \EqRef{Gateaux partial derivative of Second Order, D vector space}
следует из равенств
\EqRef{Gateaux partial derivative of Second Order, D vector space, 5},
\EqRef{Gateaux partial derivative of Second Order, D vector space, 6}.
\fi
\end{proof}

По индукции, предполагая, что определена производная Гато
$\partial^{n-1} f(x)$ порядка $n-1$, мы определим
\ShowEq{Gateaux derivative of Order n, D vector space}
\AddIndex{производную Гато порядка $n$}
{Gateaux derivative of Order n} отображения $f$.
Мы будем также полагать $\partial^0 f(x)=f(x)$.

\section{Однородное отображение}

\begin{definition}
Отображение
\ShowEq{f:V->W}
$D$\Hyph векторного пространства $V$ в
$D$\Hyph векторное пространство $W$
называется \AddIndex{однородным отображением степени $k$ над полем $F$}
{homogeneous map of degree over field, D vector space},
если для любого $a\in F$
\ShowEq{homogeneous map of degree k, D vector space}
\qed
\end{definition}

\begin{theorem}[теорема Эйлера]
\label{theorem: Euler theorem, homogeneous map, D vector space}
Пусть отображение
\ShowEq{f:V->W}
$D$\Hyph векторного пространства $V$ в
$D$\Hyph векторное пространство $W$
однородно степени $k$ над полем $F\subset Z(D)$.
\ShowEq{Euler theorem, homogeneous map, D vector space}
\end{theorem}
\begin{proof}
Продифференцируем равенство
\EqRef{homogeneous map of degree k, D vector space}
по $a$\footnote{Для отображения поля справедливо
\[
\partial f(x)(h)=\frac{df(x)}{dx}h
\]}
\ShowEq{homogeneous map of degree k, D vector space, 1}
Из теоремы
\ref{theorem: composite map, differential, D vector space}
следует
\ShowEq{homogeneous map of degree k, D vector space, 2}
Из теоремы \ref{theorem: Gateaux derivative over field F, D vector space}
и равенства \EqRef{homogeneous map of degree k, D vector space, 2}
следует
\ShowEq{homogeneous map of degree k, D vector space, 3}
Очевидно
\ShowEq{homogeneous map of degree k, D vector space, 4}
Подставим \EqRef{homogeneous map of degree k, D vector space, 3}
и \EqRef{homogeneous map of degree k, D vector space, 4}
в \EqRef{homogeneous map of degree k, D vector space, 1}
\ShowEq{homogeneous map of degree k, D vector space, 5}
Так как $\Delta a\ne 0$, то
\EqRef{Euler theorem, homogeneous map, D vector space}
следует из
\EqRef{homogeneous map of degree k, D vector space, 5}
при условии $a=1$.
\end{proof}

%\begin{theorem}
%\label{theorem: Euler theorem, homogeneous map}
Пусть отображение
\ShowEq{f:V->W}
$D$\Hyph векторного пространства $V$ в
$D$\Hyph векторное пространство $W$
однородно степени $k$ над полем $F\subset Z(D)$.
%\end{theorem}
%\begin{proof}
Из теоремы \ref{theorem: Gateaux derivative over field F, D vector space}
следует
\ShowEq{homogeneous map of degree k, D vector space, d1}
Из равенств \EqRef{Euler theorem, homogeneous map, D vector space},
\EqRef{homogeneous map of degree k, D vector space}
следует
\ShowEq{homogeneous map of degree k, D vector space, d2}
Из равенств \EqRef{homogeneous map of degree k, D vector space, d1},
\EqRef{homogeneous map of degree k, D vector space, d2}
следует
\ShowEq{homogeneous map of degree k, D vector space, d3}
Однако из равенства
\EqRef{homogeneous map of degree k, D vector space, d3}
не следует,
что отображение
\ShowEq{homogeneous map of degree k, D vector space, d4}
однородно степени $k-1$ над полем $F$.
%\end{proof}


==> Symbol.English.tex <==
%auto-ignore
\def\indexname{Special Symbols and Notations}
\OpenIndex

\SetIndexSpace%A%0
\Symb%A/0
   {minor matrix}%
   {A from b a}%
\Symb%A/0
   {minor matrix}%
   {A from columns T}%
\Symb%A/0
   {minor matrix}%
   {A from rows S}%
\Symb%A/0
   {set of vectors whose expansion relative to the basis $\Basis e$ converges normally}%
   {A plus Schauder}%
\Symb%A/0
   {minor matrix}%
   {A without column a}%
\Symb%A/0
   {minor matrix}%
   {A without columns T}%
\Symb%A/0
   {minor matrix}%
   {A without row b}%
\Symb%A/0
   {minor matrix}%
   {A without rows S}%
\Symb%A/0
   {$A\CRcirc$\Hyph linear combination}%
   {ACRcirc linear combination 1}%
\Symb%A/0
   {$A\CRcirc$\Hyph linear combination}%
   {ACRcirc linear combination 2}%
\Symb%A/0
   {active representation of group $G(f)$ in basis manifold $\mathcal B(f)$}%
   {active representation in basis manifold}%
\Symb%A/0
   {active representation of group $G(\Vector f)$ in basis manifold $\mathcal B(\Vector f)$}%
   {active representation in basis manifold, tower of representations}%
\Symb%A/0
   {affine space}%
   {affine space, division ring}%
\Symb%A/0
   {$A$\Hyph algebra of polynomials over $D$\Hyph algebra $A$}%
   {algebra of polynomials over algebra}%
\Symb%A/0
   {algebra of polynomials over $D$\Hyph algebra $A$}%
   {algebra of polynomials over D algebra}%
\Symb%A/0
   {algebra of rational mappings of algebra $A$}%
   {algebra of rational mappings of algebra}%
\Symb%A/0
   {affine space}%
   {An}%
\Symb%A/0
   {associator of $D$\Hyph algebra}%
   {associator of algebra}%
\Symb%A/0
   {\subs row ($c$\hyph row) of matrix}%
   {c row}%
\Symb%A/0
   {commutator of $D$\Hyph algebra}%
   {commutator of algebra}%
\Symb%A/0
   {component of linear map}%
   {component of linear map, vector}%
\Symb%A/0
   {component $p$ of polylinear mapping $\Vector A$}%
   {component of polyadditive map, D vector space}%
\Symb%A/0
   {component of polylinear map}%
   {component of polylinear map, vector}%
\Symb%A/0
   {conjugated $D$\Hyph  module}%
   {conjugated D module}%
\Symb%A/0
   {linear combination of vectors of $A$\Hyph module}%
   {CR linear combination in A module}%
\Symb%A/0
   {\CR power of element $A$ of biring}%
   {cr power}%
\Symb%A/0
   {\CR inverse element of biring}%
   {cr-inverse element}%
\Symb%A/0
   {\CR product of matrices}%
   {cr-product of matrices}%
\Symb%A/0
   {derivative of left shift}%
   {derivative of left shift}%
\Symb%A/0
   {derivative of left shift in $1$\Hyph parameter Lie group}%
   {derivative of left shift, 1-Parameter Group}%
\Symb%A/0
   {derivative of left shift in $1$\Hyph parameter Lie D group}%
   {derivative of left shift, 1-Parameter Group, algebra}%
\Symb%A/0
   {}%
   {derivative of right shift}%
\Symb%A/0
   {}%
   {derivative of right shift}%
\Symb%A/0
   {derivative of right shift in $1$\Hyph parameter Lie group}%
   {derivative of right shift, 1-Parameter Group}%
\Symb%A/0
   {derivative of right shift in $1$\Hyph parameter Lie D group}%
   {derivative of right shift, 1-Parameter Group, algebra}%
\Symb%A/0
   {derivative of left shift}%
   {derivative of Tstar shift}%
\Symb%A/0
   {\drc vector}%
   {drc vector}%
\Symb%A/0
   {coordinates of vector $a$ relative to Hamel basis}%
   {Hamel basis, coordinates}%
\Symb%A/0
   {hermitian conjugation in division ring}%
   {hermitian conjugation, division ring}%
\Symb%A/0
   {tensor inverse to tensor $a$}%
   {inverse tensor}%
\Symb%A/0
   {$(^j_i)$\hyph\CR quasideterminant}%
   {j i CR quasideterminant definition}%
\Symb%A/0
   {$(ji)$\hyph quasideterminant of matrix $\bfA$}%
   {j i quasideterminant definition}%
\Symb%A/0
   {$(^j_i)$\hyph \RC quasideterminant}%
   {j i RC-quasideterminant definition}%
\Symb%A/0
   {$(^j_i)$\hyph $\RCcirc$\Hyph quasideterminant}%
   {j i RCcirc-quasideterminant definition}%
\Symb%A/0
   {left fraction}%
   {left fraction}%
\Symb%A/0
   {left principal ideal}%
   {left principal ideal}%
\Symb%A/0
   {left shift in $D$\Hyph algebra}%
   {left shift, D algebra}%
\Symb%A/0
   {linear combination of vectors of $A$\Hyph module}%
   {linear combination in A module}%
\Symb%A/0
   {transformation of matrix}%
   {matrix, replacing its column}%
\Symb%A/0
   {transformation of matrix}%
   {matrix, replacing its row}%
\Symb%A/0
   {$A$\Hyph module of homogeneous polynomials over $D$\Hyph algebra $A$}%
   {module of homogeneous polynomials over algebra}%
\Symb%A/0
   {norm on $D$\Hyph module}%
   {norm on D module}%
\Symb%A/0
   {opposite algebra to algebra $A$}%
   {opposite algebra}%
\Symb%A/0
   {orbit of linear mapping}%
   {orbit of linear mapping}%
\Symb%A/0
   {derivative}%
   {overline nabla_l, definition 2}%
\Symb%A/0
   {partial linear map}%
   {partial linear map}%
\Symb%A/0
   {principal ideal}%
   {principal ideal}%
\Symb%A/0
   {quasideterminant of matrix $\bfA$}%
   {quasideterminant definition}%
\Symb%A/0
   {\sups row ($r$\hyph row) of matrix}%
   {r row}%
\Symb%A/0
   {\RC power of element $A$ of biring}%
   {rc power}%
\Symb%A/0
   {\RC inverse element of biring}%
   {rc-inverse element}%
\Symb%A/0
   {\RC product of matrices}%
   {rc-product of matrices}%
\Symb%A/0
   {\RC quasideterminant}%
   {RC-quasideterminant definition}%
\Symb%A/0
   {$\RCcirc$\Hyph quasideterminant}%
   {RCcirc-quasideterminant definition}%
\Symb%A/0
   {\rcd vector}%
   {rcd vector}%
\Symb%A/0
   {right principal ideal}%
   {right principal ideal}%
\Symb%A/0
   {right shift in $D$\Hyph algebra}%
   {right shift, D algebra}%
\Symb%A/0
   {coordinates of vector $a$ relative to Schauder basis}%
   {Schauder basis, coordinates}%
\Symb%A/0
   {set of invertible elements of algebra $A$}%
   {set of invertible elements of algebra}%
\Symb%A/0
   {set of zeros of algebra $A$}%
   {set of zeros of algebra}%
\Symb%A/0
   {set of polylinear maps of rings $R_1$, ..., $R_n$ into module $S$}%
   {set polylinear maps, ring}%
\Symb%A/0
   {skew product of vectors $\Vector a_1$, ..., $\Vector a_m$}%
   {skew product of vectors}%
\Symb%A/0
   {right shift}%
   {starT shift}%
\Symb%A/0
   {\sT shift}%
   {starT shift, fibered group}%
\Symb%A/0
   {tensor power of algebra $A$}%
   {tensor power of algebra}%
\Symb%A/0
   {tensor product of algebras}%
   {tensor product of algebras}%
\Symb%A/0
   {left shift}%
   {Tstar shift}%
\Symb%A/0
   {\Ts shift}%
   {Tstar shift, fibered group}%
\Symb%A/0
   {anholonomic coordinates of vector}%
   {vector anholonomic coordinates}%
\Symb%A/0
   {holonomic coordinates of vector}%
   {vector holonomic coordinates}%

\SetIndexSpace%B%0
\Symb%B/0
   {basis manifold of \rcd vector space $\Vector V$}%
   {basis manifold of rcd vector space}%
\Symb%B/0
   {basis manifold of vector space}%
   {basis manifold of vector space}%
\Symb%B/0
   {basis manifold of representation $f$}%
   {basis manifold representation F algebra}%
\Symb%B/0
   {basis manifold of tower of representations $\Vector f$}%
   {basis manifold tower of representations}%
\Symb%B/0
   {basis manifold of affine space}%
   {Basis Manifold, Affine Space}%
\Symb%B/0
   {basis manifold of \rcd affine space}%
   {Basis Manifold, rcd Affine Space, division ring}%
\Symb%B/0
   {basis manifold of central affine space}%
   {BCAn}%
\Symb%B/0
   {basis manifold of Euclid space}%
   {BEn}%
\Symb%B/0
   {Borel algebra}%
   {Borel algebra}%
\Symb%B/0
   {Cartesian power $\Bundle A$ of bundle $\Bundle B$}%
   {Cartesian power A of bundle B}%
\Symb%B/0
   {Cartesian power $A$ of set $B$}%
   {Cartesian power of set}%
\Symb%B/0
   {closed ball}%
   {closed ball}%
\Symb%B/0
   {basis manifold of central affine space}%
   {FCAn}%
\Symb%B/0
   {basis manifold of Euclid space}%
   {FEn}%
\Symb%B/0
   {lattice of subrepresentations of representation $f$}%
   {lattice of subrepresentations}%
\Symb%B/0
   {lattice of towers of subrepresentations of tower of representations $\Vector f$}%
   {lattice of subrepresentations, tower of representations}%
\Symb%B/0
   {open ball}%
   {open ball}%
\Symb%B/0
   {product of objects $B_1$, ..., $B_n$ in category $\mathcal A$}%
   {product of objects in category, 1 n}%
\Symb%B/0
   {right fraction}%
   {right fraction}%
\Symb%B/0
   {tensor power of representation}%
   {tensor power of representation}%
\Symb%B/0
   {tensor product of representations}%
   {tensor product of representations}%

\SetIndexSpace%C%0
\Symb%C/0
   {$\sigma$\Hyph algebra of sets measurable with respect to measure $\mu$}%
   {algebra of sets measurable with respect to measure}%
\Symb%C/0
   {central affine space}%
   {CAn}%
\Symb%C/0
   {central affine space}%
   {central affine space}%
\Symb%C/0
   {$j$th column determinant of matrix $\bfA$}%
   {column determinant}%
\Symb%C/0
   {$\CRcirc$\Hyph product of matrices of maps}%
   {cr product of matrices of mappings}%
\Symb%C/0
   {left structural constant of Lie algebra}%
   {left structural constant of Lie algebra}%
\Symb%C/0
   {right structural constant of Lie algebra}%
   {right structural constant of Lie algebra}%
\Symb%C/0
   {set of continuous multivariable maps}%
   {set continuous multivariable maps}%
\Symb%C/0
   {structural constants}%
   {structural constants}%

\SetIndexSpace%D%0
\Symb%D/0
   {basis vector of representation of Lie group}%
   {basis vector of representation of Lie group}%
\Symb%D/0
   {basis vector of representation of Lie group over algebra $A$}%
   {basis vector of representation of Lie group over algebra A}%
\Symb%D/0
   {coordinates of basis vector of representation of Lie group over algebra $A$}%
   {basis vector of representation of Lie group over algebra A, coordinates}%
\Symb%D/0
   {coordinates of basis vector of representation of Lie group}%
   {basis vector of representation of Lie group, coordinates}%
\Symb%D/0
   {component of the G\^ateaux derivative of map $f(x)$}%
   {component of Gateaux derivative}%
\Symb%D/0
   {component of the G\^ateaux derivative of map $f(x)$}%
   {component of Gateaux derivative of map, D vector space, short}%
\Symb%D/0
   {component of the G\^ateaux derivative of second order of map $f(x)$}%
   {component of Gateaux derivative of Second Order}%
\Symb%D/0
   {component of the G\^ateaux derivative of second order of map $f(x)$}%
   {component of Gateaux derivative of Second Order, D vector space}%
\Symb%D/0
   {component of the G\^ateaux derivative of map $f(x)$}%
   {component of Gateaux derivative, vector space}%
\Symb%D/0
   {conjugation in algebra}%
   {conjugation in algebra}%
\Symb%D/0
   {conjugation in ring}%
   {conjugation in ring}%
\Symb%D/0
   {coordinate \Drc vector bundle}%
   {coordinate drc vector bundle}%
\Symb%D/0
   {coordinate \rcd vector space}%
   {coordinate rcd vector space}%
\Symb%D/0
   {coordinate reference frame}%
   {coordinate reference frame, extensive definition}%
\Symb%D/0
   {diagonal in bundle $\Bundle A$}%
   {diagonal in bundle, 1}%
\Symb%D/0
   {direct product of division rings $D_1$, ..., $D_n$}%
   {direct product of division rings, 1 n}%
\Symb%D/0
   {double determinant of matrix $\bfA$}%
   {double determinant}%
\Symb%D/0
   {the Fr\'echet \Ds derivative of map $f$ of division ring}%
   {Frechet Dstar derivative of map, division ring}%
\Symb%D/0
   {the G\^ateaux \dcr derivative of map $f$ of $D$\Hyph vector space $V$ to $D$\Hyph vector space $W$}%
   {Gateaux dcr derivative of map, D vector space}%
\Symb%D/0
   {the G\^ateaux derivative of map $f$}%
   {Gateaux derivative of map}%
\Symb%D/0
   {the G\^ateaux derivative of map $f$}%
   {Gateaux derivative of map, fraction}%
\Symb%D/0
   {the G\^ateaux derivative of order $n$}%
   {Gateaux derivative of Order n}%
\Symb%D/0
   {the G\^ateaux derivative of order $n$ of map $f$ of division ring}%
   {Gateaux derivative of Order n, division ring}%
\Symb%D/0
   {the G\^ateaux derivative of order $n$ of map $f$ of algebra}%
   {Gateaux derivative of Order n, fraction, algebra}%
\Symb%D/0
   {the G\^ateaux derivative of order $n$ of map $f$ of division ring}%
   {Gateaux derivative of Order n, fraction, division ring}%
\Symb%D/0
   {the G\^ateaux derivative of second order}%
   {Gateaux derivative of Second Order}%
\Symb%D/0
   {the G\^ateaux derivative of second order of mapping $f$ of algebra}%
   {Gateaux derivative of Second Order, fraction, algebra}%
\Symb%D/0
   {the G\^ateaux derivative of second order of map $f$ of division ring}%
   {Gateaux derivative of Second Order, fraction, division ring}%
\Symb%D/0
   {the G\^ateaux differential of map $f$}%
   {Gateaux differential of map, scalar}%
\Symb%D/0
   {the G\^ateaux differential of map $f$}%
   {Gateaux differential of map, vector}%
\Symb%D/0
   {the G\^ateaux \Ds derivative of map $f$ of division ring $D$}%
   {Gateaux Dstar derivative of map, division ring}%
\Symb%D/0
   {the G\^ateaux Jacobian of map of $D$\Hyph vector space}%
   {Gateaux Jacobian of map, D vector space}%
\Symb%D/0
   {the G\^ateaux partial \dcr derivative of map $f^{\gi b}$ with respect to variable $v^{\gi a}$}%
   {Gateaux partial dcr derivative of map, 1, D vector space}%
\Symb%D/0
   {the G\^ateaux partial \dcr derivative of map $f^{\gi b}$ with respect to variable $v^{\gi a}$}%
   {Gateaux partial dcr derivative of map, 2, D vector space}%
\Symb%D/0
   {the G\^ateaux partial \dcr derivative of map $f^{\gi b}$ with respect to variable $v^{\gi a}$}%
   {Gateaux partial dcr derivative of map, 3, D vector space}%
\Symb%D/0
   {the G\^ateaux partial derivative}%
   {Gateaux partial derivative}%
\Symb%D/0
   {the G\^ateaux mixed partial derivative}%
   {Gateaux partial derivative of Second Order}%
\Symb%D/0
   {the G\^ateaux partial \rcd derivative of map $f^{\gi b}$ with respect to variable $x^{\gi a}$}%
   {Gateaux partial rcd derivative of map, 1, D vector space}%
\Symb%D/0
   {the G\^ateaux partial \rcd derivative of map $f^{\gi b}$ with respect to variable $x^{\gi a}$}%
   {Gateaux partial rcd derivative of map, 2, D vector space}%
\Symb%D/0
   {the G\^ateaux partial \rcd derivative of map $f^{\gi b}$ with respect to variable $x^{\gi a}$}%
   {Gateaux partial rcd derivative of map, 3, D vector space}%
\Symb%D/0
   {the G\^ateaux \rcd derivative of map $f$ of $D$\hyph vector space $V$ to $D$\hyph vector space $W$}%
   {Gateaux rcd derivative of map, D vector space}%
\Symb%D/0
   {the G\^ateaux \sD derivative of map $f$ of division ring $D$}%
   {Gateaux starD derivative of map, division ring}%
\Symb%D/0
   {matrices vector space}%
   {matrices vector space}%
\Symb%D/0
   {Cartan derivative}%
   {overbrace D}%
\Symb%D/0
   {derivative}%
   {overline D}%
\Symb%D/0
   {derivative $e_{(k)}$}%
   {partial(k)}%
\Symb%D/0
   {product of map over scalar}%
   {product of map over scalar}%
\Symb%D/0
   {\subs rows \drc vector space}%
   {r rows drc vector space}%
\Symb%D/0
   {speed of deviation}%
   {speed of deviation}%
\Symb%D/0
   {standard component of the G\^ateaux derivative}%
   {standard component of Gateaux derivative}%
\Symb%D/0
   {tensor product of division rings}%
   {tensor product of division rings}%
\Symb%D/0
   {tensor product of rings}%
   {tensor product of rings}%
\Symb%D/0
   {vector space type}%
   {vector space type}%

\SetIndexSpace%E%0
\Symb%E/0
   {$A\CRcirc$\Hyph basis for module}%
   {A CRcirc basis, module over algebra}%
\Symb%E/0
   {Jacobian matrix of left shift}%
   {aE, quaternion, Jacobian matrix}%
\Symb%E/0
   {affine basis}%
   {Affine Basis}%
\Symb%E/0
   {basis of vector space}%
   {Basis e}%
\Symb%E/0
   {basis in vector space $\Vector V$}%
   {basis in V}%
\Symb%E/0
   {basis of $D$\Hyph module $\mathcal L(D;A_1;A_2)$}%
   {basis L(A1,A2)}%
\Symb%E/0
   {basis of vector space}%
   {basis, vector space}%
\Symb%E/0
   {basis of $(n)$\hyph vector space}%
   {basis,n vector space}%
\Symb%E/0
   {Cartesian power of total spaces}%
   {Cartesian power of total spaces}%
\Symb%E/0
   {Cartesian product of total spaces}%
   {Cartesian product of total spaces, definition 1}%
\Symb%E/0
   {central affine basis}%
   {Central Affine Basis}%
\Symb%E/0
   {basis for \Drc vector bundle}%
   {drc basis, vector bundle}%
\Symb%E/0
   {form of reference frame}%
   {dual forms, reference frame}%
\Symb%E/0
   {Euclid space}%
   {Euclid space}%
\Symb%E/0
   {Euclid space}%
   {Euclid space, division ring}%
\Symb%E/0
   {Hamel basis}%
   {Hamel basis}%
\Symb%E/0
   {identical transformation of bundle}%
   {identical transformation of bundle}%
\Symb%E/0
   {linear automorphism of quaternioin algebra}%
   {mapping E, quaternion}%
\Symb%E/0
   {linear automorphism of quaternioin algebra}%
   {mapping E_1, quaternion}%
\Symb%E/0
   {linear automorphism of quaternioin algebra}%
   {mapping E_2, quaternion}%
\Symb%E/0
   {orthonornal basis}%
   {Orthonornal Basis}%
\Symb%E/0
   {pseudo Euclid space}%
   {pseudo Euclid space}%
\Symb%E/0
   {pseudo Euclid space}%
   {pseudo Euclid space, division ring}%
\Symb%E/0
   {quaternion algebra over the field $F$}%
   {quaternion algebra over the field}%
\Symb%E/0
   {quaternion division algebra over the field}%
   {quaternion division algebra over the fieldL}%
\Symb%E/0
   {$\RCcirc A$\Hyph linear combination}%
   {RCcircA linear combination 1}%
\Symb%E/0
   {$\RCcirc A$\Hyph linear combination}%
   {RCcircA linear combination 2}%
\Symb%E/0
   {\rcd affine basis}%
   {rcd affine basis, division ring}%
\Symb%E/0
   {reduced Cartesian product of total spaces}%
   {reduced Cartesian product of total spaces, definition 1}%
\Symb%E/0
   {Schauder basis}%
   {Schauder basis}%
\Symb%E/0
   {set of nonsingular \sT transformations of bundle $\Bundle E$}%
   {set of starT nonsingular transformations of bundle}%
\Symb%E/0
   {set of nonsingular \Ts transformations of bundle $\Bundle E$}%
   {set of Tstar nonsingular transformations of bundle}%
\Symb%E/0
   {standard coordinates of basis}%
   {standard coordinates of basis}%
\Symb%E/0
   {standard coordinates of reference frame}%
   {standard coordinates of reference frame}%
\Symb%E/0
   {vector field of reference frame}%
   {vector field of reference frame}%
\Symb%E/0
   {vector of basis}%
   {vector of basis}%

\SetIndexSpace%F%0
\Symb%F/0
   {coordinates of basis in \sups rows \rcd vector space}%
   {basis coordinates, c rows rcd vector space}%
\Symb%F/0
   {coordinates of basis in \subs rows \drc vector space}%
   {basis coordinates, r rows drc vector space}%
\Symb%F/0
   {basis for \sups rows \rcd vector space}%
   {basis, c rows rcd vector space}%
\Symb%F/0
   {basis for \subs rows \drc vector space}%
   {basis, r rows drc vector space}%
\Symb%F/0
   {central affine basis}%
   {Central Affine Basis, division ring}%
\Symb%F/0
   {component of linear map $f$ of division ring}%
   {component of linear map, division ring}%
\Symb%F/0
   {component of polylinear map}%
   {component of polylinear map}%
\Symb%F/0
   {fibered morphism from bundle $\Bundle A$ into $\Bundle B$}%
   {fibered morphism from A into B}%
\Symb%F/0
   {filter $\mathfrak{F}$ converges to set $A$}%
   {filter converges}%
\Symb%F/0
   {homomorphism of fibered universal algebras}%
   {homomorphism of fibered universal algebras}%
\Symb%F/0
   {inverse fibered correspondence}%
   {inverse fibered correspondence, 1}%
\Symb%F/0
   {inverse reduced fibered correspondence}%
   {inverse reduced fibered correspondence, 1}%
\Symb%F/0
   {map to Cartesian product}%
   {map to Cartesian product}%
\Symb%F/0
   {norm of functional}%
   {norm of functional}%
\Symb%F/0
   {norm of map}%
   {norm of map}%
\Symb%F/0
   {norm of polylinear map}%
   {norm of polymap}%
\Symb%F/0
   {norm of representation}%
   {norm of representation}%
\Symb%F/0
   {representation orbit of group $G$}%
   {orbit of Tstar representation of group}%
\Symb%F/0
   {orthonornal basis}%
   {Orthonornal Basis, division ring}%
\Symb%F/0
   {quaternion algebra  over field ${\rm {\mathbb{F}}}$}%
   {quaternion algebra F a b}%
\Symb%F/0
   {reference frame}%
   {reference frame}%
\Symb%F/0
   {reference frame, extensive definition}%
   {reference frame, extensive definition}%
\Symb%F/0
   {standard component of biadditive map $f$ over field $F$}%
   {standard component of biadditive map, division ring}%
\Symb%F/0
   {standard component of linear map}%
   {standard component of linear map, G}%
\Symb%F/0
   {standard component of polylinear map}%
   {standard component of polylinear map}%
\Symb%F/0
   {standard component of quadratic map $f$ over field $F$}%
   {standard component of quadratic map, division ring}%
\Symb%F/0
   {standard component of tensor}%
   {standard component of tensor}%
\Symb%F/0
   {sum of linear maps}%
   {sum of linear maps}%

\SetIndexSpace%G%0
\Symb%G/0
   {affine transformation group}%
   {affine transformation group}%
\Symb%G/0
   {\CR matrix group}%
   {cr-matrix group}%
\Symb%G/0
   {affine transformation group}%
   {drc affine transformation group}%
\Symb%G/0
   {fibered little group of section $h$}%
   {fibered little group}%
\Symb%G/0
   {fibered stability group of section $h$}%
   {fibered stability group}%
\Symb%G/0
   {algebra Lie of group Lie}%
   {g}%
\Symb%G/0
   {left defined algebra Lie of group Lie}%
   {gl}%
\Symb%G/0
   {right defined algebra Lie of group Lie}%
   {gr}%
\Symb%G/0
   {group of automorphisms of representation $f$}%
   {group of automorphisms of representation}%
\Symb%G/0
   {group of homomorphisms of vector space $\Vector V$}%
   {GV}%
\Symb%G/0
   {little group of $x$}%
   {little group}%
\Symb%G/0
   {orbit of effective covariant \sT representation of fibered group}%
   {orbit of effective covariant starT representation of fibered group}%
\Symb%G/0
   {orbit of effective covariant \sT representation of group}%
   {orbit of effective covariant starT representation of group}%
\Symb%G/0
   {orbit of effective covariant \Ts representation of fibered group}%
   {orbit of effective covariant Tstar representation of fibered group}%
\Symb%G/0
   {orbit of effective covariant \Ts representation of group}%
   {orbit of effective covariant Tstar representation of group}%
\Symb%G/0
   {product of groups $G_1$, ..., $G_n$}%
   {product of groups, 1 n}%
\Symb%G/0
   {\RC matrix group}%
   {rc-matrix group}%
\Symb%G/0
   {stability group of $x$}%
   {stability group}%

\SetIndexSpace%H%0
\Symb%H/0
   {Hadamard inverse of matrix}%
   {Hadamard inverse of matrix}%
\Symb%H/0
   {quaternion algebra}%
   {quaternion algebra H a b}%
\Symb%H/0
   {quaternion algebra over real field}%
   {quaternion algebra over real field}%

\SetIndexSpace%I%0
\Symb%I/0
   {infinitesimal generator of representation}%
   {infinitesimal generator I of representation}%
\Symb%I/0
   {infinitesimal generator of representation}%
   {infinitesimal generator i of representation}%
\Symb%I/0
   {Lie group infinitesimal generators}%
   {Lie group infinitesimal generators}%
\Symb%I/0
   {vector module of algebra $A$}%
   {vector module of algebra}%
\Symb%I/0
   {vector module of ring $D$}%
   {vector module of ring}%
\Symb%I/0
   {vector of element $d$ of algebra}%
   {vector of algebra}%
\Symb%I/0
   {vector of mapping $f$}%
   {vector of mapping}%
\Symb%I/0
   {vector of element $d$ of ring}%
   {vector of ring}%

\SetIndexSpace%J%0
\Symb%J/0
   {closure operator of representation $f$}%
   {closure operator, representation}%
\Symb%J/0
   {closure operator of tower of representations $\Vector f$}%
   {closure operator, tower of representations}%
\Symb%J/0
   {Jacobian matrix of right shift}%
   {Ea, quaternion, Jacobian matrix}%
\Symb%J/0
   {tower of subrepresentations of tower of representations $\Vector f$ generated by tuple of sets $\VX X$}%
   {subrepresentation generated by tuple of sets}%

\SetIndexSpace%K%0
\Symb%K/0
   {kernel of linear map}%
   {kernel of linear map}%

\SetIndexSpace%L%0
\Symb%L/0
   {left $ij$th cofactor of entry of matrix}%
   {left cofactor, matrix}%
\Symb%L/0
   {left double $ij$th cofactor of entry of matrix}%
   {left double cofactor}%
\Symb%L/0
   {left shift}%
   {left shift}%
\Symb%L/0
   {Lie derivative of connection}%
   {Lie derivative of connection}%
\Symb%L/0
   {Lie derivative of metric}%
   {Lie derivative of metric}%
\Symb%L/0
   {limit of correspondence $\Phi$ with respect to the filter $\mathfrak{F}$}%
   {limit of correspondence with respect to the filter}%
\Symb%L/0
   {limit of sequence}%
   {limit of sequence}%
\Symb%L/0
   {passive transformation}%
   {passive transformation}%
\Symb%L/0
   {set of \Acr linear maps of module $\Vector V$ into module $\Vector W$}%
   {set Acr linear maps, module}%
\Symb%L/0
   {$D$\Hyph module of continuous linear mappings of normed $D$\Hyph module $A_1$ into normed $D$\Hyph module $A_2$}%
   {set continuous linear mappings, module}%
\Symb%L/0
   {set of continuous linear maps}%
   {set continuous linear maps, vector}%
\Symb%L/0
   {set of continuous polylinear maps}%
   {set continuous polylinear maps}%
\Symb%L/0
   {\rcd vector space of linear maps of \drc vector space $V$ into \drc vector space $W$}%
   {set linear maps, drc vector space}%
\Symb%L/0
   {\drc vector space of linear maps of \rcd vector space $V$ into \rcd vector space $W$}%
   {set linear maps, rcd vector space}%
\Symb%L/0
   {set of linear maps}%
   {set linear maps, scalar}%
\Symb%L/0
   {set of linear maps}%
   {set linear maps, vector}%
\Symb%L/0
   {set of left-side nonsingular transformations of set $M$}%
   {set of left-side nonsingular transformations}%
\Symb%L/0
   {set of polylinear maps}%
   {set polylinear maps}%
\Symb%L/0
   {set of $n$\hyph linear maps}%
   {set polylinear maps An}%
\Symb%L/0
   {set of polylinear maps}%
   {set polylinear maps, D vector space}%
\Symb%L/0
   {set of polylinear maps of algebras $A_1$, ..., $A_n$ into algebra $A$}%
   {set polylinear maps, finite dimensional algebra}%
\Symb%L/0
   {set of \sT representations of division ring $S$ in additive group of division ring $R$}%
   {set sT representations, division ring}%
\Symb%L/0
   {set of \Ts representations of division ring $S$ in additive group of division ring $R$}%
   {set Ts representations, division ring}%

\SetIndexSpace%M%0
\Symb%M/0
   {set of maps to $\Omega$\Hyph group $A$}%
   {set of maps to Omega group}%
\Symb%M/0
   {set of \sT transformations of set $M$}%
   {set of starT transformations}%
\Symb%M/0
   {set of transformations of set $M$}%
   {set of transformations}%
\Symb%M/0
   {set of \Ts transformations of set $M$}%
   {set of Tstar transformations}%
\Symb%M/0
   {space of orbits of effective \sT covariant representation of the group}%
   {space of orbits of effective sT representation}%
\Symb%M/0
   {space of orbits of effective \Ts covariant representation of the group}%
   {space of orbits of effective Ts representation}%
\Symb%M/0
   {space of orbits of \Ts representation $f$ of group $G$ in set $M$}%
   {space of orbits of Ts representation}%

\SetIndexSpace%N%0
\Symb%N/0
   {norm of quaternion $x$}%
   {norm, quaternion algebra}%
\Symb%N/0
   {nucleus of $D$\Hyph algebra $A$}%
   {nucleus of algebra}%

\SetIndexSpace%O%0
\Symb%O/0
   {geometric object in coordinate representation defined in \rcd vector space}%
   {geometric object, coordinate rcd vector space}%
\Symb%O/0
   {geometric object in coordinate representation}%
   {geometric object, coordinate vector space}%
\Symb%O/0
   {geometric object defined in \rcd vector space}%
   {geometric object, rcd vector space}%
\Symb%O/0
   {octonion algebra}%
   {octonion algebra}%
\Symb%O/0
   {orbit of representation of fibered group $\Bundle G$}%
   {orbit of representation of fibered group}%
\Symb%O/0
   {orbit of representation of the group $G$}%
   {orbit of representation of group}%

\SetIndexSpace%P%0
\Symb%P/0
   {bundle}%
   {bundle}%
\Symb%P/0
   {bundle of level $2$}%
   {bundle of level 2}%
\Symb%P/0
   {bundle of level $n$}%
   {bundle of level n}%
\Symb%P/0
   {Cartesian power $n$ of bundle $\bundle{}{p}{E}{}$}%
   {Cartesian power of bundle}%
\Symb%P/0
   {Cartesian product of bundles}%
   {Cartesian product of bundles, definition 1}%
\Symb%P/0
   {passive representation of group $G(f)$ in basis manifold $\mathcal B(f)$}%
   {passive representation in basis manifold}%
\Symb%P/0
   {passive representation of group $G(\Vector f)$ in basis manifold $\mathcal B(\Vector f)$}%
   {passive representation in basis manifold, tower of representations}%
\Symb%P/0
   {reduced Cartesian product of bundles}%
   {reduced Cartesian product of bundles, definition 1}%
\Symb%P/0
   {set of nonsingular \sT transformations of bundle $\bundle{}pE{}$}%
   {set of starT nonsingular transformations of bundle, projection}%
\Symb%P/0
   {set of nonsingular \Ts transformations of bundle $\bundle{}pE{}$}%
   {set of Tstar nonsingular transformations of bundle, projection}%

\SetIndexSpace%R%0
\Symb%R/0
   {active transformation}%
   {active transformation}%
\Symb%R/0
   {\sups rows \rcd vector space}%
   {c rows rcd vector space}%
\Symb%R/0
   {Cartan curvature}%
   {Cartan curvature}%
\Symb%R/0
   {\CR rank of matrix}%
   {cr-rank of matrix}%
\Symb%R/0
   {diagonal in bundle  $\bundle{}pA{}$}%
   {diagonal in bundle, 2}%
\Symb%R/0
   {diagonal in bundle $\Bundle A$}%
   {diagonal in reduced bundle, 2}%
\Symb%R/0
   {image of $m$ under endomorphism $R$ of effective representation}%
   {endomorphism image, effective representation}%
\Symb%R/0
   {image of tuple $\VX a$ under endomorphism $\VX r$ of tower of effective representations}%
   {endomorphism image, tower of effective representations}%
\Symb%R/0
   {curvature}%
   {GLn curvature_overline}%
\Symb%R/0
   {$\RCcirc$\Hyph product of matrices of maps}%
   {rc product of matrices of mappings}%
\Symb%R/0
   {\RC rank of matrix}%
   {rc-rank of matrix}%
\Symb%R/0
   {right $ij$th cofactor of entry of matrix}%
   {right cofactor, matrix}%
\Symb%R/0
   {right double $ij$th cofactor of entry of matrix}%
   {right double cofactor}%
\Symb%R/0
   {right shift}%
   {right shift}%
\Symb%R/0
   {$i$th row determinant of matrix $\bfA$}%
   {row determinant}%
\Symb%R/0
   {scalar algebra of algebra $A$}%
   {scalar algebra of algebra}%
\Symb%R/0
   {scalar algebra of ring $D$}%
   {scalar algebra of ring}%
\Symb%R/0
   {scalar of element $d$ of algebra}%
   {scalar of algebra}%
\Symb%R/0
   {scalar of mapping $f$}%
   {scalar of mapping}%
\Symb%R/0
   {scalar of element $d$ of ring}%
   {scalar of ring}%
\Symb%R/0
   {set of right-side nonsingular transformations of set $M$}%
   {set of right-side nonsingular transformations}%

\SetIndexSpace%S%0
\Symb%S/0
   {composition of fibered correspondences}%
   {composition of fibered correspondences}%
\Symb%S/0
   {inverse fibered correspondence}%
   {inverse fibered correspondence, 2}%
\Symb%S/0
   {inverse reduced fibered correspondence}%
   {inverse reduced fibered correspondence, 2}%
\Symb%S/0
   {linear span in vector space}%
   {linear span, vector space}%
\Symb%S/0
   {image of basis $X$ under passive transformation $S$}%
   {passive transformation of basis, representation}%
\Symb%S/0
   {image of basis $\VX  X$ under passive transformation $\VX s$}%
   {passive transformation of basis, tower of representations}%
\Symb%S/0
   {symmetric group}%
   {symmetric group}%

\SetIndexSpace%T%0
\Symb%T/0
   {category of \Ts representations of $\Omega_1$\Hyph algebra $A$}%
   {category of Tstar representations of Omega1 algebra}%
\Symb%T/0
   {category of \Ts representations of $\Omega_1$\Hyph algebra from category $\mathcal A$}%
   {category of Tstar representations of Omega1 algebra from category}%
\Symb%T/0
   {tangent plane to group $G$}%
   {TaG}%
\Symb%T/0
   {trace of quaternion $x$}%
   {trace, quaternion algebra}%

\SetIndexSpace%V%0
\Symb%V/0
   {coordinate vector space}%
   {coordinate vector space}%
\Symb%V/0
   {coordinates in vector space}%
   {coordinates in vector space}%
\Symb%V/0
   {direct product of $\RCstar D_i$\hyph vector spaces $\Vector V_1$, ..., $\Vector V_n$}%
   {direct product, rcd vector space, 1 n}%
\Symb%V/0
   {dual space of \rcd vector space $\Vector V$}%
   {dual space of rcd vector space}%
\Symb%V/0
   {hermitian conjugated vector}%
   {hermitian conjugated vector}%
\Symb%V/0
   {tensor product of $D$\Hyph vector spaces}%
   {tensor product of D vector spaces}%
\Symb%V/0
   {tensor product of \Ds vector spaces}%
   {tensor product of Dstar vector spaces}%
\Symb%V/0
   {vector space}%
   {V}%

\SetIndexSpace%W%0
\Symb%W/0
   {set of coordinates of representation $J(f,X)$}%
   {coordinate set of representation}%
\Symb%W/0
   {set of tuples of coordinates of tower of representations $\Vector J(\Vector f,\VX X)$}%
   {coordinate set of tower of representations}%
\Symb%W/0
   {coordinates of basis $X'$ relative to basis $X$ of representation}%
   {coordinates of basis relative to basis, representation}%
\Symb%W/0
   {coordinates of element $m$ of representation $f$ relative to set $X$}%
   {coordinates of element relative to generating set, representation}%
\Symb%W/0
   {coordinates of element $m$ relative to set $X$}%
   {coordinates of element relative to set, representation}%
\Symb%W/0
   {tuple of coordinates of element $\Vector a*$ relative to tuple of sets $\VX X$}%
   {coordinates of element, tower of representations}%
\Symb%W/0
   {geometric object in coordinate representation defined in $\Omega_2$\Hyph algebra $M$}%
   {geometric object, coordinate representation g}%
\Symb%W/0
   {geometric object in coordinate representation defined in tuple of $\VX\Omega$\Hyph algebras $\VX A$}%
   {geometric object, coordinate tower of representations g}%
\Symb%W/0
   {geometric object defined in $\Omega_2$\Hyph algebra $M$}%
   {geometric object, representation g}%
\Symb%W/0
   {geometric object defined in tuple of $\VX\Omega$\Hyph algebras $\VX A$}%
   {geometric object, tower of representations g}%
\Symb%W/0
   {geometric object in vector space}%
   {geometric object, vector space}%
\Symb%W/0
   {set of coordinates of set $B\subset J(f,X)$}%
   {subset of coordinates of representation}%
\Symb%W/0
   {coordinates of tuple of sets $\VX B$ relative to tuple of sets $\VX X$}%
   {subset of coordinates of tower of representations}%
\Symb%W/0
   {coordinates of set $B_k$ relative to tuple of sets $\VX X$}%
   {subset of coordinates of tower of representations, k}%
\Symb%W/0
   {set of $\Omega_2$\Hyph words representing set $B\subset J(f,X)$}%
   {subset of words of representation}%
\Symb%W/0
   {superposition of coordinates of the representation $f$ and the element $m$}%
   {superposition of coordinates, representation}%
\Symb%W/0
   {superposition of coordinates of the tower of representations $\Vector f$ and the element $\VX a$}%
   {superposition of coordinates, tower of representations}%
\Symb%W/0
   {$\Omega_2$\Hyph word representing element $m\in J(f,X)$}%
   {word of element relative to generating set, representation}%
\Symb%W/0
   {set of $\Omega_2$\Hyph words of representation $J(f,X)$}%
   {word set of representation}%
\Symb%W/0
   {set of tuples of $\VX{\Omega}$\Hyph words of tower of representations $\Vector J(\Vector f,\VX X)$}%
   {word set of tower of representations}%
\Symb%W/0
   {tuple of words of element $\Vector a*$ relative to tuple of sets $\VX X$}%
   {words of element, tower of representations}%

\SetIndexSpace%X%0
\Symb%X/0
   {conjugate of quaternion $x$}%
   {conjugate of quaternion}%
\Symb%X/0
   {local basis of affine space}%
   {local basis of affine space}%
\Symb%X/0
   {anholonomic coordinate}%
   {x(k)}%

\SetIndexSpace%Z%0
\Symb%Z/0
   {center of $D$\Hyph algebra $A$}%
   {center of algebra}%
\Symb%Z/0
   {center of ring $D$}%
   {center of ring}%

\SetIndexSpace%Delta%1
\Symb%Delta/1
   {deviation of trajectories}%
   {deviation of trajectories}%
\Symb%Delta/1
   {identical transformation}%
   {identical transformation}%
\Symb%Delta/1
   {image of vector $\Vector e_k\in\Basis e$ under isomorphism to coordinate vector space}%
   {image of vector e_k, coordinate vector space}%
\Symb%Delta/1
   {Kronecker symbol}%
   {Kronecker symbol}%

\SetIndexSpace%Gamma%1
\Symb%Gamma/1
   {anholonomic coordinates of connection}%
   {anholonomic coordinates of connection}%
\Symb%Gamma/1
   {Cartan symbol}%
   {Cartan symbol}%
\Symb%Gamma/1
   {connection}%
   {conection overline}%
\Symb%Gamma/1
   {connection coefficients in $D$\Hyph affine space}%
   {connection coefficients, D affine space}%
\Symb%Gamma/1
   {connection in $D$\Hyph affine manifold}%
   {connection, affine manifold}%
\Symb%Gamma/1
   {$D$\Hyph affine connection coefficients on manifold}%
   {D affine connection coefficients, manifold}%
\Symb%Gamma/1
   {holonomic coordinates of connection}%
   {holonomic coordinates of connection}%
\Symb%Gamma/1
   {Cartan connection}%
   {overbrace Gamma i kl}%
\Symb%Gamma/1
   {set of sections of bundle}%
   {set of sections of bundle}%

\SetIndexSpace%Lambda%1
\Symb%Lambda/1
   {inverse operator to operator $\psi_l$}%
   {inverse operator to operator psi l}%
\Symb%Lambda/1
   {inverse operator to operator $\psi_r$}%
   {inverse operator to operator psi r}%

\SetIndexSpace%O%1
\Symb%O/1
   {norm of operation}%
   {norm of operation}%

\SetIndexSpace%Omega%1
\Symb%Omega/1
   {anholonomity object}%
   {anholonomity object}%

\SetIndexSpace%Psi%1
\Symb%Psi/1
   {left basic operator of Lie group over algebra $A$}%
   {L basic operator of Lie group over algebra A}%
\Symb%Psi/1
   {left basic operator of group Lie}%
   {Lie Basic Operator L}%
\Symb%Psi/1
   {left basic operator of Lie 1-parameter group}%
   {Lie Basic Operator L, 1-Parameter Group}%
\Symb%Psi/1
   {left basic operator of Lie 1-parameter group over algebra $A$}%
   {Lie Basic Operator L, 1-Parameter Group, algebra}%
\Symb%Psi/1
   {right basic operator of group Lie}%
   {Lie Basic Operator R}%
\Symb%Psi/1
   {right basic operator of Lie 1-parameter group}%
   {Lie Basic Operator R, 1-Parameter Group}%
\Symb%Psi/1
   {right basic operator of Lie 1-parameter group over algebra $A$}%
   {Lie Basic Operator R, 1-Parameter Group, algebra}%
\Symb%Psi/1
   {right basic operator of Lie group over algebra $A$}%
   {R basic operator of Lie group over algebra A}%

\SetIndexSpace%Fi%2
\Symb%Fi/2
   {Lie group composition law}%
   {Lie group composition law}%

\SetIndexSpace%Nabla%2
\Symb%Nabla/2
   {Cartan derivative}%
   {overbrace nabla_l}%
\Symb%Nabla/2
   {derivative}%
   {overline nabla_l, definition 1}%

\SetIndexSpace%Phi%2
\Symb%Phi/2
   {restriction of correspondence $\Phi$ to set $C$}%
   {restriction of correspondence}%

\SetIndexSpace%Pi%2
\Symb%Pi/2
   {Cartesian product of bundles}%
   {Cartesian product of bundles, definition 2}%
\Symb%Pi/2
   {Cartesian product of total spaces}%
   {Cartesian product of total spaces, definition 2}%
\Symb%Pi/2
   {direct product of division rings $D_i$, $i\in I$}%
   {direct product of division rings}%
\Symb%Pi/2
   {direct product of division rings $D_1$, ..., $D_n$}%
   {direct product of division rings, i 1 n}%
\Symb%Pi/2
   {direct product of $\RCstar D_i$\hyph vector spaces $\Vector V_i$, $i\in I$}%
   {direct product, rcd vector space}%
\Symb%Pi/2
   {direct product of $\RCstar D_i$\hyph vector spaces}%
   {direct product, rcd vector space, i 1 n}%
\Symb%Pi/2
   {product of groups $G_i$, $i\in I$}%
   {product of groups}%
\Symb%Pi/2
   {product of groups $G_1$, ..., $G_n$}%
   {product of groups, i 1 n}%
\Symb%Pi/2
   {product of objects $\{B_i,i\in I\}$ in category $\mathcal A$}%
   {product of objects in category}%
\Symb%Pi/2
   {product of objects $B_1$, ..., $B_n$ in category $\mathcal A$}%
   {product of objects in category, i 1 n}%
\Symb%Pi/2
   {reduced Cartesian product of bundles}%
   {reduced Cartesian product of bundles, definition 2}%
\Symb%Pi/2
   {reduced Cartesian product of total spaces}%
   {reduced Cartesian product of total spaces, definition 2}%

\SetIndexSpace%S%2
\Symb%S/2
   {fibered subset}%
   {fibered subset}%
\Symb%S/2
   {subbundle}%
   {subbundle}%

\CloseIndex


==> Symbol.Russian.tex <==
%auto-ignore
\def\indexname{Специальные символы и обозначения}
\OpenIndex

\SetIndexSpace%A%0
\Symb%
   {минорная матрица}%
   {A from b a}%
\Symb%
   {минорная матрица}%
   {A from columns T}%
\Symb%
   {минорная матрица}%
   {A from rows S}%
\Symb%
   {множество векторов, разложение которых относительно базиса $\Basis e$ сходится нормально}%
   {A plus Schauder}%
\Symb%
   {минорная матрица}%
   {A without column a}%
\Symb%
   {минорная матрица}%
   {A without columns T}%
\Symb%
   {минорная матрица}%
   {A without row b}%
\Symb%
   {минорная матрица}%
   {A without rows S}%
\Symb%
   {$A\CRcirc$\Hyph линейная комбинация}%
   {ACRcirc linear combination 1}%
\Symb%
   {$A\CRcirc$\Hyph линейная комбинация}%
   {ACRcirc linear combination 2}%
\Symb%
   {активное представление группы $G(f)$ в многообразии базисов $\mathcal B(f)$}%
   {active representation in basis manifold}%
\Symb%
   {активное представление группы $G(\Vector  f)$ в многообразии базисов $\mathcal B(\Vector f)$}%
   {active representation in basis manifold, tower of representations}%
\Symb%
   {аффинное пространство}%
   {affine space, division ring}%
\Symb%
   {$A$\Hyph алгебра многочленов над $D$\Hyph алгеброй $A$}%
   {algebra of polynomials over algebra}%
\Symb%
   {алгебра многочленов над $D$\Hyph алгеброй $A$}%
   {algebra of polynomials over D algebra}%
\Symb%
   {алгебра рациональных отображений алгебры $A$}%
   {algebra of rational mappings of algebra}%
\Symb%
   {аффинное пространство}%
   {An}%
\Symb%
   {ассоциатор $D$\Hyph алгебры}%
   {associator of algebra}%
\Symb%
   {\subs строка ($c$\hyph строка) матрицы}%
   {c row}%
\Symb%
   {коммутатор $D$\Hyph алгебры}%
   {commutator of algebra}%
\Symb%
   {компонента линейного отображения}%
   {component of linear map, vector}%
\Symb%
   {компонента $p$ полилинейного отображения $\Vector A$}%
   {component of polyadditive map, D vector space}%
\Symb%
   {компонента полилинейного отображения}%
   {component of polylinear map, vector}%
\Symb%
   {сопряжённый $D$\Hyph  модуль}%
   {conjugated D module}%
\Symb%
   {линейная комбинация векторов $A$\Hyph модуля}%
   {CR linear combination in A module}%
\Symb%
   {\CR степень элемента $A$ бикольца}%
   {cr power}%
\Symb%
   {\CR обратный элемент бикольца}%
   {cr-inverse element}%
\Symb%
   {\CR произведение матриц}%
   {cr-product of matrices}%
\Symb%
   {производная левого сдвига}%
   {derivative of left shift}%
\Symb%
   {производная левого сдвига в $1$\Hyph параметрической группе Ли}%
   {derivative of left shift, 1-Parameter Group}%
\Symb%
   {производная левого сдвига в $1$\Hyph параметрической D группе Ли}%
   {derivative of left shift, 1-Parameter Group, algebra}%
\Symb%
   {производная правого сдвига}%
   {derivative of right shift}%
\Symb%
   {производная правого сдвига}%
   {derivative of right shift}%
\Symb%
   {производная правого сдвига в $1$\Hyph параметрической группе Ли}%
   {derivative of right shift, 1-Parameter Group}%
\Symb%
   {производная правого сдвига в $1$\Hyph параметрической D группе Ли}%
   {derivative of right shift, 1-Parameter Group, algebra}%
\Symb%
   {производная левого сдвига}%
   {derivative of Tstar shift}%
\Symb%
   {\drc вектор}%
   {drc vector}%
\Symb%
   {координаты вектора $a$ относительно базиса Гамеля}%
   {Hamel basis, coordinates}%
\Symb%
   {эрмитово сопряжение в теле}%
   {hermitian conjugation, division ring}%
\Symb%
   {тензор, обратный тензору $a$}%
   {inverse tensor}%
\Symb%
   {$(^j_i)$\hyph\CR квазидетерминант}%
   {j i CR quasideterminant definition}%
\Symb%
   {$(ji)$\hyph квазидетерминант матрицы $\bfA$}%
   {j i quasideterminant definition}%
\Symb%
   {$(^j_i)$\hyph \RC квазидетерминант}%
   {j i RC-quasideterminant definition}%
\Symb%
   {$(^j_i)$\hyph $\RCcirc$\Hyph квазидетерминант}%
   {j i RCcirc-quasideterminant definition}%
\Symb%
   {левая дробь}%
   {left fraction}%
\Symb%
   {левый главный идеал}%
   {left principal ideal}%
\Symb%
   {левый сдвиг в $D$\Hyph алгебре}%
   {left shift, D algebra}%
\Symb%
   {линейная комбинация векторов $A$\Hyph модуля}%
   {linear combination in A module}%
\Symb%
   {преобразование матрицы}%
   {matrix, replacing its column}%
\Symb%
   {преобразование матрицы}%
   {matrix, replacing its row}%
\Symb%
   {$A$\Hyph модуль однородных многочленов над $D$\Hyph алгеброй $A$}%
   {module of homogeneous polynomials over algebra}%
\Symb%
   {норма в $D$\Hyph модуле}%
   {norm on D module}%
\Symb%
   {алгебра, противоположная алгебре $A$}%
   {opposite algebra}%
\Symb%
   {орбита линейного отображения}%
   {orbit of linear mapping}%
\Symb%
   {производная}%
   {overline nabla_l, definition 2}%
\Symb%
   {частное линейное отображение}%
   {partial linear map}%
\Symb%
   {главный идеал}%
   {principal ideal}%
\Symb%
   {квазидетерминант матрицы $\bfA$}%
   {quasideterminant definition}%
\Symb%
   {\sups строка ($r$\hyph строка) матрицы}%
   {r row}%
\Symb%
   {\RC степень элемента $A$ бикольца}%
   {rc power}%
\Symb%
   {\RC обратный элемент бикольца}%
   {rc-inverse element}%
\Symb%
   {\RC произведение матриц}%
   {rc-product of matrices}%
\Symb%
   {\RC квазидетерминант}%
   {RC-quasideterminant definition}%
\Symb%
   {$\RCcirc$\Hyph квазидетерминант}%
   {RCcirc-quasideterminant definition}%
\Symb%
   {\rcd вектор}%
   {rcd vector}%
\Symb%
   {правый главный идеал}%
   {right principal ideal}%
\Symb%
   {правый сдвиг в $D$\Hyph алгебре}%
   {right shift, D algebra}%
\Symb%
   {координаты вектора $a$ относительно базиса Шаудера}%
   {Schauder basis, coordinates}%
\Symb%
   {множество обратимых элементов алгебры $A$}%
   {set of invertible elements of algebra}%
\Symb%
   {множество нулей алгебры $A$}%
   {set of zeros of algebra}%
\Symb%
   {множество полилинейных отображений колец $R_1$, ..., $R_n$ в модуль $S$}%
   {set polylinear maps, ring}%
\Symb%
   {косое произведение векторов $\Vector a_1$, ..., $\Vector a_m$}%
   {skew product of vectors}%
\Symb%
   {правый сдвиг}%
   {starT shift}%
\Symb%
   {\sT сдвиг}%
   {starT shift, fibered group}%
\Symb%
   {тензорная степень алгебры $A$}%
   {tensor power of algebra}%
\Symb%
   {тензорное произведение алгебр}%
   {tensor product of algebras}%
\Symb%
   {левый сдвиг}%
   {Tstar shift}%
\Symb%
   {\Ts сдвиг}%
   {Tstar shift, fibered group}%
\Symb%
   {неголономные координаты вектора}%
   {vector anholonomic coordinates}%
\Symb%
   {голономные координаты вектора}%
   {vector holonomic coordinates}%

\SetIndexSpace%B%0
\Symb%
   {многообразие базисов \rcd векторного пространства $\Vector V$}%
   {basis manifold of rcd vector space}%
\Symb%
   {многообразие базисов векторного пространства}%
   {basis manifold of vector space}%
\Symb%
   {многообразие базисов представления $f$}%
   {basis manifold representation F algebra}%
\Symb%
   {многообразие базисов башни представлений $\Vector f$}%
   {basis manifold tower of representations}%
\Symb%
   {многообразие базисов аффинного пространства}%
   {Basis Manifold, Affine Space}%
\Symb%
   {многообразие базисов \rcd аффинного пространства}%
   {Basis Manifold, rcd Affine Space, division ring}%
\Symb%
   {многообразие базисов центро-аффинного пространства}%
   {BCAn}%
\Symb%
   {многообразие базисов евклидова пространства}%
   {BEn}%
\Symb%
   {алгебра Бореля}%
   {Borel algebra}%
\Symb%
   {декартова степень $\Bundle A$ расслоения $\Bundle B$}%
   {Cartesian power A of bundle B}%
\Symb%
   {декартова степень $A$ множества $B$}%
   {Cartesian power of set}%
\Symb%
   {замкнутый шар}%
   {closed ball}%
\Symb%
   {многообразие базисов центро-аффинного пространства}%
   {FCAn}%
\Symb%
   {многообразие базисов евклидова пространства}%
   {FEn}%
\Symb%
   {структура всех подпредставлений представления $f$}%
   {lattice of subrepresentations}%
\Symb%
   {структура башен подпредставлений башни представлений $\Vector f$}%
   {lattice of subrepresentations, tower of representations}%
\Symb%
   {открытый шар}%
   {open ball}%
\Symb%
   {произведением объектов $B_1$, ..., $B_n$ в категории $\mathcal A$}%
   {product of objects in category, 1 n}%
\Symb%
   {правая дробь}%
   {right fraction}%
\Symb%
   {тензорная степень представления}%
   {tensor power of representation}%
\Symb%
   {тензорное произведение представлений}%
   {tensor product of representations}%

\SetIndexSpace%C%0
\Symb%
   {$\sigma$\Hyph алгебра измеримых относительно меры $\mu$ множеств}%
   {algebra of sets measurable with respect to measure}%
\Symb%
   {центро-аффинное пространство}%
   {CAn}%
\Symb%
   {центро-аффинное пространство}%
   {central affine space}%
\Symb%
   {столбцовый определитель по $j$-му столбцу  матрицы $\bfA$}%
   {column determinant}%
\Symb%
   {$\CRcirc$\Hyph произведение матриц отображений}%
   {cr product of matrices of mappings}%
\Symb%
   {левые структурные константы алгебры Ли}%
   {left structural constant of Lie algebra}%
\Symb%
   {правые структурные константы алгебры Ли}%
   {right structural constant of Lie algebra}%
\Symb%
   {множество непрерывных отображений нескольких переменных}%
   {set continuous multivariable maps}%
\Symb%
   {структурные константы}%
   {structural constants}%

\SetIndexSpace%D%0
\Symb%
   {базовый вектор представления группы Ли}%
   {basis vector of representation of Lie group}%
\Symb%
   {базовый вектор представления группы Ли над алгеброй $A$}%
   {basis vector of representation of Lie group over algebra A}%
\Symb%
   {координаты базового вектора представления группы Ли над алгеброй $A$}%
   {basis vector of representation of Lie group over algebra A, coordinates}%
\Symb%
   {координаты базового вектора представления группы Ли}%
   {basis vector of representation of Lie group, coordinates}%
\Symb%
   {компонента производной Гато отображения $f(x)$}%
   {component of Gateaux derivative}%
\Symb%
   {компонента производной Гато отображения $f(x)$}%
   {component of Gateaux derivative of map, D vector space, short}%
\Symb%
   {компонента производной Гато второго порядка отображения $f(x)$}%
   {component of Gateaux derivative of Second Order}%
\Symb%
   {компонента производной Гато второго порядка отображения $f(x)$}%
   {component of Gateaux derivative of Second Order, D vector space}%
\Symb%
   {компонента производной Гато отображения $f(x)$}%
   {component of Gateaux derivative, vector space}%
\Symb%
   {сопряжение в алгебре}%
   {conjugation in algebra}%
\Symb%
   {сопряжение в кольце}%
   {conjugation in ring}%
\Symb%
   {координатное \Drc векторное расслоение}%
   {coordinate drc vector bundle}%
\Symb%
   {координатное \rcd векторное пространство}%
   {coordinate rcd vector space}%
\Symb%
   {координатная система отсчёта}%
   {coordinate reference frame, extensive definition}%
\Symb%
   {диагональ в расслоении $\Bundle A$}%
   {diagonal in bundle, 1}%
\Symb%
   {прямое произведение тел $D_1$, ..., $D_n$}%
   {direct product of division rings, 1 n}%
\Symb%
   {двойной определитель матрицы $\bfA$}%
   {double determinant}%
\Symb%
   {\Ds производная Фреше функции $f$ тела}%
   {Frechet Dstar derivative of map, division ring}%
\Symb%
   {\dcr производная Гато отображения $\Vector f$ $D$\Hyph векторного пространства $V$ в $D$\Hyph векторное пространство $W$}%
   {Gateaux dcr derivative of map, D vector space}%
\Symb%
   {производная Гато отображения $f$}%
   {Gateaux derivative of map}%
\Symb%
   {производная Гато отображения $f$}%
   {Gateaux derivative of map, fraction}%
\Symb%
   {производная Гато порядка $n$}%
   {Gateaux derivative of Order n}%
\Symb%
   {производная Гато порядка $n$ отображения $f$ тела}%
   {Gateaux derivative of Order n, division ring}%
\Symb%
   {производная Гато порядка $n$ отображения $f$ алгебры}%
   {Gateaux derivative of Order n, fraction, algebra}%
\Symb%
   {производная Гато порядка $n$ отображения $f$ тела}%
   {Gateaux derivative of Order n, fraction, division ring}%
\Symb%
   {производная Гато второго порядка}%
   {Gateaux derivative of Second Order}%
\Symb%
   {производная Гато второго порядка отображения $f$ алгебры}%
   {Gateaux derivative of Second Order, fraction, algebra}%
\Symb%
   {производная Гато второго порядка отображения $f$ тела}%
   {Gateaux derivative of Second Order, fraction, division ring}%
\Symb%
   {дифференциал Гато отображения $f$}%
   {Gateaux differential of map, scalar}%
\Symb%
   {дифференциал Гато отображения $f$}%
   {Gateaux differential of map, vector}%
\Symb%
   {\Ds производная Гато функции $f$ тела $D$}%
   {Gateaux Dstar derivative of map, division ring}%
\Symb%
   {якобиан Гато отображения $D$\Hyph векторного пространства}%
   {Gateaux Jacobian of map, D vector space}%
\Symb%
   {частная \dcr производная Гато отображения $f^{\gi b}$ по переменной $x^{\gi a}$}%
   {Gateaux partial dcr derivative of map, 1, D vector space}%
\Symb%
   {частная \dcr производная Гато отображения $f^{\gi b}$ по переменной $x^{\gi a}$}%
   {Gateaux partial dcr derivative of map, 2, D vector space}%
\Symb%
   {частная \dcr производная Гато отображения $f^{\gi b}$ по переменной $x^{\gi a}$}%
   {Gateaux partial dcr derivative of map, 3, D vector space}%
\Symb%
   {частная производная Гато}%
   {Gateaux partial derivative}%
\Symb%
   {смешанная частная производная Гато}%
   {Gateaux partial derivative of Second Order}%
\Symb%
   {частная \rcd производная Гато отображения $f^{\gi b}$ по переменной $x^{\gi a}$}%
   {Gateaux partial rcd derivative of map, 1, D vector space}%
\Symb%
   {частная \rcd производная Гато отображения $f^{\gi b}$ по переменной $x^{\gi a}$}%
   {Gateaux partial rcd derivative of map, 2, D vector space}%
\Symb%
   {частная \rcd производная Гато отображения $f^{\gi b}$ по переменной $x^{\gi a}$}%
   {Gateaux partial rcd derivative of map, 3, D vector space}%
\Symb%
   {\rcd производная Гато отображения $f$ $D$\hyph векторного пространства $V$ в $D$\hyph векторное пространство $W$}%
   {Gateaux rcd derivative of map, D vector space}%
\Symb%
   {\sD производная Гато функции $f$ тела $D$}%
   {Gateaux starD derivative of map, division ring}%
\Symb%
   {векторное пространство матриц}%
   {matrices vector space}%
\Symb%
   {производная Картана}%
   {overbrace D}%
\Symb%
   {производная}%
   {overline D}%
\Symb%
   {производная вдоль векторного поля $e_{(k)}$}%
   {partial(k)}%
\Symb%
   {произведение отображения на скаляр}%
   {product of map over scalar}%
\Symb%
   {\drc векторное пространство \subs строк}%
   {r rows drc vector space}%
\Symb%
   {скорость отклонения}%
   {speed of deviation}%
\Symb%
   {стандартная компонента производной Гато}%
   {standard component of Gateaux derivative}%
\Symb%
   {тензорное произведение тел}%
   {tensor product of division rings}%
\Symb%
   {тензорное произведение колец}%
   {tensor product of rings}%
\Symb%
   {тип векторного пространства}%
   {vector space type}%

\SetIndexSpace%E%0
\Symb%
   {$A\CRcirc$\Hyph базис модуля}%
   {A CRcirc basis, module over algebra}%
\Symb%
   {матрица Якоби левого сдвига}%
   {aE, quaternion, Jacobian matrix}%
\Symb%
   {аффинный базис}%
   {Affine Basis}%
\Symb%
   {базис векторного пространства}%
   {Basis e}%
\Symb%
   {базис в векторном пространстве $\Vector V$}%
   {basis in V}%
\Symb%
   {базис $D$\Hyph модуля $\mathcal L(D;A_1;A_2)$}%
   {basis L(A1,A2)}%
\Symb%
   {базис в векторном пространстве}%
   {basis, vector space}%
\Symb%
   {базис $(n)$\hyph векторного пространства}%
   {basis,n vector space}%
\Symb%
   {декартова степень расслоенного пространства}%
   {Cartesian power of total spaces}%
\Symb%
   {декартово произведение расслоенных пространств}%
   {Cartesian product of total spaces, definition 1}%
\Symb%
   {центро-аффинный базис}%
   {Central Affine Basis}%
\Symb%
   {базис в \Drc векторного расслоения}%
   {drc basis, vector bundle}%
\Symb%
   {форма системы отсчёта}%
   {dual forms, reference frame}%
\Symb%
   {евклидово пространство}%
   {Euclid space}%
\Symb%
   {евклидово пространство}%
   {Euclid space, division ring}%
\Symb%
   {базис Гамеля}%
   {Hamel basis}%
\Symb%
   {тождественное преобразование расслоения}%
   {identical transformation of bundle}%
\Symb%
   {линейный автоморфизм алгебры кватернионов}%
   {mapping E, quaternion}%
\Symb%
   {линейный автоморфизм алгебры кватернионов}%
   {mapping E_1, quaternion}%
\Symb%
   {линейный автоморфизм алгебры кватернионов}%
   {mapping E_2, quaternion}%
\Symb%
   {ортонормированный базис}%
   {Orthonornal Basis}%
\Symb%
   {псевдоевклидово пространство}%
   {pseudo Euclid space}%
\Symb%
   {псевдоевклидово пространство}%
   {pseudo Euclid space, division ring}%
\Symb%
   {алгебра кватернионов над полем $F$}%
   {quaternion algebra over the field}%
\Symb%
   {алгебра кватернионов с делением над полем $F$}%
   {quaternion division algebra over the fieldL}%
\Symb%
   {$\RCcirc A$\Hyph линейная комбинация}%
   {RCcircA linear combination 1}%
\Symb%
   {$\RCcirc A$\Hyph линейная комбинация}%
   {RCcircA linear combination 2}%
\Symb%
   {\rcd аффинный базис}%
   {rcd affine basis, division ring}%
\Symb%
   {приведенное декартово произведение расслоенных пространств}%
   {reduced Cartesian product of total spaces, definition 1}%
\Symb%
   {базис Шаудера}%
   {Schauder basis}%
\Symb%
   {множество невырожденных \sT преобразований расслоения $\Bundle E$}%
   {set of starT nonsingular transformations of bundle}%
\Symb%
   {множество невырожденных \Ts преобразований расслоения $\Bundle E$}%
   {set of Tstar nonsingular transformations of bundle}%
\Symb%
   {стандартные координаты базиса}%
   {standard coordinates of basis}%
\Symb%
   {стандартные координаты системы отсчёта}%
   {standard coordinates of reference frame}%
\Symb%
   {векторное поле системы отсчёта}%
   {vector field of reference frame}%
\Symb%
   {вектор базиса}%
   {vector of basis}%

\SetIndexSpace%F%0
\Symb%
   {координаты базиса в \rcd векторном пространстве \sups строк}%
   {basis coordinates, c rows rcd vector space}%
\Symb%
   {координаты базиса в \drc векторном пространстве \subs строк}%
   {basis coordinates, r rows drc vector space}%
\Symb%
   {базис в \rcd векторного пространства \sups строк}%
   {basis, c rows rcd vector space}%
\Symb%
   {базис в \drc векторном пространстве \subs строк}%
   {basis, r rows drc vector space}%
\Symb%
   {центро-аффинный}%
   {Central Affine Basis, division ring}%
\Symb%
   {компонента линейного отображения $f$ тела}%
   {component of linear map, division ring}%
\Symb%
   {компонента полилинейного отображения}%
   {component of polylinear map}%
\Symb%
   {расслоенный морфизм из расслоения $\Bundle A$ в $\Bundle B$}%
   {fibered morphism from A into B}%
\Symb%
   {фильтр $\mathfrak{F}$ сходится к множеству $A$}%
   {filter converges}%
\Symb%
   {гомоморфизм расслоенных универсальных алгебр}%
   {homomorphism of fibered universal algebras}%
\Symb%
   {обратное расслоенное соответствие}%
   {inverse fibered correspondence, 1}%
\Symb%
   {обратное приведенное расслоенное соответствие}%
   {inverse reduced fibered correspondence, 1}%
\Symb%
   {отображение в декартово произведение}%
   {map to Cartesian product}%
\Symb%
   {норма функционала}%
   {norm of functional}%
\Symb%
   {норма отображения}%
   {norm of map}%
\Symb%
   {норма полилинейного отображения}%
   {norm of polymap}%
\Symb%
   {норма представления}%
   {norm of representation}%
\Symb%
   {орбита представления группы $G$}%
   {orbit of Tstar representation of group}%
\Symb%
   {ортонормированный базис}%
   {Orthonornal Basis, division ring}%
\Symb%
   {кватернионная алгебра над полем ${\rm {\mathbb{F}}}$}%
   {quaternion algebra F a b}%
\Symb%
   {система отсчёта}%
   {reference frame}%
\Symb%
   {система отсчёта, расширенное определение}%
   {reference frame, extensive definition}%
\Symb%
   {стандартная компонента биаддитивного отображения $f$ над полем $F$}%
   {standard component of biadditive map, division ring}%
\Symb%
   {стандартная компонента линейного отображения }%
   {standard component of linear map, G}%
\Symb%
   {стандартная компонента полилинейного отображения}%
   {standard component of polylinear map}%
\Symb%
   {стандартная компонента квадратичного отображения $f$ над полем $F$}%
   {standard component of quadratic map, division ring}%
\Symb%
   {стандартная компонента тензора}%
   {standard component of tensor}%
\Symb%
   {сумма линейных отображений}%
   {sum of linear maps}%

\SetIndexSpace%G%0
\Symb%
   {группа аффинных преобразований}%
   {affine transformation group}%
\Symb%
   {\CR матричная группа}%
   {cr-matrix group}%
\Symb%
   {группа аффинных преобразований}%
   {drc affine transformation group}%
\Symb%
   {расслоенная малая группа сечения $h$}%
   {fibered little group}%
\Symb%
   {расслоенная группа стабилизации сечения $h$}%
   {fibered stability group}%
\Symb%
   {алгебра Ли группы Ли}%
   {g}%
\Symb%
   {определённая слева алгебра Ли группы Ли}%
   {gl}%
\Symb%
   {определённая справа алгебра Ли группы Ли}%
   {gr}%
\Symb%
   {группа автоморфизмов представления $f$}%
   {group of automorphisms of representation}%
\Symb%
   {группа гомоморфизмов векторного пространства $\Vector V$}%
   {GV}%
\Symb%
   {малая группа элемента $x$}%
   {little group}%
\Symb%
   {орбита ковариантного эффективного \sT представления расслоенной группы}%
   {orbit of effective covariant starT representation of fibered group}%
\Symb%
   {орбита ковариантного эффективного \sT представления группы}%
   {orbit of effective covariant starT representation of group}%
\Symb%
   {орбита ковариантного эффективного		\Ts представления расслоенной группы}%
   {orbit of effective covariant Tstar representation of fibered group}%
\Symb%
   {орбита ковариантного эффективного		\Ts представления группы}%
   {orbit of effective covariant Tstar representation of group}%
\Symb%
   {произведение групп $G_1$, ..., $G_n$}%
   {product of groups, 1 n}%
\Symb%
   {\RC матричная группа}%
   {rc-matrix group}%
\Symb%
   {группа стабилизации элемента $x$}%
   {stability group}%

\SetIndexSpace%H%0
\Symb%
   {обращение Адамара матрицы}%
   {Hadamard inverse of matrix}%
\Symb%
   {кватернионная алгебра}%
   {quaternion algebra H a b}%
\Symb%
   {алгебра кватернионов над полем действительных чисел}%
   {quaternion algebra over real field}%

\SetIndexSpace%I%0
\Symb%
   {инфинитезимальные образующие представления}%
   {infinitesimal generator I of representation}%
\Symb%
   {инфинитезимальные образующие представления}%
   {infinitesimal generator i of representation}%
\Symb%
   {инфинитезимальные образующие группы Ли}%
   {Lie group infinitesimal generators}%
\Symb%
   {модуль векторов алгебры $A$}%
   {vector module of algebra}%
\Symb%
   {модуль векторов кольца $D$}%
   {vector module of ring}%
\Symb%
   {вектор элемента $d$ алгебры}%
   {vector of algebra}%
\Symb%
   {вектор отображения $f$}%
   {vector of mapping}%
\Symb%
   {вектор элемента $d$ кольца}%
   {vector of ring}%

\SetIndexSpace%J%0
\Symb%
   {оператор замыкания представления $f$}%
   {closure operator, representation}%
\Symb%
   {оператор замыкания башни представлений $\Vector f$}%
   {closure operator, tower of representations}%
\Symb%
   {матрица Якоби правого сдвига}%
   {Ea, quaternion, Jacobian matrix}%
\Symb%
   {башня подпредставлений башни представлений $\Vector f$, порождённая кортежем множеств $\VX X$}%
   {subrepresentation generated by tuple of sets}%

\SetIndexSpace%K%0
\Symb%
   {ядро линейного отображения}%
   {kernel of linear map}%

\SetIndexSpace%L%0
\Symb%
   {левое алгебраическое дополнение элемента  $a_{i{\kern 1pt} j} $ матрицы}%
   {left cofactor, matrix}%
\Symb%
   {левое двойное алгебраическое дополнение элемента $a_{ij}$ матрицы}%
   {left double cofactor}%
\Symb%
   {левый сдвиг}%
   {left shift}%
\Symb%
   {производная Ли связности}%
   {Lie derivative of connection}%
\Symb%
   {производная Ли метрики}%
   {Lie derivative of metric}%
\Symb%
   {предел соответствия $\Phi$ по фильтру $\mathfrak{F}$}%
   {limit of correspondence with respect to the filter}%
\Symb%
   {предел последовательности}%
   {limit of sequence}%
\Symb%
   {пассивное преобразование}%
   {passive transformation}%
\Symb%
   {множество \Acr линейных отображений модуля $\Vector V$ в модуль $\Vector W$}%
   {set Acr linear maps, module}%
\Symb%
   {$D$\Hyph модуль непрерывных линейных отображений нормированного $D$\Hyph модуля $A_1$ в нормированный $D$\Hyph модуль $A_2$}%
   {set continuous linear mappings, module}%
\Symb%
   {множество непрерывных линейных отображений}%
   {set continuous linear maps, vector}%
\Symb%
   {множество непрерывных полилинейных отображений}%
   {set continuous polylinear maps}%
\Symb%
   {\rcd векторное пространство линейных отображений \drc векторного пространства $ V$ в \drc векторное пространство $W$}%
   {set linear maps, drc vector space}%
\Symb%
   {\drc векторное пространство линейных отображений \rcd векторного пространства $V$ в \rcd векторное пространство $W$}%
   {set linear maps, rcd vector space}%
\Symb%
   {множество линейных отображений}%
   {set linear maps, scalar}%
\Symb%
   {множество линейных отображений}%
   {set linear maps, vector}%
\Symb%
   {множество левосторонних невырожденных преобразований множества $M$}%
   {set of left-side nonsingular transformations}%
\Symb%
   {множество полилинейных отображений}%
   {set polylinear maps}%
\Symb%
   {множество $n$\hyph линейных отображений}%
   {set polylinear maps An}%
\Symb%
   {множество полилинейных отображений}%
   {set polylinear maps, D vector space}%
\Symb%
   {множество полилинейных отображений алгебр $A_1$, ..., $A_n$ в алгебру $A$}%
   {set polylinear maps, finite dimensional algebra}%
\Symb%
   {множество \sT представлений тела $S$ в аддитивной группе тела $R$}%
   {set sT representations, division ring}%
\Symb%
   {множество \Ts представлений тела $S$ в аддитивной группе тела $R$}%
   {set Ts representations, division ring}%

\SetIndexSpace%M%0
\Symb%
   {множество отображений в $\Omega$\Hyph группу $A$}%
   {set of maps to Omega group}%
\Symb%
   {множество \sT преобразований множества $M$}%
   {set of starT transformations}%
\Symb%
   {множество преобразований множества $M$}%
   {set of transformations}%
\Symb%
   {множество \Ts преобразований универсальной алгебры $M$}%
   {set of Tstar transformations}%
\Symb%
   {пространство орбит \sT ковариантного эффективного представления группы}%
   {space of orbits of effective sT representation}%
\Symb%
   {пространство орбит \Ts ковариантного эффективного представления группы}%
   {space of orbits of effective Ts representation}%
\Symb%
   {пространство орбит \Ts представления группы $G$ в множестве $M$}%
   {space of orbits of Ts representation}%

\SetIndexSpace%N%0
\Symb%
   {норма кватерниона $x$}%
   {norm, quaternion algebra}%
\Symb%
   {ядро $D$\Hyph алгебры $A$}%
   {nucleus of algebra}%

\SetIndexSpace%O%0
\Symb%
   {геометрический объект в координатном представлении, определённом в \rcd векторном пространстве}%
   {geometric object, coordinate rcd vector space}%
\Symb%
   {геометрический объект в координатном представлении}%
   {geometric object, coordinate vector space}%
\Symb%
   {геометрический объект, определённый в \rcd векторном пространстве}%
   {geometric object, rcd vector space}%
\Symb%
   {алгебра октонионов}%
   {octonion algebra}%
\Symb%
   {орбита представления расслоенной группы $\Bundle G$}%
   {orbit of representation of fibered group}%
\Symb%
   {орбита представления группы $G$}%
   {orbit of representation of group}%

\SetIndexSpace%P%0
\Symb%
   {расслоение}%
   {bundle}%
\Symb%
   {расслоение уровня $2$}%
   {bundle of level 2}%
\Symb%
   {расслоение уровня $n$}%
   {bundle of level n}%
\Symb%
   {декартова степень $n$ расслоения $\bundle{}{p}{E}{}$}%
   {Cartesian power of bundle}%
\Symb%
   {декартово произведение расслоений}%
   {Cartesian product of bundles, definition 1}%
\Symb%
   {пассивное представление группы $G(f)$ в многообразии базисов $\mathcal B(f)$}%
   {passive representation in basis manifold}%
\Symb%
   {пассивное представление группы $G(\Vector f)$ в многообразии базисов $\mathcal B(\Vector f)$}%
   {passive representation in basis manifold, tower of representations}%
\Symb%
   {приведенное декартово произведением расслоений}%
   {reduced Cartesian product of bundles, definition 1}%
\Symb%
   {множество невырожденных \sT преобразований расслоения $\bundle{}pE{}$}%
   {set of starT nonsingular transformations of bundle, projection}%
\Symb%
   {множество невырожденных \Ts преобразований расслоения $\bundle{}pE{}$}%
   {set of Tstar nonsingular transformations of bundle, projection}%

\SetIndexSpace%R%0
\Symb%
   {активное преобразование}%
   {active transformation}%
\Symb%
   {\rcd векторное пространство \sups строк}%
   {c rows rcd vector space}%
\Symb%
   {кривизна Картана}%
   {Cartan curvature}%
\Symb%
   {\CR ранг матрицы}%
   {cr-rank of matrix}%
\Symb%
   {диагональ в расслоении $\bundle{}pA{}$}%
   {diagonal in bundle, 2}%
\Symb%
   {диагональ в расслоении $\Bundle A$}%
   {diagonal in reduced bundle, 2}%
\Symb%
   {образ $m$ при эндоморфизме $R$ эффективного представления}%
   {endomorphism image, effective representation}%
\Symb%
   {образ кортежа $\VX a$ при эндоморфизме $\VX r$ башни эффективных представлений}%
   {endomorphism image, tower of effective representations}%
\Symb%
   {кривизна}%
   {GLn curvature_overline}%
\Symb%
   {$\RCcirc$\Hyph произведение матриц отображений}%
   {rc product of matrices of mappings}%
\Symb%
   {\RC ранг матрицы}%
   {rc-rank of matrix}%
\Symb%
   {правое алгебраическое дополнение элемента  $a_{i{\kern 1pt} j} $ матрицы}%
   {right cofactor, matrix}%
\Symb%
   {правое двойное алгебраическое дополнение элемента $a_{ij}$ матрицы}%
   {right double cofactor}%
\Symb%
   {правый сдвиг}%
   {right shift}%
\Symb%
   {строчный определитель по  $i$-й строке матрицы $\bfA$}%
   {row determinant}%
\Symb%
   {алгебра скаляров алгебры $A$}%
   {scalar algebra of algebra}%
\Symb%
   {алгебра скаляров кольца $D$}%
   {scalar algebra of ring}%
\Symb%
   {скаляр элемента $d$ алгебры}%
   {scalar of algebra}%
\Symb%
   {скаляр отображения $f$}%
   {scalar of mapping}%
\Symb%
   {скаляр элемента $d$ кольца}%
   {scalar of ring}%
\Symb%
   {множество правосторонних невырожденных преобразований множества $M$}%
   {set of right-side nonsingular transformations}%

\SetIndexSpace%S%0
\Symb%
   {произведение расслоенных соответствий}%
   {composition of fibered correspondences}%
\Symb%
   {обратное расслоенное соответствие}%
   {inverse fibered correspondence, 2}%
\Symb%
   {обратное приведенное расслоенное соответствие}%
   {inverse reduced fibered correspondence, 2}%
\Symb%
   {линейная оболочка в векторном пространстве}%
   {linear span, vector space}%
\Symb%
   {образ базиса $X$ при пассивном преобразовании $S$}%
   {passive transformation of basis, representation}%
\Symb%
   {образ базиса $\VX X$ при пассивном преобразовании $\VX s$}%
   {passive transformation of basis, tower of representations}%
\Symb%
   {симметрическая группа}%
   {symmetric group}%

\SetIndexSpace%T%0
\Symb%
   {категория \Ts представлений $\Omega_1$\Hyph алгебры $A$}%
   {category of Tstar representations of Omega1 algebra}%
\Symb%
   {категория \Ts представлений $\Omega_1$\Hyph алгебры из категории $\mathcal A$}%
   {category of Tstar representations of Omega1 algebra from category}%
\Symb%
   {касательная плоскость к группе $G$}%
   {TaG}%
\Symb%
   {след кватерниона $x$}%
   {trace, quaternion algebra}%

\SetIndexSpace%V%0
\Symb%
   {координатное векторное пространство}%
   {coordinate vector space}%
\Symb%
   {координаты в векторном пространстве}%
   {coordinates in vector space}%
\Symb%
   {прямое произведение $\RCstar D_i$\hyph векторных пространств $\Vector V_1$, ..., $\Vector V_n$}%
   {direct product, rcd vector space, 1 n}%
\Symb%
   {дуальное пространство к \rcd векторному пространству $\Vector V$}%
   {dual space of rcd vector space}%
\Symb%
   {эрмитово сопряжённый вектор}%
   {hermitian conjugated vector}%
\Symb%
   {тензорное произведение $D$\Hyph векторных пространств}%
   {tensor product of D vector spaces}%
\Symb%
   {тензорное произведение \Ds векторных пространств}%
   {tensor product of Dstar vector spaces}%
\Symb%
   {векторное пространство}%
   {V}%

\SetIndexSpace%W%0
\Symb%
   {множество координат представления $J(f,X)$}%
   {coordinate set of representation}%
\Symb%
   {множество кортежей координат башни представлений $\Vector J(\Vector f,\VX X)$}%
   {coordinate set of tower of representations}%
\Symb%
   {координаты базиса $X'$ относительно базиса $X$ представления}%
   {coordinates of basis relative to basis, representation}%
\Symb%
   {координаты элемента $m$ представления $f$ относительно множества $X$}%
   {coordinates of element relative to generating set, representation}%
\Symb%
   {координаты элемента $m$ относительно множества $X$}%
   {coordinates of element relative to set, representation}%
\Symb%
   {кортеж координат элемента $\Vector a$ относительно кортежа множеств $\VX X$}%
   {coordinates of element, tower of representations}%
\Symb%
   {геометрический объект в координатном представлении, определённом в $\Omega_2$\Hyph алгебре $M$}%
   {geometric object, coordinate representation g}%
\Symb%
   {геометрический объект в координатном представлении, определённом в кортеже $\VX\Omega$\Hyph алгебр $\VX A$}%
   {geometric object, coordinate tower of representations g}%
\Symb%
   {геометрический объект, определённый в $\Omega_2$\Hyph алгбре $M$}%
   {geometric object, representation g}%
\Symb%
   {геометрический объект, определённый в кортеже $\VX\Omega$\Hyph алгебр $\VX A$}%
   {geometric object, tower of representations g}%
\Symb%
   {геометрический объект в векторном пространстве}%
   {geometric object, vector space}%
\Symb%
   {множество координат множества $B\subset J(f,X)$}%
   {subset of coordinates of representation}%
\Symb%
   {координаты кортежа множеств $\VX B$ относительно кортежа множеств $\VX X$}%
   {subset of coordinates of tower of representations}%
\Symb%
   {координаты множества $B_k$ относительно кортежа множеств $\VX X$}%
   {subset of coordinates of tower of representations, k}%
\Symb%
   {множество $\Omega_2$\Hyph слов, представляющих множество $B\subset J(f,X)$}%
   {subset of words of representation}%
\Symb%
   {суперпозиция координат эндоморфизма представления $f$ и точки $m$}%
   {superposition of coordinates, representation}%
\Symb%
   {суперпозиция координат эндоморфизма башни представлений $\Vector f$ и элемента $\VX a$}%
   {superposition of coordinates, tower of representations}%
\Symb%
   {$\Omega_2$\Hyph слово, представляющее элемент $m\in J(f,X)$}%
   {word of element relative to generating set, representation}%
\Symb%
   {множество $\Omega_2$\Hyph слов представления $J(f,X)$}%
   {word set of representation}%
\Symb%
   {множество кортежей $\VX{\Omega}$\Hyph слов башни представлений $\Vector J(\Vector f,\VX X)$}%
   {word set of tower of representations}%
\Symb%
   {кортеж слов элемента $\Vector a$ относительно кортежа множеств $\VX X$}%
   {words of element, tower of representations}%

\SetIndexSpace%X%0
\Symb%
   {кватернион, сопряженный к кватерниону $x$}%
   {conjugate of quaternion}%
\Symb%
   {локальный базис аффинного пространства}%
   {local basis of affine space}%
\Symb%
   {неголономная координата}%
   {x(k)}%

\SetIndexSpace%Z%0
\Symb%
   {центр $D$\Hyph алгебры $A$}%
   {center of algebra}%
\Symb%
   {центр кольца $D$}%
   {center of ring}%

\SetIndexSpace%Delta%1
\Symb%
   {отклонение траекторий}%
   {deviation of trajectories}%
\Symb%
   {тождественное преобразование}%
   {identical transformation}%
\Symb%
   {образ вектора $\Vector e_k\in\Basis e$ при изоморфизме в координатное векторное пространство}%
   {image of vector e_k, coordinate vector space}%
\Symb%
   {символ Кронекерa}%
   {Kronecker symbol}%

\SetIndexSpace%Gamma%1
\Symb%
   {неголономные координаты связности}%
   {anholonomic coordinates of connection}%
\Symb%
   {символ Картана}%
   {Cartan symbol}%
\Symb%
   {связность}%
   {conection overline}%
\Symb%
   {коэффициенты связности в $D$\Hyph аффинном пространстве}%
   {connection coefficients, D affine space}%
\Symb%
   {связность в $D$\Hyph аффинном пространстве}%
   {connection, affine manifold}%
\Symb%
   {коэффициенты $D$\Hyph аффинной связности на многообразии}%
   {D affine connection coefficients, manifold}%
\Symb%
   {голономные координаты связности}%
   {holonomic coordinates of connection}%
\Symb%
   {связность Картана}%
   {overbrace Gamma i kl}%
\Symb%
   {множество сечений расслоения}%
   {set of sections of bundle}%

\SetIndexSpace%Lambda%1
\Symb%
   {обратный оператор оператора $\psi_l$}%
   {inverse operator to operator psi l}%
\Symb%
   {обратный оператор оператора $\psi_r$}%
   {inverse operator to operator psi r}%

\SetIndexSpace%O%1
\Symb%
   {норма операции}%
   {norm of operation}%

\SetIndexSpace%Omega%1
\Symb%
   {объект неголономности}%
   {anholonomity object}%

\SetIndexSpace%Psi%1
\Symb%
   {левый базовый оператор группы Ли над алгеброй $A$}%
   {L basic operator of Lie group over algebra A}%
\Symb%
   {левый базовый оператор группы Ли}%
   {Lie Basic Operator L}%
\Symb%
   {левый базовый оператор однопараметрической группы Ли}%
   {Lie Basic Operator L, 1-Parameter Group}%
\Symb%
   {левый базовый оператор однопараметрической группы Ли над алгеброй $A$}%
   {Lie Basic Operator L, 1-Parameter Group, algebra}%
\Symb%
   {правый базовый оператор группы Ли}%
   {Lie Basic Operator R}%
\Symb%
   {правый базовый оператор однопараметрической группы Ли}%
   {Lie Basic Operator R, 1-Parameter Group}%
\Symb%
   {правый базовый оператор однопараметрической группы Ли над алгеброй $A$}%
   {Lie Basic Operator R, 1-Parameter Group, algebra}%
\Symb%
   {правый базовый оператор группы Ли над алгеброй $A$}%
   {R basic operator of Lie group over algebra A}%

\SetIndexSpace%Fi%2
\Symb%
   {операция на группе Ли}%
   {Lie group composition law}%

\SetIndexSpace%Nabla%2
\Symb%
   {производная Картана}%
   {overbrace nabla_l}%
\Symb%
   {производная}%
   {overline nabla_l, definition 1}%

\SetIndexSpace%Phi%2
\Symb%
   {сужение соответсвия $\Phi$ на множество $C$}%
   {restriction of correspondence}%

\SetIndexSpace%Pi%2
\Symb%
   {декартово произведение расслоений}%
   {Cartesian product of bundles, definition 2}%
\Symb%
   {декартово произведение расслоенных пространств}%
   {Cartesian product of total spaces, definition 2}%
\Symb%
   {прямое произведение тел $D_i$, $i\in I$}%
   {direct product of division rings}%
\Symb%
   {прямое произведение тел $D_1$, ..., $D_n$}%
   {direct product of division rings, i 1 n}%
\Symb%
   {прямое произведение $\RCstar D_i$\hyph векторных пространств $\Vector V_i$, $i\in I$}%
   {direct product, rcd vector space}%
\Symb%
   {прямое произведение $\RCstar D_i$\hyph векторных пространств $\Vector V_1$, ..., $\Vector V_n$}%
   {direct product, rcd vector space, i 1 n}%
\Symb%
   {произведение групп $G_i$, $i\in I$}%
   {product of groups}%
\Symb%
   {произведение групп $G_1$, ..., $G_n$}%
   {product of groups, i 1 n}%
\Symb%
   {произведением объектов $\{B_i,i\in I\}$ в категории $\mathcal A$}%
   {product of objects in category}%
\Symb%
   {произведением объектов $B_1$, ..., $B_n$ в категории $\mathcal A$}%
   {product of objects in category, i 1 n}%
\Symb%
   {приведенное декартово произведением расслоений}%
   {reduced Cartesian product of bundles, definition 2}%
\Symb%
   {приведенное декартово произведение расслоенных пространств}%
   {reduced Cartesian product of total spaces, definition 2}%

\SetIndexSpace%S%2
\Symb%
   {расслоенное подмножество}%
   {fibered subset}%
\Symb%
   {подрасслоение}%
   {subbundle}%

\CloseIndex


==> Vector.Linear.Map.English.tex <==
%auto-ignore
\ifx\PrintBook\undefined
\else
\chapter{Linear Map of \texorpdfstring{$D$}{D}\hyph Vector Spaces}
\label{chapter: Linear map, D Vector Space}
\fi

\input{Vector.Linear.Map.Eq}

\section{Linear Map of
\texorpdfstring{$D$}{D}\hyph Vector Spaces}

Considering linear map of $D$\hyph vector spaces
we assume that division ring $D$ is finite dimensional algebra over field $F$.

\begin{definition}
\label{definition: linear map, vector space}
Let field $F$ be subring of center $Z(D)$ of division ring $D$.
Suppose $V$ and
$W$ are $D$\Hyph vector spaces.
We call map
\ShowEq{map A from V to W, vector space}
of $D$\Hyph vector space $V$
into $D$\Hyph vector space $W$
\AddIndex{linear map}{linear map}
if
\ShowEq{linear map, vector space}
Let us denote
\ShowEq{set linear maps, D vector space}
set of linear maps
\ShowEq{map A from V to W, vector space}
of $D$\Hyph vector space $V$
into $D$\Hyph vector space $W$.
\qed
\end{definition}

It is evident that linear map of \drc vector space as well
linear map of \crd vector space are linear maps.
Set of morphisms of $D$\Hyph vector space
is wider then set of morphisms of \drc vector space.
To consider linear map of vector space,
we will follow method used in section
\xRef{0701.238}{section: Linear Map of Vector Spaces}.

\begin{theorem}
\label{theorem: partial linear map of variable}
Let $D$ be division ring of characteristic $0$.
Let $V$, $W$ be  $D$\Hyph vector spaces.
Linear map
\ShowEq{map A from V to W, vector space}
relative to basis \eV V
of \rcd vector space $V$ and
basis \eV W
of \rcd vector space $W$
has form
\ShowEq{linear map in vector space}
where
\ShowEq{Aij(vi)}
linearly depends on
one variable $v^{\gii}$ and does not depends on the rest of
coordinates of vector $v$.
\end{theorem}
\begin{proof}
According to definition \ref{definition: linear map, vector space}
\ShowEq{vector expansion, linear map, D vector space, 1}
For any given $\gii$ vector
\ShowEq{vector expansion, linear map, D vector space, 2}
has only expansion
\ShowEq{vector expansion, linear map, D vector space, 3}
relative to basis \eV W of \rcd vector space.
Let us substitute \EqRef{vector expansion, linear map, D vector space, 3}
into \EqRef{vector expansion, linear map, D vector space, 1}.
We get \EqRef{linear map in vector space}.
\end{proof}

\begin{definition}
\label{definition: partial linear map of variable}
The linear map
\ShowEq{partial linear map of variable}
is called
\AddIndex{partial linear map}{partial linear map}
of variable $v^{\gii}$.
\qed
\end{definition}

We can write linear map as product of matrices
\ShowEq{linear map as product of matrices, 1}
Let us define product of matrices
\ShowEq{linear map as product of matrices, 2}
where $A=\left(A_{\gii}^{\gij}\right)$ is matrix of partial linear maps.
Using the equation
\EqRef{linear map as product of matrices, 2},
we can write the equation
\EqRef{linear map as product of matrices, 1}
in the form
\ShowEq{linear map as product of matrices, 3}

\begin{theorem}
\label{theorem: linear map, D vector space}
Let $D$ be division ring of characteristic $0$.
Linear map
\ShowEq{vector expansion, linear map, D vector space}
relative to basis \eV V
of $D$\Hyph vector space $V$ and
basis \eV W
of $D$\Hyph vector space $W$\footnote{Coordinate representation
of map \EqRef{vector expansion, linear map, D vector space}
depends on choice of basis. Equations change form if, for instance,
we choose \crd basis $\Basis r_*$ in $D$\Hyph vector space $W$.}
has form
\ShowEq{linear map, D vector space, canonical morphism}
\end{theorem}
\begin{proof}
According to theorem \ref{theorem: partial linear map of variable}
we can write linear map $A(v)$ as
\EqRef{linear map in vector space}.
Because for given indexes $\gii$, $\gij$
partial linear map
\ShowEq{Aij(vi)}
is linear with respect to variable $v^{\gii}$,
then according to \EqRef{linear map, division ring, canonical morphism}
it is possible to represent expression
\ShowEq{Aij(vi)}
as
\ShowEq{vector expansion, linear map, D vector space, 2a}
where index $s$ is numbering items.
Range of index $s$ depends on indexes $\gii$ and $\gij$.
Combining equations
\EqRef{vector expansion, linear map, D vector space, 1} and
\EqRef{vector expansion, linear map, D vector space, 2a},
we get
\ShowEq{linear map, D vector space, canonical morphism 1}
In equation
\EqRef{linear map, D vector space, canonical morphism 1},
we also summarize on the index $\gii$.
Equation \EqRef{linear map, D vector space, canonical morphism}
follows from comparison of equations
\EqRef{vector expansion, D vector space W} and
\EqRef{linear map, D vector space, canonical morphism 1}.
\end{proof}

\begin{definition}
\begin{sloppypar}
Expression
\ShowEq{component of linear map, D vector space}
in equation \EqRef{vector expansion, linear map, D vector space, 3}
is called
\AddIndex{component of linear map}{component of linear map} $A$.
\qed
\end{sloppypar}
\end{definition}

\begin{theorem}
\label{theorem: product of linear maps, D vector space}
Let $D$ be division ring of characteristic $0$.
Let \eV V be a basis of $D$\Hyph vector space $V$,
\eV U be a basis of $D$\Hyph vector space $U$,
and \eV W be a basis of $D$\Hyph vector space $W$.
Suppose diagram of maps
\[
\xymatrix{
V\ar[rr]^{C}\ar[dr]^{A} & & W\\
&U\ar[ur]^{B} &
}
\]
is commutative diagram
where linear map $A$ has presentation
\ShowEq{product of linear maps, D vector spaces, A}
relative to selected bases
and linear map $B$ has presentation
\ShowEq{product of linear maps, D vector spaces, B}
relative to selected bases.
Then map $C$ is linear map and has presentation
\ShowEq{product of linear maps, D vector spaces, C}
relative to selected bases, where\footnote{Index
$u$ appeared composite index, $u=st$.
However it is possible that some items in
\EqRef{product of linear maps, D vector spaces}
may be summed together.}
\ShowEq{product of linear maps, D vector spaces}
\end{theorem}
\begin{proof}
The map $C$ is linear map because
\ShowEq{product of linear maps, D vector spaces, 1}
Equation
\EqRef{product of linear maps, D vector spaces, C}
follows from substituting
\EqRef{product of linear maps, D vector spaces, A}
into \EqRef{product of linear maps, D vector spaces, B}.
\end{proof}

\begin{theorem}
For linear map $A$ there exists
linear map $B$ such, that
\ShowEq{components of two linear maps, D vector space}
\end{theorem}
\begin{proof}
The map $B$ is linear map because
\ShowEq{components of two linear maps, 1, D vector space}
According to equation \EqRef{linear map, D vector space, canonical morphism}
\ShowEq{components of two linear maps, 2, D vector space}
\end{proof}

\begin{theorem}
\label{theorem: linear map, 0, D vector space}
Let $D$ be division ring  of characteristic $0$.
Let
\ShowEq{map A from V to W, vector space}
linear map
of $D$\Hyph vector space $V$
into $D$\Hyph vector space $W$.
Then
\ShowEq{A(0)=0}
\end{theorem}
\begin{proof}
Corollary of equation
\ShowEq{A(0)=0 1}
\end{proof}

\begin{definition}
The set
\ShowEq{kernel of linear map, D vector space}
is called
\AddIndex{kernel of linear map}{kernel of linear map}
\ShowEq{map A from V to W, vector space}
of $D$\Hyph vector space $V$
into $D$\Hyph vector space $W$.
\qed
\end{definition}

\begin{definition}
The linear map
\ShowEq{map A from V to W, vector space}
of $D$\Hyph vector space $V$
into $D$\Hyph vector space $W$
is called
\AddIndex{singular}{singular linear map},
if
\[\text{ker}A=V\]
\qed
\end{definition}

\section{Polylinear Map
of \texorpdfstring{$D$}{D}\hyph Vector Spaces}

\begin{definition}
Let field $F$ be subring of center $Z(D)$ of division ring $D$
of characteristic $0$.
Suppose $V_1$, ..., $V_n$,
$W_1$, ..., $W_m$
are $D$\Hyph vector spaces.
We call map
\ShowEq{polylinear map of D vector spaces}
\AddIndex{polylinear map}{polylinear map}
of $\times$\hyph $D$\hyph vector space
$V_1\times...\times V_n$
into $\times$\hyph $D$\hyph vector space
$W_1\times...\times W_m$,
if
\ShowEq{polylinear map of D vector spaces, 1}
\qed
\end{definition}

\begin{definition}
Let us denote
\ShowEq{set polylinear maps, D vector space}
set of polylinear maps
of $\times$\hyph $D$\hyph vector space
$V_1\times...\times V_n$
into $\times$\hyph $D$\hyph vector space
$W_1\times...\times W_m$.
\qed
\end{definition}

\begin{theorem}
\label{theorem: polylinear map, D vector space}
Let $D$ be division ring of characteristic $0$.
For each $k\in K=[1,n]$ let \eV{V_k}
be basis in $D$\Hyph vector space $V_k$ and
\ShowEq{polylinear map 1, D vector space}
For each $l$, $1\le l\le m$, let \eV{W_l}
be basis in $D$\Hyph vector space $W_l$ and
\ShowEq{polylinear map 2, D vector space}
Polylinear map
\EqRef{polylinear map of D vector spaces}
relative to bases \eV{V_1}, ..., \eV{V_n},
\eV{W_1}, ..., \eV{W_m}
has form
\ShowEq{polylinear map, D vector space, canonical morphism}
Range $S$ of index $s$ depends on values of indexes
$\gii_1$, ..., $\gii_n$.
$\sigma_s$ is a transposition of set of variables
$\{v^{\gii_1}_1,...,v^{\gii_n}_n\}$.
\end{theorem}
\begin{proof}
Since we may consider map $A$
into $\times$\hyph $D$\hyph vector space
$W_1\times...\times W_m$
componentwise,
then we may confine to considering of map
\ShowEq{polylinear map of D vector spaces, j}

We prove statement by induction on $n$.

When $n=1$ the statement of theorem is statement of theorem
\ref{theorem: linear map, D vector space}.
In such case we may identify\footnote{In representation
\EqRef{polylinear map, D vector space, canonical morphism}
we will use following rules.
\begin{itemize}
\item If range of any index is set
consisting of one element, then we will omit corresponding
index.
\item If $n=1$, then $\sigma_s$ is identical transformation.
We will not show such transformation in the expression.
\end{itemize}}
\ShowEq{polylinear map, D vector space, canonical morphism 1}

Let statement of theorem be true for $n=k-1$.
Then it is possible to represent map
\EqRef{polylinear map of D vector spaces, j}
as
\ShowEq{polylinear map of D vector spaces, j 1}
According to statement of induction polylinear map
$B_l$ has form
\ShowEq{polylinear map, D vector space, canonical morphism 2}
According to construction $B_l=C_l(v_k)$.
Therefore, expressions
\ShowEq{polylinear map, D vector space, canonical morphism 3}
are functions of $v_k$.
Since $C_l(v_k)$ is linear map of $v_k$,
then only one expression
\ShowEq{polylinear map, D vector space, canonical morphism 3}
is linear map $v_k$, and rest expressions
\ShowEq{polylinear map, D vector space, canonical morphism 4}
do not depend on $v_k$.

Without loss of generality, assume $p=0$.
According to theorem
\ref{theorem: linear map, D vector space}
\ShowEq{polylinear map, D vector space, canonical morphism 5}
Assume $s=tr$. Let us define transposition $\sigma_s$ according to rule
\ShowEq{polylinear map, D vector space, canonical morphism sigma}
Suppose
\ShowEq{polylinear map, D vector space, canonical morphism 6}
We proved step of induction.
\end{proof}

\begin{definition}
\begin{sloppypar}
Expression
\ShowEq{component of polylinear map, D vector space}
in equation \EqRef{polylinear map, D vector space, canonical morphism}
is called
\AddIndex{component of polylinear map}
{component of polylinear map} $A$.
\qed
\end{sloppypar}
\end{definition}


==> Vector.Linear.Map.Eq.tex <==
%auto-ignore

\newcommand\eV[1]{$\Basis e_{#1}$}
\newcommand\EV[2]{e_{#1\cdot\gi{#2}}}
\def\vW{e_W}
\def\AA{A_{s\cdot 0\cdot}^{}{}_{\gii}^{\gij}}
\def\AB{A_{s\cdot 1\cdot}^{}{}_{\gii}^{\gij}}
\def\BA{B_{t\cdot 0\cdot}^{}{}_{\gij}^{\gik}}
\def\BB{B_{t\cdot 1\cdot}^{}{}_{\gij}^{\gik}}
\newcommand\CU[2]{C_{#1\cdot #2\cdot}^{}{}_{\gii}^{\gik}}

\DefEq
{
$A_{\gii}^{\gij}(v^{\gii})$
}
{Aij(vi)}

\DefEquation
{
A(v)=
\begin{pmatrix}
\EV W1&...&\EV Wm
\end{pmatrix}
\RCstar 
\begin{pmatrix}
A_{\gii}^{\giA}(v^{\gii})\\...\\A_{\gii}^{\gim}(v^{\gii})
\end{pmatrix}
}
{linear map as product of matrices, 1}

\DefEquation
{
u=A(v)
=\EV UjA_{\gii}^{\gij}(v^{\gii})
=\EV Uj\AA\ v^{\gii}\ \AB
}
{product of linear maps, D vector spaces, A}

\DefEquation
{
\begin{array}{lll}
&C_{\gii}^{\gik}(v^{\gii})
&=B_{\gij}^{\gik}(A_{\gii}^{\gij}(v^{\gii}))
\\
\CU u0
&=\CU {ts}0
&=\BA
\ \AA
\\
\CU u1
&=\CU {ts}1
&=\AB
\ \BB
\end{array}
}
{product of linear maps, D vector spaces}

\DefEquation
{
w=C(v)
=\EV WkC_{\gii}^{\gik}(v^{\gii})
=\EV Wk\CU u0\ v^{\gii}\ \CU u1
}
{product of linear maps, D vector spaces, C}

\DefEquation
{
w=B(u)
=\EV WkB_{\gij}^{\gik}(u^{\gij})
=\EV Wk\BA\ u^{\gij}\ \BB
}
{product of linear maps, D vector spaces, B}

\DefEq
{
\symb{\mathcal L(D;V;W)}1{set linear maps, vector}
}
{set linear maps, D vector space}

\DefEq
{
\[
\begin{array}{r@{\ }lr}
A(x+ y)
&=A(x)+ A(y)
&x, y \in V
\\
A(px)&=pA(x)
&p\in F
\end{array}
\]
}
{linear map, vector space}

\DefEquation
{
\begin{pmatrix}
A_{\giA}^{\giA}&...&A_{\gin}^{\giA}
\\...&...&...\\
A_{\giA}^{\gim}&...&A_{\gin}^{\gim}
\end{pmatrix}
\RCcirc
\begin{pmatrix}
v^{\giA}\\...\\v^{\gin}
\end{pmatrix}
=
\begin{pmatrix}
A_{\gii}^{\giA}(v^{\gii})\\...\\A_{\gii}^{\gim}(v^{\gii})
\end{pmatrix}
}
{linear map as product of matrices, 2}

\DefEquation
{
A(v)=
\begin{pmatrix}
\EV W1&...&\EV Wm
\end{pmatrix}
\RCstar
\begin{pmatrix}
A_{\giA}^{\giA}&...&A_{\gin}^{\giA}
\\...&...&...\\
A_{\giA}^{\gim}&...&A_{\gin}^{\gim}
\end{pmatrix}
\RCcirc
\begin{pmatrix}
v^{\giA}\\...\\v^{\gin}
\end{pmatrix}
}
{linear map as product of matrices, 3}

\DefEquation
{
A_{\gii}^{\gij}(v^{\gii})
=\AA\ v^{\gii}\ \AB
}
{vector expansion, linear map, D vector space, 2a}

\DefEq
{
\symb{A_{s\cdot p\cdot}^{}{}_{\gii}^{\gij}}1
{component of linear map, vector}
}
{component of linear map, D vector space}

\DefEquation
{
\begin{array}{l@{\ }l@{\ }l}
A(v)
&=\EV WjA_{\gii}^{\gij}(v^{\gii})\ 
&=\EV Wj\AA\ v^{\gii}\ \AB
\\
A(v)
&=\vW\RCstar A_{\gii}(v^{\gii})
&=\vW\RCstar(A_{s\cdot 0\cdot {\gii}}\ v^{\gii}\ A_{s\cdot 1\cdot {\gii}})
\end{array}
}
{linear map, D vector space, canonical morphism 1}

\DefEq
{
\begin{align}
v&=e_V\RCstar v
\nonumber
\\
\EqLabel{vector expansion, D vector space W}
w&=\vW\RCstar w
\\
\EqLabel{linear map, D vector space, canonical morphism}
w^{\gij}&=A_{\gii}^{\gij}(v^{\gii})
=\AA\ v^{\gii}\ \AB
\end{align}
}
{linear map, D vector space, canonical morphism}

\DefEquation
{
\begin{matrix}
A:v\in V\rightarrow w\in W
&w=A(v)
\end{matrix}
}
{vector expansion, linear map, D vector space}

\DefEq
{
\[A:V\rightarrow W\]
}
{map A from V to W, vector space}

\DefEq
{
$A(0)=0$.
}
{A(0)=0}

\DefEq
{
\[
A(a+0)
=A(a)+A(0)
\]
}
{A(0)=0 1}

\DefEq
{
\begin{align*}
A(
p_1, ...,
p_i+ q_i, ...,
p_n)
&=
A(
p_1, ...,
p_i, ...,
p_n)
+
A(
p_1, ...,
q_i, ...,
p_n)
\\
A(
p_1, ...,
ap_i, ...,
p_n)
&=
aA(
p_1, ...,
p_i, ...,
p_n)
\\
&\begin{matrix}
1\le i\le n
&p_i, q_i \in V_i
&a\in F
\end{matrix}
\end{align*}
}
{polylinear map of D vector spaces, 1}

\DefEq
{
\[
\begin{matrix}
v_k=v_k\CRstar e_{V_k} 
&
v_k\in V_k
\end{matrix}
\]
}
{polylinear map 1, D vector space}

\DefEq
{
\[
\begin{matrix}
w_l=w_l\CRstar e_{W_l} 
&
w_l\in W_l
\end{matrix}
\]
}
{polylinear map 2, D vector space}

\DefEq
{
\symb{\mathcal L(D;V_1,...,V_n;
W_1, ..., W_m)}1{set polylinear maps, D vector space}
}
{set polylinear maps, D vector space}

\DefEquation
{
\begin{matrix}
A:V_1\times...\times V_n\rightarrow
W_1\times...\times W_m
\\
w_1\times...\times w_m=A(v_1,...,v_n)
\end{matrix}
}
{polylinear map of D vector spaces}

\DefEq
{
\[
\begin{matrix}
A^1_{s\cdot p\cdot}{}_{\gii}^{\gij}=A_{s\cdot p\cdot}{}_{\gii}^{\gij}
&p=0, 1
\end{matrix}
\]
}
{polylinear map, D vector space, canonical morphism 1}

\DefEq
{
\[
w^{\gij}_l=
B_{t\cdot 0\cdot l\cdot}^{k-1}{}_{\gii_1...\gii_{k-1}}^{\gij}
\ \sigma_t(v^{\gii_1}_1)
\ B_{t\cdot 1.l\cdot}^{k-1}{}_{\gii_1...\gii_{k-1}}^{\gij}\ ...
\ \sigma_t(v^{\gii_{k-1}}_{k-1})
\ B_{t\cdot k-1.l\cdot}^{k-1}{}_{\gii_1...\gii_{k-1}}^{\gij}
\]
}
{polylinear map, D vector space, canonical morphism 2}

\DefEq
{
$B_{t\cdot p\cdot l\cdot}^{k-1}{}_{\gii_1...\gii_{k-1}}^{\gij}$
}
{polylinear map, D vector space, canonical morphism 3}

\DefEquation
{
\begin{array}{r@{\ }l}
w_l^{\gij}
&=A_{l\cdot}^{}{}_{\gii_1...\gii_n}^{\gij}(v^{\gii_1}_1,...,v^{\gii_n}_n)
\\
&=A_{s\cdot 0\cdot l\cdot}^n{}_{\gii_1...\gii_n}^{\gij}
\ \sigma_s(v^{i_1}_1)
\ A_{s\cdot 1.l\cdot}^n{}_{\gii_1...\gii_n}^{\gij}
\ ...
\ \sigma_s(v^{i_n}_n)
\ A_{s\cdot n\cdot l\cdot}^n{}_{\gii_1...\gii_n}^{\gij}
\end{array}
}
{polylinear map, D vector space, canonical morphism}

\DefEq
{
\[
\sigma_s=\sigma(tr)=
\left(
\begin{array}{cccc}
v^{\gii_k}_k&v^{\gii_1}_1&...&v^{\gii_{k-1}}_{k-1}
\\
v^{\gii_k}_k&\sigma_t(v^{\gii_1}_1)&...&\sigma_t(v^{\gii_{k-1}}_{k-1})
\end{array}
\right)
\]
}
{polylinear map, D vector space, canonical morphism sigma}

\DefEquation
{
\begin{matrix}
A_l:V_1\times...\times V_n\rightarrow W_l
&w_l=A_l(v_1,...,v_n)
\end{matrix}
}
{polylinear map of D vector spaces, j}

\DefEq
{
\[
\xymatrix{
V_1\times...\times V_k\ar[rr]^{A_l}\ar@{=>}[drr]_{C_l(v_k)}
& & W_l
\\
& &
\\
&&V_1\times...\times V_{k-1}\ar[uu]_{B_l} &
}
\]
\[
w_l=A_l(v_1,...,v_k)=C_l(v_k)(v_1,...,v_{k-1})
\]
}
{polylinear map of D vector spaces, j 1}

\DefEq
{
\symb{A_{s\cdot p\cdot l\cdot}^n{}_{\gii_1...\gii_n}^{\gij}}1
{component of polylinear map, vector}
}
{component of polylinear map, D vector space}

\DefEq
{
$B_{t\cdot q\cdot l\cdot}^{k-1}{}_{\gii_1...\gii_{k-1}}^{\gij}$
}
{polylinear map, D vector space, canonical morphism 4}

\DefEq
{
\[
B_{t\cdot 0\cdot l\cdot}^{k-1}{}_{\gii_1...\gii_{k-1}}^{\gij}
=\ C_{tr\cdot 0\cdot l\cdot}^k{}_{\gii_k\gii_1...\gii_{k-1}}^{\gij}
\ v^{\gii_k}_k\ C_{tr\cdot 1.l\cdot}^k{}_{\gii_k\gii_1...\gii_{k-1}}^{\gij}
\]
}
{polylinear map, D vector space, canonical morphism 5}

\DefEq
{
\[
\begin{array}{r@{\ }ll}
A_{tr\cdot q+1.l\cdot}^k{}_{\gii_k\gii_1...\gii_{k-1}}^{\gij}
&=B_{t\cdot q\cdot l\cdot}^{k-1}{}_{\gii_1...\gii_{k-1}}^{\gij}
&q=1, ..., k-1
\\
A_{tr\cdot q\cdot l\cdot}^k{}_{\gii_k\gii_1...\gii_{k-1}}^{\gij}
&=C_{tr\cdot q\cdot l\cdot}^k{}_{\gii_k\gii_1...\gii_{k-1}}^{\gij}
&q=0,1
\end{array}
\]
}
{polylinear map, D vector space, canonical morphism 6}


\DefEquation
{
\begin{matrix}
A(v)=\EV Wj\ A_{\gii}^{\gij}(v^{\gii})\ 
&v=e_V\RCstar v
\end{matrix}
}
{linear map in vector space}

\DefEq
{
$A(\EV Vi\ v^{\gii})\in W$
}
{vector expansion, linear map, D vector space, 2}

\DefEquation
{
\begin{array}{lll}
A(\EV Vi\ v^{\gii})=
\EV Wj\ A_{\gii}^{\gij}(v^{\gii})\ 
&&
A(\EV Vi\ v^{\gii})=
\vW\RCstar A_{\gii}(v^{\gii})
\end{array}
}
{vector expansion, linear map, D vector space, 3}

\DefEq
{
\symb{A_{\gii}^{\gij}}0{partial linear map}
\[
\ShowSymbol{partial linear map}:D\rightarrow D
\]
}
{partial linear map of variable}

\DefEquation
{
A(v)=A(e_V\RCstar v)
=A\left(\sum_{\gii}\EV Vi\ v^{\gii}\right)
=\sum_{\gii} A(\EV Vi\ v^{\gii})
}
{vector expansion, linear map, D vector space, 1}

\DefEq
{
\begin{align*}
C(a+b)&=B(A(a+b))
\\
&=B(A(a)+A(b))
\\
&=B(A(a))+B(A(b))
\\
&=C(a)+C(b)
\\
C(ab)&=B(A(ab))
=B(aA(b))
\\
&=aB(A(b))
=aC(b)
\\
&a,b\in V
\\
&a\in F
\end{align*}
}
{product of linear maps, D vector spaces, 1}

\DefEq
{
\begin{align*}
A(axb)&=B(x)
\\
B_{s\cdot 0\cdot}{}_{\gii}^{\gij}&=\AA\ a
\\
B_{s\cdot 1\cdot}{}_{\gii}^{\gij}&=b\ \AB
\end{align*}
}
{components of two linear maps, D vector space}

\DefEq
{
\begin{align*}
B(x+y)
&=A(a(x+y)b)
=A(axb+ayb)
=A(axb)+A(ayb)
=B(x)+B(y)
\\
B(cx)&=A(acxb)
=A(caxb)
=cA(axb)
=cB(x)
\\
&x,y\in V,c\in F
\end{align*}
}
{components of two linear maps, 1, D vector space}

\DefEq
{
\symb{\text{ker}\,f}
0{kernel of linear map}
\[
\ShowSymbol{kernel of linear map}
=\{x\in V:f(x)=0\}
\]
}
{kernel of linear map, D vector space}

\DefEq
{
\[
B_{s\cdot 0\cdot}^{}{}_{\gii}^{\gij}\ v^{\gii}\ B_{s\cdot 1\cdot}^{}{}_{\gii}^{\gij}
=\AA\ (a\ v^{\gii}\ b) \AB
=(\AA\ a) v^{\gii}\ (b\ \AB)
\]
}
{components of two linear maps, 2, D vector space}


==> Vector.Linear.Map.Russian.tex <==
%auto-ignore
\ifx\PrintBook\undefined
\else
\chapter{Линейное отображение \texorpdfstring{$D$}{D}\hyph векторных пространств}
\label{chapter: Linear map, D Vector Space}
\fi

\input{Vector.Linear.Map.Eq}

\section{Линейное отображение
\texorpdfstring{$D$}{D}\hyph векторных пространств}

При изучении линейного отображения $D$\hyph векторных пространств
мы будем рассматривать тело $D$ как конечно мерную алгебру над полем $F$.

\begin{definition}
\label{definition: linear map, vector space}
Пусть поле $F$ является подкольцом центра $Z(D)$ тела $D$.
Пусть $V$ и
$W$ - $D$\Hyph векторные пространства.
Мы будем называть отображение
\ShowEq{map A from V to W, vector space}
$D$\Hyph векторного пространства $V$
в $D$\Hyph векторное пространство $W$
\AddIndex{линейным отображением}{linear map},
если
\ShowEq{linear map, vector space}
Обозначим
\ShowEq{set linear maps, D vector space}
множество линейных отображений
\ShowEq{map A from V to W, vector space}
$D$\Hyph векторного пространства $V$
в $D$\Hyph векторное пространство $W$.
\qed
\end{definition}

Очевидно, что линейное отображение \drc векторного пространства, так же как
линейное отображение \crd векторного пространства являются линейными отображениями.
Множество морфизмов $D$\Hyph векторного пространства
шире, чем множество морфизмов \drc векторного пространства.
Чтобы рассмотреть линейное отображение векторных пространств,
мы будем следовать методике, предложенной в разделе
\xRef{0701.238}{section: Linear Map of Vector Spaces}.

\begin{theorem}
\label{theorem: partial linear map of variable}
Пусть $D$ - тело характеристики $0$.
Пусть $V$, $W$ - $D$\Hyph векторные пространства.
Линейное отображение
\ShowEq{map A from V to W, vector space}
относительно базиса \eV V
\rcd векторного пространства $V$ и
базиса \eV W
\rcd векторного пространства $W$
имеет вид
\ShowEq{linear map in vector space}
где
\ShowEq{Aij(vi)}
линейно зависит от
одной переменной $v^{\gii}$ и не зависит от остальных
координат вектора $v$.
\end{theorem}
\begin{proof}
Согласно определению \ref{definition: linear map, vector space}
\ShowEq{vector expansion, linear map, D vector space, 1}
Для любого заданного $\gii$ вектор
\ShowEq{vector expansion, linear map, D vector space, 2}
имеет единственное разложение
\ShowEq{vector expansion, linear map, D vector space, 3}
относительно базиса \eV W \rcd векторного пространства.
Подставив \EqRef{vector expansion, linear map, D vector space, 3}
в \EqRef{vector expansion, linear map, D vector space, 1},
мы получим \EqRef{linear map in vector space}.
\end{proof}

\begin{definition}
\label{definition: partial linear map of variable}
Линейное отображение
\ShowEq{partial linear map of variable}
называется
\AddIndex{частным линейным отображением}{partial linear map}
переменной $v^{\gii}$.
\qed
\end{definition}

Мы можем записать линейное отображение в виде произведения матриц
\ShowEq{linear map as product of matrices, 1}
Определим произведение матриц
\ShowEq{linear map as product of matrices, 2}
где $A=\left(A_{\gii}^{\gij}\right)$ - матрица частных линейных отображений.
Используя равенство
\EqRef{linear map as product of matrices, 2},
мы можем записать равенство
\EqRef{linear map as product of matrices, 1}
в виде
\ShowEq{linear map as product of matrices, 3}

\begin{theorem}
\label{theorem: linear map, D vector space}
Пусть $D$ - тело характеристики $0$.
Линейное отображение
\ShowEq{vector expansion, linear map, D vector space}
относительно базиса \eV V
в $D$\Hyph векторном пространстве $V$ и
базиса \eV W
в $D$\Hyph векторном пространстве $W$\footnote{Координатная запись
отображения \EqRef{vector expansion, linear map, D vector space}
зависит от выбора базиса. Равенства изменят свой вид, если например
мы выберем \crd базис $\Basis r_*$ в $D$\Hyph векторном пространстве $W$.}
имеет вид
\ShowEq{linear map, D vector space, canonical morphism}
\end{theorem}
\begin{proof}
Согласно теореме \ref{theorem: partial linear map of variable}
линейное отображение $A(v)$ можно записать в виде
\EqRef{linear map in vector space}.
Так как для заданных индексов $\gii$, $\gij$
частное линейное отображение
\ShowEq{Aij(vi)}
линейно по переменной $v^{\gii}$,
то согласно \EqRef{linear map, division ring, canonical morphism}
выражение
\ShowEq{Aij(vi)}
можно представить в виде
\ShowEq{vector expansion, linear map, D vector space, 2a}
где индекс $s$ нумерует слагаемые.
Множество значений индекса $s$ зависит от индексов $\gii$ и $\gij$.
Комбинируя равенства
\EqRef{vector expansion, linear map, D vector space, 1} и
\EqRef{vector expansion, linear map, D vector space, 2a},
мы получим
\ShowEq{linear map, D vector space, canonical morphism 1}
В равенстве
\EqRef{linear map, D vector space, canonical morphism 1}
мы суммируем также по индексу $\gii$.
Равенство \EqRef{linear map, D vector space, canonical morphism}
следует из сравнения равенств
\EqRef{vector expansion, D vector space W} и
\EqRef{linear map, D vector space, canonical morphism 1}.
\end{proof}

\begin{definition}
\begin{sloppypar}
Выражение
\ShowEq{component of linear map, D vector space}
в равенстве \EqRef{vector expansion, linear map, D vector space, 3}
называется
\AddIndex{компонентой линейного отображения}{component of linear map} $A$.
\qed
\end{sloppypar}
\end{definition}

\begin{theorem}
\label{theorem: product of linear maps, D vector space}
Пусть $D$ - тело характеристики $0$.
Пусть \eV V - базис в $D$\Hyph векторном пространстве $V$,
\eV U - базис в $D$\Hyph векторном пространстве $U$,
и \eV W - базис в $D$\Hyph векторном пространстве $W$.
Предположим, что мы имеем коммутативную диаграмму отображений
\[
\xymatrix{
V\ar[rr]^{C}\ar[dr]^{A} & & W\\
&U\ar[ur]^{B} &
}
\]
где линейное отображение $A$ имеет представление
\ShowEq{product of linear maps, D vector spaces, A}
относительно заданных базисов
и линейное отображение $B$ имеет представление
\ShowEq{product of linear maps, D vector spaces, B}
относительно заданных базисов.
Тогда отображение $C$ линейно и имеет представление
\ShowEq{product of linear maps, D vector spaces, C}
относительно заданных базисов, где\footnote{Индекс
$u$ оказался составным индексом, $u=st$.
Однако не исключено, что некоторые слагаемые в
\EqRef{product of linear maps, D vector spaces}
могут быть объединены вместе.}
\ShowEq{product of linear maps, D vector spaces}
\end{theorem}
\begin{proof}
Отображение $C$ линейно, так как
\ShowEq{product of linear maps, D vector spaces, 1}
Равенство
\EqRef{product of linear maps, D vector spaces, C}
следует из подстановки
\EqRef{product of linear maps, D vector spaces, A}
в \EqRef{product of linear maps, D vector spaces, B}.
\end{proof}

\begin{theorem}
Для линейного отображения $A$ существует
линейное отображение $B$ такое, что
\ShowEq{components of two linear maps, D vector space}
\end{theorem}
\begin{proof}
Отображение $B$ линейно, так как
\ShowEq{components of two linear maps, 1, D vector space}
Согласно равенству \EqRef{linear map, D vector space, canonical morphism}
\ShowEq{components of two linear maps, 2, D vector space}
\end{proof}

\begin{theorem}
\label{theorem: linear map, 0, D vector space}
Пусть $D$ - тело характеристики $0$.
Пусть
\ShowEq{map A from V to W, vector space}
линейное отображение
$D$\Hyph векторного пространства $V$
в $D$\Hyph векторное пространство $W$.
Тогда
\ShowEq{A(0)=0}
\end{theorem}
\begin{proof}
Следствие равенства
\ShowEq{A(0)=0 1}
\end{proof}

\begin{definition}
Множество
\ShowEq{kernel of linear map, D vector space}
называется
\AddIndex{ядром линейного отображения}{kernel of linear map}
\ShowEq{map A from V to W, vector space}
$D$\Hyph векторного пространства $V$
в $D$\Hyph векторное пространство $W$.
\qed
\end{definition}

\begin{definition}
Линейное отображение
\ShowEq{map A from V to W, vector space}
$D$\Hyph векторного пространства $V$
в $D$\Hyph векторное пространство $W$
называется
\AddIndex{вырожденным}{singular linear map},
если
\[\text{ker}A=V\]
\qed
\end{definition}

\section{Полилинейное отображение
\texorpdfstring{$D$}{D}\hyph векторного пространства}

\begin{definition}
Пусть поле $F$ является подкольцом центра $Z(D)$ тела $D$
характеристики $0$.
Пусть $V_1$, ..., $V_n$,
$W_1$, ..., $W_m$
- $D$\Hyph векторные пространства.
Мы будем называть отображение
\ShowEq{polylinear map of D vector spaces}
\AddIndex{полилинейным отображением}{polylinear map}
$\times$\hyph $D$\hyph векторного пространства
$V_1\times...\times V_n$
в $\times$\hyph $D$\hyph векторное пространство
$W_1\times...\times W_m$,
если
\ShowEq{polylinear map of D vector spaces, 1}
\qed
\end{definition}

\begin{definition}
Обозначим
\ShowEq{set polylinear maps, D vector space}
множество полилинейных отображений
$\times$\hyph $D$\hyph векторного пространства
$V_1\times...\times V_n$
в $\times$\hyph $D$\hyph векторное пространство
$W_1\times...\times W_m$.
\qed
\end{definition}

\begin{theorem}
\label{theorem: polylinear map, D vector space}
Пусть $D$ - тело характеристики $0$.
Для каждого $k\in K=[1,n]$ допустим \eV{V_k}
- базис в $D$\Hyph векторном пространстве $V_k$ и
\ShowEq{polylinear map 1, D vector space}
Для каждого $l$, $1\le l\le m$, допустим \eV{W_l}
- базис в $D$\Hyph векторном пространстве $W_l$ и
\ShowEq{polylinear map 2, D vector space}
Полилинейное отображение
\EqRef{polylinear map of D vector spaces}
относительно базисов \eV{V_1}, ..., \eV{V_n},
\eV{W_1}, ..., \eV{W_m}
имеет вид
\ShowEq{polylinear map, D vector space, canonical morphism}
Область значений $S$ индекса $s$ зависит от значений индексов
$\gii_1$, ..., $\gii_n$.
$\sigma_s$ - перестановка множества переменных
$\{v^{\gii_1}_1,...,v^{\gii_n}_n\}$.
\end{theorem}
\begin{proof}
Так как отображение $A$
в $\times$\hyph $D$\hyph векторное пространство
$W_1\times...\times W_m$
можно рассматривать покомпонентно,
то мы можем ограничиться рассмотрением отображения
\ShowEq{polylinear map of D vector spaces, j}

Мы докажем утверждение индукцией по $n$.

При $n=1$ доказываемое утверждение является утверждением теоремы
\ref{theorem: linear map, D vector space}.
При этом мы можем отождествить\footnote{В представлении
\EqRef{polylinear map, D vector space, canonical morphism}
мы будем пользоваться следующими правилами.
\begin{itemize}
\item Если область значений какого-либо индекса - это множество,
состоящее из одного элемента, мы будем опускать соответствующий
индекс.
\item Если $n=1$, то $\sigma_s$ - тождественное преобразование.
Это преобразование можно не указывать в выражении.
\end{itemize}}
\ShowEq{polylinear map, D vector space, canonical morphism 1}

Допустим, что утверждение теоремы справедливо при $n=k-1$.
Тогда отображение
\EqRef{polylinear map of D vector spaces, j}
можно представить в виде
\ShowEq{polylinear map of D vector spaces, j 1}
Согласно предположению индукции полилинейное отображение
$B_l$ имеет вид
\ShowEq{polylinear map, D vector space, canonical morphism 2}
Согласно построению $B_l=C_l(v_k)$.
Следовательно, выражения
\ShowEq{polylinear map, D vector space, canonical morphism 3}
являются функциями $v_k$.
Поскольку $C_l(v_k)$ - линейная функция $v_k$,
то только одно выражение
\ShowEq{polylinear map, D vector space, canonical morphism 3}
является линейной функцией $v_k$, и остальные выражения
\ShowEq{polylinear map, D vector space, canonical morphism 4}
не зависят от $v_k$.

Не нарушая общности, положим $p=0$.
Согласно теореме
\ref{theorem: linear map, D vector space}
\ShowEq{polylinear map, D vector space, canonical morphism 5}
Положим $s=tr$ и определим перестановку $\sigma_s$ согласно правилу
\ShowEq{polylinear map, D vector space, canonical morphism sigma}
Положим
\ShowEq{polylinear map, D vector space, canonical morphism 6}
Мы доказали шаг индукции.
\end{proof}

\begin{definition}
\begin{sloppypar}
Выражение
\ShowEq{component of polylinear map, D vector space}
в равенстве \EqRef{polylinear map, D vector space, canonical morphism}
называется \AddIndex{компонентой полилинейного отображения}
{component of polylinear map} $A$.
\qed
\end{sloppypar}
\end{definition}

